SHAPFUZZ: Efficient Fuzzing via Shapley-Guided Byte Selection

Mutation-based fuzzing is popular and effective in discovering unseen code and exposing bugs. However, only a few studies have concentrated on quantifying the importance of input bytes, which refers to the degree to which a byte contributes to the discovery of new code. They often focus on obtaining the relationship between input bytes and path constraints, ignoring the fact that not all constraint-related bytes can discover new code. In this paper, we conduct Shapely analysis to understand the effect of byte positions on fuzzing performance, and find that some byte positions contribute more than others and this property often holds across seeds. Based on this observation, we propose a novel fuzzing solution, ShapFuzz, to guide byte selection and mutation. Specifically, ShapFuzz updates Shapley values (importance) of bytes when each input is tested during fuzzing with a low overhead, and utilizes contextual multi-armed bandit to trade off between mutating high Shapley value bytes and low-frequently chosen bytes. We implement a prototype of this solution based on AFL++, i.e., ShapFuzz. We evaluate ShapFuzz against ten state-of-the-art fuzzers, including five byte schedule-reinforced fuzzers and five commonly used fuzzers. Compared with byte schedule-reinforced fuzzers, ShapFuzz discovers more edges and exposes more bugs than the best baseline on three different sets of initial seeds. Compared with commonly used fuzzers, ShapFuzz exposes 20 more bugs than the best comparison fuzzer, and discovers 6 more CVEs than the best baseline on MAGMA. Furthermore, ShapFuzz discovers 11 new bugs on the latest versions of programs, and 3 of them are confirmed by vendors.

==> obsolete/abs-1.0.tex <==
\begin{abstract}

Coverage-guided greybox fuzzing intends to enhance code coverage so that potential bugs are exposed in unseen code. 
A promising and popular solution to extend code coverage is to schedule bytes, such as grouping and mutating related bytes together. 
We conducted explainable analysis (\ie the SHAP analysis) on fuzzing, and found that the minority byte positions dominate the discovery of new code. 
Specifically, the repeated mutation of a (small) portion of bytes contributes to the most discovered code.
We further analyze that this finding can be explained by the internal logic of programs, \ie path constraints directly or indirectly influence each other.
Therefore, byte positions related to some constraints have a high chance to be related to other constraints.





Based on the finding from the explainable analysis, we propose \tool{} to optimize the mutation of the small portion of byte positions that have discovered new code (\ie the valuable positions). 
\tool{} uses a \textit{family system} to infer that the valuable positions are related to path constraints for any seed in the same family.
With the family system, \tool{} shares and combines valuable positions to boost the fuzzing of path constraints.
Since the inference may be inaccurate, \tool{} utilizes a contextual multi-armed bandit approach (CMAB) to optimize position selection, considering the execution paths (the context). 
As a result, our \tool{} prefers byte positions that are related to path constraints under the context of current execution path.
We evaluate \tool{} on two third-party testing platforms, UNIFUZZ and MAGMA.
On UNIFUZZ, in comparison to five AFL++-related fuzzers, \tool{} and \tool{}-Redqueen rank 2.62 and 1.18 on edge coverage, respectively.
% \tool{}-related fuzzers (\ie \tool{} and \tool{}-Redqueen) perform better than five AFL++-related fuzzers in terms of edge coverage. 
% \zkp{After fuzzing 24 hours, the median ranks of \tool{} and \tool{}-Redqueen are 2.62 and 1.18, respectively.}
Additionally, \tool{}-Redqueen exposes 11 more vulnerabilities than the best mode of AFL++.
On MAGMA, \tool{} and \tool{}-Redqueen expose bugs faster than the state-of-the-art fuzzers. Meanwhile, \tool{} discovers 6 more CVEs than the best of the five competing fuzzers.
% we evaluate \tool{}-related fuzzers against state-of-the-art fuzzers including AFL, AFL++, AFLFast, FairFuzz and MOPT on 20 real world programs. 
% \tool{} discovers 6 more CVEs than the best of the five competing fuzzers.



% \todo{Mutation of a small portion of byte positions can repeatedly discover new code.}
% \zkp{Mutation based fuzzing is one of the most successful and widely-used techniques to discover vulnerabilities. Existing mutation based fuzzers tend to treat each position equally during byte schedule. However, we discover that byte positions contribute differently to the discovery of code regions. Specifically, the repeated mutation of a (small) portion of byte positions contribute most of the fuzzing-discovered code.

% In this paper, we propose \tool{}, a novel fuzzer that aims to increase code coverage with explainable byte schedule. 
% \tool{} first establishes a family system to capture the valuable positions that have discovered new code from fuzzing process, and share them with other seeds in the family.
% However, a newly added seed with a completely different input format may appear.
% To increase the chances that the selected positions are useful for a seed, 
% we model the problem of selecting positions based on LinUCB, a contextual multi-armed bandit approach, which builds a probability distribution to select positions to be mutated.

% We evaluate \tool{} on two third-party testing platforms UNIFUZZ and MAGMA.
% On UNIFUZZ, \tool{}-related fuzzers (i.e., \tool{} and \tool{}-Redqueen) perform better than five existing modes of AFL++ on edge coverage. In particular, \tool{}-Redqueen exposes 11 more vulnerabilities than the best mode of AFL++.
% On MAGMA, we evaluate \tool{}-related fuzzers against state-of-the-art fuzzers including AFL, AFL++, AFLFast, FairFuzz and MOPT on 20 real world programs. 
% \tool{} discovers 6 more CVEs than the best of the five competing fuzzers.
% }
% \zhu{Example text.
% Fuzzing is known as a de facto technique to detect software security issues among both academic and industrial practitioners.
% In the set of existing fuzzing solutions, coverage-guided greybox fuzzing (CGF) has performed remarkably well in detecting real-world bugs. 
% This method aims to enhance code coverage so that potential bugs are disclosed in the unseen parts of the code. Existing studies have reported many efforts to expand code coverage, including scheduling of computational resources for certain code regions and resolving path constraints.
% In fuzzing, the problem of resolving path constraints is essentially the problem of byte schedule, including which bytes to select and how to mutate the selected bytes. 
% To analyze the contribution of each byte in discovering code, we conducted fuzzing experiments and performed SHAP (SHapley Additive exPlanations) analysis to explain the experiment results.
% Interestingly, the analysis demonstrates that 1) the mutation of the same byte positions can repeatedly discover new code coverage, and 2) the discovery of code largely depends on a (small) portion of byte positions.
% While such findings might be biased because of the program set selected in SHAP analysis, we dig deep into the reasons for the SHAP results. One reason is what we call \textit{direct coupling}, and it refers to the fact that the flip of a path constraint has to consider the results of other path constraints.
% Another reason is that different program logics may process the same format of inputs, indicating that different constraints could be related to the same positions of inputs (we call it \textit{indirect coupling}).
% }
\end{abstract}

==> obsolete/evaluation-0.1.tex <==
\section{Evaluation}
\subsection{The evaluation based on UNIFUZZ}
\subsubsection{Edge Coverage}

\begin{table}[!t]
\centering
\caption{Edge Rank.}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{\extracolsep{4pt}}lrrrrrrrrrrr@{}}
\toprule

\textbf{Time} &  \textbf{all} & \textbf{history}& \textbf{new} & \textbf{mopt} & \textbf{exploit} & \textbf{fast} & \textbf{raw} & \textbf{rare} & \textbf{compare}\\
\midrule
\textbf{1 hour} & 2.4   &   2.2  & 4.4  & 6.9   &   6.4 &  5.3  & 5.3&   7.2  &    4.4 \\
\textbf{3 hours} & 2.4   &   2.2  & 4.4  & 6.9   &   6.4 &  5.3  & 5.3&   7.2  &    4.4 \\
\textbf{6 hours} & 3.0   &   2.3  & 4.9  & 7.0   &   6.3  & 4.8  & 4.9 &  7.4   &   4.3\\
\textbf{12 hours} & 2.8  &    2.4  & 4.9 &  6.6    &  6.3  & 4.9 &  5.3  & 7.1    &  4.6\\
\textbf{24 hours} & 2.8  &    2.4  & 4.9 &  6.6    &  6.3  & 4.9 &  5.3  & 7.1    &  4.6\\

\bottomrule
\end{tabular}
}
\label{edge_rank_for_unifuzz}
\end{table}

\subsubsection{Bug Discovery}

\begin{table}[!t]
\centering
\caption{Bug Discovery.}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{\extracolsep{4pt}}lrrrrrrrrrrr@{}}
\toprule

\textbf{Program} &  \textbf{all} & \textbf{history}& \textbf{new} & \textbf{mopt} & \textbf{exploit} & \textbf{fast} & \textbf{raw} & \textbf{rare} & \textbf{compare}\\
\midrule
\textbf{tiff2pdf} & 1.0   &   1.0  & 0.0  & 1.0   &   0.0 &  0.0  & 1.0&   0.0  &    0.0 \\
\textbf{strip228} & 8.0   &   8.0  & 5.0  & 3.0   &   5.0  & 2.0  & 3.0 &  4.0   &   4.0\\
\textbf{lame} & 4.0  &    4.0  & 4.0 &  4.0    &  4.0  & 4.0 &  4.0  & 4.0    &  4.0\\
\textbf{readelf228} & 5.0  &    5.0 &  5.0 &  4.0    &  5.0  & 3.0  & 4.0  & 5.0  &    5.0\\
\textbf{nm228} & 33.0  &   32.0 & 25.0 & 22.0   &  20.0 & 21.0 & 18.0 & 30.0  &   27.0\\
\textbf{tiffsplit} & 6.0   &   6.0  & 8.0  & 5.0   &   6.0  & 5.0  & 4.0&   7.0    &  4.0\\
\textbf{tiff2bw} & 7.0   &   7.0  & 6.0 &  5.0   &   5.0  & 3.0  & 4.0  & 4.0   &   6.0\\
\textbf{objdump228} & 23.0  &   17.0 & 10.0 & 13.0   &   8.0 & 10.0  &11.0  & 6.0  &   14.0\\
\textbf{catdoc} & 3.0   &   3.0  & 3.0  & 2.0   &   2.0 &  3.0  & 3.0  & 2.0  &    3.0\\
\textbf{pdftotext} & 24.0   &  18.0 & 21.0 & 20.0   &  20.0 & 17.0 & 23.0&  20.0  &   19.0\\
\textbf{mp42aac} & 2.0  &    3.0  & 0.0  & 2.0   &   0.0  & 2.0 &  2.0  & 0.0   &   2.0\\
\textbf{tcpdump} & 2.0   &   0.0 &  0.0  & 0.0    &  0.0 &  0.0  & 1.0  & 1.0  &    1.0\\
\midrule
\textbf{Sum} & 118.0  &  104.0 & 87.0  & 81.0  &  75.0 & 70.0  & 78.0  &83.0   & 89.0 \\


\bottomrule
\end{tabular}
}
\label{unifuzz_bug}
\end{table}

\begin{figure}[htbp]
\includegraphics[width=\linewidth]{images/bug_rank.png}
\caption{Rank.}
\label{bug_rank}
\end{figure}

\subsection{The evaluation based on MAGMA}
\subsubsection{Time to find Bugs}

\begin{figure*}[htbp]
\includegraphics[width=\linewidth]{images/magma_bug.png}
\caption{Time to find Bugs.}
\label{magma_bug}
\end{figure*}

\subsection{SHAP Analysis}

\begin{table*}[!t]
\centering
\caption{The Result of SHAP Analysis. We extract the most important positions based on the data collected from 48 hours fuzzing campaigns. Top$N$\% means that the top N\% of the most important positions. $X$mins means fuzzing $X$ mins. And the value in the table represent the ratio at which the positions collected in common features after fuzzing X mins and the top N\% of the most important positions intersect. The higher the value, the better the performance. And the Baseline means that we randomly select positions into common features.}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{\extracolsep{4pt}}lrrrrrrrrrrr@{}}
\toprule

\textbf{Time} &  \textbf{Top10\%} & \textbf{Top20\%}& \textbf{Top30\%} & \textbf{Top40\%} & \textbf{Top50\%} & \textbf{Top60\%} & \textbf{Top70\%} & \textbf{Top80\%} & \textbf{Top90\%} & \textbf{Top100\%} & \textbf{Baseline}\\
\midrule
\textbf{10mins}  &0.67 &   0.59  &  0.55  &  0.52  &  0.49 &   0.46  &  0.44  &  0.42   & 0.40  &   0.38   &   0.07 \\
\textbf{20mins}  & 0.77  &  0.71  &  0.68  &  0.65   & 0.62   & 0.60  &  0.58 &   0.56  &  0.54   &  0.52    &  0.14 \\
\textbf{30mins}  & 0.81 &   0.76  &  0.73   & 0.71   & 0.68  &  0.67  &  0.64  &  0.63  &  0.61    & 0.59     & 0.17 \\
\textbf{40mins}  & 0.83  &  0.79  &  0.77  &  0.75  &  0.72  &  0.71 &   0.69  &  0.67  &  0.65  &   0.63   &   0.18 \\
\textbf{50mins}  & 0.85  &  0.81  &  0.79  &  0.78  &  0.75  &  0.73   & 0.71  &  0.69  &  0.68   &  0.66    &  0.19 \\
\textbf{60mins}  & 0.86  &  0.83   & 0.81  &  0.79  &  0.77  &  0.75   & 0.73   & 0.71  &  0.70   &  0.68   &   0.20 \\
\textbf{70mins}  & 0.87  &  0.84 &   0.82  &  0.81  &  0.78  &  0.77   & 0.75  &  0.73   & 0.72   &  0.70   &   0.20 \\
\textbf{80mins}  & 0.88  &  0.85  &  0.83  &  0.82  &  0.80  &  0.78   & 0.76  &  0.75  &  0.73  &   0.71 &     0.20 \\
\textbf{90mins}  & 0.88  &  0.86  &  0.84  &  0.83  &  0.81   & 0.79   & 0.78  &  0.76  &  0.74  &   0.73   &   0.21 \\
\textbf{100mins}  & 0.88  &  0.86  &  0.85  &  0.84  &  0.81   & 0.80   & 0.78  &  0.77 &   0.75   &  0.73    &  0.21 \\
\textbf{110mins}  & 0.89  &  0.87  &  0.85 &   0.84  &  0.82   & 0.81  &  0.79  &  0.78  &  0.76  &   0.74  &    0.21 \\
\textbf{120mins}  & 0.90  &  0.87  &  0.86 &   0.85   & 0.83  &  0.82  &  0.80 &   0.79&    0.77 &    0.75   &   0.23 \\


\bottomrule
\end{tabular}
}
\label{shap}
\end{table*}



==> obsolete/evaluation-0.2.tex <==
\section{Evaluation}
In order to evaluate \tool{}, we implement \tool{} based on AFLPlusPlus, which has integrated many fuzzing strategies. 
To reduce the influence of subjective factors on the test, we conduct our experiments on a third-party test platform.
We divided our experiments into three parts. 

\begin{itemize}
    \item \textbf{UNIFUZZ.} In the first part, we evaluate \tool{} based on UNIFUZZ, which contains a series of real-world programs and provides a standardized testing process to evaluate the performance of fuzzers on code coverage and bug discovery. We compare \tool{} with other strategies inside AFL++.
    \item \textbf{MAGMA.} In the second part, we evaluate \tool{} based on MAGMA. Unlike UNIFUZZ, MAGMA only focuses on bug discovery and has a very detailed analysis.
    \item \textbf{Further Analysis.} In the third part, we further analyze \tool{}'s performance in terms of throughput, etc., and further explore the source of \tool{}'s effect. a) we evaluate the throughput of \tool{} and perform ablation experiments to verify the efficiency of the proposed new mutation modes. b) we verify that \tool{} can discover most of the important bytes in a short time. c) We construct ablation experiments to verify that \tool{}'s improvement comes from the design of our mutation strategy.
\end{itemize}

\subsection{Experimental Setup}
\zhu{Don't leave blank between titles!}
\subsubsection{Experiment environment}
All our measurements were performed on a system running Ubuntu 18.04 with 103 cores (Intel(R) Xeon(R) Gold 6230R CPU) and 256 GiB of main memory. To make a fair comparison, each fuzzer performs single-threaded execution on one CPU core. Additionally, we repeat the experiment five times.

\subsubsection{Benchmark Fuzzers}
In our evaluation, we compare \tool{} with the state-of-the-art fuzzers, including AFL++, AFL, AFLFast, FairFuzz and MOPT.
The reasons why we chose these fuzzers are as follows.




We select 5 fuzzers to evaluate our approach. We evaluate our approach with AFL++, MOPT, AFL, AFLFast and FairFuzz.
\begin{itemize}
    \item Fioraldi et al. proposed AFL++, which is a fuzzing framework that includes many fuzzing strategies, including MOPT, Redqueen, AFLfast, etc. AFL++ has achieved outstanding results in the experiments of other papers and the evaluation of third-party test platforms such as Fuzzbench. To better integrate our strategy with other strategies, we also implement \tool{} based on AFL++. Within AFL++, we only need to adjust the parameter settings to allow \tool{} to compare fairly with other fuzzing strategies. Also, comparing within AFL++ avoids the effects of differences in implementation architectures. Finally, we use multiple different settings in AFL++ to evaluate.
    \item MOPT utilizes Particle Swarm Optimization (PSO) algorithm to optimize AFL’s mutation operator schedule based on fuzzing history information. MOPT dynamically generates the distribution for mutators to improve the fuzzing efficiency. We sets the parameter '-L'  as 5 in the evaluation.
    \item AFL, the American Fuzzy Lop, is one of the most famous fuzzers, which has discovered many bugs in real-world applications. 
    \item AFLFast is a widely-used extension of AFL, which models fuzzing process as Markov chain and prioritizes exploring those low-frequency paths to achieve better code coverage. 
    \item FairFuzz proposes a novel mutation mask creation algorithm to guide mutations to be biased towards producing inputs triggering rare branches.
\end{itemize}

\subsubsection{Initial seeds}
All fuzzers used the same initial seeds collected from UNIFUZZ, FuzzBench, Magma or public seed corpus. 
Follow the guidance of Adrian Herrera, most target programs have multiple initial seeds instead of a single initial seed.

\subsubsection{Evaluation metrics}
As the different implementations in different fuzzers, we need uniform evaluation metrics to evaluate the fuzzers’ performance. Following the guidance in Marcel Böhme, we mainly use the following two metrics. 

The first one is edge coverage which is widely used in recent research to evaluate fuzzers. Specifically, the edge coverage is only used when evaluating based on UNIFUZZ.
When we compare \tool{} with other settings in AFL++, we do not need to leverage other tools to collect the edge coverage because we have the same low-level implementation. Thus, we use the internal tool used in AFL++ to calculate the edge coverage. When we use the edge coverage, we only compare \tool{} with the other fuzzing strategies in AFL++.

The second one is the number of unique vulnerabilities, which directly indicates the performance of fuzzer. More specifically, We use ASan to de-duplicate vulnerabilities and analyze the number of unique vulnerabilities discovered by a fuzzer in each trial. Specifically, We use the top three function calls in the output report generated by ASAN to de-duplicate vulnerabilities. 

\subsection{The evaluation based on UNIFUZZ}
UNIFUZZ is an open-source, holistic, and pragmatic metrics-driven platform to evaluate fuzzers fairly. UNIFUZZ provides 20 real-world benchmark programs with multiple initial seeds. As shown in Table X, We evaluate our \tool{} on X open-source programs selected from UNIFUZZ and X widely used programs selected from other fuzzing papers as shown in Table \ref{programsUNIFUZZ}.

\begin{table}[!t]
% \renewcommand\arraystretch{1}
\centering
\caption{Target programs.}\label{programsUNIFUZZ}
\resizebox{\linewidth}{!}{
\begin{threeparttable}
\begin{tabular}{lccl}
    \toprule
    \textbf{Target} & \textbf{Source file} & \textbf{Input format} & \textbf{Test instruction} \\ \midrule
    \textbf{tiff2bw} & \multirow{2}{*}{libtiff 3.9.7} & \multirow{2}{*}{tiff} & tiff2bw @@\tnote{1}~{ } /dev/null \\
    \textbf{tiffsplit} &&& tiffsplit @@ /dev/null\\
    \midrule
    \textbf{nm} & \multirow{5}{*}{binutils-2.28} & \multirow{5}{*}{ELF} & (-A -a -l -S -s \\
    &&&\ \ \ --special-syms --synthetic\\
    &&&\ \ \ --with-symbol-versions -D @@) \\
    \textbf{objdump} &&& -S @@ \\
    \textbf{readelf} &&& -a @@ \\
    \textbf{size} &&& @@ \\
    \textbf{strip} &&& -o tmp\_file @@  \\
    \midrule
    \textbf{pdftotext} & pdftotext 4.00 & pdf & @@ /dev/null \\
    \midrule
    \textbf{infotocap} & jasper 2.0.12 & text & -o /dev/null @@ \\
    \midrule
    \textbf{mp42aac} & Bento4 1.5.1-628 & mp4 & @@ /dev/null \\
    \midrule
    \textbf{tcpdump} & tcpdump 4.8.1 + libpcap 1.8.1 & tcpdump100 & -e -vv -nr @@ \\
    \midrule
    \textbf{sqlite3} & SQLite 3.8.9 & sql &  < @@ \\
    \midrule
    \textbf{lame3.99.5} & lame 3.99.5 & wav & @@ /dev/null \\
    \midrule
    \textbf{imginfo} & ncurses 6.1 & jpg & -f @@ \\
    \midrule
    \textbf{jq} & jq 1.5 & json & . @@ \\
    \midrule
    \textbf{mujs} & mujs 1.0.2 & js & @@ \\
    \bottomrule
\end{tabular}
\begin{tablenotes}
\item[1] @@: A placeholder indicating that the input is a file.
\end{tablenotes}
\end{threeparttable}

}
\label{subjects}
\end{table}

Following the guidance of Marcel Böhme, we should avoid the situation that the observed improvements may be mainly due to design and engineering differences. Thus, we evaluate our method with the other strategies in AFL++, which minimizes engineering differences for a reliable comparison result.

Finally, we constructed 8 different versions of the AFL++. 
AFL++ uses the default setting in AFL++.  
AFL++-mopt only leverages the MOPT strategy, which utilizes Particle Swarm Optimization (PSO) algorithm to achieve mutation operator schedule.
AFL++redqueen uses the Redqueen strategy, which uses the input-to-state correspondence to resolve the constraints of magic bytes. 
AFL++-mopt-redqueen uses the MOPT strategy and the Redqueen strategy at the same time. 
AFL++-rare sets the power schedule as RARE mode, which mutates inputs to target rare branches in the program.
AFL++-fast sets the power schedule as FAST mode, which pays more attention to exploring low-frequency paths instead of high-frequency paths.
AFL++-exploit sets the power schedule as EXPLOIT mode, which is AFL's exploitation-based constant schedule.

As our proposed strategy can be treated as an independent mutation strategy in AFL++, we can integrate our strategy with other strategies in  AFL++, such as the strategy of Redqueen. \tool{}-redqueen intergates the history strategy and the Redqueen strategy together. 

Follow Marcel Böhme, we ran each fuzzer on all target programs for 12 hours. To avoid the randomness, we repeated the experiment for 5 times.


\subsubsection{Edge Coverage}
\textbf{The growth trend of edge coverage.}
Figure X illustrates the edge coverage growth of each fuzzer over 24 hours experiments on 8 programs, including $nm, objdump, readelf, size, strip, tiff2bw$  and so on.
\tool{}-related fuzzers (i.e., \tool{} and \tool{}-redqueen) achieve better performance on almost all programs over the 24 hours.
Therefore, the results indicate that the \tool{}-related fuzzers have a steady and stronger growth trend on edge coverage than other fuzzers. For instance, the confidence interval of \tool{}-redqueen and \tool{} is above other fuzzers on XXX during the fuzzing process.

\textbf{The edge coverage after fuzzing 3/6/12 hours.}To evaluate the efficiency of \tool{}-related fuzzers at the beginning of testing, we compared edge coverage after fuzzing 3/6/12 hours. The results are shown in Table X. \tool{} and \tool{}-redqueen achieve better new edge coverage on most programs than other fuzzers after fuzzing 3/6/12 hours. More specifically, after fuzzing 3 hours, the best fuzzer is \tool{} which achieves the best performance on X programs. Moreover, the second best fuzzer is \tool{}-redqueen which achieves the best performance on X programs. 

For \tool{}, it finds on average X\%, Y\%, and Z\% more edge coverage than the best fuzzer besides \tool{}-related(i.e., AFL++-mopt) at 3/6/12 hours, respectively, which indicates that \tool{} has a better performance at the beginning of fuzzing campaigns. Especially in XX, \tool{} finds more X\%, Y\%, Z\%, X\%, Y\%, Z\% and H\% edge coverage than AFL++, AFL++-fast , AFL++-rare , AFL++-exploit , AFL++-mopt, AFL++-redqueen and AFL++-mopt-redqueen. As shown in Table X, we rank each fuzzer based on edge coverage after fuzzing 3/6/12 hours and then show the average rank of fuzzers across all programs. The lower the rank is, the better the fuzzer performs. Specifically, \tool{} achieves the lowest rank at all three timing, and the second best fuzzer is \tool{}-redqueen, whose average ranks are X, Y, and Z after fuzzing 3, 6, and 9 hours. Thus, TransferFuzz-related fuzzers can find more edge coverage in the shorter limited time budget.


\textbf{The analysis of the statistical significance.}
To avoid statistical errors, We further evaluate all 9 fuzzers using Mann-Whitney U tests. More specifically, we calculate the p-values among all fuzzers regarding the edge coverage for all programs across all campaigns. P-values represent how different two fuzzers are and quantify how significant these differences are. If p $<$ 0.05, we believe that there exists a significant difference. The results are shown in Table X. Cells with a green shade represent that the edge coverage found by the corresponding two \tool{}-related fuzzers is statistically different. Based on the results of the p-value, \tool{} performs significantly better than AFL++, AFL++-fast , AFL++-rare , AFL++-exploit , AFL++-mopt, AFL++-redqueen and AFL++-mopt-redqueen on XX, XX, XX, and XX real-world programs, which performs best among all fuzzers. But \tool{}-redqueen performs significantly better than \tool{} on X real-world programs. Thus, The combiation of these two modes are efficient for the target programs that contain a lot of magic number problems.

\subsubsection{Bug Discovery}
We analyze the number of unique vulnerabilities triggered by a fuzzer based on ASan. Following the guidance of XX, we select the top three stack frames to de-duplicate vulnerabilities. 
Table X shows the number of unique vulnerabilities triggered by each fuzzer. Our statistics show \tool{}, \tool{}-redqueen, AFL++-raw, AFL++-mopt, AFL++-fast, AFL++-rare, AFL++-exploit, AFL++-redqueen, and AFL++-mopt-redqueen triggered 16, 21, 18, 18, and 9 vulnerabilities, respectively. 
\tool{}-redqueen performs the best on XX programs (XX, XX, XX). \tool{} performs the best on XX programs (XX, XX, XX). XX, XX, and XX do not perform the best on any program. 
\tool{}-related fuzzers perform the best on most of the programs.
Thus, \tool{}-related fuzzers also find more unique vulnerabilities than other fuzzers. 
This demonstrates 
The bug discovery experiment results demonstrates the effectiveness of \tool{} in fuzzing. The positions extracted by \tool{} can improve the fuzzing performance.

\subsection{Evaluation on MAGMA}
MAGMA is a ground-truth fuzzing benchmark that enables accurate and consistent fuzzer evaluation. MAGMA provides seven benchmarks with real bugs by introducing real bugs into real-world programs. Thus, we can perform a realistic evaluation of fuzzers based on MAGMA.
We integrate our \tool{} and \tool{}-redqueen into MAGMA. Then, we evaluate these two \tool{}-related fuzzers and 5 widely-used mutation-based fuzzers(AFL, AFLFast, FairFuzz, MOPT and AFL++) against MAGMA. 
Each MOPT-based fuzzer sets the parameter '-L'  as 5 in the evaluation. For AFL++, we enable the MOPT strategy and Redqueen strategy at the same time.
We run each experiment for 24 hours and repeated 5 times to avoid randomness.

\subsubsection{Bug Count and Statistical Significance}
Fig X shows the mean number of CVEs triggered by each fuzzer. 
Specifically, \tool{}-redqueen performs significantly better than all other fuzzers in X out of X programs(XX, XX, and XX). 
\tool{} is the best fuzzer for XX, XX, and XX, and \tool{}-redqueen is the best fuzzer for XX, XX, and XX.
For instance, CVE-2018-1000876 found by both \tool{} and \tool{}-redqueen triggered buffer overflow vulnerability in XX, which causes security problems. 
Therefore, \tool{}-related fuzzers focus on mutating structure-related positions, which indeed improves the performance of serious vulnerability discovery.

\subsubsection{Time to Bug}
(As shown in Fig.X, all 9 fuzzers triggered XX of the 118 MAGMA bugs after fuzzing 24 hours. This figure is generated by MAGMA, which sorts the bugs based on the mean trigger time to represent the “difficulty”. Here are X simple bugs triggered by all 9 fuzzers within 24 hours. Especially, \tool{}-redqueen triggers X bugs in X hours while the second best fuzzer(XX) only triggers Y bugs. Additionally, \tool{}-redqueen performs better than all other fuzzers because it finds X bugs that are not triggered by the other 8 fuzzers.)

\subsubsection{Survival functions}
We also show the probability of a bug surviving a 24 hours fuzzing trial of four programs generated by MAGMA, which is shown in fig.X. Dotted lines and solid lines indicate the survival functions for reached bugs and triggered bugs, respectively, and the shaded regions are confidence intervals. As the bug’s probability of survival decreases to 0 fastest, \tool{}-redqueen is the best fuzzer on these four programs.


\subsection{Overhead}
\tool{} requires collecting the information of the length mutators used and removing the redundant mutated positions to get a minimal mutation set. Moreover, our mode scheduler needs to determine the next mode to be used after each mutation. Thus, we believe that the extra approaches used by TransferFuzz are bad for fuzzing throughput. 
In order to quantify the influence on throughput, we measure the throughput of all 9 fuzzers on X programs after fuzzing 24 hours. The results are shown in Table X. Specifically, the average throughput of four \tool{}-related fuzzers (\tool{}-redqueen and \tool{}) does not drop significantly compared to the throughput of AFL++ on most programs. Surprisingly, the throughput of \tool{}-redqueen is more than AFL++-raw on X programs. Therefore, our TransferFuzz-related fuzzers do not introduce a large overhead.

\subsection{Effectiveness of algorithms }
In order to evaluate the efficiency of the new mutation mode used by \tool{}, we implement \tool{}-compare that disables the use of the new mutation mode. Note that \tool{}-compare is different from AFL++-raw since AFL++-compare still collects and analyzes the information of mutated positions. We evaluate \tool{}-compare with the other two \tool{}-related fuzzers in the fuzzer-test-suite of UNIFUZZ 12 hours for 5 times. 
The results of edge coverage are shown in Table X. It illustrates that the mutation mode helps discover more X\% more edges than \tool{}-compare. 
Especially, \tool{} and \tool{}-redqueen perform best and discover more X\% and Y\% more edges than AFL++-compare. Based on the results, we conclude that the new mutation modes used by \tool{} are efficient.

% \begin{table}[!t]
% \centering
% \caption{Edge Rank.}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{@{\extracolsep{4pt}}lrrrrrrrrrrr@{}}
% \toprule

% \textbf{Time} &  \textbf{all} & \textbf{history}& \textbf{new} & \textbf{mopt} & \textbf{exploit} & \textbf{fast} & \textbf{raw} & \textbf{rare} & \textbf{compare}\\
% \midrule
% \textbf{1 hour} & 2.4   &   2.2  & 4.4  & 6.9   &   6.4 &  5.3  & 5.3&   7.2  &    4.4 \\
% \textbf{3 hours} & 2.4   &   2.2  & 4.4  & 6.9   &   6.4 &  5.3  & 5.3&   7.2  &    4.4 \\
% \textbf{6 hours} & 3.0   &   2.3  & 4.9  & 7.0   &   6.3  & 4.8  & 4.9 &  7.4   &   4.3\\
% \textbf{12 hours} & 2.8  &    2.4  & 4.9 &  6.6    &  6.3  & 4.9 &  5.3  & 7.1    &  4.6\\
% \textbf{24 hours} & 2.8  &    2.4  & 4.9 &  6.6    &  6.3  & 4.9 &  5.3  & 7.1    &  4.6\\

% \bottomrule
% \end{tabular}
% }
% \label{edge_rank_for_unifuzz}
% \end{table}


\begin{table}[!t]
\centering
\caption{Unique Vulnerabilities.}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{\extracolsep{4pt}}cccccccccccc@{}} %crrrrrrrrrrr
\toprule

\rotatebox{90}{\textbf{Programs}} &  \rotatebox{90}{\textbf{Pozzer}} & \rotatebox{90}{\textbf{Pozzer-Redqueen}}& \rotatebox{90}{\textbf{AFL++-MOPT-Redqueen}} & \rotatebox{90}{\textbf{AFL++-MOPT}} & \rotatebox{90}{\textbf{AFL++-exploit}} & \rotatebox{90}{\textbf{AFL++-fast}} & \rotatebox{90}{\textbf{AFL++-rare}}\\
\midrule
mp42aac &                 \textbf{7.0}   &   \textbf{7.0}       &     5.0 &  5.0   &   0.0 &  0.0 &  0.0\\
imginfo  &                1.0&      1.0       &     1.0  & 1.0   &   \textbf{2.0}  & 0.0 &  0.0\\
tiff2pdf  &               \textbf{2.0} &     1.0       &     \textbf{2.0}  & \textbf{2.0}   &   0.0  & 0.0 &  0.0\\
lame       &              4.0  &    4.0       &     4.0  & 4.0   &   \textbf{5.0}  & 4.0 &  4.0\\
readelf228  &             \textbf{10.0}   &  8.0       &     4.0  & 4.0   &   3.0  & 5.0 &  5.0\\
exiv2        &           \textbf{33.0}    & 31.0       &    23.0  &23.0   &  15.0  &15.0 & 14.0\\
flvmeta       &           2.0     & 2.0       &     2.0  & 2.0   &   2.0  & 2.0 &  2.0\\
nm228          &         \textbf{43.0}&     34.0       &    30.0  &33.0   &  22.0  &20.0 & 32.0\\
tiffsplit       &        \textbf{10.0} &    \textbf{10.0}       &     9.0  & \textbf{10.0}   &   5.0  & 7.0 &  5.0\\
tiff2bw          &        \textbf{12.0}  &   9.0       &     6.0  & 8.0   &  5.0  & 5.0 &  7.0\\
objdump228        &      \textbf{30.0}   &  21.0       &    11.0  &11.0   &  12.0  &10.0 &  8.0\\
pdftotext          &     \textbf{33.0}    & 16.0       &    24.0  &29.0   &  23.0  &26.0 & 23.0\\
tcpdump             &     \textbf{3.0}     & 1.0       &     1.0  & 1.0   &   2.0  & 1.0 &  2.0\\
infotocap            &   \textbf{12.0}     &11.0       &     9.0  &11.0   &   5.0  & 9.0  & 9.0\\
\midrule
\textbf{Sum} & \textbf{203.0}  &  156.0 & 131.0  & 144.0  &  101.0 & 104.0  & 111.0\\


\bottomrule
\end{tabular}
}
\label{unifuzz_bug}
\end{table}


\subsection{Verification Experiment}



% \begin{table*}[!t]
% \centering
% \caption{The Result of SHAP Analysis. We extract the most important positions based on the data collected from 48 hours fuzzing campaigns. Top$N$\% means that the top N\% of the most important positions. $X$mins means fuzzing $X$ mins. And the value in the table represent the ratio at which the positions collected in common features after fuzzing X mins and the top N\% of the most important positions intersect. The higher the value, the better the performance. And the Baseline means that we randomly select positions into common features.}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{@{\extracolsep{4pt}}lrrrrrrrrrrr@{}}
% \toprule

% \textbf{Time} &  \textbf{Top10\%} & \textbf{Top20\%}& \textbf{Top30\%} & \textbf{Top40\%} & \textbf{Top50\%} & \textbf{Top60\%} & \textbf{Top70\%} & \textbf{Top80\%} & \textbf{Top90\%} & \textbf{Top100\%} & \textbf{Baseline}\\
% \midrule
% \textbf{10mins}  &0.67 &   0.59  &  0.55  &  0.52  &  0.49 &   0.46  &  0.44  &  0.42   & 0.40  &   0.38   &   0.07 \\
% \textbf{20mins}  & 0.77  &  0.71  &  0.68  &  0.65   & 0.62   & 0.60  &  0.58 &   0.56  &  0.54   &  0.52    &  0.14 \\
% \textbf{30mins}  & 0.81 &   0.76  &  0.73   & 0.71   & 0.68  &  0.67  &  0.64  &  0.63  &  0.61    & 0.59     & 0.17 \\
% \textbf{40mins}  & 0.83  &  0.79  &  0.77  &  0.75  &  0.72  &  0.71 &   0.69  &  0.67  &  0.65  &   0.63   &   0.18 \\
% \textbf{50mins}  & 0.85  &  0.81  &  0.79  &  0.78  &  0.75  &  0.73   & 0.71  &  0.69  &  0.68   &  0.66    &  0.19 \\
% \textbf{60mins}  & 0.86  &  0.83   & 0.81  &  0.79  &  0.77  &  0.75   & 0.73   & 0.71  &  0.70   &  0.68   &   0.20 \\
% \textbf{70mins}  & 0.87  &  0.84 &   0.82  &  0.81  &  0.78  &  0.77   & 0.75  &  0.73   & 0.72   &  0.70   &   0.20 \\
% \textbf{80mins}  & 0.88  &  0.85  &  0.83  &  0.82  &  0.80  &  0.78   & 0.76  &  0.75  &  0.73  &   0.71 &     0.20 \\
% \textbf{90mins}  & 0.88  &  0.86  &  0.84  &  0.83  &  0.81   & 0.79   & 0.78  &  0.76  &  0.74  &   0.73   &   0.21 \\
% \textbf{100mins}  & 0.88  &  0.86  &  0.85  &  0.84  &  0.81   & 0.80   & 0.78  &  0.77 &   0.75   &  0.73    &  0.21 \\
% \textbf{110mins}  & 0.89  &  0.87  &  0.85 &   0.84  &  0.82   & 0.81  &  0.79  &  0.78  &  0.76  &   0.74  &    0.21 \\
% \textbf{120mins}  & 0.90  &  0.87  &  0.86 &   0.85   & 0.83  &  0.82  &  0.80 &   0.79&    0.77 &    0.75   &   0.23 \\


% \bottomrule
% \end{tabular}
% }
% \label{shap}
% \end{table*}

\begin{table}[!t]
\centering
\caption{Time To Bugs.}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{\extracolsep{4pt}}crrrrrrrrrrr@{}}
\toprule

\rotatebox{90}{\textbf{Vulnerabilities}} & \rotatebox{90}{\textbf{Pozzer}}  & \rotatebox{90}{\textbf{Pozzer-Redqueen}} & \rotatebox{90}{\textbf{AFL++-MOPT-Redqueen}} & \rotatebox{90}{\textbf{MOPT}} & \rotatebox{90}{\textbf{FairFuzz}}  &  \rotatebox{90}{\textbf{AFL}} & \rotatebox{90}{\textbf{AFLFast}} \\
\midrule

\rowcolor{gray!20} CVE-2015-8472 & 17s & 19s & 23s & \textbf{15s} & \textbf{15s} & \textbf{15s} & \textbf{15s} \\ 
CVE-2016-1762 & 47s & 56s & 1m & \textbf{15s} & 20s & 16s & 18s \\
\rowcolor{gray!20} CVE-2018-13988 & 1m & \textbf{52s} & 1m & \textbf{52s} & 2m & 1m & 1m \\
CVE-2016-2109 & 3m & 3m & 4m & \textbf{1m} & 2m & \textbf{1m} & 2m \\
\rowcolor{gray!20} CVE-2016-6309 & 4m & 5m & 5m & \textbf{1m} & 2m & \textbf{1m} & \textbf{1m} \\
CVE-2016-10270 & \textbf{23s} & 33s & 48s & 19m & 3m & 23m & 11m \\
\rowcolor{gray!20} CVE-2016-3658 & \textbf{4m} & 7m & 17m & 1h & 25m & 1h & 1h \\
CVE-2018-14883 & 18m & 16m & 1h & 3m & 2h & \textbf{2m} & 3m \\
\rowcolor{gray!20} CVE-2017-6892 & \textbf{13m} & 30m & 32m & 33m & 3h & \textbf{13m} & 1h \\
SND017 & \textbf{4m} & 8m & 5m & 25m & 21h & 38m & 5m \\
\rowcolor{gray!20} CVE-2017-11613 & \textbf{9m} & 14m & 1h & 1h & 15h & 6h & 4h \\
CVE-2019-11034 & 6h & 15h & 15h & \textbf{1m} & 8m & 2m & \textbf{1m} \\
\rowcolor{gray!20} PDF010 & 3h & 2h & 1h & 7h & 16h & 10h & \textbf{2m} \\
CVE-2019-7663 & \textbf{3h} & \textbf{3h} & 8h & 4h & 9h & 16h & 6h \\
\rowcolor{gray!20} CVE-2019-20218 & \textbf{49m} & 1h & 2h & 16h & 11h & 9h & 9h \\
CVE-2019-9638 & \textbf{41m} & 5h & 17h & 7h & 17h & 4h & 44m \\
\rowcolor{gray!20} CVE-2015-8317 & 22m & \textbf{21m} & 1h & 3h & - & - & 12h \\
CVE-2019-7310 & 7h & \textbf{5h} & 17h & 9h & 15h & 7h & 8h \\
\rowcolor{gray!20} CVE-2020-15945 & 5h & 5h & \textbf{4h} & 14h & 15h & 13h & 16h \\
SND020 & \textbf{16m} & 17m & 19m & 7h & 21h & - & - \\
\rowcolor{gray!20} CVE-2015-3414 & \textbf{1h} & \textbf{1h} & 4h & 17h & 16h & 23h & 15h \\
CVE-2016-10269 & 2h & \textbf{44m} & 1h & 15h & 22h & 15h & - \\
\rowcolor{gray!20} CVE-2011-2696 & 18m & \textbf{17m} & 22m & 17h & - & 22h & 23h \\
CVE-2017-8363 & \textbf{13m} & 14m & 28m & 18h & 22h & - & - \\
\rowcolor{gray!20} CVE-2017-8363 & 27m & \textbf{25m} & 32m & 18h & 22h & - & - \\
CVE-2017-9047 & 33m & \textbf{28m} & 6h & 12h & - & - & - \\
\rowcolor{gray!20} CVE-2017-8361 & \textbf{14m} & 15m & 3h & 18h & 22h & - & - \\
CVE-2016-6302 & 9h & 18h & 23h & 16h & - & \textbf{3h} & 6h \\
\rowcolor{gray!20} CVE-2017-7375 & 6h & 5h & \textbf{1h} & - & - & - & - \\
CVE-2018-10768 & 5h & \textbf{4h} & 5h & 23h & - & - & 23h \\
\rowcolor{gray!20} CVE-2016-5314 & 19h & 15h & 19h & 11h & 16h & \textbf{4h} & - \\
CVE-2013-6954 & 13h & 15h & 19h & 16h & 12h & \textbf{11h} & - \\
\rowcolor{gray!20} CVE-2019-19926 & \textbf{5h} & 6h & 19h & 17h & - & 21h & 20h \\
PNG006 & - & 8m & \textbf{6m} & - & - & - & - \\
\rowcolor{gray!20} CVE-2016-2108 & \textbf{3h} & 6h & 16h & 22h & - & - & - \\
CVE-2016-10269 & 23h & \textbf{2h} & \textbf{2h} & 22h & - & - & - \\
\rowcolor{gray!20} CVE-2017-9865 & 8h & \textbf{7h} & 12h & - & - & - & - \\
CVE-2015-8784 & 22h & 23h & 21h & 20h & \textbf{18h} & - & 20h \\
\rowcolor{gray!20} CVE-2016-1836 & \textbf{22h} & \textbf{22h} & 23h & - & - & - & - \\
CVE-2017-14617 & - & - & \textbf{21h} & - & - & - & - \\
\rowcolor{gray!20} CVE-2017-3735 & 20h & - & - & \textbf{5h} & 15h & 22h & 10h \\
CVE-2017-9776 & 19h & \textbf{15h} & - & - & - & - & - \\
\rowcolor{gray!20} CVE-2013-7443 & \textbf{17h} & 21h & - & - & - & - & - \\
CVE-2019-19880 & \textbf{18h} & 22h & - & - & - & - & - \\
\rowcolor{gray!20} PDF008 & \textbf{20h} & 21h & - & - & - & - & - \\
CVE-2019-19646 & 22h & \textbf{21h} & - & - & - & - & - \\
\rowcolor{gray!20} CVE-2017-2518 & \textbf{22h} & - & - & - & - & - & - \\
CVE-2019-19317 & \textbf{22h} & - & - & - & - & - & - \\
\rowcolor{gray!50}\#The Fastest & 20 & 15 & 5 & 7 & 2 & 8 & 4 \\



\bottomrule
\end{tabular}
}
\label{TTB}
\end{table}


\begin{table*}[!t]
% \renewcommand\arraystretch{1.7}
% \newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
\centering
\caption{Original vs. \textsc{Truzz}-equipped fuzzers on the percentage of valid input generated.} \label{tab:valid_percent}
\resizebox{0.9\linewidth}{!}{
\begin{threeparttable}
\begin{tabular}{@{\extracolsep{4pt}}lccccccccccccccc@{}}
\toprule
\multirow{3}{*}{\textbf{Program}} & \multicolumn{3}{c}{\textbf{GreyOne}} & \multicolumn{3}{c}{\textbf{ProFuzzer}} & \multicolumn{3}{c}{\textbf{Pozzer}}\\
\cline{2-4} \cline{5-7} \cline{8-10}


&\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Analysis}\\ \textbf{Time}\end{tabular}} 
&\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Useful}\\ \textbf{Ratio}\end{tabular}} 
&\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Average Useful}\\ \textbf{Mutation}\end{tabular}} 

&\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Analysis}\\ \textbf{Time}\end{tabular}} 
&\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Useful}\\ \textbf{Ratio}\end{tabular}} 
&\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Average Useful}\\ \textbf{Mutation}\end{tabular}} 

&\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Analysis}\\ \textbf{Time}\end{tabular}} 
&\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Useful}\\ \textbf{Ratio}\end{tabular}} 
&\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Average Useful}\\ \textbf{Mutation}\end{tabular}} \\
&&&&&&&&&\\
\midrule

\textbf{nm} & 16721 & 3\%(135/4834) & 0.11 & 13584 & 16\%(109/665) & 0.32 & \textbf{16.68} & \textbf{68\%(55/82)} & \textbf{1.87}  \\
\textbf{tiff2bw} & 8283 & 13\%(101/762) & 0.74 & 9372 & 14\%(106/762) & 0.75 & \textbf{7} & \textbf{90\%(74/83)} & \textbf{5.87}\\
\textbf{tiffsplit} & 8875 & 68\%(104/152) & 3.18 & 10894 & 70\%(104/150) & 3.25 & \textbf{8} & \textbf{92\%(72/78)} & \textbf{6.60}\\
\textbf{objdump} & 52080 & 2\%(205/13288) & 0.45 & 29901 & 18\%(318/1794) & 0.68 & \textbf{45} & \textbf{60\%(179/299)} & \textbf{1.70} \\
\textbf{readelf} & 16739 & 3\%(99/3798) & 0.41 & 13712 & 7\%(186/2641) & 0.48 & \textbf{37} & \textbf{83\%(95/114)} & \textbf{8.70}\\
\textbf{flvmeta} & 2262 & 47\%(29/63) & 1.28 & 2222 & 23\%(42/187) & 0.46 & \textbf{2} & \textbf{40\%(14/35)} & \textbf{1.08}\\
\textbf{pdftotext} & 54447 & 3\%(267/8384) & 0.07 & 38144 & 4\%(337/8805) & 0.08 & \textbf{54} & \textbf{54\%(165/305)} & \textbf{1.11}\\
\textbf{mp42aac} & 11855 & 19\%(124/651) & 0.32 & 17234 & 22\%(132/614) & 0.35 & \textbf{9} & \textbf{68\%(69/102)} & \textbf{1.70}\\
\textbf{tcpdump} & 13219 & 2\%(88/4075) & 2.89 & 13774 & 3\%(87/2708) & 2.48 & \textbf{16} & \textbf{77\%(72/93)} & \textbf{6.36}\\
\textbf{lame3.99.5} & 75520 & 1\%(169/13077) & 0.02 & 62433 & 1\%(179/13060) & 0.02 & \textbf{80} & \textbf{73\%(74/102)} & \textbf{2.16}\\

% \textbf{size}\\
% \textbf{infotocap}\\
% \textbf{sqlite3}\\
% \textbf{imginfo}\\
% \textbf{jq}\\
% \textbf{mujs}\\

\bottomrule
\end{tabular}
\end{threeparttable}
}
\end{table*}

\begin{figure*}[htbp]
\includegraphics[width=\linewidth]{images/legend.png}
\label{legend}
\end{figure*}

\begin{figure*}[htbp]
\vspace{-1cm}
\includegraphics[width=\linewidth]{images/time_ane_edge.png}
\caption{Time Ane Edge.}
\label{time_ane_edge}
\end{figure*}

\begin{figure*}[htbp]
\includegraphics[width=\linewidth]{images/average_ranks.png}
\caption{Average Edge Ranks.}
\label{average_ranks}
\end{figure*}

==> obsolete/evaluation-0.3.tex <==
\section{Evaluation}



% \zhu{current experiments: \begin{itemize}
%     % \item UNIFUZZ: edge discovery: time to edges => move to appendix
%     \item UNIFUZZ: edge rank
%     % \item UNIFUZZ: bug discovery: \#bugs => move to appendix
%     \item UNIFUZZ: overhead
%     % \item UNIFUZZ: \tool{} vs EMS: \#edges => move to appendix?
%     \item MAGMA: \#bugs
%     \item MAGMA: time to bugs
%     \item proportion of useful positions
% \end{itemize}}

% \todo{contents \begin{itemize}
%     \item research questions
%     \item edge discovery \begin{itemize}
%         \item 
%     \end{itemize}
%     \item bug discovery
%     \item effective of selected positions
% \end{itemize}}

We implemented our \tool{} based on AFL++~\cite{aflpp}, which integrates many state-of-the-art fuzzing algorithms. To ensure the fair results, we conducted our experiments on two third-party testing platforms, UNIFUZZ\zhu{cite} and MAGMA\zhu{cite}. Our experiments were performed on a system running Ubuntu 18.04 with 103 cores (Intel(R) Xeon(R) Gold 6230R CPU) and 256 GB of memory. To ensure a fair comparison, each fuzzer ran on one CPU core.


\todo{in progress}

In order to evaluate \tool{}, we implemented \tool{} based on AFL++, which has integrated many fuzzing strategies. 
To reduce the influence of subjective factors, we conduct our experiments on a third-party testing platform.

% We divided our experiments into three parts. 
% \begin{itemize}
%     \item \textbf{Evaluation on UNIFUZZ.} In the first part, we evaluated \tool{} based on UNIFUZZ, which contains a series of real-world programs and provides a standardized testing process to evaluate the performance of fuzzers on code coverage and bug discovery. We compared \tool{} with other strategies inside AFL++. 
%     \item \textbf{Evaluation on MAGMA.} In the second part, we evaluated \tool{} based on MAGMA. Unlike UNIFUZZ, MAGMA only focuses on bug discovery and has a very detailed analysis.
%     \item \textbf{Further Analysis.} In the third part, we further analyze \tool{}'s performance in terms of throughput, etc., and further explore the source of \tool{}'s effect. a) we evaluate the throughput of \tool{} and perform ablation experiments to verify the efficiency of the proposed new mutation modes. b) we verify that \tool{} can discover most of the important bytes in a short time. c) We construct ablation experiments to verify that \tool{}'s improvement comes from the design of our mutation strategy.
% \end{itemize}

\subsection{Experimental Setup}
% \zhu{Don't leave blank between titles!}
\textbf{Experiment Environment.}
All our measurements were performed on a system running Ubuntu 18.04 with 103 cores (Intel(R) Xeon(R) Gold 6230R CPU) and 256 GiB of main memory. To make a fair comparison, each fuzzer performed single-threaded execution on one CPU core.
% Additionally, we repeat the experiment ten times.

\textbf{Benchmark Fuzzers.}
In our evaluation, we compared \tool{} with the state-of-the-art fuzzers, including AFL++, EMS, MOPT, AFLFast, FairFuzz and AFL.
The reasons why we chose these fuzzers are as follows.

% We select 5 fuzzers to evaluate our approach. We evaluate our approach with AFL++, MOPT, AFL, AFLFast and FairFuzz.
\begin{itemize}
    \item Fioraldi et al. proposed AFL++~\cite{aflpp}, which is a fuzzing framework that includes many fuzzing strategies, including MOPT, Redqueen, AFLfast, etc. AFL++ has achieved outstanding results in the experiments of other papers and the evaluation of third-party  platforms such as Fuzzbench. To better integrate our strategy with other strategies, we implemented \tool{} based on AFL++. Within AFL++, we only need to adjust the parameter settings to allow \tool{} to compare fairly with other fuzzing strategies. Also, comparing within AFL++ avoids the effects of differences in implementation architectures to obtain reliable experimental results. Finally, we use multiple different settings in AFL++ to evaluate.
    \item MOPT utilizes Particle Swarm Optimization (PSO) algorithm to optimize AFL’s mutation operator schedule based on fuzzing history information. MOPT dynamically generates the distribution for mutators to improve the fuzzing efficiency. All MOPT-related fuzzers sets the parameter '-L'  as 5 in the experiments.
    \item EMS proposes a probabilistic byte orientation model to capture mutation strategies from intra- and inter-trial history to trigger unique paths and crashes. We use the initial inter-PBOM provided by the EMS source code.
    Because EMS is implemented on the basis of MOPT, we also sets the parameter '-L'  as 5.
    \item AFLFast is a widely-used extension of AFL, which models fuzzing process as Markov chain and prioritizes exploring those low-frequency paths to achieve better code coverage. 
    \item FairFuzz proposes a novel mutation mask creation algorithm to guide mutations to be biased towards producing inputs triggering rare branches.
    \item AFL, the American Fuzzy Lop, is one of the most famous fuzzers, which has discovered many bugs in real-world applications. 
\end{itemize}

\textbf{Initial Seeds.}
All fuzzers used the same initial seeds collected from UNIFUZZ, FuzzBench, Magma or public seed corpus. 
Follow the guidance of Adrian Herrera~\cite{herrera2021seed}, most target programs have multiple initial seeds instead of a single initial seed.

\textbf{Evaluation Metrics.}
As the different implementations in different fuzzers, we need uniform evaluation metrics to evaluate the fuzzers’ performance. Following the guidance in Marcel Böhme~\cite{bohme2022reliability}, we mainly use the following two metrics. 

The first one is edge coverage which is widely used in recent research to evaluate fuzzers. 
% Specifically, the edge coverage is only used when evaluating based on UNIFUZZ.
When we compare \tool{} with other settings in AFL++, we do not need to leverage other tools to collect the edge coverage because we have the same low-level implementation. Thus, we use the internal tool \textit{afl-showmap} of AFL++ to calculate the edge coverage. 
When we compare \tool{} with EMS, we also utilize the \textit{afl-showmap} of AFL++ to uniformly calculate edge coverage.
% When we use the edge coverage, we only compare \tool{} with the other fuzzing strategies in AFL++.

The second one is the number of unique vulnerabilities, which directly indicates the performance of fuzzer. More specifically, We use ASan to de-duplicate vulnerabilities and analyze the number of unique vulnerabilities discovered by a fuzzer in each trial. Specifically, We use the top three function calls in the output report generated by ASAN to de-duplicate vulnerabilities. 

\subsection{The evaluation based on UNIFUZZ}
UNIFUZZ is an open-source, holistic, and pragmatic metrics-driven platform to evaluate fuzzers fairly. UNIFUZZ provides 20 real-world benchmark programs with multiple initial seeds. As shown in Table~\ref{programs}, We evaluated our \tool{} on 12 open-source programs selected from UNIFUZZ and 4 widely used programs selected from other fuzzing papers as shown in Table~\ref{programsUNIFUZZ}.

\begin{table}[!t]
% \renewcommand\arraystretch{1}
\centering
\caption{Target programs.\zhu{UNIFUZZ}}\label{programsUNIFUZZ}
\resizebox{\linewidth}{!}{
\begin{threeparttable}
\begin{tabular}{lccl}
    \toprule
    \textbf{Target} & \textbf{Source file} & \textbf{Input format} & \textbf{Test instruction} \\ \midrule
    \textbf{tiff2bw} & \multirow{3}{*}{libtiff 3.9.7} & \multirow{3}{*}{tiff} & tiff2bw @@\tnote{1}~{ } /dev/null \\
    \textbf{tiffsplit} &&& tiffsplit @@ /dev/null\\
    \textbf{tiff2pdf} &&& tiff2pdf @@ /dev/null\\
    \midrule
    \multirow{3}{*}{\textbf{nm}} & \multirow{6}{*}{binutils-2.28} & \multirow{4}{*}{ELF} & (-A -a -l -S -s \\
    &&&\ \ \ --special-syms --synthetic\\
    &&&\ \ \ --with-symbol-versions -D @@) \\
    \textbf{objdump} &&& -S @@ \\
    \textbf{readelf} &&& -a @@ \\
    \textbf{size} &&& @@ \\
    \midrule
    \textbf{pdftotext} & pdftotext 4.00 & pdf & @@ /dev/null \\
    \midrule
    \textbf{infotocap} & jasper 2.0.12 & text & -o /dev/null @@ \\
    \midrule
    \textbf{mp42aac} & Bento4 1.5.1-628 & mp4 & @@ /dev/null \\
    \midrule
    \multirow{2}{*}{\textbf{tcpdump}}
     & tcpdump 4.8.1 + & \multirow{2}{*}{tcpdump100} & \multirow{2}{*}{-e -vv -nr @@} \\
     & libpcap 1.8.1 && \\
    \midrule
    \textbf{flvmeta} & flvmeta 1.2.1 & flv &  @@ \\
    \midrule
    \textbf{lame3.99.5} & lame 3.99.5 & wav & @@ /dev/null \\
    \midrule
    \textbf{imginfo} & ncurses 6.1 & jpg & -f @@ \\
    \midrule
    \textbf{mujs} & mujs 1.0.2 & js & @@ \\
    \midrule
    \textbf{exiv2} & exiv2 0.26 & jpg & @@ \\
    \bottomrule
\end{tabular}
\begin{tablenotes}
\item[1] @@: A placeholder indicating that the input is a file.
\end{tablenotes}
\end{threeparttable}

}
\label{programs}
\end{table}

Following the guidance of Marcel Böhme~\cite{bohme2022reliability}, we should avoid the situation that the observed improvements may be mainly due to design and engineering differences. Thus, we integrated our strategy into AFL++ and evaluated \tool{} with the other strategies in AFL++, which minimizes engineering differences for a reliable comparison result.

Finally, we constructed 8 different versions of the AFL++. 
% AFL++ uses the default setting in AFL++.  
AFL++-mopt leverages the MOPT strategy, which utilizes Particle Swarm Optimization (PSO) algorithm to achieve mutation operator schedule.
AFL++redqueen uses the Redqueen strategy, which uses the input-to-state correspondence to resolve the constraints of magic bytes. 
AFL++-mopt-redqueen uses the MOPT strategy and the Redqueen strategy at the same time. 
AFL++-rare sets the power schedule as RARE mode, which mutates inputs to target rare branches in the program.
AFL++-fast sets the power schedule as FAST mode, which pays more attention to exploring low-frequency paths instead of high-frequency paths.
AFL++-exploit sets the power schedule as EXPLOIT mode, which is AFL's exploitation-based constant schedule.

As our proposed strategy can be treated as an independent mutation strategy in AFL++, we can integrate our strategy with other strategies in  AFL++, such as the strategy of Redqueen. \tool{}-redqueen intergates the \tool{} and the Redqueen strategy together. 

Follow Marcel Böhme~\cite{bohme2022reliability}, we ran each fuzzer on all target programs for 24 hours. To avoid the randomness, we repeated the experiment for 10 times.


\subsubsection{Edge Coverage}


\textbf{The edge discovery performance after fuzzing 1/3/6/12/24 hours.}
To evaluate the efficiency of \tool{}-related fuzzers at the beginning of testing, we compared edge discovery performance after fuzzing 1/3/6/12/24 hours. 
For each program, we calculated the average rank for each fuzzer across 10 trails based on edge coverage after fuzzing 1/3/6/12/24 hours. The lower the rank is, the better the fuzzer performs. Then, we plot the performance of each fuzzer at five time points using violin plots. 

The results are shown in Figure~\ref{average_ranks}. The performance of most fuzzers at different time points is not significantly different.
\tool{} and \tool{}-redqueen achieve better new edge coverage on most programs than other fuzzers after fuzzing 1/3/6/12/24 hours. 
Specifically, The median of \tool{}-redqueen performed best at all five timing, and the second best fuzzer is \tool{}. Thus, \tool{}-related fuzzers can find more edge coverage in the shorter limited time budget.


\begin{figure*}[htbp]
\includegraphics[width=\linewidth]{images/average_ranks.png}
\caption{
The violin plot of average edge ranks across 10 trails of different fuzzers running for 1/3/6/12/24 hours.\zhu{UNIFUZZ}}
\label{average_ranks}
\end{figure*}


% \textbf{The analysis of the statistical significance.}
% To avoid statistical errors, We further evaluate all 7 fuzzers using Mann-Whitney U tests. More specifically, we calculate the p-values among all fuzzers regarding the edge coverage for all programs across all campaigns. P-values represent how different two fuzzers are and quantify how significant these differences are. If p $<$ 0.05, we believe that there exists a significant difference. The results are shown in Table X. Cells with a green shade represent that the edge coverage found by the corresponding two \tool{}-related fuzzers is statistically different. Based on the results of the p-value, \tool{} performs significantly better than AFL++, AFL++-fast , AFL++-rare , AFL++-exploit , AFL++-mopt, AFL++-redqueen and AFL++-mopt-redqueen on XX, XX, XX, and XX real-world programs, which performs best among all fuzzers. But \tool{}-redqueen performs significantly better than \tool{} on X real-world programs. Thus, The combiation of these two modes are efficient for the target programs that contain a lot of magic number problems.


\subsubsection{Overhead}
\tool{} requires collecting the information of the length mutators used and removing the redundant mutated positions to get a minimal mutation set. Moreover, our mode scheduler needs to determine the next mode to be used after each mutation. Thus, the extra approaches used by \tool{} might have an effect on fuzzing throughput. 
In order to quantify the influence, we measured the total throughput of all 7 fuzzers on 16 programs after fuzzing 24 hours. The results are shown in Figure~\ref{throughput}. Specifically, the total throughput of two \tool{}-related fuzzers (\tool{}-redqueen and \tool{}) did not drop significantly compared to the throughput of other fuzzers. Surprisingly, the throughput of \tool{} was more than AFL++-MOPT-Redqueen, AFL++-MOPT, AFL++-Exploit and AFL++-Rare on \texttt{tiffsplit} and \texttt{exiv2}. Therefore, our \tool{}-related fuzzers do not introduce a large overhead.



\begin{figure}[htbp]
\includegraphics[width=\linewidth]{images/throughput.png}
\caption{The total throughput of different fuzzers running for 24 hours.\zhu{y axis: \#executions; UNIFUZZ}}
\label{throughput}
\end{figure}




\subsection{Evaluation on MAGMA}
MAGMA is a ground-truth fuzzing benchmark that enables accurate and consistent fuzzer evaluation. MAGMA provides several benchmarks with real bugs by introducing real bugs into real-world programs. Thus, we can perform a realistic evaluation of fuzzers based on MAGMA.
We integrated our \tool{} and \tool{}-redqueen into MAGMA. Then, we evaluated these two \tool{}-related fuzzers and 5 widely-used mutation-based fuzzers(AFL, AFLFast, FairFuzz, MOPT and AFL++) against MAGMA. 
For AFL++, we enabled the MOPT strategy and Redqueen strategy at the same time.
We ran each experiment for 24 hours and repeated 10 times to avoid randomness.

\subsubsection{The number of bugs discovery}
Table~\ref{magma_unique_bugs} shows the mean number of CVEs triggered by each fuzzer. 
Specifically, \tool{} is one of the best fuzzers in 7 out of 9 programs.
\tool{} performed significantly better than all other fuzzers on \texttt{openssl}, \texttt{poppler} and \texttt{sqlite3}. The maximum performance improvement is in \texttt{split3} compared with AFL++, which is about 2x. And \tool{}-redqueen is the only best fuzzer on \texttt{libpng} and \texttt{libtiff}.
In contrast, AFL++ did not find the most bugs in any program. 
% For instance, CVE-2018-1000876 found by both \tool{} and \tool{}-redqueen triggered buffer overflow vulnerability in XX, which causes security problems. 
Therefore, \tool{}-related fuzzers focus on mutating valuable positions, which indeed improves the performance of serious vulnerability discovery.


\begin{table}[!t]
\centering
\caption{Average number of bugs found by fuzzers.\zhu{MAGMA}}
\resizebox{\linewidth}{!}{
\begin{threeparttable}
\begin{tabular}{@{\extracolsep{4pt}}cccccccccccc@{}} %crrrrrrrrrrr
\toprule
%\rotatebox{80}{\textbf{Programs}}
\textbf{Programs} & \textbf{\tool{}}& \textbf{PoR\tnote{1}} &  \textbf{AFL++} & \textbf{AFL} & \textbf{AFLFast} & \textbf{FairFuzz} & \textbf{MOPT}\\
\midrule
libpng    & 1.44 & \textbf{2.56} &   2.22 & 1.89 & 1.00 & 1.56 & 1.56 \\
libsndfile  & \textbf{7.00} & \textbf{7.00} & 6.89 & 2.89 & 2.33 & 1.44 & 4.78 \\
libtiff   & 5.89 & \textbf{6.33}  &  6.22 & 5.44 & 4.22 & 4.67 & 5.67 \\
libxml2   & \textbf{4.22} & \textbf{4.22}  &  4.00 & 1.00 & 1.89 & 1.00 & 2.78 \\
lua       & \textbf{1.00} & \textbf{1.00}  &  0.56 & \textbf{1.00} & \textbf{1.00} & 0.89 & \textbf{1.00} \\
openssl    & \textbf{4.00} & 3.56 &  2.67 & 3.11 & 3.33 & 2.44 & 3.00 \\
php        & \textbf{3.00} & 2.56 &  2.00 & \textbf{3.00} & \textbf{3.00} & 2.56 & \textbf{3.00} \\
poppler    & \textbf{5.56} & 5.44 &  4.33 & 3.00 & 3.44 & 2.22 & 3.44 \\
sqlite3    & \textbf{4.56} & 3.78 &  2.56 & 0.89 & 1.78 & 0.89 & 0.67 \\
\midrule
\#The Most & \textbf{7} & 5 & 0 & 2 & 2 & 0 & 2\\
% \#The Sum & \textbf{36.67} & 36.45 & 31.45 & 22.22 & 21.99 & 17.67 & 25.9\\

\bottomrule
\end{tabular}
\begin{tablenotes}[para]
\item[1]PoR: \tool-Redqueen;
\end{tablenotes}
\end{threeparttable}
}
\label{magma_unique_bugs}
\end{table}

\subsubsection{Time to Bug}
We also analyzed the time that each bug was found and the results are shown in the Table~\ref{TTB}. 
In 10 trails, a total of 48 bugs were found by these 7 fuzzers. Among them, \tool{} performed the best, with a total of 46 bugs found. And \tool{} has the least TTB on 20 programs compared with others. Additionally, among the bugs discovered by \tool{}, there are 7 bugs that cannot be explored by AFL++, MOPT, FairFuzz, AFL and AFLFast.
Among the fuzzers used for comparison, AFL++ performed the best, finding 40 bugs. 
However, \tool{} found 25 bugs more than 2 $\times$ faster than AFL++.
The biggest advantage of \tool{} over AFL++, MOPT, FairFuzz, AFL and AFLFast is to extract valuable positions from the explored constraints to guide subsequent mutations.
Therefore, \tool{} can find more bugs in less time and solve the constraints of hard-to-cover branches.

\begin{table}[!t]
\centering
\caption{The time to bug (TTB) of fuzzers.\zhu{MAGMA}}
\resizebox{\linewidth}{!}{
\begin{threeparttable}
\begin{tabular}{@{\extracolsep{4pt}}crrrrrrrrrrr@{}}
\toprule
% \rotatebox{80}{\textbf{Vulnerabilities}}
\rotatebox{0}{\textbf{Vulnerabilities}} & \rotatebox{60}{\textbf{\tool{}}}  & \rotatebox{60}{\textbf{PoR\tnote{1}}} & \rotatebox{60}{\textbf{AFL++}} & \rotatebox{60}{\textbf{MOPT}} & \rotatebox{60}{\textbf{FairFuzz}}  &  \rotatebox{60}{\textbf{AFL}} & \rotatebox{60}{\textbf{AFLFast}} \\
\midrule

\rowcolor{gray!20} CVE-2015-8472 & 17s & 19s & 23s & \textbf{15s} & \textbf{15s} & \textbf{15s} & \textbf{15s} \\ 
CVE-2016-1762 & 47s & 56s & 1m & \textbf{15s} & 20s & 16s & 18s \\
\rowcolor{gray!20} CVE-2018-13988 & 1m & \textbf{52s} & 1m & \textbf{52s} & 2m & 1m & 1m \\
CVE-2016-2109 & 3m & 3m & 4m & \textbf{1m} & 2m & \textbf{1m} & 2m \\
\rowcolor{gray!20} CVE-2016-6309 & 4m & 5m & 5m & \textbf{1m} & 2m & \textbf{1m} & \textbf{1m} \\
CVE-2016-10270 & \textbf{23s} & 33s & 48s & 19m & 3m & 23m & 11m \\
\rowcolor{gray!20} CVE-2016-3658 & \textbf{4m} & 7m & 17m & 1h & 25m & 1h & 1h \\
CVE-2018-14883 & 18m & 16m & 1h & 3m & 2h & \textbf{2m} & 3m \\
\rowcolor{gray!20} CVE-2017-6892 & \textbf{13m} & 30m & 32m & 33m & 3h & \textbf{13m} & 1h \\
SND017 & \textbf{4m} & 8m & 5m & 25m & 21h & 38m & 5m \\
\rowcolor{gray!20} CVE-2017-11613 & \textbf{9m} & 14m & 1h & 1h & 15h & 6h & 4h \\
CVE-2019-11034 & 6h & 15h & 15h & \textbf{1m} & 8m & 2m & \textbf{1m} \\
\rowcolor{gray!20} PDF010 & 3h & 2h & 1h & 7h & 16h & 10h & \textbf{2m} \\
CVE-2019-7663 & \textbf{3h} & \textbf{3h} & 8h & 4h & 9h & 16h & 6h \\
\rowcolor{gray!20} CVE-2019-20218 & \textbf{49m} & 1h & 2h & 16h & 11h & 9h & 9h \\
CVE-2019-9638 & \textbf{41m} & 5h & 17h & 7h & 17h & 4h & 44m \\
\rowcolor{gray!20} CVE-2015-8317 & 22m & \textbf{21m} & 1h & 3h & - & - & 12h \\
CVE-2019-7310 & 7h & \textbf{5h} & 17h & 9h & 15h & 7h & 8h \\
\rowcolor{gray!20} CVE-2020-15945 & 5h & 5h & \textbf{4h} & 14h & 15h & 13h & 16h \\
SND020 & \textbf{16m} & 17m & 19m & 7h & 21h & - & - \\
\rowcolor{gray!20} CVE-2015-3414 & \textbf{1h} & \textbf{1h} & 4h & 17h & 16h & 23h & 15h \\
CVE-2016-10269 & 2h & \textbf{44m} & 1h & 15h & 22h & 15h & - \\
\rowcolor{gray!20} CVE-2011-2696 & 18m & \textbf{17m} & 22m & 17h & - & 22h & 23h \\
CVE-2017-8363 & \textbf{13m} & 14m & 28m & 18h & 22h & - & - \\
\rowcolor{gray!20} CVE-2017-8363 & 27m & \textbf{25m} & 32m & 18h & 22h & - & - \\
CVE-2017-9047 & 33m & \textbf{28m} & 6h & 12h & - & - & - \\
\rowcolor{gray!20} CVE-2017-8361 & \textbf{14m} & 15m & 3h & 18h & 22h & - & - \\
CVE-2016-6302 & 9h & 18h & 23h & 16h & - & \textbf{3h} & 6h \\
\rowcolor{gray!20} CVE-2017-7375 & 6h & 5h & \textbf{1h} & - & - & - & - \\
CVE-2018-10768 & 5h & \textbf{4h} & 5h & 23h & - & - & 23h \\
\rowcolor{gray!20} CVE-2016-5314 & 19h & 15h & 19h & 11h & 16h & \textbf{4h} & - \\
CVE-2013-6954 & 13h & 15h & 19h & 16h & 12h & \textbf{11h} & - \\
\rowcolor{gray!20} CVE-2019-19926 & \textbf{5h} & 6h & 19h & 17h & - & 21h & 20h \\
PNG006 & - & 8m & \textbf{6m} & - & - & - & - \\
\rowcolor{gray!20} CVE-2016-2108 & \textbf{3h} & 6h & 16h & 22h & - & - & - \\
CVE-2016-10269 & 23h & \textbf{2h} & \textbf{2h} & 22h & - & - & - \\
\rowcolor{gray!20} CVE-2017-9865 & 8h & \textbf{7h} & 12h & - & - & - & - \\
CVE-2015-8784 & 22h & 23h & 21h & 20h & \textbf{18h} & - & 20h \\
\rowcolor{gray!20} CVE-2016-1836 & \textbf{22h} & \textbf{22h} & 23h & - & - & - & - \\
CVE-2017-14617 & - & - & \textbf{21h} & - & - & - & - \\
\rowcolor{gray!20} CVE-2017-3735 & 20h & - & - & \textbf{5h} & 15h & 22h & 10h \\
CVE-2017-9776 & 19h & \textbf{15h} & - & - & - & - & - \\
\rowcolor{gray!20} CVE-2013-7443 & \textbf{17h} & 21h & - & - & - & - & - \\
CVE-2019-19880 & \textbf{18h} & 22h & - & - & - & - & - \\
\rowcolor{gray!20} PDF008 & \textbf{20h} & 21h & - & - & - & - & - \\
CVE-2019-19646 & 22h & \textbf{21h} & - & - & - & - & - \\
\rowcolor{gray!20} CVE-2017-2518 & \textbf{22h} & - & - & - & - & - & - \\
CVE-2019-19317 & \textbf{22h} & - & - & - & - & - & - \\
\rowcolor{gray!50}\#The Fastest & 20 & 15 & 5 & 7 & 2 & 8 & 4 \\



\bottomrule
\end{tabular}
\begin{tablenotes}[para]
\item[1]PoR: \tool-Redqueen;
\end{tablenotes}
\end{threeparttable}
}
\label{TTB}
\end{table}

% \subsubsection{Survival functions}
% We also show the probability of a bug surviving a 24 hours fuzzing trial of four programs generated by MAGMA, which is shown in fig.X. Dotted lines and solid lines indicate the survival functions for reached bugs and triggered bugs, respectively, and the shaded regions are confidence intervals. As the bug’s probability of survival decreases to 0 fastest, \tool{}-redqueen is the best fuzzer on these four programs.




% \begin{table}[!t]
% \centering
% \caption{Edge Rank.}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{@{\extracolsep{4pt}}lrrrrrrrrrrr@{}}
% \toprule

% \textbf{Time} &  \textbf{all} & \textbf{history}& \textbf{new} & \textbf{mopt} & \textbf{exploit} & \textbf{fast} & \textbf{raw} & \textbf{rare} & \textbf{compare}\\
% \midrule
% \textbf{1 hour} & 2.4   &   2.2  & 4.4  & 6.9   &   6.4 &  5.3  & 5.3&   7.2  &    4.4 \\
% \textbf{3 hours} & 2.4   &   2.2  & 4.4  & 6.9   &   6.4 &  5.3  & 5.3&   7.2  &    4.4 \\
% \textbf{6 hours} & 3.0   &   2.3  & 4.9  & 7.0   &   6.3  & 4.8  & 4.9 &  7.4   &   4.3\\
% \textbf{12 hours} & 2.8  &    2.4  & 4.9 &  6.6    &  6.3  & 4.9 &  5.3  & 7.1    &  4.6\\
% \textbf{24 hours} & 2.8  &    2.4  & 4.9 &  6.6    &  6.3  & 4.9 &  5.3  & 7.1    &  4.6\\

% \bottomrule
% \end{tabular}
% }
% \label{edge_rank_for_unifuzz}
% \end{table}




\subsection{Verification Experiment}
We further compared \tool{} with inference-based fuzzers to verify that the positions identified by Pozzer are more critical. The existing inference-based fuzzers have found many bugs in the real-world programs. They can find positions related to path constraints through simple instrumentation or lightweight inference methods. In this section, we performed a fine-grained analysis on the importance of the inferred positions.
% To verify that the positions identified by Pozzer are more critical, we compare Pozzer with GreyOne and ProFuzzer. 

\textbf{Fuzzers.}
Since neither GreyOne nor ProFuzzer is open source, we implemented their core algorithms to identify the related positions of path constraints, as follows:
\begin{itemize}
  \item [1)]
  ProFuzzer: ProFuzzer iterates over all 256 values at each position. If the path length changes relative to the initial seed while trying a certain value, the current position is related to path constraints, and ProFuzzer will not try any other remaining values to speed up the analysis.
  \item [2)] 
  GreyOne: Greyone tries to mutate 8 times at each position. If the variable value in cmps changes, the current position is related to path constraints.
\end{itemize}

\textbf{Experiment Setup.}
We randomly selected 10 target programs and some initial seeds for experiments under UNIFUZZ. To facilitate the comparison of effects, we analyzed each initial seed separately, and the specific experimental steps are as follows. For an initial seed s, we used Pozzer/Greyone/ProFuzzer to mutate the target seed for 3 hours respectively, and count the additional analysis time required by each fuzzer and the number of new edges they found. In particular, for the convenience of comparison, we did not update the seed queue, but continuously mutated the selected initial seed.

\textbf{Metric.} 
We propose the following three new metrics for fine-grained analysis of the above fuzzers:
\begin{itemize}
  \item [1)]
  Average analysis time: The analysis time required by each fuzzer on a seed. The shorter the analysis time, the higher the efficiency. ProFuzzer and Greyone need to set up a pilot stage for inference, so we take the time spent in the pilot stage as their analysis time. Although Pozzer does not contain a pilot stage, the de-redundancy operation will bring some additional program execution when analyzing the extracted mutation information. Therefore, for Pozzer, we counted the sum of the time to analyze all the mutation information as the analysis time.
  \item [2)] 
  The proportion of useful position: If a position is inferred and finds a new edge in the subsequent mutation process, it is called a useful position. We counted the proportion of useful positions in each fuzzer's inferred positions.
  \zhu{68\%(55/82): \tool{} inferred 82 positions, where 55 positions can be mutated to discover new edges after they have been retained as a shared position.}
  \item [3)] 
  The average number of useful mutations: If a mutation finds a new edge, then this mutation is considered a useful mutation. We use the number of useful mutations of each position to describe the importance of each position. If a position has more useful mutations, its importance is higher, and vice versa. Finally, we count the average number of useful mutations among inferred positions.
\end{itemize}

\textbf{Result.}
We only counted seeds that could complete the analysis within three hours. In particular, Pozzer could complete the analysis of all seeds, but GreyOne and ProFuzzer had some long seeds that cannot be analyzed within three hours. The results are shown in the Table~\ref{Verification}.

First, we calculated the average analysis time for each fuzzer. Among them, Pozzer took the shortest time and took 27.47 seconds on average. Then, Greyone and ProFuzzer took 26000 seconds and 21127 seconds, respectively. It can be seen that since Pozzer does not require a pilot stage, especially under long seeds, the analysis efficiency of Pozzer is much higher than that of Greyone and ProFuzzer.

We analyzed the average number of effective mutations for each Fuzzer at 1,000,000 mutations. Pozzer performed best, and its average proportion of useful position was up to 70.5\%. Moreover, Pozzer's average number of useful mutations was up to 3.715. The proportion of useful position and average number of useful mutations of GreyOne were only 16.1\% and 0.947, while that of ProFuzzer were only 17.8\% and 0.0887.
According to the above experimental results, Pozzer can find more essential positions under the premise of shorter analysis time.



% \begin{table*}[!t]
% \centering
% \caption{The Result of SHAP Analysis. We extract the most important positions based on the data collected from 48 hours fuzzing campaigns. Top$N$\% means that the top N\% of the most important positions. $X$mins means fuzzing $X$ mins. And the value in the table represent the ratio at which the positions collected in common features after fuzzing X mins and the top N\% of the most important positions intersect. The higher the value, the better the performance. And the Baseline means that we randomly select positions into common features.}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{@{\extracolsep{4pt}}lrrrrrrrrrrr@{}}
% \toprule

% \textbf{Time} &  \textbf{Top10\%} & \textbf{Top20\%}& \textbf{Top30\%} & \textbf{Top40\%} & \textbf{Top50\%} & \textbf{Top60\%} & \textbf{Top70\%} & \textbf{Top80\%} & \textbf{Top90\%} & \textbf{Top100\%} & \textbf{Baseline}\\
% \midrule
% \textbf{10mins}  &0.67 &   0.59  &  0.55  &  0.52  &  0.49 &   0.46  &  0.44  &  0.42   & 0.40  &   0.38   &   0.07 \\
% \textbf{20mins}  & 0.77  &  0.71  &  0.68  &  0.65   & 0.62   & 0.60  &  0.58 &   0.56  &  0.54   &  0.52    &  0.14 \\
% \textbf{30mins}  & 0.81 &   0.76  &  0.73   & 0.71   & 0.68  &  0.67  &  0.64  &  0.63  &  0.61    & 0.59     & 0.17 \\
% \textbf{40mins}  & 0.83  &  0.79  &  0.77  &  0.75  &  0.72  &  0.71 &   0.69  &  0.67  &  0.65  &   0.63   &   0.18 \\
% \textbf{50mins}  & 0.85  &  0.81  &  0.79  &  0.78  &  0.75  &  0.73   & 0.71  &  0.69  &  0.68   &  0.66    &  0.19 \\
% \textbf{60mins}  & 0.86  &  0.83   & 0.81  &  0.79  &  0.77  &  0.75   & 0.73   & 0.71  &  0.70   &  0.68   &   0.20 \\
% \textbf{70mins}  & 0.87  &  0.84 &   0.82  &  0.81  &  0.78  &  0.77   & 0.75  &  0.73   & 0.72   &  0.70   &   0.20 \\
% \textbf{80mins}  & 0.88  &  0.85  &  0.83  &  0.82  &  0.80  &  0.78   & 0.76  &  0.75  &  0.73  &   0.71 &     0.20 \\
% \textbf{90mins}  & 0.88  &  0.86  &  0.84  &  0.83  &  0.81   & 0.79   & 0.78  &  0.76  &  0.74  &   0.73   &   0.21 \\
% \textbf{100mins}  & 0.88  &  0.86  &  0.85  &  0.84  &  0.81   & 0.80   & 0.78  &  0.77 &   0.75   &  0.73    &  0.21 \\
% \textbf{110mins}  & 0.89  &  0.87  &  0.85 &   0.84  &  0.82   & 0.81  &  0.79  &  0.78  &  0.76  &   0.74  &    0.21 \\
% \textbf{120mins}  & 0.90  &  0.87  &  0.86 &   0.85   & 0.83  &  0.82  &  0.80 &   0.79&    0.77 &    0.75   &   0.23 \\


% \bottomrule
% \end{tabular}
% }
% \label{shap}
% \end{table*}




\begin{table*}[!t]
% \renewcommand\arraystretch{1.7}
% \newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
\centering
\caption{Verification Experiment Result.\zhu{UNIFUZZ}}
\resizebox{\linewidth}{!}{
\begin{threeparttable}
\begin{tabular}{@{\extracolsep{4pt}}lccccccccccccccc@{}}
\toprule
\multirow{3}{*}{\textbf{Programs}} & \multicolumn{3}{c}{\textbf{GreyOne}} & \multicolumn{3}{c}{\textbf{ProFuzzer}} & \multicolumn{3}{c}{\textbf{Pozzer}}\\
\cline{2-4} \cline{5-7} \cline{8-10}


&\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Analysis}\\ \textbf{Time(s)}\end{tabular}} 
&\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Useful}\\ \textbf{Ratio}\end{tabular}} 
&\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Average Useful}\\ \textbf{Mutation}\end{tabular}} 

&\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Analysis}\\ \textbf{Time(s)}\end{tabular}} 
&\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Useful}\\ \textbf{Ratio}\end{tabular}} 
&\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Average Useful}\\ \textbf{Mutation}\end{tabular}} 

&\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Analysis}\\ \textbf{Time(s)}\end{tabular}} 
&\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Useful}\\ \textbf{Ratio}\end{tabular}} 
&\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Average Useful}\\ \textbf{Mutation}\end{tabular}} \\
&&&&&&&&&\\
\midrule

\textbf{nm} & 16721 & 3\%(135/4834) & 0.11 & 13584 & 16\%(109/665) & 0.32 & \textbf{16.68} & \textbf{67\%(55/82)} & \textbf{1.87}  \\
\textbf{tiff2bw} & 8283 & 13\%(101/762) & 0.74 & 9372 & 14\%(106/762) & 0.75 & \textbf{7} & \textbf{89\%(74/83)} & \textbf{5.87}\\
\textbf{tiffsplit} & 8875 & 68\%(104/152) & 3.18 & 10894 & 69\%(104/150) & 3.25 & \textbf{8} & \textbf{92\%(72/78)} & \textbf{6.60}\\
\textbf{objdump} & 52080 & 2\%(205/13288) & 0.45 & 29901 & 18\%(318/1794) & 0.68 & \textbf{45} & \textbf{60\%(179/299)} & \textbf{1.70} \\
\textbf{readelf} & 16739 & 3\%(99/3798) & 0.41 & 13712 & 7\%(186/2641) & 0.48 & \textbf{37} & \textbf{83\%(95/114)} & \textbf{8.70}\\
\textbf{flvmeta} & 2262 & 46\%(29/63) & 1.28 & 2222 & 22\%(42/187) & 0.46 & \textbf{2} & \textbf{40\%(14/35)} & \textbf{1.08}\\
\textbf{pdftotext} & 54447 & 3\%(267/8384) & 0.07 & 38144 & 4\%(337/8805) & 0.08 & \textbf{54} & \textbf{54\%(165/305)} & \textbf{1.11}\\
\textbf{mp42aac} & 11855 & 19\%(124/651) & 0.32 & 17234 & 21\%(132/614) & 0.35 & \textbf{9} & \textbf{68\%(69/102)} & \textbf{1.70}\\
\textbf{tcpdump} & 13219 & 2\%(88/4075) & 2.89 & 13774 & 3\%(87/2708) & 2.48 & \textbf{16} & \textbf{77\%(72/93)} & \textbf{6.36}\\
\textbf{lame3.99.5} & 75520 & 1\%(169/13077) & 0.02 & 62433 & 1\%(179/13060) & 0.02 & \textbf{80} & \textbf{73\%(74/102)} & \textbf{2.16}\\

% \textbf{size}\\
% \textbf{infotocap}\\
% \textbf{sqlite3}\\
% \textbf{imginfo}\\
% \textbf{jq}\\
% \textbf{mujs}\\

\bottomrule
\end{tabular}
\end{threeparttable}
}
\label{Verification}
\end{table*}



==> obsolete/evaluation-1.0.tex <==
\section{Evaluation}

\zhu{Remember to change our fuzzer name in figures, accordingly.}

% \zhu{current experiments: \begin{itemize}
%     % \item UNIFUZZ: edge discovery: time to edges => move to appendix
%     \item UNIFUZZ: edge rank
%     % \item UNIFUZZ: bug discovery: \#bugs => move to appendix
%     \item UNIFUZZ: overhead
%     % \item UNIFUZZ: \tool{} vs EMS: \#edges => move to appendix?
%     \item MAGMA: \#bugs
%     \item MAGMA: time to bugs
%     \item proportion of useful positions
% \end{itemize}}

% \todo{contents \begin{itemize}
%     \item research questions
%     \item edge discovery \begin{itemize}
%         \item 
%     \end{itemize}
%     \item bug discovery
%     \item effective of selected positions
% \end{itemize}}

We implement our \tool{} based on AFL++~\cite{aflpp}, which integrates many state-of-the-art fuzzing algorithms. We mainly modify the mutation process and the byte schedule. During fuzzing, the mutation that discovers new local edges will be additionally analyzed to extract the valuable positions. When selecting bytes, instead of randomly mutating the entire input, \tool{} prefers mutating valuable positions of seeds.
% \zhu{a bit more info about the implementation, like which part do you change in afl++.}
% \zkp{We mainly make the following two changes to AFL++: First, during the fuzzing process, the mutation that found the local new edge will be additionally analyzed to extract the valuable positions. 
% Second, we modify the byte schedule. Instead of randomly mutating the entire input, \tool{} pays more attention to mutating valuable positions of seeds.}
In the evaluation, we evaluate our vanilla \tool{} and \tool-Redqueen that enables both \tool{} and Redqueen in AFL++. Redqueen~\cite{redqueen} extracts constant strings to pass path constraints.
Due to the limit of pages, we show more experiment results in appendix.


% In order to evaluate \tool{}, we implemented \tool{} based on AFL++, which has integrated many fuzzing strategies. 
% To reduce the influence of subjective factors, we conduct our experiments on a third-party testing platform.



\subsection{Experimental Setup}
To ensure the fair results, we conduct our experiments on two third-party testing platforms, UNIFUZZ~\cite{unifuzz} and MAGMA~\cite{magma}. Our experiments are performed on a system running Ubuntu 18.04 with 103 cores (Intel(R) Xeon(R) Gold 6230R CPU) and 256 GB of memory. Each fuzzer uses one CPU core to run one target program. All experiments run for 24 hours and repeat 10 times to avoid the randomness of fuzzing~\cite{bohme2022reliability}.
We use \textit{afl-showmap} in AFL++ to count the number of edges and compile target programs with ASAN~\cite{asan} enabled. When analyzing unique bugs, we use the top-three rule to de-duplicate bugs~\cite{Klees2018Evaluating}.

\textbf{Benchmark Fuzzers.}
We compare \tool{} with the state-of-the-art CGFs, including AFL~\cite{afl}, AFL++~\cite{aflpp}, AFLFast~\cite{aflfast}, FairFuzz~\cite{fairfuzz}, MOPT~\cite{MOPT}, and EMS~\cite{ems}.
AFL is a popular fuzzer that is the basis of many other recent fuzzers~\cite{aflfast, fairfuzz, MOPT, Yue2020EcoFuzz, ems, neuzz}. 
AFL++ is a framework that integrates many state-of-the-art fuzzers into AFL, such as MOPT, AFLfast and Redqueen. AFLFast models fuzzing process as Markov chain and prioritizes low-frequency paths to achieve better code coverage. FairFuzz proposes a novel mutation mask to guide fuzzing towards rare branches. MOPT utilizes Particle Swarm Optimization to optimize the schedule of mutation operators based on fuzzing history. EMS proposes a probabilistic byte orientation model based on the information of intra- and inter-trial history. Note that, on UNIFUZZ, the comparing fuzzers are implemented based on AFL++ (except EMS), while on MAGMA, we use the original implementations of those fuzzers.
% Both MOPT and EMS set the option `-L' to 5, which means \zhu{explain what -L mean}.


% We select 5 fuzzers to evaluate our approach. We evaluate our approach with AFL++, MOPT, AFL, AFLFast and FairFuzz.
% \begin{itemize}
%     \item Fioraldi et al. proposed AFL++~\cite{aflpp}, which is a fuzzing framework that includes many fuzzing strategies, including MOPT, Redqueen, AFLfast, etc. AFL++ has achieved outstanding results in the experiments of other papers and the evaluation of third-party  platforms such as Fuzzbench. To better integrate our strategy with other strategies, we implemented \tool{} based on AFL++. Within AFL++, we only need to adjust the parameter settings to allow \tool{} to compare fairly with other fuzzing strategies. Also, comparing within AFL++ avoids the effects of differences in implementation architectures to obtain reliable experimental results. Finally, we use multiple different settings in AFL++ to evaluate.
%     \item MOPT utilizes Particle Swarm Optimization (PSO) algorithm to optimize AFL’s mutation operator schedule based on fuzzing history information. MOPT dynamically generates the distribution for mutators to improve the fuzzing efficiency. All MOPT-related fuzzers sets the parameter '-L'  as 5 in the experiments.
%     \item EMS proposes a probabilistic byte orientation model to capture mutation strategies from intra- and inter-trial history to trigger unique paths and crashes. We use the initial inter-PBOM provided by the EMS source code.
%     Because EMS is implemented on the basis of MOPT, we also sets the parameter '-L'  as 5.
%     \item AFLFast is a widely-used extension of AFL, which models fuzzing process as Markov chain and prioritizes exploring those low-frequency paths to achieve better code coverage. 
%     \item FairFuzz proposes a novel mutation mask creation algorithm to guide mutations to be biased towards producing inputs triggering rare branches.
%     \item AFL, the American Fuzzy Lop, is one of the most famous fuzzers, which has discovered many bugs in real-world applications. 
% \end{itemize}



\textbf{Initial Seeds.}
For each target program, all fuzzers use the same initial seeds, which are collected from UNIFUZZ, FuzzBench\cite{fuzzbench}, MAGMA or public seed corpus. 
% Following the guidance of Adrian Herrera~\cite{herrera2021seed}, most target programs have multiple initial seeds instead of a single one.
Most target programs have multiple initial seeds as suggested by Adrian Herrera~\cite{herrera2021seed}.




% \textbf{Evaluation Metrics.}
% As the different implementations in different fuzzers, we need uniform evaluation metrics to evaluate fuzzers’ performance. Following the guidance in Marcel Böhme~\cite{bohme2022reliability}, we mainly use the following two metrics. 

% The first one is edge coverage which is widely used in recent research to evaluate fuzzers. 
% % Specifically, the edge coverage is only used when evaluating based on UNIFUZZ.
% When we compare \tool{} with other settings in AFL++, we do not need to leverage other tools to collect the edge coverage because we have the same low-level implementation. Thus, we use the internal tool \textit{afl-showmap} of AFL++ to calculate the edge coverage. 
% When we compare \tool{} with EMS, we also utilize the \textit{afl-showmap} of AFL++ to uniformly calculate edge coverage.
% % When we use the edge coverage, we only compare \tool{} with the other fuzzing strategies in AFL++.

% The second one is the number of unique vulnerabilities, which directly indicates the performance of fuzzer. More specifically, We use ASan to de-duplicate vulnerabilities and analyze the number of unique vulnerabilities discovered by a fuzzer in each trial. Specifically, We use the top three function calls in the output report generated by ASAN to de-duplicate vulnerabilities. 

\subsection{Evaluation on UNIFUZZ}

UNIFUZZ is an open-source, holistic, and pragmatic platform to evaluate fuzzers fairly. 
% UNIFUZZ provides 20 real-world benchmark programs with multiple initial seeds. 
As shown in Table~\ref{programsUNIFUZZ}, we use 12 open-source programs from UNIFUZZ and select 4 other programs to improve the diversity of target programs.
As for the fuzzers, we use 5 modes of AFL++ that implement the benchmark fuzzers. Of the 5 modes, AFL++-Fast stands for AFLFast, AFL++-MOPT for MOPT, AFL++-Exploit for AFL, and AFL++-Rare for FairFuzz. We also selected AFL++-MOPT-Redqueen that enables both MOPT and Redqueen. 


\begin{table}[!t]
% \renewcommand\arraystretch{1}
\centering
\caption{Target programs from UNIFUZZ.}\label{programsUNIFUZZ}
\resizebox{\linewidth}{!}{
\begin{threeparttable}
\begin{tabular}{llll}
    \toprule
    \textbf{Targets} & \textbf{Projects} & \textbf{Input formats} & \textbf{Test instructions} \\ \midrule
    \textbf{tiff2bw\tnote{2}} & \multirow{3}{*}{libtiff 3.9.7} & \multirow{3}{*}{tiff} & tiff2bw @@\tnote{1}~{ } /dev/null \\
    \textbf{tiffsplit} &&& tiffsplit @@ /dev/null\\
    \textbf{tiff2pdf\tnote{2}} &&& tiff2pdf @@ /dev/null\\
    \midrule
    \multirow{3}{*}{\textbf{nm}} & \multirow{6}{*}{binutils-2.28} & \multirow{4}{*}{ELF} & (-A -a -l -S -s \\
    &&&\ \ \ --special-syms --synthetic\\
    &&&\ \ \ --with-symbol-versions -D @@) \\
    \textbf{objdump} &&& -S @@ \\
    \textbf{readelf\tnote{2}} &&& -a @@ \\
    \textbf{size\tnote{2}} &&& @@ \\
    \midrule
    \textbf{pdftotext} & pdftotext 4.00 & pdf & @@ /dev/null \\
    \midrule
    \textbf{infotocap} & jasper 2.0.12 & text & -o /dev/null @@ \\
    \midrule
    \textbf{mp42aac} & Bento4 1.5.1-628 & mp4 & @@ /dev/null \\
    \midrule
    \multirow{2}{*}{\textbf{tcpdump}}
     & tcpdump 4.8.1 + & \multirow{2}{*}{tcpdump100} & \multirow{2}{*}{-e -vv -nr @@} \\
     & libpcap 1.8.1 && \\
    \midrule
    \textbf{flvmeta} & flvmeta 1.2.1 & flv &  @@ \\
    \midrule
    \textbf{lame3.99.5} & lame 3.99.5 & wav & @@ /dev/null \\
    \midrule
    \textbf{imginfo} & ncurses 6.1 & jpg & -f @@ \\
    \midrule
    \textbf{mujs} & mujs 1.0.2 & js & @@ \\
    \midrule
    \textbf{exiv2} & exiv2 0.26 & jpg & @@ \\
    \bottomrule
\end{tabular}
\begin{tablenotes}
\item[1] @@: A placeholder indicating that the input is a file.
\item[2] \textbf{tiff2bw, tiff2pdf, readelf} and \textbf{size} are not from UNIFUZZ
\end{tablenotes}
\end{threeparttable}

}
\end{table}

% Following the guidance of Marcel Böhme~\cite{bohme2022reliability}, we should avoid the situation that the observed improvements may be mainly due to design and engineering differences. Thus, we integrated our strategy into AFL++ and evaluated \tool{} with the other strategies in AFL++, which minimizes engineering differences for a reliable comparison result.

% Finally, we constructed 5 different versions of the AFL++. 
% % AFL++ uses the default setting in AFL++.  
% AFL++-mopt leverages the MOPT strategy, which utilizes Particle Swarm Optimization algorithm to achieve mutation operator schedule.
% AFL++redqueen uses the Redqueen strategy, which uses the input-to-state correspondence to resolve the constraints of magic bytes. 
% AFL++-mopt-redqueen uses the MOPT strategy and the Redqueen strategy at the same time. 
% AFL++-rare (FairFuzz) sets the power schedule as RARE mode, which mutates inputs to target rare branches in the program.
% AFL++-fast (AFLFast) sets the power schedule as FAST mode, which pays more attention to exploring low-frequency paths instead of high-frequency paths.
% AFL++-exploit (AFL) sets the power schedule as EXPLOIT mode, which is AFL's exploitation-based constant schedule.
% As our proposed strategy can be treated as an independent mutation strategy in AFL++, we can integrate our strategy with other strategies in  AFL++, such as the strategy of Redqueen. \tool{}-redqueen intergates the \tool{} and the Redqueen strategy together. 

% Follow Marcel Böhme~\cite{bohme2022reliability}, we ran each fuzzer on all target programs for 24 hours. To avoid the randomness, we repeated the experiment for 10 times.


\textbf{Edge Coverage.}
To evaluate the efficiency of edge discovery, we evaluate fuzzers by using the ranks of edge discovery after fuzzing 1/3/6/12/24 hours. The lower the rank is, the better the fuzzer performs. As shown in Figure~\ref{average_ranks}, the performance of most fuzzers at different running hours is not significantly different.
Yet, Figure~\ref{average_ranks} indicates that \tool{} and \tool{}-Redqueen achieve better code coverage on most programs than other fuzzers.
Specifically, the median of \tool{}-redqueen performs the best among all fuzzers, and the second best is \tool{}.
% \zkp{
We focus on the analysis of the four strongest fuzzers, namely \tool{}, \tool{}-Redqueen, AFL++-MOPT and AFL++-MOPT-Redqueen.
After fuzzing 6 hours, the median ranks of \tool{} and AFL++-MOPT are 2.25 and 4.93, respectively. This indicates that \tool{}'s strategy is more efficient than MOPT. After combining Redqueen's strategy, the median of ranks of \tool{}-Redqueen and AFL++-MOPT-Redqueen are 1.63 and 3.00, respectively.
Our \tool{}-Redqueen performs better than AFL++-MOPT-Redqueen in terms of edge discovery.
% }


% \zhu{Can you provide detailed data of the rank? something like, the median of rank of \tool{} is N\% higher than AFL++-MOPT. The same for all the following descriptions.}

% % \textbf{The edge discovery performance after fuzzing 1/3/6/12/24 hours.}
% To evaluate the efficiency of \tool{}-related fuzzers at the beginning of testing, we compare edge discovery performance after fuzzing 1/3/6/12/24 hours. 
% For each program, we calculate the average rank for each fuzzer across 10 trails based on edge coverage after fuzzing 1/3/6/12/24 hours. The lower the rank is, the better the fuzzer performs. Then, we plot the performance of each fuzzer at five time points using violin plots. 

% The results are shown in Figure~\ref{average_ranks}. The performance of most fuzzers at different time points is not significantly different.
% \tool{} and \tool{}-redqueen achieve better new edge coverage on most programs than other fuzzers after fuzzing 1/3/6/12/24 hours. 
% Specifically, The median of \tool{}-redqueen performs the best at all five timing, and the second best fuzzer is \tool{}. Thus, \tool{}-related fuzzers can find more edge coverage in the shorter limited time budget.


\begin{figure*}[t!]
\includegraphics[width=\linewidth]{images/average_ranks.png}
\caption{The violin plot of average edge ranks across 10 trails of different fuzzers after running for 1/3/6/12/24 hours. \tool{} and \tool-Redqueen rank the highest in terms of edge discovery.}
\label{average_ranks}
\end{figure*}


% \textbf{The analysis of the statistical significance.}
% To avoid statistical errors, We further evaluate all 7 fuzzers using Mann-Whitney U tests. More specifically, we calculate the p-values among all fuzzers regarding the edge coverage for all programs across all campaigns. P-values represent how different two fuzzers are and quantify how significant these differences are. If p $<$ 0.05, we believe that there exists a significant difference. The results are shown in Table X. Cells with a green shade represent that the edge coverage found by the corresponding two \tool{}-related fuzzers is statistically different. Based on the results of the p-value, \tool{} performs significantly better than AFL++, AFL++-fast , AFL++-rare , AFL++-exploit , AFL++-mopt, AFL++-redqueen and AFL++-mopt-redqueen on XX, XX, XX, and XX real-world programs, which performs best among all fuzzers. But \tool{}-redqueen performs significantly better than \tool{} on X real-world programs. Thus, The combiation of these two modes are efficient for the target programs that contain a lot of magic number problems.


\textbf{Overhead.}
\tool{} adds some extra steps to AFL++, including tracing mutators, recovering mutators, inferring related bytes, and scheduling grouped bytes. Thus, to quantify the influence of these steps on fuzzing throughput (\ie execution speed), we measure the total number of executions for each fuzzer. Figure~\ref{throughput} shows the total number of executions of all 16 programs that fuzzers run after 24 hours.
The results show that the throughput of \tool{}-Redqueen and \tool{} does not drop significantly comparing to other fuzzers.
% \tool{} requires collecting the information of the length mutators used and removing the redundant mutated positions to get a minimal mutation set. Moreover, our mode scheduler needs to determine the next mode to be used after each mutation. Thus, the extra approaches used by \tool{} might have an effect on fuzzing throughput. In order to quantify the influence, we measured the total throughput of all 7 fuzzers on 16 programs after fuzzing 24 hours. The results are shown in Figure~\ref{throughput}. Specifically, the total throughput of two \tool{}-related fuzzers (\tool{}-Redqueen and \tool{}) did not drop significantly compared to the throughput of other fuzzers.
% \zkp{
After fuzzing 24 hours, the throughput of \tool{} is lower than that of AFL++-MOPT, AFL++-MOPT-Redqueen, AFL++-Exploit and AFL++-Fast by 6.16\%, 7.91\%, 10.25\%, 8.38\%, respectively.
However, the total throughput of \tool{} and \tool{}-Redqueen are higher than AFL++-Rare by 9.75\% and 13.41\%, respectively.
% }
Surprisingly, on programs \texttt{tiffsplit} and \texttt{exiv2}, the throughput of \tool{} is higher than AFL++-MOPT-Redqueen, AFL++-MOPT, AFL++-Exploit and AFL++-Rare. 
Therefore, our \tool{}-related fuzzers do not introduce much overhead.

\textbf{\tool{} vs. EMS.}
Because some programs will occupy tens of GB of memory when tested by EMS (implementation issues of EMS), we run experiments with part of the programs on Table~\ref{programsUNIFUZZ}. To ensure data consistency, we use \textit{afl-showmap} of AFL++ to count the number of edges for EMS and \tool{}.
The results of edge coverage discovered by \tool{} and EMS are shown in the Figure~\ref{tool_vs_ems}. 
Except for the program \texttt{lame}, \tool{} performs better than EMS.
% \zkp{
Specifically, the median of edge coverage discovered by \tool{} is higher than EMS by 6.78\%, 27.89\%, 16.10\%, 9.01\%, 43.13\%, 16.57\%, 2.37\%, 15.51\%, 5.00\%, 9.38\% and 3.27\% on \texttt{imginfo}, \texttt{infotocap}, \texttt{mp42aac}, \texttt{mujs}, \texttt{objdump228}, \texttt{pdftotext}, \texttt{size}, \texttt{exiv2}, \texttt{tiff2bw}, \texttt{tiff2pdf} and \texttt{tiffsplit}, respectively.
% }



% We also compare \tool{} with EMS~\cite{ems}, which captures mutation strategies from intra- and inter-trial history to improve the fuzzing efficiency. Because some programs will occupy tens of GB of memory when tested by EMS, we only experiment with part of the programs. 
% To ensure data consistency, we uniformly used the afl-showmap of AFL++ to count edge coverage.
% We plotted the performance of \tool{} and EMS on the edge coverage, and the results are shown in the Figure~\ref{tool_vs_ems}.
% \tool{} achieved the best edge discovery performance in almost all target programs. 
% Except for \texttt{lame}, the mean of \tool{} is higher than EMS, especially on \texttt{mujs}, \texttt{mp42aac}, \texttt{objdump}, \texttt{pdftotext} and \texttt{exiv2}. Thus, \tool{} has more potential in edge discovery than EMS.

\begin{figure}[t!]
\includegraphics[width=\linewidth]{images/tool_vs_ems.png}
\caption{The boxplot of edge coverage for \tool{} and EMS. Y-axis: the number of discovered edges.}
\label{tool_vs_ems}
\end{figure}

\begin{figure}[t!]
\includegraphics[width=\linewidth]{images/throughput.png}
\caption{The total throughput of different fuzzers running for 24 hours.}
\label{throughput}
\end{figure}


\subsection{Evaluation on MAGMA}


\begin{table}[!t]
% \renewcommand\arraystretch{1}
\centering
\caption{Target programs from MAGMA.}\label{programsMAGMA}
\resizebox{\linewidth}{!}{
\begin{threeparttable}
\begin{tabular}{llll}
    \toprule
    \textbf{Projects} & \textbf{Target Programs} & \textbf{Input format}\\ \midrule
    % \multirow{2}{*}{\textbf{libpng 1.6.38}} & \multirow{2}{*}{read$\_$fuzzer, readpng} & \multirow{2}{*}{PNG}\\
    \textbf{libpng 1.6.38} & libpng\_read\_fuzzer & PNG\\
    \midrule
    \textbf{libtiff 4.1.0} & read\_rgba\_fuzzer, tiffcp & TIFF\\
    \midrule
    \multirow{2}{*}{\textbf{libxml2 2.9.10}} & \multirow{2}{*}{\makecell[c]{libxml2\_xml\_read\_memory\_fuzzer, \\ xmllint}} & \multirow{2}{*}{XML}\\
    &&\\
    \midrule
    \textbf{poppler 0.88.0} & pdf\_fuzzer, pdfimages & PDF\\
    \midrule
    \multirow{3}{*}{\textbf{openssl 3.0.0}} & \multirow{3}{*}{\makecell[c]{asn1, asn1parse, bignum, server, \\ client, x509}} & \multirow{3}{*}{Binary blobs}\\
    &&\\
    &&\\
    \midrule
    \textbf{sqlite3 3.32.0} & sqlite3\_fuzz & SQL queries\\
    \midrule
    \multirow{2}{*}{\textbf{php 8.8.0}} & \multirow{2}{*}{\makecell[c]{exif, json, parser, \\ unserialize}} & \multirow{2}{*}{Various}\\
    &&\\
    \midrule
    \textbf{libsndfile } & sndfile\_fuzzer & WAV\\
    \midrule
    \textbf{lua } & lua & LUA\\
    \bottomrule
\end{tabular}
\end{threeparttable}

}
\end{table}

MAGMA is a ground-truth fuzzing benchmark that enables accurate and consistent fuzzing evaluation. MAGMA provides several benchmarks with real-world bugs, and it can perform a realistic evaluation of fuzzers.
We integrate our \tool{} and \tool{}-Redqueen into MAGMA, and compare them to 5 widely-used mutation-based fuzzers (\ie AFL, AFLFast, FairFuzz, MOPT and AFL++-MOPT-Redqueen). AFL++-MOPT-Redqueen is the AFL++ that enables both MOPT and Redqueen. Due to configure issues of MAGMA, we use the original implementations of fuzzers rather than the implementations based on AFL++. Table~\ref{programsMAGMA} shows the target programs used in MAGMA.


% . Then, we evaluate these two \tool{}-related fuzzers and 5 widely-used mutation-based fuzzers (\ie AFL, AFLFast, FairFuzz, MOPT and FL++-MOPT-Redqueen) against MAGMA. For AFL++-MOPT-Redqueen, we enabled both MOPT strategy and Redqueen strategy at the same time in AFL++.
% We ran each experiment for 24 hours and repeated 10 times to avoid randomness.
% \zhu{Due to configure issues, Magma uses the original implementations of fuzzers rather than implementations based on AFL++.}



\textbf{Bug Discovery.}
Table~\ref{magma_unique_bugs} shows the number of CVEs triggered by each fuzzer on average. 
It shows that \tool{} performs the best on MAGMA in terms of bug discovery on average.
\tool{} exposes the most bugs on 7 of 9 programs, and \tool{}-redqueen exposes the most bugs on 5 of 9 programs.  
% \zkp{
Specifically, \tool{} performs the best on \texttt{libsndfile}, \texttt{libxml2}, \texttt{lua}, \texttt{openssl}, \texttt{php}, \texttt{poppler} and \texttt{sqlite3}, exposing 7.00, 4.22, 1.00, 4.00, 3.00, 5.56 and 4.56 bugs on average, respectively.
\tool{}-Redqueen performs the best on \texttt{libpng}, \texttt{libsndfile}, \texttt{libtiff}, \texttt{libxml2} and \texttt{lua}, finding 2.56, 7.00, 6.33, 4.22 and 1.00 bugs on average, respectively.
% }
Moreover, \tool{} performs significantly better than all the other fuzzers on \texttt{openssl}, \texttt{poppler} and \texttt{sqlite3}.
On \texttt{split3}, \tool{} discovers almost two times of bugs comparing to AFL++-MOPT-Redqueen. 
Surprisingly, AFL++-MOPT-Redqueen does not outperform other fuzzers on any program.



% The maximum performance improvement is in \texttt{split3} compared with AFL++-MOPT-Redqueen, which is about 2x. And \tool{}-redqueen is the only best fuzzer on \texttt{libpng} and \texttt{libtiff}.
% In contrast, AFL++-MOPT-Redqueen did not find the most bugs in any program. 
% % For instance, CVE-2018-1000876 found by both \tool{} and \tool{}-redqueen triggered buffer overflow vulnerability in XX, which causes security problems. 
% Therefore, \tool{}-related fuzzers focus on mutating valuable positions, which indeed improves the performance of serious vulnerability discovery.


\begin{table}[!t]
\centering
\caption{The average number of bugs found by fuzzers (on MAGMA).}
\resizebox{\linewidth}{!}{
\begin{threeparttable}
\begin{tabular}{@{\extracolsep{4pt}}cccccccccccc@{}} %crrrrrrrrrrr
\toprule
%\rotatebox{80}{\textbf{Programs}}
\textbf{Programs} & \textbf{\tool{}}& \textbf{ContR\tnote{1}} &  \textbf{AMR\tnote{2}} & \textbf{AFL} & \textbf{AFLFast} & \textbf{FairFuzz} & \textbf{MOPT}\\
\midrule
libpng    & 1.44 & \textbf{2.56} &   2.22 & 1.89 & 1.00 & 1.56 & 1.56 \\
libsndfile  & \textbf{7.00} & \textbf{7.00} & 6.89 & 2.89 & 2.33 & 1.44 & 4.78 \\
libtiff   & 5.89 & \textbf{6.33}  &  6.22 & 5.44 & 4.22 & 4.67 & 5.67 \\
libxml2   & \textbf{4.22} & \textbf{4.22}  &  4.00 & 1.00 & 1.89 & 1.00 & 2.78 \\
lua       & \textbf{1.00} & \textbf{1.00}  &  0.56 & \textbf{1.00} & \textbf{1.00} & 0.89 & \textbf{1.00} \\
openssl    & \textbf{4.00} & 3.56 &  2.67 & 3.11 & 3.33 & 2.44 & 3.00 \\
php        & \textbf{3.00} & 2.56 &  2.00 & \textbf{3.00} & \textbf{3.00} & 2.56 & \textbf{3.00} \\
poppler    & \textbf{5.56} & 5.44 &  4.33 & 3.00 & 3.44 & 2.22 & 3.44 \\
sqlite3    & \textbf{4.56} & 3.78 &  2.56 & 0.89 & 1.78 & 0.89 & 0.67 \\
\midrule
\#The Most & \textbf{7} & 5 & 0 & 2 & 2 & 0 & 2\\
% \#The Sum & \textbf{36.67} & 36.45 & 31.45 & 22.22 & 21.99 & 17.67 & 25.9\\

\bottomrule
\end{tabular}
\begin{tablenotes}[para]
\item[1]ContR: \tool-Redqueen; \item[2]AMR: AFL++-MOPT-Redqueen;
\end{tablenotes}
\end{threeparttable}
}
\label{magma_unique_bugs}
\end{table}


\textbf{Time to Bug.}
We analyze the first time that each bug is found and the results are shown in the Table~\ref{TTB}. 
In 10 trails, a total of 48 bugs are found by these 7 fuzzers. Among them, \tool{} performs the best, with a total of 46 discovered bugs. 
Additionally, among the bugs discovered by \tool{}, 7 bugs cannot be exposed by AFL++-MOPT-Redqueen, MOPT, FairFuzz, AFL and AFLFast.
As for TTB, \tool{} has the least time to bug (TTB) on 20 programs, which is the best performance among fuzzers.
% Among the fuzzers used for comparison, AFL++-MOPT-Redqueen performed the best, finding 40 bugs. 
For example, for 25 bugs, \tool{} discovers them 2$\times$ faster than AFL++-MOPT-Redqueen.
% \zkp{
Note that, \texttt{CVE-2017-2518} and \texttt{CVE-2019-19317} can only be discovered by \tool{}.
\texttt{CVE-2017-9776}, \texttt{CVE-2013-7443}, \texttt{CVE-2019-19880}, \texttt{PDF008} and \texttt{CVE-2019-19646} can only be exposed by \tool{} and \tool{}-Redqueen.
% }
Due to the advantage of solving path constraints, \tool{} exposes bugs in less time than others.

% The biggest advantage of \tool{} over AFL++-MOPT-Redqueen, MOPT, FairFuzz, AFL and AFLFast is to extract valuable positions from the explored constraints to guide subsequent mutations.
% Therefore, \tool{} can find more bugs in less time and solve the constraints of hard-to-cover branches.

\begin{table}[!t]
\centering
\caption{The time to bug (TTB) of fuzzers (on MAGMA).}
\resizebox{\linewidth}{!}{
\begin{threeparttable}
\begin{tabular}{@{\extracolsep{4pt}}crrrrrrrrrrr@{}}
\toprule
% \rotatebox{80}{\textbf{Vulnerabilities}}
\rotatebox{0}{\textbf{Vulnerabilities}} & \rotatebox{60}{\textbf{\tool{}}}  & \rotatebox{60}{\textbf{ContR\tnote{1}}} & \rotatebox{60}{\textbf{AMR\tnote{1}}} & \rotatebox{60}{\textbf{MOPT}} & \rotatebox{60}{\textbf{FairFuzz}}  &  \rotatebox{60}{\textbf{AFL}} & \rotatebox{60}{\textbf{AFLFast}} \\
\midrule

\rowcolor{gray!20} CVE-2015-8472 & 17s & 19s & 23s & \textbf{15s} & \textbf{15s} & \textbf{15s} & \textbf{15s} \\ 
CVE-2016-1762 & 47s & 56s & 1m & \textbf{15s} & 20s & 16s & 18s \\
\rowcolor{gray!20} CVE-2018-13988 & 1m & \textbf{52s} & 1m & \textbf{52s} & 2m & 1m & 1m \\
CVE-2016-2109 & 3m & 3m & 4m & \textbf{1m} & 2m & \textbf{1m} & 2m \\
\rowcolor{gray!20} CVE-2016-6309 & 4m & 5m & 5m & \textbf{1m} & 2m & \textbf{1m} & \textbf{1m} \\
CVE-2016-10270 & \textbf{23s} & 33s & 48s & 19m & 3m & 23m & 11m \\
\rowcolor{gray!20} CVE-2016-3658 & \textbf{4m} & 7m & 17m & 1h & 25m & 1h & 1h \\
CVE-2018-14883 & 18m & 16m & 1h & 3m & 2h & \textbf{2m} & 3m \\
\rowcolor{gray!20} CVE-2017-6892 & \textbf{13m} & 30m & 32m & 33m & 3h & \textbf{13m} & 1h \\
SND017 & \textbf{4m} & 8m & 5m & 25m & 21h & 38m & 5m \\
\rowcolor{gray!20} CVE-2017-11613 & \textbf{9m} & 14m & 1h & 1h & 15h & 6h & 4h \\
CVE-2019-11034 & 6h & 15h & 15h & \textbf{1m} & 8m & 2m & \textbf{1m} \\
\rowcolor{gray!20} PDF010 & 3h & 2h & 1h & 7h & 16h & 10h & \textbf{2m} \\
CVE-2019-7663 & \textbf{3h} & \textbf{3h} & 8h & 4h & 9h & 16h & 6h \\
\rowcolor{gray!20} CVE-2019-20218 & \textbf{49m} & 1h & 2h & 16h & 11h & 9h & 9h \\
CVE-2019-9638 & \textbf{41m} & 5h & 17h & 7h & 17h & 4h & 44m \\
\rowcolor{gray!20} CVE-2015-8317 & 22m & \textbf{21m} & 1h & 3h & - & - & 12h \\
CVE-2019-7310 & 7h & \textbf{5h} & 17h & 9h & 15h & 7h & 8h \\
\rowcolor{gray!20} CVE-2020-15945 & 5h & 5h & \textbf{4h} & 14h & 15h & 13h & 16h \\
SND020 & \textbf{16m} & 17m & 19m & 7h & 21h & - & - \\
\rowcolor{gray!20} CVE-2015-3414 & \textbf{1h} & \textbf{1h} & 4h & 17h & 16h & 23h & 15h \\
CVE-2016-10269 & 2h & \textbf{44m} & 1h & 15h & 22h & 15h & - \\
\rowcolor{gray!20} CVE-2011-2696 & 18m & \textbf{17m} & 22m & 17h & - & 22h & 23h \\
CVE-2017-8363 & \textbf{13m} & 14m & 28m & 18h & 22h & - & - \\
\rowcolor{gray!20} CVE-2017-8363 & 27m & \textbf{25m} & 32m & 18h & 22h & - & - \\
CVE-2017-9047 & 33m & \textbf{28m} & 6h & 12h & - & - & - \\
\rowcolor{gray!20} CVE-2017-8361 & \textbf{14m} & 15m & 3h & 18h & 22h & - & - \\
CVE-2016-6302 & 9h & 18h & 23h & 16h & - & \textbf{3h} & 6h \\
\rowcolor{gray!20} CVE-2017-7375 & 6h & 5h & \textbf{1h} & - & - & - & - \\
CVE-2018-10768 & 5h & \textbf{4h} & 5h & 23h & - & - & 23h \\
\rowcolor{gray!20} CVE-2016-5314 & 19h & 15h & 19h & 11h & 16h & \textbf{4h} & - \\
CVE-2013-6954 & 13h & 15h & 19h & 16h & 12h & \textbf{11h} & - \\
\rowcolor{gray!20} CVE-2019-19926 & \textbf{5h} & 6h & 19h & 17h & - & 21h & 20h \\
PNG006 & - & 8m & \textbf{6m} & - & - & - & - \\
\rowcolor{gray!20} CVE-2016-2108 & \textbf{3h} & 6h & 16h & 22h & - & - & - \\
CVE-2016-10269 & 23h & \textbf{2h} & \textbf{2h} & 22h & - & - & - \\
\rowcolor{gray!20} CVE-2017-9865 & 8h & \textbf{7h} & 12h & - & - & - & - \\
CVE-2015-8784 & 22h & 23h & 21h & 20h & \textbf{18h} & - & 20h \\
\rowcolor{gray!20} CVE-2016-1836 & \textbf{22h} & \textbf{22h} & 23h & - & - & - & - \\
CVE-2017-14617 & - & - & \textbf{21h} & - & - & - & - \\
\rowcolor{gray!20} CVE-2017-3735 & 20h & - & - & \textbf{5h} & 15h & 22h & 10h \\
CVE-2017-9776 & 19h & \textbf{15h} & - & - & - & - & - \\
\rowcolor{gray!20} CVE-2013-7443 & \textbf{17h} & 21h & - & - & - & - & - \\
CVE-2019-19880 & \textbf{18h} & 22h & - & - & - & - & - \\
\rowcolor{gray!20} PDF008 & \textbf{20h} & 21h & - & - & - & - & - \\
CVE-2019-19646 & 22h & \textbf{21h} & - & - & - & - & - \\
\rowcolor{gray!20} CVE-2017-2518 & \textbf{22h} & - & - & - & - & - & - \\
CVE-2019-19317 & \textbf{22h} & - & - & - & - & - & - \\
\rowcolor{gray!50}\#The Fastest & 20 & 15 & 5 & 7 & 2 & 8 & 4 \\



\bottomrule
\end{tabular}
\begin{tablenotes}[para]
\item[1]ContR: \tool-Redqueen; \item[2]AMR: AFL++-MOPT-Redqueen;
\end{tablenotes}
\end{threeparttable}
}
\label{TTB}
\end{table}

% \subsubsection{Survival functions}
% We also show the probability of a bug surviving a 24 hours fuzzing trial of four programs generated by MAGMA, which is shown in fig.X. Dotted lines and solid lines indicate the survival functions for reached bugs and triggered bugs, respectively, and the shaded regions are confidence intervals. As the bug’s probability of survival decreases to 0 fastest, \tool{}-redqueen is the best fuzzer on these four programs.




% \begin{table}[!t]
% \centering
% \caption{Edge Rank.}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{@{\extracolsep{4pt}}lrrrrrrrrrrr@{}}
% \toprule

% \textbf{Time} &  \textbf{all} & \textbf{history}& \textbf{new} & \textbf{mopt} & \textbf{exploit} & \textbf{fast} & \textbf{raw} & \textbf{rare} & \textbf{compare}\\
% \midrule
% \textbf{1 hour} & 2.4   &   2.2  & 4.4  & 6.9   &   6.4 &  5.3  & 5.3&   7.2  &    4.4 \\
% \textbf{3 hours} & 2.4   &   2.2  & 4.4  & 6.9   &   6.4 &  5.3  & 5.3&   7.2  &    4.4 \\
% \textbf{6 hours} & 3.0   &   2.3  & 4.9  & 7.0   &   6.3  & 4.8  & 4.9 &  7.4   &   4.3\\
% \textbf{12 hours} & 2.8  &    2.4  & 4.9 &  6.6    &  6.3  & 4.9 &  5.3  & 7.1    &  4.6\\
% \textbf{24 hours} & 2.8  &    2.4  & 4.9 &  6.6    &  6.3  & 4.9 &  5.3  & 7.1    &  4.6\\

% \bottomrule
% \end{tabular}
% }
% \label{edge_rank_for_unifuzz}
% \end{table}




% \subsection{Verification Experiment}
\subsection{The Effectiveness of Inferred Positions}
\todo{in progress}

We further analyze whether the valuable positions identified by \tool{} are really efficient. 
Given a seed, we define the \textit{important positions} as the positions that can discover new edges. \zhu{you define important positions, valuable positions, and useful positions. Please be consistent, or make sure they have different meaning.}
Thus, we need to obtain the ground truth of the important positions, and analyze the intersection between the important positions and valuable positions identified by \tool{}.

\textbf{Ground Truth.} 
Due to the complexity of fuzzing, it is difficult to directly analyze the ground truth of important positions.
Thus, we use SHAP analysis to analyze mutation information during fuzzing to obtain ground truth.
SHAP (SHapley Additive exPlanations) \cite{shap} is a game theoretic approach, which is widely used to explain individual predictions. Based on the game theoretically optimal Shapley values, SHAP explains the prediction of an instance by computing the contribution of each feature to the prediction. The following describes how we use SHAP analysis to analyze the important positions of each seed.

First, given a seed, in order to ensure the semantic consistency between seeds to facilitate analysis, we perform fuzzing for 48 hours without using length mutators and trimming. And we maintain a dataset for SHAP analysis.
Second, during the fuzzing process, we collect mutation information of all mutations that discover new edges, including the mutated positions and the number of new edges discovered. The extracted mutation information will be added to dataset.
Third, We try all combinations of mutated positions for each mutation information, and analyze how many new edges can be found for each combination. This characterizes the contribution of each position to the discovered new edges. The above information will be added to dataset.
Fourth, we extract the important positions from dataset based on SHAP analysis.

\textbf{Experiment Setup.}
After obtaining the ground truth of important positions, we perform fuzzing based on a single seed for 2 hours without using length mutators and trimming.
Finally, we perform experiments on \texttt{nm}, \texttt{objdump}, \texttt{readelf}, \texttt{size}, \texttt{strip}, \texttt{tiff2bw}, and \texttt{tiffsplit}.
We analyze the probability of \tool{} extracting the top 1\%, 3\%, 5\%, 7\% and 10\% of important positions at different times respectively.

\textbf{Result.}
The result is shown in the Figure \ref{shap}.
We find that \tool{} outperforms random selection at all times.
For instance, after fuzzing 10 minutes, the probability that \tool{} selects the top 1\%, 3\%, 5\%, 7\%, and 10\% of important positions are 18\%, 28\%, 32\%, 35\%, and 37\%, respectively.


\begin{figure}[t!]
\includegraphics[width=\linewidth]{images/shap.jpg}
\caption{SHAP analysis.}
\label{shap}
\end{figure}

% \zhu{SHAP experiment here.}

% \begin{table*}[!t]
% \centering
% \caption{The Result of SHAP Analysis. We extract the most important positions \zhu{define important positions} based on the data collected from 48 hours fuzzing campaigns. Top$N$\% means that the top N\% of the most important positions. $X$mins means fuzzing $X$ mins. And the value in the table represent the ratio at which the positions collected in common features after fuzzing X mins and the top N\% of the most important positions intersect. The higher the value, the better the performance. And the Baseline means that we randomly select positions into common features.}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{@{\extracolsep{4pt}}lrrrrrrrrrrr@{}}
% \toprule

% \textbf{Time} &  \textbf{Top10\%} & \textbf{Top20\%}& \textbf{Top30\%} & \textbf{Top40\%} & \textbf{Top50\%} & \textbf{Top60\%} & \textbf{Top70\%} & \textbf{Top80\%} & \textbf{Top90\%} & \textbf{Top100\%} & \textbf{Baseline}\\
% \midrule
% \textbf{10mins}  &0.67 &   0.59  &  0.55  &  0.52  &  0.49 &   0.46  &  0.44  &  0.42   & 0.40  &   0.38   &   0.07 \\
% \textbf{20mins}  & 0.77  &  0.71  &  0.68  &  0.65   & 0.62   & 0.60  &  0.58 &   0.56  &  0.54   &  0.52    &  0.14 \\
% \textbf{30mins}  & 0.81 &   0.76  &  0.73   & 0.71   & 0.68  &  0.67  &  0.64  &  0.63  &  0.61    & 0.59     & 0.17 \\
% \textbf{40mins}  & 0.83  &  0.79  &  0.77  &  0.75  &  0.72  &  0.71 &   0.69  &  0.67  &  0.65  &   0.63   &   0.18 \\
% \textbf{50mins}  & 0.85  &  0.81  &  0.79  &  0.78  &  0.75  &  0.73   & 0.71  &  0.69  &  0.68   &  0.66    &  0.19 \\
% \textbf{60mins}  & 0.86  &  0.83   & 0.81  &  0.79  &  0.77  &  0.75   & 0.73   & 0.71  &  0.70   &  0.68   &   0.20 \\
% \textbf{70mins}  & 0.87  &  0.84 &   0.82  &  0.81  &  0.78  &  0.77   & 0.75  &  0.73   & 0.72   &  0.70   &   0.20 \\
% \textbf{80mins}  & 0.88  &  0.85  &  0.83  &  0.82  &  0.80  &  0.78   & 0.76  &  0.75  &  0.73  &   0.71 &     0.20 \\
% \textbf{90mins}  & 0.88  &  0.86  &  0.84  &  0.83  &  0.81   & 0.79   & 0.78  &  0.76  &  0.74  &   0.73   &   0.21 \\
% \textbf{100mins}  & 0.88  &  0.86  &  0.85  &  0.84  &  0.81   & 0.80   & 0.78  &  0.77 &   0.75   &  0.73    &  0.21 \\
% \textbf{110mins}  & 0.89  &  0.87  &  0.85 &   0.84  &  0.82   & 0.81  &  0.79  &  0.78  &  0.76  &   0.74  &    0.21 \\
% \textbf{120mins}  & 0.90  &  0.87  &  0.86 &   0.85   & 0.83  &  0.82  &  0.80 &   0.79&    0.77 &    0.75   &   0.23 \\


% \bottomrule
% \end{tabular}
% }
% \label{shap}
% \end{table*}




==> obsolete/evaluation-1.1.tex <==
\section{Evaluation}

% \zhu{Remember to change our fuzzer name in figures, accordingly.}

% \zhu{current experiments: \begin{itemize}
%     % \item UNIFUZZ: edge discovery: time to edges => move to appendix
%     \item UNIFUZZ: edge rank
%     % \item UNIFUZZ: bug discovery: \#bugs => move to appendix
%     \item UNIFUZZ: overhead
%     % \item UNIFUZZ: \tool{} vs EMS: \#edges => move to appendix?
%     \item MAGMA: \#bugs
%     \item MAGMA: time to bugs
%     \item proportion of useful positions
% \end{itemize}}

% \todo{contents \begin{itemize}
%     \item research questions
%     \item edge discovery \begin{itemize}
%         \item 
%     \end{itemize}
%     \item bug discovery
%     \item effective of selected positions
% \end{itemize}}

We implement our \tool{} based on AFL++~\cite{aflpp}, which integrates many state-of-the-art fuzzing algorithms. We mainly modify the mutation process and the byte schedule. During fuzzing, the mutation that discovers new local edges will be additionally analyzed to extract the valuable positions. When selecting bytes, instead of randomly mutating the entire input, \tool{} prefers mutating valuable positions of seeds.
% \zhu{a bit more info about the implementation, like which part do you change in afl++.}
% \zkp{We mainly make the following two changes to AFL++: First, during the fuzzing process, the mutation that found the local new edge will be additionally analyzed to extract the valuable positions. 
% Second, we modify the byte schedule. Instead of randomly mutating the entire input, \tool{} pays more attention to mutating valuable positions of seeds.}
In the evaluation, we evaluate our vanilla \tool{} and \tool-Redqueen that enables both \tool{} and Redqueen in AFL++. Redqueen~\cite{redqueen} extracts constant strings to pass path constraints.
Due to the limit of pages, we show more experiment results in appendix.


% In order to evaluate \tool{}, we implemented \tool{} based on AFL++, which has integrated many fuzzing strategies. 
% To reduce the influence of subjective factors, we conduct our experiments on a third-party testing platform.



\subsection{Experimental Setup}
To ensure the fair results, we conduct our experiments on two third-party testing platforms, UNIFUZZ~\cite{unifuzz} and MAGMA~\cite{magma}. Our experiments are performed on a system running Ubuntu 18.04 with 103 cores (Intel(R) Xeon(R) Gold 6230R CPU) and 256 GB of memory. Each fuzzer uses one CPU core to run one target program. All experiments run for 24 hours and repeat 10 times to avoid the randomness of fuzzing~\cite{bohme2022reliability}.
We use \textit{afl-showmap} in AFL++ to count the number of edges and compile target programs with ASAN~\cite{asan} enabled. When analyzing unique bugs, we use the top-three rule to de-duplicate bugs~\cite{Klees2018Evaluating}.

\textbf{Benchmark Fuzzers.}
We compare \tool{} with the state-of-the-art CGFs, including AFL~\cite{afl}, AFL++~\cite{aflpp}, AFLFast~\cite{aflfast}, FairFuzz~\cite{fairfuzz}, MOPT~\cite{MOPT}, and EMS~\cite{ems}.
AFL is a popular fuzzer that is the basis of many other recent fuzzers~\cite{aflfast, fairfuzz, MOPT, Yue2020EcoFuzz, ems, neuzz}. 
AFL++ is a framework that integrates many state-of-the-art fuzzers into AFL, such as MOPT, AFLfast and Redqueen. AFLFast models fuzzing process as Markov chain and prioritizes low-frequency paths to achieve better code coverage. FairFuzz proposes a novel mutation mask to guide fuzzing towards rare branches. MOPT utilizes Particle Swarm Optimization to optimize the schedule of mutation operators based on fuzzing history. EMS proposes a probabilistic byte orientation model based on the information of intra- and inter-trial history. Note that, on UNIFUZZ, the comparing fuzzers are implemented based on AFL++ (except EMS), while on MAGMA, we use the original implementations of those fuzzers.
% Both MOPT and EMS set the option `-L' to 5, which means \zhu{explain what -L mean}.


% We select 5 fuzzers to evaluate our approach. We evaluate our approach with AFL++, MOPT, AFL, AFLFast and FairFuzz.
% \begin{itemize}
%     \item Fioraldi et al. proposed AFL++~\cite{aflpp}, which is a fuzzing framework that includes many fuzzing strategies, including MOPT, Redqueen, AFLfast, etc. AFL++ has achieved outstanding results in the experiments of other papers and the evaluation of third-party  platforms such as Fuzzbench. To better integrate our strategy with other strategies, we implemented \tool{} based on AFL++. Within AFL++, we only need to adjust the parameter settings to allow \tool{} to compare fairly with other fuzzing strategies. Also, comparing within AFL++ avoids the effects of differences in implementation architectures to obtain reliable experimental results. Finally, we use multiple different settings in AFL++ to evaluate.
%     \item MOPT utilizes Particle Swarm Optimization (PSO) algorithm to optimize AFL’s mutation operator schedule based on fuzzing history information. MOPT dynamically generates the distribution for mutators to improve the fuzzing efficiency. All MOPT-related fuzzers sets the parameter '-L'  as 5 in the experiments.
%     \item EMS proposes a probabilistic byte orientation model to capture mutation strategies from intra- and inter-trial history to trigger unique paths and crashes. We use the initial inter-PBOM provided by the EMS source code.
%     Because EMS is implemented on the basis of MOPT, we also sets the parameter '-L'  as 5.
%     \item AFLFast is a widely-used extension of AFL, which models fuzzing process as Markov chain and prioritizes exploring those low-frequency paths to achieve better code coverage. 
%     \item FairFuzz proposes a novel mutation mask creation algorithm to guide mutations to be biased towards producing inputs triggering rare branches.
%     \item AFL, the American Fuzzy Lop, is one of the most famous fuzzers, which has discovered many bugs in real-world applications. 
% \end{itemize}



\textbf{Initial Seeds.}
For each target program, all fuzzers use the same initial seeds, which are collected from UNIFUZZ, FuzzBench\cite{fuzzbench}, MAGMA or public seed corpus. 
% Following the guidance of Adrian Herrera~\cite{herrera2021seed}, most target programs have multiple initial seeds instead of a single one.
Most target programs have multiple initial seeds as suggested by Adrian Herrera~\cite{herrera2021seed}.




% \textbf{Evaluation Metrics.}
% As the different implementations in different fuzzers, we need uniform evaluation metrics to evaluate fuzzers’ performance. Following the guidance in Marcel Böhme~\cite{bohme2022reliability}, we mainly use the following two metrics. 

% The first one is edge coverage which is widely used in recent research to evaluate fuzzers. 
% % Specifically, the edge coverage is only used when evaluating based on UNIFUZZ.
% When we compare \tool{} with other settings in AFL++, we do not need to leverage other tools to collect the edge coverage because we have the same low-level implementation. Thus, we use the internal tool \textit{afl-showmap} of AFL++ to calculate the edge coverage. 
% When we compare \tool{} with EMS, we also utilize the \textit{afl-showmap} of AFL++ to uniformly calculate edge coverage.
% % When we use the edge coverage, we only compare \tool{} with the other fuzzing strategies in AFL++.

% The second one is the number of unique vulnerabilities, which directly indicates the performance of fuzzer. More specifically, We use ASan to de-duplicate vulnerabilities and analyze the number of unique vulnerabilities discovered by a fuzzer in each trial. Specifically, We use the top three function calls in the output report generated by ASAN to de-duplicate vulnerabilities. 

\subsection{Evaluation on UNIFUZZ}

UNIFUZZ is an open-source, holistic, and pragmatic platform to evaluate fuzzers fairly. 
% UNIFUZZ provides 20 real-world benchmark programs with multiple initial seeds. 
As shown in Table~\ref{programsUNIFUZZ}, we use 12 open-source programs from UNIFUZZ and select 4 other programs to improve the diversity of target programs.
As for the fuzzers, we use 5 modes of AFL++ that implement the benchmark fuzzers. Of the 5 modes, AFL++-Fast stands for AFLFast, AFL++-MOPT for MOPT, AFL++-Exploit for AFL, and AFL++-Rare for FairFuzz. We also selected AFL++-MOPT-Redqueen that enables both MOPT and Redqueen. 


\begin{table}[!t]
% \renewcommand\arraystretch{1}
\centering
\caption{Target programs from UNIFUZZ.}\label{programsUNIFUZZ}
\resizebox{\linewidth}{!}{
\begin{threeparttable}
\begin{tabular}{llll}
    \toprule
    \textbf{Targets} & \textbf{Projects} & \textbf{Input formats} & \textbf{Test instructions} \\ \midrule
    \textbf{tiff2bw\tnote{2}} & \multirow{3}{*}{libtiff 3.9.7} & \multirow{3}{*}{tiff} & tiff2bw @@\tnote{1}~{ } /dev/null \\
    \textbf{tiffsplit} &&& tiffsplit @@ /dev/null\\
    \textbf{tiff2pdf\tnote{2}} &&& tiff2pdf @@ /dev/null\\
    \midrule
    \multirow{3}{*}{\textbf{nm}} & \multirow{6}{*}{binutils-2.28} & \multirow{4}{*}{ELF} & (-A -a -l -S -s \\
    &&&\ \ \ --special-syms --synthetic\\
    &&&\ \ \ --with-symbol-versions -D @@) \\
    \textbf{objdump} &&& -S @@ \\
    \textbf{readelf\tnote{2}} &&& -a @@ \\
    \textbf{size\tnote{2}} &&& @@ \\
    \midrule
    \textbf{pdftotext} & pdftotext 4.00 & pdf & @@ /dev/null \\
    \midrule
    \textbf{infotocap} & jasper 2.0.12 & text & -o /dev/null @@ \\
    \midrule
    \textbf{mp42aac} & Bento4 1.5.1-628 & mp4 & @@ /dev/null \\
    \midrule
    \multirow{2}{*}{\textbf{tcpdump}}
     & tcpdump 4.8.1 + & \multirow{2}{*}{tcpdump100} & \multirow{2}{*}{-e -vv -nr @@} \\
     & libpcap 1.8.1 && \\
    \midrule
    \textbf{flvmeta} & flvmeta 1.2.1 & flv &  @@ \\
    \midrule
    \textbf{lame3.99.5} & lame 3.99.5 & wav & @@ /dev/null \\
    \midrule
    \textbf{imginfo} & ncurses 6.1 & jpg & -f @@ \\
    \midrule
    \textbf{mujs} & mujs 1.0.2 & js & @@ \\
    \midrule
    \textbf{exiv2} & exiv2 0.26 & jpg & @@ \\
    \bottomrule
\end{tabular}
\begin{tablenotes}
\item[1] @@: A placeholder indicating that the input is a file.
\item[2] \textbf{tiff2bw, tiff2pdf, readelf} and \textbf{size} are not from UNIFUZZ
\end{tablenotes}
\end{threeparttable}

}
\end{table}

% Following the guidance of Marcel Böhme~\cite{bohme2022reliability}, we should avoid the situation that the observed improvements may be mainly due to design and engineering differences. Thus, we integrated our strategy into AFL++ and evaluated \tool{} with the other strategies in AFL++, which minimizes engineering differences for a reliable comparison result.

% Finally, we constructed 5 different versions of the AFL++. 
% % AFL++ uses the default setting in AFL++.  
% AFL++-mopt leverages the MOPT strategy, which utilizes Particle Swarm Optimization algorithm to achieve mutation operator schedule.
% AFL++redqueen uses the Redqueen strategy, which uses the input-to-state correspondence to resolve the constraints of magic bytes. 
% AFL++-mopt-redqueen uses the MOPT strategy and the Redqueen strategy at the same time. 
% AFL++-rare (FairFuzz) sets the power schedule as RARE mode, which mutates inputs to target rare branches in the program.
% AFL++-fast (AFLFast) sets the power schedule as FAST mode, which pays more attention to exploring low-frequency paths instead of high-frequency paths.
% AFL++-exploit (AFL) sets the power schedule as EXPLOIT mode, which is AFL's exploitation-based constant schedule.
% As our proposed strategy can be treated as an independent mutation strategy in AFL++, we can integrate our strategy with other strategies in  AFL++, such as the strategy of Redqueen. \tool{}-redqueen intergates the \tool{} and the Redqueen strategy together. 

% Follow Marcel Böhme~\cite{bohme2022reliability}, we ran each fuzzer on all target programs for 24 hours. To avoid the randomness, we repeated the experiment for 10 times.


\subsubsection{Edge Coverage}
To evaluate the efficiency of edge discovery, we evaluate fuzzers by using the ranks of edge discovery after fuzzing 1/3/6/12/24 hours. The lower the rank is, the better the fuzzer performs. As shown in Figure~\ref{average_ranks}, the performance of most fuzzers at different running hours is not significantly different.
Yet, Figure~\ref{average_ranks} indicates that \tool{} and \tool{}-Redqueen achieve better code coverage on most programs than other fuzzers.
Specifically, the median of \tool{}-redqueen performs the best among all fuzzers, and the second best is \tool{}.
% \zkp{
We focus on the analysis of the four strongest fuzzers, namely \tool{}, \tool{}-Redqueen, AFL++-MOPT and AFL++-MOPT-Redqueen.
After fuzzing 6 hours, the median ranks of \tool{} and AFL++-MOPT are 2.25 and 4.93, respectively. This indicates that \tool{}'s strategy is more efficient than MOPT. After combining Redqueen's strategy, the median of ranks of \tool{}-Redqueen and AFL++-MOPT-Redqueen are 1.63 and 3.00, respectively.
Our \tool{}-Redqueen performs better than AFL++-MOPT-Redqueen in terms of edge discovery.
% }

% \begin{figure}[t!]
% \includegraphics[width=\linewidth]{images/LinFuzz-p.png}
% \caption{Results of P-values of (\tool{}, other fuzzers) from the Mann-Whitney U-Test.}
% \label{LinFuzz_p}
% \end{figure}

% \begin{figure}[t!]
% \includegraphics[width=\linewidth]{images/LinFuzz-R-p.png}
% \caption{Results of P-values of (\tool{}-Redqueen, other fuzzers) from the Mann-Whitney U-Test.}
% \label{LinFuzz_R_p}
% \end{figure}



\begin{table*}[!t]
% \renewcommand\arraystretch{1.7}
% \newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
\centering
\caption{Results of P-values from the Mann-Whitney U-Test.} \label{tab:valid_percent}
\resizebox{\linewidth}{!}{
\begin{threeparttable}
\begin{tabular}{@{\extracolsep{4pt}}lcrrrrrrrrr@{}}
\toprule
\multirow{3}{*}{\textbf{Program}}  & \multicolumn{5}{c}{\textbf{\tool{}}} & \multicolumn{5}{c}{\textbf{\tool{}-Redqueen}}\\
\cline{2-6} \cline{7-11}


& \textbf{AMR\tnote{1}} & \textbf{AM\tnote{2}} & \textbf{AE\tnote{3}} & \textbf{AF\tnote{4}} & \textbf{AR\tnote{5}} & \textbf{AMR} & \textbf{AM} & \textbf{AE} & \textbf{AF} & \textbf{AR}\\
\midrule
imginfo & 0.0001(-)\tnote{6} & 0.0651(+)\tnote{7} & 0.2698(+) & 0.3667(-) & 0.2363(-) & 0.1131(+) & 0.0002(+) & 0.0004(+) & 0.0002(+) & 0.0018(+) \\
infotocap & 0.2481(+) & 0.0023(+) & 0.0605(+) & 0.3525(+) & 0.0929(-) & 0.0003(+) & 0.0001(+) & 0.0001(+) & 0.0005(+) & 0.0002(+) \\
lame & 0.0814(+) & 0.0766(+) & 0.0884(+) & 0.0054(+) & 0.001(+) & 0.013(+) & 0.0314(+) & 0.0132(+) & 0.0029(+) & 0.0009(+) \\
mp42aac & 0.0001(-) & 0.0001(+) & 0.0006(+) & 0.0012(+) & 0.0005(+) & 0.007(+) & 0.0001(+) & 0.0001(+) & 0.0001(+) & 0.0001(+) \\
mujs & 0.0156(-) & 0.0001(+) & 0.0007(+) & 0.4698(+) & 0.0018(+) & 0.0001(+) & 0.0001(+) & 0.0001(+) & 0.0001(+) & 0.0001(+) \\
nm & 0.0002(-) & 0.0001(+) & 0.0009(+) & 0.0001(+) & 0.0003(+) & 0.0269(+) & 0.0001(+) & 0.0001(+) & 0.0001(+) & 0.0001(+) \\
objdump & 0.0045(-) & 0.0001(+) & 0.0001(+) & 0.0001(+) & 0.0001(+) & 0.0007(+) & 0.0001(+) & 0.0001(+) & 0.0001(+) & 0.0001(+) \\
pdftotext & 0.0106(-) & 0.0029(+) & 0.0007(+) & 0.0009(+) & 0.0003(+) & 0.0188(-) & 0.4251(+) & 0.4549(+) & 0.4399(+) & 0.2363(+) \\
readelf & 0.0004(+) & 0.0001(+) & 0.0001(+) & 0.0001(+) & 0.0001(+) & 0.0086(+) & 0.2363(+) & 0.3957(+) & 0.4849(+) & 0.0128(+) \\
size & 0.0001(-) & 0.0046(+) & 0.0409(+) & 0.0129(+) & 0.0036(+) & 0.0293(+) & 0.0001(+) & 0.0001(+) & 0.0001(+) & 0.0001(+) \\
exiv2 & 0.0001(-) & 0.0004(+) & 0.081(+) & 0.0206(+) & 0.0156(+) & 0.0018(+) & 0.0001(+) & 0.0001(+) & 0.0001(+) & 0.0001(+) \\
tcpdump & 0.0129(-) & 0.0001(+) & 0.0001(+) & 0.0014(+) & 0.0036(+) & 0.0001(+) & 0.0001(+) & 0.0001(+) & 0.0001(+) & 0.0001(+) \\
tiff2bw & 0.0057(+) & 0.0003(+) & 0.0002(+) & 0.0001(+) & 0.0001(+) & 0.0007(+) & 0.0002(+) & 0.0001(+) & 0.0001(+) & 0.0001(+) \\
tiff2pdf & 0.4824(-) & 0.0927(+) & 0.1254(+) & 0.1548(+) & 0.0004(+) & 0.0152(+) & 0.0007(+) & 0.0018(+) & 0.0013(+) & 0.0002(+) \\
tiffsplit & 0.1821(+) & 0.0002(+) & 0.0001(+) & 0.0001(+) & 0.0003(+) & 0.001(+) & 0.0001(+) & 0.0001(+) & 0.0001(+) & 0.0001(+) \\
\bottomrule
\end{tabular}
\begin{tablenotes}[para]
\item[1]AMR: AFL++-MOPT-Redqueen; 
\item[2]AM: AFL++-MOPT;  
\item[3]AE: AFL++-Exploit;
\item[4]AF: AFL++-Fast;
\item[5]AR: AFL++-Rare;
\item[6](-): The average edge coverage of \tool{} on \texttt{imginfo} is lower than that of AMR;
\item[7](+): The average edge coverage of \tool{} on \texttt{imginfo} is higher than that of AM;
\end{tablenotes}
\end{threeparttable}
}
\label{p_values}
\end{table*}

\zkp{
We further conduct a statistical significance analysis to calculate P-values using the Mann-Whitney U-test \cite{mcknight2010mann}. Specifically, we test the edge coverage collected from the ten rounds of experiments by \tool{}-related fuzzers and other fuzzers after 24 hours. P-values can describe whether the performance is significantly different between pairs of fuzzers. P-values less than 0.05 indicate a significant difference. The results are shown in Table~\ref{p_values}. Since the edge coverage found by all fuzzers under \texttt{flvmeta} is consistent, we do not analyze it.

The Mann-Whitney U-test shows that \tool{} performs significantly better than 
AFL++-MOPT, AFL++Exploit, AFL++-Fast, AFL++-Rare, and AFL++-MOPT-Redqueen on on 12, 11, 11, 13, and 2 programs, respectively.
And \tool{}-Redqueen performs significantly better than 
AFL++-MOPT, AFL++Exploit, AFL++-Fast, AFL++-Rare, and AFL++-MOPT-Redqueen on on 13, 13, 13, 14, and 13 programs, respectively.
In addition, \tool{} discover more edges than AFL++-MOPT and AFL++Exploit on all programs. And the average edge coverage of \tool{}-Redqueen is higher than AFL++-MOPT, AFL++Exploit, AFL++-Fast, and AFL++-Rare on all programs.
}



% \textbf{Time to Edge Discovery.}
% Figure~\ref{time_and_edge} illustrates the growth of edge coverage over time that each fuzzer discovers in 24 hours on all 16 programs.
% \tool{}-related fuzzers (\ie \tool{} and \tool{}-Redqueen) achieve better performance on almost all programs in 24 hours.
% The results indicate that the \tool{}-related fuzzers have a steady and stronger growth trend on edge coverage than other fuzzers. For instance, the confidence interval of \tool{}-Redqueen and \tool{} is above other fuzzers on \texttt{tiff2bw} during the fuzzing process.

% \begin{figure*}[t!]
% \centering
% \includegraphics[width=0.95\linewidth]{images/time_and_edge.png}
% \caption{The edge coverage of different fuzzers running for 24 hours (on UNIFUZZ).}
% \label{time_and_edge}
% \end{figure*}



% \zhu{Can you provide detailed data of the rank? something like, the median of rank of \tool{} is N\% higher than AFL++-MOPT. The same for all the following descriptions.}

% % \textbf{The edge discovery performance after fuzzing 1/3/6/12/24 hours.}
% To evaluate the efficiency of \tool{}-related fuzzers at the beginning of testing, we compare edge discovery performance after fuzzing 1/3/6/12/24 hours. 
% For each program, we calculate the average rank for each fuzzer across 10 trails based on edge coverage after fuzzing 1/3/6/12/24 hours. The lower the rank is, the better the fuzzer performs. Then, we plot the performance of each fuzzer at five time points using violin plots. 

% The results are shown in Figure~\ref{average_ranks}. The performance of most fuzzers at different time points is not significantly different.
% \tool{} and \tool{}-redqueen achieve better new edge coverage on most programs than other fuzzers after fuzzing 1/3/6/12/24 hours. 
% Specifically, The median of \tool{}-redqueen performs the best at all five timing, and the second best fuzzer is \tool{}. Thus, \tool{}-related fuzzers can find more edge coverage in the shorter limited time budget.


\begin{figure*}[t!]
\includegraphics[width=\linewidth]{images/average_ranks.png}
\caption{The violin plot of average edge ranks across 10 trails of different fuzzers after running for 1/3/6/12/24 hours. \tool{} and \tool-Redqueen rank the highest in terms of edge discovery.}
\label{average_ranks}
\end{figure*}


% \textbf{The analysis of the statistical significance.}
% To avoid statistical errors, We further evaluate all 7 fuzzers using Mann-Whitney U tests. More specifically, we calculate the p-values among all fuzzers regarding the edge coverage for all programs across all campaigns. P-values represent how different two fuzzers are and quantify how significant these differences are. If p $<$ 0.05, we believe that there exists a significant difference. The results are shown in Table X. Cells with a green shade represent that the edge coverage found by the corresponding two \tool{}-related fuzzers is statistically different. Based on the results of the p-value, \tool{} performs significantly better than AFL++, AFL++-fast , AFL++-rare , AFL++-exploit , AFL++-mopt, AFL++-redqueen and AFL++-mopt-redqueen on XX, XX, XX, and XX real-world programs, which performs best among all fuzzers. But \tool{}-redqueen performs significantly better than \tool{} on X real-world programs. Thus, The combiation of these two modes are efficient for the target programs that contain a lot of magic number problems.



% \subsection{Bug Discovery on UNIFUZZ}
\subsubsection{Bug Discovery on UNIFUZZ}
We analyze the number of unique bugs triggered by a fuzzer based on ASAN. Following the guidance of UNIFUZZ~\cite{unifuzz}, we select the top three stack frames to de-duplicate bugs. 
Table~\ref{unifuzz_bug} shows the number of unique bugs triggered by each fuzzer. \tool{}-Redqueen, \tool{}, AFL++-MOPT, AFL++-Fast, AFL++-Rare, AFL++-Exploit, and AFL++-MOPT-Redqueen trigger 147, 138, 83, 102, 114, 96 and 126 bugs, respectively. 
\tool{}-Redqueen finds the most bugs in 16 programs, with 9 more bugs than \tool{}. This indicates that \tool{} can be integrated with other strategies (\eg Redqueen) in AFL++ and achieves better results.
\tool{} performs the best on 7 programs, including \texttt{lame}, \texttt{tiffsplit}, \texttt{objdump}, \texttt{mp42aac}, \texttt{infotocap}, \texttt{imginfo} and \texttt{tiff2pdf}. \tool{}-Redqueen performs the best on 6 programs, including \texttt{exiv2}, \texttt{flvmeta}, \texttt{tiff2bw}, \texttt{pdftotext}, \texttt{tcpdump} and \texttt{imginfo}. 
Surprisingly, AFL++-MOPT-Redqueen, AFL++-Fast and AFL++-Rare do not perform the best on any program. 
AFL++-MOPT and AFL++-Exploit only perform the best on 1 and 2 programs, respectively.
In summary, \tool{}-related fuzzers perform the best on most of the programs.
The bug discovery experiment results demonstrate the effectiveness of \tool{}. 
% The positions extracted by \tool{} can improve the fuzzing performance.





\begin{table}[!h]
\centering
\caption{Unique bugs discovered by fuzzers (on UNIFUZZ).}
\resizebox{\linewidth}{!}{
\begin{threeparttable}
\begin{tabular}{@{\extracolsep{4pt}}cccccccccccc@{}} %crrrrrrrrrrr
\toprule
% \rotatebox{80}{\textbf{\tool-Redqueen\tnote{1}}}
\textbf{Programs} &  \textbf{LinR\tnote{1}} & \textbf{\tool{}} & \textbf{AMR\tnote{2}} & \textbf{AM\tnote{3}} & \textbf{AE\tnote{4}} & \textbf{AF\tnote{5}} & \textbf{AR\tnote{6}}\\
\midrule
% history_redqueen & history & mopt_redqueen & mopt & exploit & fast & rare \\
lame            &         8.0   &   \textbf{9.0}      &      7.0  & 5.0   &   7.0  & 4.0  & 6.0 \\
readelf228      &         4.0   &   4.0      &      4.0  & 4.0   &   \textbf{5.0}  & 4.0  & 4.0 \\
exiv2           &         \textbf{8.0}   &   6.0      &      4.0  & 4.0   &   3.0  & 5.0  & 5.0 \\
flvmeta         &        \textbf{31.0}   &  18.0      &     23.0  & 3.0   &  15.0 & 15.0 & 14.0 \\
nm228           &         2.0   &   2.0      &      2.0  & 2.0   &   2.0  & 2.0  & 2.0 \\
tiffsplit       &        35.0   &  \textbf{36.0}      &     30.0 & 20.0   &  21.0 & 21.0 & 32.0 \\
tiff2bw         &        \textbf{10.0}   &   7.0      &      9.0  & 7.0   &   5.0  & 7.0  & 5.0 \\
objdump228      &         9.0   &  \textbf{10.0}      &      6.0  & 5.0   &   5.0  & 5.0  & 7.0 \\
pdftotext       &         \textbf{5.0}   &   4.0      &      2.0  & 3.0   &   3.0  & 3.0  & 3.0 \\
mp42aac         &        16.0   &  \textbf{28.0}      &     24.0 & 20.0   &  23.0 & 26.0 & 25.0 \\
tcpdump         &         \textbf{7.0}   &   0.0      &      5.0  & 0.0   &   0.0  & 0.0  & 0.0 \\
infotocap       &         1.0   &   \textbf{2.0}      &      1.0  & 0.0   &   \textbf{2.0}  & 1.0  & \textbf{2.0} \\
imginfo         &        \textbf{11.0}   &  \textbf{11.0}      &      9.0  & 9.0   &   5.0  & 9.0  & 9.0 \\
tiff2pdf        &         0.0   &   \textbf{1.0}      &      0.0  & \textbf{1.0}   &   0.0  & 0.0  & 0.0 \\


\midrule
\textbf{Sum} & \textbf{147.0}  &  138.0 & 126.0  & 83.0  &  96.0 & 102.0  & 114.0\\


\bottomrule
\end{tabular}
\begin{tablenotes}[para]
\item[1]LinR: \tool-Redqueen; \item[2]AMR: AFL++-MOPT-Redqueen; \item[3]AM: AFL++-MOPT; \item[4]AE: AFL++-Exploit; \item[5]AF: AFL++-Fast; \item[6]AR: AFL++-Rare
\end{tablenotes}
\end{threeparttable}
}

\label{unifuzz_bug}
\end{table}



\subsubsection{Overhead}
\tool{} adds some extra steps to AFL++, including tracing mutators, recovering mutators, inferring related bytes, and scheduling grouped bytes. Thus, to quantify the influence of these steps on fuzzing throughput (\ie execution speed), we measure the total number of executions for each fuzzer. Figure~\ref{throughput} shows the total number of executions of all 16 programs that fuzzers run after 24 hours.
The results show that the throughput of \tool{}-Redqueen and \tool{} does not drop significantly comparing to other fuzzers.
% \tool{} requires collecting the information of the length mutators used and removing the redundant mutated positions to get a minimal mutation set. Moreover, our mode scheduler needs to determine the next mode to be used after each mutation. Thus, the extra approaches used by \tool{} might have an effect on fuzzing throughput. In order to quantify the influence, we measured the total throughput of all 7 fuzzers on 16 programs after fuzzing 24 hours. The results are shown in Figure~\ref{throughput}. Specifically, the total throughput of two \tool{}-related fuzzers (\tool{}-Redqueen and \tool{}) did not drop significantly compared to the throughput of other fuzzers.
% \zkp{
After fuzzing 24 hours, the throughput of \tool{} is lower than that of AFL++-MOPT, AFL++-MOPT-Redqueen, AFL++-Exploit and AFL++-Fast by 6.16\%, 7.91\%, 10.25\%, 8.38\%, respectively.
However, the total throughput of \tool{} and \tool{}-Redqueen are higher than AFL++-Rare by 9.75\% and 13.41\%, respectively.
% }
Surprisingly, on programs \texttt{tiffsplit} and \texttt{exiv2}, the throughput of \tool{} is higher than AFL++-MOPT-Redqueen, AFL++-MOPT, AFL++-Exploit and AFL++-Rare. 
Therefore, our \tool{}-related fuzzers do not introduce much overhead.

\subsubsection{\tool{} vs. EMS}
Because some programs will occupy tens of GB of memory when tested by EMS (implementation issues of EMS), we run experiments with part of the programs on Table~\ref{programsUNIFUZZ}. To ensure data consistency, we use \textit{afl-showmap} of AFL++ to count the number of edges for EMS and \tool{}.
The results of edge coverage discovered by \tool{} and EMS are shown in the Figure~\ref{tool_vs_ems}. 
Except for the program \texttt{lame}, \tool{} performs better than EMS.
% \zkp{
Specifically, the median of edge coverage discovered by \tool{} is higher than EMS by 6.78\%, 27.89\%, 16.10\%, 9.01\%, 43.13\%, 16.57\%, 2.37\%, 15.51\%, 5.00\%, 9.38\% and 3.27\% on \texttt{imginfo}, \texttt{infotocap}, \texttt{mp42aac}, \texttt{mujs}, \texttt{objdump228}, \texttt{pdftotext}, \texttt{size}, \texttt{exiv2}, \texttt{tiff2bw}, \texttt{tiff2pdf} and \texttt{tiffsplit}, respectively.
% }



% We also compare \tool{} with EMS~\cite{ems}, which captures mutation strategies from intra- and inter-trial history to improve the fuzzing efficiency. Because some programs will occupy tens of GB of memory when tested by EMS, we only experiment with part of the programs. 
% To ensure data consistency, we uniformly used the afl-showmap of AFL++ to count edge coverage.
% We plotted the performance of \tool{} and EMS on the edge coverage, and the results are shown in the Figure~\ref{tool_vs_ems}.
% \tool{} achieved the best edge discovery performance in almost all target programs. 
% Except for \texttt{lame}, the mean of \tool{} is higher than EMS, especially on \texttt{mujs}, \texttt{mp42aac}, \texttt{objdump}, \texttt{pdftotext} and \texttt{exiv2}. Thus, \tool{} has more potential in edge discovery than EMS.

\begin{figure}[t!]
\includegraphics[width=\linewidth]{images/tool_vs_ems.png}
\caption{The boxplot of edge coverage for \tool{} and EMS. Y-axis: the number of discovered edges.}
\label{tool_vs_ems}
\end{figure}

\begin{figure}[t!]
\includegraphics[width=\linewidth]{images/throughput.png}
\caption{The total throughput of different fuzzers running for 24 hours.}
\label{throughput}
\end{figure}


\subsection{Evaluation on MAGMA}


\begin{table}[!t]
% \renewcommand\arraystretch{1}
\centering
\caption{Target programs from MAGMA.}\label{programsMAGMA}
\resizebox{\linewidth}{!}{
\begin{threeparttable}
\begin{tabular}{llll}
    \toprule
    \textbf{Projects} & \textbf{Target Programs} & \textbf{Input format}\\ \midrule
    % \multirow{2}{*}{\textbf{libpng 1.6.38}} & \multirow{2}{*}{read$\_$fuzzer, readpng} & \multirow{2}{*}{PNG}\\
    \textbf{libpng 1.6.38} & libpng\_read\_fuzzer & PNG\\
    \midrule
    \textbf{libtiff 4.1.0} & read\_rgba\_fuzzer, tiffcp & TIFF\\
    \midrule
    \multirow{2}{*}{\textbf{libxml2 2.9.10}} & \multirow{2}{*}{\makecell[c]{libxml2\_xml\_read\_memory\_fuzzer, \\ xmllint}} & \multirow{2}{*}{XML}\\
    &&\\
    \midrule
    \textbf{poppler 0.88.0} & pdf\_fuzzer, pdfimages & PDF\\
    \midrule
    \multirow{3}{*}{\textbf{openssl 3.0.0}} & \multirow{3}{*}{\makecell[c]{asn1, asn1parse, bignum, server, \\ client, x509}} & \multirow{3}{*}{Binary blobs}\\
    &&\\
    &&\\
    \midrule
    \textbf{sqlite3 3.32.0} & sqlite3\_fuzz & SQL queries\\
    \midrule
    \multirow{2}{*}{\textbf{php 8.8.0}} & \multirow{2}{*}{\makecell[c]{exif, json, parser, \\ unserialize}} & \multirow{2}{*}{Various}\\
    &&\\
    \midrule
    \textbf{libsndfile } & sndfile\_fuzzer & WAV\\
    \midrule
    \textbf{lua } & lua & LUA\\
    \bottomrule
\end{tabular}
\end{threeparttable}

}
\end{table}

MAGMA is a ground-truth fuzzing benchmark that enables accurate and consistent fuzzing evaluation. MAGMA provides several benchmarks with real-world bugs, and it can perform a realistic evaluation of fuzzers.
We integrate our \tool{} and \tool{}-Redqueen into MAGMA, and compare them to 5 widely-used mutation-based fuzzers (\ie AFL, AFLFast, FairFuzz, MOPT and AFL++-MOPT-Redqueen). AFL++-MOPT-Redqueen is the AFL++ that enables both MOPT and Redqueen. Due to configure issues of MAGMA, we use the original implementations of fuzzers rather than the implementations based on AFL++. Table~\ref{programsMAGMA} shows the target programs used in MAGMA.


% . Then, we evaluate these two \tool{}-related fuzzers and 5 widely-used mutation-based fuzzers (\ie AFL, AFLFast, FairFuzz, MOPT and FL++-MOPT-Redqueen) against MAGMA. For AFL++-MOPT-Redqueen, we enabled both MOPT strategy and Redqueen strategy at the same time in AFL++.
% We ran each experiment for 24 hours and repeated 10 times to avoid randomness.
% \zhu{Due to configure issues, Magma uses the original implementations of fuzzers rather than implementations based on AFL++.}



\subsubsection{Bug Discovery}
Table~\ref{magma_unique_bugs} shows the number of CVEs triggered by each fuzzer on average. 
It shows that \tool{} performs the best on MAGMA in terms of bug discovery on average.
\tool{} exposes the most bugs on 7 of 9 programs, and \tool{}-redqueen exposes the most bugs on 5 of 9 programs.  
% \zkp{
Specifically, \tool{} performs the best on \texttt{libsndfile}, \texttt{libxml2}, \texttt{lua}, \texttt{openssl}, \texttt{php}, \texttt{poppler} and \texttt{sqlite3}, exposing 7.00, 4.22, 1.00, 4.00, 3.00, 5.56 and 4.56 bugs on average, respectively.
\tool{}-Redqueen performs the best on \texttt{libpng}, \texttt{libsndfile}, \texttt{libtiff}, \texttt{libxml2} and \texttt{lua}, finding 2.56, 7.00, 6.33, 4.22 and 1.00 bugs on average, respectively.
% }
Moreover, \tool{} performs significantly better than all the other fuzzers on \texttt{openssl}, \texttt{poppler} and \texttt{sqlite3}.
On \texttt{split3}, \tool{} discovers almost two times of bugs comparing to AFL++-MOPT-Redqueen. 
Surprisingly, AFL++-MOPT-Redqueen does not outperform other fuzzers on any program.



% The maximum performance improvement is in \texttt{split3} compared with AFL++-MOPT-Redqueen, which is about 2x. And \tool{}-redqueen is the only best fuzzer on \texttt{libpng} and \texttt{libtiff}.
% In contrast, AFL++-MOPT-Redqueen did not find the most bugs in any program. 
% % For instance, CVE-2018-1000876 found by both \tool{} and \tool{}-redqueen triggered buffer overflow vulnerability in XX, which causes security problems. 
% Therefore, \tool{}-related fuzzers focus on mutating valuable positions, which indeed improves the performance of serious vulnerability discovery.


\begin{table}[!t]
\centering
\caption{The average number of bugs found by fuzzers (on MAGMA).}
\resizebox{\linewidth}{!}{
\begin{threeparttable}
\begin{tabular}{@{\extracolsep{4pt}}cccccccccccc@{}} %crrrrrrrrrrr
\toprule
%\rotatebox{80}{\textbf{Programs}}
\textbf{Programs} & \textbf{\tool{}}& \textbf{LinR\tnote{1}} &  \textbf{AMR\tnote{2}} & \textbf{AFL} & \textbf{AFLFast} & \textbf{FairFuzz} & \textbf{MOPT}\\
\midrule
libpng    & 1.44 & \textbf{2.56} &   2.22 & 1.89 & 1.00 & 1.56 & 1.56 \\
libsndfile  & \textbf{7.00} & \textbf{7.00} & 6.89 & 2.89 & 2.33 & 1.44 & 4.78 \\
libtiff   & 5.89 & \textbf{6.33}  &  6.22 & 5.44 & 4.22 & 4.67 & 5.67 \\
libxml2   & \textbf{4.22} & \textbf{4.22}  &  4.00 & 1.00 & 1.89 & 1.00 & 2.78 \\
lua       & \textbf{1.00} & \textbf{1.00}  &  0.56 & \textbf{1.00} & \textbf{1.00} & 0.89 & \textbf{1.00} \\
openssl    & \textbf{4.00} & 3.56 &  2.67 & 3.11 & 3.33 & 2.44 & 3.00 \\
php        & \textbf{3.00} & 2.56 &  2.00 & \textbf{3.00} & \textbf{3.00} & 2.56 & \textbf{3.00} \\
poppler    & \textbf{5.56} & 5.44 &  4.33 & 3.00 & 3.44 & 2.22 & 3.44 \\
sqlite3    & \textbf{4.56} & 3.78 &  2.56 & 0.89 & 1.78 & 0.89 & 0.67 \\
\midrule
\#The Most & \textbf{7} & 5 & 0 & 2 & 2 & 0 & 2\\
% \#The Sum & \textbf{36.67} & 36.45 & 31.45 & 22.22 & 21.99 & 17.67 & 25.9\\

\bottomrule
\end{tabular}
\begin{tablenotes}[para]
\item[1]LinR: \tool-Redqueen; \item[2]AMR: AFL++-MOPT-Redqueen;
\end{tablenotes}
\end{threeparttable}
}
\label{magma_unique_bugs}
\end{table}


\subsubsection{Time to Bug}
We analyze the first time that each bug is found and the results are shown in the Table~\ref{TTB}. 
In 10 trails, a total of 48 bugs are found by these 7 fuzzers. Among them, \tool{} performs the best, with a total of 46 discovered bugs. 
Additionally, among the bugs discovered by \tool{}, 7 bugs cannot be exposed by AFL++-MOPT-Redqueen, MOPT, FairFuzz, AFL and AFLFast.
As for TTB, \tool{} has the least time to bug (TTB) on 20 programs, which is the best performance among fuzzers.
% Among the fuzzers used for comparison, AFL++-MOPT-Redqueen performed the best, finding 40 bugs. 
For example, for 25 bugs, \tool{} discovers them 2$\times$ faster than AFL++-MOPT-Redqueen.
% \zkp{
Note that, \texttt{CVE-2017-2518} and \texttt{CVE-2019-19317} can only be discovered by \tool{}.
\texttt{CVE-2017-9776}, \texttt{CVE-2013-7443}, \texttt{CVE-2019-19880}, \texttt{PDF008} and \texttt{CVE-2019-19646} can only be exposed by \tool{} and \tool{}-Redqueen.
% }
Due to the advantage of solving path constraints, \tool{} exposes bugs in less time than others.

% The biggest advantage of \tool{} over AFL++-MOPT-Redqueen, MOPT, FairFuzz, AFL and AFLFast is to extract valuable positions from the explored constraints to guide subsequent mutations.
% Therefore, \tool{} can find more bugs in less time and solve the constraints of hard-to-cover branches.

\begin{table}[!t]
\centering
\caption{The time to bug (TTB) of fuzzers (on MAGMA).}
\resizebox{\linewidth}{!}{
\begin{threeparttable}
\begin{tabular}{@{\extracolsep{4pt}}crrrrrrrrrrr@{}}
\toprule
% \rotatebox{80}{\textbf{Vulnerabilities}}
\rotatebox{0}{\textbf{Vulnerabilities}} & \rotatebox{60}{\textbf{\tool{}}}  & \rotatebox{60}{\textbf{LinR\tnote{1}}} & \rotatebox{60}{\textbf{AMR\tnote{1}}} & \rotatebox{60}{\textbf{MOPT}} & \rotatebox{60}{\textbf{FairFuzz}}  &  \rotatebox{60}{\textbf{AFL}} & \rotatebox{60}{\textbf{AFLFast}} \\
\midrule

\rowcolor{gray!20} CVE-2015-8472 & 17s & 19s & 23s & \textbf{15s} & \textbf{15s} & \textbf{15s} & \textbf{15s} \\ 
CVE-2016-1762 & 47s & 56s & 1m & \textbf{15s} & 20s & 16s & 18s \\
\rowcolor{gray!20} CVE-2018-13988 & 1m & \textbf{52s} & 1m & \textbf{52s} & 2m & 1m & 1m \\
CVE-2016-2109 & 3m & 3m & 4m & \textbf{1m} & 2m & \textbf{1m} & 2m \\
\rowcolor{gray!20} CVE-2016-6309 & 4m & 5m & 5m & \textbf{1m} & 2m & \textbf{1m} & \textbf{1m} \\
CVE-2016-10270 & \textbf{23s} & 33s & 48s & 19m & 3m & 23m & 11m \\
\rowcolor{gray!20} CVE-2016-3658 & \textbf{4m} & 7m & 17m & 1h & 25m & 1h & 1h \\
CVE-2018-14883 & 18m & 16m & 1h & 3m & 2h & \textbf{2m} & 3m \\
\rowcolor{gray!20} CVE-2017-6892 & \textbf{13m} & 30m & 32m & 33m & 3h & \textbf{13m} & 1h \\
SND017 & \textbf{4m} & 8m & 5m & 25m & 21h & 38m & 5m \\
\rowcolor{gray!20} CVE-2017-11613 & \textbf{9m} & 14m & 1h & 1h & 15h & 6h & 4h \\
CVE-2019-11034 & 6h & 15h & 15h & \textbf{1m} & 8m & 2m & \textbf{1m} \\
\rowcolor{gray!20} PDF010 & 3h & 2h & 1h & 7h & 16h & 10h & \textbf{2m} \\
CVE-2019-7663 & \textbf{3h} & \textbf{3h} & 8h & 4h & 9h & 16h & 6h \\
\rowcolor{gray!20} CVE-2019-20218 & \textbf{49m} & 1h & 2h & 16h & 11h & 9h & 9h \\
CVE-2019-9638 & \textbf{41m} & 5h & 17h & 7h & 17h & 4h & 44m \\
\rowcolor{gray!20} CVE-2015-8317 & 22m & \textbf{21m} & 1h & 3h & - & - & 12h \\
CVE-2019-7310 & 7h & \textbf{5h} & 17h & 9h & 15h & 7h & 8h \\
\rowcolor{gray!20} CVE-2020-15945 & 5h & 5h & \textbf{4h} & 14h & 15h & 13h & 16h \\
SND020 & \textbf{16m} & 17m & 19m & 7h & 21h & - & - \\
\rowcolor{gray!20} CVE-2015-3414 & \textbf{1h} & \textbf{1h} & 4h & 17h & 16h & 23h & 15h \\
CVE-2016-10269 & 2h & \textbf{44m} & 1h & 15h & 22h & 15h & - \\
\rowcolor{gray!20} CVE-2011-2696 & 18m & \textbf{17m} & 22m & 17h & - & 22h & 23h \\
CVE-2017-8363 & \textbf{13m} & 14m & 28m & 18h & 22h & - & - \\
\rowcolor{gray!20} CVE-2017-8363 & 27m & \textbf{25m} & 32m & 18h & 22h & - & - \\
CVE-2017-9047 & 33m & \textbf{28m} & 6h & 12h & - & - & - \\
\rowcolor{gray!20} CVE-2017-8361 & \textbf{14m} & 15m & 3h & 18h & 22h & - & - \\
CVE-2016-6302 & 9h & 18h & 23h & 16h & - & \textbf{3h} & 6h \\
\rowcolor{gray!20} CVE-2017-7375 & 6h & 5h & \textbf{1h} & - & - & - & - \\
CVE-2018-10768 & 5h & \textbf{4h} & 5h & 23h & - & - & 23h \\
\rowcolor{gray!20} CVE-2016-5314 & 19h & 15h & 19h & 11h & 16h & \textbf{4h} & - \\
CVE-2013-6954 & 13h & 15h & 19h & 16h & 12h & \textbf{11h} & - \\
\rowcolor{gray!20} CVE-2019-19926 & \textbf{5h} & 6h & 19h & 17h & - & 21h & 20h \\
PNG006 & - & 8m & \textbf{6m} & - & - & - & - \\
\rowcolor{gray!20} CVE-2016-2108 & \textbf{3h} & 6h & 16h & 22h & - & - & - \\
CVE-2016-10269 & 23h & \textbf{2h} & \textbf{2h} & 22h & - & - & - \\
\rowcolor{gray!20} CVE-2017-9865 & 8h & \textbf{7h} & 12h & - & - & - & - \\
CVE-2015-8784 & 22h & 23h & 21h & 20h & \textbf{18h} & - & 20h \\
\rowcolor{gray!20} CVE-2016-1836 & \textbf{22h} & \textbf{22h} & 23h & - & - & - & - \\
CVE-2017-14617 & - & - & \textbf{21h} & - & - & - & - \\
\rowcolor{gray!20} CVE-2017-3735 & 20h & - & - & \textbf{5h} & 15h & 22h & 10h \\
CVE-2017-9776 & 19h & \textbf{15h} & - & - & - & - & - \\
\rowcolor{gray!20} CVE-2013-7443 & \textbf{17h} & 21h & - & - & - & - & - \\
CVE-2019-19880 & \textbf{18h} & 22h & - & - & - & - & - \\
\rowcolor{gray!20} PDF008 & \textbf{20h} & 21h & - & - & - & - & - \\
CVE-2019-19646 & 22h & \textbf{21h} & - & - & - & - & - \\
\rowcolor{gray!20} CVE-2017-2518 & \textbf{22h} & - & - & - & - & - & - \\
CVE-2019-19317 & \textbf{22h} & - & - & - & - & - & - \\
\rowcolor{gray!50}\#The Fastest & 20 & 15 & 5 & 7 & 2 & 8 & 4 \\



\bottomrule
\end{tabular}
\begin{tablenotes}[para]
\item[1]LinR: \tool-Redqueen; \item[2]AMR: AFL++-MOPT-Redqueen;
\end{tablenotes}
\end{threeparttable}
}
\label{TTB}
\end{table}

% \subsubsection{Survival functions}
% We also show the probability of a bug surviving a 24 hours fuzzing trial of four programs generated by MAGMA, which is shown in fig.X. Dotted lines and solid lines indicate the survival functions for reached bugs and triggered bugs, respectively, and the shaded regions are confidence intervals. As the bug’s probability of survival decreases to 0 fastest, \tool{}-redqueen is the best fuzzer on these four programs.




% \begin{table}[!t]
% \centering
% \caption{Edge Rank.}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{@{\extracolsep{4pt}}lrrrrrrrrrrr@{}}
% \toprule

% \textbf{Time} &  \textbf{all} & \textbf{history}& \textbf{new} & \textbf{mopt} & \textbf{exploit} & \textbf{fast} & \textbf{raw} & \textbf{rare} & \textbf{compare}\\
% \midrule
% \textbf{1 hour} & 2.4   &   2.2  & 4.4  & 6.9   &   6.4 &  5.3  & 5.3&   7.2  &    4.4 \\
% \textbf{3 hours} & 2.4   &   2.2  & 4.4  & 6.9   &   6.4 &  5.3  & 5.3&   7.2  &    4.4 \\
% \textbf{6 hours} & 3.0   &   2.3  & 4.9  & 7.0   &   6.3  & 4.8  & 4.9 &  7.4   &   4.3\\
% \textbf{12 hours} & 2.8  &    2.4  & 4.9 &  6.6    &  6.3  & 4.9 &  5.3  & 7.1    &  4.6\\
% \textbf{24 hours} & 2.8  &    2.4  & 4.9 &  6.6    &  6.3  & 4.9 &  5.3  & 7.1    &  4.6\\

% \bottomrule
% \end{tabular}
% }
% \label{edge_rank_for_unifuzz}
% \end{table}




% % \subsection{Verification Experiment}
% \subsection{The Effectiveness of Inferred Positions}
% \todo{Moved to motivation. Delete it.}

% We further analyze whether the valuable positions identified by \tool{} are really efficient. 
% Given a seed, we define the \textit{important positions} as the positions that can discover new edges. \zhu{you define important positions, valuable positions, and useful positions. Please be consistent, or make sure they have different meaning.}
% Thus, we need to obtain the ground truth of the important positions, and analyze the intersection between the important positions and valuable positions identified by \tool{}.

% \textbf{Ground Truth.} 
% Due to the complexity of fuzzing, it is difficult to directly analyze the ground truth of important positions.
% Thus, we use SHAP analysis to analyze mutation information during fuzzing to obtain ground truth.
% SHAP (SHapley Additive exPlanations) \cite{shap} is a game theoretic approach, which is widely used to explain individual predictions. Based on the game theoretically optimal Shapley values, SHAP explains the prediction of an instance by computing the contribution of each feature to the prediction. The following describes how we use SHAP analysis to analyze the important positions of each seed.

% First, given a seed, in order to ensure the semantic consistency between seeds to facilitate analysis, we perform fuzzing (AFL++) for 48 hours without using length mutators and trimming. And we maintain a dataset for SHAP analysis.
% Second, during the fuzzing process, we collect mutation information of all mutations that discover new edges, including the mutated positions and the number of new edges discovered. The extracted mutation information will be added to dataset.
% Third, We try all combinations of mutated positions for each mutation information, and analyze how many new edges can be found for each combination. This characterizes the contribution of each position to the discovered new edges. The above information will be added to dataset.
% Fourth, we extract the important positions from dataset based on SHAP analysis.

% \textbf{Experiment Setup.}
% After obtaining the ground truth of important positions, we perform fuzzing based on a single seed for 2 hours without using length mutators and trimming.
% Finally, we perform experiments on \texttt{nm}, \texttt{objdump}, \texttt{readelf}, \texttt{size}, \texttt{strip}, \texttt{tiff2bw}, and \texttt{tiffsplit}.
% We analyze the probability of \tool{} extracting the top 1\%, 3\%, 5\%, 7\% and 10\% of important positions at different times respectively.

% \textbf{Result.}
% The result is shown in the Figure \ref{shap}.
% We find that \tool{} outperforms random selection at all times.
% For instance, after fuzzing 10 minutes, the probability that \tool{} selects the top 1\%, 3\%, 5\%, 7\%, and 10\% of important positions are 18\%, 28\%, 32\%, 35\%, and 37\%, respectively.


% \begin{figure}[t!]
% \includegraphics[width=\linewidth]{images/shap.jpg}
% \caption{SHAP analysis.}
% \label{shap}
% \end{figure}

% \zhu{SHAP experiment here.}

% \begin{table*}[!t]
% \centering
% \caption{The Result of SHAP Analysis. We extract the most important positions \zhu{define important positions} based on the data collected from 48 hours fuzzing campaigns. Top$N$\% means that the top N\% of the most important positions. $X$mins means fuzzing $X$ mins. And the value in the table represent the ratio at which the positions collected in common features after fuzzing X mins and the top N\% of the most important positions intersect. The higher the value, the better the performance. And the Baseline means that we randomly select positions into common features.}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{@{\extracolsep{4pt}}lrrrrrrrrrrr@{}}
% \toprule

% \textbf{Time} &  \textbf{Top10\%} & \textbf{Top20\%}& \textbf{Top30\%} & \textbf{Top40\%} & \textbf{Top50\%} & \textbf{Top60\%} & \textbf{Top70\%} & \textbf{Top80\%} & \textbf{Top90\%} & \textbf{Top100\%} & \textbf{Baseline}\\
% \midrule
% \textbf{10mins}  &0.67 &   0.59  &  0.55  &  0.52  &  0.49 &   0.46  &  0.44  &  0.42   & 0.40  &   0.38   &   0.07 \\
% \textbf{20mins}  & 0.77  &  0.71  &  0.68  &  0.65   & 0.62   & 0.60  &  0.58 &   0.56  &  0.54   &  0.52    &  0.14 \\
% \textbf{30mins}  & 0.81 &   0.76  &  0.73   & 0.71   & 0.68  &  0.67  &  0.64  &  0.63  &  0.61    & 0.59     & 0.17 \\
% \textbf{40mins}  & 0.83  &  0.79  &  0.77  &  0.75  &  0.72  &  0.71 &   0.69  &  0.67  &  0.65  &   0.63   &   0.18 \\
% \textbf{50mins}  & 0.85  &  0.81  &  0.79  &  0.78  &  0.75  &  0.73   & 0.71  &  0.69  &  0.68   &  0.66    &  0.19 \\
% \textbf{60mins}  & 0.86  &  0.83   & 0.81  &  0.79  &  0.77  &  0.75   & 0.73   & 0.71  &  0.70   &  0.68   &   0.20 \\
% \textbf{70mins}  & 0.87  &  0.84 &   0.82  &  0.81  &  0.78  &  0.77   & 0.75  &  0.73   & 0.72   &  0.70   &   0.20 \\
% \textbf{80mins}  & 0.88  &  0.85  &  0.83  &  0.82  &  0.80  &  0.78   & 0.76  &  0.75  &  0.73  &   0.71 &     0.20 \\
% \textbf{90mins}  & 0.88  &  0.86  &  0.84  &  0.83  &  0.81   & 0.79   & 0.78  &  0.76  &  0.74  &   0.73   &   0.21 \\
% \textbf{100mins}  & 0.88  &  0.86  &  0.85  &  0.84  &  0.81   & 0.80   & 0.78  &  0.77 &   0.75   &  0.73    &  0.21 \\
% \textbf{110mins}  & 0.89  &  0.87  &  0.85 &   0.84  &  0.82   & 0.81  &  0.79  &  0.78  &  0.76  &   0.74  &    0.21 \\
% \textbf{120mins}  & 0.90  &  0.87  &  0.86 &   0.85   & 0.83  &  0.82  &  0.80 &   0.79&    0.77 &    0.75   &   0.23 \\


% \bottomrule
% \end{tabular}
% }
% \label{shap}
% \end{table*}


\begin{table*}[!t]
% \renewcommand\arraystretch{1.7}
% \newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
\centering
\caption{The comparison of position inference. \tool{} can infer more useful positions within less inference time.}
\resizebox{\linewidth}{!}{
\begin{threeparttable}
\begin{tabular}{@{\extracolsep{4pt}}lccccccccccccccc@{}}
\toprule
\multirow{3}{*}{\textbf{Programs}} & \multicolumn{3}{c}{\textbf{GreyOne}} & \multicolumn{3}{c}{\textbf{ProFuzzer}} & \multicolumn{3}{c}{\textbf{\tool}}\\
\cline{2-4} \cline{5-7} \cline{8-10}


&\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Analysis}\\ \textbf{Time(s)}\end{tabular}} 
&\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Useful}\\ \textbf{Ratio}\end{tabular}} 
&\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Average Useful}\\ \textbf{Mutation}\end{tabular}} 

&\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Analysis}\\ \textbf{Time(s)}\end{tabular}} 
&\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Useful}\\ \textbf{Ratio}\end{tabular}} 
&\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Average Useful}\\ \textbf{Mutation}\end{tabular}} 

&\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Analysis}\\ \textbf{Time(s)}\end{tabular}} 
&\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Useful}\\ \textbf{Ratio}\end{tabular}} 
&\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Average Useful}\\ \textbf{Mutation}\end{tabular}} \\
&&&&&&&&&\\
\midrule

\textbf{nm} & 16721 & 3\%(135/4834) & 0.11 & 13584 & 16\%(109/665) & 0.32 & \textbf{16.68} & \textbf{67\%(55/82)} & \textbf{1.87}  \\
\textbf{tiff2bw} & 8283 & 13\%(101/762) & 0.74 & 9372 & 14\%(106/762) & 0.75 & \textbf{7} & \textbf{89\%(74/83)} & \textbf{5.87}\\
\textbf{tiffsplit} & 8875 & 68\%(104/152) & 3.18 & 10894 & 69\%(104/150) & 3.25 & \textbf{8} & \textbf{92\%(72/78)} & \textbf{6.60}\\
\textbf{objdump} & 52080 & 2\%(205/13288) & 0.45 & 29901 & 18\%(318/1794) & 0.68 & \textbf{45} & \textbf{60\%(179/299)} & \textbf{1.70} \\
\textbf{readelf} & 16739 & 3\%(99/3798) & 0.41 & 13712 & 7\%(186/2641) & 0.48 & \textbf{37} & \textbf{83\%(95/114)} & \textbf{8.70}\\
\textbf{flvmeta} & 2262 & 46\%(29/63) & 1.28 & 2222 & 22\%(42/187) & 0.46 & \textbf{2} & \textbf{40\%(14/35)} & \textbf{1.08}\\
\textbf{pdftotext} & 54447 & 3\%(267/8384) & 0.07 & 38144 & 4\%(337/8805) & 0.08 & \textbf{54} & \textbf{54\%(165/305)} & \textbf{1.11}\\
\textbf{mp42aac} & 11855 & 19\%(124/651) & 0.32 & 17234 & 21\%(132/614) & 0.35 & \textbf{9} & \textbf{68\%(69/102)} & \textbf{1.70}\\
\textbf{tcpdump} & 13219 & 2\%(88/4075) & 2.89 & 13774 & 3\%(87/2708) & 2.48 & \textbf{16} & \textbf{77\%(72/93)} & \textbf{6.36}\\
\textbf{lame3.99.5} & 75520 & 1\%(169/13077) & 0.02 & 62433 & 1\%(179/13060) & 0.02 & \textbf{80} & \textbf{73\%(74/102)} & \textbf{2.16}\\

% \textbf{size}\\
% \textbf{infotocap}\\
% \textbf{sqlite3}\\
% \textbf{imginfo}\\
% \textbf{jq}\\
% \textbf{mujs}\\

\bottomrule
\end{tabular}
\end{threeparttable}
}
\label{Verification}
\end{table*}



\subsection{Comparison of Inference-based Fuzzing}
\balance

In this section, we compare \tool{} with inference-based fuzzers, including GreyOne~\cite{greyone} and ProFuzzer~\cite{profuzzer}, in terms of the effectiveness of inferred positions. 
% If an inferred position can discover new code coverage in later fuzzing campaigns, it is an effective position.

\textbf{Fuzzers.} 
Since neither GreyOne nor ProFuzzer is open-source, we implement their core algorithms to identify the related positions of path constraints. For ProFuzzer, it iterates over all 256 values at each byte position, and if the path length changes relative to the initial seed, the current position is related to a path constraint. For GreyOne, it mutates 8 times at each position, and if the value of a variable in a CMP instruction changes, the current position is related to a path constraint.

% to verify that the positions identified by \tool{} are more critical. 
% The existing inference-based fuzzers have found many bugs in the real-world programs. They can find positions related to path constraints through simple instrumentation or lightweight inference methods. In this section, we performed a fine-grained analysis on the importance of the inferred positions.
% To verify that the positions identified by \tool{} are more critical, we compare \tool{} with GreyOne and ProFuzzer. 

% \textbf{Fuzzers.}
% Since neither GreyOne nor ProFuzzer is open source, we implement their core algorithms to identify the related positions of path constraints, as follows:
% \begin{itemize}
%   \item [1)]
%   ProFuzzer: ProFuzzer iterates over all 256 values at each position. If the path length changes relative to the initial seed while trying a certain value, the current position is related to path constraints, and ProFuzzer will not try any other remaining values to speed up the analysis.
%   \item [2)] 
%   GreyOne: Greyone tries to mutate 8 times at each position. If the value of a variable in a CMP instruction changes, the current position is related to a path constraint.
% \end{itemize}

\textbf{Experiment Setup.}
We randomly select 10 target programs and several initial seeds for experiments from UNIFUZZ. To facilitate the comparison of effects, we analyze each initial seed separately, and the specific experimental steps are as follows. For an initial seed, we use \tool{}, Greyone and ProFuzzer to mutate the target seed for 3 hours, respectively. Then, we count the additional analysis time required by each fuzzer and the number of new edges they discover. In particular, for the convenience of comparison, we do not update the seed queue but continuously mutate the selected initial seed.

\textbf{Comparison Metrics.} 
We use the following three new metrics for fine-grained analysis of the above fuzzers:
\begin{itemize}
  \item [1)]
  \textit{Average analysis time}: The analysis time required by each fuzzer to infer related positions. Both ProFuzzer and GreyOne use a pilot stage for inference. Since \tool{} does not contain a pilot stage, we regard the time of analyzing mutation information as the analysis time.
%   The shorter the analysis time, the higher the efficiency. ProFuzzer and Greyone need to set up a pilot stage for inference, so we take the time spent in the pilot stage as their analysis time. Although \tool{} does not contain a pilot stage, the de-redundancy operation will bring some additional program execution when analyzing the extracted mutation information. Therefore, for \tool{}, we counted the sum of the time to analyze all the mutation information as the analysis time.
  \item [2)] 
  \textit{The proportion of useful position}: If a position is inferred and finds a new edge in the subsequent mutation process, it is called a useful position. \textit{\textbf{For \tool{}, we do not count the first time when an inferred position is retained.}} We record the proportion of useful positions in all inferred positions.
%   \zhu{68\%(55/82): \tool{} inferred 82 positions, where 55 positions can be mutated to discover new edges after they have been retained as a shared position.}
  \item [3)] 
  \textit{The average number of useful mutations}: If the mutation of inferred positions finds a new edge, this mutation is a useful mutation.
%   If a mutation finds a new edge, then this mutation is considered a useful mutation. 
  We use this metric to describe the importance of each position. 
  If a position has more useful mutations, it is more important.
% , and vice versa. Finally, we count the average number of useful mutations among inferred positions.
\end{itemize}

\textbf{Result.}
We only include seeds that can complete the analysis within three hours. In three hours, \tool{} can complete the analysis of all seeds, but both GreyOne and ProFuzzer have some long seeds that cannot complete the analysis. The results are shown in the Table~\ref{Verification}.
For the average analysis time, \tool{} spends the shortest time, which is 27.47 seconds on average. Greyone and ProFuzzer take about 26000 seconds and 21127 seconds, respectively. 
Since \tool{} does not require a pilot stage, especially for long seeds, the analysis efficiency of \tool{} is much higher than that of Greyone and ProFuzzer.
We analyze the average number of useful mutations for each fuzzer at 1,000,000 mutations. \tool{} perform the best, and its average proportion of useful positions is up to 70.5\%. Moreover, \tool{}'s average number of useful mutations is up to 3.715. The proportion of useful positions and average number of useful mutations of GreyOne are only 16.1\% and 0.947, while that of ProFuzzer are only 17.8\% and 0.0887.
According to the above experimental results, \tool{} can find more useful positions within shorter analysis time.





==> obsolete/evaluation-2.0.tex <==


\section{Evaluation} \label{sec:eval}

We implement our \tool{} based on AFL++~\cite{aflpp}, which integrates many state-of-the-art fuzzing algorithms. We mainly modify the mutation process and the byte schedule. 
% During fuzzing, the mutation that discovers self-new edges will be additionally analyzed to calculate the Shapley Values of bytes. 
% When selecting bytes, instead of randomly mutating the entire input, \tool{} prefers mutating valuable positions of seeds.
In the evaluation, we evaluate our \tool{} with byte schedule-reinforced fuzzers and commonly used fuzzers.
% In the evaluation, we evaluate our vanilla \tool{} and \tool-Redqueen that enables both \tool{} and Redqueen in AFL++. Redqueen~\cite{redqueen} extracts constant strings to pass path constraints.
% Due to the limit of pages, we show more experiment results in appendix.
% Although our experiments are conducted on source code, our solution can also be performed on executable binaries by using binary instrumentation tools to get the feedback of edge coverage.
% \zhu{no need for source code.}







\begin{table}[!t]
% \renewcommand\arraystretch{1}
\centering
\caption{Target programs from UNIFUZZ.}\label{programsUNIFUZZ}
\resizebox{0.9\linewidth}{!}{
\begin{threeparttable}
\begin{tabular}{llll}
    \toprule
    \textbf{Targets} & \textbf{Projects} & \textbf{Input formats} & \textbf{Test instructions} \\ \midrule
    \textbf{tiff2bw\tnote{2}} & \multirow{3}{*}{libtiff 3.9.7} & \multirow{3}{*}{tiff} & tiff2bw @@\tnote{1}~{ } /dev/null \\
    \textbf{tiffsplit} &&& tiffsplit @@ /dev/null\\
    \textbf{tiff2pdf\tnote{2}} &&& tiff2pdf @@ /dev/null\\
    \midrule
    \multirow{3}{*}{\textbf{nm}} & \multirow{6}{*}{binutils-2.28} & \multirow{4}{*}{ELF} & (-A -a -l -S -s \\
    &&&\ \ \ --special-syms --synthetic\\
    &&&\ \ \ --with-symbol-versions -D @@) \\
    \textbf{objdump} &&& -S @@ \\
    \textbf{readelf\tnote{2}} &&& -a @@ \\
    \textbf{size\tnote{2}} &&& @@ \\
    \midrule
    \textbf{pdftotext} & pdftotext 4.00 & pdf & @@ /dev/null \\
    \midrule
    \textbf{infotocap} & jasper 2.0.12 & text & -o /dev/null @@ \\
    \midrule
    \textbf{mp42aac} & Bento4 1.5.1-628 & mp4 & @@ /dev/null \\
    \midrule
    \multirow{2}{*}{\textbf{tcpdump}}
     & tcpdump 4.8.1 + & \multirow{2}{*}{tcpdump100} & \multirow{2}{*}{-e -vv -nr @@} \\
     & libpcap 1.8.1 && \\
    \midrule
    \textbf{flvmeta} & flvmeta 1.2.1 & flv &  @@ \\
    \midrule
    \textbf{lame3.99.5} & lame 3.99.5 & wav & @@ /dev/null \\
    \midrule
    \textbf{imginfo} & ncurses 6.1 & jpg & -f @@ \\
    \midrule
    \textbf{mujs} & mujs 1.0.2 & js & @@ \\
    \midrule
    \textbf{exiv2} & exiv2 0.26 & jpg & @@ \\
    \bottomrule
\end{tabular}
\begin{tablenotes}
\item[1] @@: A placeholder indicating that the input is a file.
\item[2] \textbf{tiff2bw, tiff2pdf, readelf} and \textbf{size} are not from UNIFUZZ
\end{tablenotes}
\end{threeparttable}

}
\end{table}



% \subsection{Experimental Setup}
To ensure fair results, we conduct our experiments on two third-party testing platforms, UNIFUZZ~\cite{unifuzz} and MAGMA~\cite{magma}. Our experiments are performed on a system running Ubuntu 18.04 with 103 cores (Intel(R) Xeon(R) Gold 6230R CPU) and 256 GB of memory. Each fuzzer uses one CPU core to run one target program. 
% All experiments run for 24 hours and repeat 10 times to avoid the randomness of fuzzing~\cite{bohme2022reliability}.

\noindent\textbf{Evaluation Metrics.}
We use \textit{afl-showmap} in AFL++ to count the number of edges and compile target programs with ASAN~\cite{asan} enabled. When analyzing unique bugs, we use the top-three rule to de-duplicate bugs~\cite{Klees2018Evaluating}.


\noindent\textbf{Target Programs and Initial Seeds.}
We select 16 commonly used programs for testing from UNIFUZZ and other papers, as shown in the Table \ref{programsUNIFUZZ}.
For each target program, all fuzzers use the same initial seeds, which are collected from UNIFUZZ, FuzzBench\cite{fuzzbench} or public seed corpus. 
Most target programs have multiple initial seeds as suggested by Adrian Herrera~\cite{herrera2021seed}.


\zkp{




\begin{table*}[!t]
\centering
\caption{Edge Coverage and Analysis Time comparison between different fuzzers (on \texttt{ALL SEEDS}).}
\resizebox{\linewidth}{!}{
\begin{threeparttable}
\begin{tabular}{@{\extracolsep{4pt}}cc|ccc|ccc|ccc|ccc|ccc|ccc@{}} %crrrrrrrrrrr
\toprule
% \rotatebox{80}{\textbf{\tool-Redqueen\tnote{1}}}
% \textbf{Program} & \textbf{ave. Length} & \textbf{\tool{}} & \textbf{GreyOne} & \textbf{ProFuzzer} & \textbf{Angora} & \textbf{PreFuzz} & \textbf{NEUZZ} \\
\multicolumn{2}{c}{\textbf{Programs}} & \multicolumn{3}{c}{\textbf{\tool{}}} & \multicolumn{3}{c}{\textbf{GreyOne}} & \multicolumn{3}{c}{\textbf{ProFuzzer}} & \multicolumn{3}{c}{\textbf{Angora}} & \multicolumn{3}{c}{\textbf{PreFuzz}} & \multicolumn{3}{c}{\textbf{NEUZZ}}\\
\textbf{Name} & \textbf{ave. Length}& \textbf{Cov.} & \textbf{Time} & \textbf{\#Bug}& \textbf{Cov.} & \textbf{Time} & \textbf{\#Bug}& \textbf{Cov.} & \textbf{Time} & \textbf{\#Bug}& \textbf{Cov.} & \textbf{Time} & \textbf{\#Bug}& \textbf{Cov.} & \textbf{Time} & \textbf{\#Bug}& \textbf{Cov.} & \textbf{Time} & \textbf{\#Bug}\\
\midrule

tiff2pdf & 448 & 4401 & 85s & 0 & 4486 & 35207s & 0 & 4578 & 12694s & 1 & 2314 & 235s & 0 & 3475 & G & 1 & 2832 & G\tnote{1}~ & 1 \\ 
lame & 13818 & 3656 & 3985s & 5 & 3645 & 80225s & 4 & 3649 & 70003s & 4 & 2265 & 5813s & 4 & - & - & 0 & -\tnote{2} & - & 0 \\ 
readelf & 272030 & 5611 & 1048s & 4 & 5058 & 78788s & 3 & 5168 & 74878s & 6 & 5786 & 3758s & 6 & - & - & 0 & - & - & 0 \\ 
exiv2 & 25633 & 3790 & 135s & 15 & 3626 & 35401s & 5 & 3698 & 32311s & 12 & 4291 & 615s & 11 & 2866 & G & 0 & - & - & 0 \\ 
flvmeta & 16454 & 230 & 0s & 2 & 230 & 32782s & 2 & 230 & 11625s & 2 & 230 & 201s & 2 & - & - & 0 & - & - & 0 \\ 
nm & 272030 & 3136 & 248s & 17 & 2628 & 83058s & 9 & 2750 & 81747s & 10 & 2657 & 2351s & 51 & - & - & 0 & - & - & 0 \\ 
tiffsplit & 10032 & 1709 & 5s & 7 & 1699 & 13398s & 5 & 1719 & 6220s & 6 & 890 & 291s & 1 & 1189 & G & 2 & 1113 & G & 1 \\ 
tiff2bw & 10032 & 1839 & 87s & 6 & 1870 & 12709s & 6 & 1848 & 8702s & 5 & 1180 & 310s & 1 & 1651 & G & 0 & 1441 & G & 0 \\ 
objdump & 272030 & 4958 & 742s & 14 & 3864 & 79211s & 4 & 4106 & 83913s & 5 & 3192 & 3672s & 3 & - & - & 0 & - & - & 0 \\ 
pdftotext & 12465 & 6613 & 3508s & 23 & 5794 & 80548s & 2 & 5777 & 80591s & 3 & 4250 & 14801s & 2 & 4902 & G & 5 & 4394 & G & 0 \\ 
mp42aac & 31988 & 1266 & 19s & 2 & 1144 & 75949s & 0 & 1166 & 66141s & 0 & 1120 & 540s & 0 & 1017 & G & 0 & 950 & G & 0 \\ 
tcpdump & 6983 & 12764 & 328s & 1 & 11558 & 50599s & 1 & 11879 & 29383s & 0 & 7615 & 2510s & 3 & 4672 & G & 0 & 6019 & G & 0 \\ 
mujs & 6983 & 4136 & 0s & 0 & 4020 & 18157s & 0 & 3979 & 7181s & 0 & 2364 & 8829s & 0 & 2432 & G & 0 & 2393 & G & 0 \\ 
size & 272030 & 1860 & 188s & 0 & 1667 & 77562s & 0 & 1690 & 78671s & 0 & 1988 & 2032s & 0 & - & - & 0 & - & - & 0 \\ 
infotocap & 2519 & 1817 & 276s & 7 & 1670 & 39193s & 6 & 1530 & 44335s & 5 & 940 & 1104s & 0 & 1266 & G & 1 & 1071 & G & 0 \\ 
imginfo & 2519 & 1895 & 30s & 0 & 1818 & 36298s & 0 & 1744 & 43274s & 0 & 1384 & 184s & 0 & - & - & 0 & - & - & 0 \\
\midrule
\textbf{Total} & ~  & \textbf{59681} & & \textbf{103} & 54777 & & 47 & 55511 & & 59 & 42466 & & 84 & 23470 & & 9 & 20213 & & 2 \\

% tiff2pdf & 448 & 4401(85s) & 0 & 4486(35207s) & 0 & 4578(12694s) & 1 & 2314(235s) & 0 & 3475(G) & 1 & 2832(G\tnote{1}~) & 1 \\ 
% lame & 13818 & 3656(3985s) & 5 & 3645(80225s) & 4 & 3649(70003s) & 4 & 2265(5813s) & 4 & - & 0 & -\tnote{2} & 0 \\ 
% readelf & 272030 & 5611(1048s) & 4 & 5058(78788s) & 3 & 5168(74878s) & 6 & 5786(3758s) & 6 & - & 0 & - & 0 \\ 
% exiv2 & 25633 & 3790(135s) & 15 & 3626(35401s) & 5 & 3698(32311s) & 12 & 4291(615s) & 11 & 2866(G) & 0 & - & 0 \\ 
% flvmeta & 16454 & 230(0s) & 2 & 230(32782s) & 2 & 230(11625s) & 2 & 230(201s) & 2 & - & 0 & - & 0 \\ 
% nm & 272030 & 3136(248s) & 17 & 2628(83058s) & 9 & 2750(81747s) & 10 & 2657(2351s) & 51 & - & 0 & - & 0 \\ 
% tiffsplit & 10032 & 1709(5s) & 7 & 1699(13398s) & 5 & 1719(6220s) & 6 & 890(291s) & 1 & 1189(G) & 2 & 1113(G) & 1 \\ 
% tiff2bw & 10032 & 1839(87s) & 6 & 1870(12709s) & 6 & 1848(8702s) & 5 & 1180(310s) & 1 & 1651(G) & 0 & 1441(G) & 0 \\ 
% objdump & 272030 & 4958(742s) & 14 & 3864(79211s) & 4 & 4106(83913s) & 5 & 3192(3672s) & 3 & - & 0 & - & 0 \\ 
% pdftotext & 12465 & 6613(3508s) & 23 & 5794(80548s) & 2 & 5777(80591s) & 3 & 4250(14801s) & 2 & 4902(G) & 5 & 4394(G) & 0 \\ 
% mp42aac & 31988 & 1266(19s) & 2 & 1144(75949s) & 0 & 1166(66141s) & 0 & 1120(540s) & 0 & 1017(G) & 0 & 950(G) & 0 \\ 
% tcpdump & 6983 & 12764(328s) & 1 & 11558(50599s) & 1 & 11879(29383s) & 0 & 7615(2510s) & 3 & 4672(G) & 0 & 6019(G) & 0 \\ 
% mujs & 6983 & 4136(0s) & 0 & 4020(18157s) & 0 & 3979(7181s) & 0 & 2364(8829s) & 0 & 2432(G) & 0 & 2393(G) & 0 \\ 
% size & 272030 & 1860(188s) & 0 & 1667(77562s) & 0 & 1690(78671s) & 0 & 1988(2032s) & 0 & - & 0 & - & 0 \\ 
% infotocap & 2519 & 1817(276s) & 7 & 1670(39193s) & 6 & 1530(44335s) & 5 & 940(1104s) & 0 & 1266(G) & 1 & 1071(G) & 0 \\ 
% imginfo & 2519 & 1895(30s) & 0 & 1818(36298s) & 0 & 1744(43274s) & 0 & 1384(184s) & 0 & - & 0 & - & 0 \\ 
% \midrule
% \textbf{Total} & ~  & \textbf{59681} & \textbf{103} & 54777 & 47 & 55511 & 59 & 42466 & 84 & 23470 & 9 & 20213 & 2 \\ 


% tiff2pdf &448 &4401(85s) &4486(35207s) &4578(12694s) &2314(235s) &3475(G) &2832(G\tnote{1}~) \\
% lame &13818 &3656(3985s) &3645(80225s) &3649(70003s) &2265(5813s) &- &-\tnote{2} \\
% readelf &272030 &5611(1048s) &5058(78788s) &5168(74878s) &5786(3758s) &- &- \\
% exiv2 &25633 &3790(135s) &3626(35401s) &3698(32311s) &4291(615s) &2866(G) &- \\
% flvmeta &16454 &230(0s) &230(32782s) &230(11625s) & 230(201s) &- &- \\
% nm &272030 &3136(248s) &2628(83058s) &2750(81747s) &2657(2351s) &- &- \\
% tiffsplit &10032 &1709(5s) &1699(13398s) &1719(6220s) &890(291s) &1189(G) &1113(G) \\
% tiff2bw &10032 &1839(87s) &1870(12709s) &1848(8702s) &1180(310s) &1651(G) &1441(G) \\
% objdump &272030 &4958(742s) &3864(79211s) &4106(83913s) &3192(3672s) &- &- \\
% pdftotext &12465 &6613(3508s) &5794(80548s) &5777(80591s) &4250(14801s) &4902(G) &4394(G) \\
% mp42aac &31988 &1266(19s) &1144(75949s) &1166(66141s) & 1120(540s) &1017(G) &950(G) \\
% tcpdump &6983 &12764(328s) &11558(50599s) &11879(29383s) &7615(2510s) &4672(G) &6019(G) \\
% mujs &6983 &4136(0s) &4020(18157s) &3979(7181s) &2364(8829s) &2432(G) &2393(G) \\
% size &272030 &1860(188s) &1667(77562s) &1690(78671s) &1988(2032s) &- &- \\
% infotocap &2519 &1817(276s) &1670(39193s) &1530(44335s) &940(1104s) &1266(G) &1071(G) \\
% imginfo &2519 &1895(30s) &1818(36298s) &1744(43274s) &1384(184s) &- &- \\
% \midrule
% \textbf{Total} & & \textbf{59681} &54777 &55511 &42466 &23470 &20213 \\

\bottomrule
\end{tabular}
\begin{tablenotes}[para]
\item[1]G: A GPU is required to train the model.
\item[2]-: The fuzzer fails to run on this program due to large input size.
\end{tablenotes}
\end{threeparttable}
}

\label{all_seeds}
\end{table*}

\begin{table*}[!t]
\centering
\caption{Edge Coverage and Analysis Time comparison between different fuzzers (on \texttt{SEEDS<10000}).}
\resizebox{\linewidth}{!}{
\begin{threeparttable}
\begin{tabular}{@{\extracolsep{4pt}}cc|ccc|ccc|ccc|ccc|ccc|ccc@{}} %crrrrrrrrrrr
\toprule
% \rotatebox{80}{\textbf{\tool-Redqueen\tnote{1}}}
% \textbf{Program} & \textbf{ave. Length} & \textbf{\tool{}} & \textbf{GreyOne} & \textbf{ProFuzzer} & \textbf{Angora} & \textbf{PreFuzz} & \textbf{NEUZZ} \\
\multicolumn{2}{c}{\textbf{Programs}} & \multicolumn{3}{c}{\textbf{\tool{}}} & \multicolumn{3}{c}{\textbf{GreyOne}} & \multicolumn{3}{c}{\textbf{ProFuzzer}} & \multicolumn{3}{c}{\textbf{Angora}} & \multicolumn{3}{c}{\textbf{PreFuzz}} & \multicolumn{3}{c}{\textbf{NEUZZ}}\\
\textbf{Name} & \textbf{ave. Length}& \textbf{Cov.} & \textbf{Time} & \textbf{\#Bug}& \textbf{Cov.} & \textbf{Time} & \textbf{\#Bug}& \textbf{Cov.} & \textbf{Time} & \textbf{\#Bug}& \textbf{Cov.} & \textbf{Time} & \textbf{\#Bug}& \textbf{Cov.} & \textbf{Time} & \textbf{\#Bug}& \textbf{Cov.} & \textbf{Time} & \textbf{\#Bug}\\
\midrule

tiff2pdf & 448 & 4461& 30s & 1 & 4450& 39189s & 0 & 4552& 15278s & 0 & 2306& 50s & 0 & 3466& G & 0 & 2543& G\tnote{1}~ & 0 \\ 
readelf & 4230 & 5359& 77s & 5 & 5346& 39952s & 6 & 5272& 38537s & 3 & 5554& 1628s & 7 & 4540& G & 6 & 4208& G & 4 \\ 
exiv2 & 8437 & 3882& 196s & 7 & 3385& 50513s & 4 & 3691& 31915s & 3 & 3903& 2365s & 9 & 3881& G & 0 & 3151& G & 0 \\ 
nm & 4230 & 2822& 17s & 30 & 2818& 29069s & 20 & 2884& 13905s & 22 & 2409& 2056s & 35 & 2260& G & 14 & 1749& G & 0 \\ 
tiffsplit & 7222 & 1718& 4s & 6 & 1725& 13541s & 6 & 1715& 4519s & 7 & 919& 219s & 3 & 1203& G & 2 & 1128& G & 0 \\ 
tiff2bw & 7222 & 1882& 42s & 7 & 1876& 12031s & 6 & 1808& 6040s & 6 & 1186& 200s & 1 & 1594& G & 0 & 1489& G & 0 \\ 
objdump & 4230 & 4654& 104s & 16 & 4145& 75874s & 10 & 4414& 50760s & 13 & 3085& 4182s & 13 & 3560& G & 4 & 3136& G & 0 \\ 
tcpdump & 2305 & 12963& 227s & 1 & 12164& 40025s & 1 & 12497& 13022s & 0 & 7826& 2119s & 1 & 7963& G & 1 & 6251& G & 0 \\ 
mujs & 2305 & 4145& 0s & 0 & 4000& 19877s & 0 & 4015& 7078s & 0 & 2383& 8677s & 0 & 2589& G & 1 & 2388& G & 0 \\ 
size & 4230 & 1795& 22s & 0 & 1785& 12623s & 0 & 1812& 9547s & 0 & 1794& 1259s & 1 & 1458& G & 0 & 1224& G & 0 \\ 
infotocap & 2519 & 1807& 457s & 8 & 1767& 38278s & 5 & 1399& 45154s & 2 & 840& 1647s & 0 & 1159& G & 1 & 1074& G & 0 \\ 
imginfo & 2519 & 2486& 9s & 0 & 1744& 26514s & 0 & 1680& 24268s & 0 & 1413& 244s & 0 & 1464& G & 0 & 1176& G & 0 \\
\midrule
\textbf{Total} &  & \textbf{47974} & & \textbf{81} & 45205 & & 58 & 45739 & & 56 & 33618 & & 70 & 35137 & & 29 & 29517 & & 4 \\ 

% tiff2pdf & 448 & 4461(30s) & 1 & 4450(39189s) & 0 & 4552(15278s) & 0 & 2306(50s) & 0 & 3466(G) & 0 & 2543(G\tnote{1}~) & 0 \\ 
% readelf & 4230 & 5359(77s) & 5 & 5346(39952s) & 6 & 5272(38537s) & 3 & 5554(1628s) & 7 & 4540(G) & 6 & 4208(G) & 4 \\ 
% exiv2 & 8437 & 3882(196s) & 7 & 3385(50513s) & 4 & 3691(31915s) & 3 & 3903(2365s) & 9 & 3881(G) & 0 & 3151(G) & 0 \\ 
% nm & 4230 & 2822(17s) & 30 & 2818(29069s) & 20 & 2884(13905s) & 22 & 2409(2056s) & 35 & 2260(G) & 14 & 1749(G) & 0 \\ 
% tiffsplit & 7222 & 1718(4s) & 6 & 1725(13541s) & 6 & 1715(4519s) & 7 & 919(219s) & 3 & 1203(G) & 2 & 1128(G) & 0 \\ 
% tiff2bw & 7222 & 1882(42s) & 7 & 1876(12031s) & 6 & 1808(6040s) & 6 & 1186(200s) & 1 & 1594(G) & 0 & 1489(G) & 0 \\ 
% objdump & 4230 & 4654(104s) & 16 & 4145(75874s) & 10 & 4414(50760s) & 13 & 3085(4182s) & 13 & 3560(G) & 4 & 3136(G) & 0 \\ 
% tcpdump & 2305 & 12963(227s) & 1 & 12164(40025s) & 1 & 12497(13022s) & 0 & 7826(2119s) & 1 & 7963(G) & 1 & 6251(G) & 0 \\ 
% mujs & 2305 & 4145(0s) & 0 & 4000(19877s) & 0 & 4015(7078s) & 0 & 2383(8677s) & 0 & 2589(G) & 1 & 2388(G) & 0 \\ 
% size & 4230 & 1795(22s) & 0 & 1785(12623s) & 0 & 1812(9547s) & 0 & 1794(1259s) & 1 & 1458(G) & 0 & 1224(G) & 0 \\ 
% infotocap & 2519 & 1807(457s) & 8 & 1767(38278s) & 5 & 1399(45154s) & 2 & 840(1647s) & 0 & 1159(G) & 1 & 1074(G) & 0 \\ 
% imginfo & 2519 & 2486(9s) & 0 & 1744(26514s) & 0 & 1680(24268s) & 0 & 1413(244s) & 0 & 1464(G) & 0 & 1176(G) & 0 \\ 
% \midrule
% \textbf{Total} &  & \textbf{47974} & \textbf{81} & 45205 & 58 & 45739 & 56 & 33618 & 70 & 35137 & 29 & 29517 & 4 \\ 


% tiff2pdf &448 &4461(30s) &4450(39189s) &4552(15278s) &2306(50s) &3466(G) &2543(G\tnote{1}~) \\
% readelf &4230 &5359(77s) &5346(39952s) &5272(38537s) &5554(1628s) &4540(G) &4208(G) \\
% exiv2 &8437 &3882(196s) &3385(50513s) &3691(31915s) &3903(2365s) &3881(G) &3151(G) \\
% nm &4230 &2822(17s) &2818(29069s) &2884(13905s) &2409(2056s) &2260(G) &1749(G) \\
% tiffsplit &7222 &1718(4s) &1725(13541s) &1715(4519s) &919(219s) &1203(G) &1128(G) \\
% tiff2bw &7222 &1882(42s) &1876(12031s) &1808(6040s) &1186(200s) &1594(G) &1489(G) \\
% objdump &4230 &4654(104s) &4145(75874s) &4414(50760s) &3085(4182s) &3560(G) &3136(G) \\
% tcpdump &2305 &12963(227s) &12164(40025s) &12497(13022s) &7826(2119s) &7963(G) &6251(G) \\
% mujs &2305 &4145(0s) &4000(19877s) &4015(7078s) &2383(8677s) &2589(G) &2388(G) \\
% size &4230 &1795(22s) &1785(12623s) &1812(9547s) &1794(1259s) &1458(G) &1224(G) \\
% infotocap &2519 &1807(457s) &1767(38278s) &1399(45154s) &840(1647s) &1159(G) &1074(G) \\
% imginfo &2519 &2486(9s) &1744(26514s) &1680(24268s) &1413(244s) &1464(G) &1176(G) \\
% \midrule
% \textbf{Total} & & \textbf{47974} &45205 &45739 &33618 &35137 &29517 \\

\bottomrule
\end{tabular}
\begin{tablenotes}[para]
\item[1]G: A GPU is required to train the model. 
\end{tablenotes}
\end{threeparttable}
}
\label{seeds_10000}
\end{table*}


\begin{table*}[!t]
\centering
\caption{Edge Coverage and Analysis Time comparison between different fuzzers (on \texttt{SEEDS<1000}).}
\resizebox{\linewidth}{!}{
\begin{threeparttable}
\begin{tabular}{@{\extracolsep{4pt}}cc|ccc|ccc|ccc|ccc|ccc|ccc@{}} %crrrrrrrrrrr
\toprule
% \rotatebox{80}{\textbf{\tool-Redqueen\tnote{1}}}
% \textbf{Program} & \textbf{ave. Length} & \textbf{\tool{}} & \textbf{GreyOne} & \textbf{ProFuzzer} & \textbf{Angora} & \textbf{PreFuzz} & \textbf{NEUZZ} \\
\multicolumn{2}{c}{\textbf{Programs}} & \multicolumn{3}{c}{\textbf{\tool{}}} & \multicolumn{3}{c}{\textbf{GreyOne}} & \multicolumn{3}{c}{\textbf{ProFuzzer}} & \multicolumn{3}{c}{\textbf{Angora}} & \multicolumn{3}{c}{\textbf{PreFuzz}} & \multicolumn{3}{c}{\textbf{NEUZZ}}\\
\textbf{Name} & \textbf{ave. Length}& \textbf{Cov.} & \textbf{Time} & \textbf{\#Bug}& \textbf{Cov.} & \textbf{Time} & \textbf{\#Bug}& \textbf{Cov.} & \textbf{Time} & \textbf{\#Bug}& \textbf{Cov.} & \textbf{Time} & \textbf{\#Bug}& \textbf{Cov.} & \textbf{Time} & \textbf{\#Bug}& \textbf{Cov.} & \textbf{Time} & \textbf{\#Bug}\\
\midrule

tiff2pdf & 448 & 4383 & 99s & 1 & 4493 & 39407s & 0 & 4449 & 12856s & 1 & 2459 & 58s & 0 & 3398 & G & 1 & 2709 & G\tnote{1}~ & 1 \\ 
readelf & 324 & 4983 & 34s & 4 & 4875 & 13088s & 3 & 4763 & 5978s & 0 & 5131 & 299s & 5 & 4144 & G & 0 & 3760 & G & 0 \\ 
nm & 324 & 1876 & 2s & 0 & 1872 & 9869s & 0 & 1891 & 4521s & 0 & 1838 & 65s & 0 & 1424 & G & 0 & 1103 & G & 0 \\ 
tiffsplit & 858 & 1721 & 4s & 6 & 1712 & 17187s & 4 & 1697 & 8743s & 6 & 935 & 19s & 4 & 1155 & G & 2 & 1134 & G & 0 \\ 
tiff2bw & 858 & 1882 & 6s & 8 & 1829 & 13096s & 4 & 1861 & 7278s & 8 & 1263 & 13s & 1 & 1533 & G & 0 & 1435 & G & 0 \\ 
objdump & 324 & 3629 & 25s & 0 & 3667 & 19014s & 0 & 3731 & 9879s & 0 & 2422 & 1143s & 0 & 2624 & G & 1 & 2275 & G & 0 \\ 
tcpdump & 451 & 11594 & 59s & 0 & 10465 & 19800s & 0 & 10827 & 7126s & 0 & 7355 & 2077s & 1 & 5948 & G & 0 & 4499 & G & 0 \\ 
mujs & 451 & 4153 & 0s & 0 & 3973 & 15638s & 0 & 4027 & 6055s & 0 & 2421 & 8605s & 0 & 2590 & G & 1 & 2418 & G & 0 \\ 
size & 324 & 1752 & 4s & 0 & 1733 & 7343s & 0 & 1747 & 3455s & 0 & 1672 & 128s & 0 & 1331 & G & 0 & 1225 & G & 0 \\ 
infotocap & 432 & 1824 & 131s & 7 & 1782 & 33321s & 6 & 1679 & 34827s & 5 & 895 & 160s & 0 & 1164 & G & 0 & 1308 & G & 0 \\ 
imginfo & 432 & 1625 & 2s & 0 & 1494 & 26077s & 0 & 1611 & 24070s & 0 & 1307 & 43s & 0 & 1413 & G & 0 & 1105 & G & 0 \\

\midrule
\textbf{Total} & ~ & \textbf{39422} & & \textbf{40} & 37895 & & 21 & 38283 & & 37 & 27698 & & 25 & 26724 & & 5 & 22971 & & 1 \\ 


% tiff2pdf &448 &4383(99s) &4493(39407s) &4449(12856s) &2459(58s) &3398(G) &2709(G\tnote{1}~) \\
% readelf &324 &4983(34s) &4875(13088s) &4763(5978s) &5131(299s) &4144(G) &3760(G) \\
% % exiv2 &5748 &3639(229s) &3547(39426s) &3741(26408s) &4261(580s) &3718(G) &779(G) \\
% nm &324 &1876(2s) &1872(9869s) &1891(4521s) &1838(65s) &1424(G) &1103(G) \\
% tiffsplit &858 &1721(4s) &1712(17187s) &1697(8743s) &935(19s) &1155(G) &1134(G) \\
% tiff2bw &858 &1882(6s) &1829(13096s) &1861(7278s) &1263(13s) &1533(G) &1435(G) \\
% objdump &324 &3629(25s) &3667(19014s) &3731(9879s) &2422(1143s) &2624(G) &2275(G) \\
% tcpdump &451 &11594(59s) &10465(19800s) &10827(7126s) &7355(2077s) &5948(G) &4499(G) \\
% mujs &451 &4153(0s) &3973(15638s) &4027(6055s) &2421(8605s) &2590(G) &2418(G) \\
% size &324 &1752(4s) &1733(7343s) &1747(3455s) &1672(128s) &1331(G) &1225(G) \\
% infotocap &432 &1824(131s) &1782(33321s) &1679(34827s) &895(160s) &1164(G) &1308(G) \\
% imginfo &432 &1625(2s) &1494(26077s) &1611(24070s) &1307(43s) &-\tnote{2} &- \\
% \midrule
% \textbf{Total} & & \textbf{39422} &37895 &38283 &27698 &25311 &21866 \\

\bottomrule
\end{tabular}
\begin{tablenotes}[para]
\item[1]G: A GPU is required to train the model.
\end{tablenotes}
\end{threeparttable}
}

\label{seeds_1000}
\end{table*}

\subsection{\tool{} vs. Byte Schedule-Reinforced Fuzzers}
In this section, we compare \tool{} with five state-of-the-art byte schedule-reinforced fuzzers. We analyze their performance on three sets of initial seeds with different lengths, observing their effectiveness in edge coverage, bug detection, and analysis time.

\subsubsection{Compared Fuzzers}
There are three main types of existing methods for identifying important bytes in seed files, including inference-based fuzzers, neural network-based fuzzers, and taint-based fuzzers. In order to compare the performance of \tool{} with these three category fuzzers in different scenarios, we designed a diverse set of experiments to analyze the pros and cons of each fuzzer. 
Specifically, we compared \tool{} with five state-of-the-art fuzzers that are Greyone~\cite{greyone}, ProFuzzer~\cite{profuzzer}, NEUZZ~\cite{neuzz}, PreFuzz~\cite{prefuzz} and Angora\cite{angora}.


\textbf{Inference-based fuzzer.}
Inference-based fuzzers mutate all bytes of a seed before scheduling mutation, and determine the importance of each byte based on its execution, such as Greyone~\cite{greyone} and ProFuzzer~\cite{profuzzer}. Greyone iterates over each byte in the input, observing whether the state of a CMP instruction in the program changes. If it does, then the byte is related to the target CMP. ProFuzzer iterates over all 256 values at each byte and determines the type of each byte (e.g., size and offset) based on changes in the path length. However, since these two fuzzers are not open-sourced, we implement their core ideas based on AFL++. For GreyOne, we mutate each byte of the seed and observe whether the number of CMPs with unexplored branches changes. If it does, we consider the byte to be CMP-related. For ProFuzzer, we mutate each byte of the seed four times and observe whether the execution path changes. If it does, we consider the byte to be control flow-related. Finally, we randomly mutate the identified CMP-related bytes or control flow-related bytes.

\textbf{Neural network-based fuzzer.}
Neural network-based fuzzers refer to \todo{the ones} that use neural networks to identify the important bytes of a seed, such as NEUZZ~\cite{neuzz} and PreFuzz~\cite{prefuzz}. NEUZZ identifies bytes related to program branches using deep learning models. PreFuzz optimizes the edge and byte selection mechanism of NEUZZ.

\textbf{Taint-based fuzzer.}
Taint-based fuzzers refer to fuzzers that use taint analysis to analyze the bytes related to path constraints, such as Angora~\cite{angora}. Angora uses byte-level taint analysis to track which input bytes are related to path constraints.




\subsubsection{Experiment Setup}
% We selected 16 commonly used programs for testing from UNIFUZZ and other papers, as shown in the Table \ref{programsUNIFUZZ}.
% For each target program, all fuzzers use the same initial seeds, which are collected from UNIFUZZ, FuzzBench\cite{fuzzbench}, MAGMA or public seed corpus. 
% Most target programs have multiple initial seeds as suggested by Adrian Herrera~\cite{herrera2021seed}.
The recognition of important bytes by inference-based fuzzers, neural network-based fuzzers, and taint-based fuzzers is significantly influenced by the length of the seed. The longer the seed, the longer the analysis time required by these methods. Seeds with long length may fail the execution of existing fuzzers. However, \tool{} does not need to analyze each byte of the seed one by one, nor does it require building a neural network model. Therefore, the analysis time of \tool{} is not significantly affected by the length of the seed. To analyze the performance of each fuzzer on initial seeds of different lengths, we divide the initial seeds into three groups based on their length and conduct experiments on each of them separately. The length related groups are \texttt{ALL SEEDS}, \texttt{SEEDS<10000} (seeds \todo{that have} less than 10,000 bytes), and \texttt{SEEDS<1000} (seeds \todo{that have} less than 1,000 bytes). We analyze the analysis time, edge coverage, and bug discovery of each fuzzer in the three experimental environments. All experiments run for 24 hours and repeat 5 times.


\subsubsection{Edge Coverage and Analysis Time}
Tables \ref{all_seeds}, \ref{seeds_10000} and \ref{seeds_1000} show the edge coverage and analysis time achieved by six fuzzers on three sets of different initial seeds. From Table \ref{all_seeds}, with all the initial seeds provided, \tool{} discovers a total of 59681 edges, which are 4170 more edges than the second best fuzzer, ProFuzzer. Notably, NEUZZ and PreFuzz only discover 20213 and 23470 edges (about 1/3 edges discovered by \tool{}) respectively on 16 programs. On programs like \texttt{lame}, NEUZZ and PreFuzz fail to run the fuzzer because of long seed lengths, 
% resulting in a model that is too large and further causing an OOM error during training.
resulting in a large model that causes an OOM error during training.
As for analysis time, \tool{} consistently requires less time to analyze all programs compared to other fuzzers. For example, \tool{} uses less than 1000 seconds to analyze 13 programs, while GreyOne and ProFuzzer require more than 10000 seconds for most programs. This is because GreyOne and ProFuzzer have to analyze each byte of the seed before mutation, which means that \todo{the} analysis time is proportional to \todo{the} seed length. Angora requires less than 1000 seconds to analyze 7 programs, indicating that \todo{the} \tool{}'s analysis time is still superior to \todo{the} traditional taint analysis.
NEUZZ and PreFuzz require an additional GPU for analysis, which consumes a significant amount of resources.

From Table \ref{seeds_10000} and \ref{seeds_1000}, as the length of the seed decreases, the analysis time of all fuzzers decreases, particularly for GreyOne and ProFuzzer.
For example, with \texttt{ALL SEEDS}, ProFuzzer takes 81747 seconds to analyze \texttt{nm}, but with \texttt{SEED < 1000}, the analysis time \todo{decreases} to 4521 seconds.
Notably, \tool{} exhibits the most stable performance among the three experiments and consistently achieves the highest edge coverage on most programs.
Finally, \tool{} discovers the most total edges across all three experiments.


% \begin{table}[!t]
% \centering
% \caption{The number of unique bugs discovered by different
% fuzzers (on \texttt{ALL SEEDS}).}
% \resizebox{\linewidth}{!}{
% \begin{threeparttable}
% \begin{tabular}{@{\extracolsep{4pt}}cccccccccccc@{}} %crrrrrrrrrrr
% \toprule
% % \rotatebox{80}{\textbf{\tool-Redqueen\tnote{1}}}
% \textbf{Programs} & \textbf{\tool{}} & \textbf{GreyOne} & \textbf{ProFuzzer} & \textbf{Angora} & \textbf{PreFuzz} & \textbf{NEUZZ}\\
% \midrule

% tiff2pdf &0 &0 &1 &0 &1 &1 \\
% tiffsplit &7 &5 &6 &1 &2 &1 \\
% pdftotext &23 &2 &3 &2 &5 &0 \\
% % mujs &0 &0 &0 &0 &0 &0 \\
% infotocap &7 &6 &5 &0 &1 &0 \\
% lame &5 &4 &4 &4 &0 &0 \\
% readelf &4 &3 &6 &6 &0 &0 \\
% exiv2 &15 &5 &12 &11 &0 &0 \\
% flvmeta &2 &2 &2 &2 &0 &0 \\
% nm &17 &9 &10 &51 &0 &0 \\
% tiff2bw &6 &6 &5 &1 &0 &0 \\
% objdump &14 &4 &5 &3 &0 &0 \\
% mp42aac &2 &0 &0 &0 &0 &0 \\
% tcpdump &1 &1 &0 &3 &0 &0 \\
% % imginfo &0 &0 &0 &0 &0 &0 \\
% \midrule
% \textbf{Total} & \textbf{103} &47 &59 &84 &9 &2 \\


% \bottomrule
% \end{tabular}
% \end{threeparttable}
% }

% \label{all_seeds}
% \end{table}

% \begin{table}[!t]
% \centering
% \caption{The number of unique bugs discovered by different
% fuzzers (on \texttt{SEEDS<10000}).}
% \resizebox{\linewidth}{!}{
% \begin{threeparttable}
% \begin{tabular}{@{\extracolsep{4pt}}cccccccccccc@{}} %crrrrrrrrrrr
% \toprule
% % \rotatebox{80}{\textbf{\tool-Redqueen\tnote{1}}}
% \textbf{Programs} & \textbf{\tool{}} & \textbf{GreyOne} & \textbf{ProFuzzer} & \textbf{Angora} & \textbf{PreFuzz} & \textbf{NEUZZ}\\
% \midrule

% tiff2pdf &1 &0 &0 &0 &0 &0 \\
% readelf &5 &6 &3 &7 &6 &4 \\
% nm &30 &20 &22 &35 &14 &0 \\
% tiffsplit &6 &6 &7 &3 &2 &0 \\
% objdump &16 &10 &13 &13 &4 &0 \\
% tcpdump &1 &1 &0 &1 &1 &0 \\
% mujs &0 &0 &0 &0 &1 &0 \\
% infotocap &8 &5 &2 &0 &1 &0 \\
% % imginfo &0 &0 &0 &0 &0 &0 \\
% exiv2 &7 &4 &3 &9 &0 &0 \\
% tiff2bw &7 &6 &6 &1 &0 &0 \\
% size &0 &0 &0 &1 &0 &0 \\
% \midrule
% \textbf{Total} & \textbf{81} &58 &56 &70 &29 &4 \\


% \bottomrule
% \end{tabular}
% \end{threeparttable}
% }

% \label{seeds_10000}
% \end{table}


% \begin{table}[!t]
% \centering
% \caption{The number of unique bugs discovered by different
% fuzzers (on \texttt{SEEDS<1000}).}
% \resizebox{\linewidth}{!}{
% \begin{threeparttable}
% \begin{tabular}{@{\extracolsep{4pt}}cccccccccccc@{}} %crrrrrrrrrrr
% \toprule
% % \rotatebox{80}{\textbf{\tool-Redqueen\tnote{1}}}
% \textbf{Programs} & \textbf{\tool{}} & \textbf{GreyOne} & \textbf{ProFuzzer} & \textbf{Angora} & \textbf{PreFuzz} & \textbf{NEUZZ}\\
% \midrule

% tiff2pdf &1 &0 &1 &0 &1 &1 \\
% tiffsplit &6 &4 &6 &4 &2 &0 \\
% objdump &0 &0 &0 &0 &1 &0 \\
% tcpdump &0 &0 &0 &1 &0 &0 \\
% mujs &0 &0 &0 &0 &1 &0 \\
% infotocap &7 &6 &5 &0 &0 &0 \\
% readelf &4 &3 &0 &5 &0 &0 \\
% exiv2 &14 &4 &17 &14 &0 &0 \\
% tiff2bw &8 &4 &8 &1 &0 &0 \\
% % imginfo &0 &0 &0 &0 &0 &0 \\
% \midrule
% \textbf{Total} & \textbf{40} &21 &37 &25 &5 &1 \\


% \bottomrule
% \end{tabular}
% \end{threeparttable}
% }

% \label{seeds_1000}
% \end{table}


\subsubsection{Unique Bugs}
Tables \ref{all_seeds}, \ref{seeds_10000} and \ref{seeds_1000} \todo{present} the number of unique bugs discovered by each fuzzer on three sets of initial seeds.
In all cases, \tool{} is able to discover more unique bugs than other fuzzers. On \texttt{ALL SEEDS}, \tool{} finds 103 unique bugs, which is 19 more than the best performing comparison fuzzer, Angora. On \texttt{SEEDS<10000}, \tool{} discovers 81 unique bugs, which is 11 more than the second-ranked fuzzer, Angora. On \texttt{SEEDS<1000}, \tool{} discovers 40 unique bugs, which is 3 more than the best performing comparison fuzzer, ProFuzzer.
Notably, we find that a fuzzer's performance in terms of edge coverage and bug discovery is not always consistent. For example, although Angora does not perform as well as GreyOne and ProFuzzer in terms of edge coverage, it still discover more bugs. However, \tool{} achieves the best performance in both edge coverage and bug discovery.

% \textbf{Conclusion.} \tool{}'s performance is less affected by the length of the initial seed. Compared to other three-class fuzzers, \tool{} consistently achieved the highest edge coverage, most unique bugs, and shortest analysis time across different lengths of initial seeds.
}

\subsection{\tool{} vs. Commonly Used Fuzzers}
In this section, we compare \tool{} with some commonly used fuzzers to further demonstrate its superior performance. 
To ensure fair results, we conduct our experiments on two third-party testing platforms, UNIFUZZ~\cite{unifuzz} and MAGMA~\cite{magma}.
All experiments run for 24 hours and repeat 10 times to avoid the randomness of fuzzing~\cite{bohme2022reliability}.


\subsubsection{Compared Fuzzers}
We compare \tool{} with the state-of-the-art CGFs, including AFL~\cite{afl}, AFL++~\cite{aflpp}, AFLFast~\cite{aflfast}, FairFuzz~\cite{fairfuzz}, MOPT~\cite{MOPT}, and EMS~\cite{ems}.
In this section, we implement AFL, AFLFast, MOPT and FairFuzz as a mode in AFL++.
AFL is a popular fuzzer that is the basis of many other recent fuzzers~\cite{aflfast, fairfuzz, MOPT, Yue2020EcoFuzz, ems, neuzz}. 
AFL++ is a framework that integrates many state-of-the-art fuzzers into AFL, such as MOPT, AFLfast and Redqueen.
In our evaluation, We enable AFL++'s Redqueen mutator and MOPT mutator, which is the best-performing configuration of AFL++.
AFLFast models the fuzzing process as a Markov chain and prioritizes low-frequency paths to achieve better code coverage. FairFuzz proposes a novel mutation mask to guide fuzzing towards rare branches. MOPT utilizes Particle Swarm Optimization to optimize the schedule of mutation operators based on fuzzing history. 
% EMS proposes a probabilistic byte orientation model based on the information of intra- and inter-trial history. 
% Note that, on UNIFUZZ, the comparing fuzzers are implemented based on AFL++ (except EMS), while on MAGMA, we use the original implementations of those fuzzers.
For MOPT and MOPT related fuzzers, we set $-L = 5$. 
%Each MOPT-based fuzzer employs ‘-L 5’ as the configuration in the evaluation.
%Chenyang Lyu
%\cite{ems}

\subsubsection{Edge Coverage}
To evaluate the efficiency of edge discovery, we evaluate fuzzers by using the ranks of edge discovery after fuzzing 1/3/24 hours. The lower the rank is, the better the fuzzer performs. As shown in Figure~\ref{average_ranks}, the performance of most fuzzers at different running hours is not significantly different.
Yet, Figure~\ref{average_ranks} indicates that \tool{} achieves better code coverage on most programs than other fuzzers.
After fuzzing for 1 and 3 hours, the median rank of \tool{} is 1.5 and 1.5, respectively, which indicates that the fuzzing efficiency of \tool{} in a short period of time is higher.
% After fuzzing 1 hour and 3 hours, the median of \tool{} performs the best among all fuzzers, and the second best is AFL++. Specifically, after one and three hours of fuzzing, ShapFuzz discover the most new edges on A and B Programs, respectively.
% Specifically, after fuzzing 1 hour and 3 hours, the median of \tool{} performs the best among all fuzzers, and the second best is AFL++.
% We focus on the analysis of the four strongest fuzzers, namely \tool{}, \tool{}-Redqueen, MOPT and AFL++.
After fuzzing 24 hours, the median rank of \tool{} is 1.81. 
This indicates that \tool{}'s strategy is more efficient than MOPT whose the median rank is 4.75. 
% After combining Redqueen's strategy, the median of ranks of \tool{}-Redqueen and AFL++ are 1.18 and 2.68, respectively.
% Our \tool{}-Redqueen performs better than AFL++ in terms of edge discovery.

\begin{figure}[!t]
\includegraphics[width=\linewidth]{images/average_ranks.png}
\caption{The violin plot of average edge ranks across 10 trails of different fuzzers after running for 1/3/24 hours. 
% \tool{} ranks the highest in terms of edge discovery.
}
\label{average_ranks}
\end{figure}


\begin{table}[!t]
\centering
\caption{The number of unique bugs discovered by different fuzzers (on UNIFUZZ).}
\resizebox{\linewidth}{!}{
\begin{threeparttable}
\begin{tabular}{@{\extracolsep{4pt}}cccccccccccc@{}} %crrrrrrrrrrr
\toprule

% \textbf{Programs} &  \textbf{ShapR\tnote{1}} & \textbf{\tool{}} & \textbf{AFL++} & \textbf{MOPT} & \textbf{AFL} & \textbf{AFLFast} & \textbf{FairFuzz}\\
% \midrule
% tiff2pdf          &       1 &      1 &           \textbf{2} &   1 &      0 &   0 &   0 \\
% lame              &       4 &      4 &            4 &   4 &      \textbf{5} &   4 &   4 \\
% readelf        &       \textbf{8} &      6 &            4 &   4 &      3 &   5 &   5 \\
% exiv2             &      \textbf{31} &     18 &           23 &   3 &     15 &  15 &  14 \\
% flvmeta           &       2 &      2 &            2 &   2 &      2 &   2 &   2 \\
% nm             &      34 &     \textbf{35} &           31 &  21 &     22 &  22 &  30 \\
% tiffsplit         &      \textbf{10} &      7 &            9 &   7 &      5 &   7 &   5 \\
% tiff2bw           &      \textbf{10} &     \textbf{10} &            6 &   5 &      5 &   5 &   7 \\
% objdump        &      23 &     \textbf{29} &           11 &   8 &     12 &  10 &   8 \\
% pdftotext         &      17 &     \textbf{27} &           24 &  20 &     25 &  24 &  23 \\
% mp42aac           &       \textbf{7} &      0 &            5 &   0 &      0 &   0 &   0 \\
% tcpdump           &       1 &      \textbf{2} &            1 &   0 &      \textbf{2} &   1 &   \textbf{2} \\
% infotocap         &      \textbf{11} &     \textbf{11} &            9 &   9 &      5 &   9 &   9 \\
% imginfo           &       1 &      0 &            1 &   0 &      \textbf{2} &   0 &   0 \\

\textbf{Programs} & \textbf{\tool{}} & \textbf{AFL++} & \textbf{MOPT} & \textbf{AFL} & \textbf{AFLFast} & \textbf{FairFuzz}\\
\midrule
tiff2pdf           &      1 &           2 &   1 &      0 &   0 &   0 \\
lame               &      4 &            4 &   4 &      5 &   4 &   4 \\
readelf         &      6 &            4 &   4 &      3 &   5 &   5 \\
exiv2              &     18 &           23 &   3 &     15 &  15 &  14 \\
flvmeta            &      2 &            2 &   2 &      2 &   2 &   2 \\
nm              &     35 &           31 &  21 &     22 &  22 &  30 \\
tiffsplit          &      7 &            9 &   7 &      5 &   7 &   5 \\
tiff2bw            &     10 &            6 &   5 &      5 &   5 &   7 \\
objdump         &     29 &           11 &   8 &     12 &  10 &   8 \\
pdftotext          &     27 &           24 &  20 &     25 &  24 &  23 \\
mp42aac            &      0 &            5 &   0 &      0 &   0 &   0 \\
tcpdump            &      2 &            1 &   0 &    2 &   1 &   2 \\
infotocap          &    11 &            9 &   9 &      5 &   9 &   9 \\
imginfo            &      0 &            1 &   0 &     2 &   0 &   0 \\


\midrule
\textbf{Total}  &  \textbf{152} & 132  & 84  & 103 & 104 & 109\\


\bottomrule
\end{tabular}
\end{threeparttable}
}

\label{unifuzz_bug}
\end{table}

% \subsection{Bug Discovery on UNIFUZZ}
\subsubsection{Bug Discovery on UNIFUZZ}
\begin{sloppypar}
We analyze the number of unique bugs triggered by a fuzzer based on ASAN. Following the guidance of UNIFUZZ~\cite{unifuzz}, we select the top three stack frames to de-duplicate bugs. 
Table~\ref{unifuzz_bug} shows the number of unique bugs triggered by each fuzzer. \tool{}, MOPT, AFLFast, FairFuzz, AFL, and AFL++ trigger 152, 84, 103, 104, 109 and 132 bugs, respectively. 
\tool{} finds the most bugs in 16 programs, with 20 more bugs than AFL++. 
% This indicates that \tool{} can be integrated with other strategies (\eg Redqueen) and achieves better results.
Specifically, \tool{} performs the best on 8 programs, including \texttt{nm}, \texttt{readelf}, \texttt{flvmeta}, \texttt{tiff2bw}, \texttt{objdump}, \texttt{pdftotext}, \texttt{tcpdump} and \texttt{infotocap}. 
% \tool{}-Redqueen performs the best on 6 programs, including \texttt{readelf}, \texttt{exiv2}, \texttt{tiffsplit}, \texttt{tiff2bw}, \texttt{mp42aac} and \texttt{infotocap}. 
Surprisingly, MOPT and AFLFast do not perform the best on any program. 
AFL++, AFL and FairFuzz only perform the best on 5, 3 and 1 programs, respectively.
In summary, \tool{} performs the best on most of the programs.
The bug discovery experiment results demonstrate the effectiveness of \tool{}. 
% The positions extracted by \tool{} can improve the fuzzing performance.

Furthermore, we use \tool{} to test some of the latest versions of programs and successfully found several previously unknown bugs. The results are shown in the Table~\ref{latestVersion}.
We find 11 bugs in 6 programs. Particularly, two bugs have been confirmed by developers as previously undiscovered bugs, and one bug has been fixed in the beta version.
The remaining 8 bugs are still being confirmed.
\end{sloppypar}








\begin{table}[!t]
\centering
\caption{New bugs discovered by \tool{} on the latest versions of programs.}
\resizebox{0.9\linewidth}{!}{
\begin{threeparttable}
\begin{tabular}{@{\extracolsep{4pt}}lccc@{}} %crrrrrrrrrrr
\toprule
% \rotatebox{80}{\textbf{\tool-Redqueen\tnote{1}}}
\textbf{Programs} & \textbf{Known Vulnerabilities}  & \textbf{Unknown Vulnerabilities} & \textbf{Sum}\\
\midrule
infotocap & 0 & 1 & 1\\
imginfo & 0 & 1 & 1\\
mp42aac & (submitted)\tnote{1} & (submitted) & 2\\
jhead & (submitted) & (submitted) & 4\\
cflow & (submitted) & (submitted) & 2\\
mujs & 1 & 0 & 1\\
\hline
Total & & & 11 \\
\bottomrule
\end{tabular}
\begin{tablenotes}[para]
(submitted): We have submitted the bugs and have no response yet. 
\end{tablenotes}
\end{threeparttable}
}
\label{latestVersion}
\end{table}


\subsubsection{Overhead}
\tool{} adds some extra steps to AFL++, including tracing mutators, recovering mutators, and calculating the Shapley Values of bytes. Thus, to quantify the influence of these steps on fuzzing throughput (\ie execution speed), we measure the total number of executions for each fuzzer. Figure~\ref{throughput} shows the total number of executions of all 16 programs that fuzzers run after 24 hours.
The results show that the throughput of \tool{} does not drop significantly comparing to other fuzzers.
After fuzzing 24 hours, the throughput of \tool{} is lower than that of MOPT, AFL++, AFL and AFLFast by 6.16\%, 7.91\%, 10.25\%, 8.38\%, respectively.
However, the total throughput of \tool{} is higher than FairFuzz by 9.75\%.
Surprisingly, on programs \texttt{tiffsplit} and \texttt{exiv2}, the throughput of \tool{} is higher than AFL++, MOPT, AFL and FairFuzz. 
Therefore, our \tool{} does not introduce much overhead.

\begin{figure}[h!]
\includegraphics[width=\linewidth]{images/throughput.png}
\caption{The total throughput of different fuzzers running for 24 hours.}
\label{throughput}
\end{figure}


\subsubsection{Evaluation on MAGMA}




\begin{table}[!t]
% \renewcommand\arraystretch{1}
\centering
\caption{Target programs from MAGMA.}\label{programsMAGMA}
\resizebox{0.9\linewidth}{!}{
\begin{threeparttable}
\begin{tabular}{llll}
    \toprule
    \textbf{Projects} & \textbf{Target Programs} & \textbf{Input format}\\ \midrule
    % \multirow{2}{*}{\textbf{libpng 1.6.38}} & \multirow{2}{*}{read$\_$fuzzer, readpng} & \multirow{2}{*}{PNG}\\
    \textbf{libpng 1.6.38} & libpng\_read\_fuzzer & PNG\\
    \midrule
    \textbf{libtiff 4.1.0} & read\_rgba\_fuzzer, tiffcp & TIFF\\
    \midrule
    \multirow{2}{*}{\textbf{libxml2 2.9.10}} & \multirow{2}{*}{\makecell[c]{libxml2\_xml\_read\_memory\_fuzzer, \\ xmllint}} & \multirow{2}{*}{XML}\\
    &&\\
    \midrule
    \textbf{poppler 0.88.0} & pdf\_fuzzer, pdfimages & PDF\\
    \midrule
    \multirow{3}{*}{\textbf{openssl 3.0.0}} & \multirow{3}{*}{\makecell[c]{asn1, asn1parse, bignum, server, \\ client, x509}} & \multirow{3}{*}{Binary blobs}\\
    &&\\
    &&\\
    \midrule
    \textbf{sqlite3 3.32.0} & sqlite3\_fuzz & SQL queries\\
    \midrule
    \multirow{2}{*}{\textbf{php 8.8.0}} & \multirow{2}{*}{\makecell[c]{exif, json, parser, \\ unserialize}} & \multirow{2}{*}{Various}\\
    &&\\
    \midrule
    \textbf{libsndfile } & sndfile\_fuzzer & WAV\\
    \midrule
    \textbf{lua } & lua & LUA\\
    \bottomrule
\end{tabular}
\end{threeparttable}

}
\end{table}

To further evaluate the bug-finding performance of \tool{}, we conduct experiments on MAGMA.
MAGMA is a ground-truth fuzzing benchmark that enables accurate and consistent fuzzing evaluation. MAGMA provides several benchmarks with real-world bugs, and it can perform a realistic evaluation of fuzzers.
We integrate our \tool{} into MAGMA, and compare them to 5 widely-used mutation-based fuzzers (\ie AFL, AFLFast, FairFuzz, MOPT and AFL++). AFL++ is the AFL++ that enables both MOPT and Redqueen. Due to configure issues of MAGMA, we use the original implementations of fuzzers rather than the implementations based on AFL++. Table~\ref{programsMAGMA} shows the target programs used in MAGMA.



\textbf{Bug Discovery.}
Table~\ref{magma_unique_bugs} shows the number of CVEs triggered by each fuzzer on average. 
It shows that \tool{} performs the best on MAGMA in terms of bug discovery on average.
\tool{} exposes the most bugs on 7 of 9 programs.  

Specifically, \tool{} performs the best on \texttt{libsndfile}, \texttt{libxml2}, \texttt{lua}, \texttt{openssl}, \texttt{php}, \texttt{poppler} and \texttt{sqlite3}, exposing 7.00, 4.22, 1.00, 4.00, 3.00, 5.56 and 4.56 bugs on average, respectively.
% \tool{}-Redqueen performs the best on \texttt{libpng}, \texttt{libsndfile}, \texttt{libtiff}, \texttt{libxml2} and \texttt{lua}, finding 2.56, 7.00, 6.33, 4.22 and 1.00 bugs on average, respectively.
Moreover, \tool{} performs significantly better than all the other fuzzers on \texttt{openssl}, \texttt{poppler} and \texttt{sqlite3}.
On \texttt{splite3}, \tool{} discovers almost two times the number of bugs compared to AFL++. 
Surprisingly, AFL++ only exposes the most bugs on 2 programs.



\begin{table}[h]
\centering
\caption{The average number of bugs found by different fuzzers (on MAGMA).}
\resizebox{\linewidth}{!}{
\begin{threeparttable}
\begin{tabular}{@{\extracolsep{4pt}}cccccccccccc@{}} %crrrrrrrrrrr
\toprule
%\rotatebox{80}{\textbf{Programs}}
% \textbf{Programs} & \textbf{\tool{}}& \textbf{ShapR\tnote{1}} &  \textbf{AFL++} & \textbf{AFL} & \textbf{AFLFast} & \textbf{FairFuzz} & \textbf{MOPT}\\
% \midrule
% libpng    & 1.44 & \textbf{2.56} &   2.22 & 1.89 & 1.00 & 1.56 & 1.56 \\
% libsndfile  & \textbf{7.00} & \textbf{7.00} & 6.89 & 2.89 & 2.33 & 1.44 & 4.78 \\
% libtiff   & 5.89 & \textbf{6.33}  &  6.22 & 5.44 & 4.22 & 4.67 & 5.67 \\
% libxml2   & \textbf{4.22} & \textbf{4.22}  &  4.00 & 1.00 & 1.89 & 1.00 & 2.78 \\
% lua       & \textbf{1.00} & \textbf{1.00}  &  0.56 & \textbf{1.00} & \textbf{1.00} & 0.89 & \textbf{1.00} \\
% openssl    & \textbf{4.00} & 3.56 &  2.67 & 3.11 & 3.33 & 2.44 & 3.00 \\
% php        & \textbf{3.00} & 2.56 &  2.00 & \textbf{3.00} & \textbf{3.00} & 2.56 & \textbf{3.00} \\
% poppler    & \textbf{5.56} & 5.44 &  4.33 & 3.00 & 3.44 & 2.22 & 3.44 \\
% sqlite3    & \textbf{4.56} & 3.78 &  2.56 & 0.89 & 1.78 & 0.89 & 0.67 \\
% \midrule
% \#The Best\tnote{2} & \textbf{7} & 5 & 0 & 2 & 2 & 0 & 2\\

\textbf{Programs} & \textbf{\tool{}} &  \textbf{AFL++} & \textbf{AFL} & \textbf{AFLFast} & \textbf{FairFuzz} & \textbf{MOPT}\\
\midrule
libpng    & 1.44  &   \textbf{2.22} & 1.89 & 1.00 & 1.56 & 1.56 \\
libsndfile  & \textbf{7.00}  & 6.89 & 2.89 & 2.33 & 1.44 & 4.78 \\
libtiff   & 5.89   &  \textbf{6.22} & 5.44 & 4.22 & 4.67 & 5.67 \\
libxml2   & \textbf{4.22}   &  4.00 & 1.00 & 1.89 & 1.00 & 2.78 \\
lua       & \textbf{1.00}   &  0.56 & \textbf{1.00} & \textbf{1.00} & 0.89 & \textbf{1.00} \\
openssl    & \textbf{4.00}  &  2.67 & 3.11 & 3.33 & 2.44 & 3.00 \\
php        & \textbf{3.00}  &  2.00 & \textbf{3.00} & \textbf{3.00} & 2.56 & \textbf{3.00} \\
poppler    & \textbf{5.56}  &  4.33 & 3.00 & 3.44 & 2.22 & 3.44 \\
sqlite3    & \textbf{4.56}  &  2.56 & 0.89 & 1.78 & 0.89 & 0.67 \\
\midrule
\#The Best\tnote{1} & \textbf{7}  & 2 & 2 & 2 & 0 & 2\\
\bottomrule
\end{tabular}
\begin{tablenotes}[para]
\item[1]\#The Best: the number of programs that a fuzzer performs the best.
\end{tablenotes}
\end{threeparttable}
}
\label{magma_unique_bugs}
\end{table}


\textbf{Time to Bug.}
We analyze the first time that each bug is found and the results are shown in the Table~\ref{TTB}. 
In 10 trails, a total of 48 bugs are found by these 7 fuzzers. Among them, \tool{} performs the best, with a total of 46 discovered bugs. 
Additionally, among the bugs discovered by \tool{}, 7 bugs cannot be exposed by AFL++, MOPT, FairFuzz, AFL and AFLFast.
As for TTB, \tool{} has the least time to bug (TTB) on 20 programs, which is the best performance among fuzzers.
% Among the fuzzers used for comparison, AFL++ performed the best, finding 40 bugs. 
For example, for 25 bugs, \tool{} discovers them 2$\times$ faster than AFL++.
% \zkp{
Note that, \texttt{CVE-2017-2518} and \texttt{CVE-2019-19317} can only be discovered by \tool{}.
\texttt{CVE-2017-9776}, \texttt{CVE-2013-7443}, \texttt{CVE-2019-19880}, \texttt{PDF008} and \texttt{CVE-2019-19646} can only be exposed by \tool{}.
% }
Due to the advantage of solving path constraints, \tool{} exposes bugs in less time than others.


\begin{table}[!t]
\centering
\caption{The time to bug (TTB) of fuzzers (on MAGMA). \tool{} performs the best in discovering bugs.}
\resizebox{\linewidth}{!}{
\begin{threeparttable}
\begin{tabular}{@{\extracolsep{4pt}}crrrrrrrrrrr@{}}
\toprule
% \rotatebox{80}{\textbf{Vulnerabilities}}
\rotatebox{0}{\textbf{Vulnerabilities}} & \rotatebox{60}{\textbf{\tool{}}}   & \rotatebox{60}{\textbf{AFL++}} & \rotatebox{60}{\textbf{MOPT}} & \rotatebox{60}{\textbf{FairFuzz}}  &  \rotatebox{60}{\textbf{AFL}} & \rotatebox{60}{\textbf{AFLFast}} \\
\midrule

\rowcolor{gray!20} CVE-2015-8472 & 17s & 23s & \textbf{15s} & \textbf{15s} & \textbf{15s} & \textbf{15s} \\ 
CVE-2016-1762 & 47s & 1m & \textbf{15s} & 20s & 16s & 18s \\
\rowcolor{gray!20} CVE-2018-13988 & 1m & 1m & \textbf{52s} & 2m & 1m & 1m \\
CVE-2016-2109 & 3m & 4m & \textbf{1m} & 2m & \textbf{1m} & 2m \\
\rowcolor{gray!20} CVE-2016-6309 & 4m & 5m & \textbf{1m} & 2m & \textbf{1m} & \textbf{1m} \\
CVE-2016-10270 & \textbf{23s} & 48s & 19m & 3m & 23m & 11m \\
\rowcolor{gray!20} CVE-2016-3658 & \textbf{4m} & 17m & 1h & 25m & 1h & 1h \\
CVE-2018-14883 & 18m & 1h & 3m & 2h & \textbf{2m} & 3m \\
\rowcolor{gray!20} CVE-2017-6892 & \textbf{13m} & 32m & 33m & 3h & \textbf{13m} & 1h \\
SND017 & \textbf{4m} & 5m & 25m & 21h & 38m & 5m \\
\rowcolor{gray!20} CVE-2017-11613 & \textbf{9m} & 1h & 1h & 15h & 6h & 4h \\
CVE-2019-11034 & 6h & 15h & \textbf{1m} & 8m & 2m & \textbf{1m} \\
\rowcolor{gray!20} PDF010 & 3h & 1h & 7h & 16h & 10h & \textbf{2m} \\
CVE-2019-7663 & \textbf{3h} & 8h & 4h & 9h & 16h & 6h \\
\rowcolor{gray!20} CVE-2019-20218 & \textbf{49m} & 2h & 16h & 11h & 9h & 9h \\
CVE-2019-9638 & \textbf{41m} & 17h & 7h & 17h & 4h & 44m \\
\rowcolor{gray!20} CVE-2015-8317 & 22m & 1h & 3h & - & - & 12h \\
CVE-2019-7310 & 7h & 17h & 9h & 15h & 7h & 8h \\
\rowcolor{gray!20} CVE-2020-15945 & 5h & \textbf{4h} & 14h & 15h & 13h & 16h \\
SND020 & \textbf{16m} & 19m & 7h & 21h & - & - \\
\rowcolor{gray!20} CVE-2015-3414 & \textbf{1h} & 4h & 17h & 16h & 23h & 15h \\
CVE-2016-10269 & 2h & 1h & 15h & 22h & 15h & - \\
\rowcolor{gray!20} CVE-2011-2696 & 18m & 22m & 17h & - & 22h & 23h \\
CVE-2017-8363 & \textbf{13m} & 28m & 18h & 22h & - & - \\
\rowcolor{gray!20} CVE-2017-8363 & 27m & 32m & 18h & 22h & - & - \\
CVE-2017-9047 & 33m & 6h & 12h & - & - & - \\
\rowcolor{gray!20} CVE-2017-8361 & \textbf{14m} & 3h & 18h & 22h & - & - \\
CVE-2016-6302 & 9h & 23h & 16h & - & \textbf{3h} & 6h \\
\rowcolor{gray!20} CVE-2017-7375 & 6h & \textbf{1h} & - & - & - & - \\
CVE-2018-10768 & 5h & 5h & 23h & - & - & 23h \\
\rowcolor{gray!20} CVE-2016-5314 & 19h & 19h & 11h & 16h & \textbf{4h} & - \\
CVE-2013-6954 & 13h & 19h & 16h & 12h & \textbf{11h} & - \\
\rowcolor{gray!20} CVE-2019-19926 & \textbf{5h} & 19h & 17h & - & 21h & 20h \\
PNG006 & - & \textbf{6m} & - & - & - & - \\
\rowcolor{gray!20} CVE-2016-2108 & \textbf{3h} & 16h & 22h & - & - & - \\
CVE-2016-10269 & 23h & \textbf{2h} & 22h & - & - & - \\
\rowcolor{gray!20} CVE-2017-9865 & 8h & 12h & - & - & - & - \\
CVE-2015-8784 & 22h & 21h & 20h & \textbf{18h} & - & 20h \\
\rowcolor{gray!20} CVE-2016-1836 & \textbf{22h} & 23h & - & - & - & - \\
CVE-2017-14617 & - & \textbf{21h} & - & - & - & - \\
\rowcolor{gray!20} CVE-2017-3735 & 20h & - & \textbf{5h} & 15h & 22h & 10h \\
CVE-2017-9776 & 19h & - & - & - & - & - \\
\rowcolor{gray!20} CVE-2013-7443 & \textbf{17h} & - & - & - & - & - \\
CVE-2019-19880 & \textbf{18h} & - & - & - & - & - \\
\rowcolor{gray!20} PDF008 & \textbf{20h} & - & - & - & - & - \\
CVE-2019-19646 & 22h & - & - & - & - & - \\
\rowcolor{gray!20} CVE-2017-2518 & \textbf{22h} & - & - & - & - & - \\
CVE-2019-19317 & \textbf{22h} & - & - & - & - & - \\
\rowcolor{gray!50}\#The Fastest\tnote{1} & \textbf{20} & 5 & 7 & 2 & 8 & 4 \\

\bottomrule
\end{tabular}
\begin{tablenotes}[para]
\item[1]\#The Fastest: The number of vulnerabilities that are discovered the fastest by the fuzzer.
\end{tablenotes}
\end{threeparttable}
}
\label{TTB}
\end{table}



% \begin{table*}[!t]
% % \renewcommand\arraystretch{1.7}
% % \newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
% \centering
% \caption{The comparison of position inference. \tool{} can infer more useful positions within less inference time.}
% \resizebox{\linewidth}{!}{
% \begin{threeparttable}
% \begin{tabular}{@{\extracolsep{4pt}}lccccccccccccccc@{}}
% \toprule
% \multirow{3}{*}{\textbf{Programs}} & \multicolumn{3}{c}{\textbf{GreyOne}} & \multicolumn{3}{c}{\textbf{ProFuzzer}} & \multicolumn{3}{c}{\textbf{\tool}}\\
% \cline{2-4} \cline{5-7} \cline{8-10}


% &\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Analysis}\\ \textbf{Time(s)}\end{tabular}} 
% &\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Useful}\\ \textbf{Ratio}\end{tabular}} 
% &\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Average Useful}\\ \textbf{Mutation}\end{tabular}} 

% &\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Analysis}\\ \textbf{Time(s)}\end{tabular}} 
% &\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Useful}\\ \textbf{Ratio}\end{tabular}} 
% &\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Average Useful}\\ \textbf{Mutation}\end{tabular}} 

% &\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Analysis}\\ \textbf{Time(s)}\end{tabular}} 
% &\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Useful}\\ \textbf{Ratio}\end{tabular}} 
% &\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Average Useful}\\ \textbf{Mutation}\end{tabular}} \\
% &&&&&&&&&\\
% \midrule

% \textbf{nm} & 16721 & 3\%(135/4834) & 0.11 & 13584 & 16\%(109/665) & 0.32 & \textbf{16.68} & \textbf{67\%(55/82)} & \textbf{1.87}  \\
% \textbf{tiff2bw} & 8283 & 13\%(101/762) & 0.74 & 9372 & 14\%(106/762) & 0.75 & \textbf{7} & \textbf{89\%(74/83)} & \textbf{5.87}\\
% \textbf{tiffsplit} & 8875 & 68\%(104/152) & 3.18 & 10894 & 69\%(104/150) & 3.25 & \textbf{8} & \textbf{92\%(72/78)} & \textbf{6.60}\\
% \textbf{objdump} & 52080 & 2\%(205/13288) & 0.45 & 29901 & 18\%(318/1794) & 0.68 & \textbf{45} & \textbf{60\%(179/299)} & \textbf{1.70} \\
% \textbf{readelf} & 16739 & 3\%(99/3798) & 0.41 & 13712 & 7\%(186/2641) & 0.48 & \textbf{37} & \textbf{83\%(95/114)} & \textbf{8.70}\\
% \textbf{flvmeta} & 2262 & 46\%(29/63) & 1.28 & 2222 & 22\%(42/187) & 0.46 & \textbf{2} & \textbf{40\%(14/35)} & \textbf{1.08}\\
% \textbf{pdftotext} & 54447 & 3\%(267/8384) & 0.07 & 38144 & 4\%(337/8805) & 0.08 & \textbf{54} & \textbf{54\%(165/305)} & \textbf{1.11}\\
% \textbf{mp42aac} & 11855 & 19\%(124/651) & 0.32 & 17234 & 21\%(132/614) & 0.35 & \textbf{9} & \textbf{68\%(69/102)} & \textbf{1.70}\\
% \textbf{tcpdump} & 13219 & 2\%(88/4075) & 2.89 & 13774 & 3\%(87/2708) & 2.48 & \textbf{16} & \textbf{77\%(72/93)} & \textbf{6.36}\\
% \textbf{lame3.99.5} & 75520 & 1\%(169/13077) & 0.02 & 62433 & 1\%(179/13060) & 0.02 & \textbf{80} & \textbf{73\%(74/102)} & \textbf{2.16}\\

% \bottomrule
% \end{tabular}
% \end{threeparttable}
% }
% \label{Verification}
% \end{table*}





\subsection{Comparison with Byte Mutation Solution}

EMS is the latest fuzzer focusing on byte mutation, which reuses history byte values that trigger unique paths and crashes. 
Because some programs will occupy tens of GB of memory when tested by EMS (implementation issues of EMS), we run experiments with part of the programs on Table~\ref{programsUNIFUZZ}. To ensure data consistency, we use \textit{afl-showmap} of AFL++ to count the number of edges for EMS and \tool{}.
The results of edge coverage discovered by \tool{} and EMS are shown in the Figure~\ref{tool_vs_ems}. 
Except for the program \texttt{lame}, \tool{} performs better than EMS.
Specifically, the median of edge coverage discovered by \tool{} is higher than EMS by 6.78\%, 27.89\%, 16.10\%, 9.01\%, 43.13\%, 16.57\%, 2.37\%, 15.51\%, 5.00\%, 9.38\% and 3.27\% on \texttt{imginfo}, \texttt{infotocap}, \texttt{mp42aac}, \texttt{mujs}, \texttt{objdump}, \texttt{pdftotext}, \texttt{size}, \texttt{exiv2}, \texttt{tiff2bw}, \texttt{tiff2pdf} and \texttt{tiffsplit}, respectively.
As to the performance of unique bugs discovered by the two fuzzers, the results are shown in Table \ref{unifuzz_bug_ems}. \tool{} triggers more bugs on 6 programs, while EMS only triggers more bugs on 2 programs. 
% \tool{} and EMS perform the same on the remaining 2 programs. 
Our \tool{} discovers 90 bugs on these programs while EMS only discovers 39 bugs.




\begin{figure}[htbp]
\centering
\includegraphics[width=0.9\linewidth]{images/tool_vs_ems.png}
\caption{The boxplot of edge coverage for \tool{} and EMS. Y-axis: the number of discovered edges.}
\label{tool_vs_ems}
\end{figure}

\begin{table}[htbp]
\centering
\caption{The number of unique bugs discovered by \tool{} and EMS (on UNIFUZZ).}
\resizebox{0.4\linewidth}{!}{
\begin{threeparttable}
\begin{tabular}{@{\extracolsep{4pt}}lcc@{}} %crrrrrrrrrrr
\toprule
% \rotatebox{80}{\textbf{\tool-Redqueen\tnote{1}}}
\textbf{Programs} &   \textbf{EMS} & \textbf{\tool{}}\\
\midrule
lame       &  4 &     4 \\
exiv2      & 13 &    15 \\
tiffsplit  &  8 &     6 \\
tiff2bw    &  8 &     8 \\
objdump &  1 &    15 \\
pdftotext  &  1 &    25 \\
mp42aac    &  1 &     0 \\
infotocap  &  3 &    10 \\
tiff2pdf   &  0 &     2 \\
readelf &  0 &     5 \\
\hline
Total & 39 & \textbf{90} \\

\bottomrule
\end{tabular}
\end{threeparttable}
}
\label{unifuzz_bug_ems}
\end{table}




\subsection{Ablation Study of \tool{}}

\tool{} has two main components that are calculation of Shapley values (Sections~\ref{subsec:cg_all} and \ref{sec:shap_update}) and Shapley-guided byte selection (Section~\ref{subsec:mutate}).
Since Shapley-guided byte selection cannot be performed without Shapley values, we do not compare this component. Since the process of calculating the Shapley value introduces some additional mutations, we want to analyze the impact they have. To analyze the impact of calculating Shapley values, we implement \tool{}-modeling to compare with \tool{}. For \tool{}-modeling, we remove the Shapley-guided byte selection and randomly select positions to mutate.



% To analyze the impact of each component, we need to compare the performance of the following two variants of \tool{} that are \tool{}-modeling and \tool{}-mutation.
% For \tool{}-modeling (Section~\ref{subsec:cg_all}), the process of calculating the Shapley value introduces some additional mutations, and we want to analyze the impact they have. We remove the Shapley-guided mutation with CMAB of \tool{}. We randomly select positions on the seed to mutate. 
% For \tool{}-mutation (Section~\ref{subsec:mutate}), we remove modeling fuzzing as Shapley Analysis of \tool{}. However, Shapley-guided mutation with CMAB cannot be used without Shapley Analysis modeling. We thus do not consider this case.

% Therefore, we only need to compare the performance of \tool{} and \tool{}-modeling.
We evaluated two fuzzers \tool{} and \tool-modeling in UNIFUZZ for 24 hours for 5 times.
The result is shown in the Figure~\ref{ablation}.
With the help of Shapley-guided mutation, \tool{} discovers more new edges under most procedures. 
For instance, the median of \tool{} is higher than \tool-modeling on \texttt{objdump}, \texttt{nm}, \texttt{tiffsplit}, \texttt{lame}, \texttt{exiv2}, \texttt{tiff2bw}, \texttt{tcpdum} and \texttt{mp42aac}.
It illustrates that Shapley-guided mutation can indeed generate a more useful mutation possibility distribution for seeds.

\begin{figure}[t!]
\centering
\includegraphics[width=0.9\linewidth]{images/ablation.png}
\caption{ The boxplot of edge coverage for \tool{} and
\tool{}-modeling. Y-axis: the number of discovered edges.}
\label{ablation}
\end{figure}










\subsection{Comparison with Inference-based Fuzzers}
\balance
In this section, we compare \tool{} with inference-based fuzzers, including GreyOne~\cite{greyone} and ProFuzzer~\cite{profuzzer}, in terms of the effectiveness of inferred bytes. 
% For \tool{}, inferred bytes are the bytes that contribute to edge discovery (\ie non-zero Shapley values). For GreyOne and ProFuzzer, the inferred bytes are CMP-related bytes.
% If an inferred position can discover new code coverage in later fuzzing campaigns, it is an effective position.

% \noindent\textbf{Fuzzers.} 
% For \tool{}, if the Shapley value of a byte is greater than 0, then this byte is a Shapley byte.
% Since neither GreyOne nor ProFuzzer is open-source, we implement their core algorithms to identify the related bytes of path constraints. 
% For ProFuzzer, it iterates over all 256 values at each byte, and if the path length changes relative to the initial seed, the current byte is a CMP-related byte. 
% For GreyOne, it mutates 8 times at each byte, and if the value of a variable in a CMP instruction changes, the current byte is a CMP-related byte.

% Since neither GreyOne nor ProFuzzer is open-source, we implement their core algorithms to identify the related bytes of path constraints. 
% For ProFuzzer, it iterates over all 256 values at each byte, and if the path length changes relative to the initial seed, the current byte is related to a path constraint. 
% For GreyOne, it mutates 8 times at each byte, and if the value of a variable in a CMP instruction changes, the current byte is related to a path constraint.


\noindent\textbf{Experiment Setup.}
We randomly select 10 target programs and several initial seeds for experiments from UNIFUZZ.
To compare the efficiency gap between the Shapley bytes identified by \tool{} and the CMP-related bytes identified by GreyOne and ProFuzzer, we analyze each initial seed separately, and the specific experimental steps are as follows. 
For an initial seed, we use \tool{}, Greyone and ProFuzzer to infer the Shapley bytes or CMP-related bytes and mutate these bytes randomly for 3 hours, respectively. 
Then, we count the additional analysis time required by each fuzzer and the number of new edges they discover. In particular, for the convenience of comparison, we do not update the seed queue but continuously mutate the selected initial seed.

% We randomly select 10 target programs and several initial seeds for experiments from UNIFUZZ.
% To facilitate the comparison of effects, we analyze each initial seed separately, and the specific experimental steps are as follows. 
% For an initial seed, we use \tool{}, Greyone and ProFuzzer to mutate the target seed for 3 hours, respectively. 
% Then, we count the additional analysis time required by each fuzzer and the number of new edges they discover. In particular, for the convenience of comparison, we do not update the seed queue but continuously mutate the selected initial seed.

\noindent\textbf{Comparison Metrics.} 
We use the following two new metrics for fine-grained analysis of the above fuzzers:
\begin{itemize}
  % \item [1)]
  % \textit{Average analysis time}: The analysis time required by each fuzzer to infer CMP-related bytes or Shapley bytes. Both ProFuzzer and GreyOne use a pilot stage for inference. 
  % Since \tool{} does not contain a pilot stage, we regard the time of Shapley analysis as the analysis time.
  \item [1)] 
  \textit{The proportion of useful bytes}: If a byte is inferred and finds a new edge in the subsequent mutation process, it is called a useful byte. \textit{\textbf{For \tool{}, we do not count the first time when an inferred byte is retained.}} We record the proportion of useful bytes in all inferred bytes.
  \item [2)] 
  \textit{The average number of useful mutations}: If the mutation of inferred bytes finds a new edge, this mutation is a useful mutation.
  We use this metric to describe the importance of each byte. 
  If a byte has more useful mutations, it is more important.
\end{itemize}

\noindent\textbf{Result.}
We only include seeds that can complete the analysis within three hours. In three hours, \tool{} can complete the analysis of all seeds, but both GreyOne and ProFuzzer have some long seeds that cannot complete the analysis. The results are shown in the Table~\ref{Verification}.
% For the average analysis time, \tool{} spends the shortest time, which is 27.47 seconds on average. Greyone and ProFuzzer take about 26000 seconds and 21127 seconds, respectively. 
% Since \tool{} does not require a pilot stage, especially for long seeds, the analysis efficiency of \tool{} is much higher than that of Greyone and ProFuzzer.
We analyze the average number of useful mutations for each fuzzer at 1,000,000 mutations. \tool{} perform the best, and its average proportion of useful bytes is up to 70.5\%. Moreover, \tool{}'s average number of useful mutations is up to 3.715. The proportion of useful bytes and average number of useful mutations of GreyOne are only 16.1\% and 0.947, while that of ProFuzzer are only 17.8\% and 0.0887.
According to the above experimental results, \tool{} can find more useful bytes within shorter analysis time.


\begin{table}[h]
% \renewcommand\arraystretch{1.7}
% \newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
\centering
\caption{The comparison of position inference. \tool{} can infer more useful positions.}
\resizebox{\linewidth}{!}{
\begin{threeparttable}
\begin{tabular}{@{\extracolsep{4pt}}lccccccccccc@{}}
\toprule
\multirow{2}{*}{\textbf{Programs}} & \multicolumn{2}{c}{\textbf{GreyOne}} & \multicolumn{2}{c}{\textbf{ProFuzzer}} & \multicolumn{2}{c}{\textbf{\tool}}\\
\cline{2-3} \cline{4-5} \cline{6-7}


& UR\tnote{1} & AUM\tnote{2} & UR & AUM  & UR & AUM \\

% &\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Useful}\\ \textbf{Ratio}\end{tabular}} 
% &\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Average Useful}\\ \textbf{Mutation}\end{tabular}} 


% &\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Useful}\\ \textbf{Ratio}\end{tabular}} 
% &\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Average Useful}\\ \textbf{Mutation}\end{tabular}} 


% &\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Useful}\\ \textbf{Ratio}\end{tabular}} 
% &\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Average Useful}\\ \textbf{Mutation}\end{tabular}} \\
% &&&&&&\\
\midrule

\textbf{nm} & 3\%(135/4834) & 0.11 & 16\%(109/665) & 0.32 & \textbf{67\%(55/82)} & \textbf{1.87}  \\
\textbf{tiff2bw} & 13\%(101/762) & 0.74 & 14\%(106/762) & 0.75 & \textbf{89\%(74/83)} & \textbf{5.87}\\
\textbf{tiffsplit} & 68\%(104/152) & 3.18 & 69\%(104/150) & 3.25 & \textbf{92\%(72/78)} & \textbf{6.60}\\
\textbf{objdump} & 2\%(205/13288) & 0.45 & 18\%(318/1794) & 0.68 & \textbf{60\%(179/299)} & \textbf{1.70} \\
\textbf{readelf} & 3\%(99/3798) & 0.41 & 7\%(186/2641) & 0.48 & \textbf{83\%(95/114)} & \textbf{8.70}\\
\textbf{flvmeta} & 46\%(29/63) & 1.28 & 22\%(42/187) & 0.46 & \textbf{40\%(14/35)} & \textbf{1.08}\\
\textbf{pdftotext} & 3\%(267/8384) & 0.07 & 4\%(337/8805) & 0.08 & \textbf{54\%(165/305)} & \textbf{1.11}\\
\textbf{mp42aac} & 19\%(124/651) & 0.32 & 21\%(132/614) & 0.35 & \textbf{68\%(69/102)} & \textbf{1.70}\\
\textbf{tcpdump} & 2\%(88/4075) & 2.89 & 3\%(87/2708) & 2.48 & \textbf{77\%(72/93)} & \textbf{6.36}\\
\textbf{lame3.99.5} & 1\%(169/13077) & 0.02 & 1\%(179/13060) & 0.02 & \textbf{73\%(74/102)} & \textbf{2.16}\\

\bottomrule
\end{tabular}
\begin{tablenotes}[para]
\item[1]UR: Useful Ratio.
\item[2]AUM: Average Useful Mutation.
\end{tablenotes}
\end{threeparttable}
}
\label{Verification}
\end{table}


\subsection{Case Study}
In the previous experiments, we demonstrate the superiority of \tool{} in terms of edge coverage and bug discovery. In this section, we explore the insights of \tool{}.
As shown in the Figure \ref{tiff2pdf}, we select a code snippet from \texttt{tiff2pdf} to illustrate why the analysis time of \tool{} is shorter and why it can discover more new edges. In \texttt{tiff2pdf}, there are more than 10 \texttt{if} statements directly related to \texttt{t2p->tiff\_samplesperpixel}, and Figure \ref{tiff2pdf} shows only a part of them. 
Assume that a successful mutation flips one of the \texttt{if} statements, and then we analyze the high Shapley-value bytes, i.e., the bytes that contribute the most to the coverage. When we want to explore the remaining \texttt{if} statements related to \texttt{t2p->tiff\_samplesperpixel} in \texttt{tiff2pdf}, we can prioritize mutating the high Shapley-value bytes extracted earlier to quickly explore these \texttt{if} statements. 
However, it is difficult to infer which \texttt{if} statements share relevant bytes with each other directly. Therefore, we use the CMAB method to continuously analyze the relationships between constraints during attempts, which can help alleviate this problem. For more details, please refer to Section \ref{subsec:mutate}.
% \zhu{Why cannot others do the same thing?}
\zkp{However, for GreyOne, ProFuzzer, and Angora, the relationship between bytes and \texttt{if} statements in each path of the program needs to be re-analyzed, which consumes a lot of time.
For NEUZZ and PreFuzz, they cannot accurately analyze the relationship between input bytes and \texttt{if} statements. 
% and can only analyze from a high level which bytes are more important.
}

\begin{figure}[tp]
    \centering
\begin{lstlisting}

void t2p_read_tiff_data(T2P* t2p, TIFF* input){
    if(t2p->tiff_samplesperpixel>4){...}
    ...
    if(t2p->tiff_samplesperpixel==0){...}
    ...
    switch(t2p->tiff_photometric){
        ...
        case PHOTOMETRIC_RGB: 
            ...
            if(t2p->tiff_samplesperpixel == 3){...}
            ...
            if(t2p->tiff_samplesperpixel > 3){...}
            ...
    }
}
\end{lstlisting}
\caption{A partial code snippet extracted from  \texttt{tiff2pdf}. \texttt{t2p->tiff\_samplesperpixel} is used multiple times at different program locations.}\label{tiff2pdf}
\end{figure}



==> obsolete/intro-0.1.tex <==

\section{Introduction}

Traditional machine learning extracts features from training data to predict future outcomes. But the training data is not always enough, and its collection could be difficult and expensive. Transfer learning is an important tool in machine learning to solve the problem of insufficient training data. 
More specifically, If there are two domains and two learners need to learn for their tasks (domain A has enough training data and domain B does not), transfer learning can improve the learner from domain B based on the common features extracted from domain A. However, transfer learning assumes that the source domain and the target domain are related. Otherwise, the performance of transfer learning will decrease. Thus, there are three points in transfer learning: domain, task, and transfer feature.

Multi-task learning is one of the techniques in transfer learning, which requires the source and target domains to be the same and that the source and target tasks are different but related. Common multi-task learning architectures include Hard parameter sharing and Soft parameter sharing. The general structure of hard parameter sharing is shown in \ref{framework_transfer}. In hard parameter sharing, neural network models of different tasks jointly use the shared Layers to extract some common features, and then set task-specific layers for each different task to learn the task-specific features based on common features. 

\begin{figure}[htbp]
\includegraphics[width=\linewidth]{images/transfer_learning_framework.jpg}
\caption{The framework of transfer learning.}
\label{framework_transfer}
\end{figure}

So why do we treat fuzzing campaigns as transfer learning?
As shown in \ref{workflow_fuzzing}, a fuzzer selects a seed and performs exploration on it in the fuzzing campaign. Then, we treat it as a learning process whose target is to explore all unexplored neighbor branches, i.e., to satisfy the constraints of unexplored neighbor branches.
In other words, satisfying the constraints of unexplored neighbor branches is equal to reversing the states of the corresponding cmps. All learning processes maintain a global virgin\_bits that records which edges have been explored. 
However, existing solutions ignore the relationships between different learning processes and treat these processes as independent processes. 
In real-world programs, as there are many relationships between different cmps, such as sharing the same related bytes among multiple cmps, different learning processes are not independent of each other. When we are in the process of exploring a seed, it will be more efficient if we can use the transfer features extracted from other processes. 
We also preform an experiment to prove it.  We find that different edge discoveries may share part of the same related bytes. The details are shown in fig X. We believe these same related bytes could be the relationship between different edge discoveries.

\begin{figure}[htbp]
\includegraphics[width=\linewidth]{images/fuzzing_campaigns.jpg}
\caption{The workflow of fuzzing. \zhu{The insight is that all execution paths of a program together perform the complete functionalities of the program. Therefore, different execution paths are somehow correlated to each other, which offers the possibility to model the fuzzing process as transfer learning.}}
\label{workflow_fuzzing}
\end{figure}


But how do combine fuzzing and transfer learning?
In order to bring fuzzing campaigns into the definition of transfer learning, we have to determine the domain, task, and transferring feature. 
As the cmps in the program determine the execution state directly, we set the task as a learning process, i.e., the exploration for a seed, and set the domain as the program input space.
In fuzzing campaign, we have a lot of seeds to be explored and there is only one program input space. Thus, we have multiple tasks and all tasks share the same program input space. In other words, the source and target domains are the same, but the source and target tasks are different.
According to the classification in \cite{weiss2016survey}, the fuzzing campaign is more like multi-task learning in transfer learning.

To model fuzzing campaigns as multi-task learning, we still need to verify that different tasks are related. The most important factor in a learning process is how to reverse the state of the cmps with unexplored branches. Fortunately, we find it is common that different cmps share the same related bytes under the same input (as shown in fig1), which means that the cmps in different learning processes may share part of the same related bytes. More details are introduced in Section III-A. Thus, a learning process is likely to be related to other processes. 
However, We still can not determine which processes are related based on this phenomenon.

Thus, we propose an adaptive strategy to quality the relationship between two tasks during the fuzzing campaigns.
More specifically, we assign $p$ to represent how related two tasks are. 1 represents two tasks that are very related and 0 represents two tasks that are not related. Assume that there are two seeds, A and B. 
In the beginning, we assume that two tasks are related and set $p$ as 1. Thus, When we explore seed A, we can use the common features extracted from seed B to generate the task-specific features to guide the exploration. During the mutation stage, we collect the feedback information to update $p$. More specifically, the value of $p$ will decrease with the increase of the number of mutations on the corresponding seed. If we can find new paths based on common features, we will increase the value of $p$. Otherwise, we will decrease the value of $p$, which indicates reducing the correlation between these two tasks.

But how can we extract the common features from the learning process?
In machine learning, the common features will be extracted automatically with the shared layers. As efficiency is important to fuzzing, we can not use neural networks to extract common features because of the high overhead of the training model. Thus, we have to find a feature that can be collected in a lightweight method. As the experiment in fig1 shows that different cmps share part of the same features, the most intuitive idea is to set the common feature as the cmp-related bytes. If a byte is related to one cmp, it is also likely related to other cmps. 
Thus, we collect the unexplored cmp-related bytes during a learning process(i.e., the exploration of a seed), then mutate these bytes again in another learning process. But the collection of this feature is time-consuming as we need to analyze each cmp in each seed. For example, Given the seed length is $10000$, the execution speed as $1000/s$, and the seed num is $1000$, even if we use the state-of-art inference method used by Greyone, we need $10000*1000/1000 = 10000$ seconds to finish the analysis. 

We can extract similar features in a more lightweight method. If the bytes in the seed are mutated and we find a new path, we can conclude that these bytes are related to certain cmps in the initial path exercised by the initial seed. Thus, we set the positions that used to be mutated and found new paths successfully as the common features. And the collection of this feature is easy and lightweight. 

Although it is easy to collect common features, there are some problems existing with its use. The max problem is that the meaning of a position in different program inputs is not always the same. If we record the useful mutated positions in seed A, we can not directly use them in the fuzzing of seed B as we are not sure that the same positions have the same meaning in seeds A and B. And there are many factors that may change positions' meanings. We summarize the following main factors.

First, as a fuzzing campaign may have multiple initial seeds, the same position in different seeds will have different meanings (challenge I). 
Before fuzzing, we need to prepare some initial inputs. And the initial inputs are usually manually created according to the input specifications of programs under test or collected from the Internet. It is difficult that all initial inputs have the same length and the same position in each input have the same meaning. Thus, we need to overcome the difficulties caused by different initial seeds.


Second, the meaning of the same position may change because of the insert/delete mutators(challenge II).
Generally speaking, AFL-based fuzzers have three mutation stages: deterministic stage, havoc stage, and splicing stage. In the havoc stage, a fuzzer will select different mutators based on its chosen strategy. And the mutators can be divided into two parts, overwrite mutators and length mutators. The latter consists of two parts, insertion and deletion. If length mutators are used, the input length and the meanings of some positions will be changed. For example, if a seed has N bytes and we delete the Mth byte, the meanings of the Mth to (N-1)th bytes will be changed because the relative position of each byte changes.

Third, the meaning of the same position may change because of the trimming operation(challenge III).
Throughput is one of the most important features in AFL-based fuzzers, the fuzzers improved from AFL. Considering the limited time budget of fuzzing campaigns, we can test more mutated inputs based on the high throughput, which improves the efficiency of fuzzing. 
As large files make the target binary run slower, the file size has a dramatic impact on the performance of fuzzing. 
Trimming is an easy way to automatically trim down input files and ensure that these changes make the files have no effect on the execution path. However, trimming is just like delete mutators which change the input length. And the meaning of the same position will be changed too.

Forth, as not every mutation is necessary, we need to extract a minimal mutation set(challenge IV). 
If not, we will introduce a lot of redundant mutations, so that almost all bytes are related to the discovery of new paths after hours of fuzzing. Thus, we can not locate the real useful mutated positions efficiently. We perform an experiment on AFL-test under a single initial seed to prove it. We record the mutated positions of new path discovery without using any length mutators and trimming to avoid changing the position meaning. As shown in \ref{influence_withdraw}, we find that almost all bytes are related to the discovery of new paths after X hours. 

\begin{figure}[htbp]
\includegraphics[width=\linewidth]{images/The_influence_of_withdraw_operation.png}
\caption{The influence of withdraw operation.}
\label{influence_withdraw}
\end{figure}

To solve the aforementioned challenges and use the transfer feature successfully, we propose novel strategies to speed up the fuzzing campaign. 
More specifically, TransferFuzz divides the fuzzing campaigns into multi-fuzzing campaigns based on the inheritance relationship (challenge I).
An initial seed and the inputs generated from it without using length mutators belong to a race, i.e., a child fuzzing campaign. Each race needs to maintain a local virgin\_bits to avoid the influence of meaning changed for the same position caused by multiple initial seeds. Further, expect updating the global virgin\_bits, all strategies are performed within a single race.

In each race, it needs to do the following work. 
First, to avoid the influence of meaning changed for the same position caused by trimming, we construct a map\_vector for each seed to record the relative position with reference to the initial seed of the corresponding race(challenge III). Second, we temporarily record the mutated positions and the mutators used.  To avoid the influence of meaning changed for the same position caused by length mutators and remove useless mutators, we need to withdraw all mutators used and verify whether the same path is found when a new path is found. (challenge II) 

For the collection of common features, we collect the useful mutated positions into the common features pool after removing the redundant (challenge IV). 

For the generation of task-specific features, we assign a weight for each common feature to describe the relationship between the common feature and the target task, then we will randomly combine different common features based on the weights. We call the mutation strategy as history mode.

After obtaining the transfer features, we also construct a history mode to mutate seeds in the havoc stage based on this information. More specifically, we prioritize the positions recorded in the transfer feature vector. Besides history mode, we also have a new mode to focus on the new edges found by the current seed and try to explore these new edges. We analyze the related bytes of new edges found by each seed based on dichotomy-FTI. Then, we focus on mutating these bytes in the new mode. 
We rename the normal mutation strategy as random mode. In order to find the best mode that should be used in the current mutation, we propose a novel mode scheduler. Specifically, we choose to use the mode that has the lowest per\_path\_cost which represents the number of mutations needed to discover a new path in a mode. The per\_path\_cost is smaller, and the efficiency of the corresponding mode is higher. 

In this paper, we implement the prototype of XXX based on AFLPlusPlus. (Experiment Result) 
We compare the fuzzing performance of XXX with multiple modes of AFLPlusPlus and conduct fuzz
testing on XX target programs. The experimental results show that
XXX discover more XX% code coverage and bugs than almost all existing modes in AFLPlusPlus. We summarize our contributions as follows.

==> obsolete/intro-0.2.tex <==



\section{Introduction}

% \zhu{ our keys?:
% \begin{itemize}
%     \item the combination of different path constraints result in different execution paths
%     \item an input position may be used as a path constraint in different program logics
% \end{itemize}}

\todo{Our \tool{} aims to use the relations between path constraints. While determining the relation between path constraints is quite challenging, the relation offers fuzzing a different perspective to improve efficiency.:\begin{itemize}
    \item dataflow analysis? taint analysis?
    \item the path constraints are the main (maybe the only?) road rocks for coverage discovery
    \item grammars somehow reflect the control flows of programs
    \item existing solutions neglect the fact that different path constraints have complex relations. They build relations between some input bytes and one path constraint at one time. they focus on a single path constraint.
    \item observations: complex relations between path constraints: \begin{itemize}
        \item direct relation: the combination of different path constraints result in different execution paths
        \item indirect relation: an input position may be used by different path constraints in different program logics
    \end{itemize}
    \item Questions: \begin{itemize}
        \item Why do we use family? the relation between family and the observations : in path A, position $a$ is related to constraint; then in path B, we hope the position $a$ is still related to constraint.
    \end{itemize}
    \item reduce search space: the key is to prioritize some bytes to reduce search space in input. existing solutions focus on prioritizing bytes related to a single path constraint.
\end{itemize}}


The path constraints are the main road rocks for coverage discovery. If we can solve more path constraints, more new edges can be found. To solve the path constraints, there are mainly two methods: symbolic execution and inference. Symbolic execution uses a constraint solver to generate inputs to solve constraints along execution paths. Inference-based fuzzers apply perturbation to each position in the seed and observe the change in the value of the program variable to obtain the related position of each path constraint.

However, existing solutions neglect the fact that different path constraints have complex relations. They build relations between some input bytes and one path constraint at one time. The relations between different path constraints can be grouped in real programs into the following two categories.

\begin{itemize}
  \item [1)] 
  Direct relation: the combination of different path constraints result in different execution paths.   
  \item [2)]
  Indirect relation: an input position may be used by different path constraints in different program logics.
\end{itemize}

Both methods mentioned above are inefficient in these cases. They focus more on how to identify more accurate valuable positions for a single path constraint while ignoring the use of the relations between different path constraints to improve the efficiency of fuzzing.

The key to solving both cases lies in fully using the path constraints' related positions (i.e., valuable positions).

\begin{itemize}
  \item [1)] 
  For direct relation, if we can jointly mutate the valuable positions corresponding to multiple path constraints, then we can try more combinations of different path constraints to discover new edges that are difficult to be explored by symbolic execution and inference.
  \item [2)]
  For indirect relation, if we can establish positions mapping between seeds that execute different program logics, then we can achieve the information exchange of valuable positions between seeds. When mutating a new seed, even if we do not analyze this seed, we can directly obtain potential valuable positions from other seeds, thereby improving the fuzzing efficiency.
\end{itemize}

In order to utilize valuable positions more efficiently, there are three key challenges as follows.

\textbf{The $challenge I$ is how to identify valuable positions without introducing additional overhead.} Although the inference-based method is easy to implement, it faces a time-consuming analysis process. In ProFuzzer, it needs to mutate each byte in the input 255 times, which takes much time. Especially in the case of long input, the required analysis time is unacceptable. 
For example, assume the input size is 10kB and the target program execute 1000 times per second.
Thus, the required analysis time is 10240 * 255/1000 = 2611 seconds. In Greyone, although it is not necessary to mutate each byte 255 times, Greyone needs to perform additional instrumentation for target programs to extract the specific value of the target cmps at runtime. 
However, the execution speed of the instrumented program is seriously slowed down.

\textbf{The $challenge II$ is how to achieve the exchange of valuable positions information between seeds.} The biggest problem of information exchange between seeds is the alignment problem. This is mainly caused by the following three reasons: 1) the length of the initial seed and the meaning of each position are inconsistent; 2) the effect of trimming on the length of the seed; 3) the effect of length mutators such as insert and delete. In order to be able to exchange information between seeds, a matching mechanism is needed to find positions with the same meaning on different seeds.


\textbf{The $challenge III$ is how to choose suitable valuable positions for mutation?} The importance of a position is not constant, and it changes over time. We need to design an algorithm that can dynamically update the position distribution based on the mutation results.

To address these challenges, we propose \tool{}, a lightweight family-based inference analysis method, to address the above three challenges.
To solve the problem in challenge I, 

To solve the problem in challenge I, \tool{} extract enough useful mutation information from havoc stage to integrate the pilot stage into the havoc stage.

To solve the problem in challenge II, 
\tool{} proposes a novel Family System to cluster all seeds based on the inheritance relationship, which coarsely maintains semantic consistency within a family.
Then, \tool{} maintains a shared pool in each family to record the valuable positions in each seed. 
All seeds in the same family can assess the shared pool. Thus, through some seeds only assigned less energy to mutate, they can also find their own valuable positions according to the shared pool based on the semantic consistency within a family.

To solve the problem in challenge III, \tool{} uses the LinUCB model to generate a possibility distribution for a seed.






\zhu{add citations where necessary}

In target programs used in fuzzing, their input usually consists of two parts: structure field and data field \zhu{structure-changing field and structure-preserving field? \cite{Nguyen2022BeDivFuzz}}. Among them, the structure field refers to the bytes related to the path change, and the data field refers to the information carried in the input (such as the specific content in the picture), which has nothing to do with the execution path of the program.
In coverage-guided fuzzing, for higher coverage, existing fuzzers try to mutate bytes in structure fields to avoid wasting time on data fields. To achieve this purpose, there are mainly the following two methods.
%在常见的fuzzing所用的目标程序中，他们的input通常由结构字段和数据字段两部分构成。其中，结构字段是指那些与路径变化相关的bytes，而数据字段是指input中所承载的信息（例如图片中的具体内容），它们和程序的执行路径无关。
%在coverage-guided fuzzing中，为了更高的coverage，现有的fuzzers都尽量去突变结构字段中的bytes，以免在数据字段之上浪费时间。为了实现这一目的，现有主要有以下两种方法。

\textbf{Traditional grammatical rule-based methods.} The input is parsed based on the specific grammar rules of the target program, and the input is divided into structure fields and data fields. However, this solution needs to prepare the specific grammar rules of the target program in advance, which requires a lot of human resources and time.
%1、传统的解决方案：基于目标程序的具体语法规则对Input进行解析，将Input切分为结构字段以及数据字段；例如，XX和XX利用解析器对Inputs进行解析，从而......。但是，该方案需要提前准备好目标程序的具体语法规则，这需要耗费大量的人力与时间。并且，如ProFuzzer中所述，由于在不同的应用场景下，相同的bytes可以分别为数据字段和控制字段，所以.....

\textbf{Inference-based methods.} In order to solve the dependence of traditional solutions on grammar knowledge, inference-based methods emerge as the times require. Specifically, inference-based methods will set up a pilot stage before havoc stage to perform mutation testing on each byte in the input to observe whether the execution state change. If the  execution state change, the byte is located in the structure field; otherwise, the byte is located in the data field. This type of method (e.g., ProFuzzer, Greyone) often only requires additional instrumentation of some program execution information, and the implementation is straightforward. For ProFuzzer, it needs to try all the values of each byte one by one and construct a feature vector based on the corresponding path length to analyze the specific type of each byte. For Greyone, it only pays attention to which bytes are located in the structure field. It needs to mutate each byte several times and check whether the value of cmp changes. If it changes, the mutated byte is located in the structure field. However, inference-based methods also face the following two problems.
%inference-based的解决方案：为了解决传统方案对语法知识的依赖，inference-based的方法应运而生。具体来说，此类方法会设置一个pilot stage，在正式的fuzzing之前提前对input中的每个byte进行突变测试，观察路径/cmp值是否发生变化。如果执行路径/cmp值发生变化，说明该byte位于结构字段之中；否则，该byte位于数据字段之中。这类方法（eg：ProFuzzer、Greyone）往往只需要额外插桩部分程序运行信息，实现上非常简单。对于ProFuzzer来说，它需要逐个尝试每个byte的所有值并基于对应路径长度来构造特征向量，从而分析每个byte的具体类型。对于Greyone而言，它只关注哪些bytes位于结构字段，它需要对每个byte突变数次并查看cmp的值是否发生变化，如果变化则说明该byte位于结构字段之中。然而，inference-based的方法也就面临着以下两个问题。

\textbf{First, although the inference-based method is easy to implement, it faces a time-consuming analysis process.} In ProFuzzer, it needs to mutate each byte in the input 255 times, which takes much time. Especially in the case of long input, the required analysis time is unacceptable. 
For example, assume the input size is 10kB and the target program execute 1000 times per second.
Thus, the required analysis time is 10240 * 255/1000 = 2611 seconds. In Greyone, although it is not necessary to mutate each byte 255 times, Greyone needs to perform additional instrumentation for target programs to extract the specific value of the target cmps at runtime. 
However, the execution speed of the instrumented program is seriously slowed down.
%We have tested it on AFL++, and the program execution speed after instrumentation is seriously slowed down (given specific data).
%• 一、Inference-based的方法虽然实现简单，但是面临着分析过程耗时的问题。在ProFuzzer中，它需要对input中的每个byte突变255次，这个过程需要耗费大量的时间。特别是在长input的情况，所需要的分析时长难以让人接受。例如，假设有一个input大小为10kB，目标测试程序每秒可执行1000次，则需要的分析时间为10240 * 255/1000 = 2611秒。而在Greyone中，虽然不需要对每个byte都突变255次，但是Greyone需要对每个目标程序进行额外的插桩，来提取出目标cmps在运行时的具体值。我们在AFLPlusPlus上经过测试，插桩后的程序程序执行速度严重减慢（给出具体数据）。

\textbf{Second, although inference-based methods also perform mutation in the pilot stage, its efficiency is relatively low.} In essence, the mutation method in the pilot stage is consistent with the deterministic stage in AFL, which is to mutate each byte in the input one by one. However, MOPT has pointed out that the deterministic mutation strategy is inefficient, and long-term exposure to this strategy will affect the overall efficiency of fuzzing. Therefore, there is an urgent need for a new method of identifying structure fields that do not depend on grammar knowledge and do not require much analysis time.
%inference-based在plot stage时虽然也在进行突变，但是其效率是较为低下的。实质上，inference-based的方法中的plot stage的突变方式和AFL中的deterministic stage是一致的，都是对input中的各个byte逐个进行突变。但是，MOPT已经指出deterministic的突变策略效率很低，长期处于该策略会影响fuzzing的整体效率。所以，现在急需一个既不依赖于语法知识，也不需要耗费大量分析时间的新的识别结构字段的方法。

\textbf{Third, the inference-based method does not mutate multiple positions simultaneously during the pilot stage?, mainly to avoid the following two reasons.} 1) If multiple positions are mutated at once, they may contain redundant positions. We cannot determine which position's mutation caused the change of execution state, which will cause an over-taint problem.
2) If multiple positions are mutated at one time, the number of mutation combinations that need to be tried in the pilot stage will exponentially increase, causing the problem of extended analysis time. However, only considering the case of mutating a single position will cause an under-taint problem. Some execution states need to mutate multiple positions simultaneously before they can be discovered. \zhu{Will this really be a problem? Although they do not mutate multiple positions at inference stage, they mutate multiple positions during the main fuzzing stage.}\zkp{But they do not infer the structure-related positions during the main fuzzing stage. And this problem has been mentioned in the paper of GREYONE.} \zhu{==> waste energy in havoc stage}
%第三，inference-based method do not mutate multiple positions at the same time，这么做主要是为了避免以下两个问题。1）一次性突变多个positions可能会包含冗余的positions，无法确定new coverage来自于哪个position的突变，这样就会造成over-taint的情况；2）如果一次性突变多个positions，那么在pilot stage所需要尝试的突变组合数就会快速增长，造成分析时间过长的问题。但是，仅仅考虑突变单个position的情况会造成under-taint的问题，有些new coverage需要同时突变多个positions才可以被发现。

We call the data pair of mutated positions and mutation result obtained by performing a mutation on a seed as \textbf{mutation information}, namely (mutated position, execution state changed or not).
The essence of the pilot stage is to mutate each byte in the seed to obtain a dataset that contains much mutation information.
Then, the structure-related positions can be extracted from the dataset.
In the dataset, the $feature\ vector$ is a mutated position, and the $label$ is whether execution state changed.
In particular, there is only one position within the $feature\ vector$. Therefore, the structure-related positions can be found directly according to the dataset. In other words, if the $label$ is 1, the position recorded in the $feature\ vector$ is structure-related. Since the mutation of the pilot stage will cover every position in the seed, all positions will be analyzed.
%• Pliot stage的实质就是通过对种子中的每一个byte进行突变得到一个“input为mutated positions序列，label为路径/cmp值是否改变”的数据集，然后再从该数据集中提取结构字段的位置信息。特别的，该数据集input的内仅有一个位置。所以，可以直接根据该数据集找到该种子结构字段的所处位置。具体的，如果label为1时，input中的position即为结构字段的位置。由于Plot stage的突变会覆盖到种子上的每一个position，所以该数据集中会有所有positions的数据，进而对所有的positions进行分析。（画图说明）


As the fuzzing process can complete hundreds or thousands of mutations in one second, if we can extract enough useful mutation information to replace the dataset generated by the pilot stage, we can \textbf{integrate the pilot stage into the havoc stage}. Thus, there is no need to set the pilot stage for analysis, which improves the fuzzing efficiency. 

However, there are many difficulties in integrating the pilot stage into havoc stage. We need to overcome the following challenges.

First, we collect mutation information to replace the dataset generated by the pilot stage. However, collecting all mutation information in havoc stage is impractical, which takes much time. Due to the randomness of fuzzing, most of the mutation information does not contain any information. That is, they will not cause execution state changes. Therefore, a lightweight strategy must be deployed to extract more useful mutation information from massive data (\textbf{Challenge I}). 

After we have a new dataset generated from havoc stage, we extract the structure-related positions for each seed from it. However, the dataset generated from the pilot stage and the dataset generated from havoc stage are inconsistent in $feature\ vector$. Since only one position is mutated at a time in the pilot stage, the $feature\ vector$ length of the former is 1. As multiple positions could be mutated simultaneously in havoc stage, the $feature\ vector$ length of the latter is likely to be greater than 1. Therefore, we need an inference-based analysis method suitable for mutating multiple positions simultaneously (\textbf{Challenge II}).

If we want to analyze all seeds with the above method, then each seed needs to be allocated enough energy to mutate in havoc stage. However, not all seeds will be allocated much energy to mutate. How do seeds that are allocated less energy extract enough information to analyze their structural fields (\textbf{Challenge III})? Therefore, a reasonable strategy is required to extract the structure-related positions for the seeds with low energy.
% In this paper, we propose a lightweight sharing mechanism-based structural field analysis method. We have the following steps to integrate the pilot stage into havoc stage stage. 

% First, it collects useful mutation information to replace the dataset generated by the pilot stage. -> What is useful mutation information? 
% Can we extract the structure-related positions for each seed from this new dataset?
% Why can the dataset generated by the pilot stage be replaced?

% Second, it identifies the structure-related positions for each seed. -> how to extract the structure-related positions when a seed mutates multiple positions at once. 





% However, we need to address the following three main challenges.
%• 由于Fuzzing过程中一秒钟都可以完成成百上千次的突变，如果我们可以从中提取出部分有用的突变信息来替代plot stage生成的数据集，我们就可以将plot stage融入到实际的fuzzing过程中，从而不需要额外设置plot stage进行分析。但是，我们需要解决以下三个主要挑战。

% \textbf{Challenge I}: What is useful mutation information? Why can the dataset generated by the pilot stage be replaced? Due to the randomness of fuzzing, most of the mutation information do not contain any information. That is, they will not cause changes in paths or changes in cmps' values. Therefore, we need to extract useful mutation information from massive data to replace the data set generated by the pilot stage.
%Challenge I：什么是有用的突变信息？为什么可以对plot stage生成的数据集进行替换？由于fuzzing的随机性，绝大部分的突变结果都不包含任何信息量，即不会造成路径的变化或者cmp值的改变。所以，我们需要从海量的数据中抽取出有用的突变信息出来，从而去替代plot stage所生成的数据集。

% \textbf{Challenge II}: To replace the dataset, a large amount of mutation information is required for selection.
% However, not all seeds will be allocated a large amount of energy to mutate.
% How do seeds that are allocated less energy extract enough information to analyze their structural fields?
%Challenge II：如果根据“一”中的方法替换pilot stage，则需要有大量的突变数据来进行选择。但是，并不是所有的种子都会被分配大量的能量进行突变。对于那些分配能量较少的种子，如何提取足够的信息来分析自己的结构字段？

% \textbf{Challenge III}: Can the recognition accuracy of the inference-based method be achieved after the replacement? Can we get better results on coverage?
%Challenge III：替代之后能否达到inference-based方法的识别精度？能否在coverage上取得更好的效果？

\zhu{You should explicitly mention the reasons of your solutions. Greyone infers structure-related bytes BEFORE it finds new coverage. So the structure-related bytes are useful when discovering new bytes. But your recorded bytes have already discovered new coverage, how come that they are useful when discovering new coverage in the future? You need to answer this question very carefully.}
\zkp{As we introduce a new indicator $local\ new\ edges$, I think we do not need to answer this question any more. $Local\ new\ edges$ is not equal to traditional new edges.} \zhu{you still need to answer this because the essential objective is to discover global new edges. You have to link the local new edges to the global new edges.} \zkp{For the same path constraint, the related positions on different seeds may not be consistent. We have constructed position mapping for seeds within the same family, but we have no way to construct position mapping between families. If we only collect data based on global new edges, then we will miss some valuable positions for some partial seeds. For example, given initial seeds $A$ and $B$, they have no semantic consistency. If the path constraint $X$ is resolved when $position 1$ of $A$ is mutated, then $position 1$ will be added to the shared pool of the family where $A$ is located. However, since there is no semantic consistency between $A$ and $B$, we have no way to find the related positions of path constraint $X$ in seed $B$ according to the position mapping relationship. At the same time, since path constraint $X$ has already been solved, the next time the seed $B$ is mutated and path constraint $X$ is solved, we will not extract valuable positions from it. Thus, we have no way to find the related positions of path constraint $X$ in seed B. Finally, if we can't find the related positions of all path constraints on all seeds, it will naturally affect the improvement of fuzzing efficiency.}

We propose \tool{}, a lightweight family-based inference analysis method, to address the above three challenges.
To solve the problem in challenge I, we propose a novel indicator $local\ new\ edges$ to extract more useful mutation information without introducing time-consuming problem or data explosion problem.
Specifically, given a seed $t$, local new edges are the edges that have not been covered by the seed $t$ and the mutated inputs from the past.
Thus, \tool{} construct inference dataset based on the mutation that finds local new edges. In addition, we use 48h fuzzing data for SHAP analysis in the section X to get the ground truth of important positions for each seed. Then, we verify that the structure-related bytes we identify can cover most of the important positions within 1h.
% First, \tool{} extracts the mutation information and finds new edges to replace the dataset generated by the pilot stage.
To solve the problem in challenge II,  \tool{} removes all irrelevant mutated positions in the dataset to achieve accurate inference analysis when having multiple mutated positions simultaneously.
To solve the problem in challenge III, 
\tool{} proposes a novel Family System to cluster all seeds based on the inheritance relationship, which coarsely maintains semantic consistency within a family.
Then, \tool{} maintains a shared pool in each family to record the structure-related positions in each seed. 
All seeds in the same family can assess the shared pool. Thus, through some seeds only assigned less energy to mutate, they can also find their own structure-related positions according to the shared pool based on the semantic consistency within a family.
% Finally, We construct a SHAP analysis to identify the important positions in the seed and verify that Pozzer can cover most of the important positions in a short time.

In this paper, we implement the prototype of \tool{} based on AFL++. (Experiment Result) 
In order to avoid subjective factors, we evaluated \tool{} on two third-party platforms, UNIFUZZ and MAGMA.
In UNIFUZZ, we evaluate \tool{}-related fuzzers (i.e. \tool{} and \tool{}-Redqueen) and multiple existing modes of AFL++ on XX target program. \tool{} discovers more XX\% and X\% on code coverage and bugs than the best mode existing in AFL++, respectively.
In MAGMA, we evaluate these two \tool{}-related fuzzers and 5 widely-used mutation-based fuzzers(AFL, AFLFast, FairFuzz, MOPT and AFL++) on X programs. \tool{}-Redqueen exposes more X CVEs that the best compared fuzzer.


We summarize our contributions as follows.
\begin{itemize}
    \item We propose a family system to achieve the integration of the pilot stage and havoc stage. Based on semantic consistency, the seeds are divided into multiple families, which allows different seeds in the same family to share the structure-related positions identified by themselves to improve the efficiency of fuzzing.
    \item We propose a Family-Based Mutation Mode, which uses the LinUCB model to identify valuable positions within the family's shared pool for each seed to guide the mutation direction.
    \item We implement a prototype \tool{} based on AFL++, evaluate it based on UNIFUZZ and MAGMA platforms. The results indicate that \tool{} outperforms various state-of-the-art fuzzers on edge coverage and bug discovery.
\end{itemize}

==> obsolete/intro-0.3.tex <==



\section{Introduction}

% \zhu{ our keys?:
% \begin{itemize}
%     \item the combination of different path constraints result in different execution paths
%     \item an input position may be used as a path constraint in different program logics
% \end{itemize}}
% \zhu{KEY: existing solution infer a fixed group for mutation; our solution evolves the groups during fuzzing?}


For analyzing security issues in software, both academic and industrial practitioners regard fuzzing as the de facto detection technique~\cite{zhu2022roadmap}.
Among all the fuzzing solutions, coverage-guided greybox fuzzing (CGF) has achieved a great success in detecting real-world bugs~\cite{ossfuzz, onefuzz, feng2021snipuzz}. 
It aims to discover new code coverage so that bugs may be disclosed in those unseen code. Existing research has spent many efforts in expanding code coverage, including scheduling computing resources for certain code regions~\cite{aflfast, fairfuzz, Yue2020EcoFuzz} and resolving path constraints~\cite{angora, driller, SymFuzz, qsym, dowser, matryoshka}.
While scheduling computing resources is an implicit way to expand code coverage, resolving path constraints is an explicit way to achieve it. Since path constraints guard a certain code region, any success in passing path constraints most likely results in new code coverage. However, resolving path constraints is not a free lunch as those constraints may be quite complicated. 


% Existing solutions for resolving path constraints can be categorized into symbolic execution based solutions and inference based solutions \zhu{citations}. Symbolic execution builds formula for constraints along an execution path and uses constraint solver to generate inputs that satisfy those constraints \zhu{citations}.
Because fuzzing repeatedly tests a program, a promising solution for resolving path constraints is to infer the relationships among input bytes and mutate related bytes together in later fuzzing campaigns~\cite{greyone, ems, profuzzer, neuzz}.
For instance, some fuzzers build the relationship among input bytes if they influence the same path constraint~\cite{greyone, ems, angora, vuzzer, steelix} or construct the same data type~\cite{profuzzer, angora}.
The inference can reduce the search space of passing constraints if fuzzing combines the related bytes into groups and mutates inputs based on groups. 
For instance, mutating 12 bytes can generate $256^{12}$ different inputs while mutating 4 bytes at a time (4 bytes a group) only generates $3\times256^{4}$ different inputs. 
If a path constraint can be resolved by mutating one group, the combination of bytes can significantly improve the efficiency of code discovery. 
% Existing research builds the relationship among input bytes if they influence the same path constraint \zhu{cite; greyone, ems} or construct the same data type \zhu{cite; profuzzer}. \zhu{more fuzzers?} 


Essentially, the groups of bytes reflect the formats of inputs, which further represent the internal logic of programs. However, the existing inference solutions only reveal the shallow logic of programs. Those solutions only infer the relationships of bytes for a single path constraint at a time. Each time, the bytes related to a single path constraint are mutated, which neglects the fact that different path constraints may be heavily coupled. For example, to pass the condition $if(b == 0x123)$, we may need to figure out all the conditions that the variable $b$ depends on, such as $if(a == 0x22)\{b = 0x12\}$. In this case, it is insufficient to only mutate the bytes related to the variable $b$ for passing the path constraint. Therefore, in order to fuzz deep program logic, the inference for related bytes is required to consider the coupling of path constraints.



In this paper, we propose \tool{}, a lightweight fuzzer, to mutate inputs considering the coupling of path constraints. We infer and group the bytes related to the coupled path constraints based on two observations. A straightforward observation is what we call \textit{direct coupling}, where the flip of a path constraint must consider the results of other path constraints.
% different path constraints in the same execution path influence or use the same data. 
The exploration of directly coupled path constraints will lead to deep code in programs (exemplified in Section~\ref{sec:motivation}). Another observation is that different program logics may process the same format of inputs, indicating that different constraints are related to the same positions of inputs (we call it \textit{indirect coupling}). 
The usage of indirect coupling helps fuzzing quickly explore new code if a fuzzer only mutates the corresponding input positions (exemplified in Section~\ref{sec:motivation}).


Based on the two observations, our \tool{} builds a \textit{family system}.
The key of the family system is to maintain the semantic information in inputs, where we regard the positions of inputs are more important than the values.


% Because input generation is the key stage in fuzzing, we identify two types of coupling to help input generation.  


% To overcome the coupling of path constraints, an intuitive solution is to analyze dataflow based on taint analysis. However, taint analysis is not only slow but also suffering from inaccuracy due to over taint and under taint \zhu{cite;}. 


% \todo{how to transit?}
% % In this paper, we intent to improve the performance of fuzzing by grouping bytes based on the coupling among path constraints.
% % Although determining the coupling among path constraints is quite challenging \zhu{cite; dataflow, taint analysis}, the coupling offers us a different perspective to boost fuzzing.
% % Although determining the coupling among path constraints is quite challenging \zhu{cite; dataflow, taint analysis}, fuzzing can group input bytes based on the coupling.\todo{or use the next sentence}
% It is quite challenging to accurately analyze whether different path constraints are coupled due to the difficulty for analyzing control flow and data flow in programs~\zhu{cite; dataflow, taint analysis;}. 
% % Yet, due to the nature of repeat testing, fuzzing can still group bytes based on coupling despite the inaccurate coupling relation.
% Yet, the inaccurate information of coupling can still be utilized to infer the relationships between input bytes.
% % From the perspective of grouping input bytes, we observe two types of coupling, which are
% In order to group bytes based on coupling, the coupling of path constraints can be categorized into \textit{direct coupling} and \textit{indirect coupling}. The direct coupling indicates the same data used by variables in different path constraints. On the other hand, the indirect coupling indicates the same input format shared among different execution paths, \ie different program logics. 
% % different program logics, \ie the coupling is built by the input format. For the direct coupling, 



\todo{Our \tool{} aims to use the relations between path constraints. While determining the relation between path constraints is quite challenging, the relation offers fuzzing a different perspective to improve efficiency.:\begin{itemize}
    % \item dataflow analysis? taint analysis?
    % \item the path constraints are the main (maybe the only?) road rocks for coverage discovery
    % \item grammars somehow reflect the control flows of programs
    % \item existing solutions neglect the fact that different path constraints have complex relations. They build relations between some input bytes and one path constraint at one time. they focus on a single path constraint.
    \item some challenges to overcome the coupling of path constraints
    \item we propose \tool{} to solve the challenges based on two observations
    \item observations: complex relations between path constraints: \begin{itemize}
        \item direct relation: the combination of different path constraints result in different execution paths
        \item indirect relation: an input position may be used by different path constraints in different program logics
    \end{itemize}
    \item others: \begin{itemize}
        \item Why do we use family? the relation between family and the observations : in path A, position $a$ is related to constraint; then in path B, we hope the position $a$ is still related to constraint.
         \item reduce search space: the key is to prioritize some bytes to reduce search space in input. existing solutions focus on prioritizing bytes related to a single path constraint.
        \item KEY: existing solution infer a fixed group for mutation; our solution evolves the groups during fuzzing.
        \item fuzzing can repeatedly try to figure out the combination of bytes for coupling constraints. therefore, it can still infer the byte relation based on coupling.
    \end{itemize}
\end{itemize}}


The path constraints are the main road rocks for coverage discovery. If we can solve more path constraints, more new edges can be found. To solve the path constraints, there are mainly two methods: symbolic execution and inference. Symbolic execution uses a constraint solver to generate inputs to solve constraints along execution paths. Inference-based fuzzers apply perturbation to each position in the seed and observe the change in the value of the program variable to obtain the related position of each path constraint.

However, existing solutions neglect the fact that different path constraints have complex relations. They build relations between some input bytes and one path constraint at one time. The relations between different path constraints can be grouped in real programs into the following two categories.

\begin{itemize}
  \item [1)] 
  Direct relation: the combination of different path constraints result in different execution paths.   
  \item [2)]
  Indirect relation: an input position may be used by different path constraints in different program logics.
\end{itemize}

Both methods mentioned above are inefficient in these cases. They focus more on how to identify more accurate valuable positions for a single path constraint while ignoring the use of the relations between different path constraints to improve the efficiency of fuzzing.

The key to solving both cases lies in fully using the path constraints' related positions (i.e., valuable positions).

\begin{itemize}
  \item [1)] 
  For direct relation, if we can jointly mutate the valuable positions corresponding to multiple path constraints, then we can try more combinations of different path constraints to discover new edges that are difficult to be explored by symbolic execution and inference.
  \item [2)]
  For indirect relation, if we can establish positions mapping between seeds that execute different program logics, then we can achieve the information exchange of valuable positions between seeds. When mutating a new seed, even if we do not analyze this seed, we can directly obtain potential valuable positions from other seeds, thereby improving the fuzzing efficiency.
\end{itemize}

In order to utilize valuable positions more efficiently, there are three key challenges as follows.

\textbf{The $challenge I$ is how to identify valuable positions without introducing additional overhead.} Although the inference-based method is easy to implement, it faces a time-consuming analysis process. In ProFuzzer, it needs to mutate each byte in the input 255 times, which takes much time. Especially in the case of long input, the required analysis time is unacceptable. 
For example, assume the input size is 10kB and the target program execute 1000 times per second.
Thus, the required analysis time is 10240 * 255/1000 = 2611 seconds. In Greyone, although it is not necessary to mutate each byte 255 times, Greyone needs to perform additional instrumentation for target programs to extract the specific value of the target cmps at runtime. 
However, the execution speed of the instrumented program is seriously slowed down.

\textbf{The $challenge II$ is how to achieve the exchange of valuable positions information between seeds.} The biggest problem of information exchange between seeds is the alignment problem. This is mainly caused by the following three reasons: 1) the length of the initial seed and the meaning of each position are inconsistent; 2) the effect of trimming on the length of the seed; 3) the effect of length mutators such as insert and delete. In order to be able to exchange information between seeds, a matching mechanism is needed to find positions with the same meaning on different seeds.


\textbf{The $challenge III$ is how to choose suitable valuable positions for mutation?} The importance of a position is not constant, and it changes over time. We need to design an algorithm that can dynamically update the position distribution based on the mutation results.

To address these challenges, we propose \tool{}, a lightweight family-based inference analysis method, to address the above three challenges.
To solve the problem in challenge I, 

To solve the problem in challenge I, \tool{} extract enough useful mutation information from havoc stage to integrate the pilot stage into the havoc stage.

To solve the problem in challenge II, 
\tool{} proposes a novel Family System to cluster all seeds based on the inheritance relationship, which coarsely maintains semantic consistency within a family.
Then, \tool{} maintains a shared pool in each family to record the valuable positions in each seed. 
All seeds in the same family can assess the shared pool. Thus, through some seeds only assigned less energy to mutate, they can also find their own valuable positions according to the shared pool based on the semantic consistency within a family.

To solve the problem in challenge III, \tool{} uses the LinUCB model to generate a possibility distribution for a seed.






\zhu{add citations where necessary}

In target programs used in fuzzing, their input usually consists of two parts: structure field and data field \zhu{structure-changing field and structure-preserving field? \cite{Nguyen2022BeDivFuzz}}. Among them, the structure field refers to the bytes related to the path change, and the data field refers to the information carried in the input (such as the specific content in the picture), which has nothing to do with the execution path of the program.
In coverage-guided fuzzing, for higher coverage, existing fuzzers try to mutate bytes in structure fields to avoid wasting time on data fields. To achieve this purpose, there are mainly the following two methods.
%在常见的fuzzing所用的目标程序中，他们的input通常由结构字段和数据字段两部分构成。其中，结构字段是指那些与路径变化相关的bytes，而数据字段是指input中所承载的信息（例如图片中的具体内容），它们和程序的执行路径无关。
%在coverage-guided fuzzing中，为了更高的coverage，现有的fuzzers都尽量去突变结构字段中的bytes，以免在数据字段之上浪费时间。为了实现这一目的，现有主要有以下两种方法。

\textbf{Traditional grammatical rule-based methods.} The input is parsed based on the specific grammar rules of the target program, and the input is divided into structure fields and data fields. However, this solution needs to prepare the specific grammar rules of the target program in advance, which requires a lot of human resources and time.
%1、传统的解决方案：基于目标程序的具体语法规则对Input进行解析，将Input切分为结构字段以及数据字段；例如，XX和XX利用解析器对Inputs进行解析，从而......。但是，该方案需要提前准备好目标程序的具体语法规则，这需要耗费大量的人力与时间。并且，如ProFuzzer中所述，由于在不同的应用场景下，相同的bytes可以分别为数据字段和控制字段，所以.....

\textbf{Inference-based methods.} In order to solve the dependence of traditional solutions on grammar knowledge, inference-based methods emerge as the times require. Specifically, inference-based methods will set up a pilot stage before havoc stage to perform mutation testing on each byte in the input to observe whether the execution state change. If the  execution state change, the byte is located in the structure field; otherwise, the byte is located in the data field. This type of method (e.g., ProFuzzer, Greyone) often only requires additional instrumentation of some program execution information, and the implementation is straightforward. For ProFuzzer, it needs to try all the values of each byte one by one and construct a feature vector based on the corresponding path length to analyze the specific type of each byte. For Greyone, it only pays attention to which bytes are located in the structure field. It needs to mutate each byte several times and check whether the value of cmp changes. If it changes, the mutated byte is located in the structure field. However, inference-based methods also face the following two problems.
%inference-based的解决方案：为了解决传统方案对语法知识的依赖，inference-based的方法应运而生。具体来说，此类方法会设置一个pilot stage，在正式的fuzzing之前提前对input中的每个byte进行突变测试，观察路径/cmp值是否发生变化。如果执行路径/cmp值发生变化，说明该byte位于结构字段之中；否则，该byte位于数据字段之中。这类方法（eg：ProFuzzer、Greyone）往往只需要额外插桩部分程序运行信息，实现上非常简单。对于ProFuzzer来说，它需要逐个尝试每个byte的所有值并基于对应路径长度来构造特征向量，从而分析每个byte的具体类型。对于Greyone而言，它只关注哪些bytes位于结构字段，它需要对每个byte突变数次并查看cmp的值是否发生变化，如果变化则说明该byte位于结构字段之中。然而，inference-based的方法也就面临着以下两个问题。

\textbf{First, although the inference-based method is easy to implement, it faces a time-consuming analysis process.} In ProFuzzer, it needs to mutate each byte in the input 255 times, which takes much time. Especially in the case of long input, the required analysis time is unacceptable. 
For example, assume the input size is 10kB and the target program execute 1000 times per second.
Thus, the required analysis time is 10240 * 255/1000 = 2611 seconds. In Greyone, although it is not necessary to mutate each byte 255 times, Greyone needs to perform additional instrumentation for target programs to extract the specific value of the target cmps at runtime. 
However, the execution speed of the instrumented program is seriously slowed down.
%We have tested it on AFL++, and the program execution speed after instrumentation is seriously slowed down (given specific data).
%• 一、Inference-based的方法虽然实现简单，但是面临着分析过程耗时的问题。在ProFuzzer中，它需要对input中的每个byte突变255次，这个过程需要耗费大量的时间。特别是在长input的情况，所需要的分析时长难以让人接受。例如，假设有一个input大小为10kB，目标测试程序每秒可执行1000次，则需要的分析时间为10240 * 255/1000 = 2611秒。而在Greyone中，虽然不需要对每个byte都突变255次，但是Greyone需要对每个目标程序进行额外的插桩，来提取出目标cmps在运行时的具体值。我们在AFLPlusPlus上经过测试，插桩后的程序程序执行速度严重减慢（给出具体数据）。

\textbf{Second, although inference-based methods also perform mutation in the pilot stage, its efficiency is relatively low.} In essence, the mutation method in the pilot stage is consistent with the deterministic stage in AFL, which is to mutate each byte in the input one by one. However, MOPT has pointed out that the deterministic mutation strategy is inefficient, and long-term exposure to this strategy will affect the overall efficiency of fuzzing. Therefore, there is an urgent need for a new method of identifying structure fields that do not depend on grammar knowledge and do not require much analysis time.
%inference-based在plot stage时虽然也在进行突变，但是其效率是较为低下的。实质上，inference-based的方法中的plot stage的突变方式和AFL中的deterministic stage是一致的，都是对input中的各个byte逐个进行突变。但是，MOPT已经指出deterministic的突变策略效率很低，长期处于该策略会影响fuzzing的整体效率。所以，现在急需一个既不依赖于语法知识，也不需要耗费大量分析时间的新的识别结构字段的方法。

\textbf{Third, the inference-based method does not mutate multiple positions simultaneously during the pilot stage?, mainly to avoid the following two reasons.} 1) If multiple positions are mutated at once, they may contain redundant positions. We cannot determine which position's mutation caused the change of execution state, which will cause an over-taint problem.
2) If multiple positions are mutated at one time, the number of mutation combinations that need to be tried in the pilot stage will exponentially increase, causing the problem of extended analysis time. However, only considering the case of mutating a single position will cause an under-taint problem. Some execution states need to mutate multiple positions simultaneously before they can be discovered. \zhu{Will this really be a problem? Although they do not mutate multiple positions at inference stage, they mutate multiple positions during the main fuzzing stage.}\zkp{But they do not infer the structure-related positions during the main fuzzing stage. And this problem has been mentioned in the paper of GREYONE.} \zhu{==> waste energy in havoc stage}
%第三，inference-based method do not mutate multiple positions at the same time，这么做主要是为了避免以下两个问题。1）一次性突变多个positions可能会包含冗余的positions，无法确定new coverage来自于哪个position的突变，这样就会造成over-taint的情况；2）如果一次性突变多个positions，那么在pilot stage所需要尝试的突变组合数就会快速增长，造成分析时间过长的问题。但是，仅仅考虑突变单个position的情况会造成under-taint的问题，有些new coverage需要同时突变多个positions才可以被发现。

We call the data pair of mutated positions and mutation result obtained by performing a mutation on a seed as \textbf{mutation information}, namely (mutated position, execution state changed or not).
The essence of the pilot stage is to mutate each byte in the seed to obtain a dataset that contains much mutation information.
Then, the structure-related positions can be extracted from the dataset.
In the dataset, the $feature\ vector$ is a mutated position, and the $label$ is whether execution state changed.
In particular, there is only one position within the $feature\ vector$. Therefore, the structure-related positions can be found directly according to the dataset. In other words, if the $label$ is 1, the position recorded in the $feature\ vector$ is structure-related. Since the mutation of the pilot stage will cover every position in the seed, all positions will be analyzed.
%• Pliot stage的实质就是通过对种子中的每一个byte进行突变得到一个“input为mutated positions序列，label为路径/cmp值是否改变”的数据集，然后再从该数据集中提取结构字段的位置信息。特别的，该数据集input的内仅有一个位置。所以，可以直接根据该数据集找到该种子结构字段的所处位置。具体的，如果label为1时，input中的position即为结构字段的位置。由于Plot stage的突变会覆盖到种子上的每一个position，所以该数据集中会有所有positions的数据，进而对所有的positions进行分析。（画图说明）


As the fuzzing process can complete hundreds or thousands of mutations in one second, if we can extract enough useful mutation information to replace the dataset generated by the pilot stage, we can \textbf{integrate the pilot stage into the havoc stage}. Thus, there is no need to set the pilot stage for analysis, which improves the fuzzing efficiency. 

However, there are many difficulties in integrating the pilot stage into havoc stage. We need to overcome the following challenges.

First, we collect mutation information to replace the dataset generated by the pilot stage. However, collecting all mutation information in havoc stage is impractical, which takes much time. Due to the randomness of fuzzing, most of the mutation information does not contain any information. That is, they will not cause execution state changes. Therefore, a lightweight strategy must be deployed to extract more useful mutation information from massive data (\textbf{Challenge I}). 

After we have a new dataset generated from havoc stage, we extract the structure-related positions for each seed from it. However, the dataset generated from the pilot stage and the dataset generated from havoc stage are inconsistent in $feature\ vector$. Since only one position is mutated at a time in the pilot stage, the $feature\ vector$ length of the former is 1. As multiple positions could be mutated simultaneously in havoc stage, the $feature\ vector$ length of the latter is likely to be greater than 1. Therefore, we need an inference-based analysis method suitable for mutating multiple positions simultaneously (\textbf{Challenge II}).

If we want to analyze all seeds with the above method, then each seed needs to be allocated enough energy to mutate in havoc stage. However, not all seeds will be allocated much energy to mutate. How do seeds that are allocated less energy extract enough information to analyze their structural fields (\textbf{Challenge III})? Therefore, a reasonable strategy is required to extract the structure-related positions for the seeds with low energy.
% In this paper, we propose a lightweight sharing mechanism-based structural field analysis method. We have the following steps to integrate the pilot stage into havoc stage stage. 

% First, it collects useful mutation information to replace the dataset generated by the pilot stage. -> What is useful mutation information? 
% Can we extract the structure-related positions for each seed from this new dataset?
% Why can the dataset generated by the pilot stage be replaced?

% Second, it identifies the structure-related positions for each seed. -> how to extract the structure-related positions when a seed mutates multiple positions at once. 





% However, we need to address the following three main challenges.
%• 由于Fuzzing过程中一秒钟都可以完成成百上千次的突变，如果我们可以从中提取出部分有用的突变信息来替代plot stage生成的数据集，我们就可以将plot stage融入到实际的fuzzing过程中，从而不需要额外设置plot stage进行分析。但是，我们需要解决以下三个主要挑战。

% \textbf{Challenge I}: What is useful mutation information? Why can the dataset generated by the pilot stage be replaced? Due to the randomness of fuzzing, most of the mutation information do not contain any information. That is, they will not cause changes in paths or changes in cmps' values. Therefore, we need to extract useful mutation information from massive data to replace the data set generated by the pilot stage.
%Challenge I：什么是有用的突变信息？为什么可以对plot stage生成的数据集进行替换？由于fuzzing的随机性，绝大部分的突变结果都不包含任何信息量，即不会造成路径的变化或者cmp值的改变。所以，我们需要从海量的数据中抽取出有用的突变信息出来，从而去替代plot stage所生成的数据集。

% \textbf{Challenge II}: To replace the dataset, a large amount of mutation information is required for selection.
% However, not all seeds will be allocated a large amount of energy to mutate.
% How do seeds that are allocated less energy extract enough information to analyze their structural fields?
%Challenge II：如果根据“一”中的方法替换pilot stage，则需要有大量的突变数据来进行选择。但是，并不是所有的种子都会被分配大量的能量进行突变。对于那些分配能量较少的种子，如何提取足够的信息来分析自己的结构字段？

% \textbf{Challenge III}: Can the recognition accuracy of the inference-based method be achieved after the replacement? Can we get better results on coverage?
%Challenge III：替代之后能否达到inference-based方法的识别精度？能否在coverage上取得更好的效果？

\zhu{You should explicitly mention the reasons of your solutions. Greyone infers structure-related bytes BEFORE it finds new coverage. So the structure-related bytes are useful when discovering new bytes. But your recorded bytes have already discovered new coverage, how come that they are useful when discovering new coverage in the future? You need to answer this question very carefully.}
\zkp{As we introduce a new indicator $local\ new\ edges$, I think we do not need to answer this question any more. $Local\ new\ edges$ is not equal to traditional new edges.} \zhu{you still need to answer this because the essential objective is to discover global new edges. You have to link the local new edges to the global new edges.} \zkp{For the same path constraint, the related positions on different seeds may not be consistent. We have constructed position mapping for seeds within the same family, but we have no way to construct position mapping between families. If we only collect data based on global new edges, then we will miss some valuable positions for some partial seeds. For example, given initial seeds $A$ and $B$, they have no semantic consistency. If the path constraint $X$ is resolved when $position 1$ of $A$ is mutated, then $position 1$ will be added to the shared pool of the family where $A$ is located. However, since there is no semantic consistency between $A$ and $B$, we have no way to find the related positions of path constraint $X$ in seed $B$ according to the position mapping relationship. At the same time, since path constraint $X$ has already been solved, the next time the seed $B$ is mutated and path constraint $X$ is solved, we will not extract valuable positions from it. Thus, we have no way to find the related positions of path constraint $X$ in seed B. Finally, if we can't find the related positions of all path constraints on all seeds, it will naturally affect the improvement of fuzzing efficiency.}

We propose \tool{}, a lightweight family-based inference analysis method, to address the above three challenges.
To solve the problem in challenge I, we propose a novel indicator $local\ new\ edges$ to extract more useful mutation information without introducing time-consuming problem or data explosion problem.
Specifically, given a seed $t$, local new edges are the edges that have not been covered by the seed $t$ and the mutated inputs from the past.
Thus, \tool{} construct inference dataset based on the mutation that finds local new edges. In addition, we use 48h fuzzing data for SHAP analysis in the section X to get the ground truth of important positions for each seed. Then, we verify that the structure-related bytes we identify can cover most of the important positions within 1h.
% First, \tool{} extracts the mutation information and finds new edges to replace the dataset generated by the pilot stage.
To solve the problem in challenge II,  \tool{} removes all irrelevant mutated positions in the dataset to achieve accurate inference analysis when having multiple mutated positions simultaneously.
To solve the problem in challenge III, 
\tool{} proposes a novel Family System to cluster all seeds based on the inheritance relationship, which coarsely maintains semantic consistency within a family.
Then, \tool{} maintains a shared pool in each family to record the structure-related positions in each seed. 
All seeds in the same family can assess the shared pool. Thus, through some seeds only assigned less energy to mutate, they can also find their own structure-related positions according to the shared pool based on the semantic consistency within a family.
% Finally, We construct a SHAP analysis to identify the important positions in the seed and verify that Pozzer can cover most of the important positions in a short time.

In this paper, we implement the prototype of \tool{} based on AFL++. (Experiment Result) 
In order to avoid subjective factors, we evaluated \tool{} on two third-party platforms, UNIFUZZ and MAGMA.
In UNIFUZZ, we evaluate \tool{}-related fuzzers (i.e. \tool{} and \tool{}-Redqueen) and multiple existing modes of AFL++ on XX target program. \tool{} discovers more XX\% and X\% on code coverage and bugs than the best mode existing in AFL++, respectively.
In MAGMA, we evaluate these two \tool{}-related fuzzers and 5 widely-used mutation-based fuzzers(AFL, AFLFast, FairFuzz, MOPT and AFL++) on X programs. \tool{}-Redqueen exposes more X CVEs that the best compared fuzzer.


We summarize our contributions as follows.
\begin{itemize}
    \item We propose a family system to achieve the integration of the pilot stage and havoc stage. Based on semantic consistency, the seeds are divided into multiple families, which allows different seeds in the same family to share the structure-related positions identified by themselves to improve the efficiency of fuzzing.
    \item We propose a Family-Based Mutation Mode, which uses the LinUCB model to identify valuable positions within the family's shared pool for each seed to guide the mutation direction.
    \item We implement a prototype \tool{} based on AFL++, evaluate it based on UNIFUZZ and MAGMA platforms. The results indicate that \tool{} outperforms various state-of-the-art fuzzers on edge coverage and bug discovery.
\end{itemize}

==> obsolete/intro-0.4.tex <==



\section{Introduction}

% \zhu{ our keys?:
% \begin{itemize}
%     \item the combination of different path constraints result in different execution paths
%     \item an input position may be used as a path constraint in different program logics
% \end{itemize}}
% \zhu{KEY: existing solution infer a fixed group for mutation; our solution evolves the groups during fuzzing?}


For analyzing security issues in software, both academic and industrial practitioners regard fuzzing as the de facto detection technique~\cite{zhu2022roadmap}.
Among all the fuzzing solutions, coverage-guided greybox fuzzing (CGF) has achieved a great success in detecting real-world bugs~\cite{ossfuzz, onefuzz, feng2021snipuzz, aflchurn}. 
It aims to discover new code coverage so that bugs may be disclosed in those unseen code. Existing research has spent many efforts in expanding code coverage, including scheduling computing resources for certain code regions~\cite{aflfast, fairfuzz, Yue2020EcoFuzz} and resolving path constraints~\cite{angora, driller, SymFuzz, qsym, dowser, matryoshka}.
While scheduling computing resources is an implicit way to expand code coverage, resolving path constraints is an explicit way to achieve it. Since path constraints guard a certain code region, any success in passing path constraints most likely results in new code coverage. However, resolving path constraints is not a free lunch as those constraints may be quite complicated. 


% Existing solutions for resolving path constraints can be categorized into symbolic execution based solutions and inference based solutions \zhu{citations}. Symbolic execution builds formula for constraints along an execution path and uses constraint solver to generate inputs that satisfy those constraints \zhu{citations}.
Because fuzzing repeatedly tests a program, a promising solution for resolving path constraints is to infer the relationships among input bytes and mutate related bytes together in later fuzzing campaigns~\cite{greyone, ems, profuzzer, neuzz}.
For instance, some fuzzers build the relationship among input bytes if they influence the same path constraint~\cite{greyone, ems, angora, vuzzer, steelix} or construct the same data type~\cite{profuzzer, angora}.
The inference can reduce the search space of passing constraints if fuzzing combines the related bytes into groups and mutates inputs based on groups. 
For instance, mutating 12 bytes can generate $256^{12}$ different inputs while mutating 4 bytes at a time (4 bytes a group) only generates $3\times256^{4}$ different inputs. 
If a path constraint can be resolved by mutating one group, the combination of bytes can significantly improve the efficiency of code discovery. 
% Existing research builds the relationship among input bytes if they influence the same path constraint \zhu{cite; greyone, ems} or construct the same data type \zhu{cite; profuzzer}. \zhu{more fuzzers?} 


Essentially, the groups of bytes reflect the formats of inputs, which further represent the internal logic of programs. However, the existing inference solutions only reveal the shallow logic of programs. Those solutions only infer the relationships of bytes for a single path constraint at a time. Each time, the bytes related to a single path constraint are mutated, which neglects the fact that different path constraints may be heavily coupled. For example, to pass the condition $if(b == 0x123)$, we may need to figure out all the conditions that the variable $b$ depends on, such as $if(a == 0x22)\{b = 0x12\}$. In this case, it is insufficient to only mutate the bytes related to the variable $b$ for passing the path constraint. Therefore, in order to fuzz deep program logic, the inference for related bytes is required to consider the coupling of path constraints.



In this paper, we propose \tool{}, a lightweight fuzzer, to mutate inputs considering the coupling of path constraints. \tool{} infers and groups the bytes related to the coupled path constraints based on two observations. One observation is what we call \textit{direct coupling}, where the flip of a path constraint must consider the results of other path constraints.
% different path constraints in the same execution path influence or use the same data. 
The exploration of directly coupled path constraints will lead to deep code in programs (exemplified in Section~\ref{sec:motivation}). Another observation is that different program logics may process the same format of inputs, indicating that different constraints are related to the same positions of inputs (we call it \textit{indirect coupling}). 
The usage of indirect coupling helps fuzzing quickly explore new code if a fuzzer only mutates the corresponding input positions (exemplified in Section~\ref{sec:motivation}).


Based on the two observations, \tool{} builds a \textit{family system} to share positions that have discovered new code coverage (observation of indirect coupling) and combine the shared positions to mutate members in the same family (observation of direct coupling).
To achieve that, the family system is required to ensure that, for any seed in a family, the shared positions are still related to the seed's corresponding path constraints.
% the positions shared in the family are related to path constraints for every member.
% To achieve that, the family system is required to maintain the semantic meaning of positions among different seeds (\ie the retained inputs). In other words, the family system is required to make sure that the positions shared in a family are still related to path constraints when the length of a seed is changed.
% Basically, two seeds belong to the same family if they are obtained by mutating the same seed without changing its length. In this way, \tool{} can roughly maintain the semantic meaning of input positions.
To satisfy the requirement, a family is built if seeds (\ie the retained inputs) in the family are obtained by mutating the same seed without changing its length.
Since the meaning of each position may be changed by the trimming stage, which is performed to reduce the length of seeds, \tool{} traces the change of positions to maintain the meaning of positions. 
However, the building process of a family can only roughly satisfy the requirement.
% ensure that, for any seed in the family, the shared positions are still related to path constraints. 
To improve the possibility that the selected positions for a seed are related to path constraints, \tool{} uses LinUCB \zhu{cite; the general explanation of LinUCB} to dynamically generate a probability distribution for selecting positions based on the feedback of fuzzing.
% select shared positions.
% LinUCB dynamically generates a probability distribution based on the feedback of fuzzing, and \tool{} selects shared positions based on the distribution.
Note that, the positions selected by LinUCB may be related to more than one path constraint so that the directly coupled path constraints can be resolved.

% Instead of mutating inputs byte by byte to obtain the bytes related to path constraints, \tool{} 

\zkp{

Based on the two observations, there are two main challenges here to leveraging the coupling of path constraints.
\begin{itemize}
  \item [1)]
  Challenge I: How to infer the related bytes of a single path constraint in a more lightweight method?
  \item [2)] 
  Challenge II: How to group bytes based on the relations between path constraints?
\end{itemize}

To overcome Challenge I, instead of utilizing an additional pilot stage to analyze each position like inference-based fuzzer, Pozzer integrates the pilot stage into the havoc stage and directly extracts useful data from the fuzzing process. 
Specifically, \tool{} collects mutation information from those mutations that flip path constraints to analyze the related positions.
Thus, the analysis time of Pozzer is not affected by seed length. 
Since a constraint can be passed by multiple seeds, a constraint may be inferred repeatedly.
As all seeds share a constraint space, different seeds can share the related positions they found for the same constraint.
However, there are many factors in the fuzzing process that may cause alignment problems between seeds, such as different initial seed structures, trimming and other operations.
To solve this problem, establishing a position mapping between seeds is necessary.
However, due to the complexity of the seed structure, it is difficult to find the semantic mapping between seeds with different structures.
If two seeds have an inheritance relationship, they are more likely to have the same structures.
Therefore, we propose a \textbf{family system} based on the inheritance relationship. More specifically, we use the initial seed to establish a family, and the offspring seeds obtained from its mutation will be added to the family.
In a family, we use a \textit{semantic tracking algorithm} to establish the semantic mapping between seeds within the family.
Each seed has an independent relative position space, and the position inside the seed is called the \textit{relative position}.
To achieve semantic mapping, we need to map the relative position of each seed to the same absolute position space so that alignment can be achieved.
Thus, each family builds an absolute position space based on the ancestor seed who constructs this family.
The semantic tracking algorithm maps the relative position in the seed to the absolute position space based on the position mapping between seeds during seed generation, which achieves semantic mapping.
% In a family, we use a \textit{semantic tracking algorithm} and \textit{absolute position space mechanism} to establish the semantic mapping between seeds within the family.
% 1) \textbf{Semantic tracking algorithm}. The semantic tracking algorithm tracks position mapping between seeds during seed generation.
% 2) \textbf{Absolute position space mechanism.} Each seed has an independent relative position space, and the position inside the seed is called the \textit{relative position}.
% To achieve semantic mapping, we need to map the relative position of each seed to the same absolute position space so that alignment can be achieved.
% Thus, each family builds an absolute position space based on the ancestor seed who constructs this family.
% The absolute position space mechanism maps the relative position in the seed to the absolute position space based on the semantic tracking algorithm to achieve semantic mapping.
Then, different seeds can communicate in the same absolute position space, avoiding alignment problems.
Finally, seeds within the same family can exchange information based on semantic mapping to speed up the analysis process. 
% To solve this problem, Pozzer proposes a \textit{family system}. 
% The key of the family system is to maintain the \textit{semantic mapping} (i.e., find positions with the same meaning on different seeds) in inputs, where we regard the positions of inputs are more important than the values. 
% %We define \textit{valuable positions} as positions related to all solved path constraints in a seed. 
% %valuable positions就是所有solved path constraints的related positions的合集；因为我们得到valuable positions的前提是发现了新边，所以只能够找到solved constraints的related positions
% To achieve semantic mapping, Pozzer first groups seeds into a family based on \textit{semantic preservation algorithm}, which tracks position mapping between seeds. 
% Then, each family builds a \textit{absolute position space} based on the ancestor seed who constructs this family, and the position inside a seed is called \textit{relative position}.
% Each seed can map its relative position to the absolute position space based on the semantic preservation algorithm to obtain the \textit{absolute position}.
% Then, different seeds can communicate in the same absolute position space, avoiding alignment problems.
% % Thus, each family maintains a \textit{shared pool} to record the absolute positions of valuable positions of each seed.
% % Finally, the seeds in the same family can share the valuable positions based on shared pool according to semantic mapping to speed up the analysis process. 
% Finally, seeds within the same family can exchange information based on semantic mapping to speed up the analysis process. 

% To achieve semantic mapping, each seed can convert its internal relative position into absolute position space based on \textit{semantic preservation algorithm}, which tracks position mapping between seeds. 
% Each seed in the family convert its internal relative position into a universal absolute position through absolute position space, so that information exchange can be achieved between different seeds.
% Pozzer groups seeds into a family based on \textit{semantic preservation algorithm}, which tracks position mapping between seeds. 
% specific \textit{absolute scales}. All seeds in the family can 
% By establishing \textit{absolute scales}, seeds within the same family can achieve semantic mapping.
% Specifically, each family owns a specific \textit{absolute scales}
% Each family maintains a \textit{shared pool} to record valuable positions of all constraints.
% Any seed in the family can share the valuable positions found by it or use the valuable positions found by others.
% The key of the family system is to maintain the semantic information in inputs, where we regard the positions of inputs are more important than the values. 
% The seeds in the same family can share the related positions of constraints based on semantic information to speed up the analysis process. 

\zhu{efficiency->family system: 1. length of input (mutate every byte); 2. repeated inference of the same constraint.}

To solve the problem of Challenge II, Pozzer utilizes a LinUCB model to group the positions related to constraints. 
Given a seed, the purpose of mutation is to explore unsolved constraints around the seed.
% To explore unsolved constraints considering the coupling of path constraints, the key is constantly flipping the related solved path constraints, that is, to mutate the related positions of the related solved constraints.
From the analysis at Section~\ref{sec:motivation}, it can be seen that the key of exploring unsolved constraints considering the coupling of path constraints is to constantly flip the related solved path constraints, that is, to mutate the related positions of the related solved constraints.
As the logic of real programs is complex, it is challenging to directly analyze the relationship between constraints.
And the purpose of obtaining the path constraints relationship is grouping related positions of the related solved path constraints. 
%Given a seed, we can group positions related to all solved path constraints as \textit{valuable positions}. 
Thus, we can group positions directly based on the relationship between unsolved constraints and all \textit{valuable positions} (i.e., the positions related to all solved path constraints in a seed).
%At the same time, given a seed, since the purpose of obtaining the path constraints relationship is grouping positions, we can directly find the relationship between unsolved constraints and all valuable positions to group positions.
% Since it is challenging to directly analyze the relationship between constraints, we use the LinUCB model to continuously learn the relationship between unsolved constraints and valuable positions during the fuzzing process.
% We group all valuable positions of solved constraints into a \textit{candidate pool}.
To achieve this goal, Pozzer first assumes that all solved constraints are related to unsolved constraints, that is, mutate all  valuable positions.
Then, Pozzer uses a LinUCB model to dynamically generate a distribution for valuable positions based on the fuzzing feedback, which is used to measure the relationship between the unsolved constraints and each position valuable positions, that is, to indirectly measure the relationship between the unsolved constraints and solved constraints.
Finally, Pozzer constructs byte groups based on the distribution.
}

% Based on the two observations, our \tool{} builds a \textit{family system}. The key of the family system is to maintain the semantic information in inputs, where we regard the positions of inputs are more important than the values.





% \todo{Our \tool{} aims to use the relations between path constraints. While determining the relation between path constraints is quite challenging, the relation offers fuzzing a different perspective to improve efficiency.:\begin{itemize}
%     % \item dataflow analysis? taint analysis?
%     % \item the path constraints are the main (maybe the only?) road rocks for coverage discovery
%     % \item grammars somehow reflect the control flows of programs
%     % \item existing solutions neglect the fact that different path constraints have complex relations. They build relations between some input bytes and one path constraint at one time. they focus on a single path constraint.
%     % \item some challenges to overcome the coupling of path constraints
%     % \item we propose \tool{} to solve the challenges based on two observations
%     % \item observations: complex relations between path constraints: \begin{itemize}
%     %     \item direct relation: the combination of different path constraints result in different execution paths
%     %     \item indirect relation: an input position may be used by different path constraints in different program logics
%     % \end{itemize}
%     \item others: \begin{itemize}
%         \item Why do we use family? the relation between family and the observations : in path A, position $a$ is related to constraint; then in path B, we hope the position $a$ is still related to constraint.
%          \item reduce search space: the key is to prioritize some bytes to reduce search space in input. existing solutions focus on prioritizing bytes related to a single path constraint.
%         \item KEY: existing solution infer a fixed group for mutation; our solution evolves the groups during fuzzing.
%         \item fuzzing can repeatedly try to figure out the combination of bytes for coupling constraints. therefore, it can still infer the byte relation based on coupling.
%     \end{itemize}
% \end{itemize}}



We implement the prototype of \tool{} based on AFL++. 
In order to avoid subjective factors, we evaluated \tool{} on two third-party platforms: UNIFUZZ, which contains several real-world programs and MAGMA, which provides a series of real-world programs with real bugs introduced.
On UNIFUZZ, we evaluate \tool{}-related fuzzers (i.e. \tool{} and \tool{}-Redqueen) and 5 existing modes of AFL++ on 16 target programs.
\tool{}-related fuzzers achieve better new edge coverage on most programs than other fuzzers after fuzzing 1/3/6/12/24 hours.
In addition, \tool{}-Redqueen discovered more 11 vulnerabilities than the best mode in AFL++.
On MAGMA, we evaluated \tool{}-related fuzzers and 5 widely-used mutation-based fuzzers(AFL, AFLFast, FairFuzz, MOPT and AFL++) on 20 programs. \tool{} exposed more 6 CVEs than the best compared fuzzer.
We further evaluated \tool{} with the existing inference-based fuzzers.
The positions inferred by \tool{} have more potential than others.


We summarize our contributions as follows.
\begin{itemize}
    \item We propose a family system to achieve the integration of the pilot stage and havoc stage. Based on semantic consistency, the seeds are divided into multiple families, which allows different seeds in the same family to share the structure-related positions identified by themselves to improve the efficiency of fuzzing.
    \item We propose a Family-Based Mutation Mode, which uses the LinUCB model to identify valuable positions within the family's shared pool for each seed to guide the mutation direction.
    \item We implement a prototype \tool{} based on AFL++, evaluate it based on UNIFUZZ and MAGMA platforms. The results indicate that \tool{} outperforms various state-of-the-art fuzzers on edge coverage and bug discovery.
\end{itemize}

==> obsolete/intro-1.0.tex <==



\section{Introduction}

\todo{enhance the description of reinforcement learning (LinUCB) and shap.}

Fuzzing is known as a de facto technique to detect software security issues among both academic and industrial practitioners~\cite{zhu2022roadmap}.
In the set of existing fuzzing solutions, coverage-guided greybox fuzzing (CGF) has performed remarkably well in detecting real-world bugs~\cite{ossfuzz, onefuzz, feng2021snipuzz, aflchurn}. 
This method aims to enhance code coverage so that potential bugs are disclosed in the unseen parts of the code. Existing studies have  reported many efforts to expand code coverage, including scheduling of computational resources for certain code regions~\cite{aflfast, fairfuzz, Yue2020EcoFuzz, mobfuzz} and resolving path constraints~\cite{angora, qsym, dowser, tfuzz, digfuzz, huang2020pangolin}.
While scheduling computational resources is an implicit way to expand code coverage, resolving path constraints is an explicit way to achieve the same. Since path constraints guard certain code regions, any success in passing path constraints most likely results in new code coverage. However, resolving path constraints is not a trivial task as those constraints may be quite complicated. 



In fuzzing, a promising solution for resolving path constraints is to infer the relationships among input bytes and mutate related bytes together in later fuzzing campaigns~\cite{greyone, ems, profuzzer, neuzz, mtfuzz, pata}.
For instance, some fuzzers establish a relationship between the input bytes that influence the same path constraint~\cite{greyone, ems, angora, vuzzer, steelix} or construct the same data type~\cite{profuzzer, angora}.
Such inferences can reduce the search space of passing constraints if fuzzing combines related bytes into groups and mutates them on a group basis. 
For instance, mutating 12 bytes can generate $256^{12}$ different inputs, while mutating 4 bytes at a time (4 bytes a group) only generates $3\times256^{4}$ inputs.
If a path constraint is related to just one group, the combination of bytes can significantly improve the efficiency of code discovery. 
 


Essentially, the groups reflect the format of inputs, which further represent the internal logic of programs. However, the existing inference solutions only give a shallow view to the logic of programs. These solutions only infer the relationships between bytes for a single path constraint at a time. Each time, the bytes related to a single path constraint are mutated. This neglects the fact that different path constraints might be heavily coupled. For example, to pass the condition $if(b == 0x123)$, we may need to figure out all the conditions that the variable $b$ depends on, such as $if(a == 0x22)\{b = 0x12\}$. In this case, it is insufficient to only mutate the bytes related to the variable $b$ for the path constraint to be passed. Therefore, in order to fuzz code guarded by complex constraints, the inference algorithm (of related bytes) needs to consider the coupling of path constraints.

\begin{figure*}[t!]
\centering
\includegraphics[width=0.8\linewidth]{images/motivation.pdf}
\caption{Example of direct and indirect coupling from \texttt{readelf}.}
\label{readelf_example}
\end{figure*}

In this paper, we propose \tool{}, a lightweight fuzzer that mutates inputs by considering the coupling of path constraints. \tool{} infers and groups the bytes related to the coupled path constraints based on two observations. One observation is what we call \textit{direct coupling}, and it refers to the fact that the flip of a path constraint has to consider the results of other path constraints.
The exploration of directly coupled path constraints will lead to deep codes in programs (exemplified in Section~\ref{sec:motivation}). Another observation is that different program logics may process the same format of inputs, indicating that different constraints are related to the same positions of inputs (we call it \textit{indirect coupling}). 
The usage of indirect coupling helps fuzzing quickly explore new code if a fuzzer only mutates the corresponding input positions (exemplified in Section~\ref{sec:motivation}).


Based on the two observations, \tool{} builds a \textit{family system} to share positions that have discovered new code coverage (observation of indirect coupling) and combine the shared positions to mutate members in the same family (observation of direct coupling).
To achieve that, the family system is required to ensure that, for any seed (\ie a retained input) in a family, the shared positions are still related to the seed's corresponding path constraints.
To satisfy the requirement, a family is built if seeds in the family are obtained by mutating a original seed without changing its length.
Since the meaning of each position may be changed by the trimming stage, which is performed to reduce the length of seeds, \tool{} traces the change of positions to maintain the meaning of positions. 
However, the building process of a family can only roughly satisfy the requirement. 
To improve the possibility that the selected positions for a seed are related to (unsolved) path constraints, \tool{} uses LinUCB \cite{linucb} to dynamically generate a probability distribution for the selection of positions. \zhu{a bit more about LinUCB; What problem can LinUCB solve? How to solve? what's the benefit of using LinUCB?}
Note that, the positions selected by LinUCB may be related to more than one path constraint so that the directly coupled path constraints can be fuzzed.

\todo{revise.}
We implement \tool{} based on AFL++~\cite{aflpp}, and evaluate it on two third-party platforms, including 1) UNIFUZZ~\cite{unifuzz}, which contains real-world programs, and 2) MAGMA~\cite{magma}, which provides a series of real-world programs with known bugs.
On UNIFUZZ, we evaluate \tool{}-related fuzzers (\ie \tool{} and \tool{}-Redqueen) and 5 existing modes of AFL++ on 16 target programs.
The results show that, in terms of coverage discovery, \tool{}-related fuzzers perform better than other fuzzers after running 1/3/6/12/24 hours.
Additionally, \tool{}-Redqueen discovers 11 more vulnerabilities than the best mode in AFL++.
On MAGMA, we evaluate \tool{}-related fuzzers and 5 widely-used mutation-based fuzzers (\ie AFL~\cite{afl}, AFL++-MOPT-Redqueen, AFLFast~\cite{aflfast}, FairFuzz~\cite{fairfuzz} and MOPT~\cite{MOPT}) on 20 programs. \tool{} exposes 6 more CVEs than the best of the 5 comparing fuzzers.
Additionally, we compare \tool{} to EMS~\cite{ems}, and the results show that \tool{} outperforms EMS in terms of edge discovery.
Our experiments also demonstrate that most of our inferred positions can discover new code coverage, which excludes the first time a position is retained.



We summarize our contributions as follows. \todo{revise?}
\begin{itemize}
    \item We observe that input bytes can be grouped based on direct coupling and indirect coupling of path constraints. We then propose \tool{}, which uses a family system to share positions of inputs among seeds in a family. The shared positions can be grouped to resolve directly and indirectly coupled path constraints.
    % We propose a family system to achieve the integration of the pilot stage and havoc stage. Based on semantic consistency, the seeds are divided into multiple families, which allows different seeds in the same family to share the structure-related positions identified by themselves to improve the efficiency of fuzzing.
    \item To improve the effectiveness of shared positions in discovering new code coverage, \tool{} uses LinUCB to schedule the combination of shared positions.
    % We propose a Family-Based Mutation Mode, which uses the LinUCB model to identify valuable positions within the family's shared pool for each seed to guide the mutation direction.
    \item We implement \tool{} based on AFL++, and evaluate it based on the platforms UNIFUZZ and MAGMA. The results indicate that \tool{} outperforms various state-of-the-art fuzzers in terms of edge coverage and bug discovery.
\end{itemize}



% \zkp{

% Based on the two observations, there are two main challenges here to leveraging the coupling of path constraints.
% \begin{itemize}
%   \item [1)]
%   Challenge I: How to infer the related bytes of a single path constraint in a more lightweight method?
%   \item [2)] 
%   Challenge II: How to group bytes based on the relations between path constraints?
% \end{itemize}

% To overcome Challenge I, instead of utilizing an additional pilot stage to analyze each position like inference-based fuzzer, \tool{} integrates the pilot stage into the havoc stage and directly extracts useful data from the fuzzing process. 
% Specifically, \tool{} collects mutation information from those mutations that flip path constraints to analyze the related positions.
% Thus, the analysis time of \tool{} is not affected by seed length. 
% Since a constraint can be passed by multiple seeds, a constraint may be inferred repeatedly.
% As all seeds share a constraint space, different seeds can share the related positions they found for the same constraint.
% However, there are many factors in the fuzzing process that may cause alignment problems between seeds, such as different initial seed structures, trimming and other operations.
% To solve this problem, establishing a position mapping between seeds is necessary.
% However, due to the complexity of the seed structure, it is difficult to find the semantic mapping between seeds with different structures.
% If two seeds have an inheritance relationship, they are more likely to have the same structures.
% Therefore, we propose a \textbf{family system} based on the inheritance relationship. More specifically, we use the initial seed to establish a family, and the offspring seeds obtained from its mutation will be added to the family.
% In a family, we use a \textit{semantic tracking algorithm} to establish the semantic mapping between seeds within the family.
% Each seed has an independent relative position space, and the position inside the seed is called the \textit{relative position}.
% To achieve semantic mapping, we need to map the relative position of each seed to the same absolute position space so that alignment can be achieved.
% Thus, each family builds an absolute position space based on the ancestor seed who constructs this family.
% The semantic tracking algorithm maps the relative position in the seed to the absolute position space based on the position mapping between seeds during seed generation, which achieves semantic mapping.
% % In a family, we use a \textit{semantic tracking algorithm} and \textit{absolute position space mechanism} to establish the semantic mapping between seeds within the family.
% % 1) \textbf{Semantic tracking algorithm}. The semantic tracking algorithm tracks position mapping between seeds during seed generation.
% % 2) \textbf{Absolute position space mechanism.} Each seed has an independent relative position space, and the position inside the seed is called the \textit{relative position}.
% % To achieve semantic mapping, we need to map the relative position of each seed to the same absolute position space so that alignment can be achieved.
% % Thus, each family builds an absolute position space based on the ancestor seed who constructs this family.
% % The absolute position space mechanism maps the relative position in the seed to the absolute position space based on the semantic tracking algorithm to achieve semantic mapping.
% Then, different seeds can communicate in the same absolute position space, avoiding alignment problems.
% Finally, seeds within the same family can exchange information based on semantic mapping to speed up the analysis process. 
% % To solve this problem, \tool{} proposes a \textit{family system}. 
% % The key of the family system is to maintain the \textit{semantic mapping} (i.e., find positions with the same meaning on different seeds) in inputs, where we regard the positions of inputs are more important than the values. 
% % %We define \textit{valuable positions} as positions related to all solved path constraints in a seed. 
% % %valuable positions就是所有solved path constraints的related positions的合集；因为我们得到valuable positions的前提是发现了新边，所以只能够找到solved constraints的related positions
% % To achieve semantic mapping, \tool{} first groups seeds into a family based on \textit{semantic preservation algorithm}, which tracks position mapping between seeds. 
% % Then, each family builds a \textit{absolute position space} based on the ancestor seed who constructs this family, and the position inside a seed is called \textit{relative position}.
% % Each seed can map its relative position to the absolute position space based on the semantic preservation algorithm to obtain the \textit{absolute position}.
% % Then, different seeds can communicate in the same absolute position space, avoiding alignment problems.
% % % Thus, each family maintains a \textit{shared pool} to record the absolute positions of valuable positions of each seed.
% % % Finally, the seeds in the same family can share the valuable positions based on shared pool according to semantic mapping to speed up the analysis process. 
% % Finally, seeds within the same family can exchange information based on semantic mapping to speed up the analysis process. 

% % To achieve semantic mapping, each seed can convert its internal relative position into absolute position space based on \textit{semantic preservation algorithm}, which tracks position mapping between seeds. 
% % Each seed in the family convert its internal relative position into a universal absolute position through absolute position space, so that information exchange can be achieved between different seeds.
% % \tool{} groups seeds into a family based on \textit{semantic preservation algorithm}, which tracks position mapping between seeds. 
% % specific \textit{absolute scales}. All seeds in the family can 
% % By establishing \textit{absolute scales}, seeds within the same family can achieve semantic mapping.
% % Specifically, each family owns a specific \textit{absolute scales}
% % Each family maintains a \textit{shared pool} to record valuable positions of all constraints.
% % Any seed in the family can share the valuable positions found by it or use the valuable positions found by others.
% % The key of the family system is to maintain the semantic information in inputs, where we regard the positions of inputs are more important than the values. 
% % The seeds in the same family can share the related positions of constraints based on semantic information to speed up the analysis process. 

% \zhu{efficiency->family system: 1. length of input (mutate every byte); 2. repeated inference of the same constraint.}

% To solve the problem of Challenge II, \tool{} utilizes a LinUCB model to group the positions related to constraints. 
% Given a seed, the purpose of mutation is to explore unsolved constraints around the seed.
% % To explore unsolved constraints considering the coupling of path constraints, the key is constantly flipping the related solved path constraints, that is, to mutate the related positions of the related solved constraints.
% From the analysis at Section~\ref{sec:motivation}, it can be seen that the key of exploring unsolved constraints considering the coupling of path constraints is to constantly flip the related solved path constraints, that is, to mutate the related positions of the related solved constraints.
% As the logic of real programs is complex, it is challenging to directly analyze the relationship between constraints.
% And the purpose of obtaining the path constraints relationship is grouping related positions of the related solved path constraints. 
% %Given a seed, we can group positions related to all solved path constraints as \textit{valuable positions}. 
% Thus, we can group positions directly based on the relationship between unsolved constraints and all \textit{valuable positions} (i.e., the positions related to all solved path constraints in a seed).
% %At the same time, given a seed, since the purpose of obtaining the path constraints relationship is grouping positions, we can directly find the relationship between unsolved constraints and all valuable positions to group positions.
% % Since it is challenging to directly analyze the relationship between constraints, we use the LinUCB model to continuously learn the relationship between unsolved constraints and valuable positions during the fuzzing process.
% % We group all valuable positions of solved constraints into a \textit{candidate pool}.
% To achieve this goal, \tool{} first assumes that all solved constraints are related to unsolved constraints, that is, mutate all  valuable positions.
% Then, \tool{} uses a LinUCB model to dynamically generate a distribution for valuable positions based on the fuzzing feedback, which is used to measure the relationship between the unsolved constraints and each position valuable positions, that is, to indirectly measure the relationship between the unsolved constraints and solved constraints.
% Finally, \tool{} constructs byte groups based on the distribution.
% }



==> obsolete/intro-1.1.tex <==



\section{Introduction}

% \zhu{enhance the description of reinforcement learning and shap. 
% \begin{itemize}
%     \item problem of inference-based fuzzing: duplicated inference: a same constraint is inferred in different seeds; constraints may share the same input format (indirect coupling); the longer a seed is, the more time the fuzzer needs to infer related bytes.
%     \item Question: while a position has already discovered new code coverage, can we still focus on it? Why do we repeatedly use the same positions?
%     \item Question: Can the bytes inferred by our \tool{} cover the bytes inferred by others?: Probably no. Some inferred bytes by greyone cannot discover new edges.
%     \item Question: for existing seed-scheduling fuzzers~\cite{Yue2020EcoFuzz}, they intend to focus on seeds that have discovered more new code coverage. The question is, since theoretically, the total coverage discovered by a seed is fixed, how is this solution effective in discovering new code coverage? ==> we need to exchange information between seeds.
% \end{itemize}
% }

% \todo{\begin{itemize}
%     \item with the popularity of fuzzing, many fuzzing solutions can improve the efficiency of discovering code coverage;
%     \item they have proposed many theories or develop algorithms based on intuitive observation to achieve it; EMS: migrate the byte values; we are trying to migrate byte positions
%     \item based on our fuzzing experience, we observe that most edges are discovered by a small portion of input bytes;
%     \item byte schedule is important so that we use SHAP to dig deep into the reasons.
%     \item we use SHAP to demonstrate the observation
%     \item we further dig deep into the reasons of the phenomenon, and observe two reasons: direct and indirect coupling
% \end{itemize}}

Fuzzing is known as a de facto technique to detect software security issues among both academic and industrial practitioners~\cite{zhu2022roadmap}.
In the set of existing fuzzing solutions, coverage-guided greybox fuzzing (CGF) has performed remarkably well in detecting real-world bugs~\cite{ossfuzz, onefuzz, feng2021snipuzz, aflchurn}. 
This method aims to enhance code coverage so that potential bugs are disclosed in the unseen parts of the code. Existing studies have reported many efforts to expand code coverage, including scheduling of computational resources for certain code regions~\cite{aflfast, fairfuzz, Yue2020EcoFuzz, mobfuzz} and resolving path constraints~\cite{angora, qsym, dowser, tfuzz, digfuzz, huang2020pangolin}.
While scheduling computational resources is an implicit way to expand code coverage, resolving path constraints is an explicit way to achieve the same. Since path constraints guard certain code regions, any success in passing path constraints most likely results in new code coverage. However, resolving path constraints is not a trivial task as those constraints may be quite complicated. 




In fuzzing, the problem of resolving path constraints is essentially the byte scheduling, including which bytes to select and how to mutate the selected bytes~\cite{greyone, ems, profuzzer, neuzz, mtfuzz, pata, angora}. 
To analyze the contribution of each byte in discovering code, we conducted fuzzing experiments and performed SHapley Additive exPlanations (SHAP~\cite{shap} analysis to explain the experiment results.
Interestingly, the analysis demonstrates that 1) \textit{\textbf{the mutation of the same byte positions can repeatedly discover new code}}, and 2) \textit{\textbf{the discovery of code largely depends on a (small) portion of byte positions}}.
While such findings might be biased because of the program set selected in SHAP analysis, we dive deep into the reasons for the SHAP results. One reason is \textit{direct coupling} (different constraints related to the same positions of inputs), which refers to the fact that the flip of a path constraint has to consider the results of other path constraints. For example, to pass the condition $if(b == 0x123)$, we may need to figure out all the conditions that the variable $b$ depends on, such as $if(a == 0x22)\{b = 0x12\}$.
The exploration of directly coupled path constraints will lead to deep code in programs (exemplified in Section~\ref{sec:motivation}). Another reason is that different program logic may process the same format of inputs, indicating that different constraints could be related to the same positions of inputs (we call it \textit{indirect coupling}).
The usage of indirect coupling helps fuzzing quickly explore new code if a fuzzer only mutates the corresponding byte positions (exemplified in Section~\ref{sec:motivation}).



The results of SHAP analysis indicate that byte positions contribute differently to the discovery of code regions. Then, why do we treat each position equally during byte schedule? 
According to the findings, the repeated mutation of a (small) portion of byte positions can identify most of the fuzzing-discovered code.
Put differently, the positions that have discovered new code (\ie \textit{valuable positions}) deserve more computational resources. 
However, existing solutions for resolving path constraints neglect the difference between byte positions. 
For instance, some fuzzers establish a relationship between the input bytes that influence the same path constraint~\cite{greyone, ems, angora, vuzzer, steelix} or construct the same data type~\cite{profuzzer, angora}, and mutate the related bytes as a group.
Although such grouping can reduce the search space of passing constraints, they continue to infer other constraint-related bytes, without intentionally repeating the mutation of valuable positions. \chao{<-- Any proofs to support this argument? Bytes are likely to be repeatedly mutated during fuzzing even in a random fuzzing solution, I think.} \zhu{I add `intentionally'.}
Moreover, since their grouped bytes are related to a single path constraint, which neglects the coupled ones, the existing solutions only give a shallow view to the logic of programs.


\begin{figure*}[!t]
\centering
\subfigure[SHAP analysis of \texttt{readelf}]{\includegraphics[width=0.41\linewidth]{images/motivation_readelf_shap.png}} 
\subfigure[SHAP analysis of \texttt{tiff2bw}]{ \includegraphics[width=0.41\linewidth]{images/motivation_tiff2bw_shap.png}}
\subfigure[SHAP analysis of \texttt{nm}]{\includegraphics[width=0.41\linewidth]{images/motivation_nm_shap.png}} 
\subfigure[SHAP analysis of \texttt{objdump}]{\includegraphics[width=0.41\linewidth]{images/motivation_objdump_shap.png}}
\subfigure[SHAP analysis of \texttt{size}]{\includegraphics[width=0.41\linewidth]{images/motivation_size_shap.png}}
\subfigure[SHAP analysis of \texttt{tiffsplit}]{\includegraphics[width=0.41\linewidth]{images/motivation_tiffsplit_shap.png}}
\subfigure[Example of direct and indirect coupling from \texttt{readelf}\label{example_readelf}]{\includegraphics[width=0.85\linewidth]{images/motivation.pdf}}
\caption{The number of edges contributed by each byte position and the reason for the results of SHAP analysis.}\label{shap_and_example}
\end{figure*}


% \todo{in progress}

% In fuzzing, a promising solution for resolving path constraints is to infer the relationships among input bytes and mutate related bytes together in later fuzzing campaigns~\cite{greyone, ems, profuzzer, neuzz, mtfuzz, pata}.
% For instance, some fuzzers establish a relationship between the input bytes that influence the same path constraint~\cite{greyone, ems, angora, vuzzer, steelix} or construct the same data type~\cite{profuzzer, angora}.
% Such inferences can reduce the search space of passing constraints if fuzzing combines related bytes into groups and mutates them on a group basis. 
% For instance, mutating 12 bytes can generate $256^{12}$ different inputs, while mutating 4 bytes at a time (4 bytes a group) only generates $3\times256^{4}$ inputs.
% If a path constraint is related to just one group, the combination of bytes can significantly improve the efficiency of code discovery. 
 


% Essentially, the groups reflect the format of inputs, which further represent the internal logic of programs. However, the existing inference solutions only give a shallow view to the logic of programs. These solutions only infer the relationships between bytes for a single path constraint at a time. Each time, the bytes related to a single path constraint are mutated. This neglects the fact that different path constraints might be heavily coupled. For example, to pass the condition $if(b == 0x123)$, we may need to figure out all the conditions that the variable $b$ depends on, such as $if(a == 0x22)\{b = 0x12\}$. In this case, it is insufficient to only mutate the bytes related to the variable $b$ for the path constraint to be passed. Therefore, in order to fuzz code guarded by complex constraints, the inference algorithm (of related bytes) needs to consider the coupling of path constraints.

% \begin{figure*}[t!]
% % \vspace{-0.6cm} 
% \centering
% \includegraphics[width=0.8\linewidth]{images/motivation.pdf}
% \caption{Example of direct and indirect coupling from \texttt{readelf}.}
% \label{readelf_example}
% \end{figure*}



% In this paper, we propose \tool{}, a lightweight fuzzer that mutates inputs by considering the coupling of path constraints. \tool{} infers and groups the bytes related to the coupled path constraints based on two observations. One observation is what we call \textit{direct coupling}, and it refers to the fact that the flip of a path constraint has to consider the results of other path constraints. The exploration of directly coupled path constraints will lead to deep code in programs (exemplified in Section~\ref{sec:motivation}). Another observation is that different program logics may process the same format of inputs, indicating that different constraints could be related to the same positions of inputs (we call it \textit{indirect coupling}). The usage of indirect coupling helps fuzzing quickly explore new code if a fuzzer only mutates the corresponding byte positions (exemplified in Section~\ref{sec:motivation}).


Based on the SHAP analysis, we propose \tool{}, which builds a \textit{family system} and utilizes \textit{contextual bandit} to 1) share the positions that have discovered new code, and 2) combine the shared positions to mutate members in the same family.
To achieve that, the family system is required to ensure that, for any seed (\ie a retained input) in a family, the shared positions are still related to the seed's corresponding path constraints.
To satisfy the requirement, a family is built if the seeds in the family are obtained just by mutating an original seed without changing its length.
Since the meaning of each position may be changed at the trimming stage, which is performed to reduce the length of the seeds, \tool{} traces the change of positions to maintain the meaning of positions. 
However, the building process of a family can only roughly satisfy the requirement. 
To increase the chances that the selected positions for a seed are related to (unsolved) path constraints, \tool{} uses a contextual multi-armed bandit approach to schedule bytes by considering the context of byte positions.
% to dynamically generate a probability distribution for the selection of positions.  
The context used by \tool{} is the feature vector extracted from execution paths. 
Note that, \tool{} will select positions related to multiple path constraints, so that the directly coupled path constraints can be fuzzed.
% the positions selected by \tool{} may be related to multiple path constraints, so that the directly coupled path constraints can be fuzzed.


We implemented \tool{} based on AFL++~\cite{aflpp}, and evaluated it on two third-party platforms, including 1) UNIFUZZ~\cite{unifuzz}, which contains real-world programs, and 2) MAGMA~\cite{magma}, which provides a series of real-world programs with known bugs.
On UNIFUZZ, we evaluated \tool{}-related fuzzers (\ie \tool{} and \tool{}-Redqueen) and five existing modes of AFL++ on 16 target programs.
The results show that, in terms of code coverage, \tool{}-related fuzzers perform better than other fuzzers after running for 1/3/6/12/24 hours.
For instance, the median ranks of \tool{} and \tool{}-Redqueen are 2.62 and 1.18 after fuzzing 24 hours, respectively.
% \zkp{
% For instance, the median ranks of \tool{} and \tool{}-Redqueen are 2.62 and 1.18 after fuzzing 24 hours, respectively. \tool{} finds 12, 55, 42, 36 and 24 more vulnerabilities than AFL++-MOPT-Redqueen, AFL++-MOPT, AFL++-Exploit, AFL++-Fast and AFL++-Rare, respectively.
% }
Additionally, \tool{}-Redqueen discovers 11 more vulnerabilities than the best mode of AFL++.
On MAGMA, we evaluated \tool{}-related fuzzers and five widely-used mutation-based fuzzers (\ie AFL~\cite{afl}, AFL++-MOPT-Redqueen, AFLFast~\cite{aflfast}, FairFuzz~\cite{fairfuzz} and MOPT~\cite{MOPT}) on 20 programs. \tool{} exposes six more CVEs than the best of the five competing fuzzers.
Additionally, we compare \tool{} to EMS~\cite{ems}, and the results show that \tool{} outperforms EMS in terms of edge discovery. \chao{<-- The comparison with EMS is not very strong. How about bug findings?}
% Our experiments also demonstrate that most of our inferred positions can discover new code, which excludes the first time a position is retained.
% Our experiments also demonstrate that most of our inferred positions can discover new code after the first time the positions have discovered new code.


We summarize our contributions as follows.
\begin{itemize}
    \item We use SHAP to explain the contribution of byte positions in terms of code discovery. The results indicate that the repeated mutation of a (small) portion of positions can improve the efficiency of code discovery.
    % \todo{SHAP experiment: why do we use the valuable positions?}
    \item We ascertain that two derivatives for the SHAP results are the direct and indirect coupling of path constraints. We then propose \tool{}, which uses a family system to share the positions of inputs among seeds in a family. The shared positions can be grouped to resolve directly and indirectly coupled path constraints.
    % We propose a family system to achieve the integration of the pilot stage and havoc stage. Based on semantic consistency, the seeds are divided into multiple families, which allows different seeds in the same family to share the structure-related positions identified by themselves to improve the efficiency of fuzzing.
    \item To further improve the effectiveness of shared positions in discovering new code, \tool{} uses a contextual multi-armed bandit approach to optimize the selection of shared positions.
    \item We implemented \tool{} based on AFL++, and evaluated it on UNIFUZZ and MAGMA platforms. The results indicate that \tool{} outperforms various state-of-the-art fuzzers in terms of edge coverage and bug discovery.
\end{itemize}

\chao{This section has too many details, but does not highlight the key points properly.}



==> obsolete/intro-2.0.tex <==



\section{Introduction}
\zkp{
\begin{itemize}
    \item What is the contribution of each byte to the code discovery?
    \item Quantify the contribution of each byte to the code discovery using shapely value.
    \item Two conclusions are obtained:
    \begin{itemize}
        \item the discovery of code largely depends on a small portion of byte positions.
        \item the mutation of the same byte positions can repeatedly discover new code.
    \end{itemize}
    \item (Findings -> How to improve fuzzing efficiency) If we can identify valuable positions during the fuzzing process, we can allocate more energy to them for mutation, thereby improving the fuzzing efficiency.
    \item Specifically, to discover new code, the input bytes should satisfy branch constraints of different execution paths. These constraints are not independent, i.e., they influence each other along the same execution path or even across different execution paths. Some constraints are nested together (denoted as {\em direct coupling}) in a program path, and thus require mutating a group of input bytes to pass. Some constraints are shared across program paths of different inputs (denoted as {\em indirect coupling}), suggesting that repeatedly mutating certain bytes may still discover new code. 
    \item Using valuable positions to guide fuzzing faces three challenges:
    \begin{itemize}
        \item 
    \end{itemize}
\end{itemize}
}

% \zhu{enhance the description of reinforcement learning and shap. 
% \begin{itemize}
%     \item problem of inference-based fuzzing: duplicated inference: a same constraint is inferred in different seeds; constraints may share the same input format (indirect coupling); the longer a seed is, the more time the fuzzer needs to infer related bytes.
%     \item Question: while a position has already discovered new code coverage, can we still focus on it? Why do we repeatedly use the same positions?
%     \item Question: Can the bytes inferred by our \tool{} cover the bytes inferred by others?: Probably no. Some inferred bytes by greyone cannot discover new edges.
%     \item Question: for existing seed-scheduling fuzzers~\cite{Yue2020EcoFuzz}, they intend to focus on seeds that have discovered more new code coverage. The question is, since theoretically, the total coverage discovered by a seed is fixed, how is this solution effective in discovering new code coverage? ==> we need to exchange information between seeds.
% \end{itemize}
% }

% \todo{\begin{itemize}
%     \item with the popularity of fuzzing, many fuzzing solutions can improve the efficiency of discovering code coverage;
%     \item they have proposed many theories or develop algorithms based on intuitive observation to achieve it; EMS: migrate the byte values; we are trying to migrate byte positions
%     \item based on our fuzzing experience, we observe that most edges are discovered by a small portion of input bytes;
%     \item byte schedule is important so that we use SHAP to dig deep into the reasons.
%     \item we use SHAP to demonstrate the observation
%     \item we further dig deep into the reasons of the phenomenon, and observe two reasons: direct and indirect coupling
% \end{itemize}}
% \zkp{
Mutation-based fuzzing is a widely-used technique to detect software security issues among both academic and industrial practitioners.
In general, to generate new inputs, it includes seed selection (the next seed to be mutated), energy assignment (the number of mutants assigned to the selected seed), and byte mutation (the strategy to select and mutate bytes).
% In general, it selects which seeds to mutate (seed selection), then decides how many mutants to yield (energy allocation), and determines which bytes to mutate and how to mutate (byte mutation).
For byte mutation, many existing solutions have been developed to expand code coverage. We can divide these solutions into three categories.
The first category is utilizing taint analysis to track and mutate the related bytes of path constraints, such as TaintScope~\cite{taintscope}, Dowser~\cite{dowser} and Angora~\cite{angora}.
The second category improves fuzzers by inferring the dependence between bytes and constraints, including GREYONE~\cite{greyone}, ProFuzzer~\cite{profuzzer} and PATA~\cite{pata}.
The third category determines where to mutate seeds via extracting information from history data, such as NEUZZ~\cite{neuzz}, MTFuzz~\cite{mtfuzz} and EMS~\cite{ems}.
Because byte mutation has great impact on fuzzing performance, a core question to answer is \textit{what is the contribution of each byte to the code discovery?} 
However, none of the existing solutions have studied this question.
% Although these fuzzers understand the impact of byte selection and mutation on fuzzing, none of them researches on the question about the contribution of each byte to the code discovery.
\zkp{(What is the significance of studying this problem/Why we study this problem)}

% }
% Fuzzing is known as a de facto technique to detect software security issues among both academic and industrial practitioners~\cite{zhu2022roadmap}.
% \chao{It would be better to focus on mutation-based fuzzing directly, which consists of several critical steps: select which seeds to mutate (seed selection), decide how many mutants to yield (energy allocation), decide which bytes to mutate and how to mutate (byte mutation).}
% In the set of existing fuzzing solutions, coverage-guided greybox fuzzing (CGF) has performed remarkably well in detecting real-world bugs~\cite{ossfuzz, onefuzz, feng2021snipuzz, aflchurn}. 
% This method aims to enhance code coverage so that potential bugs are disclosed in the unseen parts of the code. Existing studies have reported many efforts to expand code coverage, including scheduling of computational resources for certain code regions~\cite{aflfast, fairfuzz, Yue2020EcoFuzz, mobfuzz} and resolving path constraints~\cite{angora, qsym, dowser, tfuzz, digfuzz, huang2020pangolin}.
% However, only a few solutions have studied the selection and mutation of input bytes~\cite{greyone, pata, ems, profuzzer, neuzz, mtfuzz}. \chao{It would be better to classify these closely-related solutions into several categories. BTW, put the names of these solutions here rather than just citation links.}
% Those solutions focus on grouping bytes that influence the same path constraints or constructing the same data type. Yet, none of them studies the contribution of bytes to the code discovery.
% \chao{These two sentences should be rephrased. The first sentence fails to cover all closely-related solutions, and the second one fails to express why it is necessary. Maybe we can say that, selecting which bytes to mutate would have great impact on fuzzing performance, a core question to answer is that what is the contribution of each byte to the code discovery, and none of existing solutions have studied this question.}
% To the best of our knowledge, only EMS~\cite{ems} studies the optimization of selecting bytes.
% While scheduling computational resources is an implicit way to expand code coverage, resolving path constraints is an explicit way to achieve the same. Since path constraints guard certain code regions, any success in passing path constraints most likely results in new code coverage. However, resolving path constraints is not a trivial task as those constraints may be quite complicated. 


% In fuzzing, the problem of resolving path constraints is essentially the byte scheduling, including which bytes to select and how to mutate the selected bytes~\cite{greyone, ems, profuzzer, neuzz, mtfuzz, pata, angora}. 
\zkp{(Explain why shapely value is used: ) To study the contribution of each byte, we model the selection and mutation process of bytes as a teamwork process.
In cooperative game theory, shapely value is used to measure the contribution made by each member of a team.
Therefore, we can also use shapely value to quantify the contribution of each byte to new edge discovery.
}
To analyze the contribution of each byte in discovering code, we conducted a group of fuzzing experiments and performed SHapley Additive exPlanations (SHAP)~\cite{shap} analysis to study the experiment results.
Interestingly, the analysis demonstrates that (1) \textit{the discovery of code largely depends on a small portion of byte positions}, and (2) \textit{the mutation of the same byte positions can repeatedly discover new code}. \zkp{More details of the experiments are introduced in Section~\ref{sec:motivation}.}

\zkp{This section keeps explaining the source of findings, but never explains the relationship between findings and improving the efficiency of fuzzing.}
Though such findings might be biased because the number of programs and seed inputs used in the experiments are limited, we notice that this matches with the nature of program logic.
Specifically, to discover new code, the input bytes should satisfy branch constraints of different execution paths. These constraints are not independent, i.e., they influence each other along the same execution path or even across different execution paths. Some constraints are nested together (denoted as {\em direct coupling}) in a program path, and thus require mutating a group of input bytes to pass. Some constraints are shared across program paths of different inputs (denoted as {\em indirect coupling}), suggesting that repeatedly mutating certain bytes may still discover new code.
% This nature indicates that the byte positions, which resolve one path constraint, have a high chance to be able to resolve another constraint, in or not in the same execution path.
% While such findings might be biased because of the program set selected in SHAP analysis, we dive deep into the reasons for the SHAP results. 
% One reason is \textit{direct coupling} (different constraints related to the same positions of inputs), which refers to the fact that the flip of a path constraint has to consider the results of other path constraints. For example, to pass the condition $if(b == 0x123)$, we may need to figure out all the conditions that the variable $b$ depends on, such as $if(a == 0x22)\{b = 0x12\}$.
% The exploration of directly coupled path constraints will lead to deep code in programs (exemplified in Section~\ref{sec:motivation}). Another reason is that different program logic may process the same format of inputs, indicating that different constraints could be related to the same positions of inputs (we call it \textit{indirect coupling}).
% The usage of indirect coupling helps fuzzing quickly explore new code if a fuzzer only mutates the corresponding byte positions (exemplified in Section~\ref{sec:motivation}).

\zkp{(Findings -> How to improve fuzzing efficiency) }



The results of SHAP analysis indicate that, byte positions contribute differently to the discovery of code regions,
% Then, why do we treat each position equally during byte schedule? 
% According to the findings, 
and the repeated mutation of a (small) portion of byte positions can identify most of the discovered code during fuzzing.
\zkp{
(Explain why these findings can improve the fuzzing efficiency)
}
Based on these findings, we can therefore optimize the fuzzing process by addressing the following two questions. 
The first one is how to identify the \textit{valuable positions}, \ie the byte positions that contribute mostly to discovering code.
The second one is how to efficiently utilize these valuable positions across different seeds.
% , so that we can save time identifying valuable positions for different seeds.

% Put differently, the positions that have discovered new code (\ie \textit{valuable positions}) deserve more computational resources. 
% However, existing solutions for resolving path constraints neglect the difference between byte positions. 
% For instance, some fuzzers establish a relationship between the input bytes that influence the same path constraint~\cite{greyone, ems, angora, vuzzer, steelix} or construct the same data type~\cite{profuzzer, angora}, and mutate the related bytes as a group.
% Although such grouping can reduce the search space of passing constraints, they continue to infer other constraint-related bytes, without intentionally repeating the mutation of valuable positions. \chao{<-- Any proofs to support this argument? Bytes are likely to be repeatedly mutated during fuzzing even in a random fuzzing solution, I think.} \zhu{I add `intentionally'.}
% Moreover, since their grouped bytes are related to a single path constraint, which neglects the coupled ones, the existing solutions only give a shallow view to the logic of programs.


% \todo{in progress}

% In fuzzing, a promising solution for resolving path constraints is to infer the relationships among input bytes and mutate related bytes together in later fuzzing campaigns~\cite{greyone, ems, profuzzer, neuzz, mtfuzz, pata}.
% For instance, some fuzzers establish a relationship between the input bytes that influence the same path constraint~\cite{greyone, ems, angora, vuzzer, steelix} or construct the same data type~\cite{profuzzer, angora}.
% Such inferences can reduce the search space of passing constraints if fuzzing combines related bytes into groups and mutates them on a group basis. 
% For instance, mutating 12 bytes can generate $256^{12}$ different inputs, while mutating 4 bytes at a time (4 bytes a group) only generates $3\times256^{4}$ inputs.
% If a path constraint is related to just one group, the combination of bytes can significantly improve the efficiency of code discovery. 
 


% Essentially, the groups reflect the format of inputs, which further represent the internal logic of programs. However, the existing inference solutions only give a shallow view to the logic of programs. These solutions only infer the relationships between bytes for a single path constraint at a time. Each time, the bytes related to a single path constraint are mutated. This neglects the fact that different path constraints might be heavily coupled. For example, to pass the condition $if(b == 0x123)$, we may need to figure out all the conditions that the variable $b$ depends on, such as $if(a == 0x22)\{b = 0x12\}$. In this case, it is insufficient to only mutate the bytes related to the variable $b$ for the path constraint to be passed. Therefore, in order to fuzz code guarded by complex constraints, the inference algorithm (of related bytes) needs to consider the coupling of path constraints.

% \begin{figure*}[t!]
% % \vspace{-0.6cm} 
% \centering
% \includegraphics[width=0.8\linewidth]{images/motivation.pdf}
% \caption{Example of direct and indirect coupling from \texttt{readelf}.}
% \label{readelf_example}
% \end{figure*}



% In this paper, we propose \tool{}, a lightweight fuzzer that mutates inputs by considering the coupling of path constraints. \tool{} infers and groups the bytes related to the coupled path constraints based on two observations. One observation is what we call \textit{direct coupling}, and it refers to the fact that the flip of a path constraint has to consider the results of other path constraints. The exploration of directly coupled path constraints will lead to deep code in programs (exemplified in Section~\ref{sec:motivation}). Another observation is that different program logics may process the same format of inputs, indicating that different constraints could be related to the same positions of inputs (we call it \textit{indirect coupling}). The usage of indirect coupling helps fuzzing quickly explore new code if a fuzzer only mutates the corresponding byte positions (exemplified in Section~\ref{sec:motivation}).


In this paper, we propose \tool{} to address the two problems and guide fuzzers to select valuable bytes to mutate.
% \chao{This paragraph does not address the two problems accordingly.}\zhu{revised.}
\tool{} first assumes that the byte positions that have discovered new code are potential valuable positions.
To effectively utilize valuable positions across seeds, it then builds a \textit{family system} to share these.
The purpose of the family system is to ensure that the shared positions are related to the corresponding path constraints of any family member.  
Finally, to optimize the use of potential valuable positions, \tool{} utilizes a \textit{contextual multi-armed bandit} (CMAB) based on the family system.
The CMAB, which considers the context of valuable positions, optimizes byte mutation by predicting and seeking out the best rewards, \ie code discovery.
The CMAB tries some of the potential valuable positions, and decides to assign more energy to certain positions based on the reward of those trials.
As a result, \tool{} has a high chance to select and combine the positions with the highest contribution for byte mutation.

% It then utilizes a \textit{contextual multi-armed bandit} (CMAB) approach to further infer the most contributing byte positions.
% The CMAB approach is designed based on a \textit{family system}, which improves the effectiveness of utilizing valuable positions across seeds.
% Then, it builds a \textit{family system} and utilizes a \textit{contextual multi-armed bandit} (CMAB) approach to 1) share the valuable positions among seeds, and 2) optimize the mutation of the shared positions.



% Since the byte positions that have discovered new code already contribute to the code discovery, we assume that they are the valuable positions.
% To efficiently use valuable positions, \tool{} builds a \textit{family system} and utilizes a \textit{contextual multi-armed bandit} (CMAB) approach to 1) share the valuable positions among seeds, and 2) optimize the mutation of the shared positions.
% To achieve that, the family system is required to ensure that, for any seed in a family, the shared positions are still related to the seed's corresponding path constraints.
% To satisfy the requirement, a family is built if the seeds in the family are obtained just by mutating an original seed without changing its length.
% Since the meaning of each position may be changed at the trimming stage, which is performed to reduce the length of the seeds, \tool{} traces the change of positions to maintain the meaning of positions. 
% However, the building process of a family can only roughly satisfy the requirement. 
% \chao{It's not clear why CMAB can solve this issue.}
% To increase the chances that the selected positions for a seed are related to (unsolved) path constraints, \tool{} uses a contextual multi-armed bandit (CMAB) approach to schedule bytes by considering the context of them.
% % to dynamically generate a probability distribution for the selection of positions.  
% The context used by \tool{} is the feature vector extracted from execution paths. 
% Note that, \tool{} will select positions related to multiple path constraints, so that the directly coupled path constraints can be fuzzed.
% % the positions selected by \tool{} may be related to multiple path constraints, so that the directly coupled path constraints can be fuzzed.


We implement \tool{} based on AFL++~\cite{aflpp}, and evaluate it on two third-party platforms, including 1) UNIFUZZ~\cite{unifuzz}, which contains real-world programs, and 2) MAGMA~\cite{magma}, which provides a series of real-world programs with known bugs.
On UNIFUZZ, we evaluate \tool{}-related fuzzers (\ie \tool{} and \tool{}-Redqueen) and five existing modes of AFL++ on 16 target programs.
The results show that, in terms of code coverage, \tool{}-related fuzzers perform better than other fuzzers after running for 1/3/6/12/24 hours.
For instance, the median ranks of \tool{} and \tool{}-Redqueen are 2.62 and 1.18 after fuzzing 24 hours, respectively.
% \zkp{
% For instance, the median ranks of \tool{} and \tool{}-Redqueen are 2.62 and 1.18 after fuzzing 24 hours, respectively. \tool{} finds 12, 55, 42, 36 and 24 more vulnerabilities than AFL++-MOPT-Redqueen, AFL++-MOPT, AFL++-Exploit, AFL++-Fast and AFL++-Rare, respectively.
% }
Additionally, \tool{} discovers 20 more bugs than the best mode of AFL++.
On MAGMA, we evaluate \tool{}-related fuzzers and five widely-used mutation-based fuzzers (\ie AFL~\cite{afl}, AFL++-MOPT-Redqueen, AFLFast~\cite{aflfast}, FairFuzz~\cite{fairfuzz} and MOPT~\cite{MOPT}) on 20 programs. \tool{} exposes six more CVEs than the best of the five competing fuzzers.
Additionally, \tool{} also outperforms EMS~\cite{ems} in terms of both edge and bug discovery. 
% \chao{<-- The comparison with EMS is not very strong. How about bug findings?} \zkp{The EMS bug findings are very poor. I'll check to see if there is a problem somewhere and release the results later.}
% Our experiments also demonstrate that most of our inferred positions can discover new code, which excludes the first time a position is retained.
% Our experiments also demonstrate that most of our inferred positions can discover new code after the first time the positions have discovered new code.


We summarize our contributions as follows.
\begin{itemize}
    \item We use SHAP to explain the contribution of byte positions in terms of code discovery. The results indicate that the repeated mutation of a small portion of positions can improve the efficiency of code discovery. We ascertain that two derivatives for the SHAP results are the direct and indirect coupling of path constraints. 
    % \todo{SHAP experiment: why do we use the valuable positions?}
    \item We propose \tool{}, which uses a family system to share the positions of inputs among seeds in a family. The shared positions can be grouped to resolve directly and indirectly coupled path constraints.
    % We propose a family system to achieve the integration of the pilot stage and havoc stage. Based on semantic consistency, the seeds are divided into multiple families, which allows different seeds in the same family to share the structure-related positions identified by themselves to improve the efficiency of fuzzing.
    \item We present a contextual multi-armed bandit approach to optimize the selection of shared positions, to further improve the effectiveness of shared positions in discovering new code.
    \item We implemented \tool{} based on AFL++, and evaluated it on UNIFUZZ and MAGMA platforms. The results indicate that \tool{} outperforms various state-of-the-art fuzzers in terms of edge coverage and bug discovery.
\end{itemize}

% \chao{This section has too many details, but does not highlight the key points properly.}\zhu{have revised the intro.}


% \begin{figure*}[!t]
% \centering
% \subfigure[SHAP analysis of \texttt{readelf}]{\includegraphics[width=0.28\linewidth]{images/motivation_readelf_shap.png}} 
% \subfigure[SHAP analysis of \texttt{tiff2bw}]{ \includegraphics[width=0.28\linewidth]{images/motivation_tiff2bw_shap.png}}
% \subfigure[SHAP analysis of \texttt{nm}]{\includegraphics[width=0.28\linewidth]{images/motivation_nm_shap.png}} 
% \subfigure[SHAP analysis of \texttt{objdump}]{\includegraphics[width=0.28\linewidth]{images/motivation_objdump_shap.png}}
% \subfigure[SHAP analysis of \texttt{size}]{\includegraphics[width=0.28\linewidth]{images/motivation_size_shap.png}}
% \subfigure[SHAP analysis of \texttt{tiffsplit}]{\includegraphics[width=0.28\linewidth]{images/motivation_tiffsplit_shap.png}}
% \subfigure[Example of direct and indirect coupling from \texttt{readelf}\label{example_readelf}]{\includegraphics[width=0.85\linewidth]{images/motivation.pdf}}
% \caption{The number of edges contributed by each byte position and the reason for the results of SHAP analysis.}\label{shap_and_example}
% \end{figure*}


\begin{figure*}
    \centering
    \begin{minipage}{\textwidth}
    \centering
    \includegraphics[width=0.85\linewidth]{images/shap_legend.png}
    \end{minipage}
    \begin{minipage}{\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/shap_result.jpg}
    \caption{The number of edges contributed by each byte position (SHAP analysis).}
    \label{shap_res}
    \end{minipage}
    % \begin{minipage}{\textwidth}
    % \centering
    % \includegraphics[width=0.85\linewidth]{images/motivation.pdf}
    % \caption{The number of edges contributed by each byte position and the reason for the results of SHAP analysis.}
    % \label{example_readelf}
    % \end{minipage}
\end{figure*}


% \begin{figure*}[t!]
% \centering
% \includegraphics[width=0.85\linewidth]{images/shap_legend.png}
% \label{shap_legend}
% \end{figure*}

% \begin{figure*}[t!]
% \vspace{-0.4cm} 
% \setlength{\abovecaptionskip}{0.cm}
% \centering
% \includegraphics[width=\linewidth]{images/shap_result.jpg}
% \caption{SHAP analysis of \texttt{nm}, \texttt{objdump}, \texttt{readelf}, \texttt{size}, \texttt{tiff2bw} and \texttt{tiffsplit}}
% \label{shap_res}
% \end{figure*}


\begin{figure*}[t!]
\centering
\includegraphics[width=0.85\linewidth]{images/motivation.pdf}
\caption{The reason for the results of SHAP analysis.}
\label{example_readelf}
\end{figure*}



==> obsolete/intro-2.1.tex <==



\section{Introduction}
% \zkp{
% \begin{itemize}
%     \item What is the contribution of each byte to the code discovery?
%     \item Quantify the contribution of each byte to the code discovery using shapely value.
%     \item Two conclusions are obtained:
%     \begin{itemize}
%         \item the discovery of code largely depends on a small portion of byte positions.
%         \item the mutation of the same byte positions can repeatedly discover new code.
%     \end{itemize}
%     \item (Findings -> How to improve fuzzing efficiency) If we can identify valuable positions during the fuzzing process, we can allocate more energy to them for mutation, thereby improving the fuzzing efficiency.
%     \item Specifically, to discover new code, the input bytes should satisfy branch constraints of different execution paths. These constraints are not independent, i.e., they influence each other along the same execution path or even across different execution paths. Some constraints are nested together (denoted as {\em direct coupling}) in a program path, and thus require mutating a group of input bytes to pass. Some constraints are shared across program paths of different inputs (denoted as {\em indirect coupling}), suggesting that repeatedly mutating certain bytes may still discover new code. 
%     \item Using valuable positions to guide fuzzing faces three challenges:
%     \begin{itemize}
%         \item 
%     \end{itemize}
% \end{itemize}
% }

% \zhu{enhance the description of reinforcement learning and shap. 
% \begin{itemize}
%     \item problem of inference-based fuzzing: duplicated inference: a same constraint is inferred in different seeds; constraints may share the same input format (indirect coupling); the longer a seed is, the more time the fuzzer needs to infer related bytes.
%     \item Question: while a position has already discovered new code coverage, can we still focus on it? Why do we repeatedly use the same positions?
%     \item Question: Can the bytes inferred by our \tool{} cover the bytes inferred by others?: Probably no. Some inferred bytes by greyone cannot discover new edges.
%     \item Question: for existing seed-scheduling fuzzers~\cite{Yue2020EcoFuzz}, they intend to focus on seeds that have discovered more new code coverage. The question is, since theoretically, the total coverage discovered by a seed is fixed, how is this solution effective in discovering new code coverage? ==> we need to exchange information between seeds.
% \end{itemize}
% }

% \todo{\begin{itemize}
%     \item with the popularity of fuzzing, many fuzzing solutions can improve the efficiency of discovering code coverage;
%     \item they have proposed many theories or develop algorithms based on intuitive observation to achieve it; EMS: migrate the byte values; we are trying to migrate byte positions
%     \item based on our fuzzing experience, we observe that most edges are discovered by a small portion of input bytes;
%     \item byte schedule is important so that we use SHAP to dig deep into the reasons.
%     \item we use SHAP to demonstrate the observation
%     \item we further dig deep into the reasons of the phenomenon, and observe two reasons: direct and indirect coupling
% \end{itemize}}
% \zkp{
Mutation-based fuzzing is a widely-used technique to detect software security issues among both academic and industrial practitioners.
In general, to generate new inputs, it includes seed selection (the next seed to be mutated), energy assignment (the number of mutants assigned to the selected seed), and byte mutation (the strategy to select and mutate bytes).
% In general, it selects which seeds to mutate (seed selection), then decides how many mutants to yield (energy allocation), and determines which bytes to mutate and how to mutate (byte mutation).
For byte mutation, many existing solutions have been developed to expand code coverage. We can divide these solutions into three categories.
The first category is utilizing taint analysis to track and mutate the related bytes of path constraints, such as TaintScope~\cite{taintscope}, Dowser~\cite{dowser} and Angora~\cite{angora}.
The second category improves fuzzers by inferring the dependence between bytes and constraints, including GREYONE~\cite{greyone}, ProFuzzer~\cite{profuzzer} and PATA~\cite{pata}.
The third category determines where to mutate seeds via extracting information from history data, such as NEUZZ~\cite{neuzz}, MTFuzz~\cite{mtfuzz} and EMS~\cite{ems}.
Because byte mutation has great impact on fuzzing performance, a core question to answer is \textit{what is the contribution of each byte to the code discovery?} 
However, none of the existing solutions have studied this question.
% Although these fuzzers understand the impact of byte selection and mutation on fuzzing, none of them researches on the question about the contribution of each byte to the code discovery.
% \zkp{(What is the significance of studying this problem/Why we study this problem)}

% }
% Fuzzing is known as a de facto technique to detect software security issues among both academic and industrial practitioners~\cite{zhu2022roadmap}.
% \chao{It would be better to focus on mutation-based fuzzing directly, which consists of several critical steps: select which seeds to mutate (seed selection), decide how many mutants to yield (energy allocation), decide which bytes to mutate and how to mutate (byte mutation).}
% In the set of existing fuzzing solutions, coverage-guided greybox fuzzing (CGF) has performed remarkably well in detecting real-world bugs~\cite{ossfuzz, onefuzz, feng2021snipuzz, aflchurn}. 
% This method aims to enhance code coverage so that potential bugs are disclosed in the unseen parts of the code. Existing studies have reported many efforts to expand code coverage, including scheduling of computational resources for certain code regions~\cite{aflfast, fairfuzz, Yue2020EcoFuzz, mobfuzz} and resolving path constraints~\cite{angora, qsym, dowser, tfuzz, digfuzz, huang2020pangolin}.
% However, only a few solutions have studied the selection and mutation of input bytes~\cite{greyone, pata, ems, profuzzer, neuzz, mtfuzz}. \chao{It would be better to classify these closely-related solutions into several categories. BTW, put the names of these solutions here rather than just citation links.}
% Those solutions focus on grouping bytes that influence the same path constraints or constructing the same data type. Yet, none of them studies the contribution of bytes to the code discovery.
% \chao{These two sentences should be rephrased. The first sentence fails to cover all closely-related solutions, and the second one fails to express why it is necessary. Maybe we can say that, selecting which bytes to mutate would have great impact on fuzzing performance, a core question to answer is that what is the contribution of each byte to the code discovery, and none of existing solutions have studied this question.}
% To the best of our knowledge, only EMS~\cite{ems} studies the optimization of selecting bytes.
% While scheduling computational resources is an implicit way to expand code coverage, resolving path constraints is an explicit way to achieve the same. Since path constraints guard certain code regions, any success in passing path constraints most likely results in new code coverage. However, resolving path constraints is not a trivial task as those constraints may be quite complicated. 


% In fuzzing, the problem of resolving path constraints is essentially the byte scheduling, including which bytes to select and how to mutate the selected bytes~\cite{greyone, ems, profuzzer, neuzz, mtfuzz, pata, angora}. 
\zkp{(Explain why shapely value is used: ) 
In cooperative game theory, shapely value is used to measure the contribution made by each member of a team.
To study the contribution of each byte, we model byte mutation as a teamwork process.
Therefore, we can also use shapely value to quantify the contribution of each byte to new edge discovery.
}
We conducted a group of fuzzing experiments and performed shapely value~\cite{Shapley} analysis to study the experiment results.
Interestingly, the analysis demonstrates that (1) \textit{the discovery of code largely depends on a small portion of byte positions}, and (2) \textit{the mutation of the same byte positions can repeatedly discover new code}. \zkp{More details of the experiments are introduced in Section~\ref{sec:motivation}.}

% \zkp{This section keeps explaining the source of findings, but never explains the relationship between findings and improving the efficiency of fuzzing.}
% Though such findings might be biased because the number of programs and seed inputs used in the experiments are limited, we notice that this matches with the nature of program logic.
We notice that such findings match with the nature of program logic.
Specifically, to discover new code, the input bytes should satisfy branch constraints of different execution paths. These constraints are not independent, i.e., they influence each other along the same execution path or even across different execution paths. Some constraints are nested together (denoted as {\em direct coupling}) in a program path, and thus require mutating a group of input bytes to pass. Some constraints are shared across program paths of different inputs (denoted as {\em indirect coupling}), suggesting that repeatedly mutating certain bytes may still discover new code.
% This nature indicates that the byte positions, which resolve one path constraint, have a high chance to be able to resolve another constraint, in or not in the same execution path.
% While such findings might be biased because of the program set selected in SHAP analysis, we dive deep into the reasons for the SHAP results. 
% One reason is \textit{direct coupling} (different constraints related to the same positions of inputs), which refers to the fact that the flip of a path constraint has to consider the results of other path constraints. For example, to pass the condition $if(b == 0x123)$, we may need to figure out all the conditions that the variable $b$ depends on, such as $if(a == 0x22)\{b = 0x12\}$.
% The exploration of directly coupled path constraints will lead to deep code in programs (exemplified in Section~\ref{sec:motivation}). Another reason is that different program logic may process the same format of inputs, indicating that different constraints could be related to the same positions of inputs (we call it \textit{indirect coupling}).
% The usage of indirect coupling helps fuzzing quickly explore new code if a fuzzer only mutates the corresponding byte positions (exemplified in Section~\ref{sec:motivation}).

% 


% \zkp{(Findings -> How to improve fuzzing efficiency) }
The results of SHAP analysis indicate that, byte positions contribute differently to the discovery of code regions,
% Then, why do we treat each position equally during byte schedule? 
% According to the findings, 
and the repeated mutation of a (small) portion of byte positions can identify most of the discovered code during fuzzing.
% \zkp{
% (Explain why these findings can improve the fuzzing efficiency)
% }
\zkp{
Based on these findings, we can therefore optimize the fuzzing process by identifying valuable positions(\ie the byte positions that contribute to discovering code) during fuzzing and focusing on mutations for them. However, guiding fuzzing with valuable positions encounters following three problems.

First, due to the complicated calculation process of shapely value, it is time-consuming to directly quantify the contribution of each byte to code discovery during the fuzzing process. Therefore, \textit{Problem I} is: \textit{How to perform lightweight inference for valuable positions during fuzzing?}

Second, the inference process of the valuable positions of each seed is independent.
However, due to the similarity between some seeds, they may have the same valuable positions, which can be used to improve the inference efficiency.
Thus, \textit{Problem II} is: \textit{How to efficiently utilize these valuable positions across different seeds, so that we can save time identifying valuable positions for different seeds.}

Third, after getting the valuable positions, we need to mutate them to find more new edges. 
However, valuable positions will become stale
after a period of testing, which indicates we need to continuously increase the number of valuable positions during fuzzing.
Thus, \textit{Problem III} is: \textit{How to increase the number of valuable positions while using valuable positions to guide the mutation direction?}


}




% Based on these findings, we can therefore optimize the fuzzing process by addressing the following three questions. 
% The first one is how to identify the \textit{valuable positions}, \ie the byte positions that contribute to discovering code.
% The second one is how to efficiently utilize these valuable positions across different seeds, so that we can save time identifying valuable positions for different seeds.
% The third one is how to guide the mutation based on valuable positions.
% , so that we can save time identifying valuable positions for different seeds.

% Put differently, the positions that have discovered new code (\ie \textit{valuable positions}) deserve more computational resources. 
% However, existing solutions for resolving path constraints neglect the difference between byte positions. 
% For instance, some fuzzers establish a relationship between the input bytes that influence the same path constraint~\cite{greyone, ems, angora, vuzzer, steelix} or construct the same data type~\cite{profuzzer, angora}, and mutate the related bytes as a group.
% Although such grouping can reduce the search space of passing constraints, they continue to infer other constraint-related bytes, without intentionally repeating the mutation of valuable positions. \chao{<-- Any proofs to support this argument? Bytes are likely to be repeatedly mutated during fuzzing even in a random fuzzing solution, I think.} \zhu{I add `intentionally'.}
% Moreover, since their grouped bytes are related to a single path constraint, which neglects the coupled ones, the existing solutions only give a shallow view to the logic of programs.


% \todo{in progress}

% In fuzzing, a promising solution for resolving path constraints is to infer the relationships among input bytes and mutate related bytes together in later fuzzing campaigns~\cite{greyone, ems, profuzzer, neuzz, mtfuzz, pata}.
% For instance, some fuzzers establish a relationship between the input bytes that influence the same path constraint~\cite{greyone, ems, angora, vuzzer, steelix} or construct the same data type~\cite{profuzzer, angora}.
% Such inferences can reduce the search space of passing constraints if fuzzing combines related bytes into groups and mutates them on a group basis. 
% For instance, mutating 12 bytes can generate $256^{12}$ different inputs, while mutating 4 bytes at a time (4 bytes a group) only generates $3\times256^{4}$ inputs.
% If a path constraint is related to just one group, the combination of bytes can significantly improve the efficiency of code discovery. 
 


% Essentially, the groups reflect the format of inputs, which further represent the internal logic of programs. However, the existing inference solutions only give a shallow view to the logic of programs. These solutions only infer the relationships between bytes for a single path constraint at a time. Each time, the bytes related to a single path constraint are mutated. This neglects the fact that different path constraints might be heavily coupled. For example, to pass the condition $if(b == 0x123)$, we may need to figure out all the conditions that the variable $b$ depends on, such as $if(a == 0x22)\{b = 0x12\}$. In this case, it is insufficient to only mutate the bytes related to the variable $b$ for the path constraint to be passed. Therefore, in order to fuzz code guarded by complex constraints, the inference algorithm (of related bytes) needs to consider the coupling of path constraints.

% \begin{figure*}[t!]
% % \vspace{-0.6cm} 
% \centering
% \includegraphics[width=0.8\linewidth]{images/motivation.pdf}
% \caption{Example of direct and indirect coupling from \texttt{readelf}.}
% \label{readelf_example}
% \end{figure*}



% In this paper, we propose \tool{}, a lightweight fuzzer that mutates inputs by considering the coupling of path constraints. \tool{} infers and groups the bytes related to the coupled path constraints based on two observations. One observation is what we call \textit{direct coupling}, and it refers to the fact that the flip of a path constraint has to consider the results of other path constraints. The exploration of directly coupled path constraints will lead to deep code in programs (exemplified in Section~\ref{sec:motivation}). Another observation is that different program logics may process the same format of inputs, indicating that different constraints could be related to the same positions of inputs (we call it \textit{indirect coupling}). The usage of indirect coupling helps fuzzing quickly explore new code if a fuzzer only mutates the corresponding byte positions (exemplified in Section~\ref{sec:motivation}).

\zkp{
In this paper, we propose \tool{} to address the aforementioned three problems.
To solve the time-consuming problem of shapely value calculation in \textit{Problem I}, we propose a lightweight valuable position inference algorithm, which integrates the calculation process of shapely value into the fuzzing process. Specifically, we record the mutated positions sequence of each mutation. If the mutated input discovers new code coverage, we compute the marginal contribution of each position within the mutated positions sequence. Then for each position, we accumulate its marginal contribution on all mutations to get the \textit{edge contribution}. If the edge contribution of a position is greater than 0, we consider it to be a valuable position. 
% Note that we only deal with mutated input without length mutators because length mutators can cause most positions to change.

To share valuable positions across different seeds in \textit{Problem II}, we propose a family system. We cluster seeds into families based on inheritance relationship and seed length. 
% Each family maintains its own shared pool, which records the valuable positions that all seeds in the family have discovered. 
In each family, we will maintain a shared pool for sharing the valuable positions found by all seeds in the family.
Each seed can either add the valuable positions it discovers to the shared pool or obtain its unknown valuable positions from the shared pool.

To solve the update problem of valuable positions in \textit{Problem III}, We design two modes in the mutation stage: family-based mutation and havoc mutation.
Among them, family-based mutation mutates valuable positions to discover more new code, while havoc mutation mutates all positions to infer more valuable positions.
We use a simple yet effective indicator to quantify the efficiency of each mutation mode and select the best mode
in the next mutation round.

}



% In this paper, we propose \tool{} to address the two problems and guide fuzzers to select valuable bytes to mutate.
% % \chao{This paragraph does not address the two problems accordingly.}\zhu{revised.}
% \tool{} first assumes that the byte positions that have discovered new code are potential valuable positions.
% To effectively utilize valuable positions across seeds, it then builds a \textit{family system} to share these.
% The purpose of the family system is to ensure that the shared positions are related to the corresponding path constraints of any family member.  
% Finally, to optimize the use of potential valuable positions, \tool{} utilizes a \textit{contextual multi-armed bandit} (CMAB) based on the family system.
% The CMAB, which considers the context of valuable positions, optimizes byte mutation by predicting and seeking out the best rewards, \ie code discovery.
% The CMAB tries some of the potential valuable positions, and decides to assign more energy to certain positions based on the reward of those trials.
% As a result, \tool{} has a high chance to select and combine the positions with the highest contribution for byte mutation.

% It then utilizes a \textit{contextual multi-armed bandit} (CMAB) approach to further infer the most contributing byte positions.
% The CMAB approach is designed based on a \textit{family system}, which improves the effectiveness of utilizing valuable positions across seeds.
% Then, it builds a \textit{family system} and utilizes a \textit{contextual multi-armed bandit} (CMAB) approach to 1) share the valuable positions among seeds, and 2) optimize the mutation of the shared positions.



% Since the byte positions that have discovered new code already contribute to the code discovery, we assume that they are the valuable positions.
% To efficiently use valuable positions, \tool{} builds a \textit{family system} and utilizes a \textit{contextual multi-armed bandit} (CMAB) approach to 1) share the valuable positions among seeds, and 2) optimize the mutation of the shared positions.
% To achieve that, the family system is required to ensure that, for any seed in a family, the shared positions are still related to the seed's corresponding path constraints.
% To satisfy the requirement, a family is built if the seeds in the family are obtained just by mutating an original seed without changing its length.
% Since the meaning of each position may be changed at the trimming stage, which is performed to reduce the length of the seeds, \tool{} traces the change of positions to maintain the meaning of positions. 
% However, the building process of a family can only roughly satisfy the requirement. 
% \chao{It's not clear why CMAB can solve this issue.}
% To increase the chances that the selected positions for a seed are related to (unsolved) path constraints, \tool{} uses a contextual multi-armed bandit (CMAB) approach to schedule bytes by considering the context of them.
% % to dynamically generate a probability distribution for the selection of positions.  
% The context used by \tool{} is the feature vector extracted from execution paths. 
% Note that, \tool{} will select positions related to multiple path constraints, so that the directly coupled path constraints can be fuzzed.
% % the positions selected by \tool{} may be related to multiple path constraints, so that the directly coupled path constraints can be fuzzed.


We implement \tool{} based on AFL++~\cite{aflpp}, and evaluate it on two third-party platforms, including 1) UNIFUZZ~\cite{unifuzz}, which contains real-world programs, and 2) MAGMA~\cite{magma}, which provides a series of real-world programs with known bugs.
On UNIFUZZ, we evaluate \tool{}-related fuzzers (\ie \tool{} and \tool{}-Redqueen) and four existing modes of AFL++ on 16 target programs.
The results show that, in terms of code coverage, \tool{}-related fuzzers perform better than other fuzzers after running for 1/3/6/12/24 hours.
For instance, the median ranks of \tool{} and \tool{}-Redqueen are 2.62 and 1.18 after fuzzing 24 hours, respectively.
% \zkp{
% For instance, the median ranks of \tool{} and \tool{}-Redqueen are 2.62 and 1.18 after fuzzing 24 hours, respectively. \tool{} finds 12, 55, 42, 36 and 24 more vulnerabilities than AFL++-MOPT-Redqueen, AFL++-MOPT, AFL++-Exploit, AFL++-Fast and AFL++-Rare, respectively.
% }
Additionally, \tool{} discovers 20 more bugs than the best mode of AFL++.
On MAGMA, we evaluate \tool{}-related fuzzers and five widely-used mutation-based fuzzers (\ie AFL~\cite{afl}, AFL++-MOPT-Redqueen, AFLFast~\cite{aflfast}, FairFuzz~\cite{fairfuzz} and MOPT~\cite{MOPT}) on 20 programs. \tool{} exposes six more CVEs than the best of the five competing fuzzers.
Additionally, \tool{} also outperforms EMS~\cite{ems} in terms of both edge and bug discovery. 
% \chao{<-- The comparison with EMS is not very strong. How about bug findings?} \zkp{The EMS bug findings are very poor. I'll check to see if there is a problem somewhere and release the results later.}
% Our experiments also demonstrate that most of our inferred positions can discover new code, which excludes the first time a position is retained.
% Our experiments also demonstrate that most of our inferred positions can discover new code after the first time the positions have discovered new code.


We summarize our contributions as follows.
\begin{itemize}
    \item We use shapely value to explain the contribution of byte positions in terms of code discovery. The results indicate that the repeated mutation of a small portion of positions can improve the efficiency of code discovery. We ascertain that two derivatives for the results are the direct and indirect coupling of path constraints. 
    % \todo{SHAP experiment: why do we use the valuable positions?}
    \item \zkp{We propose a valuable position inference algorithm, which infers the valuable positions on the seed based on the shapley value. We further integrate the calculation process of shapely value into the fuzzing process to improve inference efficiency.}
    \item \zkp{We present a family system to share valuable positions among seeds in a family. The shared positions can be grouped to resolve directly and indirectly coupled path constraints.}
    % We propose a family system to achieve the integration of the pilot stage and havoc stage. Based on semantic consistency, the seeds are divided into multiple families, which allows different seeds in the same family to share the structure-related positions identified by themselves to improve the efficiency of fuzzing.
    % \item We present a contextual multi-armed bandit approach to optimize the selection of shared positions, to further improve the effectiveness of shared positions in discovering new code.
    \item We implemented \tool{} based on AFL++, and evaluated it on UNIFUZZ and MAGMA platforms. The results indicate that \tool{} outperforms various state-of-the-art fuzzers in terms of edge coverage and bug discovery.
\end{itemize}

% \chao{This section has too many details, but does not highlight the key points properly.}\zhu{have revised the intro.}


% \begin{figure*}[!t]
% \centering
% \subfigure[SHAP analysis of \texttt{readelf}]{\includegraphics[width=0.28\linewidth]{images/motivation_readelf_shap.png}} 
% \subfigure[SHAP analysis of \texttt{tiff2bw}]{ \includegraphics[width=0.28\linewidth]{images/motivation_tiff2bw_shap.png}}
% \subfigure[SHAP analysis of \texttt{nm}]{\includegraphics[width=0.28\linewidth]{images/motivation_nm_shap.png}} 
% \subfigure[SHAP analysis of \texttt{objdump}]{\includegraphics[width=0.28\linewidth]{images/motivation_objdump_shap.png}}
% \subfigure[SHAP analysis of \texttt{size}]{\includegraphics[width=0.28\linewidth]{images/motivation_size_shap.png}}
% \subfigure[SHAP analysis of \texttt{tiffsplit}]{\includegraphics[width=0.28\linewidth]{images/motivation_tiffsplit_shap.png}}
% \subfigure[Example of direct and indirect coupling from \texttt{readelf}\label{example_readelf}]{\includegraphics[width=0.85\linewidth]{images/motivation.pdf}}
% \caption{The number of edges contributed by each byte position and the reason for the results of SHAP analysis.}\label{shap_and_example}
% \end{figure*}


% \begin{figure*}
%     \centering
%     \begin{minipage}{\textwidth}
%     \centering
%     \includegraphics[width=0.85\linewidth]{images/shap_legend.png}
%     \end{minipage}
    
%     \begin{minipage}{\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{images/shap_result.jpg}
%     \caption{The number of edges contributed by each byte position (SHAP analysis).}
%     \label{shap_res}
%     \end{minipage}
%     % \begin{minipage}{\textwidth}
%     % \centering
%     % \includegraphics[width=0.85\linewidth]{images/motivation.pdf}
%     % \caption{The number of edges contributed by each byte position and the reason for the results of SHAP analysis.}
%     % \label{example_readelf}
%     % \end{minipage}
% \end{figure*}




\begin{figure*} 
  \centering 
  \subfigure[The number of edges contributed by each byte position (SHAP analysis).\label{shap_res}]{\includegraphics[width=0.65\linewidth]{images/shap_result_new.png}}
  \subfigure[Top X\% positions of the shapey value VS Percentage of contributing new edges.\label{shap_scatter}]{\includegraphics[width=0.34\linewidth]{images/shap_scatter.png}} 
  \caption{Shapely Value Analysis.} 
  %\label{fig1} 
\end{figure*} 


% \begin{figure*}[t!]
% \centering
% \includegraphics[width=0.85\linewidth]{images/shap_legend.png}
% \label{shap_legend}
% \end{figure*}

% \begin{figure*}[t!]
% \vspace{-0.4cm} 
% \setlength{\abovecaptionskip}{0.cm}
% \centering
% \includegraphics[width=\linewidth]{images/shap_result.jpg}
% \caption{SHAP analysis of \texttt{nm}, \texttt{objdump}, \texttt{readelf}, \texttt{size}, \texttt{tiff2bw} and \texttt{tiffsplit}}
% \label{shap_res}
% \end{figure*}


\begin{figure*}[t!]
\centering
\includegraphics[width=0.85\linewidth]{images/motivation.pdf}
\caption{The reason for the results of SHAP analysis.}
\label{example_readelf}
\end{figure*}



==> obsolete/intro-3.0.tex <==



\section{Introduction}
% \zkp{
% \begin{itemize}
%     \item What is the contribution of each byte to the code discovery?
%     \item Quantify the contribution of each byte to the code discovery using shapely value.
%     \item Two conclusions are obtained:
%     \begin{itemize}
%         \item the discovery of code largely depends on a small portion of byte positions.
%         \item the mutation of the same byte positions can repeatedly discover new code.
%     \end{itemize}
%     \item (Findings -> How to improve fuzzing efficiency) If we can identify valuable positions during the fuzzing process, we can allocate more energy to them for mutation, thereby improving the fuzzing efficiency.
%     \item Specifically, to discover new code, the input bytes should satisfy branch constraints of different execution paths. These constraints are not independent, i.e., they influence each other along the same execution path or even across different execution paths. Some constraints are nested together (denoted as {\em direct coupling}) in a program path, and thus require mutating a group of input bytes to pass. Some constraints are shared across program paths of different inputs (denoted as {\em indirect coupling}), suggesting that repeatedly mutating certain bytes may still discover new code. 
%     \item Using valuable positions to guide fuzzing faces three challenges:
%     \begin{itemize}
%         \item 
%     \end{itemize}
% \end{itemize}
% }

% \zhu{enhance the description of reinforcement learning and shap. 
% \begin{itemize}
%     \item problem of inference-based fuzzing: duplicated inference: a same constraint is inferred in different seeds; constraints may share the same input format (indirect coupling); the longer a seed is, the more time the fuzzer needs to infer related bytes.
%     \item Question: while a position has already discovered new code coverage, can we still focus on it? Why do we repeatedly use the same positions?
%     \item Question: Can the bytes inferred by our \tool{} cover the bytes inferred by others?: Probably no. Some inferred bytes by greyone cannot discover new edges.
%     \item Question: for existing seed-scheduling fuzzers~\cite{Yue2020EcoFuzz}, they intend to focus on seeds that have discovered more new code coverage. The question is, since theoretically, the total coverage discovered by a seed is fixed, how is this solution effective in discovering new code coverage? ==> we need to exchange information between seeds.
% \end{itemize}
% }

% \todo{\begin{itemize}
%     \item with the popularity of fuzzing, many fuzzing solutions can improve the efficiency of discovering code coverage;
%     \item they have proposed many theories or develop algorithms based on intuitive observation to achieve it; EMS: migrate the byte values; we are trying to migrate byte positions
%     \item based on our fuzzing experience, we observe that most edges are discovered by a small portion of input bytes;
%     \item byte schedule is important so that we use SHAP to dig deep into the reasons.
%     \item we use SHAP to demonstrate the observation
%     \item we further dig deep into the reasons of the phenomenon, and observe two reasons: direct and indirect coupling
% \end{itemize}}
% \zkp{
Mutation-based fuzzing is a widely-used technique to detect software security issues among both academic and industrial practitioners.
In general, to generate new inputs, it includes seed selection (the next seed to be mutated), energy assignment (the number of mutants assigned to the selected seed), and byte mutation (the strategy to select and mutate bytes).
% In general, it selects which seeds to mutate (seed selection), then decides how many mutants to yield (energy allocation), and determines which bytes to mutate and how to mutate (byte mutation).
For byte mutation, many existing solutions have been developed to expand code coverage. We can divide these solutions into three categories.
The first category is utilizing taint analysis to track and mutate the related bytes of path constraints, such as TaintScope~\cite{taintscope}, Dowser~\cite{dowser} and Angora~\cite{angora}.
The second category improves fuzzers by inferring the dependence between bytes and constraints, including GREYONE~\cite{greyone}, ProFuzzer~\cite{profuzzer} and PATA~\cite{pata}.
The third category determines where to mutate seeds via extracting information from history data, such as NEUZZ~\cite{neuzz}, MTFuzz~\cite{mtfuzz} and EMS~\cite{ems}.
Because byte mutation has great impact on fuzzing performance, a core question to answer is \textit{what is the contribution of each byte to the code discovery?} 
However, none of the existing solutions have studied this question.
% Although these fuzzers understand the impact of byte selection and mutation on fuzzing, none of them researches on the question about the contribution of each byte to the code discovery.
% \zkp{(What is the significance of studying this problem/Why we study this problem)}

% }
% Fuzzing is known as a de facto technique to detect software security issues among both academic and industrial practitioners~\cite{zhu2022roadmap}.
% \chao{It would be better to focus on mutation-based fuzzing directly, which consists of several critical steps: select which seeds to mutate (seed selection), decide how many mutants to yield (energy allocation), decide which bytes to mutate and how to mutate (byte mutation).}
% In the set of existing fuzzing solutions, coverage-guided greybox fuzzing (CGF) has performed remarkably well in detecting real-world bugs~\cite{ossfuzz, onefuzz, feng2021snipuzz, aflchurn}. 
% This method aims to enhance code coverage so that potential bugs are disclosed in the unseen parts of the code. Existing studies have reported many efforts to expand code coverage, including scheduling of computational resources for certain code regions~\cite{aflfast, fairfuzz, Yue2020EcoFuzz, mobfuzz} and resolving path constraints~\cite{angora, qsym, dowser, tfuzz, digfuzz, huang2020pangolin}.
% However, only a few solutions have studied the selection and mutation of input bytes~\cite{greyone, pata, ems, profuzzer, neuzz, mtfuzz}. \chao{It would be better to classify these closely-related solutions into several categories. BTW, put the names of these solutions here rather than just citation links.}
% Those solutions focus on grouping bytes that influence the same path constraints or constructing the same data type. Yet, none of them studies the contribution of bytes to the code discovery.
% \chao{These two sentences should be rephrased. The first sentence fails to cover all closely-related solutions, and the second one fails to express why it is necessary. Maybe we can say that, selecting which bytes to mutate would have great impact on fuzzing performance, a core question to answer is that what is the contribution of each byte to the code discovery, and none of existing solutions have studied this question.}
% To the best of our knowledge, only EMS~\cite{ems} studies the optimization of selecting bytes.
% While scheduling computational resources is an implicit way to expand code coverage, resolving path constraints is an explicit way to achieve the same. Since path constraints guard certain code regions, any success in passing path constraints most likely results in new code coverage. However, resolving path constraints is not a trivial task as those constraints may be quite complicated. 


% \zhu{1. what is the contribution of each byte to the code discovery? 2. Intuitively, we can use Shapley Analysis to calculate the contribution of each byte; 3. we then formulate the process of byte schedule as Shapley Analysis; 4. each test of fuzzing is one trial of shapley analysis; 5. yet, fuzzing is stateful, which means the result of new edges depends on the previous discovery of edges. Shapley analysis is not stateful; 6. To satisfy the process of Shapley analysis, we need to build a bitmap for each seed, which introduces much overhead; 7. we observe that sharing positions is common in fuzzing; 8. based on the observation, we simplify the Shapley analysis with the family system; 9. The observation also provides the support for the prediction of new edges; 10. Why will this solution fall in local optimum? (Use Havoc mode to solve local optimum).}

% In fuzzing, the problem of resolving path constraints is essentially the byte scheduling, including which bytes to select and how to mutate the selected bytes~\cite{greyone, ems, profuzzer, neuzz, mtfuzz, pata, angora}. 
\zkp{(Explain why shapely value is used: ) 
In cooperative game theory, shapely value is used to measure the contribution made by each member of a team.
To study the contribution of each byte, we model byte mutation as a teamwork process.
Therefore, we can also use shapely value to quantify the contribution of each byte to new edge discovery.
}
We conducted a group of fuzzing experiments and performed shapely value~\cite{Shapley} analysis to study the experiment results.
Interestingly, the analysis demonstrates that (1) \textit{the discovery of code largely depends on a small portion of byte positions}, and (2) \textit{the mutation of the same byte positions can repeatedly discover new code}. \zkp{More details of the experiments are introduced in Section~\ref{sec:motivation}.}

% \zkp{This section keeps explaining the source of findings, but never explains the relationship between findings and improving the efficiency of fuzzing.}
% Though such findings might be biased because the number of programs and seed inputs used in the experiments are limited, we notice that this matches with the nature of program logic.
We notice that such findings match with the nature of program logic.
Specifically, to discover new code, the input bytes should satisfy branch constraints of different execution paths. These constraints are not independent, i.e., they influence each other along the same execution path or even across different execution paths. Some constraints are nested together (denoted as {\em direct coupling}) in a program path, and thus require mutating a group of input bytes to pass. Some constraints are shared across program paths of different inputs (denoted as {\em indirect coupling}), suggesting that repeatedly mutating certain bytes may still discover new code.
% This nature indicates that the byte positions, which resolve one path constraint, have a high chance to be able to resolve another constraint, in or not in the same execution path.
% While such findings might be biased because of the program set selected in SHAP analysis, we dive deep into the reasons for the SHAP results. 
% One reason is \textit{direct coupling} (different constraints related to the same positions of inputs), which refers to the fact that the flip of a path constraint has to consider the results of other path constraints. For example, to pass the condition $if(b == 0x123)$, we may need to figure out all the conditions that the variable $b$ depends on, such as $if(a == 0x22)\{b = 0x12\}$.
% The exploration of directly coupled path constraints will lead to deep code in programs (exemplified in Section~\ref{sec:motivation}). Another reason is that different program logic may process the same format of inputs, indicating that different constraints could be related to the same positions of inputs (we call it \textit{indirect coupling}).
% The usage of indirect coupling helps fuzzing quickly explore new code if a fuzzer only mutates the corresponding byte positions (exemplified in Section~\ref{sec:motivation}).

% 


% \zkp{(Findings -> How to improve fuzzing efficiency) }
The results of SHAP analysis indicate that, byte positions contribute differently to the discovery of code regions,
% Then, why do we treat each position equally during byte schedule? 
% According to the findings, 
and the repeated mutation of a (small) portion of byte positions can identify most of the discovered code during fuzzing.
% \zkp{
% (Explain why these findings can improve the fuzzing efficiency)
% }
\zkp{
Based on these findings, we can therefore optimize the fuzzing process by identifying valuable positions(\ie the byte positions that contribute to discovering code) during fuzzing and focusing on mutations for them. However, guiding fuzzing with valuable positions encounters following three problems.

First, due to the complicated calculation process of shapely value, it is time-consuming to directly quantify the contribution of each byte to code discovery during the fuzzing process. Therefore, \textit{Problem I} is: \textit{How to perform lightweight inference for valuable positions during fuzzing?}

Second, the inference process of the valuable positions of each seed is independent.
However, due to the similarity between some seeds, they may have the same valuable positions, which can be used to improve the inference efficiency.
Thus, \textit{Problem II} is: \textit{How to efficiently utilize these valuable positions across different seeds, so that we can save time identifying valuable positions for different seeds.}

Third, after getting the valuable positions, we need to mutate them to find more new edges. 
However, valuable positions will become stale
after a period of testing, which indicates we need to continuously increase the number of valuable positions during fuzzing.
Thus, \textit{Problem III} is: \textit{How to increase the number of valuable positions while using valuable positions to guide the mutation direction?}


}




% Based on these findings, we can therefore optimize the fuzzing process by addressing the following three questions. 
% The first one is how to identify the \textit{valuable positions}, \ie the byte positions that contribute to discovering code.
% The second one is how to efficiently utilize these valuable positions across different seeds, so that we can save time identifying valuable positions for different seeds.
% The third one is how to guide the mutation based on valuable positions.
% , so that we can save time identifying valuable positions for different seeds.

% Put differently, the positions that have discovered new code (\ie \textit{valuable positions}) deserve more computational resources. 
% However, existing solutions for resolving path constraints neglect the difference between byte positions. 
% For instance, some fuzzers establish a relationship between the input bytes that influence the same path constraint~\cite{greyone, ems, angora, vuzzer, steelix} or construct the same data type~\cite{profuzzer, angora}, and mutate the related bytes as a group.
% Although such grouping can reduce the search space of passing constraints, they continue to infer other constraint-related bytes, without intentionally repeating the mutation of valuable positions. \chao{<-- Any proofs to support this argument? Bytes are likely to be repeatedly mutated during fuzzing even in a random fuzzing solution, I think.} \zhu{I add `intentionally'.}
% Moreover, since their grouped bytes are related to a single path constraint, which neglects the coupled ones, the existing solutions only give a shallow view to the logic of programs.


% \todo{in progress}

% In fuzzing, a promising solution for resolving path constraints is to infer the relationships among input bytes and mutate related bytes together in later fuzzing campaigns~\cite{greyone, ems, profuzzer, neuzz, mtfuzz, pata}.
% For instance, some fuzzers establish a relationship between the input bytes that influence the same path constraint~\cite{greyone, ems, angora, vuzzer, steelix} or construct the same data type~\cite{profuzzer, angora}.
% Such inferences can reduce the search space of passing constraints if fuzzing combines related bytes into groups and mutates them on a group basis. 
% For instance, mutating 12 bytes can generate $256^{12}$ different inputs, while mutating 4 bytes at a time (4 bytes a group) only generates $3\times256^{4}$ inputs.
% If a path constraint is related to just one group, the combination of bytes can significantly improve the efficiency of code discovery. 
 


% Essentially, the groups reflect the format of inputs, which further represent the internal logic of programs. However, the existing inference solutions only give a shallow view to the logic of programs. These solutions only infer the relationships between bytes for a single path constraint at a time. Each time, the bytes related to a single path constraint are mutated. This neglects the fact that different path constraints might be heavily coupled. For example, to pass the condition $if(b == 0x123)$, we may need to figure out all the conditions that the variable $b$ depends on, such as $if(a == 0x22)\{b = 0x12\}$. In this case, it is insufficient to only mutate the bytes related to the variable $b$ for the path constraint to be passed. Therefore, in order to fuzz code guarded by complex constraints, the inference algorithm (of related bytes) needs to consider the coupling of path constraints.

% \begin{figure*}[t!]
% % \vspace{-0.6cm} 
% \centering
% \includegraphics[width=0.8\linewidth]{images/motivation.pdf}
% \caption{Example of direct and indirect coupling from \texttt{readelf}.}
% \label{readelf_example}
% \end{figure*}



% In this paper, we propose \tool{}, a lightweight fuzzer that mutates inputs by considering the coupling of path constraints. \tool{} infers and groups the bytes related to the coupled path constraints based on two observations. One observation is what we call \textit{direct coupling}, and it refers to the fact that the flip of a path constraint has to consider the results of other path constraints. The exploration of directly coupled path constraints will lead to deep code in programs (exemplified in Section~\ref{sec:motivation}). Another observation is that different program logics may process the same format of inputs, indicating that different constraints could be related to the same positions of inputs (we call it \textit{indirect coupling}). The usage of indirect coupling helps fuzzing quickly explore new code if a fuzzer only mutates the corresponding byte positions (exemplified in Section~\ref{sec:motivation}).

\zkp{
In this paper, we propose \tool{} to address the aforementioned three problems.
To solve the time-consuming problem of shapely value calculation in \textit{Problem I}, we propose a lightweight valuable position inference algorithm, which integrates the calculation process of shapely value into the fuzzing process. Specifically, we record the mutated positions sequence of each mutation. If the mutated input discovers new code coverage, we compute the marginal contribution of each position within the mutated positions sequence. Then for each position, we accumulate its marginal contribution on all mutations to get the \textit{edge contribution}. If the edge contribution of a position is greater than 0, we consider it to be a valuable position. 
% Note that we only deal with mutated input without length mutators because length mutators can cause most positions to change.

To share valuable positions across different seeds in \textit{Problem II}, we propose a family system. We cluster seeds into families based on inheritance relationship and seed length. 
% Each family maintains its own shared pool, which records the valuable positions that all seeds in the family have discovered. 
In each family, we will maintain a shared pool for sharing the valuable positions found by all seeds in the family.
Each seed can either add the valuable positions it discovers to the shared pool or obtain its unknown valuable positions from the shared pool.

To solve the update problem of valuable positions in \textit{Problem III}, We design two modes in the mutation stage: family-based mutation and havoc mutation.
Among them, family-based mutation mutates valuable positions to discover more new code, while havoc mutation mutates all positions to infer more valuable positions.
We use a simple yet effective indicator to quantify the efficiency of each mutation mode and select the best mode
in the next mutation round.

}



% In this paper, we propose \tool{} to address the two problems and guide fuzzers to select valuable bytes to mutate.
% % \chao{This paragraph does not address the two problems accordingly.}\zhu{revised.}
% \tool{} first assumes that the byte positions that have discovered new code are potential valuable positions.
% To effectively utilize valuable positions across seeds, it then builds a \textit{family system} to share these.
% The purpose of the family system is to ensure that the shared positions are related to the corresponding path constraints of any family member.  
% Finally, to optimize the use of potential valuable positions, \tool{} utilizes a \textit{contextual multi-armed bandit} (CMAB) based on the family system.
% The CMAB, which considers the context of valuable positions, optimizes byte mutation by predicting and seeking out the best rewards, \ie code discovery.
% The CMAB tries some of the potential valuable positions, and decides to assign more energy to certain positions based on the reward of those trials.
% As a result, \tool{} has a high chance to select and combine the positions with the highest contribution for byte mutation.

% It then utilizes a \textit{contextual multi-armed bandit} (CMAB) approach to further infer the most contributing byte positions.
% The CMAB approach is designed based on a \textit{family system}, which improves the effectiveness of utilizing valuable positions across seeds.
% Then, it builds a \textit{family system} and utilizes a \textit{contextual multi-armed bandit} (CMAB) approach to 1) share the valuable positions among seeds, and 2) optimize the mutation of the shared positions.



% Since the byte positions that have discovered new code already contribute to the code discovery, we assume that they are the valuable positions.
% To efficiently use valuable positions, \tool{} builds a \textit{family system} and utilizes a \textit{contextual multi-armed bandit} (CMAB) approach to 1) share the valuable positions among seeds, and 2) optimize the mutation of the shared positions.
% To achieve that, the family system is required to ensure that, for any seed in a family, the shared positions are still related to the seed's corresponding path constraints.
% To satisfy the requirement, a family is built if the seeds in the family are obtained just by mutating an original seed without changing its length.
% Since the meaning of each position may be changed at the trimming stage, which is performed to reduce the length of the seeds, \tool{} traces the change of positions to maintain the meaning of positions. 
% However, the building process of a family can only roughly satisfy the requirement. 
% \chao{It's not clear why CMAB can solve this issue.}
% To increase the chances that the selected positions for a seed are related to (unsolved) path constraints, \tool{} uses a contextual multi-armed bandit (CMAB) approach to schedule bytes by considering the context of them.
% % to dynamically generate a probability distribution for the selection of positions.  
% The context used by \tool{} is the feature vector extracted from execution paths. 
% Note that, \tool{} will select positions related to multiple path constraints, so that the directly coupled path constraints can be fuzzed.
% % the positions selected by \tool{} may be related to multiple path constraints, so that the directly coupled path constraints can be fuzzed.


We implement \tool{} based on AFL++~\cite{aflpp}, and evaluate it on two third-party platforms, including 1) UNIFUZZ~\cite{unifuzz}, which contains real-world programs, and 2) MAGMA~\cite{magma}, which provides a series of real-world programs with known bugs.
On UNIFUZZ, we evaluate \tool{}-related fuzzers (\ie \tool{} and \tool{}-Redqueen) and four existing modes of AFL++ on 16 target programs.
The results show that, in terms of code coverage, \tool{}-related fuzzers perform better than other fuzzers after running for 1/3/6/12/24 hours.
For instance, the median ranks of \tool{} and \tool{}-Redqueen are 2.62 and 1.18 after fuzzing 24 hours, respectively.
% \zkp{
% For instance, the median ranks of \tool{} and \tool{}-Redqueen are 2.62 and 1.18 after fuzzing 24 hours, respectively. \tool{} finds 12, 55, 42, 36 and 24 more vulnerabilities than AFL++-MOPT-Redqueen, AFL++-MOPT, AFL++-Exploit, AFL++-Fast and AFL++-Rare, respectively.
% }
Additionally, \tool{} discovers 20 more bugs than the best mode of AFL++.
On MAGMA, we evaluate \tool{}-related fuzzers and five widely-used mutation-based fuzzers (\ie AFL~\cite{afl}, AFL++-MOPT-Redqueen, AFLFast~\cite{aflfast}, FairFuzz~\cite{fairfuzz} and MOPT~\cite{MOPT}) on 20 programs. \tool{} exposes six more CVEs than the best of the five competing fuzzers.
Additionally, \tool{} also outperforms EMS~\cite{ems} in terms of both edge and bug discovery. 
% \chao{<-- The comparison with EMS is not very strong. How about bug findings?} \zkp{The EMS bug findings are very poor. I'll check to see if there is a problem somewhere and release the results later.}
% Our experiments also demonstrate that most of our inferred positions can discover new code, which excludes the first time a position is retained.
% Our experiments also demonstrate that most of our inferred positions can discover new code after the first time the positions have discovered new code.


We summarize our contributions as follows.
\begin{itemize}
    \item We use shapely value to explain the contribution of byte positions in terms of code discovery. The results indicate that the repeated mutation of a small portion of positions can improve the efficiency of code discovery. We ascertain that two derivatives for the results are the direct and indirect coupling of path constraints. 
    % \todo{SHAP experiment: why do we use the valuable positions?}
    \item \zkp{We propose a valuable position inference algorithm, which infers the valuable positions on the seed based on the shapley value. We further integrate the calculation process of shapely value into the fuzzing process to improve inference efficiency.}
    \item \zkp{We present a family system to share valuable positions among seeds in a family. The shared positions can be grouped to resolve directly and indirectly coupled path constraints.}
    % We propose a family system to achieve the integration of the pilot stage and havoc stage. Based on semantic consistency, the seeds are divided into multiple families, which allows different seeds in the same family to share the structure-related positions identified by themselves to improve the efficiency of fuzzing.
    % \item We present a contextual multi-armed bandit approach to optimize the selection of shared positions, to further improve the effectiveness of shared positions in discovering new code.
    \item We implemented \tool{} based on AFL++, and evaluated it on UNIFUZZ and MAGMA platforms. The results indicate that \tool{} outperforms various state-of-the-art fuzzers in terms of edge coverage and bug discovery.
\end{itemize}

% \chao{This section has too many details, but does not highlight the key points properly.}\zhu{have revised the intro.}


% \begin{figure*}[!t]
% \centering
% \subfigure[SHAP analysis of \texttt{readelf}]{\includegraphics[width=0.28\linewidth]{images/motivation_readelf_shap.png}} 
% \subfigure[SHAP analysis of \texttt{tiff2bw}]{ \includegraphics[width=0.28\linewidth]{images/motivation_tiff2bw_shap.png}}
% \subfigure[SHAP analysis of \texttt{nm}]{\includegraphics[width=0.28\linewidth]{images/motivation_nm_shap.png}} 
% \subfigure[SHAP analysis of \texttt{objdump}]{\includegraphics[width=0.28\linewidth]{images/motivation_objdump_shap.png}}
% \subfigure[SHAP analysis of \texttt{size}]{\includegraphics[width=0.28\linewidth]{images/motivation_size_shap.png}}
% \subfigure[SHAP analysis of \texttt{tiffsplit}]{\includegraphics[width=0.28\linewidth]{images/motivation_tiffsplit_shap.png}}
% \subfigure[Example of direct and indirect coupling from \texttt{readelf}\label{example_readelf}]{\includegraphics[width=0.85\linewidth]{images/motivation.pdf}}
% \caption{The number of edges contributed by each byte position and the reason for the results of SHAP analysis.}\label{shap_and_example}
% \end{figure*}


% \begin{figure*}
%     \centering
%     \begin{minipage}{\textwidth}
%     \centering
%     \includegraphics[width=0.85\linewidth]{images/shap_legend.png}
%     \end{minipage}
    
%     \begin{minipage}{\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{images/shap_result.jpg}
%     \caption{The number of edges contributed by each byte position (SHAP analysis).}
%     \label{shap_res}
%     \end{minipage}
%     % \begin{minipage}{\textwidth}
%     % \centering
%     % \includegraphics[width=0.85\linewidth]{images/motivation.pdf}
%     % \caption{The number of edges contributed by each byte position and the reason for the results of SHAP analysis.}
%     % \label{example_readelf}
%     % \end{minipage}
% \end{figure*}




% \begin{figure*} 
%   \centering 
%   \subfigure[The number of edges contributed by each byte position (SHAP analysis).\label{shap_res}]{\includegraphics[width=0.65\linewidth]{images/shap_result_new.png}}
%   \subfigure[Top X\% positions of the shapey value VS Percentage of contributing new edges.\label{shap_scatter}]{\includegraphics[width=0.34\linewidth]{images/shap_scatter.png}} 
%   \caption{Shapely Value Analysis.} 
%   %\label{fig1} 
% \end{figure*} 




% \begin{figure*}[t!]
% \centering
% \includegraphics[width=0.85\linewidth]{images/shap_legend.png}
% \label{shap_legend}
% \end{figure*}

% \begin{figure*}[t!]
% \vspace{-0.4cm} 
% \setlength{\abovecaptionskip}{0.cm}
% \centering
% \includegraphics[width=\linewidth]{images/shap_result.jpg}
% \caption{SHAP analysis of \texttt{nm}, \texttt{objdump}, \texttt{readelf}, \texttt{size}, \texttt{tiff2bw} and \texttt{tiffsplit}}
% \label{shap_res}
% \end{figure*}


\begin{figure*}[t!]
\centering
\includegraphics[width=0.85\linewidth]{images/motivation.pdf}
\caption{The reason for the results of SHAP analysis.}
\label{example_readelf}
\end{figure*}



==> obsolete/intro-3.1.tex <==
\section{Introduction}

Mutation-based fuzzing is a widely-used technique to detect software security issues among both academic and industrial practitioners~\cite{zhu2022roadmap}.
% In general, to generate new inputs, it includes seed selection (the next seed to be mutated), energy assignment (the number of mutants assigned to the selected seed), and byte mutation (the strategy to select and mutate bytes).
In general, to mutate an input, there are two core choices to make: which bytes to mutate (byte selection) and what new values to use (value update).
Existing solutions often rely on expert experience to recognize critical input bytes (\eg magic number bytes) for mutation. 
% For byte mutation, many existing solutions have been developed to expand code coverage. We can divide these solutions into three categories.
The first category of solutions utilizes taint analysis to track the bytes related to path constraints. TaintScope~\cite{taintscope}, Dowser~\cite{dowser} and Angora~\cite{angora} are examples of the first category.
The second category indirectly infers the dependence between bytes and constraints. Members of this category include GREYONE~\cite{greyone}, REDQUEEN~\cite{redqueen}, ProFuzzer~\cite{profuzzer} and PATA~\cite{pata}.
The third category finds where to mutate by extracting information from historical data. NEUZZ~\cite{neuzz}, MTFuzz~\cite{mtfuzz} and EMS~\cite{ems} fall into the third category.
But general byte selection (not just critical bytes) is an underexplored problem. A fundamental question to answer is \textit{what is the contribution of each byte to code discovery?} 
% However, none of the existing solutions have studied this question.
% \chao{this argument is too strong.}

 
Basically, discovering new edges is due to the cooperation of certain bytes, or more precisely, their cooperative mutations. This motivates us to take the perspective of Cooperative Game Theory~\cite{Shapley} and study the byte scheduling of fuzzing as a process of Shapley analysis~\cite{shap}.
% 
% To understand the result of Shapley analysis in fuzzing, 
We have conducted a set of fuzzing experiments and performed Shapley analysis to determine the contribution of each byte to discovering new code. That is, we use Shapley analysis to evaluate the importance of input bytes.
Interestingly, the analysis demonstrates that (1) \textit{the discovery of new code largely depends on a small portion of byte positions}, and (2) \textit{the mutation of the same byte positions can repeatedly discover new code}.
% \textit{the mutation of the same byte positions can repeatedly discover new code}. 
% \todo{change: the repetitive mutations of certain bytes can still lead to the discovery of new program paths.}


% \zhu{If a byte is related to more path constraints, it will have a larger Shapley value. We notice that the two findings match with the nature of program logic. For example, a byte may be related to multiple path constraints in a program. }

\zkp{
We observe that these two findings match the nature of program logic. Specifically, some input bytes are repeatedly utilized in path constraints that prevent fuzzing from discovering code. Our experiments also demonstrated that 86\% bytes are related to multiple CMP instructions (more details in Section~\ref{sec:motivation}). 
% More details are introduced in Section \ref{sec:motivation}. 
Thus, \todo{add: repetitive} mutation of some certain input bytes (important bytes) can efficiently solve constraints in different paths. 
The Shapley value, which can evaluate the importance of input bytes, is promising to guide and boost fuzzing.
The key insight is to get the important bytes by using Shapley analysis on one path constraint. Then, for other path constraints that have the same important bytes, we can solve them efficiently by focusing on mutating those bytes.
% If $N$ path constraints are related to the same input bytes, we can obtain the information of constraint-related bytes by exploring one of those paths. For the remaining $N-1$ constraints, we can solve them efficiently in the subsequent fuzzing campaigns by focusing on mutating those constraint-related bytes. By using Shapley analysis, we not only obtain the constraint-related bytes but also get the importance of them.



To capture and utilize important bytes, we calculate Shapley values based on Shapley analysis. 
However, the full Shapley analysis of a byte requires that all the possible inputs related to the byte have been generated and tested. 
Then, no new inputs can be generated for the byte after the full Shapley analysis, making the Shapley values useless for guiding fuzzing.
Therefore, we propose to utilize \textit{temporary} Shapley values calculated by \textit{incomplete} Shapley analysis to guide fuzzing.
The aforementioned empirical observation implies that this is feasible.
For bytes that temporarily have high Shapley values, they still have the probability to be related to multiple unseen path constraints. Thus, repeated mutation of them may solve those unseen path constraints and improve the efficiency of discovering new code.


We leverage this insight and propose \tool{} to boost the efficiency of byte selection based on Shapley analysis. Specifically, we formulate the solution to byte selection as a Shapley analysis across multiple seed inputs.
To reduce the overhead of calculating Shapley values, we classify seeds into different \textit{families} and share Shapley values for each family, and further transform the Shapley value calculation into a form that can be gradually updated by each seed input. We further utilize contextual multi-armed bandit (CMAB) to maximize the efficiency of fuzzing when using \textit{incomplete} Shapley values.
% The CMAB is used to make a trade-off between updating Shapley values for all bytes and mutating bytes with higher Shapley values. 
On the one hand, high Shapley value bytes might not be useful in some situations, \eg all related constraints of a byte have been explored. Consequently, CMAB assesses the efficiency of each byte based on the mutation performance of the selected bytes. On the other hand, since we obtain incomplete Shapley values during fuzzing, we still need to provide more opportunities for low-frequently chosen bytes to obtain more accurate Shapley values. Therefore, we use CMAB to make a trade-off between mutating high Shapley value bytes and low-frequently chosen bytes.



%%% Kunpeng's version
% The findings above demonstrate that bytes are not equal. Several methods have been proposed to infer important bytes in a seed, such as NEUZZ~\cite{neuzz}, GreyOne~\cite{greyone}, Angora~\cite{angora}, and so on. However, these approaches require additional testing or model-building to complete the inference, neglecting the potential benefits of utilizing fuzzing history. We discover that important bytes can be extracted from fuzzing history, and repeatedly mutating these bytes can lead to the discovery of new edges. More specifically, different path constraints may contain common important bytes. Assuming there are $N$ path constraints containing common important bytes, if we extract these important bytes while exploring a particular path constraint, we may be able to solve the remaining $N-1$ constraints faster in the subsequent fuzzing process by focusing on mutating these important bytes. Our insights rely on the widespread presence of path constraints containing common important bytes. We conduct relevant statistics on 16 programs and found this to be a common occurrence.


% To leverage fuzzing history, the key challenge lies in capturing and utilizing important bytes. First, we quantify the contribution of each byte using Shapley Value. The higher a byte's Shapley Value, the more crucial it is. However, the computation of Shapley Value is time-consuming. Thus, we model the fuzzing process as a Shapley Value computation procedure, introducing minimal overhead. Second, we employ Contextual Multi-Armed Bandits (CMAB) to achieve efficient byte scheduling. By focusing on mutating high Shapley value bytes (i.e., important bytes), we can quickly resolve other related path constraints. However, in some specific cases (e.g., when all related constraints of a byte have been explored), high Shapley value bytes may not be useful. Consequently, CMAB assesses the efficiency of each byte based on the mutation performance of the selected bytes. Simultaneously, since we obtain incomplete Shapley values during the fuzzing process, we still need to provide more opportunities for low-frequency chosen bytes to obtain more accurate Shapley values. In summary, we use CMAB to make a trade-off between mutating high Shapley value bytes and low-frequency chosen bytes.
}

% % However, due to the complexity and overhead of Shapley analysis, it is impractical to directly guide fuzzing based on Shapley analysis.
% The Shapley values, as the result of Shapley analysis, reflect the importance (contribution) of bytes, and therefore can be utilized to guide byte selection for fuzzing. 
% However, the full Shapley analysis of a byte requires that all the possible inputs related to the byte have been generated and tested. 
% Then, no new inputs can be generated for the byte after the full Shapley analysis, making the Shapley values useless for guiding fuzzing.
% % even though we obtain the importance of the byte, it cannot be utilized to guide fuzzing because no new inputs can be generated for the byte.
% % 
% % There is a conflict to use Shapley values to guide fuzzing. 
% % On the one hand, Shapley values calculated during fuzzing is incomplete because the calculation does not use all possible inputs. The problem of incomplete Shapley values is that they cannot accurately reflect the importance of a byte. On the other hand, if the calculation is complete, all possible inputs have been generated. No more inputs can be generated to discover new code. 
% % Fortunately, the root causes for Shapley results in Section~\ref{sec:motivation} allow the use of incomplete Shapley values. Even for positions that temporarily have high Shapley values, they still have the chance to be related to multiple (unseen) path constraints. Therefore, the incomplete Shapley values can still be utilized to guide fuzzing. Besides, we use CMAB to mitigate the problem of incomplete Shapley values.
% % 
% Therefore, we propose to utilize \textit{temporary} Shapley values calculated by \textit{incomplete} Shapley analysis to guide fuzzing.
% The aforementioned empirical observation implies that this is feasible.
% % % 
% % Fortunately, due to the properties of program logic and fuzzing, we can still use Shapley values to boost fuzzing efficiency.
% % % 
% % These findings indicate that even though the Shapley values of bytes are incomplete \chao{why incomplete?}, they can still guide fuzzing.
% % % to assign more energy to bytes with high (incomplete) Shapley values.
% For bytes that temporarily have high Shapley values, they still have the probability to be related to multiple unseen path constraints. Thus, repeated mutation of them may solve those unseen path constraints and discover new code.


% We leverage this insight and propose \tool{} to boost the efficiency of byte selection based on Shapley analysis. Specifically, we formulate the solution to byte selection as a Shapley analysis across multiple seed inputs.
% To reduce the overhead of calculating Shapley values, we classify seeds into different \textit{families} and share Shapley values for each family, and further transform the Shapley value calculation into a form that can be gradually updated by each seed input. We further utilize contextual multi-armed bandit (CMAB) to maximize the efficiency of fuzzing with \textit{incomplete} Shapley values.
% Specifically, the CMAB is used to make a trade-off between updating Shapley values for all bytes and mutating bytes with higher Shapley values. 
% % We then implement \tool{} to boost the efficiency of byte selection based on Shapley analysis. 
 



% \zhu{TODO:}
% This enables us to analyze the contributions of bytes in seeds. 



% \zkp{(Explain why shapely value is used: ) To study the contribution of each byte, we model the selection and mutation process of bytes as a teamwork process.
% In cooperative game theory, shapely value is used to measure the contribution made by each member of a team.
% Therefore, we can also use shapely value to quantify the contribution of each byte to new edge discovery.
% }
% To analyze the contribution of each byte in discovering code, we conducted a group of fuzzing experiments and performed SHapley Additive exPlanations (SHAP)~\cite{shap} analysis to study the experiment results.
% Interestingly, the analysis demonstrates that (1) \textit{the discovery of code largely depends on a small portion of byte positions}, and (2) \textit{the mutation of the same byte positions can repeatedly discover new code}. \zkp{More details of the experiments are introduced in Section~\ref{sec:motivation}.}

% \zkp{This section keeps explaining the source of findings, but never explains the relationship between findings and improving the efficiency of fuzzing.}
% Though such findings might be biased because the number of programs and seed inputs used in the experiments are limited, we notice that this matches with the nature of program logic.
% Specifically, to discover new code, the input bytes should satisfy branch constraints of different execution paths. These constraints are not independent, i.e., they influence each other along the same execution path or even across different execution paths. Some constraints are nested together (denoted as {\em direct coupling}) in a program path, and thus require mutating a group of input bytes to pass. Some constraints are shared across program paths of different inputs (denoted as {\em indirect coupling}), suggesting that repeatedly mutating certain bytes may still discover new code.


% \zkp{(Findings -> How to improve fuzzing efficiency) }



% The results of SHAP analysis indicate that, byte positions contribute differently to the discovery of code regions,
% and the repeated mutation of a (small) portion of byte positions can identify most of the discovered code during fuzzing.
% \zkp{
% (Explain why these findings can improve the fuzzing efficiency)
% }
% Based on these findings, we can therefore optimize the fuzzing process by addressing the following two questions. 
% The first one is how to identify the \textit{valuable positions}, \ie the byte positions that contribute mostly to discovering code.
% The second one is how to efficiently utilize these valuable positions across different seeds.


% In this paper, we propose \tool{} to address the two problems and guide fuzzers to select valuable bytes to mutate.
% \tool{} first assumes that the byte positions that have discovered new code are potential valuable positions.
% To effectively utilize valuable positions across seeds, it then builds a \textit{family system} to share these.
% The purpose of the family system is to ensure that the shared positions are related to the corresponding path constraints of any family member.  
% Finally, to optimize the use of potential valuable positions, \tool{} utilizes a \textit{contextual multi-armed bandit} (CMAB) based on the family system.
% The CMAB, which considers the context of valuable positions, optimizes byte mutation by predicting and seeking out the best rewards, \ie code discovery.
% The CMAB tries some of the potential valuable positions, and decides to assign more energy to certain positions based on the reward of those trials.
% As a result, \tool{} has a high chance to select and combine the positions with the highest contribution for byte mutation.


% We implement \tool{} based on AFL++~\cite{aflpp}, and evaluate it on two third-party platforms, including 1) UNIFUZZ~\cite{unifuzz}, which contains real-world programs, and 2) MAGMA~\cite{magma}, which provides a series of real-world programs with known bugs.
% On UNIFUZZ, we evaluate \tool{}-related fuzzers (\ie \tool{} and \tool{}-Redqueen) and five existing modes of AFL++ on 16 target programs.
% The results show that, in terms of code coverage, \tool{}-related fuzzers perform better than other fuzzers after running for 1/3/6/12/24 hours.
% For instance, the median ranks of \tool{} and \tool{}-Redqueen are 2.62 and 1.18 after fuzzing 24 hours, respectively.
% Additionally, \tool{} discovers 20 more bugs than the best mode of AFL++.
% On MAGMA, we evaluate \tool{}-related fuzzers and five widely-used mutation-based fuzzers (\ie AFL~\cite{afl}, AFL++-MOPT-Redqueen, AFLFast~\cite{aflfast}, FairFuzz~\cite{fairfuzz} and MOPT~\cite{MOPT}) on 20 programs. \tool{} exposes six more CVEs than the best of the five competing fuzzers.
% Additionally, \tool{} also outperforms EMS~\cite{ems} in terms of both edge and bug discovery. 

% We leverage this insight and propose \tool{} to boost the efficiency of byte selection based on Shapley analysis.
We implemented a prototype \tool{} based on AFL++~\cite{aflpp}.
We evaluate them on two third-party benchmarks, including 1) UNIFUZZ~\cite{unifuzz}, which contains real-world programs, and 2) MAGMA~\cite{magma}, which provides a series of real-world programs with known bugs. 
We compare their performance with 10 widely-used fuzzers, including 5 byte schedule-reinforced fuzzers (GreyOne~\cite{greyone}, ProFuzzer~\cite{profuzzer}, Angora~\cite{angora}, PreFuzz~\cite{prefuzz} and NEUZZ~\cite{neuzz}) and 5 commonly used fuzzers (AFL++~\cite{aflpp}, MOPT~\cite{MOPT}, AFLFast~\cite{aflfast}, FairFuzz~\cite{fairfuzz} and AFL~\cite{afl}).
% including AFL++~\cite{aflpp}, MOPT~\cite{MOPT}, AFLFast~\cite{aflfast}, FairFuzz~\cite{fairfuzz} and AFL~\cite{afl}.
\zkp{
Compared with byte schedule-reinforced fuzzers, when all initial seeds are given, \tool{} discovers 4170 more edges and exposes 19 more bugs than the best baseline.
In addition, when given two initial seed sets with lengths less than 10,000 and 1,000, \tool{} is still able to discover the most edges and expose the most bugs.
Compared with commonly used fuzzers, \tool{} discovers 20 to 68 more bugs than other five fuzzers, and exposes six more CVEs than the best of the five fuzzers.
Furthermore, \tool{} discovers 11 new bugs, 3 of which are confirmed by vendors.
}




% On UNIFUZZ, in terms of code coverage, \tool{} performs better than other fuzzers after running for 1/3/6/12/24 hours. For instance, the median ranks of \tool{} and \tool{}-Redqueen are 2.62 and 1.18 after fuzzing 24 hours, respectively. 
% Additionally, \tool{} discovers 20 to 68 more bugs than other five fuzzers.
% On MAGMA, \tool{} exposes six more CVEs than the best of the five fuzzers.
% Furthermore, \tool{} discovers 11 new bugs, 3 of which are confirmed by vendors.



We summarize our contributions as follows.
\begin{itemize}
    \item Based on Shapley analysis, we perform empirical experiments to study the contributions of bytes in terms of code discovery. The results indicate that the repeated mutation of a small portion of positions can improve the efficiency of code discovery. We ascertain that the main derivative for the Shapley results is that a byte may be related to multiple path constraints.
    % two derivatives for the SHAP results are the direct and indirect coupling of path constraints. 
  
    \item We formally formulate byte selection as Shapley analysis and transform the calculation of Shapley values into a form that can be updated gradually during fuzzing. We propose \tool{}, which uses Shapley values to guide byte selection and presents a contextual multi-armed bandit approach to optimize Shapley-guided byte selection.
    
    % We propose \tool{}, which uses a family system to share the positions of inputs among seeds in a family. The shared positions can be grouped to resolve directly and indirectly coupled path constraints.
    % \item We present a contextual multi-armed bandit approach to optimize the selection of shared positions, to further improve the effectiveness of shared positions in discovering new code.
    
    \item We implement \tool{} based on AFL++, and evaluate it on UNIFUZZ and MAGMA platforms. The results indicate that \tool{} outperforms various state-of-the-art fuzzers in terms of edge coverage and bug discovery. 
    % We open source \tool{} at  \url{https://github.com/ShapFuzz/ShapFuzz}.
\end{itemize}







==> obsolete/intro_backup.tex <==



\section{Introduction}

% \zhu{ our keys?:
% \begin{itemize}
%     \item the combination of different path constraints result in different execution paths
%     \item an input position may be used as a path constraint in different program logics
% \end{itemize}}
% \zhu{KEY: existing solution infer a fixed group for mutation; our solution evolves the groups during fuzzing?}


Fuzzing is known as a de facto technique to detect software security issues among both academic and industrial practitioners~\cite{zhu2022roadmap}.
In the set of existing fuzzing solutions, coverage-guided greybox fuzzing (CGF) has performed remarkably well in detecting real-world bugs~\cite{ossfuzz, onefuzz, feng2021snipuzz, aflchurn}. 
This method aims to enhance code coverage so that potential bugs are disclosed in the unseen parts of the code. Existing studies have  reported many efforts to expand code coverage, including scheduling of computational resources for certain code regions~\cite{aflfast, fairfuzz, Yue2020EcoFuzz} and resolving path constraints~\cite{angora, driller, SymFuzz, qsym, dowser, matryoshka}.
While scheduling computational resources is an implicit way to expand code coverage, resolving path constraints is an explicit way to achieve the same. Since path constraints guard certain code regions, any success in passing path constraints most likely results in new code coverage. However, resolving path constraints is not a trivial task as those constraints may be quite complicated. 


% Existing solutions for resolving path constraints can be categorized into symbolic execution based solutions and inference based solutions \zhu{citations}. Symbolic execution builds formula for constraints along an execution path and uses constraint solver to generate inputs that satisfy those constraints \zhu{citations}.
Because fuzzing repeatedly tests a program, a promising solution for resolving path constraints is to infer the relationships among input bytes and mutate related bytes together in later fuzzing campaigns~\cite{greyone, ems, profuzzer, neuzz}.
For instance, some fuzzers build the relationship among input bytes if they influence the same path constraint~\cite{greyone, ems, angora, vuzzer, steelix} or construct the same data type~\cite{profuzzer, angora}.
The inference can reduce the search space of passing constraints if fuzzing combines the related bytes into groups and mutates inputs based on groups. 
For instance, mutating 12 bytes can generate $256^{12}$ different inputs while mutating 4 bytes at a time (4 bytes a group) only generates $3\times256^{4}$ different inputs. 
If a path constraint can be resolved by mutating one group, the combination of bytes can significantly improve the efficiency of code discovery. 
% Existing research builds the relationship among input bytes if they influence the same path constraint \zhu{cite; greyone, ems} or construct the same data type \zhu{cite; profuzzer}. \zhu{more fuzzers?} 


Essentially, the groups of bytes reflect the formats of inputs, which further represent the internal logic of programs. However, the existing inference solutions only reveal the shallow logic of programs. Those solutions only infer the relationships of bytes for a single path constraint at a time. Each time, the bytes related to a single path constraint are mutated, which neglects the fact that different path constraints may be heavily coupled. For example, to pass the condition $if(b == 0x123)$, we may need to figure out all the conditions that the variable $b$ depends on, such as $if(a == 0x22)\{b = 0x12\}$. In this case, it is insufficient to only mutate the bytes related to the variable $b$ for passing the path constraint. Therefore, in order to fuzz deep program logic, the inference for related bytes is required to consider the coupling of path constraints.

\begin{figure*}[t!]
\centering
\includegraphics[width=0.8\linewidth]{images/motivation.pdf}
\caption{A motivating example of direct and indirect coupling from \texttt{readelf}.}
\label{readelf_example}
\end{figure*}

In this paper, we propose \tool{}, a lightweight fuzzer, to mutate inputs considering the coupling of path constraints. \tool{} infers and groups the bytes related to the coupled path constraints based on two observations. One observation is what we call \textit{direct coupling}, where the flip of a path constraint must consider the results of other path constraints.
The exploration of directly coupled path constraints will lead to deep code in programs (exemplified in Section~\ref{sec:motivation}). Another observation is that different program logics may process the same format of inputs, indicating that different constraints are related to the same positions of inputs (we call it \textit{indirect coupling}). 
The usage of indirect coupling helps fuzzing quickly explore new code if a fuzzer only mutates the corresponding input positions (exemplified in Section~\ref{sec:motivation}).


Based on the two observations, \tool{} builds a \textit{family system} to share positions that have discovered new code coverage (observation of indirect coupling) and combine the shared positions to mutate members in the same family (observation of direct coupling).
To achieve that, the family system is required to ensure that, for any seed (\ie a retained input) in a family, the shared positions are still related to the seed's corresponding path constraints.
To satisfy the requirement, a family is built if seeds in the family are obtained by mutating a original seed without changing its length.
Since the meaning of each position may be changed by the trimming stage, which is performed to reduce the length of seeds, \tool{} traces the change of positions to maintain the meaning of positions. 
However, the building process of a family can only roughly satisfy the requirement. 
To improve the possibility that the selected positions for a seed are related to (unsolved) path constraints, \tool{} uses LinUCB \cite{linucb} to dynamically generate a probability distribution for the selection of positions. \zhu{a bit more about LinUCB; What problem can LinUCB solve? How to solve? what's the benefit of using LinUCB?}
Note that, the positions selected by LinUCB may be related to more than one path constraint so that the directly coupled path constraints can be fuzzed.


We implemented \tool{} based on AFL++, and evaluated it on two third-party platforms, including 1) UNIFUZZ, which contains real-world programs, and 2) MAGMA, which provides a series of real-world programs with known bugs.
On UNIFUZZ, we evaluated \tool{}-related fuzzers (\ie \tool{} and \tool{}-Redqueen) and 5 existing modes of AFL++ on 16 target programs.
The results show that, in terms of coverage discovery, \tool{}-related fuzzers perform better than other fuzzers after running 1/3/6/12/24 hours.
Additionally, \tool{}-Redqueen discovered 11 more vulnerabilities than the best mode in AFL++.
On MAGMA, we evaluated \tool{}-related fuzzers and 5 widely-used mutation-based fuzzers (AFL, AFLFast, FairFuzz, MOPT and AFL++) on 20 programs. \tool{} exposed 6 more CVEs than the best of the 5 comparing fuzzers.
Our experiments also demonstrate that most of our inferred positions can discover new code coverage, which excludes the first time a position is retained.




We summarize our contributions as follows. \todo{revise?}
\begin{itemize}
    \item We observe that input bytes can be grouped based on direct coupling and indirect coupling of path constraints. We then propose \tool{}, which uses a family system to share positions of inputs among seeds in a family. The shared positions can be grouped to resolve directly and indirectly coupled path constraints.
    % We propose a family system to achieve the integration of the pilot stage and havoc stage. Based on semantic consistency, the seeds are divided into multiple families, which allows different seeds in the same family to share the structure-related positions identified by themselves to improve the efficiency of fuzzing.
    \item To improve the effectiveness of shared positions in discovering new code coverage, \tool{} uses LinUCB to schedule the combination of shared positions.
    % We propose a Family-Based Mutation Mode, which uses the LinUCB model to identify valuable positions within the family's shared pool for each seed to guide the mutation direction.
    \item We implement \tool{} based on AFL++, and evaluate it based on the platforms UNIFUZZ and MAGMA. The results indicate that \tool{} outperforms various state-of-the-art fuzzers in terms of edge coverage and bug discovery.
\end{itemize}



% \zkp{

% Based on the two observations, there are two main challenges here to leveraging the coupling of path constraints.
% \begin{itemize}
%   \item [1)]
%   Challenge I: How to infer the related bytes of a single path constraint in a more lightweight method?
%   \item [2)] 
%   Challenge II: How to group bytes based on the relations between path constraints?
% \end{itemize}

% To overcome Challenge I, instead of utilizing an additional pilot stage to analyze each position like inference-based fuzzer, Pozzer integrates the pilot stage into the havoc stage and directly extracts useful data from the fuzzing process. 
% Specifically, \tool{} collects mutation information from those mutations that flip path constraints to analyze the related positions.
% Thus, the analysis time of Pozzer is not affected by seed length. 
% Since a constraint can be passed by multiple seeds, a constraint may be inferred repeatedly.
% As all seeds share a constraint space, different seeds can share the related positions they found for the same constraint.
% However, there are many factors in the fuzzing process that may cause alignment problems between seeds, such as different initial seed structures, trimming and other operations.
% To solve this problem, establishing a position mapping between seeds is necessary.
% However, due to the complexity of the seed structure, it is difficult to find the semantic mapping between seeds with different structures.
% If two seeds have an inheritance relationship, they are more likely to have the same structures.
% Therefore, we propose a \textbf{family system} based on the inheritance relationship. More specifically, we use the initial seed to establish a family, and the offspring seeds obtained from its mutation will be added to the family.
% In a family, we use a \textit{semantic tracking algorithm} to establish the semantic mapping between seeds within the family.
% Each seed has an independent relative position space, and the position inside the seed is called the \textit{relative position}.
% To achieve semantic mapping, we need to map the relative position of each seed to the same absolute position space so that alignment can be achieved.
% Thus, each family builds an absolute position space based on the ancestor seed who constructs this family.
% The semantic tracking algorithm maps the relative position in the seed to the absolute position space based on the position mapping between seeds during seed generation, which achieves semantic mapping.
% % In a family, we use a \textit{semantic tracking algorithm} and \textit{absolute position space mechanism} to establish the semantic mapping between seeds within the family.
% % 1) \textbf{Semantic tracking algorithm}. The semantic tracking algorithm tracks position mapping between seeds during seed generation.
% % 2) \textbf{Absolute position space mechanism.} Each seed has an independent relative position space, and the position inside the seed is called the \textit{relative position}.
% % To achieve semantic mapping, we need to map the relative position of each seed to the same absolute position space so that alignment can be achieved.
% % Thus, each family builds an absolute position space based on the ancestor seed who constructs this family.
% % The absolute position space mechanism maps the relative position in the seed to the absolute position space based on the semantic tracking algorithm to achieve semantic mapping.
% Then, different seeds can communicate in the same absolute position space, avoiding alignment problems.
% Finally, seeds within the same family can exchange information based on semantic mapping to speed up the analysis process. 
% % To solve this problem, Pozzer proposes a \textit{family system}. 
% % The key of the family system is to maintain the \textit{semantic mapping} (i.e., find positions with the same meaning on different seeds) in inputs, where we regard the positions of inputs are more important than the values. 
% % %We define \textit{valuable positions} as positions related to all solved path constraints in a seed. 
% % %valuable positions就是所有solved path constraints的related positions的合集；因为我们得到valuable positions的前提是发现了新边，所以只能够找到solved constraints的related positions
% % To achieve semantic mapping, Pozzer first groups seeds into a family based on \textit{semantic preservation algorithm}, which tracks position mapping between seeds. 
% % Then, each family builds a \textit{absolute position space} based on the ancestor seed who constructs this family, and the position inside a seed is called \textit{relative position}.
% % Each seed can map its relative position to the absolute position space based on the semantic preservation algorithm to obtain the \textit{absolute position}.
% % Then, different seeds can communicate in the same absolute position space, avoiding alignment problems.
% % % Thus, each family maintains a \textit{shared pool} to record the absolute positions of valuable positions of each seed.
% % % Finally, the seeds in the same family can share the valuable positions based on shared pool according to semantic mapping to speed up the analysis process. 
% % Finally, seeds within the same family can exchange information based on semantic mapping to speed up the analysis process. 

% % To achieve semantic mapping, each seed can convert its internal relative position into absolute position space based on \textit{semantic preservation algorithm}, which tracks position mapping between seeds. 
% % Each seed in the family convert its internal relative position into a universal absolute position through absolute position space, so that information exchange can be achieved between different seeds.
% % Pozzer groups seeds into a family based on \textit{semantic preservation algorithm}, which tracks position mapping between seeds. 
% % specific \textit{absolute scales}. All seeds in the family can 
% % By establishing \textit{absolute scales}, seeds within the same family can achieve semantic mapping.
% % Specifically, each family owns a specific \textit{absolute scales}
% % Each family maintains a \textit{shared pool} to record valuable positions of all constraints.
% % Any seed in the family can share the valuable positions found by it or use the valuable positions found by others.
% % The key of the family system is to maintain the semantic information in inputs, where we regard the positions of inputs are more important than the values. 
% % The seeds in the same family can share the related positions of constraints based on semantic information to speed up the analysis process. 

% \zhu{efficiency->family system: 1. length of input (mutate every byte); 2. repeated inference of the same constraint.}

% To solve the problem of Challenge II, Pozzer utilizes a LinUCB model to group the positions related to constraints. 
% Given a seed, the purpose of mutation is to explore unsolved constraints around the seed.
% % To explore unsolved constraints considering the coupling of path constraints, the key is constantly flipping the related solved path constraints, that is, to mutate the related positions of the related solved constraints.
% From the analysis at Section~\ref{sec:motivation}, it can be seen that the key of exploring unsolved constraints considering the coupling of path constraints is to constantly flip the related solved path constraints, that is, to mutate the related positions of the related solved constraints.
% As the logic of real programs is complex, it is challenging to directly analyze the relationship between constraints.
% And the purpose of obtaining the path constraints relationship is grouping related positions of the related solved path constraints. 
% %Given a seed, we can group positions related to all solved path constraints as \textit{valuable positions}. 
% Thus, we can group positions directly based on the relationship between unsolved constraints and all \textit{valuable positions} (i.e., the positions related to all solved path constraints in a seed).
% %At the same time, given a seed, since the purpose of obtaining the path constraints relationship is grouping positions, we can directly find the relationship between unsolved constraints and all valuable positions to group positions.
% % Since it is challenging to directly analyze the relationship between constraints, we use the LinUCB model to continuously learn the relationship between unsolved constraints and valuable positions during the fuzzing process.
% % We group all valuable positions of solved constraints into a \textit{candidate pool}.
% To achieve this goal, Pozzer first assumes that all solved constraints are related to unsolved constraints, that is, mutate all  valuable positions.
% Then, Pozzer uses a LinUCB model to dynamically generate a distribution for valuable positions based on the fuzzing feedback, which is used to measure the relationship between the unsolved constraints and each position valuable positions, that is, to indirectly measure the relationship between the unsolved constraints and solved constraints.
% Finally, Pozzer constructs byte groups based on the distribution.
% }



==> obsolete/motivation-0.1.tex <==

\section{Motivation}
\subsection{Why model fuzzing campaigns as transfer learning?}

Fuzzing campaigns has been modeled as multiple different models from different perspectives. AFLFast prefers assigning more computing resources to the paths that are exercised with low frequency via formulating fuzzing campaigns as a Markov chain. EcoFuzz models the process of seeds schedule as a variant of the Adversarial Multi-Armed Bandit Model problem, which improves the efficiency of edge coverage discovery. But both of them do not consider the relationship between different processes (i.e. the exploration of multiple seeds) at the byte level. 

It is difficult to explain the reason in a short space why we model fuzzing campaigns as transfer learning because a learning process has too many factors that need to be considered. To be simplified, we use cmps to illustrate the motivation of TransferFuzz since cmps directly affect the branch behavior. More specifically, we redefine the learning process as the process of resolving a cmp constraint here. And the most efficient method of exploring the branches of a cmp is to focus on mutating the related bytes of it.

In order to utilize the relationship between different learning processes, we assume it is common that different cmps have part of the same related bytes.  Based on this assumption, it will be more efficient to satisfy the constraint of the cmps with unexplored branches via leveraging the related bytes of other cmps. And we can save a lot of time by inferring the related bytes for target cmps. 
Thus, we need to prove the above assumption. We perform some experiments to provide some insights. 

\subsubsection{How likely is a byte being related to multiple cmps at the same time?}

\textbf{Experiment Settings.}
First, we run AFL-test on a single seed for one hour to collect an inital seed corpus.
Second, we perform FTI on each input to analyze the related position of each cmp that has been exercised. More specially, for each input, we mutate each byte to all other 255 values, and then obverse the value of target cmps weather changed. If mutating the value of position i and the value of cmp j have been changed, we believe that position i is related to cmp j. 
Third, we count a byte is related to how many cmps are at the same time.
Finally, we select five programs and each program is provided with multiple initial seeds. We analyze the average data across multiple initial seeds to draw a figure shown in fig.X.

\textbf{Result.}
Based on the results in fig.X, most of the bytes are related to multiple cmps at the same time.
For instance, X bytes are related to 32~64 cmps at the same time in XX.

\textbf{Conclusion}
From the experiment, we can find that if a byte is related to one cmp, it has a high possibility to be related to multiple other different cmps.

\subsubsection{How often does position reusing happen?}
\textbf{Experiment Settings.}
First, we construct AFL-test by expecting the trimming, insert/delete mutators, and splicing to ensure that the meanings of the same position in different inputs are the same.
Second, we record the positions that have been mutated for each mutation. 
If new paths are found by this mutated input, we recover each mutated position to its initial value one by one. After recovering position i, we put the recovered input into the target program to execute. If the same new path still can be found, we maintain this recovery and recover the next mutated position. Otherwise, we abort this recovery, reset its value, record this position and then recover the next mutated position. 
For example, as shown in fig x, assume a seed has ten bytes, the first and the second bytes have been mutated and this mutated input found a new path. Note that the initial value of these two bytes is 0 and 1. After mutation,  these two bytes are set to 3 and 4. First, we recover the value of the first byte to 0. We execute this recovered input and find that the same new path still can be found. Thus, we maintain the value of the first byte as 0. Second, we recover the value of the second byte to 1. But we can not find the same path by executing this recovered input. Finally, we believe that the second byte is related to the discovery of this new path and record of this position.

If a path is found and all the mutated positions can not be recovered, we believe that these positions are related to the discovery of this path. Then, we record these positions in our feature vector. 
If another path is found and its related positions after recovering have been added to the feature vector, we believe this is position reusing.
In order to indicate the ratio of position reusing among all the positions stored in the feature vector, we perform the following experiments.
Thus, we not only record the positions related to path discovery into the feature vector but also record how many paths discovery are related to a position at the same time, i.e., position reusing.

We perform this experiment on 7 programs for X hours. And each program has a single initial seed to ensure the same position in different inputs has the same meaning. 

\textbf{Conclusion.}
If a byte is related to a path discovery, it is likely to be related to the discovery of other multiple paths. For instance, X bytes is related to 32~64 paths discovery at the same time in XX. Thus, the phenomenon of position reusing is common in most programs.

However, the state-of-the-art fuzzers ignore these two phenomena and simply believe that the exploration of different seeds is independent of each other. If the common features can be extracted among multiple learning processes, the fuzzing campaigns could be far more efficient. 

\subsection{Why we can not just abort the strategies in the above four challenges?}

For the above challenge I to III, the most intuitive solution is not to use the corresponding strategy. For example, if we do not use length mutators, we will not be haunted by challenge two. However, these strategies are important for fuzzing. For the challenge I, it is impossible that only use a single seed when fuzzing real-world programs. In OSS-Fuzz, almost all programs have multiple initial seeds used for fuzzing. For challenges II and III, we perform a compared experiment to indicate the significance of these two operations. We construct AFL-length without the use of the length mutators and construct AFL-trim without the use of trimming. As shown in fig 6, we will miss a lot of edge coverage if we do not use these strategies. Thus, we can not just simply abort these strategies to overcome the above challenges II and III. 

To solve the effect of multiple initial seeds in challenge 1, we treat an initial seed and the inputs generated from it without using length mutators into one race. 
Thus, the fuzzing campaign is divided into multiple child campaigns just like multiprocessing.
In AFL-based fuzzers, most of them will maintain a virgin\_bits to record which edges have been exercised. In our method, we also maintain virgin\_bits as a global variable. The difference is that each race extra maintains a local virgin\_bits which can only be accessed by inputs belonging to this race, which is similar to multiprocessing, i.e., child processes can access global variables and their private variables. 
Additionally, each race also maintains its transfer feature vector to record which positions have been mutated and found new paths successfully. Thus, the challenge I has been overcome. 

For challenges II, we record the length mutators used when a mutated input is generated. If a new path is found, we try to withdraw all length mutators and 
get a withdrawn input. If the withdrawn still can find the new path, we replace the original mutated input with the withdrawn input. Thus, we remove the influence of length mutators. Otherwise, we just save the init mutated input normally.

The key point to overcoming challenges III is to maintain the relative position with reference to the initial seed. Each seed that discovers a new path or new edge should maintain a map\_vector to record the relative position with reference to the initial seed of its race. Thus, though a seed has been trimmed, we are still able to indicate that each position in this seed is corresponding to which position in the initial seed. 

For challenges IV, the key point is also the withdraw operation. For each mutated input that found a new path, we compare the mutated input and its parent seed byte by byte and try to reset each byte to its initial value. Note that mutated input is generated from the parent seed. If the new path still can be found, we just reset the next byte. Otherwise, we recover its value in mutated input. After trying to reset all bytes, we can obtain the minimal mutation set to find the new path. each mutation in this set is necessary for the discovery of the new path.

==> obsolete/motivation-0.2.tex <==

\section{MOTIVAION}


\subsection{Multiple Position Inference System}

The dataset generated from pilot stage only contains the mutation information that caused the execution states to be changed.
As there are too much mutation information causing execution states changed, we can not collect all those mutation information to form a new dataset, which may cause data explosion problems.
Therefore, to extract more valuable data, we only consider those mutations that find new edge. 
After our experiments, using the granularity of edge can obtain enough data for further analysis.







We can infer which positions may be structure fields from the mutation information that caused the execution states to be changed.
However, there are too much mutation information causing changes in execution states.
To extract more valuable data, we only consider those mutations that find new coverage(e.g., new edge and new cmps' value).

During the havoc stage, multiple bytes are often selected for a mutation, and not all bytes are necessary for new coverage.
Therefore, we cannot directly use these data to replace the dataset of the pilot stage.
Otherwise, there will be a lot of redundancy.

Essentially, if we can remove those mutated positions that are irrelevant to the discovery of new coverage, leaving only the \textbf{necessary} mutated positions, we can achieve mutating multiple bytes at the same time without causing an over-taint problem. The \textbf{necessary} means that a new coverage cannot be found without mutating one position. 
So we can get the following conclusion: if a mutated input mutates multiple \textbf{necessary} positions and finds a new coverage, then we believe that these positions are all related to the new coverage.
Therefore, if we can de-redundant the mutation information collected during the fuzzing process, we can replace the dataset generated by the pilot stage with this mutation information.

We finally chose edge as the indicator in the choice of coverage granularity.

%只有引起execution states发生变化的突变信息中，我们才可以推断出哪些positions可能是结构字段。但是，造成execution states改变的突变信息实在太多，所以，我们认为那些发现了new coverage的突变信息是有用的。但是，由于实际的fuzzing过程中往往会选择多个bytes进行突变，并且不是所有的bytes对于new coverage而言都是必要的。所以，我们并不能直接用这些数据去替换pilot stage的数据集；否则，会出现大量的冗余现象。
%实质上，如果我们能够将那些与新边/新的cmp值的发现无关的mutated positions去除掉只留下“必要”的mutated positions，我们就可以实现mutate multiple bytes at the same time而不会造成over-taint。这里的“必要”是指，少突变一个position都无法发现新边/新的cmp值。因此我们可以得到以下结论：如果某个mutated input突变了多个“必要”的positions并发现了new coverage（eg：新边/新的cmp值），那么我们就可以认为这些positions都和new coverage的发现相关。所以，如果我们能够将fuzzing过程中收集到的突变信息去冗余的话，我们就可以用这些突变信息替换pilot stage收集到的数据集。在coverage粒度的选择上，我们最终选择了edge作为indicator。

\subsection{Challenge II}

However, the above scheme assumes that the number of mutations for each seed is sufficient. In fact, the distribution of energy among the seeds is very uneven, with some seeds being allocated a large amount of energy and some seeds being able to mutate only a few hundred times.

In order to solve the problem of insufficient data for some seeds, we propose a family system to coarsely divide all seeds into multiple families based on inheritance relationship. In each family, all seeds coarsely maintain semantic consistency. \textbf{Semantic consistency} means that the same position on different seeds have similar meanings.
Then, each family maintains a shared pool for recording positions that may be structural fields on all seeds within the family.
Moreover, any seed can also use the position extracted from other seeds in the shared pool.
Therefore, for seeds with less energy allocated in the family, it can also directly access the shared pool to know which positions may be located in the structure field to mutate them. For different seeds within the family, they can communicate the positions of the structural fields they found, thereby reducing the required analysis resources.

However, since the mutation process of fuzzing is random, a completely different new seed will likely appear during the mutation process. Therefore, the positions recorded in the shared pool no longer apply to these seeds. To this end, we introduce the LinUCB model to determine the probability that each position in the shared pool is a structural field on each seed. Specifically, within a family, we regard each position in the shared pool as an arm and seeds as a user. At the same time, we extract the path feature vector of each seed based on the path feature generation algorithm to characterize its path feature as the user's attribute. Finally, the rarity of the path taken after the mutation is used as the reward. Based on the above definitions, we build a LinUCB model to adaptively determine the relationship between all positions in the pool and each seed.

%然而，上述方案依赖于突变次数足够的假设之下。实际上，各个种子之间的能量分配很不均匀，部分种子会被分配大量的能量，而部分种子却仅能够突变数百次。为了解决部分种子的数据量不足的问题，我们提出了基于语义一致性原则的聚类算法。语义一致性原则是指在不同的种子上的同一个位置的意义具有相似的意义。然后，我们基于语义一致性原则将fuzzing过程中的所有的seeds划分为多个族群，每个族群内部维护着语义一致性。在每个族群内部维护一个shared pool，记录该种群内所有种子上可能为结构字段的positions。由于语义一致性的存在，在同一个种群内，任意种子识别出来的结构字段的位置会被加入到shared pool，同时也可以使用shared pool由其他种子上提取出来的结构字段的位置信息。所以，对于种群内所分配能量较少的种子，它也可以直接访问shared pool，知道自己的哪些bytes可能位于结构字段，从而对它们重点进行突变。对于族群内的不同seeds，他们之间可以交流各自发现的结构字段所在的positions，从而减少所需要的分析资源。

%但是，由于fuzzing的突变过程是不确定性的，在突变过程中很有可能出现一个完全不一样的新种子。所以，shared pool中记录的positions对这些seeds就不再适用。为此，我们引入cMBA model来判断shared pool中的每个position在各个seed上为结构字段的概率。具体的，在一个种群内，我们将shared pool中的各个position视为一个arm，将seeds视为user。同时，我们基于路径特征生成算法提取出各个种子的路径特征向量以表征其路径特征作为user的属性。最后，将突变后所走的路径的稀有程度作为reward。基于上述定义，我们构建cMBA模型来实现自适应地判断pool中所有positions与各个seeds之间的关系。

\subsection{Challenge III}

Finally, although we sacrifice some precision while implementing lightweight implementation, we can still cover most of the most important bytes in a short time.
Since our method does not actively analyze the meaning of each byte like the inference-based method, there may be a phenomenon of missing some bytes with less impact (that is, bytes that are difficult to cause execution states change by mutation).
Although the probability of the above phenomenon in the inference-based method will decrease with the increase of the number of tests for each byte in the pilot stage, it will cause a greater time consumption problem.
At the same time, these bytes in the new coverage is often redundant. For example, in Greyone, if we explore if($a > 10000$), where a is of type u32 and the initial seed yields a value of 0.
Although Greyone can identify all the relevant bytes of a, only the high-order bytes are useful for the exploration of the edge, the low-order bytes are redundant, and the mutation of the low-order bytes will not make the discovery of a new edge.
Second, we use the 48h data for SHAP analysis in the section X experiment to get the ground truth of the important bytes. Finally, we found that our method can cover most of the important bytes within one hour.

%最后，虽然我们在轻量化实现的同时牺牲了部分的精度，但是我们仍然可以在短时间内覆盖到大部分的important bytes。由于我们的方法并没有像inference-based的方法一样去主动分析每一个byte的含义，所以对于部分影响较小的bytes（即，突变难以造成路径变化的bytes），可能会出现missing的现象。虽然inference-based的方法出现上述现象的概率会随着pilot阶段对每个byte测试次数的增加而降低，但是会造成更大的时间消耗。同时，这部分bytes在new coverage的发现往往是冗余的。例如，在Greyone中，如果对if(a > 10000)进行探索，其中，a是u32类型，并且初始种子所得到的a的值为0。虽然Greyone可以识别出a的所有相关bytes，但是，只有位于高位的bytes对于该边的探索而言是有用的，低位的bytes是冗余的，低位bytes的突变并不会使得new edge的发现。其次，我们在section X实验中利用48h的数据进行SHAP analysis，得到important bytes的ground truth。最后，我们发现我们的方法可以在1h内就覆盖到大部分的important bytes。


==> obsolete/motivation-1.0.tex <==

% Our propose: The integration of pilot stage and havoc stage
% Our Challenges:
%   Challenge I
%   Challenge II
%   Challenge III
%       Family System
%       Family-Based Mutation Mode
%           Maintain shared pool
%           Family-Based Mutation Strategy
%
%


\section{Motivation} \label{sec:motivation}

% \zhu{show the motivations of your design.}
% \subsection{Example}
% \lstdefinestyle{mystyle}{
%   language=C,
%   backgroundcolor=\color{white}, commentstyle=\color{codegreen},
%   keywordstyle=\color{blue}, %\color{magenta},
%   numberstyle=\tiny\color{codegray},
%   stringstyle=\color{codepurple},
%   basicstyle=\ttfamily\footnotesize,
%   breakatwhitespace=false,         
%   breaklines=true,                 
%   captionpos=b,     
%   frame=single,
%   keepspaces=true,                 
%   numbers=left,                    
%   numbersep=5pt,                  
%   showspaces=false,                
%   showstringspaces=false,
%   showtabs=false,                  
%   tabsize=2
% }

% \subsection{Indirect relation}
% \begin{lstlisting}[style = mystyle, caption={Code snippet extracted from \texttt{readelf}}, label={Indirect}, float=t!]  
% static bool process_object(Filedata* filedata){
%     ...
%     if(!process_relocs(filedata))
%         res = false;
%     ...
%     if(!process_version_sections(filedata))
%         res = false;
%     ...
%     if (!process_section_contents (filedata))
%         res = false;
% }
% static bool process_relocs(Filedata* filedata){
%     ...
%     if(do_using_dynamic){...}
%     else{
%         ...
%         if(section->sh_type != SHT_RELA
%           && section->sh_type != SHT_REL
%           && section->sh_type != SHT_RELR){...}
%         ...
%     }
%     return true;
% }
% static bool process_version_sections(Filedata* filedata){
%     ...
%     switch(section->sh_type){
%         case SHT_GNU_verdef:{...}
%         case SHT_GNU_verneed:{...}
%         ...
%     }
%     ...
% }
% static bool process_section_contents (Filedata * filedata){
%     bool res = true;
%     if(! do_dump) return true;
%     ...
%     if(dump & HEX_DUMP){...; res = false;}
%     if(dump & RELOC_DUMP){...; res = false;}
%     ...
%     return res;
% }
% \end{lstlisting}



% \zhu{change contents if Figure~\ref{readelf_example} is changed. Link lines to the figure.}

In this section, we exemplify our observation of direct and indirect coupling of path constraints, using a real-world program \texttt{readelf}.
The program \texttt{readelf} processes files with ELF format and shows the information of ELF. An ELF file is mainly composed of a series of sections, whose information is recorded and managed by the section headers. 
As shown in Figure~\ref{readelf_example}, \texttt{readelf} processes ELF files via a sequence of tasks. For example, to process objects, \texttt{readelf} will execute the sequence of functions \texttt{process\_relocs()}, \texttt{process\_version\_sections()}, and \texttt{process\_section\_contents()}.


\textit{Direct Coupling.} The direct coupling indicates the direct influence among different path constraints along the same execution path. In Figure~\ref{readelf_example}, the path constraint in line 5 is defined by the function \texttt{process\_section\_contents()}, whose boolean output is determined by the constraints of lines 16, 17 and 18. That is, the constraint in line 5 is determined by three other constraints. To make the condition in line 5 to be \textit{true} (\ie the value of \texttt{res} in line 19 is \textit{false}), an input needs to satisfy 1) condition in line 16 is \textit{false}, and 2) one of the conditions in lines 17 and 18 is \textit{true}. This requires a fuzzer to fuzz the constraints of lines 16, 17 and 18 simultaneously. 
% Meanwhile, due to the complexity of the constraint in line 9, existing inference solutions, such as GreyOne~\cite{greyone}, have difficulty in building relationship between input bytes and the constraint. 
Therefore, a combination of bytes related to different constraints can help fuzz code lines that are guarded by complex path constraints (\ie the deep code).


\textit{Indirect Coupling.} The indirect coupling indicates that two path constraints process the same input format. For example, in Figure~\ref{readelf_example}, both the constraints of lines 10 and 23 check the value of \texttt{sh\_type}, which represents the types of sections. 
% \zhu{describe the meaning of \texttt{sh\_type}} \zkp{An ELF file is mainly composed of a series of sections, and the section's information is recorded and managed by the section header. \texttt{sh\_type} is the type of section}. 
Therefore, if a seed $S_1$ has inferred the related input positions of \texttt{sh\_type} to resolve the constraint in line 10, a fuzzer can mutate those positions in another seed $S_2$ that intends to resolve the constraint in line 23. As long as the meaning of those positions maintains the same between seeds $S_1$ and $S_2$, the fuzzer can quickly explore the \texttt{case}s in function \texttt{process\_version\_sections()}. To verify that the indirect coupling is common in programs, we analyzed the number of input positions that are related to multiple CMP instructions. We randomly selected several seeds for each program, and mutated each seed byte by byte using the method of GreyOne~\cite{greyone} to analyze the positions related to CMPs. GreyOne determines a CMP-related byte if change of the byte can lead to the change of values in a CMP. The results are shown in Figure~\ref{CMPs}, which indicates that most positions are related to multiple CMPs and some positions are even related to more than 256 CMPs. 
Therefore, to boot the efficiency of fuzzing, a fuzzer can mutate positions that have discovered new coverage in other execution paths.




% \textbf{Scene Description.}
% An ELF file is mainly composed of a series of sections, and the section's information is recorded and managed by the section header. 
% Listing~\ref{readelf_example} is extracted from $readelf$, a program used to view file information in ELF format. During the processing of ELF files by readelf, the following tasks need to be completed in order: Process the reloc section, display the contents of the version sections, and so on. Among them, each task is implemented by a corresponding sub-function.
% % However, within these sub-functions, it is necessary to access the type information of each section to select the corresponding program logic for processing.


% \textbf{Direct Relation.}
% In real programs, it is very common that the value of the path constraint is directly determined by the return value of a function inside it, such as line 9. The state of line 9 is determined by the return value of \textit{process\_section\_contents}. If the inner function is discrete, it is difficult for inference methods to find their related positions in the pilot stage. This is because the mutation of a single position is difficult to cause the value of the discrete function to change. 

% However, if we try combine different path constraints, we may be able to solve the constraint of line 9. More specifically, line 35, 37, 38 are related to the return value of \textit{process\_section\_contents}. Suppose the initial seed make \textit{process\_section\_contents} return directly at line 35 without being able to explore to line 10. If we want \textit{process\_section\_contents} to return false, then we need to make the state of line 35 false and one of lines 37 and 38 to be true. This requires us to combine the constraints of line 35, 37, 38 at the same time, and mutate their related positions to achieve this.


% \textbf{Indirect Relation.}
% The relations of constraints between two different paths can be divided into two parts: 1) shared constraints, the constraints shared by two paths; 2) path-specific constraints, the constraints specific to one path relative to another. As shown in Figure~\ref{readelf_example}, we select parts of the code from realelf to illustrate both cases. Given seeds $A$ and $B$, the code line sequence passed by seed $A$ is:$[3->12->14->22->6->24]$, and the code line sequence passed by seed $B$ is:$[3->12->15->22->6->24]$. For code lines $26\sim 30$, it is both passed by two paths, so it is shared constraint. For code lines $15\sim 21$, they are only passed by seed B, so they are path-specific constraints.

% For shared path constraints, it is easy to understand that different paths share similar valuable positions. For path-specific constraints, they may share valuable positions with other constraints. As in the Figure~\ref{readelf_example}, the valuable positions of the shared constraints $26\sim 30$ and path-specific constraints $15\sim 21$ are consistent, namely the type variable $sh\_type$ of each section. Thus, when we mutate seed B, we can directly use the valuable positions obtained in seed A to mutate, which can save analysis time and improve fuzzing efficiency.
% We also design an experiment to demonstrate the generality of the above phenomenon. We analyzed the overlap of valuable positions between path constraints on 5 programs. More specifically, we randomly select several seeds under each program, and then mutate each position one by one using the method of GreyOne~\cite{greyone} to analyze the related positions (\ie valuable positions) of each path constraint. As shown in the Figure~\ref{CMPs}, we analyze the proportion of a position associated with multiple path constraints simultaneously. As can be seen from the figure, most of the valuable positions are associated with multiple path constraints at the same time.
% Therefore, when we mutate a new seed, we can preferentially mutate the valuable positions found by other seeds to improve the fuzzing efficiency.

\begin{figure}[t!]
\includegraphics[width=0.9\linewidth]{images/motivation_cmps.png}
\caption{The number of input positions related to multiple CMPs. Most input positions are related to multiple CMPs.}
\label{CMPs}
\end{figure}




% Assume seeds A and B take two different program paths, but they both go through the two sub-functions $process\_relocs$ and $process\_version\_sections$. 
% Common path constraints. 不再需要额外的分析而直接获取valuable positions所在的位置。
% Seed-specific path constraints. 如果我们能够获取path constraints之间的关系，那么就可以直接将valuable positions直接映射过去，这样就不需要额外的分析了。但是，我并没有寻找the relations between path constraints的部分。
% 思路：
%   - path constraints之间存在relation，但是existing fuzzers都忽略了这个信息 -> 如果我们可以获取并利用好relation的相关信息，就可以提高fuzzing效率
%   - 但是，获取path constraints之间的relation非常困难，不过，这提供了一个优化的方向：也就是在对一个new seed突变时，利用之前提取出来的valuable positions进行加速。
%   - 所以，对不同cmps共享相关bytes的普遍性情况进行分析 -> 结果证明时普遍的，所以上述的优化方向可行
% 对于direct relation：反复突变之前的path constraints来寻找new edges
% 对于indirect relation：在处理new path constraint时，优先使用从其他path constraints上提取出来的valuable positions；但是，大部分的path constraints直接是不存在indirect relation关系的，所以，我们用LinUCB模型在突变过程中根据反馈动态调整各个path constraints的valuable positions的被使用概率
% in a different path, the constraint-related position is still related to path constraint
% an input position may be used by different path constraints in different program logics
% in path A, position a is related to constraint; then in path B, we hope the position a is still related to constraint.

% the constraints' relations between two paths可以分为两部分：1）shared path constraints；2）path-specific constraints
% 对于shared path constraints而言，不同的path共享相似的valuable positions是很容易理解的
% 对于path-specific constraints而言，举例说明该情况，并用“不同cmps共享相关bytes”的统计实验来说明上述情况的普遍性
% 所以说，我们在对一条new path进行突变时，可以优先访问并突变其他path上的valuable positions，来提高fuzzing的效率

% 对于Inference-based methods来说，每个种子都需要重新分析一次

% \textbf{Our idea.}


% \subsection{Direct relation}
% \begin{lstlisting}[style = mystyle, caption={Direct relation}, label={Direct}, float=t!]  
% //a is realted to input[0:1], b is realted to input[2:3]
% void test(u16 a, u16 b){
%     u8 c, d;
%     if(a == 0){c = 1;}
%     else{c = 0;}
%     if(b == 0){d = 1;}
%     else{d = 0;}
%     ...
%     if(c*d == 1){...}
%     else if(c*d == 0){...}
% }
% \end{lstlisting}
% \begin{lstlisting}[style = mystyle, caption={Code snippet extracted from $objdump$}, label={Direct}, float=t!]  
% static void objdump_print_addr (bfd_vma vma,
% 		    struct disassemble_info *inf,
% 		    bool skip_zeroes){
%     bool skip_find = false;
%     ...
%     if(aux->reloc != NULL && ...)
%     {
%       ...
%       if(bfd_is_und_section(...))
%     	    skip_find = true;
%     }
%     if(!skip_find)
%         sym = find_symbol_for_address(vma, ...);
%     objdump_print_addr_with_sym(aux->abfd, ...);
% }
% \end{lstlisting}



% Given a initial seed $s$, and the code line sequence passed by it is:[6->12->13->14]. Assume the edge [12,14] is our exploration target. To explore the edge [12,14], we have to 


% Listing \ref{Direct} is an example of a direct relation between path constraints. Assume line 7 is our exploration target. Line 7 is not directly related to any bytes, and the result of line 4 determines its result. If the result of line 4 is $True$, the input will flow into line 7. Otherwise, the input will flow into line 8.

% \textbf{Inference-based method.}
% Suppose the first byte and the second byte in the initial seed are 1 and 1, and it takes the path of line 5. In the pilot stage of inference-based methods, only a byte will be mutated in a mutation, which leads to all mutated inputs flowing into line 5. Thus, they can not find any position related to line 7 in the pilot stage. Thus, they can not explore line 7 because of ignoring the relation between line 7 and line 4.

% \textbf{Our idea.} If we try the combination of different path constraints during mutation, it is possible to discover new edges that are difficult to discover by inference-based methods. For example, if we mutate to try to flip the result in line 4 (i.e., mutate variable $a$), then we can successfully explore line 7.
% 并没有获取过constraints relation


==> obsolete/motivation-2.0.tex <==


\section{Motivation} \label{sec:motivation}

In this section, we first use SHAP to analyze the contribution of byte positions in terms of edge coverage. 
Then, we exemplify the direct and indirect coupling of path constraints, using a real-world program \texttt{readelf}. 


\paragraph{Explainability Analysis.} 

Shapley Value is a post-hoc interpretation method for blackbox models. Its core idea is to calculate the average marginal contribution of a feature value across all possible combinations of feature values, to interpret the blackbox model.
% The SHAP analysis is a post-hoc interpretation method for blackbox models \cite{shap, lundberg2017unified}.
% Its core idea is to calculate the Shapley Value of each feature, \ie the average marginal contribution of a feature value across all possible combinations of feature values, to interpret the blackbox model.
For a single sample, the Shapley Value calculated for each feature can be interpreted as how that feature contributes to the predicted value of the model.
% Each mutation in the fuzzing process can be regarded as a sample, the mutated positions as the features, the number of new discovered edges as the output, and the execution of the target program as the black box model.
% Therefore, we can use SHAP analysis to calculate the number of new edges contributed by each byte position.
% \zkp{SHAP analysis belongs to the method of post-hoc interpretation of models \cite{shap, lundberg2017unified}.
% Its core idea is to calculate the Shapley Value of each feature, \ie the average marginal contribution of the feature values across all possible combinations of feature values, to interpret the black box model.
% For a single sample, the Shapley Value calculated for each feature variable can be interpreted as how that feature affects the predicted value of the model.
% Each mutation in the fuzzing process can be considered as a sample, the mutated positions are the features, the number of new edges found is the output, and the execution of the target program can be considered as a black box model.
% Thus, We can use SHAP analysis to explore how many new edges are contributed by each mutated position.}

\zkp{
Given an N-dimensional sample and a prediction function $val(*)$ corresponding to a black-box model, We want to calculate the contribution $\phi_{j}$ of the $j$th feature $x_{j}$ of this sample. 
Suppose $S$ is a feature subset excluding $x_{j}$, i.e., $S \subseteq\left(x_{1}, \ldots x_{M}\right) \backslash x_{j}$.
Following Lloyd S. Shapley~\cite{Shapley}, the formula for calculating the contribution $\phi_{j} $ is:

\begin{equation} \label{equ:shapely}
    \phi_{j}=\sum_{S \subseteq\left(x_{1}, \ldots x_{M}\right) \backslash x_{j}} \frac{|S| !(M-|S|-1) !}{M !}\left(val\left(S \cup x_{j}\right)-val(S)\right)
\end{equation}

Among them, $val\left(S \cup x_{j}\right)-val(S)$ is the marginal contribution of feature $x_{j}$ on feature subset $S$, that is, the influence of feature $x_{j}$ on the predicted value of the model.
The above formula just calculates the shapely values of features under a single sample. Suppose we want to analyze the feature importance of the model under multiple samples. In that case, we need to calculate the weighted average of the shapely values of the target feature under all samples.
}

\zkp{To quantify the contribution of each position to edge discovery,}
% To perform the SHAP analysis, 
we used AFL++ to run fuzzing experiments with a set of diversified seed inputs for 48 hours. \zkp{Each fuzzing experiment is only performed on a single initial seed.}
Note that the byte positions are relative to seeds. A same position may have different meanings in different seeds of different lengths, so we removed the mutations that would change the length of seeds during the fuzzing experiments. 
% \chao{It seems only test cases of a fixed length will be evaluated. Therefore, the result highly depends on the original seeds.}\zkp{Yes, so we experimented on multiple seeds.} 
In the experiments, if mutation of some byte positions discovers new code, we iterate all the combinations of those mutated bytes, and record the new edges discovered by each combination. \zkp{For example, suppose a mutation finds new edges, and its mutated positions are \{1,3,4\}. 
We need to collect additionally how many new edges each subset \{1\}/\{3\}/\{4\}/\{1,3\}/\{1,4\}/\{3,4\} can discover.
}
Then we calculate the contribution of each position based on Equation~\ref{equ:shapely}. 
Finally, we accumulate all contributions of a position across all mutations.
The result of our analysis is the contribution of each byte position to code discovery.
% We collected data about the positions that discover new edges and the number of edges discovered by the positions. We then iterated all combinations of those positions, and recorded the number of edges discovered by each combination.
% \chao{Is "new coverage" relative to the very first seed's performance or the accumulated performance? How do you iterate all combinations in 48 hours? It seems you just simply count the co-existence between position combinations and edge coverage increment.}\zkp{"new coverage" relative to the accumulated performance.}\zhu{revised.} 
% The result of our SHAP analysis is the contribution of each byte position that discovers new edges (\eg the first position contributes to the discovery of 12 edges).
% Figure~\ref{shap_and_example} shows the results of SHAP analysis, and more results are shown in Figure~\ref{shap_appendix} in Appendix~\ref{sec:append_shap}.

\zkp{
We conduct experiments on 18 programs, including \textit{nm}, \textit{readelf}, \textit{size}, \textit{objdump}, \textit{tiff2bw}, \textit{tiffsplit} and so on.
There are also 9 types of program input, including \textit{elf}, \textit{tiff}, \textit{pdf}, \textit{text}, \textit{mp4}, \textit{flv}, \textit{wav}, \textit{jpg} and \textit{mp3}.
We repeated the experiment three times to avoid the influence of randomness.
% cflow - c
% 
}

\zkp{Due to space limitations, we only show part of the results. The remaining data will be presented in the appendix.}
As shown in Figure~\ref{shap_res}, for the positions that contribute the most (the top 30 positions) to edge discovery, almost all of them can discover new edges repeatedly. More than half of the edges are discovered after the first time a position has discovered new edges. Additionally, most edges are discovered by a small percentage of positions. Specifically, the top 5\% positions contribute to the discovery of 80.72\%, 65.05\%, 72.78\%, 83.21\%, 99.11\%, and 99.54\% edges on \texttt{nm}, \texttt{objdump}, \texttt{readelf}, \texttt{size}, \texttt{tiff2bw}, and \texttt{tiffsplit}, respectively. 

\zkp{
We also draw a scatter diagram to describe how many new edges are contributed by the top X\% positions of the shapey value.
The result is shown in the figure.
A point in the figure indicates that under a program and an initial seed, the top X\% positions of the shapey value can contribute Y\% of the new edges.
We found that under some programs, 1\% of bytes can contribute more than 80\% of new edges.

\begin{figure}[!t]
\includegraphics[width=0.95\linewidth]{images/scatter.png}
\caption{Top X\% positions of the shapey value VS Percentage of contributing new edges.}
\label{trimming}
\end{figure}
}





% \zhu{\begin{itemize}
%     \item shap to show reuse of valuable positions can still discover new coverage
%     \item we find two reasons for the result: direct and indirect coupling
% \end{itemize}}


% \zhu{SHAP analysis: while a path constraint may be related to multiple bytes, not all of them \textit{contribute the same} to the flip of the constraint. For example, in Greyone, if we explore if($a > 10000$), where $a$ is of type u32 and the initial seed yields a value of 0.
% Although Greyone can identify all the relevant bytes of a, only the high-order bytes are useful for the exploration of the edge, the low-order bytes are redundant, and the mutation of the low-order bytes will not make the discovery of a new edge.} 
% \zkp{In addition, we find that most of the edge discovery of programs is contributed by a small percentage of positions. More specifically, top 5\% positions contribute to the edge discovery of 80.72\%, 65.05\%, 72.78\%, 83.21\%, 99.11\%, and 99.54\% on \texttt{nm}, \texttt{objdump}, \texttt{readelf}, \texttt{size}, \texttt{tiff2bw}, and \texttt{tiffsplit}, respectively.}

% In this section, we exemplify our observation of direct and indirect coupling of path constraints, using a real-world program \texttt{readelf}.
% \chao{The following two reasons have nothing to do with SHAP analysis results, i.e., a small number of bytes are important and repeatedly mutating them could improve coverage.}
% \zhu{revised in the following. See if they are connected.}

\paragraph{Interpretability of the SHAP results.}
Two of the reasons for the SHAP results are the direct and indirect coupling of path constraints.
The \textit{direct coupling} means that the flipping of a path constraint has to consider the results of other path constraints in the same execution path. Therefore, repeated mutation of certain bytes can explore all the directly coupled constraints.
On the other hand, different program logic may process the same format of inputs, indicating that different constraints could be related to the same positions of different inputs (\textit{indirect coupling}).
Therefore, the mutation of the same byte positions across different seeds can discover new code along different paths.


\begin{figure*}[t!]
\includegraphics[width=\linewidth]{images/framework.png}
\caption{The Framework of \tool{}. Based on the SHAP analysis, \tool{} organizes seeds via the family system. To maximize the code discovery, CMAB is utilized to optimize the selection of byte positions. 
% \chao{Very confusing. In Section 3.2, the probability is related to position selecting, but it relates to mutation in this figure. Further, when will this probability be calculated? How does it affect the seed mutation? How does this process integrate with a general fuzzing process, i.e., how seed selection and mutation works if considering the family system and the probability-based position selection?} \zkp{revised.}
}
\label{Framework}
\end{figure*}

We exemplify the two reasons by a real-world program \texttt{readelf} in this section.
The program \texttt{readelf} processes files with ELF format and shows the information of ELF. An ELF file is mainly composed of a series of sections whose information is recorded and managed by the section headers. 
As shown in Figure~\ref{example_readelf}, \texttt{readelf} processes ELF files via a sequence of tasks. For example, to process objects, \texttt{readelf} will execute the sequence of functions \texttt{process\_relocs()}, \texttt{process\_version\_sections()}, and \texttt{process\_section\_contents()}.



\textit{Direct Coupling.} The direct coupling indicates the direct influence among different path constraints along the same execution path. In Figure~\ref{example_readelf}, the path constraint in line 5 is defined by the function \texttt{process\_section\_contents()}, whose boolean output is determined by the constraints of lines 16, 17 and 18. That is, the constraint in line 5 is determined by three other constraints. To make the condition in line 5 \textit{true} (\ie the value of \texttt{res} in line 19 is \textit{false}), an input needs to satisfy 1) condition in line 16 is \textit{false}, and 2) one of the conditions in lines 17 and 18 is \textit{true}. This requires a fuzzer to fuzz the constraints of lines 16, 17 and 18 simultaneously. 
Therefore, the repeated mutation of bytes related to a single constraint can help fuzz code lines that are guarded by complex path constraints (\ie deep code).
% \chao{This argument shows grouping is useful, but the SHAP analysis does not show related evidence.}\zhu{revised the last sentence.}


\textit{Indirect Coupling.} The indirect coupling indicates that two path constraints process the same input format. For example, in Figure~\ref{example_readelf}, both the constraints of lines 10 and 23 check the value of \texttt{sh\_type}, which represents the types of sections. 
Therefore, if a seed $S_1$ has inferred the related byte positions of \texttt{sh\_type} to resolve the constraint in line 10, a fuzzer can mutate those positions in another seed $S_2$ that intends to resolve the constraint in line 23. As long as the meaning of those positions remains the same between seeds $S_1$ and $S_2$, the fuzzer can quickly explore the \texttt{case}s in function \texttt{process\_version\_sections()}. 
% To verify that the indirect coupling is common in programs, we analyzed the number of byte positions that are related to multiple CMP instructions. We randomly selected several seeds for each program, and mutated each seed byte by byte using the method of GreyOne~\cite{greyone} to analyze the positions related to CMPs. GreyOne determines a CMP-related byte if change of the byte can lead to the change of values in a CMP. The results are shown in Figure~\ref{CMPs}, which indicates that most positions are related to multiple CMPs and some positions are even related to more than 256 CMPs. 
Therefore, to boost the efficiency of fuzzing, a fuzzer can repeatedly mutate positions that have discovered new coverage across different execution paths.
% \chao{This argument only shows position knowledge is reusable in other seeds.} \zhu{revised the last sentence.}

% \begin{figure}[t!]
% \includegraphics[width=\linewidth]{images/motivation_shap.png}
% \label{shap}
% \end{figure}



% \begin{figure}[t!]
% \includegraphics[width=0.9\linewidth]{images/motivation_cmps.png}
% \caption{The number of byte positions related to multiple CMPs. Most byte positions are related to multiple CMPs.}
% \label{CMPs}
% \end{figure}





==> obsolete/motivation-2.1.tex <==


\section{Motivation} \label{sec:motivation}

In this section, we first use Shapley Value to analyze the contribution of byte positions in terms of edge coverage. 
Then, we exemplify the direct and indirect coupling of path constraints, using a real-world program \texttt{readelf}. 


\paragraph{Explainability Analysis.} 

Shapley Value is a post-hoc interpretation method for blackbox models. Its core idea is to calculate the average marginal contribution of a feature value across all possible combinations of feature values, to interpret the blackbox model.
% The SHAP analysis is a post-hoc interpretation method for blackbox models \cite{shap, lundberg2017unified}.
% Its core idea is to calculate the Shapley Value of each feature, \ie the average marginal contribution of a feature value across all possible combinations of feature values, to interpret the blackbox model.
For a single sample, the Shapley Value calculated for each feature can be interpreted as how that feature contributes to the predicted value of the model.
% Each mutation in the fuzzing process can be regarded as a sample, the mutated positions as the features, the number of new discovered edges as the output, and the execution of the target program as the black box model.
% Therefore, we can use SHAP analysis to calculate the number of new edges contributed by each byte position.
% \zkp{SHAP analysis belongs to the method of post-hoc interpretation of models \cite{shap, lundberg2017unified}.
% Its core idea is to calculate the Shapley Value of each feature, \ie the average marginal contribution of the feature values across all possible combinations of feature values, to interpret the black box model.
% For a single sample, the Shapley Value calculated for each feature variable can be interpreted as how that feature affects the predicted value of the model.
% Each mutation in the fuzzing process can be considered as a sample, the mutated positions are the features, the number of new edges found is the output, and the execution of the target program can be considered as a black box model.
% Thus, We can use SHAP analysis to explore how many new edges are contributed by each mutated position.}

\zkp{
Given an N-dimensional sample and a prediction function $val(*)$ corresponding to a black-box model, We want to calculate the contribution $\phi_{j}$ of the $j$th feature $x_{j}$ of this sample. 
Suppose $S$ is a feature subset excluding $x_{j}$, i.e., $S \subseteq\left(x_{1}, \ldots x_{M}\right) \backslash x_{j}$.
Following Lloyd S. Shapley~\cite{Shapley}, the formula for calculating the contribution $\phi_{j} $ is:

\begin{equation} \label{equ:shapely}
    \phi_{j}=\sum_{S \subseteq\left(x_{1}, \ldots x_{M}\right) \backslash x_{j}} \frac{|S| !(M-|S|-1) !}{M !}\left(val\left(S \cup x_{j}\right)-val(S)\right)
\end{equation}

Among them, $val\left(S \cup x_{j}\right)-val(S)$ is the marginal contribution of feature $x_{j}$ on feature subset $S$, that is, the influence of feature $x_{j}$ on the predicted value of the model.
The above formula just calculates the shapely values of features under a single sample. Suppose we want to analyze the feature importance of the model under multiple samples. In that case, we need to calculate the weighted average of the shapely values of the target feature under all samples.
}

\zkp{To quantify the contribution of each position to edge discovery,}
% To perform the SHAP analysis, 
we used AFL++ to run fuzzing experiments with a set of diversified seed inputs for 48 hours. \zkp{Each fuzzing experiment is only performed on a single initial seed.}
Note that the byte positions are relative to seeds. A same position may have different meanings in different seeds of different lengths, so we removed the mutations that would change the length of seeds during the fuzzing experiments. 
% \chao{It seems only test cases of a fixed length will be evaluated. Therefore, the result highly depends on the original seeds.}\zkp{Yes, so we experimented on multiple seeds.} 
In the experiments, if mutation of some byte positions discovers new code, we iterate all the combinations of those mutated bytes, and record the new edges discovered by each combination. \zkp{For example, suppose a mutation finds new edges, and its mutated positions are \{1,3,4\}. 
We need to collect additionally how many new edges each subset \{1\}/\{3\}/\{4\}/\{1,3\}/\{1,4\}/\{3,4\} can discover.
}
Then we calculate the contribution of each position based on Equation~\ref{equ:shapely}. 
Finally, we accumulate all contributions of a position across all mutations.
The result of our analysis is the contribution of each byte position to code discovery.
% We collected data about the positions that discover new edges and the number of edges discovered by the positions. We then iterated all combinations of those positions, and recorded the number of edges discovered by each combination.
% \chao{Is "new coverage" relative to the very first seed's performance or the accumulated performance? How do you iterate all combinations in 48 hours? It seems you just simply count the co-existence between position combinations and edge coverage increment.}\zkp{"new coverage" relative to the accumulated performance.}\zhu{revised.} 
% The result of our SHAP analysis is the contribution of each byte position that discovers new edges (\eg the first position contributes to the discovery of 12 edges).
% Figure~\ref{shap_and_example} shows the results of SHAP analysis, and more results are shown in Figure~\ref{shap_appendix} in Appendix~\ref{sec:append_shap}.

\zkp{
We conduct experiments on 18 programs, including \textit{nm}, \textit{readelf}, \textit{size}, \textit{objdump}, \textit{tiff2bw}, \textit{tiffsplit} and so on.
There are also 9 types of program input, including \textit{elf}, \textit{tiff}, \textit{pdf}, \textit{text}, \textit{mp4}, \textit{flv}, \textit{wav}, \textit{jpg} and \textit{mp3}.
We repeated the experiment three times to avoid the influence of randomness.
% cflow - c
% 
}

\zkp{Due to space limitations, we only show part of the results. The remaining data will be presented in the appendix.}
As shown in Figure~\ref{shap_res}, for the positions that contribute the most (the top 30 positions) to edge discovery, almost all of them can discover new edges repeatedly. More than half of the edges are discovered after the first time a position has discovered new edges. Additionally, most edges are discovered by a small percentage of positions. Specifically, the top 5\% positions contribute to the discovery of 80.72\%, 65.05\%, 72.78\%, 83.21\%, 99.11\%, and 99.54\% edges on \texttt{nm}, \texttt{objdump}, \texttt{readelf}, \texttt{size}, \texttt{tiff2bw}, and \texttt{tiffsplit}, respectively. 

\zkp{
We also draw a scatter diagram to describe how many new edges are contributed by the top X\% positions of the shapey value.
The result is shown in the Figure~\ref{shap_scatter}.
A point in the figure indicates that under a program and an initial seed, the top X\% positions of the shapey value can contribute Y\% of the new edges.
We found that under some programs, 1\% of bytes can contribute more than 80\% of new edges.

% \begin{figure}[!t]
% \includegraphics[width=0.95\linewidth]{images/scatter.png}
% \caption{Top X\% positions of the shapey value VS Percentage of contributing new edges.}
% \label{trimming}
% \end{figure}
}





% \zhu{\begin{itemize}
%     \item shap to show reuse of valuable positions can still discover new coverage
%     \item we find two reasons for the result: direct and indirect coupling
% \end{itemize}}


% \zhu{SHAP analysis: while a path constraint may be related to multiple bytes, not all of them \textit{contribute the same} to the flip of the constraint. For example, in Greyone, if we explore if($a > 10000$), where $a$ is of type u32 and the initial seed yields a value of 0.
% Although Greyone can identify all the relevant bytes of a, only the high-order bytes are useful for the exploration of the edge, the low-order bytes are redundant, and the mutation of the low-order bytes will not make the discovery of a new edge.} 
% \zkp{In addition, we find that most of the edge discovery of programs is contributed by a small percentage of positions. More specifically, top 5\% positions contribute to the edge discovery of 80.72\%, 65.05\%, 72.78\%, 83.21\%, 99.11\%, and 99.54\% on \texttt{nm}, \texttt{objdump}, \texttt{readelf}, \texttt{size}, \texttt{tiff2bw}, and \texttt{tiffsplit}, respectively.}

% In this section, we exemplify our observation of direct and indirect coupling of path constraints, using a real-world program \texttt{readelf}.
% \chao{The following two reasons have nothing to do with SHAP analysis results, i.e., a small number of bytes are important and repeatedly mutating them could improve coverage.}
% \zhu{revised in the following. See if they are connected.}

\paragraph{Interpretability of the SHAP results.}
Two of the reasons for the SHAP results are the direct and indirect coupling of path constraints.
The \textit{direct coupling} means that the flipping of a path constraint has to consider the results of other path constraints in the same execution path. Therefore, repeated mutation of certain bytes can explore all the directly coupled constraints.
On the other hand, different program logic may process the same format of inputs, indicating that different constraints could be related to the same positions of different inputs (\textit{indirect coupling}).
Therefore, the mutation of the same byte positions across different seeds can discover new code along different paths.


\begin{figure*}[t!]
\includegraphics[width=\linewidth]{images/framework-2.0.png}
\caption{The Framework of \tool{}. Based on the SHAP analysis, \tool{} organizes seeds via the family system. To maximize the code discovery, CMAB is utilized to optimize the selection of byte positions. 
% \chao{Very confusing. In Section 3.2, the probability is related to position selecting, but it relates to mutation in this figure. Further, when will this probability be calculated? How does it affect the seed mutation? How does this process integrate with a general fuzzing process, i.e., how seed selection and mutation works if considering the family system and the probability-based position selection?} \zkp{revised.}
}
\label{Framework}
\end{figure*}

We exemplify the two reasons by a real-world program \texttt{readelf} in this section.
The program \texttt{readelf} processes files with ELF format and shows the information of ELF. An ELF file is mainly composed of a series of sections whose information is recorded and managed by the section headers. 
As shown in Figure~\ref{example_readelf}, \texttt{readelf} processes ELF files via a sequence of tasks. For example, to process objects, \texttt{readelf} will execute the sequence of functions \texttt{process\_relocs()}, \texttt{process\_version\_sections()}, and \texttt{process\_section\_contents()}.



\textit{Direct Coupling.} The direct coupling indicates the direct influence among different path constraints along the same execution path. In Figure~\ref{example_readelf}, the path constraint in line 5 is defined by the function \texttt{process\_section\_contents()}, whose boolean output is determined by the constraints of lines 16, 17 and 18. That is, the constraint in line 5 is determined by three other constraints. To make the condition in line 5 \textit{true} (\ie the value of \texttt{res} in line 19 is \textit{false}), an input needs to satisfy 1) condition in line 16 is \textit{false}, and 2) one of the conditions in lines 17 and 18 is \textit{true}. This requires a fuzzer to fuzz the constraints of lines 16, 17 and 18 simultaneously. 
Therefore, the repeated mutation of bytes related to a single constraint can help fuzz code lines that are guarded by complex path constraints (\ie deep code).
% \chao{This argument shows grouping is useful, but the SHAP analysis does not show related evidence.}\zhu{revised the last sentence.}


\textit{Indirect Coupling.} The indirect coupling indicates that two path constraints process the same input format. For example, in Figure~\ref{example_readelf}, both the constraints of lines 10 and 23 check the value of \texttt{sh\_type}, which represents the types of sections. 
Therefore, if a seed $S_1$ has inferred the related byte positions of \texttt{sh\_type} to resolve the constraint in line 10, a fuzzer can mutate those positions in another seed $S_2$ that intends to resolve the constraint in line 23. As long as the meaning of those positions remains the same between seeds $S_1$ and $S_2$, the fuzzer can quickly explore the \texttt{case}s in function \texttt{process\_version\_sections()}. 
% To verify that the indirect coupling is common in programs, we analyzed the number of byte positions that are related to multiple CMP instructions. We randomly selected several seeds for each program, and mutated each seed byte by byte using the method of GreyOne~\cite{greyone} to analyze the positions related to CMPs. GreyOne determines a CMP-related byte if change of the byte can lead to the change of values in a CMP. The results are shown in Figure~\ref{CMPs}, which indicates that most positions are related to multiple CMPs and some positions are even related to more than 256 CMPs. 
Therefore, to boost the efficiency of fuzzing, a fuzzer can repeatedly mutate positions that have discovered new coverage across different execution paths.
% \chao{This argument only shows position knowledge is reusable in other seeds.} \zhu{revised the last sentence.}

% \begin{figure}[t!]
% \includegraphics[width=\linewidth]{images/motivation_shap.png}
% \label{shap}
% \end{figure}



% \begin{figure}[t!]
% \includegraphics[width=0.9\linewidth]{images/motivation_cmps.png}
% \caption{The number of byte positions related to multiple CMPs. Most byte positions are related to multiple CMPs.}
% \label{CMPs}
% \end{figure}





==> obsolete/motivation-3.0.tex <==


\section{Motivation} \label{sec:motivation}



In this section, we first use Shapley Value to analyze the contribution of byte positions in terms of edge coverage. 
Then, we exemplify the direct and indirect coupling of path constraints, using a real-world program \texttt{readelf}. 
Finally, based on the coupling relationship between constraints, we believe that the seeds may share valuable positions, and design experiments to verify it.

\subsection{Explainability Analysis}
The relationship between position and edge discovery is complex, including direct correlation and indirect correlation.
Most existing methods only solve the direct correlation, such as GREYONE, Angora, etc.
The indirect correlation is complicated because it is affected by the CFG graph. Only some simple cases can be solved at present.
For example, Matryoshka aims to solve the problem of nested conditions.
However, nested conditions are only one case that is indirectly related.
Indirect correlations also include more complex situations.
Therefore, we approach this problem from the perspective of statistical analysis.
We regard the fuzzing process as a black box model, the input is mutated positions, and the output is the number of new edges discovered. In other words, we look for the relationship between position and edge discovery from a higher dimension.

Shapley Value is a post-hoc interpretation method for blackbox models. Its core idea is to calculate the average marginal contribution of a feature value across all possible combinations of feature values, to interpret the blackbox model. For a single sample, the Shapley Value calculated for each feature can be interpreted as how that feature contributes to the predicted value of the model. Therefore, we use Shapely Value to analyze the relationship between position and edge discovery.

Given an N-dimensional sample and a prediction function $val(*)$ corresponding to a black-box model, We want to calculate the contribution $\phi_{j}$ of the $j$th feature $x_{j}$ of this sample. 
Suppose $S$ is a feature subset excluding $x_{j}$, i.e., $S \subseteq\left(x_{1}, \ldots x_{M}\right) \backslash x_{j}$.
Following Lloyd S. Shapley~\cite{Shapley}, the formula for calculating the contribution $\phi_{j} $ is:

\begin{equation} \label{equ:shapely}
    \phi_{j}=\sum_{S \subseteq\left(x_{1}, \ldots x_{M}\right) \backslash x_{j}} \frac{|S| !(M-|S|-1) !}{M !}\left(val\left(S \cup x_{j}\right)-val(S)\right)
\end{equation}

Among them, $val\left(S \cup x_{j}\right)-val(S)$ is the marginal contribution of feature $x_{j}$ on feature subset $S$, that is, the influence of feature $x_{j}$ on the predicted value of the model.
The above formula just calculates the shapely values of features under a single sample. Suppose we want to analyze the feature importance of the model under multiple samples. In that case, we need to calculate the weighted average of the shapely values of the target feature under all samples.

To quantify the contribution of each position to edge discovery on a seed, we used AFL++ to run fuzzing experiments with a set of diversified seed inputs. 
Specifically, we continuously mutate each initial seed for 24 hours.
Note that only the initial seed is mutated in this process, and the new seeds generated by it are not mutated. During the mutation process, if mutation of some byte positions discovers new code, we iterate all the combinations of those mutated bytes, and record the new edges discovered by each combination. For example, suppose a mutation finds new edges, and its mutated positions are \{1,3,4\}. 
We need to collect additionally how many new edges each subset \{1\}/\{3\}/\{4\}/\{1,3\}/\{1,4\}/\{3,4\} can discover. Then we calculate the contribution of each position based on Equation~\ref{equ:shapely}. 
Finally, we accumulate all contributions of a position across all mutations.
The result of our analysis is the contribution of each byte position to code discovery.

We conduct experiments on 18 programs, including \textit{nm}, \textit{readelf}, \textit{size}, \textit{objdump}, \textit{tiff2bw}, \textit{tiffsplit} and so on.
There are also 9 types of program input, including \textit{elf}, \textit{tiff}, \textit{pdf}, \textit{text}, \textit{mp4}, \textit{flv}, \textit{wav}, \textit{jpg} and \textit{mp3}.
% We repeated the experiment three times to avoid the influence of randomness.
We draw a scatter diagram to describe how many new edges are contributed by the top X\% positions of the shapey value.
The result is shown in the Figure~\ref{shap_scatter}.
A point in the figure indicates that under a program and a seed, the top X\% positions of the shapey value can contribute Y\% of the new edges.
We found that under some programs, 1\% of bytes can contribute more than 80\% of new edges.
Therefore, we can draw a conclusion: The discovery of code largely depends on a small portion of byte positions.

Given a seed, we call the positions on the seed that contribute to edge discovery as valuable positions. Therefore, if we can identify valuable positions before the mutation and allocate more energy to them for mutation, the efficiency of fuzzing can be improved.
However, shapely value is a post-hoc interpretation algorithm. The valuable positions it identifies can only show that it was useful in the past but may not perform well in the future.
Therefore, we need to design a scheme to obtain the valuable positions of the seed before the mutation.

\subsection{Sharing of Valuable Position}
We found that there is a complex relationship between constraints: direct coupling and indirect coupling.
The \textit{direct coupling} means that the flipping of a path constraint has to consider the results of other path constraints in the same execution path. 
On the other hand, different program logic may process the same format of inputs, indicating that different constraints could be related to the same positions of different inputs (\textit{indirect coupling}).
The coupling relationship between constraints may cause the same valuable positions on the seed $S1$ of the path $A$ and the seed $S2$ of the path $B$, i.e., valuable positions are shared between different seeds.
Therefore, when mutating S1, if we can identify its valuable positions and map them to the seed $S2$, then we can get the valuable positions of $S2$ before mutating $S2$.

\begin{figure*}[t!]
\includegraphics[width=\linewidth]{images/framework-2.0.png}
\caption{The Framework of \tool{}. Based on the SHAP analysis, \tool{} organizes seeds via the family system. To maximize the code discovery, CMAB is utilized to optimize the selection of byte positions. 
% \chao{Very confusing. In Section 3.2, the probability is related to position selecting, but it relates to mutation in this figure. Further, when will this probability be calculated? How does it affect the seed mutation? How does this process integrate with a general fuzzing process, i.e., how seed selection and mutation works if considering the family system and the probability-based position selection?} \zkp{revised.}
}
\label{Framework}
\end{figure*}


\begin{sloppypar}
We exemplify the case of sharing valuable positions between different seeds by a real-world program \texttt{readelf} in this section.
The program \texttt{readelf} processes files with ELF format and shows the information of ELF. An ELF file is mainly composed of a series of sections whose information is recorded and managed by the section headers. 
As shown in Figure~\ref{example_readelf}, \texttt{readelf} processes ELF files via a sequence of tasks. For example, to process objects, \texttt{readelf} will execute the sequence of functions \texttt{process\_relocs()}, \texttt{process\_version\_sections()}, and \texttt{process\_section\_contents()}.
\end{sloppypar}


\textit{Direct Coupling.} The direct coupling indicates the direct influence among different path constraints along the same execution path. In Figure~\ref{example_readelf}, the path constraint in line 5 is defined by the function \texttt{process\_section\_contents()}, whose boolean output is determined by the constraints of lines 16, 17 and 18. That is, the constraint in line 5 is determined by three other constraints. To make the condition in line 5 \textit{true} (\ie the value of \texttt{res} in line 19 is \textit{false}), an input needs to satisfy 1) condition in line 16 is \textit{false}, and 2) one of the conditions in lines 17 and 18 is \textit{true}.
Assume that seed \textit{A} returns from line 16 and seed \textit{B} returns from line 19.
The valuable positions of seed \textit{A} are the related positions of line 16 and the valuable positions of seed \textit{B} include the related positions of line 16, line 17 and line 18.
Therefore, there are shared valuable positions between seed seed \textit{A} and seed \textit{B}, \ie the related positions of line 16. If we have identified the valuable positions of seed \textit{A} during the mutation process, then we can consider them to be the valuable positions of \textit{B} at the same time.
% This requires a fuzzer to fuzz the constraints of lines 16, 17 and 18 simultaneously. 
% Therefore, the repeated mutation of bytes related to a single constraint can help fuzz code lines that are guarded by complex path constraints (\ie deep code).
% \chao{This argument shows grouping is useful, but the SHAP analysis does not show related evidence.}\zhu{revised the last sentence.}

\textit{Indirect Coupling.} The indirect coupling indicates that two path constraints process the same input format. For example, in Figure~\ref{example_readelf}, both the constraints of lines 10 and 23 check the value of \texttt{sh\_type}, which represents the types of sections. 
Assume that seed \textit{A} passes line 10 and seed \textit{B} passes line 23.
Seed \textit{A} and seed \textit{B} share part of valuable positions, \ie the related positions of \texttt{sh\_type}. Thus, the valuable positions identified by seed \textit{A} can be used by seed \textit{B}.

% Therefore, if a seed $S_1$ has inferred the related byte positions of \texttt{sh\_type} to resolve the constraint in line 10, a fuzzer can mutate those positions in another seed $S_2$ that intends to resolve the constraint in line 23. As long as the meaning of those positions remains the same between seeds $S_1$ and $S_2$, the fuzzer can quickly explore the \texttt{case}s in function \texttt{process\_version\_sections()}. 
% To verify that the indirect coupling is common in programs, we analyzed the number of byte positions that are related to multiple CMP instructions. We randomly selected several seeds for each program, and mutated each seed byte by byte using the method of GreyOne~\cite{greyone} to analyze the positions related to CMPs. GreyOne determines a CMP-related byte if change of the byte can lead to the change of values in a CMP. The results are shown in Figure~\ref{CMPs}, which indicates that most positions are related to multiple CMPs and some positions are even related to more than 256 CMPs. 
% Therefore, to boost the efficiency of fuzzing, a fuzzer can repeatedly mutate positions that have discovered new coverage across different execution paths.

The above two cases prove that the sharing of valuable positions exists between seeds. Therefore, after we use Shapely Value to obtain the valuable positions of a seed, we can share it with other seeds. In this way, we can obtain the valuable positions of the seeds before the mutation, and allocate more energy to them for the mutation to improve the efficiency of fuzzing.

To prove the effectiveness of the above scheme, we also need to experiment to verify whether the sharing of valuable positions between seeds is common.
We conduct experiments on multiple seeds.
Specifically, given an initial seed, we fuzz it for 48 hours.
During the fuzzing process, we use Shapely Value to analyze the valuable positions of all seeds.
Finally, we count the overlap of the valuable positions of all seeds in the seed queue.
The result is shown in the figure.
We found that sharing valuable positions between seeds is common.
For instance, ...
Therefore, we can identify valuable positions from mutated seeds and share them with unmutated seeds, thereby improving fuzzing efficiency.



==> obsolete/motivation-3.1.tex <==


\section{Motivation} \label{sec:motivation}

The aim of coverage-guided fuzzing is to expand the code coverage, which motivates us to study the contributions of bytes in inputs in terms of discovering new coverage.
In this section, we study the contributions of bytes (or the importance of bytes) in terms of code discovery.


\paragraph{Shapley Analysis.} Since bytes are collaboratively mutated to explore code, we use the concept of Shapley value, which is a solution concept in Cooperative Game Theory, to analyze the contributions of bytes. The core idea of Shapley value is to traverse all possible combinations and calculate the average marginal contribution of a byte based on the gains of those combinations. More details are explained in Section~\ref{subsec:shapval}. 
To calculate Shapley values of bytes in a seed, we regard \textit{the number of new edges} discovered by a combination as the gain. However, a seed with length $N$ has $256^N$ possible combinations, which is too many to be tested. To obtain a relatively accurate Shapley value for a byte, we sufficiently run fuzzing with random mutation for 48 hours for \textit{a single seed}. 
Specifically, we use AFL++ to run fuzzing on 18 programs with a set of initial seeds for 48 hours. Each fuzzing experiment is only performed on a single initial seed of a program. The experiments are repeated three times to avoid the influence of randomness. The 18 programs, such as \texttt{nm}, \texttt{tiff2bw}, \texttt{flvmeta}, \texttt{imginfo}, \texttt{infotocap}, \texttt{lame}, \texttt{mp42aac} and \texttt{mp3gain}, include 9 different types of inputs that are \texttt{elf}, \texttt{tiff}, \texttt{pdf}, \texttt{text}, \texttt{mp4}, \texttt{flv}, \texttt{wav}, \texttt{jpg} and \texttt{mp3}. During fuzzing, if a mutation discovers new edges, we will recover all the subsets of related bytes and test the result. For example, if the mutation of positions $\{1,3,4\}$ discovers new edges (the gain $R$), all the subsets $\{1\}/\{3\}/\{4\}/\{1,3\}/\{1,4\}/\{3,4\}$ will be recovered, and their results will be tested. This ensures that all possible combinations related to the gain $R$ are analyzed. Notably, we remove the mutators that can change the length of a seed so that each byte does not change its relative position.



\begin{figure}[!t]
\includegraphics[width=0.9\linewidth]{images/scatter_mutate_a_seed_48h.png}
\caption{The contributions of bytes. X\% of new edges are contributed by top Y\% bytes. Each dot is a seed of a program.}
\label{shap_exp_per}
\end{figure}


\begin{figure*}[t!]
\centering
\includegraphics[width=0.85\linewidth]{images/motivation.pdf}
\caption{The reason for the results of SHAP analysis.}
\label{example_readelf}
\end{figure*}



The experiment results are shown in Figure~\ref{shap_exp_per}, where each dot means that for a program and an initial seed, X\% of new edges are contributed by top Y\% bytes. The results indicate that a small portion of bytes contribute the most to discovering new edges.
Specifically, the top 4\% positions contribute to the discovery of 97.43\%, 88.72\%, 86.10\%, 94.16\%, 87.96\%, and 100.00\% edges on \texttt{pdftotext}, \texttt{tcpdump}, \texttt{infotocap}, \texttt{strip}, \texttt{objdump}, and \texttt{flvmeta}, respectively.
On some programs, such as tiffsplit, the top 1\% bytes can contribute more than 90\% of new edges.
This also indicates that some bytes repeatedly discover new code during fuzzing.




% In this section, we first use SHAP to analyze the contribution of byte positions in terms of edge coverage. 
% Then, we exemplify the direct and indirect coupling of path constraints, using a real-world program \texttt{readelf}. 


% \paragraph{Explainability Analysis.} 

% Shapley value is a post-hoc interpretation method for blackbox models. Its core idea is to calculate the average marginal contribution of a feature value across all possible combinations of feature values, to interpret the blackbox model.
% % The SHAP analysis is a post-hoc interpretation method for blackbox models \cite{shap, lundberg2017unified}.
% % Its core idea is to calculate the Shapley value of each feature, \ie the average marginal contribution of a feature value across all possible combinations of feature values, to interpret the blackbox model.
% For a single sample, the Shapley value calculated for each feature can be interpreted as how that feature contributes to the predicted value of the model.
% % Each mutation in the fuzzing process can be regarded as a sample, the mutated positions as the features, the number of new discovered edges as the output, and the execution of the target program as the black box model.
% % Therefore, we can use SHAP analysis to calculate the number of new edges contributed by each byte position.
% % \zkp{SHAP analysis belongs to the method of post-hoc interpretation of models \cite{shap, lundberg2017unified}.
% % Its core idea is to calculate the Shapley value of each feature, \ie the average marginal contribution of the feature values across all possible combinations of feature values, to interpret the black box model.
% % For a single sample, the Shapley value calculated for each feature variable can be interpreted as how that feature affects the predicted value of the model.
% % Each mutation in the fuzzing process can be considered as a sample, the mutated positions are the features, the number of new edges found is the output, and the execution of the target program can be considered as a black box model.
% % Thus, We can use SHAP analysis to explore how many new edges are contributed by each mutated position.}

% \zkp{
% Given an N-dimensional sample and a prediction function $val(*)$ corresponding to a black-box model, We want to calculate the contribution $\phi_{j}$ of the $j$th feature $x_{j}$ of this sample. 
% Suppose $S$ is a feature subset excluding $x_{j}$, i.e., $S \subseteq\left(x_{1}, \ldots x_{M}\right) \backslash x_{j}$.
% Following Lloyd S. Shapley~\cite{Shapley}, the formula for calculating the contribution $\phi_{j} $ is:

% \begin{equation} \label{equ:shapely}
%     \phi_{j}=\sum_{S \subseteq\left(x_{1}, \ldots x_{M}\right) \backslash x_{j}} \frac{|S| !(M-|S|-1) !}{M !}\left(val\left(S \cup x_{j}\right)-val(S)\right)
% \end{equation}

% Among them, $val\left(S \cup x_{j}\right)-val(S)$ is the marginal contribution of feature $x_{j}$ on feature subset $S$, that is, the influence of feature $x_{j}$ on the predicted value of the model.
% The above formula just calculates the shapely values of features under a single sample. Suppose we want to analyze the feature importance of the model under multiple samples. In that case, we need to calculate the weighted average of the shapely values of the target feature under all samples.
% }

% \zkp{To quantify the contribution of each position to edge discovery,}
% % To perform the SHAP analysis, 
% we used AFL++ to run fuzzing experiments with a set of diversified seed inputs for 48 hours. \zkp{Each fuzzing experiment is only performed on a single initial seed.}
% Note that the byte positions are relative to seeds. A same position may have different meanings in different seeds of different lengths, so we removed the mutations that would change the length of seeds during the fuzzing experiments. 
% % \chao{It seems only test cases of a fixed length will be evaluated. Therefore, the result highly depends on the original seeds.}\zkp{Yes, so we experimented on multiple seeds.} 
% In the experiments, if mutation of some byte positions discovers new code, we iterate all the combinations of those mutated bytes, and record the new edges discovered by each combination. \zkp{For example, suppose a mutation finds new edges, and its mutated positions are \{1,3,4\}. 
% We need to collect additionally how many new edges each subset \{1\}/\{3\}/\{4\}/\{1,3\}/\{1,4\}/\{3,4\} can discover.
% }
% Then we calculate the contribution of each position based on Equation~\ref{equ:shapely}. 
% Finally, we accumulate all contributions of a position across all mutations.
% The result of our analysis is the contribution of each byte position to code discovery.
% % We collected data about the positions that discover new edges and the number of edges discovered by the positions. We then iterated all combinations of those positions, and recorded the number of edges discovered by each combination.
% % \chao{Is "new coverage" relative to the very first seed's performance or the accumulated performance? How do you iterate all combinations in 48 hours? It seems you just simply count the co-existence between position combinations and edge coverage increment.}\zkp{"new coverage" relative to the accumulated performance.}\zhu{revised.} 
% % The result of our SHAP analysis is the contribution of each byte position that discovers new edges (\eg the first position contributes to the discovery of 12 edges).
% % Figure~\ref{shap_and_example} shows the results of SHAP analysis, and more results are shown in Figure~\ref{shap_appendix} in Appendix~\ref{sec:append_shap}.

% \zkp{
% We conduct experiments on 18 programs, including \textit{nm}, \textit{readelf}, \textit{size}, \textit{objdump}, \textit{tiff2bw}, \textit{tiffsplit} and so on.
% There are also 9 types of program input, including \textit{elf}, \textit{tiff}, \textit{pdf}, \textit{text}, \textit{mp4}, \textit{flv}, \textit{wav}, \textit{jpg} and \textit{mp3}.
% We repeated the experiment three times to avoid the influence of randomness.
% % cflow - c
% % 
% }

% \zkp{Due to space limitations, we only show part of the results. The remaining data will be presented in the appendix.}
% As shown in Figure~\ref{shap_res}, for the positions that contribute the most (the top 30 positions) to edge discovery, almost all of them can discover new edges repeatedly. More than half of the edges are discovered after the first time a position has discovered new edges. Additionally, most edges are discovered by a small percentage of positions. Specifically, the top 5\% positions contribute to the discovery of 80.72\%, 65.05\%, 72.78\%, 83.21\%, 99.11\%, and 99.54\% edges on \texttt{nm}, \texttt{objdump}, \texttt{readelf}, \texttt{size}, \texttt{tiff2bw}, and \texttt{tiffsplit}, respectively. 

% \zkp{
% We also draw a scatter diagram to describe how many new edges are contributed by the top X\% positions of the shapey value.
% The result is shown in the figure.
% A point in the figure indicates that under a program and an initial seed, the top X\% positions of the shapey value can contribute Y\% of the new edges.
% We found that under some programs, 1\% of bytes can contribute more than 80\% of new edges.}





% \zhu{\begin{itemize}
%     \item shap to show reuse of valuable positions can still discover new coverage
%     \item we find two reasons for the result: direct and indirect coupling
% \end{itemize}}


% \zhu{SHAP analysis: while a path constraint may be related to multiple bytes, not all of them \textit{contribute the same} to the flip of the constraint. For example, in Greyone, if we explore if($a > 10000$), where $a$ is of type u32 and the initial seed yields a value of 0.
% Although Greyone can identify all the relevant bytes of a, only the high-order bytes are useful for the exploration of the edge, the low-order bytes are redundant, and the mutation of the low-order bytes will not make the discovery of a new edge.} 
% \zkp{In addition, we find that most of the edge discovery of programs is contributed by a small percentage of positions. More specifically, top 5\% positions contribute to the edge discovery of 80.72\%, 65.05\%, 72.78\%, 83.21\%, 99.11\%, and 99.54\% on \texttt{nm}, \texttt{objdump}, \texttt{readelf}, \texttt{size}, \texttt{tiff2bw}, and \texttt{tiffsplit}, respectively.}

% In this section, we exemplify our observation of direct and indirect coupling of path constraints, using a real-world program \texttt{readelf}.
% \chao{The following two reasons have nothing to do with SHAP analysis results, i.e., a small number of bytes are important and repeatedly mutating them could improve coverage.}
% \zhu{revised in the following. See if they are connected.}



\paragraph{Interpretability of The Shapley Results.}
In a program input, not all bytes pertain to path constraints. Even for the bytes related to the same path constraint, they contribute differently to solving the constraint. For instance, in the snippet \textit{if ((int)a > 0xeffff)}, the mutation of the two high bytes is more likely to satisfy the condition while the mutation of the two low bytes may not be able to satisfy it. 
Moreover, a byte may be related to more than one path constraint, which increases the Shapley value of the byte. From the perspective of program logic, this is the result of path coupling. 
One the one hand, along the same execution path, the flipping of a path constraint has to consider the results of other path constraints. For example, in Figure~\ref{example_readelf}, the path constraint in line 5 is defined by the function \texttt{process\_section\_contents()}, whose boolean output is determined by the constraints of lines 16, 17 and 18. Thus, input bytes related to lines 16, 17 and 18 also contribute to the solving of constraint in line 5. On the other hand, different program logics may process the same bytes of inputs. For instance, in Figure~\ref{example_readelf}, both the constraints of lines 10 and 23 check the value of \texttt{sh\_type}, which represents the types of sections in the program. 



% Two of the reasons for the SHAP results are the direct and indirect coupling of path constraints.
% The \textit{direct coupling} means that the flipping of a path constraint has to consider the results of other path constraints in the same execution path. Therefore, repeated mutation of certain bytes can explore all the directly coupled constraints.
% On the other hand, different program logic may process the same format of inputs, indicating that different constraints could be related to the same positions of different inputs (\textit{indirect coupling}).
% Therefore, the mutation of the same byte positions across different seeds can discover new code along different paths.


\begin{figure*}[t!]
\includegraphics[width=0.9\linewidth]{images/framework.png}
\caption{The Framework of \tool{}. Based on the SHAP analysis, \tool{} organizes seeds via the family system. To maximize the code discovery, CMAB is utilized to optimize the selection of byte positions.
% \chao{Very confusing. In Section 3.2, the probability is related to position selecting, but it relates to mutation in this figure. Further, when will this probability be calculated? How does it affect the seed mutation? How does this process integrate with a general fuzzing process, i.e., how seed selection and mutation works if considering the family system and the probability-based position selection?} \zkp{revised.}
}
\label{Framework}
\end{figure*}


\paragraph{Insight.}
Since only a small portion of bytes contribute the most to the discovery of new code, \textit{the Shapley analysis can be utilized to obtain those important bytes and more energy is assigned to them during fuzzing}. 
% However, the most significant challenge is the overwhelmed overhead of Shapley analysis as it requires to traverse all possible combinations.
In Section~\ref{sec:design}, we transform the calculation of Shapley value into a form that can be utilized to guide fuzzing.

% In Section~\ref{sec:design}, we simplify and approximate the calculation of Shapley value based on the property of fuzzing and use it to guide byte mutation of fuzzing.



% \zhu{TODO: \begin{itemize}
%     \item 1. we can use shapley to obtain the most important positions and assign more energy to these bytes;
%     \item 2. challenges to use cooperative game in fuzzing: too much overhead==> simplify the shapley calculation;(In the motivation, the shapley analysis is not simplified.)
%     \item Reason: not all cmp-related bytes contribute equally to the solving of path constraints; some bytes are not related to path constraints
% \end{itemize}}

% We exemplify the two reasons by a real-world program \texttt{readelf} in this section.
% The program \texttt{readelf} processes files with ELF format and shows the information of ELF. An ELF file is mainly composed of a series of sections whose information is recorded and managed by the section headers. 
% As shown in Figure~\ref{example_readelf}, \texttt{readelf} processes ELF files via a sequence of tasks. For example, to process objects, \texttt{readelf} will execute the sequence of functions \texttt{process\_relocs()}, \texttt{process\_version\_sections()}, and \texttt{process\_section\_contents()}.



% \textit{Direct Coupling.} The direct coupling indicates the direct influence among different path constraints along the same execution path. In Figure~\ref{example_readelf}, the path constraint in line 5 is defined by the function \texttt{process\_section\_contents()}, whose boolean output is determined by the constraints of lines 16, 17 and 18. That is, the constraint in line 5 is determined by three other constraints. To make the condition in line 5 \textit{true} (\ie the value of \texttt{res} in line 19 is \textit{false}), an input needs to satisfy 1) condition in line 16 is \textit{false}, and 2) one of the conditions in lines 17 and 18 is \textit{true}. This requires a fuzzer to fuzz the constraints of lines 16, 17 and 18 simultaneously. 
% Therefore, the repeated mutation of bytes related to a single constraint can help fuzz code lines that are guarded by complex path constraints (\ie deep code).
% % \chao{This argument shows grouping is useful, but the SHAP analysis does not show related evidence.}\zhu{revised the last sentence.}


% \textit{Indirect Coupling.} The indirect coupling indicates that two path constraints process the same input format. For example, in Figure~\ref{example_readelf}, both the constraints of lines 10 and 23 check the value of \texttt{sh\_type}, which represents the types of sections. 
% Therefore, if a seed $S_1$ has inferred the related byte positions of \texttt{sh\_type} to resolve the constraint in line 10, a fuzzer can mutate those positions in another seed $S_2$ that intends to resolve the constraint in line 23. As long as the meaning of those positions remains the same between seeds $S_1$ and $S_2$, the fuzzer can quickly explore the \texttt{case}s in function \texttt{process\_version\_sections()}. 
% % To verify that the indirect coupling is common in programs, we analyzed the number of byte positions that are related to multiple CMP instructions. We randomly selected several seeds for each program, and mutated each seed byte by byte using the method of GreyOne~\cite{greyone} to analyze the positions related to CMPs. GreyOne determines a CMP-related byte if change of the byte can lead to the change of values in a CMP. The results are shown in Figure~\ref{CMPs}, which indicates that most positions are related to multiple CMPs and some positions are even related to more than 256 CMPs. 
% Therefore, to boost the efficiency of fuzzing, a fuzzer can repeatedly mutate positions that have discovered new coverage across different execution paths.
% % \chao{This argument only shows position knowledge is reusable in other seeds.} \zhu{revised the last sentence.}

% % \begin{figure}[t!]
% % \includegraphics[width=\linewidth]{images/motivation_shap.png}
% % \label{shap}
% % \end{figure}



% \begin{figure}[t!]
% \includegraphics[width=0.9\linewidth]{images/motivation_cmps.png}
% \caption{The number of byte positions related to multiple CMPs. Most byte positions are related to multiple CMPs.}
% \label{CMPs}
% \end{figure}






==> obsolete/relate-1.0.tex <==
\section{Related Work}

Our work is a coverage-guided greybox fuzzing that aims to effectively resolve path constraints. The existing solutions for resolving path constraints include hybrid fuzzing, taint-based fuzzing, and other types of fuzzing.

\textbf{Hybrid fuzzing.}
Symbolic execution uses a constraint solver to generate an input that drives program execution to a specific path.
Hybrid fuzzing utilizes both symbolic execution and fuzzing to explore program states. In hybrid fuzzing, symbolic execution is used to solve the constraints of hard-to-cover branches when fuzzing suffers from passing path constraints. 
% Such a combination of technologies has found many vulnerabilities in real-world programs.

Although hybrid fuzzing can solve path constraints efficiently, it still suffers from path explosion inherited from symbolic execution. Therefore, the state-of-the-art fuzzers selectively address path constraints to avoid this problem. Driller~\cite{driller} uses selective concolic execution to explore those uncovered paths instead of all paths. Dowser~\cite{dowser} proposes to solve the paths that are most likely to trigger buffer-overflow vulnerabilities. SymFuzz~\cite{SymFuzz} leverages symbolic execution to detect dependencies among the bit positions of an input for a program. QSYM~\cite{qsym} utilizes instruction-level selective symbolic execution to make hybrid fuzzing scalable enough to test large applications.
Although there have been many methods to optimize the efficiency of hybrid fuzzing, it still faces the problem of being time-consuming when there is a complex relations between path constraints. 
In contrast, \tool{} pass path constraints in a lightweight manner to speed up the exploration of hard-to-cover branches.

\textbf{Taint-based fuzzing.}
% \textbf{Taint Analysis.} 
Taint analysis builds the relationships between input bytes and path constraints.
Taint-based fuzzers use taint tracking to determine which part of the input will be mutated to reach the target code blocks. Angora~\cite{angora} utilizes the byte-level taint analysis to track which input bytes flow into path constraints. Then Angora mutates only these bytes based on a gradient descent algorithm to solve path constraints. 
To explore deeply nested conditional statements, Matryoshka~\cite{matryoshka} identifies nesting conditional statements and mutates the input to solve all path constraints simultaneously. VUzzer~\cite{vuzzer} tracks the related bytes of comparisons of magic bytes and generates inputs to satisfy the constraints. 

While taint analysis is efficient in resolving constraints on hard-to-cover branches, it can also be time-consuming. Thus, some methods propose more lightweight methods to help track such taint information. Steelix~\cite{steelix} instruments the comparison progress information additionally to penetrate magic bytes more effectively.
REDQUEEN~\cite{redqueen} exploits the input-to-state correspondence to solve hard fuzzing problems. 
ProFuzzer~\cite{profuzzer} iterates through all possible values and collects the corresponding execution profiles for each byte. Then ProFuzzer groups fields and determines their corresponding type from these profiles. 
GREYONE~\cite{greyone} mutates input bytes in a pilot stage and monitors the variable value changes to infer the tainted bytes.
To make taint analysis path-aware, PATA~\cite{pata} records values of each occurrence of variables. 
% \zhu{\tool{} does not need to mutate inputs byte by byte so that it is efficient and lightweight.}
% \zhu{If the inner function is discrete, it is difficult for inference methods to find their related positions in the pilot stage. This is because the mutation of a single position is difficult to cause the value of the discrete function to change. }

While ensuring accuracy, inference-based fuzzers are simple yet efficient. However, the relationship between their efficiency and input length is strong. Since the pilot stage mutates inputs byte by byte, inference can become time-consuming when analyzing long inputs. On the contrary, \tool{} integrates the pilot stage into the havoc stage. Thus, \tool{} remains efficient regardless of the length of the input. 
On the other hand, Taint-based fuzzers and inference-based fuzzers focus on a single path constraint and neglect the relations between path constraints. \tool{} extracts valuable positions from previously resolved path constraints to solve those complex constraints. 
 
% \zhu{Angora: resolving the nested condition; based on taint analysis; time consuming;} 

% \textbf{Inference.} 

% Slow + ignore the relations between constraints.

% Both of the above methods ignore the relations between constraints.
% At the same time, Taint Tracking is slow, inference needs to set up an additional inefficient pilot stage for analysis, and the analysis of long seeds takes a long time.

\textbf{Other Fuzzing Strategies.}
NEUZZ~\cite{neuzz} builds the relationships between input bytes and branch behaviors via deep learning models. Then NEUZZ preferentially mutates the bytes with high score, indicating those bytes have high chance to be related to branches.
As the same program logics can be repeatedly used within a single program, EMS~\cite{ems} captures the byte-level mutation strategies from intra- and inter-trial history to explore new paths and crashes.
While EMS focuses on the values of input segments, our \tool{} focuses on the positions of inputs. An input position may be used as a path constraint in different program logics, and the different program logics probably use different CMP instructions.



==> obsolete/technique-0.1.tex <==

\section{DESIGN}
\subsection{Framework}
As shown in \ref{Framework}, TransferFuzz adds two components of transfer learning based on the workflow of fuzzing campaigns, i.e., the collection of common features and the generation of task-specific features. The green blocks are the transfer learning-related components.

More specifically, TransferFuzz divides the fuzzing campaigns into multi-fuzzing campaigns based on the inheritance relationship and extracts the common features during the exploration of seeds in each child fuzzing campaign.
Then, TransferFuzz generates task-specific features based on common features during the exploration of a seed, and uses them to guide the fuzzing. Finally, TransferFuzz constructs three mutation modes and dynamically chooses the best mode to determine the positions to be mutated.
The details are as follows.

\begin{figure}[htbp]
\includegraphics[width=\linewidth]{images/framework.jpg}
\caption{Framework.}
\label{Framework}
\end{figure}

\subsection{Multi-fuzzing campaign system}
\subsubsection{Definition}
We formally define the common features as the positions that have been mutated and found new edges successfully and define the cross-seeds meaning invariance as the same position in different seeds having the same meaning. 
In order to leverage the common features to guide the fuzzing, we need to maintain the cross-seed meaning invariance between the source seed extracting the common features and the target seed using the common features. For example, we mutate position i in seed A, find a new edge, and record position i into the common features vector. If we want to mutate the position i in seed B based on common features, we need to ensure the meanings of position i in seed A and seed B are consistent, i.e., maintain the cross-seed meaning invariance. Thus, we group the seeds that obtain cross-seed meaning invariance into one race, and the seeds in the same race can share common features. 

\subsubsection{Resource allocation}
Just like the traditional AFL-based fuzzers, all the seeds share a global variable virgin\_bits to record the edges found by all seeds, i.e., all the races.
However, only maintaining a global virgin\_bits is not enough, which causes the missing of some common features in a specific race. For example, there are two races, and position i is a common feature in both two races. If race A first set position i as a common feature, the edges found by mutating position i have been set to 'found' state in global virgin\_bits. Then, race B can not include position i as its common feature.
To extract more abundant common features, each race maintains a local virgin\_bits to record the edges found by the inputs in this race. Each time a seed is mutated to find a new path, both global virgin\_bits, and local virgin\_bits will be updated. 
We define the local common features as the positions that have been mutated and found new edges successfully regarding the local virgin\_bits. Each race maintains a local common features vector to record all local common features in this race.
Thus, if position i is mutated, we will check local virgin\_bits to determine whether local new edges are found. If found, we add the mutated positions into the local common features vector. In summary, each race maintains a local virgin\_bits and a local transfer features vector, and all races share a global virgin\_bits.

\subsubsection{How to construct a race}
In order to maintain the cross-seed meaning invariance in a race, the mutated inputs generated from length mutators can not be included. These inputs will be added to a random race, which does not maintain local virgin\_bits and local common features vector. Thus, random races can not leverage common features to mutate. Finally, we will maintain the same number of races as the initial seed as normal races, and a random race.

However, the using of length mutators to generate mutated inputs is common. If we do not impose any restrictions on the use of length mutators, the number of the inputs stored in normal races will be small but random race's will be large. Thus, we should try to limit the use of length mutators.  Therefore, we propose a grammar preservation system to maintain the cross-seed meaning invariance between the initial seed and new seeds generated from it. The grammar preservation system focus on migrating two main phenomena that use the length mutators. 

First, length mutators could be used in the havoc stage, which breaks the cross-seed meaning invariance. During one mutation, we store the length mutators used in a stack. The details as shown in fig X. The length mutators can be divided into two categories, insertion and deletion. For insertion, we record the inserted position and the length of the memory to be inserted. For deletion, we extra record the deleted memory. If a new edge is found, we pop mutators one by one from the top of the stack, and then withdraw all mutators. In the withdrawing stage, we delete the inserted memory for the insertion mutator and insert the deleted memory for the deletion mutator. After all length mutators have been withdrawn, we put the withdrawn input into the target program. If the new edge still can be found, we retain the withdrawn input into the seed corpus. Otherwise, we still retain the original mutated input into the seed corpus. 

\begin{figure}[htbp]
\includegraphics[width=\linewidth]{images/race_construction.jpg}
\caption{race construction. \zhu{change race to family? race has multiple definitions}}
\label{race_construction}
\end{figure}

Second, trimming also changes the seed length and we can not withdraw the deletion operations. Thus, we need to track the relative position with reference to the initial seed of the current race. More specially, as only delete mutators will be used at this stage, the length of the seeds must be shortened or consistent after trimming. According to the definition of the race, only the input generated from the initial seed without using length mutators can be included in a race. Then, the length of inputs in a race must be shorter than the initial seed in this race because of trimming. Thus, we set the initial seed as the benchmark of its race. Each input need to maintain a map\_vector to indicate the relative position with reference to the initial seed. We show an example in fig x. Assume that in a race, the initial seed has 7 bytes, so that its map\_vector is [1,2,3,4,5,6,7]. And a trimmed seed is generated from the initial seed by trimming down the fourth and fifth bytes, so that its map\_vector is [1,2,3,6,7]. For instance, '6' in the map\_vector of the trimmed seed means that the fourth byte in the trimmed seed is corresponding to the sixth byte in the initial seed. Further, if an input B is generated from seed A by trimming down the first 2 bytes, the map\_vector of B will be [3,6,7]. 

Therefore, we conclude the process of constructing a race. First, we construct N+1 races where N is the number of initial seeds, and each initial seed is assigned to one race. Second, for the new seeds without using length mutators, we directly add them into the race where their parent seed belongs. Third, for the new seeds using length mutators, we try to withdraw all length mutators. If the withdrawn seed still can find the path, we add the withdrawn seed into the corresponding race.

==> obsolete/technique-0.2.tex <==



\section{DESIGN}

\zhu{Don't leave blank between titles!}

\todo{subsections: \begin{itemize}
    \item overview \begin{itemize}
        \item describe figure
    \end{itemize}
    \item why do we use discover-new-edge positions (valuable positions)? \begin{itemize}
        \item ???Only a part of CMP related bytes contribute to the coverage discovery. The SHAP experiment.
        \item direct relation => combination of path constraints equals to combination of corresponding positions
        \item indirect relation => in a different path, the constraint-related position is still related to path constraint
    \end{itemize}
    \item how to organize discover-new-edge positions: seed family \begin{itemize}
        \item position mapping: maintain structure, same meaning for a position;
        \item optimize the selection of positions in the shared pool: LinUCB
    \end{itemize}
    \item switch between expanding discover-new-edge positions and utilizing discover-new-edge positions
    \item discussion: \begin{itemize}
        \item we can use different existing solutions to expand discover-new-edge positions
    \end{itemize}
\end{itemize}}


As shown in Figure~\ref{Framework}, the basic procedure of \tool{} contains the following three steps. 
%First, \tool{} integrates the pilot stage into the havoc stage.
we cluster seeds into multiple families based on inheritance relationship during the fuzzing process.
Second, all seeds in a family will jointly maintain a shared pool, sharing their valuable positions discovered in the mutation process.
Third, in order to judge the relationship between each position recorded in the shared pool in each family and each seed in a more fine-grained manner, we use the LinUCB model to analyze and find the most valuable positions of the shared pool for each seed individually. Then, we use these positions to mutate, called history mode. And we rename the normal mutation strategy as random mode.
Fourth, a mode scheduling algorithm is proposed, which uses the mutation performance of each mode on the current seed to select the best mode dynamically.
%The basic procedure of \tool{} contains the following steps.First，我们利用继承关系粗粒度地完成种子聚类，将fuzzing过程中所得到的所有种子分为多个family。Second，每个family内的所有种子会共同维护一个shared pool，共享自己在突变过程中发现的structure-realted positions。Third，为了更加细粒度地判断每个family内shared pool中记录的各个position与种群内的各个种子之间的关系，我们利用LinUCB model进行分析，个性化地为每个种子找到shared pool最有价值的 positions，并利用这些positions进行突变，称为history mode。Fourth，对于那些一次性发现多条新边的new seed，额外构建了new mode来对其所发现的新边的相关bytes进行突变。Fifth，提出了一个mode调度算法，利用各个modes在当前种子上的突变表现来动态选择最佳的mode。

\begin{figure*}[htbp]
\includegraphics[width=\linewidth]{images/framework.jpg}
\caption{The Framework of Pozzer.}
\label{Framework}
\end{figure*}

\subsection{Inference for single constraint}
The first challenge is to infer the related bytes of a single path constraint in a more lightweight method. To address this challenge, \tool{} accelerates the process of inference from two perspectives. First, as the traditional inference methods are time-consuming when processing long inputs, \tool{} integrates the pilot stage into the havoc stage. Second, to avoid the repeated inference of the same constraint on different seeds, \tool{} proposes a family system to achieve information sharing between seeds.

\subsubsection{The Integration of Pilot Stage and Havoc Stage}
% \textbf{Valuable Positions.}
% \textbf{Why can the pilot stage be integrated into the havoc stage?}
% \textbf{Choice of Indicator.}

\textbf{The Overview of Dataset Replacement.}
In the inference-based methods, they maintain a dataset for each seed to identify their own valuable positions. 
As shown in Figure~\ref{dataset}, given a seed $t$, they mutate each position one by one and observe whether the execution state changes. If the execution state changes, the mutated position will construct a \textit{mutation information tuple} (mutated positions, execution state changed or not), which will be added to the dataset.
After testing all positions in the seed $t$, the obtained dataset will be used to identify its valuable positions. 
As they only mutate one position at once, the mutated positions stored in the dataset must belong to valuable positions. 

\begin{figure}[htbp]
\includegraphics[width=\linewidth]{images/dataset.jpg}
\caption{The datasets generated from pilot stage and havoc stage.}
\label{dataset}
\end{figure}

When the length of seed $t$ is large, the inference-based fuzzers suffer from the time-consuming problem. In ProFuzzer~\cite{profuzzer}, it needs to mutate each position in the input 255 times, which takes unacceptable time.
% Especially in the case of long input, the required analysis time is unacceptable. 
For example, assume the input size is 10kB and the target program execute 1000 times per second.
Thus, the required analysis time is 10240 * 255/1000 = 2611 seconds. 

To address this problem, Pozzer utilizes the mutation information collected from havoc stage to replace the dataset generated from the pilot stage as shown in Figure~\ref{dataset}. 
Specifically, assume that a seed $t$ is being mutated in havoc stage.
If a mutation change the execution state of seed $t$, we construct a mutation information tuple based on the mutated positions and changes in execution state.
Finally, the tuple will be add into dataset.

\textbf{Choice of Indicator.}
The construction of the dataset relies on efficient indicator, which decides what data to collect. 
In order to design a proper indicator, we need to figure out what dataset we want to get.
The key of exploring unsolved constraints considering the coupling of path constraints is to constantly flip the related solved path constraints, that is, to mutate the positions that can flip related solved constraints. 
However, not all related positions of constraints can make the result flipped. For example, if you explore $if(a > 10000)$ in Greyone, where a is of type u32, and a is 0 from the initial seed. Although we can identify all related positions of a, only the high-order positions are useful for edge exploration, and the low-order positions are redundant. The mutation of low-order positions can not flip this constraint. Thus, We expect the dataset constructed above to have the following three characteristics: 1) Low overhead. 2) Easy to extract enough data. 3) able to extract positions that can flip constraints.

The indicator is generally the execution state of the program, including the matching status of cmps, the discovery of new edges, and so on. However, there are some problems with existing indicators. 
We can not collect mutation information that changes the matching status of cmps, which may cause data explosion problems. And it requires extra instrumentation, slowing down the execution speed. Moreover, it also may infer many redundant positions.
We can not collect mutation information that discovers new edge, which has the problem of data imbalance problems. 
Seeds that mutate first can discover more new edges easy to be found and collect a lot of data, 
while seeds that mutate later are more likely to encounter data shortages.
Therefore, we designed a new indicator in a compromise: \textit{local new edges}.

Formally, we give the definition of local new edges. 
In AFL-based fuzzer, all seeds will maintain a global bitmap to record edges that have been found.
If a seed discovers a new edge in the global bitmap, we call this new edge as \textbf{global new edge}.
To extract more useful mutation information, we maintain a local bitmap for each seed to record edges found by it and its mutated inputs.
If a mutated input generated from a seed $t$ finds a new edge in the local bitmap of seed $t$, we call this new edge as \textbf{local new edge}.

% Thus, we only collect mutation information tuples based on those mutations that find local new edges.
During the havoc stage, when we are mutating seed $t$, the mutated inputs find local new edges will be used to construct mutation information tuples. Then, those mutation information tuples will be added to the dataset of seed $t$.
% Therefore, we only consider those mutations that find new edges relative to the current seed.
% Specifically, if a mutated input generated form a seed $t$ finds a local new edge, we will construct a mutation information tuple and add it into the dataset of seed $t$.
% In other words, each seed maintains a bitmap to record edges found by it and its mutated inputs.
% If a mutated input generated form a seed $t$ finds a new edge in the bitmap of seed $t$, 
% After our experiments, using the granularity of the edge can obtain enough data for further analysis.

\textbf{Multiple Positions Inference Algorithm.}
After we have a new dataset generated from havoc stage, we extract the valuable positions for each seed from it. However, the dataset generated from the pilot stage and the dataset generated from havoc stage are inconsistent. Since only one position is mutated at a time in the pilot stage, the number of mutated positions of the former is 1. As multiple positions could be mutated simultaneously in havoc stage, the number of mutated positions of the latter is likely to be greater than 1. Therefore, we need an inference-based analysis method suitable for mutating multiple positions simultaneously.
Otherwise, there will be much redundancy.

Essentially, if we can remove those mutated positions that are irrelevant to the discovery of new edges, leaving only the \textit{necessary} mutated positions, we can achieve mutating multiple bytes at the same time without causing an over-taint problem. The \textit{necessary} means that new edges cannot be found without mutating any position. 
So we can get the following conclusion: if a mutated input mutates multiple \textit{necessary} positions and finds a new edge, then we believe these positions are valuable positions.
Therefore, if we can de-duplicate mutated positions in the mutation information collected from the havoc stage, we can replace the dataset generated by the pilot stage with those mutation information.


\subsection{Family System}
Since a constraint can be passed by multiple seeds, a constraint may be inferred repeatedly.
As all seeds share a constraint space, different seeds can share the related positions they found for the same constraint.
However, there are many factors in the fuzzing process that may cause alignment problems between seeds, such as different initial seed structures, trimming and other operations.
To solve this problem, establishing a position mapping between seeds is necessary.
However, due to the complexity of the seed structure, it is difficult to find the semantic mapping between seeds with different structures.
If two seeds have an inheritance relationship, they are more likely to have the same structures.
Therefore, we propose a \textbf{family system} based on the inheritance relationship. In a family, we use a \textit{semantic tracking algorithm} and \textit{absolute position space mechanism} to establish the semantic mapping between seeds within the family.
Finally, seeds within the same family can exchange information based on semantic mapping to speed up the analysis process. 
% Why we need semantic mapping? 
% To achieve semantic mapping, 就需要去建立种子之间的位置映射。
% 但是，由于种子结构的复杂性，我们很难去寻找具有不同结构的种子之间的semantic mapping。
% 如果两个种子之间具有继承关系，那么它们更有可能有着同一套种子结构。
% 所以，我们基于继承关系建立了family system。更具体的，我们利用初始种子建立一个family，由其突变所得的子代seeds会被加入到该种群中。
% 在一个family中，我们利用semantic tracking algorithm和absolute position space mechanism为family内的各个种子之间建立semantic mapping。
% 1)Semantic tracking algorithm. Semantic tracking algorithm tracks position mapping between seeds during the process of seed generation。
% 2)Absolute position space mechanism. 每个种子拥有独立的一套relative position space，种子内部的位置称为relative position。
% 要想实现semantic mapping，就需要将各个种子的relative position映射到同一个absolute position space，这样才能够实现对齐。
% 所以，each family builds a absolute position space based on the ancestor seed who constructs this family。
% 最后，absolute position space mechanism 基于semantic tracking algorithm将种子内的相对位置映射到绝对位置空间，来实现semantic mapping。

% Since a constraint can be passed by multiple seeds, a constraint may be inferred repeatedly. As all seeds share a constraint space, different seeds can share the related positions they found for the same constraint, which can speed up the analysis process. However, there are many factors in the fuzzing process that may cause alignment problems between seeds, such as different initial seed structures, trimming and other operations. To solve this problem, \tool{} proposes a \textit{family system} to coarsely divide all seeds into multiple families based on inheritance relationship. 
% To achieve all seeds maintain \textit{semantic mapping} in the same family, \tool{} utilizes \textit{semantic preservation algorithm} to track position mapping between seeds.
% \textit{Semantic mapping} means that positions with the same meaning can be found between seeds. 



% However, the above scheme assumes that the number of mutations for each seed is sufficient. In fact, the distribution of energy among the seeds is very uneven, with some seeds being allocated a large amount of energy and some seeds being able to mutate only a few hundred times (Challenge III).

% In order to solve the problem of insufficient data for some seeds, we propose a \textbf{family system} to coarsely divide all seeds into multiple families based on inheritance relationship. In each family, all seeds coarsely maintain $semantic\ consistency$. $Semantic\ consistency$ means that the same position on different seeds have similar meanings.
% Then, we achieve \textbf{information sharing within the family}.
% Each family maintains a shared pool for recording valuable positions on all seeds within it.
% Moreover, in a family, any seed can also use the positions extracted from other seeds in the shared pool.
% Therefore, for new seeds in the family, it can also directly access the shared pool to know which positions may be valuable positions. For different seeds within the family, they can communicate the valuable positions they found, thereby reducing the required analysis resources.

\zhu{link "family" to motivation}

% However, since the mutation process of fuzzing is random, a completely different new seed will likely appear during the mutation process. Therefore, the positions recorded in the shared pool no longer apply to these seeds. To this end, we introduce the LinUCB model to determine the probability that each position in the shared pool is a structural field on each seed. Specifically, within a family, we regard each position in the shared pool as an arm and seeds as a user. At the same time, we extract the path feature vector of each seed based on the path feature generation algorithm to characterize its path feature as the user's attribute. Finally, the rarity of the path taken after the mutation is used as the reward. Based on the above definitions, we build a LinUCB model to adaptively determine the relationship between all positions in the pool and each seed.

%然而，上述方案依赖于突变次数足够的假设之下。实际上，各个种子之间的能量分配很不均匀，部分种子会被分配大量的能量，而部分种子却仅能够突变数百次。为了解决部分种子的数据量不足的问题，我们提出了基于语义一致性原则的聚类算法。语义一致性原则是指在不同的种子上的同一个位置的意义具有相似的意义。然后，我们基于语义一致性原则将fuzzing过程中的所有的seeds划分为多个族群，每个族群内部维护着语义一致性。在每个族群内部维护一个shared pool，记录该种群内所有种子上可能为结构字段的positions。由于语义一致性的存在，在同一个种群内，任意种子识别出来的结构字段的位置会被加入到shared pool，同时也可以使用shared pool由其他种子上提取出来的结构字段的位置信息。所以，对于种群内所分配能量较少的种子，它也可以直接访问shared pool，知道自己的哪些bytes可能位于结构字段，从而对它们重点进行突变。对于族群内的不同seeds，他们之间可以交流各自发现的结构字段所在的positions，从而减少所需要的分析资源。

%但是，由于fuzzing的突变过程是不确定性的，在突变过程中很有可能出现一个完全不一样的新种子。所以，shared pool中记录的positions对这些seeds就不再适用。为此，我们引入cMBA model来判断shared pool中的每个position在各个seed上为结构字段的概率。具体的，在一个种群内，我们将shared pool中的各个position视为一个arm，将seeds视为user。同时，我们基于路径特征生成算法提取出各个种子的路径特征向量以表征其路径特征作为user的属性。最后，将突变后所走的路径的稀有程度作为reward。基于上述定义，我们构建cMBA模型来实现自适应地判断pool中所有positions与各个seeds之间的关系。



% In order to allow different seeds to share their own structure field information, we need to cluster the seeds according to semantic consistency.
% First, we constructed a family system based on the inheritance relationship to roughly divide all seeds into multiple families to reduce the probability of missing.
% Then, to adaptively judge the relationship between each position recorded in the shared pool and each seed in the family, we introduced the LinUCB model for analysis.
%为了不同的种子之间可以共享自己的结构字段信息，我们需要将种子根据语义一致性原则将种子进行聚类。首先，我们基于继承关系构建了Family System粗略地将所有种子划分多个种群，减少missing的概率。然后，为了更精准地自适应地判断shared pool中记录的各个position与种群内各个种子的相关程度，我们引入了cMBA模型进行分析。

\subsubsection{Definition of Family}
% Formally, we define semantic consistency: Suppose there are two seeds $a$, and $b$ of the same length. If for any position $i$, the $ith$ byte in $a$ and the $ith$ byte in $b$ have similar meanings, it means that there is semantic consistency between a and b.

% However, suppose we want to obtain the semantic consistency relationship between each seed accurately. In that case, we need to use tools such as a grammar parser to analyze each seed, which is very time-consuming. Also, due to the randomness of the fuzzing process, some illegal seeds are likely to be generated. For these seeds, not even the help of a parser can be done.

% Therefore, we first roughly divide the families. We assume that semantic consistency is maintained between parent and child seeds without using length mutators \zhu{should explain what is length mutators}.\zkp{Length mutators are those mutators that can change the length of the input, such as insert, delete, etc.} However, since the mutation process of seeds is random, it is very likely that a new seed with a completely different structure will be obtained after several generations of mutation. At this time, our hypothesis is no longer satisfied. Therefore, we introduce LinUCB to judge the relationship between each position recorded in the shared pool and each seed in the family and identify those positions useless to the current seed.

We give the formal definition of Family: Suppose there are seeds $a$, $b$. Seed $b$ is derived from a mutation of seed $a$, i.e., seed $a$ is the parent of seed $b$. If no length mutators are used in the process of mutating seed $a$ to obtain seed $b$, the seeds $a$ and $b$ belong to the same family.

At the same time, the family relationship is also transitive: if seeds $a$ and $b$ belong to the same family, and seeds $b$ and $c$ also belong to the same family, then seeds $a$, $b$, and $c$ belong to the same family.

In each family, there are two roles: ancestor and offspring. The ancestor refers to the seed that forms the family, that is, the first seed to join the family. offspring refers to those new seeds that are mutated from the ancestor without using length mutators, including the ancestor's children, grandchildren, and so on.

Then, the family needs to maintain a \textit{shared pool} to record valuable positions on all seeds within the family. All seeds in the family can access or add elements to the shared pool, and the subsequent mutation process will be performed based on the shared pool.

Finally, to implement the indicator of local new edge, each family maintains a local bitmap to record the edges found by the seeds in this family.

%正式的，我们给出语义一致性的定义。假设存在两个相同长度的种子a、b以及一个position i。如果对于任意的i，a中的第i个字节和b中的第i个字节具有相近的意义，说明a和b之间存在语义一致性。

%但是，如果想要精准地得到各个种子之间的语义一致性关系，需要利用语法解析器等工具对各个种子进行分析，这个过程非常的耗时。并且，由于fuzzing过程的随机性，很可能生成一些不合法的种子。对于这些种子，即使有语法解析器的帮助也无能为力。

%所以，我们先进行粗略地划分种群。我们假设在不使用length mutators的前提下，父种子和子种子之间是维持着语义一致性的。但是，由于种子的突变过程是随机的，很有可能在经过几代的突变之后，得到一个结构完全不一样的新种子，这时我们的假设就不再使用。所以，我们引入cMBA判断shared pool中记录的各个position与种群内各个种子之间的关系，识别出那些对当前seed无用的positions。

%我们给出Family的正式定义：假设存在种子a、b。种子b来源于种子a的突变，即种子a是种子b的父亲。如果在对种子a突变得到种子b的过程中没有使用length mutators，我们认为种子a和种子b属于同一个种群。

%同时，Family的关系还具有传递性：假设a和b属于同一个family，b和c也属于同一个family，则a、b、c属于同一个family。

%在每个Family中，有两种角色：leader以及member。leader是指形成该种群的那个种子，即：第一个加入到该种群的种子。member是指那些由leader未使用length mutators突变而来的新种子，包括leader的子代、孙代等等。我们粗略地认为member与leader之间保持着语义一致性原则。

%最后，Family需要维护一个shared pool，用来记录哪些位置位于结构字段，family内的所有种子都可以进行访问或增加元素，并且后续的突变过程会基于shared pool进行突变。




\subsubsection{Family Scheduling Algorithm}
We divide all the seeds into the Formal Part and Candidate Part. Seeds in the Formal Part will create a new family or belong to an existing family, while seeds in the Candidate Part will not belong to any family.
%我们将所有的种子划分为Formal Part和Candidate Part两部分。在Formal Part中的种子会构建一个新的种群或者是归属于某个已有的种群，而在Candidate Part中的种子不会归属于任何族群。

\textbf{Initialization.}
In order to avoid the explosion of the number of families caused by the excessive number of initial seeds, we use whether new edges are found as an indicator for assigning the initial seeds to the Formal Part. So, if an initial seed finds a new edge, it will be added to the Formal Part to form a new family and become the ancestor  of this family; otherwise, it will be added to the Candidate Part.
Then, if the seed in the Candidate Part found multiple new edges during the mutation process, we migrate it to the Formal Part, form a new family, and become a ancestor .
%initialization: 为了避免初始种子数量过多的情况，我们将是否发现新边作为初始种子分配到Formal Part的指标。所以，如果一个初始种子发现了新边，将将其加入到Formal Part中形成一个新的种群，并且成为该种群的ancestor ；否则，将其加入到Candidate Part。最后，如果Candidate Part中的种子被突变过发现了多条新边，我们将其迁移到Formal Part中，形成一个新的种群并且成为ancestor 。

\textbf{Update the offspring sequence.}
When we mutate seed $i$ to obtain new seed $s$, if length mutators are not used in the mutation process, the new seeds will be added to the offspring sequence of the family where seed i is located. However, to maintain the semantic mapping in a family, the mutated inputs generated from length mutators can not be included. These inputs will be added to the Candidate Part, which does not maintain a shared pool. Thus, the seeds in the Candidate Part can not leverage the stored positions in the shared pool to mutate.

However, the using of length mutators to generate mutated inputs is common. If we do not impose any restrictions on using length mutators, the number of seeds stored in the Formal Part will be small, but the Candidate Part will be large. Thus, we should try to limit the use of length mutators. Therefore, we propose a grammar preservation system to maintain semantic consistency.

The length mutators could be used in the havoc stage, which breaks the semantic consistency. During one mutation, we store the length mutators used in a stack—the details as shown in Figure~\ref{withdraw}. The length mutators can be divided into two categories, insertion and deletion. For insertion, we record the inserted position and the memory length to be inserted. For deletion, we extra record the deleted memory. If a new edge is found, we pop mutators one by one from the top of the stack and withdraw all mutators. In the withdrawing stage, we delete the inserted memory for the insertion mutator and insert the deleted memory for the deletion mutator. 
As shown in Figure~\ref{withdraw}, we give an example. First, we get the first mutator, i.e., (insertion,1,1), from the top of the stack. To withdraw this insertion mutator, we delete the inserted memory block marked in red. Second, we get the next mutator (deletion,4,3). Then we need to insert the memory block marked in green. 

After all length mutators have been withdrawn, we put the withdrawn input into the target program. If the new edge still can be found, we retain the withdrawn input into the seed corpus. Otherwise, we still retain the original mutated input into the seed corpus.

\begin{figure}[htbp]
\includegraphics[width=\linewidth]{images/withdraw.jpg}
\caption{The withdraw operation.}
\label{withdraw}
\end{figure}

\subsubsection{Semantic Tracking Algorithm}
\zhu{absolute position is more important than relative position in format. absolute position: positions in original seed; relative position: positions within seeds}

\textbf{Absolute position space.} 
Before adding the valuable positions into the shared pool, we need to convert the relative positions in each seed into absolute positions, so that we can express them uniformly.
% As only delete mutators will be used in the trimming stage, the length of the seeds must be shortened or consistent after trimming.
According to the definition of the family, only the input generated from a seed without using length mutators can be included in a family.
Then, the length of seeds in a family's offspring sequence must be shorter than the ancestor in this family because of trimming.
Thus, we set the ancestor as the benchmark of its family.
We define the position inside the seed as \textbf{relative position}.
If the relative position i is corresponding to position j in the ancestor according to the trimming chain, the position j is called \textbf{absolute position}.

\textbf{Position mapping.} \zhu{to maintain the structural meanings.}
Due to trimming, although length mutators are not used in the generation of offspring, differences in length may still occur between seeds within the same family.
If we directly record the relative positions of the valuable positions in each seed into the shared pool, there will be a problem of semantic inconsistency. 
For instance, $seed\ A$ is generated from $initial\ seed$ by trimming the red block as shown in Figure~\ref{trimming}. If we mutate the fourth position and find a new edge, we add '4' into the shared pool. However, as position 4 in $seed\ A$ corresponds to position 6 in $initial\ seed$ based on the trimming relationship, position 4 in $seed\ A$ and $initial\ seed$ have different meanings. Thus, we cannot directly use '4' to locate the valuable position of the initial seed. 

Therefore, each seed needs to maintain a \textbf{mapping vector} with the same length as its own to complete the mapping from relative positions to absolute positions.
We show a example in Figure~\ref{trimming}. Assume that in a family, the ancestor has 7 bytes, so that its map\_vector is [1,2,3,4,5,6,7]. And a trimmed seed generated from ancestor by trimming down the fourth and fifth bytes, so that its map\_vector is [1,2,3,6,7]. For instance, $6$ in the map\_vector of trimmed seed means that the fourth byte in trimmed seed is corresponding to the sixth byte in ancestor. Further, if a input B generated from seed A by trimming down the first 2 bytes, the map\_vector of B will be [3,6,7].
Finally, the positions recorded by the shared pool are absolute positions. When each seed interacts with the shared pool, it needs to use the map vector to convert its relative positions into absolute positions first, so that there will be no semantic inconsistency.

\begin{figure}[htbp]
\includegraphics[width=\linewidth]{images/trimming.jpg}
\caption{The example of mapping mechanism.}
\label{trimming}
\end{figure}



\begin{algorithm}[!t]
\footnotesize
\caption{Update the structure-related absolute positions stored in shared pool.}\label{alg:SharedPool}
\KwIn{
The seed being mutated, $s\_orig$.
The mapping vector of $s\_orig$, $m$.
The mutated input found new edges generated from $s\_orig$, $s$.
The Candidate Part, $C$.
The stack that record the length mutators have been used, $Stack$. 
}
\If{$s\_orig \in C$ }{
    $C \gets s$
}\Else{
    \If{$Stack \neq \emptyset$ }{
        $RecoveredInput = Withdraw(Stack)$\\
        \If{$RecoveredInput\ can\ find\ the\ same\ new\ edges$ }{
            $s = RecoveredInput$\\
        }\Else{
            $C \gets s$
        }
    }\Else{
        \For{$ t = 1,2,3,...,Length $}{
            \If{$s[t] \neq s\_orig[t]$ }{
                $tmp = s[t]$\\
                $s[t] = s\_orig[t]$\\
                \If{$s\ can\ not\ find\ the\ same\ new\ edges$ }{
                    $s[t] = tmp$\\
                    $Record\ m[t]\ into\ the\ shared\ pool\ of\ the\ family$\\
                    $where\ s\_orig\ is\ located$\\
                }
            }
        }
        $Record\ s\ into\ the\ Offspring\ Sequence\ of\ the\ family$\\
        $where\ s\_orig\ is\ located$\\
    }
}
\end{algorithm}

\textbf{Overall Algorithm.}
As shown in Algorithm~\ref{alg:SharedPool}, if a mutated input generated from a seed that exists in the Formal Part finds a new edge, we need to withdraw all the length mutators. If the withdrawn input can not find the same new edge, we add the original mutated input into the Candidate Part. Otherwise, we need to withdraw redundant mutations to keep the minimal change while maintaining the same effect, which ensures the accuracy of the positions stored in the shared pool. If we do not do that, almost all positions will be added to the shared pool. 

More specifically, we compare the withdrawn input with the original seed byte by byte. For mutated position i, we reset it with the corresponding value in the original seed and put it into the program. If the same new edge still can be found, we reset the next mutated position. Otherwise, we withdraw this resetting operation and add map[i] (i.e., the absolute position of position i) into the shared pool. For instance, if a mutated input is [1,2,3,6,7], its original seed is [1,2,3,4,5], and its map vector is [1,2,3,7,8], we first reset the value of the fourth byte to 4 and test it. We find the same new edge is exercised so that we reset the next mutated position.
Then we reset the value of the fifth byte to 5. However, a new edge can not be found. Thus, we withdraw this resetting operation, i.e., set the fifth byte to 7, and add map[5]=8 into the shared pool.

\subsection{Family-Based Mutation Mode}

Based on the shared pool in each family, we propose a novel family-based mutation strategy to efficiently select the most valuable positions to be mutated for each seed.
In a family, since the fuzzing mutations are random, a completely different new seed may appear after many mutations. In other words, semantic consistency is violated with other family seeds. At this time, the structure-related absolute positions recorded in the shared pool of the family are no longer applicable to this seed. To solve this problem, we use the LinUCB model to analyze the relationship between all positions in the shared pool and the current seed.
%在一个family中，由于fuzzing的突变都是随机的，所以在经过多次的突变之后，有可能会出现一个完全不一样的新种子，也就是与该family的其他种子之间违背了语义一致性。这时候，该family的shared pool所记录的结构字段的absolute positions就不再适用于这个新种子。为了解决这个问题，我们利用cMBA model来建模shared pool中的所有positions与当前种子的关系。

\subsubsection{Why do we use LinUCB?}
After we determine which seed to mutate, we need to select appropriate positions from the shared pool to mutate.
Therefore, the most intuitive idea is to use the MBA model for processing. \zhu{more reason} \zkp{In previous studies, the MBA model has been shown to have a good effect on seed schedules. For example, EcoFuzz treats each seed as an arm and defines the reward of each trial as generating an input that triggers a new path. Since the position selection problem is essentially an $Exploration\ \&\ Exploitation$ problem}, we regard the positions recorded in the shared pool as arms and define the reward of each trial as generating an input that triggers a new path.
However, MBA is a context-free algorithm. MBA assumes that the reward of each arm does not change with different users. That is, MBA assumes that a position in the shared pool has the same meaning for different seeds.
This is unrealistic since the mutation is a random process. Some anomalous seeds with significant structural changes may be generated. For these abnormal seeds, it is necessary to identify which positions in the shared pool are useless for the seeds.
Therefore, we need to consider the seeds' characteristics (i.e., user characteristics) to get a personalized selection scheme. Therefore, we adopt the contextual bandit algorithm, which considers contextual information when implementing the exploration\&exploitation problem. Therefore, it is more suitable for actual personalized recommendation scenarios.
Since throughput is an essential indicator in fuzzing, we must use a more lightweight algorithm. Thus, we finally chose LinUCB for modeling. LinUCB is a general contextual bandit algorithm that has a high calculation speed.
Therefore, we regard the seed as a user and the positions recorded in the shared pool as arms. In addition, LinUCB also needs to determine two key factors: user feature and reward.

%Why we use cMBA？当我们确定好将要被突变的种子之后，我们需要从shared pool中选择合适的positions进行突变。因此，最直观的想法就是利用MBA模型进行处理：regard the positions recorded in shared pool as arms and define the reward of each trial as generating an input that triggers new path. 但是，MBA是一个context free的算法。MBA有一个前提假设：假设各个arm的reward并不会随着用户的变化而变化，即假设shared pool中的同一position对于不同的seeds而言都具有相同的意义。这显然是不现实的，因为突变是一个随机的过程，完全可能生成出一些结构发生剧烈变化的新种子。对于这些异常种子，就需要识别出shared pool哪些positions对于该种子而言是无用的。所以，我们需要将种子自身的特征考虑进来（i.e., 用户特征），得到个性化的选择方案。因此，我们采用Contextual Bandit算法，这类算法在实现E&E时考虑了上下文信息，因而更加适合实际的个性化推荐场景。因此，we regard the seed as user，and regard the positions recorded in shared pool as arms. 此外，cMBA还需要确定两个关键因素：user feature以及reward。

\subsubsection{User feature.}
The most intuitive feature that can reflect the structural changes between seeds is the execution path of the seeds. If the structure changes, it is likely that the execution path of the seed will also change. So, the easiest way is to use the edges that the seed passes through as the user feature. However, since most target test programs have tens of thousands of edges, the number of parameters to be stored for processing would be huge.
Therefore, we need to compress user features to save time and space overhead. As shown in Figure~\ref{FeatureGeneration}, we have the following steps:

a) Execute all the seeds to get their execution paths, form them into a dataset, and then use the k-means algorithm to cluster all the seeds into N classes.

b) Extract the center of each class as the central node.

c) Calculate the similarity between each seed and the N central nodes to form an N-dimensional feature vector. Then use this vector to characterize the path feature of each seed. We use Jaccard similarity coefficient to measure the similarity. Given two seeds $a$ and $b$, and assume that seed $a$ exercises the path $P_{a}$ and seed $b$ exercises the path $P_{b}$. The similarity $s(a,b)$ between seeds $a$ and $b$ can be calculated as:

$$
s(a,b) = \frac{|P_{a}\cap P_{b}|}{|P_{a}\cup P_{b}|}
$$

\begin{figure}[htbp]
\includegraphics[width=\linewidth]{images/FeatureGeneration.jpg}
\caption{K-means Based Feature Generation Algorithm.}
\label{FeatureGeneration}
\end{figure}

%能够反应种子之间结构发生变化的最直观的特征就是种子的执行路径。如果结构发生了变化，那么种子的执行路径很可能也会发生变化。所以，最简单的方法就是把种子所经过的边作为user feature。但是，由于大部分的目标测试程序都含有成千上万条边，这样处理所需存储的参数量就会非常庞大，耗时太长。所以，我们需要对user features进行压缩以节省时间和空间开销。有以下几个步骤：1）执行所有的种子得到其执行路径，将所有的执行路径形成一个数据集，再利用k-means算法对所有的种子进行聚类，聚成N个类。2）提取出每个类的中心作为中心节点3）计算每个种子与这N个中心节点之间的相似度并构成一个N维特征向量，并以此来表征每个种子的路径特征。

\subsubsection{Reward.}
For higher coverage, we need to consider two factors: a) which positions are are structure-related in the current seed; b) which positions are more likely to generate new seeds that can discover new coverage. Therefore, we design the reward as:

$$
Reward = Changed * Rareness
$$

Among them, $Changed$ indicates whether the path is changed after the selected positions (i.e., arms) are mutated. This is to determine whether each position in the shared pool is structure-related. $Rareness$ refers to the rarity of the path taken by the mutated input. The rarer it is, the more valuable the mutation is. In other words, $Rareness$ is to further explore those more valuable positions.
%为了更高的coverage，我们需要考虑两个因素：1）哪些positions位于当前种子的结构字段之中；2）哪些positions更有可能生成可以发现new coverage的新种子。所以，我们将reward设计为：reward = changed * rareness.其中，changed表示对所选择的positions(i.e., arms)进行突变之后，是否造成了路径的改变。这是为了判断各个position是否位于当前种子的结构字段之中。rareness是指mutated input所走路径的稀有程度，越稀有说明本次突变越有可能发现新边。这是为了进一步发掘那些有价值的positions。

\subsubsection{The implement of LinUCB model.}
To save computation time, we use the LinUCB model for our purpose.

\textbf{Initialize.}
Each position in the shared pool needs to maintain a set of parameters ($A$ and $b$) for collecting user characteristics and corresponding rewards. $A$ and $b$ are initialized as
$$
    A = I_{d}
$$
$$
    b = 0_{(d*1)}
$$

\textbf{Calculate the fitness of each position in the shared pool.}
Given a seed $t$ with feature vector $x_{t}$ and a position $a$ recorded in shared pool with a unknown coefficient vector ${\theta}_{a}$.
The expected reward $E[r_{t,a}|x_{t}]$ that can be obtained at each position is:
$$
    E[r_{t,a}|x_{t}] = x_{t}^{T} * {\theta}_{a}
$$
Among them, $r_{t,a}$ is the reward of the seed $t$ at position $a$. And the optimal coefficient $\hat{\theta}_{a}$ can be estimated by the following formula:
$$
\hat{\theta}_{a} = A_{a}^{-1}b_{a}
$$

In addition to the expected reward, we also need to calculate the upper confidence bound for each position $U_{t,a}$, and the formula is as follows:

$$
    U_{t,a} = \alpha  \sqrt{x_{t}^{T} A_{a}^{-1} x_{t}}
$$

Therefore, the final fitness of each position $Fitness(t,a)$ is defined as:
$$
Fitness(t,a) = E[r_{t,a}|x_{t}] + U_{t,a}
$$
Then, we generate a probability distribution based on the fitness of each position and select positions to mutate according to it. The greater the fitness, the greater the probability that it will be selected for mutation.

%shared pool中的每一个position需要维护一组参数（A_a以及b_a）用于收集用户特征以及相应的reward，A_a和b_a分别初始化为 2）计算shared pool中每个position的fitness 对于一个种子来说，在每个position上所能够获得的期望收益如下：除了期望收益之外，我们还需要计算每个position的置信上界，公式如下所示：因此，每个position最终的fitness定义为：fitness = expected reward + 置信上界。然后，我们根据每个position的fitness生成概率分布，根据概率分布选择positions进行突变。如果fitness越大，那么其被选择进行突变的概率也就越大。

\textbf{Update parameter.}
Generally speaking, LinUCB only recommends the position with the highest fitness and then updates the parameters $A_{a}$ and $b_{a}$ according to the feature of the current seed and the obtained reward. However, in a mutation process of fuzzing, not only is a single position mutated but multiple positions are mutated simultaneously. Therefore, we need to design a parameter update strategy suitable for fuzzing.

To reduce the computation time, instead of updating the parameters after each mutation, we use the accumulated data to update after completing all mutations for a seed. 
When we mutating a seed $t$, the specific process is as follows:

a) We maintain an array $rewards[MAX]$ to record the reward accumulated by each position during the mutation process of seed $t$. Among them, $MAX$ is the maximum number of positions. Then, we maintain a data $hit\_nums[MAX]$ to record the number of times each position is selected.

b) Assume that $N$ positions are selected for mutation in a mutation process, and reward $c$ is obtained. Then we add the $average\ reward$ of this mutation to the $N$ positions in the rewards array. The $average\ reward$ is defined as:
$$
average\ reward = c/N
$$

c) When the mutation to seed $t$ is complete, we calculate the final reward for each position based on the $rewards$ and $hit\_nums$ arrays. For the position $a$ in the shared pool, the final reward $r_{t,a}$ is defined as: 
$$
r_{t,a} = rewards[a]/hit\_nums[a].
$$

d) Finally, we update the parameters $A_{a}$ and $b_{a}$ of all positions according to the feature vector $x_{t}$ of the seed and its final reward at each position:
$$
A_{a} = A_{a} + x_{t,a} x_{t,a}^{T}
$$
$$
b_{a} = b_{a} + r_{t,a} x_{t,a}
$$

\begin{algorithm}[!t]
\footnotesize
\caption{The implement of linUCB model}\label{alg:LinUCB}
\KwIn{$\alpha$ $\in$ $ \mathbb{R}_{+} $ }
\For{$ t = 1,2,3,...,T $}{
    $Observe\ the\ feature\ of\ the\ current\ seed\ t:x_{t} \in \mathbb{R}_{d}$\\
    $Fitness = []$\\
    \For{$ a \in all\ positions\ in\ shared\ pool $}{
        \If{$a\ is\ new$}{
            $A_{a} = I_{d}$\\
            $b_{a} = 0_{d*1}$\\
        }
        $\hat{\theta}_{a} = A_{a}^{-1}b_{a}$\\
        $p_{t,a} = \hat{\theta}_{a}^{T}x_{t} + \alpha  \sqrt{x_{t}^{T} A_{a}^{-1} x_{t}}$\\
        $Fitness \gets p_{t,a}$\\
    }
    $Distribution = Generate(Fitness)$\\
    $Mutate\ based\ on\ Distribution\ and\ calculate\ r_{t,a},\ a \in all\ positions$\\
    \For{$ a \in all\ positions\ in\ shared\ pool $}{
        $A_{a} = A_{a} + x_{t} x_{t}^{T}$\\
        $b_{a} = b_{a} + r_{t,a} x_{t}$\\
    }
}
\end{algorithm}


The specific algorithm of LinUCB is shown in the Algorithm~\ref{alg:LinUCB}.
Among them, the parameter $\alpha$ in line 0 determines whether it is inclined to exploration or exploitation.
Lines 3-10 calculate the expected reward of each position and its confidence interval to generate the final fitness.
Line 11 generates a probability distribution based on the fitness of each position.
Line 12 selects positions to mutate according to the distribution and collects the corresponding data.
Lines 13-15 update each position's parameter matrix according to each position's final reward and the current seed's feature vector.


\subsection{Mode scheduler}
\zhu{Maybe we can describe this part as the prioritization of input bytes. I think essentially, you prioritize the bytes in the shared pool, and then mutate the rest bytes. no?}\zkp{More precisely, the random mode is used to update the shared pool of each family, while the history mode dynamically selects appropriate positions from the shared pool for mutation according to the LinUCB model.}

Further, We construct two modes for the havoc stage, history mode and random mode. Each mode has its focal point. The details are shown as follows. \zhu{why?} \zkp{In random mode, we randomly select positions to mutate, and collect data to extract valuable positions to update the shared pool within each family. And history mode will extract positions from the shared pool for mutation based on LinUCB model. Therefore, history mode depends on random mode. We need an efficient mode scheduler that constantly switches between the two modes during fuzzing.}

\textbf{History Mode.}
In history mode, we pay attention to the structure field of mutation seeds.
Based on the shared pool in each family, we propose a history mode to use this information. When entering history mode, we use the LinUCB model to calculate the fitness of each position stored in the shared pool for the current seed and generate a probability distribution based on the fitness. Finally, we select the mutation position based on the probability distribution.

\textbf{Random Mode.}
Expect for history mode, we rename the normal mutation strategy as random mode.

\textbf{Mode scheduler.}
In order to find the best mode that should be used in the current mutation, we propose a novel mode scheduler. Specifically, we record the number of executions $ExecNum$ and new paths found $PathFound$ in each mode. As shown in Equation X, we calculate the number of executions needed to discover a new path ($per\_path\_cost$) for two modes. The smaller the $per\_path\_cost$ is, the higher the corresponding mode's efficiency. 
Finally, we select the best mode based on it.\zhu{how? based on probability?}\zkp{Instead of choosing based on probability, we directly choose the mode that currently performs best on $per\_path\_cost$.}
$$
per\_path\_cost = ExecNum / PathFound
$$


==> obsolete/technique-1.0.tex <==



\section{Design of \tool{}}
% \todo{subsections: \begin{itemize}
%     \item overview \begin{itemize}
%         \item describe figure
%     \end{itemize}
%     \item why do we use discover-new-edge positions (valuable positions)? \begin{itemize}
%         \item ???Only a part of CMP related bytes contribute to the coverage discovery. The SHAP experiment.
%         \item direct relation => combination of path constraints equals to combination of corresponding positions
%         \item indirect relation => in a different path, the constraint-related position is still related to path constraint
%     \end{itemize}
%     \item how to organize discover-new-edge positions: seed family \begin{itemize}
%         \item position mapping: maintain structure, same meaning for a position;
%         \item optimize the selection of positions in the shared pool: LinUCB
%     \end{itemize}
%     \item switch between expanding discover-new-edge positions and utilizing discover-new-edge positions: why do we need this?
%     \item discussion: \begin{itemize}
%         \item we can use different existing solutions to expand discover-new-edge positions
%     \end{itemize}
% \end{itemize}}






% \zhu{we first declare the difference between byte positions and input bytes. An input byte ignores the order of the byte, while a byte position considers the order of it.}

Our \tool{} focuses on the byte schedule and prefers the valuable byte positions. Based on our SHAP analysis, since valuable positions have already discovered new codes, we can predict that those positions can discover more codes in later fuzzing campaigns. Figure~\ref{Framework} shows the framework that our \tool{} utilizes the valuable positions to boost fuzzing. \tool{} establishes a family system to share valuable positions within family members, \ie seeds in a family. The shared positions will improve the performance of code discovery because of the coupled path constraints exemplified in Section~\ref{sec:motivation}. To schedule shared positions efficiently and effectively, \tool{} utilizes LinUCB, a contextual multi-armed bandit approach, to build probability distribution for selecting byte positions. Finally, the Mode Scheduler switches fuzzing between family-based mutation mode and random mutation mode. If existing valuable positions can no longer discover new codes, \tool{} will be switched to the random mutation mode to obtain new valuable positions. Note that, the random mutation mode can be replaced by the existing fuzzing solutions that resolve path constraints.



% % \subsection{Framework.}
% Motivated by the aforementioned observations, we design the \tool{} as a lightweight framework to perform mutations considering the coupling of path constraints.
% As shown in Figure~\ref{Framework}, the basic procedure of \tool{} contains the following three steps. 
% %First, \tool{} integrates the pilot stage into the havoc stage.
% First, we cluster seeds into multiple families based on inheritance relationship during the fuzzing process.
% Seeds within the same family maintain semantic consistency at a coarse-grained level.
% Second, all seeds in a family will jointly maintain a shared pool, sharing their valuable positions discovered in the mutation process.
% Each seed can exchange the valuable positions found by itself with other seeds based on shared pool.
% Third, as fuzzing is random, and the structure of the seeds can easily change during mutation.
% Thus, the positions recorded in the shared pool are not valuable positions for all seeds.
% In order to judge the relationship between each position in the shared pool and each seed in a more fine-grained manner, we utilize the LinUCB model to analyze the relationship between each seed and position in the shared pool. 
% Given a seed, LinUCB model generates a distribution for positions in the shared pool to indicate whether each position in the shared pool is a valuable position.
% Then, we group positions based on the distribution and perform mutation, called history mode. And we rename the normal mutation strategy as random mode.
% Random mode is used to collect information of valuable positions and history mode focus on mutating the inferred valuable positions.
% To achieve the best fuzzing efficiency, we need to schedule between the two modes at the right time.
% Fourth, a mode scheduling algorithm is proposed, which uses the mutation performance of each mode on the current seed to select the best mode dynamically.


% % • 为什么需要提取出valuable positions
% % 		‣ 从Motivation中的分析可知，解决direct relation需要反复翻转已探索过的constraints。
% % 		‣ 但是，利用传统的inference based的方法提取constraints的相关positions有以下几个缺点
% % 			• 需要设置额外的pilot stage，并且在处理长input太过费时
% % 			• 可能会提取到很多的冗余positions，这些positions并不能够翻转constraints
% % 		‣ fuzzing 过程中很容易获得大量的mutation information，可以用来提取能够翻转constraints的positions。
% % 		‣ 我们观察到：给定一个种子，如果对position i突变发现了新边，说明i一定是constraints的相关positions，并且能够翻转constraints
% % 		‣ valuable positions: positions that have discovered new code coverage.
% % 		‣ 那么，如果我们能够提取valuable positions，并且对valuable positions进行突变，就可以解决direct relation。
% % 		‣ 同时，我们对valuable positions进行组合，也可以解决indirect的问题
% % 		‣ 但是，基于上述观察提取valuable positions也存在一些问题
% % 			• fuzzing过程中一次并不是只突变一个position，而是同时突变多个positions。但是，并不是所有的positions的突变都对new edge的发现有帮助
% % 			• 基于上述观察提取valuable positions的方法需要对所有种子都分配足够的能量进行突变，这样才可以提取足够的数据用来提取valuable positions
% % 		‣ 为什么我们只考虑new edge，而不是path change？如果收集那些造成path change的mutation information的话，会存在数据量爆炸的问题。


% \subsection{why do we use valuable positions?}
% From the analysis in Motivation, it can be seen that solving the direct relation requires repeatedly flipping the constraints that have been explored. Flipping constraints requires mutating their related positions. However, using the traditional inference based method to extract the related positions of constraints has the following disadvantages.
% \begin{itemize}
%     \item Inference-based methods will set up a pilot stage before havoc stage to perform mutation testing on each byte in the input to observe whether the execution state change. Although the inference-based method is easy to implement, this method suffers from time-consuming problem for long input. 
%     For example, ProFuzzer is one of the widely used inference-based fuzzers. It needs to try all the values of each byte one by one and construct a feature vector based on the corresponding path length to analyze the specific type of each byte. Assume the input size is 10kB and the target program execute 1000 times per second. Thus, the required analysis time is 10240 * 256/1000 = 2621 seconds.
%     \item Not all related positions of constraints identified by inference-based methods can make the result flipped. For example, if you explore $if(a > 10000)$ in Greyone, where a is of type u32, and a is 0 from the initial seed. Although we can identify all related positions of a, only the high-order positions can flip this constraint. Thus the low-order positions are redundant for solving direct relation.
% \end{itemize}

% The fuzzing process can complete hundreds or thousands of mutations in one second, which can be used to extract positions that can flip constraints. Thus, there is no need to set the pilot stage for analysis, which improves the fuzzing efficiency. 
% We observe that if the mutation of position \textit{i} finds a new edge, it means that position \textit{i} must be the related position of constraints and able to flip constraints. 

% We define \textit{valuable positions} as the positions that have discovered new code coverage \zhu{defined in intro. keep this definition because it is used in later sections}. Then, if we can extract the valuable positions in the seed and mutate the valuable positions, we can solve the direct relation. At the same time, the combination of valuable positions can also solve the problem of indirect relation.
% Why do we only consider new edge, not path change? If we collect mutation information that causes path changes, there will be a problem of data explosion. And the collected data has a lot of redundant information.

% However, there are some problems with extracting valuable positions based on the above observations. 

% First, not only one position is mutated at a time, but multiple positions are mutated at the same time. However, not all mutations of positions are helpful for the discovery of new edges. Therefore, we desing an \textit{multiple positions inference algorithm} suitable for mutating multiple positions simultaneously.

% \textbf{Multiple Positions Inference Algorithm.}
% Essentially, if we can remove those mutated positions that are irrelevant to the discovery of new edges, leaving only the \textit{necessary} mutated positions, we can achieve mutating multiple bytes at the same time without causing an over-taint problem. The \textit{necessary} means that new edges cannot be found without mutating any position. 
% So we can get the following conclusion: if a mutated input mutates multiple \textit{necessary} positions and finds a new edge, then we believe these positions are valuable positions.
% Therefore, if we can de-duplicate mutated positions in the mutation information collected from the havoc stage, we can replace the dataset generated by the pilot stage with those mutation information.

% Second, if we want to analyze all seeds with the above method, then each seed needs to be allocated enough energy to mutate in havoc stage. However, not all seeds will be allocated much energy to mutate. Therefore, we propose a \textit{family system} to extract the valuable positions for the seeds with low energy.




\subsection{Family System}

To efficiently utilize valuable byte positions, \tool{} establishes a \textit{family system} to share and combine positions. \tool{} shares valuable positions to fuzz indirectly coupled path constraints, while it combines them to fuzz directly coupled path constraints.
The family system is required to ensure that the shared positions under different contexts (\ie execution paths) are still related to path constraints. 
Therefore, a family is built that, any seed $S_a$ (except the first one) in the family is added when $S_a$ is obtained by mutating another seed $S_o$ in the same family, without changing the length of $S_o$.
% Then, seeds in a family can roughly maintain the semantic meaning of byte positions.
In a family, \tool{} puts all valuable positions in a \textit{shared pool}. Since the length of a seed may be changed (\eg due to the trimming stage), \tool{} tracks the byte positions among seeds in a family.


\subsubsection{Shared Pool}
% \textbf{Shared Pool.}
Each family has its own shared pool.
When mutating a seed, \tool{} prefers to select byte positions from the shared pool. However, the number of valuable positions will be significantly decreased in later families because fuzzing can discover less and less new codes over time. Since the valuable positions are essentially the ones related to path constraints, we extend the definition of them based on families. 
If mutation of some positions can discover codes that all seeds in a family have never discovered, those positions are valuable positions in the family. 
Thus, the shared pool can capture the most of the path constraints related to a family. As shown in Figure~\ref{Framework}, seeds in a family can reuse and combine shared positions to improve efficiency of code discovery.


\subsubsection{Position Tracking}
Even though a family is built without mutations that change seed length, the length of a seed may still be changed, for example, by the trimming stage. To uniformly select byte positions when they are changed, all positions in a shared pool are recorded based on the first seed. \tool{} tracks the changes of positions among seeds so that positions are selected uniformly.
% To solve this problem, the byte positions recorded in a shared pool are the positions of the first seed in a family.
% Therefore, when using positions in the shared pool, we need to track the changed positions among seeds so that the positions are treated correctly. 
For instance, in Figure~\ref{trimming}, three seeds are in a family, where the seeds $S_1$ and $S_2$ are trimmed, and the seed $S_o$ is the first seed in the family.
On the one hand, if the forth position of seed $S_1$ discovers new codes, \tool{} will add the number 6 into the shared pool because it maps to the sixth position of seed $S_o$. On the other hand, when selecting the position 6 from the shared pool for the seed $S_2$, \tool{} will mutate the second byte of $S_2$ based on the position tracking.
As a result, \tool{} can correctly record and select valuable positions from a shared pool.

\begin{figure}[!t]
\includegraphics[width=\linewidth]{images/trimming.jpg}
\caption{Position tracking. \tool{} tracks the changes of byte positions.}
\label{trimming}
\end{figure}


\subsubsection{Family Update}
The key of building a family is that the mutation does not change the length of original seeds. However, many fuzzers mutate seeds via changing the length of seeds, such as inserting bytes and deleting bytes. To enrich family members, \tool{} will withdraw all mutators that change length when new codes are discovered.
If the result can still find the same new edges after withdrawing those mutators, \tool{} will retain the result to a family.
For example, as shown in Figure~\ref{fig:family_update}, if an input $i_1$ discovers new edges, \tool{} will withdraw all mutators that change length, which generates another input $i_2$. If $i_2$ can still find the same new edges that $i_1$ finds, \tool{} retains $i_2$ to a family.
Otherwise, $i_1$ will form a new family if mutation of $i_1$ can further discover new edges.
As a result, \tool{} has a reasonable number of families and family members.


\begin{figure}[!t]
\includegraphics[width=\linewidth]{images/upate.png}
\caption{The update of family and family members.}
\label{fig:family_update}
\end{figure}




% In Section~\ref{sec:motivation}, \todo{why do we propose family system?}



% To extract the valuable positions for the seeds allocated low energy, we proposes a \textit{family system} to achieve information sharing between seeds.
% Thus, we can extract the valuable positions for the seeds allocated low energy from the seeds allocated large energy. 
% Moreover, seeds can also exchange valuable positions they found with each other to speed up the analysis.
% As information sharing requires maintaining \textit{semantic consistency} (i.e., the same position on different seeds has similar meanings) between seeds, we proposes a \textit{family system} to group seeds with semantic consistency.
% However, the meaning of the same position on different seeds is often inconsistent, mainly due to the following reasons.
% \begin{itemize}
%     \item Problem I: Different initial seeds may have different structures, which may lead to inconsistent meanings of most positions between seeds. 
%     \item Problem II: Even if two seeds are mutated from the same initial seed, the use of length mutators will cause the seed length to change, which may change the structure of the seed.
%     \item Problem III: Trimming also affects semantic consistency between seeds.
% \end{itemize}
% Thus, we utilize \textit{family system} to solve problem I and II.
% And we solve the problem III based on a \textit{semantic tracking algorithm}, which tracks position mapping between seeds.

% \subsubsection{Definition of Family}
% We give the formal definition of Family: Suppose there are seeds \textit{a}, \textit{b}. Seed \textit{b} is derived from a mutation of seed \textit{a}, i.e., seed \textit{a} is the parent of seed \textit{b}. If no length mutators are used in the process of mutating seed \textit{a} to obtain seed \textit{b}, the seeds \textit{a} and \textit{b} belong to the same family.

% % At the same time, the family relationship is also transitive: if seeds $a$ and $b$ belong to the same family, and seeds $b$ and $c$ also belong to the same family, then seeds $a$, $b$, and $c$ belong to the same family.

% In each family, there are two roles: ancestor and offspring. The ancestor refers to the seed that forms the family, that is, the first seed to join the family. offspring refers to those new seeds that are mutated from the ancestor without using length mutators, including the ancestor's children, grandchildren, and so on.

% Then, the family needs to maintain a \textit{shared pool} to record valuable positions on all seeds within the family. All seeds in the family can access or add elements to the shared pool, and the subsequent mutation process will be performed based on the shared pool.

% However, the difficulty of finding new edges increases over time. Seeds that mutate first can discover more new edges easy to be found and collect a lot of data, 
% while seeds that mutate later are more likely to encounter data shortages. 
% Therefore, the valuable positions collected by the family processed first are richer than those processed later.
% To solve this problem, we designed a new indicator: \textit{local new edges}. \zhu{local new edges: increase the number of valuable positions in a family;}

% In AFL-based fuzzer, all seeds will maintain a global bitmap to record edges that have been found.
% If a seed discovers a new edge in the global bitmap, we call this new edge as \textit{global new edge}.
% To extract more useful mutation information, we maintain a local bitmap \zhu{local bitmap: for one family; later family may generate less and less valuable positions} for each initial seed to record edges found by it and its mutated inputs.
% If a mutated input generated from a seed \textit{t} finds a new edge in the local bitmap of seed \textit{t}, we call this new edge as \textit{local new edge}.
% Based on \textit{local new edges}, there will be no problem of insufficient data between families due to the problem of processing sequence.

% Finally, to implement the indicator of local new edge, each family maintains a local bitmap to record the edges found by the seeds in this family.

% \subsubsection{Family Scheduling Algorithm \zhu{Family Update}}

% We divide all the seeds into the Formal Part and Candidate Part. Seeds in the Formal Part will create a new family or belong to an existing family, while seeds in the Candidate Part will not belong to any family.

% \textit{Family schedule.}
% In order to avoid the explosion of the number of families caused by the excessive number of initial seeds, we use whether new edges are found as an indicator for assigning the initial seeds to the Formal Part. So, if an initial seed finds a new edge, it will be added to the Formal Part to form a new family and become the ancestor  of this family; otherwise, it will be added to the Candidate Part.
% Then, if the seed in the Candidate Part found multiple new edges during the mutation process, we migrate it to the Formal Part, form a new family, and become a ancestor .
% \zhu{if seeds in candidate part can further discover new edges, we will form a new family. At least two seeds in a family?}

% \textit{Update the offspring sequence.}
% When we mutate seed \textit{i} to obtain new seed \textit{s}, if length mutators are not used in the mutation process, the new seeds will be added to the offspring sequence of the family where seed \textit{i} is located. However, to maintain the semantic consistency in a family, the mutated inputs generated from length mutators can not be included. These inputs will be added to the Candidate Part, which does not maintain a shared pool. Thus, the seeds in the Candidate Part can not leverage the stored positions in the shared pool to mutate.

% However, the using of length mutators to generate mutated inputs is common. If we do not impose any restrictions on using length mutators, the number of seeds stored in the Formal Part will be small, but the Candidate Part will be large. Thus, we should try to limit the use of length mutators. Therefore, we propose a grammar preservation system to maintain semantic consistency.

% The length mutators could be used in the havoc stage, which breaks the semantic consistency. During one mutation, we store the length mutators used in a stack—the details as shown in Figure~\ref{withdraw}. The length mutators can be divided into two categories, insertion and deletion. For insertion, we record the inserted position and the memory length to be inserted. For deletion, we extra record the deleted memory. If a new edge is found, we pop mutators one by one from the top of the stack and withdraw all mutators. In the withdrawing stage, we delete the inserted memory for the insertion mutator and insert the deleted memory for the deletion mutator. 
% As shown in Figure~\ref{withdraw}, we give an example. First, we get the first mutator, i.e., (insertion,1,1), from the top of the stack. To withdraw this insertion mutator, we delete the inserted memory block marked in red. Second, we get the next mutator (deletion,4,3). Then we need to insert the memory block marked in green. 

% After all length mutators have been withdrawn, we put the withdrawn input into the target program. If the new edge still can be found, we retain the withdrawn input into the seed corpus. Otherwise, we still retain the original mutated input into the seed corpus.

% \begin{figure}[htbp]
% \includegraphics[width=\linewidth]{images/withdraw.jpg}
% \caption{The withdraw operation.\zhu{delete this figure, and add one to show the update of family and family members?}}
% \label{withdraw}
% \end{figure}


% \subsubsection{Semantic Tracking Algorithm\zhu{Position Tracking}}
% \zhu{absolute position is more important than relative position in format. absolute position: positions in original seed; relative position: positions within seeds}

% Due to trimming, although length mutators are not used in the generation of offspring, differences in length may still occur between seeds within the same family.
% If we directly record the relative positions of the valuable positions in each seed into the shared pool, there will be a problem of semantic inconsistency. 
% For instance, \textit{seed A} is generated from \textit{initial seed} by trimming the red block as shown in Figure~\ref{trimming}. If we mutate the fourth position and find a new edge, we add '4' into the shared pool. However, as position 4 in \textit{seed A} corresponds to position 6 in \textit{initial seed}  based on the trimming relationship, position 4 in \textit{seed A} and \textit{initial seed}  have different meanings. Thus, we cannot directly use '4' to locate the valuable position of the initial seed. 

% Each seed has an independent relative position space, and the position inside the seed is called the \textit{relative position}.
% To achieve semantic consistency between seeds, we need to map the relative position of each seed to the same absolute position space.
% Specifically, before adding the valuable positions into the shared pool, we need to convert the relative positions in each seed into absolute positions, so that we can express them uniformly.
% % As only delete mutators will be used in the trimming stage, the length of the seeds must be shortened or consistent after trimming.
% According to the definition of the family, only the input generated from a seed without using length mutators can be included in a family.
% Then, the length of seeds in a family's offspring sequence must be shorter than the ancestor in this family because of trimming.
% Thus, we set the ancestor as the benchmark of its family.
% If the relative position i is corresponding to position j in the ancestor according to the trimming chain, the position j is called \textbf{absolute position}.

% Therefore, each seed needs to maintain a \textbf{mapping vector} with the same length as its own to complete the mapping from relative positions to absolute positions.
% We show a example in Figure~\ref{trimming}. Assume that in a family, the ancestor has 7 bytes, so that its map\_vector is [1,2,3,4,5,6,7]. And a trimmed seed generated from ancestor by trimming down the fourth and fifth bytes, so that its map\_vector is [1,2,3,6,7]. For instance, \textit{6} in the map\_vector of trimmed seed means that the fourth byte in trimmed seed is corresponding to the sixth byte in ancestor. Further, if a input B generated from seed A by trimming down the first 2 bytes, the map\_vector of B will be [3,6,7].
% Finally, the positions recorded by the shared pool are absolute positions. When each seed interacts with the shared pool, it needs to use the map vector to convert its relative positions into absolute positions first, so that there will be no semantic inconsistency.


% \begin{figure}[htbp]
% \includegraphics[width=\linewidth]{images/trimming.jpg}
% \caption{The example of mapping mechanism.}
% \label{trimming}
% \end{figure}

% \begin{algorithm}[!t]
% \footnotesize
% \caption{Update the structure-related absolute positions stored in shared pool.}\label{alg:SharedPool}
% \KwIn{
% The seed being mutated, $s\_orig$.
% The mapping vector of $s\_orig$, $m$.
% The mutated input found new edges generated from $s\_orig$, $s$.
% The Candidate Part, $C$.
% The stack that record the length mutators have been used, $Stack$. 
% }
% \If{$s\_orig \in C$ }{
%     $C \gets s$
% }\Else{
%     \If{$Stack \neq \emptyset$ }{
%         $RecoveredInput = Withdraw(Stack)$\\
%         \If{$RecoveredInput\ can\ find\ the\ same\ new\ edges$ }{
%             $s = RecoveredInput$\\
%         }\Else{
%             $C \gets s$
%         }
%     }\Else{
%         \For{$ t = 1,2,3,...,Length $}{
%             \If{$s[t] \neq s\_orig[t]$ }{
%                 $tmp = s[t]$\\
%                 $s[t] = s\_orig[t]$\\
%                 \If{$s\ can\ not\ find\ the\ same\ new\ edges$ }{
%                     $s[t] = tmp$\\
%                     $Record\ m[t]\ into\ the\ shared\ pool\ of\ the\ family$\\
%                     $where\ s\_orig\ is\ located$\\
%                 }
%             }
%         }
%         $Record\ s\ into\ the\ Offspring\ Sequence\ of\ the\ family$\\
%         $where\ s\_orig\ is\ located$\\
%     }
% }
% \end{algorithm}

% \textbf{Overall Algorithm.}
% Algorithm~\ref{alg:SharedPool} shows how the shared pool of each family is updated.
% If a mutated input generated from a seed that exists in the Formal Part finds a new edge, we need to withdraw all the length mutators. If the withdrawn input can not find the same new edge, we add the original mutated input into the Candidate Part. Otherwise, we need to withdraw redundant mutations to keep the minimal change while maintaining the same effect, which ensures the accuracy of the positions stored in the shared pool. If we do not do that, almost all positions will be added to the shared pool. 

% More specifically, we compare the withdrawn input with the original seed byte by byte. For mutated position i, we reset it with the corresponding value in the original seed and put it into the program. If the same new edge still can be found, we reset the next mutated position. Otherwise, we withdraw this resetting operation and add map[i] (i.e., the absolute position of position i) into the shared pool. For instance, if a mutated input is [1,2,3,6,7], its original seed is [1,2,3,4,5], and its map vector is [1,2,3,7,8], we first reset the value of the fourth byte to 4 and test it. We find the same new edge is exercised so that we reset the next mutated position.
% Then we reset the value of the fifth byte to 5. However, a new edge can not be found. Thus, we withdraw this resetting operation, i.e., set the fifth byte to 7, and add map[5]=8 into the shared pool.

\subsection{Contextual Bandit for Byte Schedule}

The family system can only roughly ensure that positions in a shared pool are related to path constraints under any context. Over time, a newly added seed may be completely different to the first seed in the same family in terms of input format. That is, these two seeds may exercise different program logics. 


To optimize the selection of shared positions so that they are related to path constraints, \tool{} models the problem of selecting positions as a contextual multi-armed bandit (CMAB) problem. 
Based on the experience of playing some arms, the CMAB intends to optimize the rewards of playing multi-armed bandits, considering the personality of a player (\ie the context). 
The CMAB problem is the trade-off between playing more arms and focusing on some specific arms, \ie the problem of \textit{exploration vs. exploitation}.
For byte schedule, each byte position in a shared pool is an arm, and the seed selecting positions is the player. Meanwhile, the context for the CMAB problem is the execution path that the current seed exercises. 
% Therefore, the CMAB for \tool{} intends to optimize the selection of shared positions so that they are related to constraints that the current seed examines.
Therefore, the CMAB for byte schedule is to balance between trying out some positions and focusing on the best positions. 
\tool{} utilizes LinUCB~\cite{linucb}, one of the solutions for the CMAB problem, to build a probability distribution for selecting positions.

\subsubsection{Scores of Positions}
The probability distribution is built based on the scores of positions, where positions with larger scores have higher chance to be selected.
The scores calculated by LinUCB includes the expected reward and the upper confidence bound.
Given a seed $s$ with the feature vector $x_{s}$ (\ie the context) and a position $p$ recorded in a shared pool, the expected reward $E[r_{s,p}|x_{s}]$ can be calculated by:
\begin{equation} \label{equ:E_calculation}
E[r_{s,p}|x_{s}] = x_{s}^{T} * A_{p}^{-1}b_{p},
\end{equation}
where $r_{s,p}$ is the reward of the seed $s$ at position $p$, and $A_{p}$ and $b_{p}$ are the parameters maintained by the position $p$. Both $A_{p}$ and $b_{p}$ will be updated during fuzzing. 



The second part of a score is the upper confidence bound $U_{s,p}$, which is calculated as:
\begin{equation} \label{equ:U_calculation}
U_{s,p} = \sqrt{x_{s}^{T} A_{p}^{-1} x_{s}}
\end{equation}



Then, the score of each position $Score(s,p)$ is defined as:
\begin{equation} \label{equ:Fitness_calculation}
Score(s,p) = E[r_{s,p}|x_{s}] + \alpha U_{s,p},
\end{equation}
where $\alpha$ is a hyper-parameter for users to set.
Based on our experience, we set $\alpha = 0.5$ in our experiments.
For Equation~(\ref{equ:Fitness_calculation}), the more a position is selected, the smaller its $U_{s,p}$ is. Therefore, \tool{} achieves the trade-off between exploration and exploitation.


\subsubsection{Feature Vector (The Context)} 
Different from other fuzzers, our \tool{} considers the context when optimizing byte selection. The calculation of both $E[r_{s,p}|x_{s}]$ and $U_{s,p}$ contains the context $x_s$. Recall that the selected shared positions need to be related to path constraints for the current seed. Since edges contain path constraints, \tool{} uses the set of edges that the current seed examines as the context. 
Usually, the number of edges is large in an execution path, which leads to the oversize feature vector. 
To solve this problem, \tool{} compresses a set of edges into a fixed dimensional vector by using K-means clustering~\cite{kmeans}. 
As shown in Figure~\ref{FeatureGeneration}, \tool{} first collects all the exercised execution paths into bitmaps, in which the examined edges are marked with 1 or otherwise 0. Then, the K-means is utilized to cluster seeds into $k$ classes based on their corresponding execution paths. Based on our experience, we set $k = 20$. The feature vector of a seed is now a $k$-dimensional vector, of which each dimension is calculated based on the Jaccard similarity between the current execution path and the central path of a class. For Jaccard similarity~\cite{jaccard1912distribution}, given two seeds $s_1$ and $s_2$, and their corresponding paths $\mathcal{P}_{s_1}$ and $\mathcal{P}_{s_2}$, the similarity $Similarity(s_1, s_2)$ between seeds $s_1$ and $s_2$ can be calculated as:

\begin{equation}
    Similarity(s_1, s_2) = \frac{|\mathcal{P}_{s_1}\cap \mathcal{P}_{s_2}|}{|\mathcal{P}_{s_1}\cup \mathcal{P}_{s_2}|}
\end{equation}
where edges in $\mathcal{P}_{s_1} \cap \mathcal{P}_{s_2}$ belong to both paths, and edges in $\mathcal{P}_{s_1} \cup \mathcal{P}_{s_2}$ contain all edges in both paths. $|\bullet|$ is the number of edges.

\begin{figure}[!t]
\includegraphics[width=\linewidth]{images/FeatureGeneration.jpg}
\caption{K-means Based Feature Generation Algorithm.}
\label{FeatureGeneration}
\end{figure}


\subsubsection{Parameter Update}
The other part of Equation~(\ref{equ:Fitness_calculation}) is to update the parameters $A_p$ and $b_p$ for the position $p$, which are calculated by:

\begin{equation} \label{equ:A_update}
A_{p}^{n+1} = A_{p}^{n} + x_{s} x_{s}^{T},
\end{equation}
\begin{equation} \label{equ:b_update}
b_{p}^{n+1} = b_{p}^{n} + r_{s,p} x_{s},
\end{equation}
where $n$ is the step that $A_{p}$ and $b_{p}$ are updated, and $r_{s,p}$ is the reward that mutation of the position $p$ in the seed $s$ obtains. 


Different from the original LinUCB that a reward is obtained by playing one arm, fuzzing has a high chance to play multiple arms at a time, \ie mutating multiple shared positions simultaneously. In this case, the reward is not for a single position, but for multiple positions. Therefore, \tool{} assigns the average reward to each selected position. The reward is calculated as:

\begin{equation} \label{equ:final_reward}
    r_{s,p} = \frac{\sum_{i}^{N_{hits}}(\frac{r_i}{M_i})}{N_{hits}},
\end{equation}
where $r_i$ is the reward for the i-th time that the position $p$ is selected, and $M_i$ is the number of all positions being selected at the i-th time. The term $\frac{r_i}{M_i}$ is then the average reward assigned to the position $p$ at the i-th time. To speed up the updating process, \tool{} calculates the final reward for a position after the mutation for a seed has completed. Thus, $N_{hits}$ in Equation~(\ref{equ:final_reward}) is the total number of times the position $p$ has been selected.
Finally, $r_{s,p}$ is the average reward of all mutations that select the position $p$ in the seed $s$.  

% \zhu{fuzzing plays multiple arms (mutating multiple positions) at a time, and the reward is for all the mutated positions, which cannot be separated. So we divide the reward by N selected positions, and assign the result to each position.}


\subsubsection{Individual Reward}
The Equation~(\ref{equ:final_reward}) needs the individual reward $r_i$ for a single selection of multiple positions. 
Since \tool{} intends to schedule constraint-related positions, a straightforward reward is the change state after mutating a position. However, such kind of reward only has two values 0 and 1. To further differentiate positions, we introduce the \textit{frequency} of a seed being mutated to the calculation of rewards. Equation~(\ref{equ:Reward}) is the reward used by \tool{}: 

\begin{equation} \label{equ:Reward}
r_i = IsChanged \times f,
\end{equation}
where \textit{IsChanged} is 1 when the path changes or otherwise 0, and $f$ is the frequency that the seed is mutated. The frequency is calculated as $f = \frac{N_{mut}}{N_{total}}$, and $N_{mut}$ is the number of mutations that perform on the seed and $N_{total}$ is the total number of executions during fuzzing.

% \begin{equation} \label{equ:freq}
% f = \frac{N_{mut}}{N_{total}}
% \end{equation}


% Based on the shared pool in each family, we propose a novel family-based mutation strategy to group valuable positions to be mutated for each seed.
% In a family, since the fuzzing mutations are random, a completely different new seed may appear after many mutations. In other words, semantic consistency of this seed is violated with other family seeds. At this time, the valuable positions recorded in the shared pool of the family may be useless to this seed. To solve this problem, we use the LinUCB model to analyze the relationship between all positions in the shared pool and the current seed.
%在一个family中，由于fuzzing的突变都是随机的，所以在经过多次的突变之后，有可能会出现一个完全不一样的新种子，也就是与该family的其他种子之间违背了语义一致性。这时候，该family的shared pool所记录的结构字段的absolute positions就不再适用于这个新种子。为了解决这个问题，我们利用cMBA model来建模shared pool中的所有positions与当前种子的关系。

% \subsubsection{Why do we use LinUCB?}
% %What is byte schedule
% %引出fuzzing的EE问题 -> 说明user是什么，arm是什么
% %MAB在解决fuzzing的EE问题上表现很好，但是，它们都不是个性化的
% %所以，我们引入CBA
% %CBA在选择时会考虑到user的特性，即context。例如，对学生推荐电脑产品等等。
% %而在fuzzing中，context是每个种子自己的特性，即自己的结构特征；也就是说，我们根据种子自身的结构特征在shared pool中进行种子选择。
% %throughout -> 最终选择LinUCB
% Given a seed, we perform byte schedule to determine which position to be mutated from the shared pool.
% Due to the randomness of fuzzing, not all positions in the shared pool are useful for the current seed.
% Thus, we need to find positions from the shared pool that are useful for the current seed during the mutation process.
% In essence, byte schedule is actually solving the \textit{Exploration \& Exploitation} problem.
% We treat the \textit{arm} as the position in shared pool and \textit{reward} as the performance of this mutation (e.g., finding a new edge), and define the \textit{user} as the current seed.
% In the \textit{Exploration} stage, we tend to try out some positions in shared pool to get more information to describe the relations between the positions and the current seed.
% In the \textit{Exploitation} stage, we tend to select those positions that have performed best in the past.

% In previous studies, the Multi-Armed Bandits(MBA) model has been shown to have a good effect on the \textit{Exploration \& Exploitation} problem of seed schedule. For example, EcoFuzz proposes a variant of the Adversarial Multi-Armed Bandit (VAMAB) model and use it to model seed schedule problem. Specifically, it treats each seed as an arm and defines the reward of each trial as generating an input that triggers a new path.

% % After we determine which seed to be mutated, we need to select appropriate positions from the shared pool to mutate, i.e. byte schedule.
% % Therefore, the most intuitive idea is to use the MBA model for processing. \zhu{more reason} \zkp{In previous studies, the MBA model has been shown to have a good effect on seed schedules. For example, EcoFuzz treats each seed as an arm and defines the reward of each trial as generating an input that triggers a new path. Since the position selection problem is essentially an $Exploration\ \&\ Exploitation$ problem}, we regard the positions recorded in the shared pool as arms and define the reward of each trial as generating an input that triggers a new path.

% However, MBA model is a context-free algorithm. MBA assumes that the reward of each arm does not change with different users. 
% If we use MBA model to model our byte schedule problem, a positions in the shared pool is either useful or useless for all seeds at the same time.
% This also hides an assumption: A position in the shared pool has the same meaning for different seeds.
% However, it is unrealistic since the mutation is a random process. Some anomalous seeds with significant structural changes may be generated. For these abnormal seeds, it is necessary to identify which positions in the shared pool are useless for themselves.
% Therefore, we need to consider the seeds' characteristics (i.e., user characteristics) to get a personalized byte schedule. Therefore, we adopt the contextual bandit algorithm, which considers contextual information when solving the \textit{Exploration \& Exploitation} problem. We treat the \textit{context} as the features of the current. Thus, we construct a personalized byte schedule based on the features of the seeds.

% Since throughput is an essential indicator in fuzzing, we need a more lightweight algorithm. Thus, we finally chose LinUCB \cite{linucb} for modeling.
% LinUCB is a general contextual bandit algorithm that has a high calculation speed.
% % \subsubsection{How to model Byte schedule with LinUCB}
% To model byte schedule based on LinUCB model, we regard the seed as a \textit{user} and the positions recorded in the shared pool as \textit{arms}. 
% In addition, we also need to address the following issues.
% \begin{itemize}
%     \item How to get the \textit{context} and \textit{reward}?
%     \item How to use LinUCB for byte scheduling?
%     \item How to update parameters of LinUCB?
% \end{itemize}

% In the recommendation scenario, different users have different points of interest, preferences, purchasing power and other factors. Therefore, it is necessary to provide users with personalized recommendations, i.e., contextual-bandit algorithm.


% \subsubsection{LinUCB Model.}
% %概括LinUCB的总体流程
% Following previous work \cite{linucb, langford2007epoch}, the main workflow of LinUCB is as follows. 

% % Recommendation Scenario. Suppose there are $A$ arms to be recommended and the LinUCB model will make $N$ trials.


% \textbf{Symbols Definition.}
% \begin{itemize}
%     \item We define the user as $u$ and a set $\mathcal{A}$ of arms.
%     \item A user can get a payoff $r$ after selecting an arm.
%     \item A feature vector $x$ can be constructed between the information of each user and each arm, i.e. $context$.
%     \item Each arm maintains two parameters $A$ and $b$ for accumulating the previous feature vectors and their payoffs.
% \end{itemize}

% \textbf{The Recommendation Process of LinUCB.}
% Suppose there are $\mathcal{A}$ arms to be recommended and the LinUCB model will make $T$ trials. In trial $t$:
% \begin{itemize}
%     \item Since the users and the arms that can be selected under different trials may be different, we get the current user $u_{t}$ and a set $\mathcal{A}_{t}$ of arms, and observe features of all arms $a \in \mathcal{A}_{t}:x_{u_{t},a}$
%     % The user $u_{n}$ and each arm $a \in A_{n}$ can compose a feature vector $f_{u_{n},a}$ of their respective information, i.e. $context$.
%     \item Considering the payoff estimate and model uncertainty reduction, We calculate a fitness $p_{t,a}$ for each arm $a \in \mathcal{A}_{t}$ based on the Equation \ref{equ:E_calculation}.
%     % the expected reward $E[r_{t,a}|x_{u_{t},a}]$ of each arm $a \in A_{t}$ based on the Equation \ref{equ:E_calculation}.
%     \begin{equation} \label{equ:E_calculation}
%     p_{u_{t},a} = x_{u_{t},a}^{T} * A_{a}^{-1}b_{a} + \alpha  \sqrt{x_{u_{t},a}^{T} A_{a}^{-1} x_{u_{t},a}}
%     \end{equation}
%     % Based on the history data, LinUCB selects a arm $a_{t}$ according to feature vectors, and observes the corresponding reward $r_{u_{t},a_{t}}$, that is, the rewards that $u_{t}$ gets on $a_{t}$.
%     \item Choose arm $a_{t}$ = $\arg\max_{a \in A_{t}}p_{u_{t},a}$ and observe the corresponding payoff $r_{t}$
%     \item Update the parameters $A$ and $b$ of each arm $a$ based on Equation \ref{equ:A_update} and \ref{equ:b_update}.
%     \begin{equation} \label{equ:A_update}
%     A_{a} = A_{a} + x_{u_{t},a} x_{u_{t},a}^{T}
%     \end{equation}
    
%     \begin{equation} \label{equ:b_update}
%     b_{a} = b_{a} + r_{t} x_{u_{t},a}
%     \end{equation}
%     % Construct the $(f_{u_{n},a_{t}}, a_{t}, r_{u_{t},a_{t}})$ tuple for updating the recommendation strategy of LinUCB.
%     \item Repeat the above steps to continuously update the recommended strategy.
% \end{itemize}


% To model byte schedule based on LinUCB model, we regard the seed as a user and the positions recorded in the shared pool as arms. 
% In addition, 
% % LinUCB also needs to determine two key factors: user feature and reward.
% we also need to address the following issues.
% \begin{itemize}
%     \item What are the feature vector and reward?
%     \item How to use LinUCB for byte schedule?
%     \item How to update parameters of LinUCB?
% \end{itemize}


%Why we use cMBA？当我们确定好将要被突变的种子之后，我们需要从shared pool中选择合适的positions进行突变。因此，最直观的想法就是利用MBA模型进行处理：regard the positions recorded in shared pool as arms and define the reward of each trial as generating an input that triggers new path. 但是，MBA是一个context free的算法。MBA有一个前提假设：假设各个arm的reward并不会随着用户的变化而变化，即假设shared pool中的同一position对于不同的seeds而言都具有相同的意义。这显然是不现实的，因为突变是一个随机的过程，完全可能生成出一些结构发生剧烈变化的新种子。对于这些异常种子，就需要识别出shared pool哪些positions对于该种子而言是无用的。所以，我们需要将种子自身的特征考虑进来（i.e., 用户特征），得到个性化的选择方案。因此，我们采用Contextual Bandit算法，这类算法在实现E&E时考虑了上下文信息，因而更加适合实际的个性化推荐场景。因此，we regard the seed as user，and regard the positions recorded in shared pool as arms. 此外，cMBA还需要确定两个关键因素：user feature以及reward。


% \subsubsection{How to use LinUCB for byte schedule?}
% % To save computation time, we use the LinUCB model for our purpose.

% \textit{Initialize.}
% In LinUCB \cite{linucb}, each arm (i.e., each position in the shared pool) needs to maintain a set of parameters (\textit{A} and \textit{b}) for accumulating feature vectors and corresponding rewards. And \textit{A} and \textit{b} are initialized as
% \begin{equation} \label{equ:A_definition}
% A = I_{d}
% \end{equation}
% \begin{equation} \label{equ:b_definition}
% b = 0_{(d*1)}
% \end{equation}
% Among them, \textit{d} represents the length of feature vector.

% % \textit{Calculate the $fitness$ of each position in the shared pool.}
% \textit{Select positions to be mutated.}
% Both \textit{exploration} and \textit{exploitation} should be taken into account when choosing positions. 
% Thus, given a seed, we calculate a fitness for each position in the shared pool to represent the possibility of being selected.
% To achieve \textit{exploitation} and \textit{exploitation}, we introduce the expected reward and the upper confidence bound of each position into the calculation of \textit{fitness}.


% Given a seed \textit{s} with feature vector $x_{s}$ and a position \textit{p} recorded in shared pool, the expected reward $E[r_{s,p}|x_{s}]$ that can be obtained by Equation \ref{equ:E_calculation}.
% % \begin{equation} \label{equ:E_calculation}
% % E[r_{s,p}|x_{s}] = x_{s}^{T} * A_{p}^{-1}b_{p}
% % \end{equation}
% Among them, $r_{s,p}$ is the reward of the seed \textit{s} at position \textit{p}. And $A_{p}$ and $b_{p}$ are the parameters maintained by positions \textit{p}.
% % And the optimal coefficient $\hat{\theta}_{a}$ can be estimated by the following formula:
% % \begin{equation} \label{equ:theta_calculation}
% % \hat{\theta}_{a} = A_{a}^{-1}b_{a}
% % \end{equation}

% In addition to the expected reward, we also need to calculate the upper confidence bound for each position $U_{s,p}$ based on the Equation \ref{equ:U_calculation}:
% % \begin{equation} \label{equ:U_calculation}
% % U_{s,p} =   \sqrt{x_{s}^{T} A_{p}^{-1} x_{s}}
% % \end{equation}

% Therefore, the \textit{fitness} of each position \textit{Fitness(s,p)} is defined as:
% % \begin{equation} \label{equ:Fitness_calculation}
% % Fitness(s,p) = E[r_{s,p}|x_{s}] + \alpha U_{s,p}
% % \end{equation}
% Among them, $\alpha$ is used to choose whether to prefer exploration or exploitation.
% The smaller the $\alpha$, the more prone to exploitation.

% Finally, we generate a probability distribution based on the fitness of each position and select positions to mutate according to it. The greater the fitness, the greater the probability that it will be selected for mutation.

%shared pool中的每一个position需要维护一组参数（A_a以及b_a）用于收集用户特征以及相应的reward，A_a和b_a分别初始化为 2）计算shared pool中每个position的fitness 对于一个种子来说，在每个position上所能够获得的期望收益如下：除了期望收益之外，我们还需要计算每个position的置信上界，公式如下所示：因此，每个position最终的fitness定义为：fitness = expected reward + 置信上界。然后，我们根据每个position的fitness生成概率分布，根据概率分布选择positions进行突变。如果fitness越大，那么其被选择进行突变的概率也就越大。

% \subsubsection{Feature vector in context.}
% The \textit{context} of a seed is generally expressed in terms of \textit{feature vector}.
% Essentially, what causes the positions in the shared pool to be useless for the current seed is that the structure of the seed has changed in the mutation.
% However, the most intuitive feature that can reflect the structural changes between seeds is the execution path of the seeds. If the structure changes, it is likely that the execution path of the seed will also change. 
% Thus, the easiest way is to use the edges that the seed passes through as the feature vector. However, since most target test programs have tens of thousands of edges, the number of parameters to be stored for processing would be huge.
% Therefore, we need to compress the feature vector to save time and space overhead. As shown in Figure~\ref{FeatureGeneration}, we have the following steps:

% a) Execute all the seeds to get their execution paths, form them into a dataset, and then use the k-means algorithm to cluster all the seeds into N classes.

% b) Extract the center of each class as the central node.

% c) Calculate the similarity between each seed and the N central nodes to form an N-dimensional feature vector. We set N to 20 finally. Then we use this vector to characterize the path feature of each seed. We use Jaccard similarity coefficient to measure the similarity. Given two seeds \textit{a} and \textit{b}, and assume that seed \textit{a} exercises the path $P_{a}$ and seed \textit{b} exercises the path $P_{b}$. The similarity \textit{s(a,b)} between seeds \textit{a} and \textit{b} can be calculated as:

% $$
% s(a,b) = \frac{|P_{a}\cap P_{b}|}{|P_{a}\cup P_{b}|}
% $$

% \begin{figure}[htbp]
% \includegraphics[width=\linewidth]{images/FeatureGeneration.jpg}
% \caption{K-means Based Feature Generation Algorithm.}
% \label{FeatureGeneration}
% \end{figure}

%能够反应种子之间结构发生变化的最直观的特征就是种子的执行路径。如果结构发生了变化，那么种子的执行路径很可能也会发生变化。所以，最简单的方法就是把种子所经过的边作为user feature。但是，由于大部分的目标测试程序都含有成千上万条边，这样处理所需存储的参数量就会非常庞大，耗时太长。所以，我们需要对user features进行压缩以节省时间和空间开销。有以下几个步骤：1）执行所有的种子得到其执行路径，将所有的执行路径形成一个数据集，再利用k-means算法对所有的种子进行聚类，聚成N个类。2）提取出每个类的中心作为中心节点3）计算每个种子与这N个中心节点之间的相似度并构成一个N维特征向量，并以此来表征每个种子的路径特征。

% \subsubsection{Reward.}
% \zhu{for updating parameters.}
% Our goal of modeling the byte schedule using LinUCB is twofold: one is to find useful positions in the shared pool for each seed within the family and construct a personalized byte schedule. The another one is to mutate those that are more likely to generate new seeds that can discover new coverage. Therefore, we design the reward as:

% % \begin{equation} \label{equ:Reward}
% % Reward = Changed \times Rareness
% % \end{equation}

% Among them, \textit{Changed} indicates whether the path is changed after the selected positions (i.e., arms) are mutated. This is to determine whether each position in the shared pool is useful, i.e., whether the constraints of the program can be reversed. 
% \textit{Changed} is a Boolean variable. \textit{Changed} takes 1 when the mutated input is inconsistent with the execution path of the initial seed. Otherwise, \textit{Changed} takes 0.

% \textit{Rareness} refers to the hit frequency by previously-generated inputs.
% Given a path \textit{P} and the number of times it has been hit \textit{h}, the \textit{Rareness} of the path \textit{P} is calculated by \ref{equ:Rareness}.
% \begin{equation} \label{equ:Rareness}
% Rareness = \frac{h}{Total\_execs}
% \end{equation}

% Among them, \textit{Total\_execs} is the total number of executions in the fuzzing process.
% The rarer the path is, the more valuable this mutation is. 
% % In other words, $Rareness$ is to further explore those more valuable positions.
% %为了更高的coverage，我们需要考虑两个因素：1）哪些positions位于当前种子的结构字段之中；2）哪些positions更有可能生成可以发现new coverage的新种子。所以，我们将reward设计为：reward = changed * rareness.其中，changed表示对所选择的positions(i.e., arms)进行突变之后，是否造成了路径的改变。这是为了判断各个position是否位于当前种子的结构字段之中。rareness是指mutated input所走路径的稀有程度，越稀有说明本次突变越有可能发现新边。这是为了进一步发掘那些有价值的positions。


% \subsubsection{Update parameters of LinUCB}
% Generally speaking, LinUCB only recommends the position \textit{p} with the highest fitness, and then updates its parameters $A_{p}$ and $b_{p}$ according to the feature of the current seed and the obtained reward. However, in a mutation process of fuzzing, not only is a single position mutated but multiple positions are mutated simultaneously. Therefore, we need to design a parameter update strategy suitable for fuzzing.

% To reduce the computation time, instead of updating the parameters after each mutation, we use the accumulated data to update after completing all mutations for a seed. 
% When we mutating a seed \textit{s}, the specific process is as follows:

% a) We maintain an array \textit{rewards[MAX]} to record the reward accumulated by each position during the mutation process of seed \textit{s}. Among them, \textit{MAX} is the maximum number of positions. Then, we maintain an array \textit{hit\_nums[MAX]} to record the number of times each position is selected.

% b) Assume that \textit{N} positions are selected in a mutation, and reward \textit{r} is obtained. Then we add the \textit{average reward} of this mutation to the \textit{N} positions in the rewards array. The \textit{average reward} is defined as Equation \ref{equ:average_reward_calculation}.
% \begin{equation} \label{equ:average_reward_calculation}
% average\ reward = \frac{r}{N}
% \end{equation}

% c) When the mutation to seed \textit{s} is complete, we calculate the final reward for each position based on the \textit{rewards} and $hit\_nums$ arrays. For the position \textit{p} in the shared pool, the final reward $r_{s,p}$ is defined as: 
% \begin{equation} \label{equ:final_reward_calculation}
% r_{s,p} = \frac{rewards[p]}{hit\_nums[p]}
% \end{equation}

% d) Finally, we update the parameters $A_{p}$ and $b_{p}$ of position \textit{p} according to the feature vector $x_{s}$ of the seed and its final reward at each position:
% \begin{equation} \label{equ:A_update}
% A_{p}^{n+1} = A_{p}^{n} + x_{s} x_{s}^{T}
% \end{equation}

% \begin{equation} \label{equ:b_update}
% b_{p}^{n+1} = b_{p}^{n} + r_{s,p} x_{s}
% \end{equation}

\begin{algorithm}[!t]
\footnotesize
\caption{The implementation of LinUCB model}\label{alg:LinUCB}
\KwIn{$\alpha$ $\in$ $ \mathbb{R}_{+} $ }
\For{$ t = 1,2,3,...,T $}{
    $Observe\ the\ feature\ of\ the\ current\ seed\ s:x_{s} \in \mathbb{R}_{d}$\\
    $Score = []$\\
    \For{$ p \in all\ positions\ in\ shared\ pool $}{
        \If{$p\ is\ new$}{
            $A_{p} = I_{d}$\\
            $b_{p} = 0_{d*1}$\\
        }
        $\hat{\theta}_{p} = A_{p}^{-1}b_{p}$\\
        $Score \gets \hat{\theta}_{p}^{T}x_{s} + \alpha  \sqrt{x_{s}^{T} A_{p}^{-1} x_{s}}$\\
    }
    $Distribution = Generate(Score)$\\
    $Mutate\ based\ on\ Distribution\ and\ calculate\ r_{s,p},\ p \in all\ positions$\\
    \For{$ p \in all\ positions\ in\ shared\ pool $}{
        $A_{p} = A_{p} + x_{s} x_{s}^{T}$\\
        $b_{p} = b_{p} + r_{s,p} x_{s}$\\
    }
}
\end{algorithm}

\subsubsection{Overall Algorithm}
The specific algorithm of LinUCB is shown in the Algorithm~\ref{alg:LinUCB}.
Lines 3-10 calculate the expected reward of each position and its confidence interval to generate the final score.
Line 11 generates a probability distribution based on the score of each position.
Line 12 selects positions to mutate according to the distribution and collects the corresponding data.
Lines 13-15 update each position's parameter matrix according to each position's final reward and the current seed's feature vector.


\subsection{Increase of Valuable Positions}
The family system and CMAB optimize the selection of valuable positions. Theoretically, some specific byte positions can discover a fixed number of edges. Therefore, we need to continuously increase the number of valuable position during fuzzing. To achieve it, \tool{} switches between family-based mutation and random mutation. The family-based mutation is the strategy described in this section, while the random mutation is to randomly select byte positions and mutate them.
To switch mutation modes, \tool{} uses a simple yet effective indicator calculated as:

\begin{equation} \label{equ:cost}
c = \frac{N_{exec}}{N_{new\_paths}},
\end{equation}
where $N_{exec}$ is the number of executions, and $N_{new\_paths}$ is the number of new paths found in those executions. 


The result $c$ is the cost to discover one new path. Lower cost $c$ indicates the higher efficiency of a mutation mode.
Both family-based mutation and random mutation have their own costs $c$. When deciding the mode to perform, \tool{} compares the costs of the two modes, and selects the mode with lower cost.



% \todo{In Progress}


% \zhu{Maybe we can describe this part as the prioritization of input bytes. I think essentially, you prioritize the bytes in the shared pool, and then mutate the rest bytes. no?}\zkp{More precisely, the random mode is used to update the shared pool of each family, while the history mode dynamically selects appropriate positions from the shared pool for mutation according to the LinUCB model.}

% Further, We construct two modes for the havoc stage, \textit{history mode} and \textit{random mode}. 
% In random mode, we randomly select positions to mutate, and collect data to extract valuable positions to update the shared pool within each family. \zhu{Although we use random mutation to update or obtain more valuable positions, we can use existing solutions to achieve it.} And history mode will extract positions from the shared pool for mutation based on LinUCB model. 
% In history mode, we pay attention to the valuable positions of seeds.
% We use the LinUCB model to calculate the fitness of each position stored in the shared pool for the current seed and generate a probability distribution based on the fitness. Finally, we select the mutation position based on the probability distribution.

% Therefore, history mode depends on random mode. We need an efficient mode scheduler that constantly switches between the two modes during fuzzing.

% \textit{Mode scheduler.}
% In order to find the best mode that should be used in the current mutation, we propose a novel mode scheduler. Specifically, we record the number of executions \textit{ExecNum} and new paths found \textit{PathFound} in each mode. As shown in following equation, we calculate the number of executions needed to discover a new path (\textit{per\_path\_cost}) for two modes. The smaller the \textit{per\_path\_cost} is, the higher the corresponding mode's efficiency. 
% Finally, we directly choose the mode that currently performs best on \textit{per\_path\_cost}.
% % \begin{equation} \label{equ:cost}
% % per\_path\_cost = \frac{ExecNum}{PathFound}
% % \end{equation}



\subsection{Threats to Validity}

Our \tool{} is proposed based on the results of SHAP analysis, which is an empirical study. Thus, we concern about the generality of our claims due to the small number of samples. 
However, we analyze the root causes of the SHAP results to support our claims.  
The root causes, direct and indirect coupling of path constraints, are the observations of the nature of programs, which is independent from our empirical study.
Even if our claim cannot include all programs, we believe it satisfies the most of modern programs.


The second concern comes from the internal validity, which is our solution to optimize byte selection. 
Our solution is based on two presumptions. The first is that we have valuable positions for us to optimize. The second is that our family system can capture the structural information of target programs. 
For the first presumption, we use the random mutation mode to obtain the valuable positions.
However, random mutations have the limitation to increase the number of valuable positions.
To solve this problem, we can use the existing solutions that can find the constraint-related byte positions, such as GreyOne\zhu{cite}, Angora\zhu{cite} and Driller\zhu{cite}. These solutions are efficiently in finding positions related to a single path constraint, which is exactly what we want.
For the second presumption, it is mainly used to share valuable positions among different seeds. That is, valuable positions in different seeds are still related to path constraints.
However, the family system can only roughly satisfy this requirement. 
One solution to solve this is to analyze programs case by case. That is, we capture the structural information based on syntax analysis tools or even manually determine the constraint-related positions in different seeds.
Yet, we believe such solution limits the scalability of fuzzing, \ie it is only effective in specific programs.
Although the family system cannot accurately capture the structural information, the CMAB refines the selection of valuable positions, which is scalable to fuzz programs.



% \zhu{external and internal threats.}

% \zhu{limitations of \tool{}: 1) needs initial valuable positions ==> our experiment results show the efficacy of our solution; with popularity of fuzzing, we have many initial seeds; we can use existing solutions to get constraint-related bytes. 2) The family system can be improved.}

% \zkp{
% In the design of \tool{}, the valuable position sharing is achieved between seeds in a family, which is mainly because of the challenge of establishing a position mapping between seeds that have different structures.
% In addition, if we can build position mapping between different structure seeds via the analysis of some syntax analysis tools, valuable position sharing can be achieved among different families.
% For instance, we can find the positions of headers with the same meaning on different seeds and thus build a position mapping between them.


% 2) 
% In the design of \tool{}, 
% we extract the valuable positions based on the local new edge indicator, which significantly improves the efficiency of exploring edge coverage and finding bugs.
% On the other hand, we can also extract other position information from a more fine-grained indicator.
% For example, we can find which position is related to path constraints by indicator of path change.
% Thus, we can construct a multi-granularity level indicator system to extract more useful position information from the mutation process at different granularities.

% }



==> obsolete/technique-2.0.tex <==


\vspace{-5mm}
\section{Design of \tool{}}


Our \tool{} focuses on the byte mutation and seeks out valuable byte positions. 
Based on our SHAP analysis, when positions have already discovered new code, we predict that those positions can discover more code in later fuzzing campaigns. 
Therefore, we regard such positions as valuable positions and optimize the use of them based on our family system and CMAB.
Figure~\ref{Framework} shows the framework of our \tool{}, which optimizes the valuable positions to boost fuzzing. \tool{} establishes a family system to share valuable positions within family members, \ie seeds in a family. The shared positions improve the performance of code discovery because of the coupled path constraints as shown in Section~\ref{sec:motivation}. To schedule shared positions efficiently and effectively, \tool{} utilizes a contextual multi-armed bandit approach to build a probability distribution for mutating byte positions.
The positions that are more likely to discover new code will be assigned a high selection probability.
% Finally, \tool{} switches mutation mode between family-based mutation mode and random mutation mode. 
Finally, if existing valuable positions can no longer discover new code efficiently, \tool{} will randomly mutate bytes to obtain new valuable positions. 
% Note that, the random mutation can be replaced by the existing fuzzing solutions that resolve path constraints.
Notably, the CMAB model may select positions that are related to multiple path constraints, which can help fuzz directly coupled constraints.

% \chao{This design has utilized the observations (1) some bytes are more important and worthy mutating; and (2) this knowledge can be shared among a family of seeds. But where is the last observation used, i.e., (3) some bytes should be mutated together?}
% \zhu{revised.}
% \zkp{In the process of position selecting, we have implemented the combination of positions.
% Specifically, which positions can be combined is mainly determined by the probability distribution generated by the LinUCB model.
% Finally, we update the internal parameters of LinUCB based on the feedback of the mutation results.}


\subsection{Family System}

To efficiently utilize valuable byte positions, \tool{} establishes a \textit{family system} to share positions. 
% \tool{} shares valuable positions to fuzz indirectly coupled path constraints, while it combines them to fuzz directly coupled path constraints.
The family system tries to ensure that the shared positions under different seeds are still related to path constraints. 
Therefore, a family is built such that any seed $S_a$ (except the first one) in the family is added when $S_a$ is obtained by mutating another seed $S_o$ in the same family, without changing the length of $S_o$.
% Then, seeds in a family can roughly maintain the semantic meaning of byte positions.
Within a family, \tool{} puts all valuable positions in a \textit{shared pool}. Since the length of a seed may be changed (\eg during the trimming stage), \tool{} tracks the byte positions among seeds in a family.


\subsubsection{Shared Pool}
% \textbf{Shared Pool.}
Each family has its own shared pool.
When mutating a seed, \tool{} prefers byte positions from the shared pool. However, the number of valuable positions significantly decreases in later families because fuzzing can discover less and less new code over time. Since the valuable positions are essentially the ones related to path constraints, we extend their definition based on families. 
If mutation of some positions can discover code that all seeds in a family have never discovered, those positions are valuable positions in the family. 
Thus, the shared pool can capture most of the path constraints related to a family. As shown in Figure~\ref{Framework}, seeds in a family can reuse and combine shared positions to improve efficiency of code discovery.


\subsubsection{Position Tracking}
Even though a family is built without mutations that change seed length, the length of a seed may still be changed, for example, by the trimming stage. To uniformly select byte positions when they are changed, all positions in a shared pool are recorded based on the first seed. \tool{} tracks the changes of positions among seeds so that positions are selected uniformly.
For instance, in Figure~\ref{trimming}, three seeds are in a family, where the seeds $S_1$ and $S_2$ are trimmed, and the seed $S_o$ is the first seed in the family.
On the one hand, if the forth position of seed $S_1$ discovers new code, \tool{} will add the number 6 into the shared pool because it maps to the sixth position of seed $S_o$. On the other hand, when selecting the position 6 from the shared pool for the seed $S_2$, \tool{} will mutate the second byte of $S_2$ based on the position tracking.
As a result, \tool{} can correctly record and select valuable positions from a shared pool.

\begin{figure}[!t]
\includegraphics[width=0.95\linewidth]{images/trimming.jpg}
\caption{Position tracking. \tool{} tracks the changes of byte positions.}
\label{trimming}
\end{figure}


\subsubsection{Family Update}
The key of building a family is that the mutation does not change the length of original seeds. However, many fuzzers mutate seeds via changing the length of seeds, such as inserting bytes and deleting bytes. To enrich family members, \tool{} will withdraw all mutators that change length when new code are discovered.
If the result can still find the same new edges after withdrawing those mutators, \tool{} will retain the result to a family.
For example, as shown in Figure~\ref{fig:family_update}, if an input $i_1$ discovers new edges, \tool{} will withdraw all mutators that change length, which generates another input $i_2$. If $i_2$ can still find the same new edges that $i_1$ finds, \tool{} retains $i_2$ to a family.
Otherwise, $i_1$ will form a new family if mutation of $i_1$ can further discover new edges.
As a result, \tool{} has a reasonable number of families and family members.




\subsection{Contextual Bandit for Byte Schedule}


The family system can only roughly ensure that positions in a shared pool are related to path constraints under any context. Over time, a newly added seed may be completely different to the first seed in the same family in terms of input format. 
% That is, these two seeds may exercise different program logic.
In addition, the family system cannot infer valuable positions from the constraint-related positions.
% \chao{It's unclear why the following probability distribution calculation could solve this issue.} \zhu{revised.}
% \zkp{We need to judge whether each position in the shared pool is valuable for the current seed.
% However, directly analyzing their relationship is challenging.
% In the multi-armed bandit problem, we need to find the arm that is more likely to get the highest reward among multiple arms.
% The common solution is to determine the highest expectation of each arm in finite trials.
% Because our goal is similar to the multi-armed bandit problem, we decide to continuously mutate the positions in the shared pool and extract feedback information to judge whether each position in the shared pool is valuable.
% Considering the same position may have different meanings between different seeds, we proposes a variant of the contextual multi-armed bandit (CMAB) model to achieve a personalized byte selection strategy for seeds.% }
To optimize the selection of valuable positions so that they can maximize code discovery, \tool{} models the problem of selecting positions as a contextual multi-armed bandit (CMAB) problem. Based on the experience of playing some arms, the CMAB tries to maximize the rewards of playing multi-armed bandits, taking into account the personality of a player (\ie the context).
The CMAB problem is the trade-off between playing more arms and focusing on some specific arms, \ie the problem of \textit{exploration vs. exploitation}.
From the perspective of program logic, the CMAB in \tool{} shares valuable positions to fuzz indirectly coupled path constraints, while it combines them to fuzz directly coupled path constraints.
Specifically, the reward of CMAB is mainly the code discovery of mutating some positions, which helps determine the constraint-related positions under the current context.
Meanwhile, the maximization of the reward reflects the search of the most contributing byte positions.
Each byte position in a shared pool is an arm, and the seed that selects positions is the player. 
% \chao{<-- grammar error. It is not clear what is a player.}\zhu{done.} 
The context for the CMAB problem is the feature vector extracted from the execution path that the current seed exercises. 
% \chao{<-- context 2}\zhu{revised}
% Therefore, the CMAB for \tool{} intends to optimize the selection of shared positions so that they are related to constraints that the current seed examines.
Therefore, the CMAB for byte mutation is to balance between exploring more positions and exploiting the best positions. 
% \tool{} utilizes LinUCB~\cite{linucb}, one of the solutions for the CMAB problem, to build a probability distribution for selecting positions.
Based on CMAB, \tool{} builds a probability distribution for selecting positions, and it prefers the positions that are more likely to discover new code.


\begin{figure}[t!]
\includegraphics[width=\linewidth]{images/upate.png}
\caption{The update of family and family members.}
\label{fig:family_update}
\end{figure}


\subsubsection{Scores of Positions}
% \zkp{}
%maintain a dataset

To introduce context into position selection, we need to build a relationship between context and reward, which relies on the history data. Thus, each arm needs to maintain a dataset $(\mathcal{D}, \mathcal{R})$, where $\mathcal{D}$ is a set of all history feature vectors and $\mathcal{R}$ is a set of corresponding rewards.
To achieve balance between exploitation and exploration, the scores calculated by \tool{} includes the expected reward and the upper confidence bound.

\textit{Expected Reward.} To avoid affecting throughput, we assume a linear relationship between the reward and the feature vector to save computational time. 
Given a seed $s$, the feature vector $x_{s}$ extracted from the corresponding execution path (\ie the context), and a position $p$ recorded in a shared pool, the expected reward $E[r_{s,p}|x_{s}]$ can be calculated by:

\begin{equation} \label{equ:E_calculation}
E[r_{s,p}|x_{s}] = x_{s}^{T}\hat{\theta}, %A_{p}^{-1}b_{p}
\end{equation}
where $\hat{\theta}$ is the best coefficient vector. 
Applying ridge regression to the dataset $(\mathcal{D}, \mathcal{R})$,
$\hat{\theta}$ can be estimated by:
\begin{equation} 
\hat{\theta} = (D_{p}^{T}D_{p} + I_{k})^{-1} D_{p}^{T} R_{p},
\end{equation}
where $(D_{p}, R_{p})$ is the dataset maintained by position $p$, $I_{k}$ is a k-dimensional identity matrix, and $k$ is the dimension of the feature vector.

\textit{Upper Confidence Bound.}
The second part of a score is the upper confidence bound $U_{s,p}$, which is calculated based on~\cite{walsh2009exploring}:
\begin{equation} \label{equ:U_calculation}
U_{s,p} = \sqrt{x_{s}^{T} (D_{p}^{T}D_{p} + I_{d})^{-1} x_{s}}
\end{equation}

Then, the score of each position $Score(s,p)$ is defined as:
\begin{equation} \label{equ:Fitness_calculation}
Score(s,p) = E[r_{s,p}|x_{s}] + \alpha U_{s,p},
\end{equation}
where $\alpha$ is a hyper-parameter for users to set.
Based on our experience, we set $\alpha = 0.5$ in our experiments.
For Equation~(\ref{equ:Fitness_calculation}), the more a position is selected, the smaller its $U_{s,p}$ is. Therefore, \tool{} achieves the trade-off between exploration and exploitation.




% The probability distribution is built based on the scores of positions, where positions with larger scores have higher chance to be selected.
% The scores calculated by \tool{} includes the expected reward and the upper confidence bound.
% Given a seed $s$, the feature vector $x_{s}$ extracted from the corresponding execution path (\ie the context), \chao{<-- context 3, confusing}\zhu{revised} and a position $p$ recorded in a shared pool, the expected reward $E[r_{s,p}|x_{s}]$ can be calculated by:
% \begin{equation} \label{equ:E_calculation}
% E[r_{s,p}|x_{s}] = x_{s}^{T}A_{p}^{-1}b_{p},
% \end{equation}
% where $r_{s,p}$ is the reward of the seed $s$ at position $p$, and $A_{p}$ and $b_{p}$ are the parameters maintained by the position $p$. \chao{What are their meanings then?} \zkp{
% $A_{p}$ and $b_{p}$ accumulate the feature vector encountered and the reward obtained.
% } Both $A_{p}$ and $b_{p}$ will be updated during fuzzing. 



% The second part of a score is the upper confidence bound $U_{s,p}$, which is calculated as:
% \begin{equation} \label{equ:U_calculation}
% U_{s,p} = \sqrt{x_{s}^{T} A_{p}^{-1} x_{s}}
% \end{equation}



% Then, the score of each position $Score(s,p)$ is defined as:
% \begin{equation} \label{equ:Fitness_calculation}
% Score(s,p) = E[r_{s,p}|x_{s}] + \alpha U_{s,p},
% \end{equation}
% where $\alpha$ is a hyper-parameter for users to set.
% Based on our experience, we set $\alpha = 0.5$ in our experiments.
% For Equation~(\ref{equ:Fitness_calculation}), the more a position is selected, the smaller its $U_{s,p}$ is. Therefore, \tool{} achieves the trade-off between exploration and exploitation.


\subsubsection{Feature Vector (The Context)} 
Different from other fuzzers, our \tool{} considers the context when optimizing byte selection. The calculation of both $E[r_{s,p}|x_{s}]$ and $U_{s,p}$ in Equation~(\ref{equ:Fitness_calculation}) contains the context $x_s$. Recall that the selected shared positions need to be related to path constraints for the current seed. Since edges contain path constraints, \tool{} uses the execution paths that the current seed exercises as the context. 

Usually, the number of edges is large in an execution path, which leads to oversized feature vectors. 
To solve this problem, \tool{} compresses a set of edges into a fixed dimensional vector by using K-means clustering~\cite{kmeans}. 
As shown in Figure~\ref{FeatureGeneration}, 
\tool{} first collects all the exercised execution paths into bitmaps, in which the examined edges are marked with 1, and 0 otherwise. Then, the K-means method is utilized to cluster seeds into $k$ classes based on their corresponding execution paths. Based on our experiments, we set $k = 20$, as this performs the best. 
% \chao{Why are execution traces clustered into 20 classes? It lacks justification or interpretable meanings.} \zhu{revised.}
% \zkp{20 is the best value obtained by a simple comparison experiment. But now I have not conducted formal experiments here.}


The feature vector of a seed is now a $k$-dimensional vector, of which each dimension is calculated based on the Jaccard similarity between the current execution path and the central path of a class. 
% \chao{The following similarity score is just one value, how do you set all 20 dimensions of the feature vector?} \zhu{explained by the new variable $V$.}
% \zkp{The following similarity score is the similarity between the path executed by the current seed and a central path of a class.
% We compute the similarity between the current seed and the central paths of all 20 classes separately to get the feature vector.
% }
For Jaccard similarity~\cite{jaccard1912distribution}, given two seeds $s_a$ and $s_b$, and their corresponding paths $\mathcal{P}_{s_a}$ and $\mathcal{P}_{s_b}$, the similarity $\mathcal{L}(s_a, s_b)$ between seeds $s_a$ and $s_b$ is calculated as:
% \chao{Here, the score is calculated based on paths. But the feature vector (context) is said to be the set of edges in the first paragraph of this section.}\zhu{revised to feature vector of path}

\begin{equation}
    \mathcal{L}(s_a, s_b) = \frac{|\mathcal{P}_{s_a}\cap \mathcal{P}_{s_b}|}{|\mathcal{P}_{s_a}\cup \mathcal{P}_{s_b}|}
\end{equation}
where edges in $\mathcal{P}_{s_a} \cap \mathcal{P}_{s_b}$ belong to both paths, and edges in $\mathcal{P}_{s_a} \cup \mathcal{P}_{s_b}$ contain all edges in both paths. $|\bullet|$ is the number of edges. Thus, given the current seed $s$ and the $k$ central seeds $s_1, s_2, ..., s_{k}$, the feature vector for $s$ is $V(s) = [\mathcal{L}(s, s_1), \mathcal{L}(s, s_2), ..., \mathcal{L}(s, s_{k})]$.

\begin{figure}[!t]
\includegraphics[width=\linewidth]{images/FeatureGeneration.jpg}
\caption{K-means Based Feature Generation.}
\label{FeatureGeneration}
\end{figure}


\subsubsection{Dataset Update}

% \chao{Please explain your design choice before introducing the details of how it is implemented. This is a common question existed in the whole paper.} \zhu{revised.}
% \zkp{The calculation of the score relies on $A_{p}$ and $b_{p}$, while $A_{p}$ and $b_{p}$ accumulate the feature vector encountered and the reward obtained.
% Since the importance of each position is changing during the fuzzing process, we need to keep updating A and b to ensure that the calculated scores are accurate.
% }
% The other part of Equation~(\ref{equ:Fitness_calculation}) is to update the parameters $A_p$ and $b_p$ for the position $p$, which are calculated by:

% \begin{equation} \label{equ:A_update}
% A_{p}^{n+1} = A_{p}^{n} + x_{s} x_{s}^{T},
% \end{equation}
% \begin{equation} \label{equ:b_update}
% b_{p}^{n+1} = b_{p}^{n} + r_{s,p} x_{s},
% \end{equation}
% where $n$ is the step that $A_{p}$ and $b_{p}$ are updated, and $r_{s,p}$ is the reward that mutation of the position $p$ in the seed $s$ obtains. 
% \chao{What are the meanings of these symbols? Why do you setup formulas like this?} \zkp{Following \cite{linucb}.}

% \zkp{After the mutation of seed $s$ is completed, we also collect data to update the dataset of all selected positions.}
To update the score of each position, we update data for the dataset $(D_p, R_p)$ after the mutation of a seed $s$ is completed.
Different from the traditional CMAB where a reward is obtained by playing one arm, fuzzing has a high chance to play multiple arms at a time, \ie mutating multiple shared positions simultaneously. In this case, the reward is not for a single position, but for multiple positions. Therefore, \tool{} assigns the average reward to each selected position. Given a position $p$, the reward is calculated as:

\begin{equation} \label{equ:final_reward}
    r_{s,p} = \frac{\sum_{i}^{N_{hits}}(\frac{r_i}{M_i})}{N_{hits}},
\end{equation}
where $r_i$ is the reward for the $i$-th time that the position $p$ is selected, and $M_i$ is the number of all positions being selected at the i-th time. The term $\frac{r_i}{M_i}$ is then the average reward assigned to the position $p$ at the i-th time. To speed up the updating process, \tool{} calculates the final reward for a position after the mutation for a seed has completed. Thus, $N_{hits}$ in Equation~(\ref{equ:final_reward}) is the total number of times the position $p$ has been selected.
Thus, $r_{s,p}$ is the average reward of all mutations that select the position $p$ in the seed $s$.
Finally, the tuple $(x_{s}, r_{s,p})$ of position $p$ is added into the dataset $(D_p, R_p)$.
% \zkp{and the tuple $(x_{s}, r_{s,p})$ will be added to the dataset of position $p$.}

% \zhu{fuzzing plays multiple arms (mutating multiple positions) at a time, and the reward is for all the mutated positions, which cannot be separated. So we divide the reward by N selected positions, and assign the result to each position.}


\subsubsection{Individual Reward}
The Equation~(\ref{equ:final_reward}) needs the individual reward $r_i$ for a single selection of multiple positions. 
Since \tool{} tries to schedule constraint-related positions, a straightforward reward is the change state after mutating a position. However, such kind of reward only has two values 0 and 1. To further differentiate positions, we introduce the \textit{frequency} of a seed being mutated to the calculation of rewards. Equation~(\ref{equ:Reward}) is the reward used by \tool{}: 

\begin{equation} \label{equ:Reward}
r_i = IsChanged \times f,
\end{equation}
where \textit{IsChanged} is 1 when the path changes or otherwise 0, and $f$ is the frequency that the seed is mutated. The frequency is calculated as $f = \frac{N_{mut}}{N_{total}}$, and $N_{mut}$ is the number of mutations that perform on the seed and $N_{total}$ is the total number of executions during fuzzing.


\begin{algorithm}[!t]
\footnotesize
\caption{The implementation of Reinforcement Learning }\label{alg:reinforce}
\KwIn{$\alpha$ $\in$ $ \mathbb{R}_{+} $ }
\For{$ t = 1,2,3,...,T $}{
    $Observe\ the\ feature\ of\ the\ current\ seed\ s:x_{s} \in \mathbb{R}_{d}$\\
    $Score = []$\\
    \For{$ p \in all\ positions\ in\ shared\ pool $}{
        $Observe\ the\ dataset\ (D_{p}, R_{p})\ maintained\ by\ position\ p$\\
        $\hat{\theta}_{p} = (D_{p}^{T}D_{p} + I_{d})^{-1} D_{p}^{T} R_{p}$\\
        $Score \gets \hat{\theta}_{p}^{T}x_{s} + \alpha  \sqrt{x_{s}^{T} (D_{p}^{T}D_{p} + I_{d})^{-1} x_{s}}$\\
    }
    $Distribution = Generate(Score)$\\
    $Mutate\ based\ on\ Distribution\ and\ calculate\ r_{s,p},\ p \in all\ positions$\\
    \For{$ p \in all\ positions\ in\ shared\ pool $}{
        $(D_{p}, R_{p}) \gets (x_{s}, r_{s,p})$
    }
}
\end{algorithm}

\subsubsection{Overall Algorithm}
The specific algorithm of CMAB is shown in the Algorithm~\ref{alg:reinforce}.
Lines 2-7 calculate the expected reward of each position and its confidence interval to generate the final score.
Line 8 generates a probability distribution based on the score of each position.
Line 9 selects positions to mutate according to the distribution and collects the corresponding data.
Lines 10-11 update each position's dataset according to each position's final reward and the current seed's feature vector.


\subsection{Increase of Valuable Positions}
The family system and CMAB optimize the selection of valuable positions. 
% Theoretically, some specific byte positions can discover a fixed number of edges. \chao{Where are the theory? Just simply argue that some bytes will get aging after a while of testing.} 
However, valuable positions will become stale after a period of testing, which indicates they will discover less edges over time.
Therefore, we need to continuously increase the number of valuable positions during fuzzing. To achieve this, \tool{} switches between family-based mutation and random mutation. Family-based mutation is the strategy described in this section, while random mutation will simply select byte positions randomly and mutate them.
To switch mutation modes, \tool{} uses a simple yet effective indicator calculated as:

\begin{equation} \label{equ:cost}
c = \frac{N_{exec}}{N_{new\_paths}},
\end{equation}
where $N_{exec}$ is the number of executions, and $N_{new\_paths}$ is the number of new paths found in those executions. 


The result $c$ is the cost to discover one new path. Lower cost $c$ indicates higher efficiency of a mutation mode.
Both family-based mutation and random mutation have their own costs $c$. When deciding the mode to perform, \tool{} compares the costs of the two modes, and selects the mode with lower cost.



\subsection{Threats to Validity}

Our \tool{} is proposed based on the results of SHAP analysis, which is an empirical method. Thus, we were concerned about the generality of our claims due to the small number of samples. 
However, we analyzed the root causes of the SHAP results to support our claims.  
These root causes, direct and indirect coupling of path constraints, are general observations of the nature of programs and independent from our empirical study.
Even if our claim does not include all programs, we believe it satisfies the majority of modern programs.


The second concern comes from the internal threat to validity, which is our solution to optimize byte selection. 
Our solution is based on two assumptions. The first is that there are valuable positions for us to optimize. The second is that our family system can capture the structural information of target programs. 
For the first assumption, we use the random mutation mode to obtain valuable positions.
However, random mutations can only increase the number of valuable positions up to a limit.
To solve this problem, we can use existing solutions that find constraint-related byte positions, such as GreyOne~\cite{greyone}, Angora~\cite{angora} and Driller~\cite{driller}. These solutions are efficient in finding positions related to a single path constraint, which is exactly what we want.
For the second assumption, it is mainly used to share valuable positions among different seeds. This requires that valuable positions in different seeds are still related to path constraints.
However, the family system can only roughly satisfy this requirement. 
One solution to solve this is to analyze programs case by case. That is, we capture the structural information based on syntax analysis tools or even manually determine the constraint-related positions in different seeds.
Yet, we believe such a solution limits the scalability of fuzzing, \ie it is only effective in specific programs.
Although the family system cannot accurately capture structural information, CMAB refines the selection of valuable positions, which is scalable to fuzz programs.





==> obsolete/technique-2.1.tex <==


% \vspace{-5mm}
\section{Design of \tool{}}

\zkp{

Our \tool{} focuses on the byte mutation and seeks out valuable byte positions. 
Figure~\ref{Framework} shows the framework of our \tool{}, which optimizes the valuable positions to boost fuzzing.

First, we propose the Family System to reorganize the seeds. More specifically, we cluster seeds into families based on the inheritance relationship and seed length. Each family maintains a shared pool for recording the found valuable positions of all seeds in the family.

Then, we randomly select a seed to mutate and obtain its valuable positions from the shared pool of the family where the seed is located. To solve the utilization and update problems of valuable positions, we design two modes in the mutation stage: family-based mutation and havoc mutation.
Family-based mutation focuses on mutating valuable positions.
The havoc mutation randomly mutates all positions to expand valuable positions.

Finally, we identify the valuable positions of the seed based on the shapely value, and integrate the calculation process into fuzzing to achieve a lightweight inference process.
We record the mutated positions sequence of each mutation.
If mutated input discovers new code, we use the shapely value to calculate the contribution of each position to obtain valuable positions and record them in the shared pool of the family.

\subsection{Valuable Positions Inference based on Shapely Value}
From the analysis of motivation, we know that most of the new edges are contributed by a small number of seed positions.
Formally, we define positions that contribute to edge discovery as valuable positions.
Moreover, repeated mutations of valuable positions can still find more new edges.

To identify valuable positions, we need to quantify the \textit{edge contribution} of each position, \ie the contribution to edge discovery.
Given a mutation $M$ in the fuzzing process and the mutation position sequence $M\_pos = \{pos_{1}, \ldots, pos_{n}\}$. We regard the execution process of the target program as a black-box model, whose input is the mutation position sequence $M\_pos$, and outputs the number of new edges $E$ found by the mutated input. However, not all contributions in the mutation position sequence $M\_pos$ are the same. There are often many redundant mutated positions. Therefore, we can use the shapely value to calculate the marginal contribution of each mutated position.
If we accumulate the marginal contribution of position $pos_{i}$ on all mutations, we can get the edge contribution of $pos_{i}$.

Due to the time-consuming calculation process of shapely value, we cannot directly apply it to infer valuable positions in the fuzzing process. To quantify the edge contribution of each position more lightweight, we optimize from the following two aspects.

\textbf{Reduce the number of mutations to analyze. }
In the fuzzing process, most of the mutations cannot discover new edges, and they are not helpful for the inference of valuable positions.
If we analyze millions of mutations in the fuzzing process, the time required is unacceptable.
Therefore, we only performed analysis on those mutations that discovered new edges.

\textbf{Simplify the calculation process of shapely value. }
According to the Equation~\ref{equ:shapely}, the shapely value is the weighted average of the marginal contribution of the target feature in all feature combination subsets under a given sample.
% If we use it during fuzzing, it will seriously reduce efficiency.
% Assuming that the mutation position sequence has 32 positions, to calculate the contribution of each position, we need to additionally analyze the number of new edges found in $2^{32}$ mutation position sequence subsets.
% Therefore, we propose a more lightweight calculation method.

% Suppose there are $N$ mutated positions in a mutation, and some new edges are found.
% First, we eliminate those redundant mutated positions through the marginal contribution of each position on the largest mutated positions sequence subset to obtain the necessary mutated positions. In other words, these positions must be mutated simultaneously to discover these new edges, and one less mutation will not work.
% Then, since redundant mutation positions do not affect the results, we only need to analyze the marginal contribution of each position on a subset of necessary mutation positions.
% However, when analyzing a subset of necessary mutation positions, some necessary mutated positions must not be mutated, which will cause us to be unable to discover new edges. Therefore, the obtained Shapely Value is 0, which does not affect the final result.
% Therefore, we only calculate the marginal contribution of each position on the largest subset.

Assuming that several mutations are performed on a seed $s$, $F$ is all mutation samples that find new edges.
Given a position $i$, its edge contribution is $\beta$, and the calculation formula is:
\begin{equation} \label{equ:edgeContribution}
\beta = \sum_{M \subseteq F} val(M) - val(M/pos_{i})
\end{equation}
Among them, $val(M)$ is the number of new edges found by mutation $M$.
$M/pos_{i}$ is to cancel the mutation of $pos_{i}$ in mutation $M$.
For each mutation, we only consider the marginal contribution of each position on the largest mutation position sequence set, which can reduce the time complexity to the O(n) level. If $\beta > 0$, position i is considered to be a valuable position.

Note that we only deal with mutated input without length mutators because length mutators can cause most positions to change.
Moreover, the length mutation operator can easily change the seed structure, making the analysis more difficult.
Figure~\ref{Inference} presents the overall process of valuable position inference.
Given a seed $S$, and its mutated inputs $A$, $B$ and $C$. Among them, $A$ and $C$ found 3 new edges, and $B$ found no new ones. Then, we calculate the marginal contribution of each position in mutations $A$, $B$ and $C$ based on the formula \ref{equ:edgeContribution}. In $A$, the marginal contributions of $pos 1$ and $pos 2$ are 2 and 1, respectively. Since $pos 3$ and $pos 4$ have not been mutated, their marginal contribution is 0. Similarly, the marginal contributions of $pos 1$ and $pos 3$ in $C$ are 1 and 2, respectively. Since $B$ does not discover the new edge, we skip it. Finally, we accumulate the marginal contribution of each position under all mutations, and get the edge contributions of $pos 1, pos 2, pos 3$ and $pos 4$ to be 3, 1, 2 and 0, respectively. Therefore, $pos 1, pos 2, pos 3$ are valuable positions.

\begin{figure}[!t]
\includegraphics[width=0.95\linewidth]{images/Inference.png}
\caption{The overall process of valuable position inference.}
\label{Inference}
\end{figure}

\subsection{Family System}
To speed up the inference of valuable positions, we propose a family system that can divide seeds into multiple families in a lightweight method.
In each family, we will maintain a shared pool for sharing the valuable positions found by all seeds in the family.

\subsubsection{Why Family System Matters}
Shapely Value is a posterior algorithm, which can only show that the valuable positions on a seed were efficient in the past.
However, efficiency in the past does not mean efficiency in the future.
We need to identify the valuable positions of the seed before mutation to discover more new edges.
It can be seen from motivation that there is a constraint relationship between constraints, which indicates that the same valuable positions may exist between different seeds.
Moreover, we have experimentally verified the universality of sharing valuable positions among seeds in X.
Therefore, we can identify valuable positions from mutated seeds and share them with unmutated seeds, thereby improving fuzzing efficiency.

However, what kind of seeds can share valuable positions?
To solve this problem, we cluster seeds into families based on semantic consistency (i.e., the same position has the same semantics on different seeds).
In the same family, different seeds have the same valuable positions. Therefore, they can share the inference process of valuable positions, thus saving inference time. In other words, if a seed in a family finds some valuable positions during the mutation process, other seeds in the family can directly regard these positions as valuable positions, avoiding repeated inference processes.

% The above inference of valuable positions is for a single seed, which depends on a single seed being allocated enough energy for the mutation to obtain sufficient information.
% However, many studies have pointed out that the potential of different seeds is also different. If high energy is allocated to those low-potential seeds, it will affect the fuzzing efficiency.
% To alleviate this problem, we can cluster seeds into families based on semantic consistency (i.e., the same position has the same semantics on different seeds).
% In the same family, different seeds have the same valuable positions. Therefore, they can share the inference process of valuable positions, thus saving inference time. In other words, if a seed in a family finds some valuable positions during the mutation process, other seeds in the family can directly regard these positions as valuable positions, avoiding repeated inference processes.

However, there are significant differences in structure and length between seeds.
The same position can also have completely different meanings on different seeds.
Even with corresponding grammatical analysis tools, the judgment of semantic consistency is very time-consuming and complicated.
Therefore, we expand the determination range of the family to avoid missing those seeds that meet the semantic consistency.
Therefore, we propose two key conditions for semantic consistency between seeds: inheritance relationship and length consistency.
If the above conditions are met between seeds, then they may be able to maintain semantic consistency. Otherwise, we cannot decide due to the complexity of the seed structure.

\textbf{Inheritance relationship. }
Structural consistency among seeds is the advance of semantic consistency.
It is very difficult to directly determine whether the structure consistency between seeds is maintained, which needs to rely on complex grammar parsing tools.
However, we can establish structural connections between seeds through inheritance relationships.
Suppose seed $A$ is mutated from seed $B$, and $x$ positions are mutated.
If $x$ is 0, then $A$ and $B$ must maintain structural consistency.
And, the larger $x$ is, the smaller the probability that $A$ and $B$ maintain structural consistency. This is because the more mutation positions, the greater the probability of causing changes in the seed structure.
So, if there is an inheritance relationship between seeds, it is possible for them to maintain structural consistency. Otherwise, it is difficult to judge lightly.

\textbf{Length consistency. }
If the lengths between seeds are inconsistent, then semantic consistency must not be satisfied.
To share valuable positions between seeds with inconsistent lengths, we need to build position mapping between seeds to link positions with the same semantics.
However, the construction of position mapping becomes difficult due to the existence of length mutators such as insertion/deletion in the fuzzing process.
Therefore, we only consider the semantic consistency between those seeds with the same length.

\subsubsection{Family Construct}
To share valuable positions, we group those seeds with inheritance relationships and consistent length into a family.
The key of building a family is that the mutation does not change the length of original seeds. However, many fuzzers mutate seeds via changing the length of seeds, such as inserting bytes and deleting bytes. To enrich family members, \tool{} will withdraw all mutators that change length when new code are discovered.
If the result can still find the same new edges after withdrawing those mutators, \tool{} will retain the result to a family based on inheritance relationship and seed length.
if we select a seed from family $N$ and generate an 
For example, as shown in Figure~\ref{fig:family_update}, we select a seed from family $N$ and mutate it. 
If an input $i_1$ discovers new edges, \tool{} will withdraw all mutators that change length, which generates another input $i_2$. If $i_2$ can still find the same new edges that $i_1$ finds, \tool{} retains $i_2$ to the family $N$.
Otherwise, $i_1$ will form a new family $N+1$ if mutation of $i_1$ can further discover new edges.
As a result, \tool{} has a reasonable number of families and family members. 

\begin{figure}[t!]
\includegraphics[width=\linewidth]{images/upate.png}
\caption{The update of family and family members.}
\label{fig:family_update}
\end{figure}

\subsubsection{Shared Pool}
To share valuable positions within the family, each family has its own shared pool to record all valuable positions found by all seeds in the family.
A seed can either add the found valuable positions to the shared pool, or obtain the unknown valuable positions from the shared pool.
The update process of the shared pool is shown in Algorithm~\ref{alg:sharedPool}.

\begin{algorithm}[h]
\footnotesize
\caption{The update process of the shared pool.}\label{alg:sharedPool}
% \KwIn{$\alpha$ $\in$ $ \mathbb{R}_{+} $ }
\While{$True$}{
    $s \gets selectSeed(M)$\;
    $f \gets getFamily(s)$\;
    $energy \gets calEnergy(s)$\;
    \While{$energy > 0$}{
        $s_{new} \gets mutate(s)$\;
        $E \gets findsNewEdges(s_{new})$\;
        \If{$E \neq \emptyset$}{
            $pos_{v} \gets shapelyAnalysis(s, s_{new})$\;
            $s_{w} \gets withdraw(s_{new})$\;
            $res \gets stillFindNewEdges(s_{w})$\;
            \eIf{$res == 1$}{
                $addToFamily(f.members, s_{w})$\;
                $addToSharedPool(f.sharedPool, pos_{v})$\;
                $addToQueue(s_{w})$\;
            }
            {
                $constructNewFamily(s_{new}, pos_{v})$\;
                $addToQueue(s_{new})$\;
            }
        }
        $energy \gets energy - 1$\;
    }
}
\end{algorithm}

\tool{} first mutates the selected seed $s$ and gets the family $f$ (lines 2-6) where the seed is located. If the mutated input $s_{new}$ finds a new edge, we infer the valuable positions $pos_{v}$ on the seed $s$ based on formula X (lines 7-9). To avoid the use of the length mutation operator affecting the update of the family, we try to withdraw all the length mutation operators to get $S_{w}$(line 10).
If $S_{w}$ can still find the same new edge, we add $S_{w}$ to members of the family $f$ and add valuable positions $pos_{v}$ to the shared pool of the family $f$(lines 11-13).
Otherwise, we construct a new family using $s_{new}$ and $pos_{v}$.

\subsection{Family-based Mutation}
After obtaining the valuable positions of each seed, we assign more energy to them for the mutation to discover new edges.
Therefore, we propose a family-based mutation.
More specifically, given a seed, we will obtain valuable positions from the shared pool of the family where the seed is located.
Then, we randomly select positions from their valuable positions for mutation.

However, valuable positions will become stale after a period of testing, which indicates they will discover less edges over time.
Therefore, we need to continuously increase the number of valuable positions during fuzzing. To achieve this, \tool{} switches between family-based mutation and random mutation. Family-based mutation is the strategy described in this section, while random mutation will simply select byte positions randomly and mutate them.
To switch mutation modes, \tool{} uses a simple yet effective indicator calculated as:

\begin{equation} \label{equ:cost}
c = \frac{N_{exec}}{N_{new\_paths}},
\end{equation}
where $N_{exec}$ is the number of executions, and $N_{new\_paths}$ is the number of new paths found in those executions. 


The result $c$ is the cost to discover one new path. Lower cost $c$ indicates higher efficiency of a mutation mode.
Both family-based mutation and random mutation have their own costs $c$. When deciding the mode to perform, \tool{} compares the costs of the two modes, and selects the mode with lower cost.

}



\subsection{Threats to Validity}

Our \tool{} is proposed based on the results of SHAP analysis, which is an empirical method. Thus, we were concerned about the generality of our claims due to the small number of samples. 
However, we analyzed the root causes of the SHAP results to support our claims.  
These root causes, direct and indirect coupling of path constraints, are general observations of the nature of programs and independent from our empirical study.
Even if our claim does not include all programs, we believe it satisfies the majority of modern programs.


The second concern comes from the internal threat to validity, which is our solution to optimize byte selection. 
Our solution is based on two assumptions. The first is that there are valuable positions for us to optimize. The second is that our family system can capture the structural information of target programs. 
For the first assumption, we use the random mutation mode to obtain valuable positions.
However, random mutations can only increase the number of valuable positions up to a limit.
To solve this problem, we can use existing solutions that find constraint-related byte positions, such as GreyOne~\cite{greyone}, Angora~\cite{angora} and Driller~\cite{driller}. These solutions are efficient in finding positions related to a single path constraint, which is exactly what we want.
For the second assumption, it is mainly used to share valuable positions among different seeds. This requires that valuable positions in different seeds are still related to path constraints.
However, the family system can only roughly satisfy this requirement. 
One solution to solve this is to analyze programs case by case. That is, we capture the structural information based on syntax analysis tools or even manually determine the constraint-related positions in different seeds.
Yet, we believe such a solution limits the scalability of fuzzing, \ie it is only effective in specific programs.
Although the family system cannot accurately capture structural information, CMAB refines the selection of valuable positions, which is scalable to fuzz programs.





==> obsolete/technique-3.0.tex <==


% \vspace{-5mm}
\section{Design of \tool{}}

\zkp{

Our \tool{} focuses on the byte mutation and seeks out valuable byte positions. 
Figure~\ref{Framework} shows the framework of our \tool{}, which optimizes the valuable positions to boost fuzzing.

First, we propose the Family System to reorganize the seeds. More specifically, we cluster seeds into families based on the inheritance relationship and seed length. Each family maintains a shared pool for recording the found valuable positions of all seeds in the family.

Then, we randomly select a seed to mutate and obtain its valuable positions from the shared pool of the family where the seed is located. To solve the utilization and update problems of valuable positions, we design two modes in the mutation stage: family-based mutation and havoc mutation.
Family-based mutation focuses on mutating valuable positions.
The havoc mutation randomly mutates all positions to expand valuable positions.

Finally, we identify the valuable positions of the seed based on the shapely value, and integrate the calculation process into fuzzing to achieve a lightweight inference process.
We record the mutated positions sequence of each mutation.
If mutated input discovers new code, we use the shapely value to calculate the contribution of each position to obtain valuable positions and record them in the shared pool of the family.

\subsection{Valuable Positions Inference based on Shapely Value}
From the analysis of motivation, we know that most of the new edges are contributed by a small number of seed positions.
Formally, we define positions that contribute to edge discovery as valuable positions.
Moreover, repeated mutations of valuable positions can still find more new edges.

To identify valuable positions, we need to quantify the \textit{edge contribution} of each position, \ie the contribution to edge discovery.
Given a mutation $M$ in the fuzzing process and the mutation position sequence $M\_pos = \{pos_{1}, \ldots, pos_{n}\}$. We regard the execution process of the target program as a black-box model, whose input is the mutation position sequence $M\_pos$, and outputs the number of new edges $E$ found by the mutated input. However, not all contributions in the mutation position sequence $M\_pos$ are the same. There are often many redundant mutated positions. Therefore, we can use the shapely value to calculate the marginal contribution of each mutated position.
If we accumulate the marginal contribution of position $pos_{i}$ on all mutations, we can get the edge contribution of $pos_{i}$.

Due to the time-consuming calculation process of shapely value, we cannot directly apply it to infer valuable positions in the fuzzing process. To quantify the edge contribution of each position more lightweight, we optimize from the following two aspects.

\textbf{Reduce the number of mutations to analyze. }
In the fuzzing process, most of the mutations cannot discover new edges, and they are not helpful for the inference of valuable positions.
If we analyze millions of mutations in the fuzzing process, the time required is unacceptable.
Therefore, we only performed analysis on those mutations that discovered new edges.

\textbf{Simplify the calculation process of shapely value. }
According to the Equation~\ref{equ:shapely}, the shapely value is the weighted average of the marginal contribution of the target feature in all feature combination subsets under a given sample, and its time complexity is $2^{N}$.
If we use it during fuzzing, it will seriously reduce efficiency.
Assuming that the mutation position sequence has 32 positions, to calculate the contribution of each position, we need to additionally analyze the number of new edges found in $2^{32}$ mutation position sequence subsets.
Therefore, we propose a more lightweight calculation method.
Assuming that several mutations are performed on a seed $s$, $F$ is all mutation samples that find new edges.
Given a position $i$, its edge contribution is $\beta$, and the calculation formula is:
\begin{equation} \label{equ:edgeContribution}
\beta = \sum_{M \subseteq F} val(M) - val(M/pos_{i})
\end{equation}
Among them, $val(M)$ is the number of new edges found by mutation $M$.
$M/pos_{i}$ is to cancel the mutation of $pos_{i}$ in mutation $M$.
For each mutation, we only consider the marginal contribution of each position on the largest mutation position sequence set, which can reduce the time complexity to the O(n) level. If $\beta > 0$, position i is considered to be a valuable position.

Note that we only deal with mutated input without length mutators because length mutators can cause most positions to change.
Moreover, the length mutation operator can easily change the seed structure, making the analysis more difficult.
Figure~\ref{Inference} presents the overall process of valuable position inference.
Given a seed $S$, and its mutated inputs $A$, $B$ and $C$. Among them, $A$ and $C$ found 3 new edges, and $B$ found no new ones. Then, we calculate the marginal contribution of each position in mutations $A$, $B$ and $C$ based on the formula \ref{equ:edgeContribution}. In $A$, the marginal contributions of $pos 1$ and $pos 2$ are 2 and 1, respectively. Since $pos 3$ and $pos 4$ have not been mutated, their marginal contribution is 0. Similarly, the marginal contributions of $pos 1$ and $pos 3$ in $C$ are 1 and 2, respectively. Since $B$ does not discover the new edge, we skip it. Finally, we accumulate the marginal contribution of each position under all mutations, and get the edge contributions of $pos 1, pos 2, pos 3$ and $pos 4$ to be 3, 1, 2 and 0, respectively. Therefore, $pos 1, pos 2, pos 3$ are valuable positions.

\begin{figure}[!t]
\includegraphics[width=0.95\linewidth]{images/Inference.png}
\caption{The overall process of valuable position inference.}
\label{Inference}
\end{figure}

\subsection{Family System}
To speed up the inference of valuable positions, we propose a family system that can divide seeds into multiple families in a lightweight method.
In each family, we will maintain a shared pool for sharing the valuable positions found by all seeds in the family.

\subsubsection{Why Family System Matters}
% The above inference of valuable positions is for a single seed, which depends on a single seed being allocated enough energy for the mutation to obtain sufficient information.
% However, many studies have pointed out that the potential of different seeds is also different. If high energy is allocated to those low-potential seeds, it will affect the fuzzing efficiency.
% To alleviate this problem, 

Shapely Value is a posterior algorithm, which can only show that the valuable positions on a seed were efficient in the past.
However, efficiency in the past does not mean efficiency in the future.
We need to identify the valuable positions of the seed before mutation to discover more new edges.
It can be seen from motivation that there is a connection between constraints, which indicates that the same valuable positions may exist between different seeds.
Moreover, we have experimentally verified the universality of sharing valuable positions among seeds in X.
Therefore, we can identify valuable positions from mutated seeds and share them with unmutated seeds, thereby improving fuzzing efficiency.

What kind of seeds can share valuable positions?
To solve this problem, we cluster seeds into families based on semantic consistency (i.e., the same position has the same semantics on different seeds).
In the same family, different seeds have the same valuable positions. Therefore, they can share the inference process of valuable positions, thus saving inference time. In other words, if a seed in a family finds some valuable positions during the mutation process, other seeds in the family can directly regard these positions as valuable positions, avoiding repeated inference processes.

However, there are significant differences in structure and length between seeds.
The same position can also have completely different meanings on different seeds.
Even with corresponding grammatical analysis tools, the judgment of semantic consistency is very time-consuming and complicated.
Therefore, we expand the determination range of the family to avoid missing those seeds that meet the semantic consistency.
Therefore, we propose two key conditions for semantic consistency between seeds: inheritance relationship and length consistency.
If the above conditions are met between seeds, then they may be able to maintain semantic consistency. Otherwise, we cannot decide due to the complexity of the seed structure.

\textbf{Inheritance relationship. }
Structural consistency among seeds is the advance of semantic consistency.
It is very difficult to directly determine whether the structure consistency between seeds is maintained, which needs to rely on complex grammar parsing tools.
However, we can establish structural connections between seeds through inheritance relationships.
Suppose seed $A$ is mutated from seed $B$, and $x$ positions are mutated.
If $x$ is 0, then $A$ and $B$ must maintain structural consistency.
And, the larger $x$ is, the smaller the probability that $A$ and $B$ maintain structural consistency. This is because the more mutation positions, the greater the probability of causing changes in the seed structure.
So, if there is an inheritance relationship between seeds, it is possible for them to maintain structural consistency. Otherwise, it is difficult to judge lightly.

\textbf{Length consistency. }
If the lengths between seeds are inconsistent, then semantic consistency must not be satisfied.
To share valuable positions between seeds with inconsistent lengths, we need to build position mapping between seeds to link positions with the same semantics.
However, the construction of position mapping becomes difficult due to the existence of length mutators such as insertion/deletion in the fuzzing process.
Therefore, we only consider the semantic consistency between those seeds with the same length.

\subsubsection{Family Construct}
To share valuable positions, we group those seeds with inheritance relationships and consistent length into a family.
The key of building a family is that the mutation does not change the length of original seeds. However, many fuzzers mutate seeds via changing the length of seeds, such as inserting bytes and deleting bytes. To enrich family members, \tool{} will withdraw all mutators that change length when new code are discovered.
If the result can still find the same new edges after withdrawing those mutators, \tool{} will retain the result to a family based on inheritance relationship and seed length.
if we select a seed from family $N$ and generate an 
For example, as shown in Figure~\ref{fig:family_update}, we select a seed from family $N$ and mutate it. 
If an input $i_1$ discovers new edges, \tool{} will withdraw all mutators that change length, which generates another input $i_2$. If $i_2$ can still find the same new edges that $i_1$ finds, \tool{} retains $i_2$ to the family $N$.
Otherwise, $i_1$ will form a new family $N+1$ if mutation of $i_1$ can further discover new edges.
As a result, \tool{} has a reasonable number of families and family members. 

\begin{figure}[t!]
\includegraphics[width=\linewidth]{images/upate.png}
\caption{The update of family and family members.}
\label{fig:family_update}
\end{figure}

\subsubsection{Shared Pool}
To share valuable positions within the family, each family has its own shared pool to record all valuable positions found by all seeds in the family.
A seed can either add the found valuable positions to the shared pool, or obtain the unknown valuable positions from the shared pool.
The update process of the shared pool is shown in Algorithm~\ref{alg:sharedPool}.

\begin{algorithm}[h]
\footnotesize
\caption{The update process of the shared pool.}\label{alg:sharedPool}
% \KwIn{$\alpha$ $\in$ $ \mathbb{R}_{+} $ }
\While{$True$}{
    $s \gets selectSeed(M)$\;
    $f \gets getFamily(s)$\;
    $energy \gets calEnergy(s)$\;
    \While{$energy > 0$}{
        $s_{new} \gets mutate(s)$\;
        $E \gets findsNewEdges(s_{new})$\;
        \If{$E \neq \emptyset$}{
            $pos_{v} \gets shapelyAnalysis(s, s_{new})$\;
            $s_{w} \gets withdraw(s_{new})$\;
            $res \gets stillFindNewEdges(s_{w})$\;
            \eIf{$res == 1$}{
                $addToFamily(f.members, s_{w})$\;
                $addToSharedPool(f.sharedPool, pos_{v})$\;
                $addToQueue(s_{w})$\;
            }
            {
                $constructNewFamily(s_{new}, pos_{v})$\;
                $addToQueue(s_{new})$\;
            }
        }
        $energy \gets energy - 1$\;
    }
}
\end{algorithm}

\tool{} first mutates the selected seed $s$ and gets the family $f$ (lines 2-6) where the seed is located. If the mutated input $s_{new}$ finds a new edge, we infer the valuable positions $pos_{v}$ on the seed $s$ based on formula X (lines 7-9). To avoid the use of the length mutation operator affecting the update of the family, we try to withdraw all the length mutation operators to get $S_{w}$(line 10).
If $S_{w}$ can still find the same new edge, we add $S_{w}$ to members of the family $f$ and add valuable positions $pos_{v}$ to the shared pool of the family $f$(lines 11-13).
Otherwise, we construct a new family using $s_{new}$ and $pos_{v}$.

\subsection{Family-based Mutation}
After obtaining the valuable positions of each seed, we assign more energy to them for the mutation to discover new edges.
Therefore, we propose a family-based mutation.
More specifically, given a seed, we will obtain valuable positions from the shared pool of the family where the seed is located.
Then, we randomly select positions from their valuable positions for mutation.

However, valuable positions will become stale after a period of testing, which indicates they will discover less edges over time.
Therefore, we need to continuously increase the number of valuable positions during fuzzing. To achieve this, \tool{} switches between family-based mutation and random mutation. Family-based mutation is the strategy described in this section, while random mutation will simply select byte positions randomly and mutate them.
To switch mutation modes, \tool{} uses a simple yet effective indicator calculated as:

\begin{equation} \label{equ:cost}
c = \frac{N_{exec}}{N_{new\_paths}},
\end{equation}
where $N_{exec}$ is the number of executions, and $N_{new\_paths}$ is the number of new paths found in those executions. 


The result $c$ is the cost to discover one new path. Lower cost $c$ indicates higher efficiency of a mutation mode.
Both family-based mutation and random mutation have their own costs $c$. When deciding the mode to perform, \tool{} compares the costs of the two modes, and selects the mode with lower cost.

}



\subsection{Threats to Validity}

Our \tool{} is proposed based on the results of SHAP analysis, which is an empirical method. Thus, we were concerned about the generality of our claims due to the small number of samples. 
However, we analyzed the root causes of the SHAP results to support our claims.  
These root causes, direct and indirect coupling of path constraints, are general observations of the nature of programs and independent from our empirical study.
Even if our claim does not include all programs, we believe it satisfies the majority of modern programs.


The second concern comes from the internal threat to validity, which is our solution to optimize byte selection. 
Our solution is based on two assumptions. The first is that there are valuable positions for us to optimize. The second is that our family system can capture the structural information of target programs. 
For the first assumption, we use the random mutation mode to obtain valuable positions.
However, random mutations can only increase the number of valuable positions up to a limit.
To solve this problem, we can use existing solutions that find constraint-related byte positions, such as GreyOne~\cite{greyone}, Angora~\cite{angora} and Driller~\cite{driller}. These solutions are efficient in finding positions related to a single path constraint, which is exactly what we want.
For the second assumption, it is mainly used to share valuable positions among different seeds. This requires that valuable positions in different seeds are still related to path constraints.
However, the family system can only roughly satisfy this requirement. 
One solution to solve this is to analyze programs case by case. That is, we capture the structural information based on syntax analysis tools or even manually determine the constraint-related positions in different seeds.
Yet, we believe such a solution limits the scalability of fuzzing, \ie it is only effective in specific programs.
Although the family system cannot accurately capture structural information, CMAB refines the selection of valuable positions, which is scalable to fuzz programs.





==> obsolete/technique-3.1.tex <==
\section{Design of \tool} \label{sec:design}
\zhu{TODO: describe this section; }




\subsection{Cooperative Game in Fuzzing}
As mentioned, bytes in a seed are collaboratively mutated to discover new edges. In this section, we formulate the process of byte mutation as a cooperative game and use Shapley value to quantify the contribution of each byte. We simplify the calculation of Shapley value to increase the efficiency of fuzzing.



% \zhu{TODO: rephrase this paragraph}
% Since the contribution of different positions on a seed to code discovery is inconsistent, we use the Shapley Value to quantify the contribution of each position.
% Moreover, we also use program features to simplify Shapley Value's calculation process to identify those more important positions in the fuzzing process.


\subsubsection{Shapley Value} \label{subsec:shapval}

The Shapley Value is a solution used in Cooperative Game Theory that fairly distributes gains among several players working in a coalition. 
Formally, a cooperative game is defined as: $N$ players form a coalition $S$ and obtain a gain $R$.
Shapley Value can be used to quantify the contribution of each player in a game.
% Following Lloyd S. Shapley~\cite{Shapley},
In the Cooperative Game Theory,
the Shapley Value $\phi_{j}$ of the player $x_{j}$ to the coalition can be calculated as~\cite{Shapley}:
\begin{equation} \label{equ:shapely}
    \phi_{j}=\sum_{S \subseteq X \backslash \{x_{j}\}} \frac{|S| !(N-|S|-1) !}{N !}(\mathcal{F}(S \cup \{x_{j}\})-\mathcal{F}(S)),
\end{equation}
where there are $N$ players in the game, and a coalition $S$ is formed by $m (m \leq N)$ players.
$X$ is the set of all players and $X \backslash \{x_{j}\}$ is all possible coalitions of players excluding the player $x_{j}$. $|S|$ is the number of players in the set $S$.
$\mathcal{F}(*)$ is a characteristic function that describes the gain $R$ that the coalition of players can obtain, i.e., $R = \mathcal{F}(S)$.
$\mathcal{F}(S \cup \{x_{j}\})-\mathcal{F}(S)$ is the marginal contribution of the player $x_{j}$ on the coalition $S$, which describes the effect on the gain of including the player $x_{j}$. In other words, the Shapley value $\phi_{j}$ is a weighted average of $x_{j}$'s marginal contributions across all possible player coalitions. 


% \zhu{remove this?}
% The Equation~(\ref{equ:shapely}) only calculates the Shapley value of the player $x_j$ in a single sample. In some scenarios, such as machine learning, different samples will be utilized to calculate Shapley values for the same player. To measure the importance of a player when multiple samples exist, studies accumulate the Shapley values of the player on all samples~\cite{SV1,SV2,SV3}. Specifically, assuming that $Y$ is the set containing all samples, the importance of the player $x_j$ is calculated as:
% \begin{equation} \label{equ:featureImportance}
%     \eta_{j}=\sum_{y \in Y}\phi_{y,j}
% \end{equation}


% We take the machine learning for housing price to exemplify the concept of Shapley Value. To predict the housing price, a machine learning model $M$ is trained from a dataset $D$ with three features


% \zhu{Give a concrete example of ML here.}
% \zkp{For example, in the housing price prediction problem, we can use Shapley Value to determine the importance of each feature.
% Suppose there is a simple housing price dataset $D$, and a model $M$ trained from it.
% Each record in the dataset describes the information of a house, including three features(\ie size, number of bedrooms, number of bathrooms) and a label(\ie price).
% We can think of each feature as a player and the price as a gain.
% Based on Equation~\ref{equ:shapely}, we can quantify the contribution of each feature to price in each record in the data set $D$, \ie Shapley Value.
% To get the feature importance, we accumulate the Shapley Values of each feature on all records.}
% In a game, there are $N$ players, and $m (m \leq N)$ players can form a coalition $S$.
% Then, the characteristic function is used to complete the mapping between coalition $S$ and gain, which is used to calculate the gain that the current coalition can obtain.

% Thus, the application of Shapley Value to describe the contribution of each player in a cooperative game needs to determine the following key issues:
% \begin{itemize}
%     \item what is a game?
%     \item How to define player, coalition, gain and characteristic function in a game?
% \end{itemize}


% \subsection{Shapley Value in Machine Learning\zhu{remove this subsection}}
% The machine learning model is a blackbox, and the internal mechanism is extremely complex, which is difficult to describe in human-understandable language.
% In order to quantify the importance of each feature in a machine learning model, many studies~\cite{SV1,SV2,SV3} have used Shapley Value for research.
% In machine learning, a game refers to inputting a sample into the model and getting the model's output.
% Assuming that there is an N-dimensional sample $x$, we can complete the conceptual mapping: 
% \textbf{player} refers to a feature $f_{j}$ in the sample.
% \textbf{coalition} is feature subset $S \subseteq F$, where $F$ is the set of all features. The value of sample $x$ on feature subset $S$ constitutes model input $x_{S}$.
% \textbf{gain} refers to the model output obtained by the machine learning model for the model input.
% \textbf{characteristic function} refers to the machine learning model $f(*)$, which is used to complete the mapping from model input to model output.
% Note that the model on different feature subsets is different.
% We need to retrain the model based on each feature subset $S \subseteq F$. Thus, $f_{S}(*)$ is trained with the feature subset $S$.
% Formally, the Shapley Value $\phi_{j}$ of the $j$th feature $f_{j}$ of the sample $x$ can be calculated as:
% \begin{equation} \label{equ:shapelyML}
%     \phi_{x,j}=\sum_{S \subseteq F \backslash \{f_{j}\}} \frac{|S| !(N-|S|-1) !}{N !}(f_{S \cup \{f_{j}\}}(x_{S \cup \{f_{j}\}})-f_{S}(x_{S}))
% \end{equation}

% The Shapley Value calculated for each feature can be interpreted as how that feature contributes to the predicted value of the model.
% However, the Equation~\ref{equ:shapelyML} just calculates the Shapley Value of a feature in a single sample. If we want to analyze the feature importance of the model, we need to accumulate the Shapley Values of the target feature on all samples.
% Assume $X$ are the set containing all samples. Thus, the feature importance $\eta_{j}$ of feature $f_{j}$ is calculated as:
% % \begin{equation} \label{equ:featureImportance}
% %     \eta_{j}=\sum_{x \in X}\phi_{x,j}
% % \end{equation}

% \subsection{Shapley Value in Fuzzing\zhu{Cooperative Game in One Seed}}
\subsection{Cooperative Game in One Seed} \label{sec:cg_oneseed}
\zhu{TODO}
From the perspective of Cooperative Game Theory, we understand the mutation process for a seed as a learning process to analyze the relationships between positions and code discovery.
The mutation process includes several mutations, and each mutation mainly has the following three steps: select mutated positions, generate the mutation input, and put it into the target program for execution.
Discovering all new edges in the target program essentially requires constantly flipping the CMPs in the program.
The flipping of CMPs has two cases: If we flip those CMPs with unexplored branches, we can directly discover new edges. Flipping those CMPs where all branches have been explored may also trigger other program logic to discover new edges deep in the program.
Thus, we believe that a position's efficiency is determined by its contributions to CMP flipping.
Since a mutation may mutate multiple positions simultaneously, the CMP flipping is the result of the coalition of positions.
Naturally, we can use Shapley Value to measure the contribution of each position in a mutation.

The mutation process for a seed involves several mutations to the seed.
Since Shapley Value analyzes an observation, we regard a mutation as an observation.
To apply Shapley Value to analyze each mutation, we need to redefine the concepts required by Shapley Value in fuzzing.

\subsubsection{Conceptual mapping between fuzzing and cooperative game}
In the mutation process for a seed $S$, assume there is a mutation $M$ and the mutation position sequence $M_{pos} = \{p_{1}, \ldots, p_{n}\}$.
In a mutation, we generate a mutated input for the seed $S$ based on the mutated position sequence, and put the mutated input into the target program to execute to get the feedback result.
We treat a mutation on seed $S$ as \textbf{a game}.
More specifically, we treat a position on the seed $S$ as a \textbf{player}, and the mutated position sequence $M_{pos}$ as a \textbf{coalition}.
Our goal is to establish the mapping relationship between position and CMP flipping, that is, to analyze which positions on the seed $S$ can flip CMPs.
The most intuitive idea is to define \textbf{gain} as whether the path exercised by the mutated input has changed relative to the seed $S$. If it changes, it means that mutated positions contribute to CMP flipping. Otherwise, it does not.

But for a CMP, it is enough for us to extract only one combination of positions that can flip it on the seed $S$.
Repeated extraction will only cause functional redundancy. That is, multiple extracted positions are related to the same CMP.
Therefore, we finally define \textbf{gain} as: the number of new edges found by the mutated input relative to the seed $S$, that is, the number of \textbf{self-new edges}. Note that the \textbf{self-new edges} of the seed $S$ refer to the new edges discovered relative to the seed $S$ and its generated mutated inputs.
Finally, we define the \textbf{characteristic function} $\mathcal{F}(*)$ as:
Given a seed $S$ and target program $P$, the mapping between mutated position sequence and the number of self-new edges.


\subsubsection{Simplification of Shapley Value Calculation}

Suppose in a mutation of seed $S$, mutation position sequence $M_{pos} = \{p_{1}, \ldots, p_{n}\}$. There are a total of $N$ mutated positions. Based on the Equation~\ref{equ:shapely} of Shapley Value, the contribution $\phi_{j}$ of position $p_{j}$ to CMP flipping can be calculated as:
\begin{equation} \label{equ:shapelyFuzzing}
    \phi_{j}=\sum_{T \subseteq M_{pos} \backslash \{p_{j}\}} \frac{|T| !(N-|T|-1) !}{N !}(\mathcal{F}(T \cup \{p_{j}\})-\mathcal{F}(T))
\end{equation}

The contribution of position $p_{j}$ in the mutation $M$ is the weighted average of the marginal contribution of the position $p_{j}$ in all possible subsets of the mutation position sequence $M_{pos}$, which brings a time complexity of $2^{N}$.
If we quantify the contribution of each position to CMP flipping during the fuzzing process, the throughput will be severely reduced, which will affect the efficiency of fuzzing.
Therefore, we need to use program features to simplify the calculation Equation~\ref{equ:shapelyFuzzing}.

First of all, we found that there are often some redundant mutated positions in a mutation. Mutation of redundant positions does not affect the discovery of self-new edges.
Formally, given the mutation position sequence $M_{pos} = \{p_{1}, \ldots, p_{n}\}$. If position $p_{j}$ satisfies the formula ~\ref{equ:redundant}, it means that the mutation of position $p_{j}$ is redundant.
\begin{equation} \label{equ:redundant}
    \mathcal{F}(M_{pos}) = \mathcal{F}(M_{pos} \backslash \{p_{j}\})
\end{equation}
Therefore, the effect of $M_{pos} \backslash \{p_{j}\}$ is the same as $M_{pos}$.
Then, we can replace $M_{pos}$ with $M_{pos} \backslash \{p_{j}\}$ so that the number of positions we need to analyze is reduced.

Secondly, the flipping of CMPs in the program often depends on the simultaneous mutation of multiple positions, that is, the 0-N case.
Suppose a CMP flip depends on the simultaneous mutation of all positions in $M_{pos} = \{p_{1}, \ldots, p_{n}\}$. Therefore, any subset of $M_{pos}$ cannot flip this CMP, that is:
\begin{equation} \label{equ:necessary}
    \mathcal{F}(m) = 0, m \subset M_{pos}
\end{equation}

In this case, the Equation~\ref{equ:shapelyFuzzing} can be simplified to:
\begin{equation} \label{equ:shapelyFuzzing01}
    \phi_{j}= \frac{|M_{pos}| !(N-|M_{pos}|-1) !}{N !}(\mathcal{F}(M_{pos}))
\end{equation}
So, $\phi_{j}$ is no longer related to $j$.
Suppose we can determine that each position in a mutation is necessary. In that case, we can directly use the formula ~\ref{equ:shapelyFuzzing01} to calculate the Shapley Value of each position, so that we no longer need to analyze the execution of the $M_{pos}$ subset.

Based on the above two characteristics, we propose our simplified Shapley Value calculation algorithm. The specific process is shown in the algorithm~\ref{alg:shapley}.

\begin{algorithm}[h]
\footnotesize
\caption{Simplified Shapley Value calculation algorithm}\label{alg:shapley}
\KwIn{
    A mutation $M$,the mutated position sequence $M_{pos} = \{p_{1}, \ldots, p_{n}\}$ and a function $\mathcal{F}(*)$ mapping between mutated position sequence and self-new edges.
    
}

$SV[n] = {0}$\; 
$totalEdges = \mathcal{F}(M_{pos})$\;
$flag = 1$\;
\For{$pos \in M_{pos}$}{
    \If{$\mathcal{F}(M_{pos} \backslash \{pos\}) == totalEdges$}{
        $M_{pos}.delete(pos)$\;
    }
    \lElseIf{$\mathcal{F}(M_{pos} \backslash \{pos\}) \neq 0$}{
        $flag = 0$
    }
}
\eIf{$flag$}{
    $averageSV = simplifiedShapleyAnalysis(M_{pos}, \mathcal{F})$\;
    \For{$i \in n$}{
        $SV[i] = averageSV$\;
    }
}
{
    \For{$i \in n$}{
        $SV[i] = shapleyAnalysis(M_{pos}, \mathcal{F})$\;
    }
}
\end{algorithm}

Based on the algorithm ~\ref{alg:shapley}, we can quantify the contribution of each position to CMP flipping in each mutation, that is, the Shapley Value.
First, given the mutated position sequence $M_{pos}$, we initialize the Shapley Value of each position in $M_{pos}$, and record the number of self-new edges $totalEdges$ found by $M_{pos}$ (lines 1-2).
Second, we cancel the mutation of each position one by one, and remove redundant positions to reduce the number of positions required for analysis (lines 4-6).
Third, we analyze whether the mutation conforms to the 0-N case.
Specifically, we analyze whether the discovery of self-new edges depends on the simultaneous mutation of all remaining positions. If other values other than 0 and $totalEdges$ are found when canceling the mutation of each position, it means that the 0-N case is not met (line 7).
Finally, in the 0-N case, we consider all remaining positions to contribute equally to the self-new edges. Therefore, we directly use Equation~\ref{equ:shapelyFuzzing01} to calculate the Shapley Value of each position without analyzing the results of each subset (lines 8-11).
If it does not meet the 0-1 situation, we will continue to use the formula ~\ref{equ:shapelyFuzzing} for detailed analysis (lines 12-14).

\subsubsection{Position Importance}
Since the mutation process for a seed includes several mutations, we can accumulate the Shapley Value of a position on all mutations to obtain position importance. Position importance is used to quantify the importance of a position on the seed in CMP flipping.
Formally, assume that during the mutation process on the seed $S$, $R$ is the set of mutations for which self-new edges are found. The position importance $\beta_{j}$ of position $p_{i}$ can be calculated as:
\begin{equation} \label{equ:totalContribution}
\beta_{j} = \sum_{r \in R} SV_{r,p_{i}}
\end{equation}
Among them, $SV_{r,p_{i}}$ represents the Shapley Value of $p_{i}$ in the mutation $r$.


% \section{family system}
\subsection{Cooperative Game Across Seeds}
% \zhu{Title: 2.4 cooperative game across seeds}

However, according to the formula~\ref{equ:totalContribution}, the calculation of position importance relies on a single seed having enough mutations.
However, the energy distribution of seeds during fuzzing is inconsistent.
Some seeds can only be mutated dozens of times, which cannot accurately calculate the position importance of each position on the seed.
Suppose we can gather those seeds with the same position importance distribution into a family. In that case, these seeds can share the calculation process of position importance, that is, put the mutations of these seeds together to generate a shared position importance distribution.
The same position importance distribution means that the same position on different seeds has the same position importance.
Specifically, assuming that seeds $A$ and $B$ have the same position importance distribution, the mutation sets of seeds $A$ and $B$ are $M_{A}$ and $M_{B}$, respectively.
Therefore, we can combine $M_{A}$ and $M_{B}$ to get a shared mutation set $M_{A, B}$.
Finally, based on Equation~\ref{equ:totalContribution}, we can use $M_{A, B}$ to generate the shared position importance distribution of seeds $A$ and $B$.

% \subsection{Why does the Family System matters}
So, how to gather those seeds with the same position importance distribution into a family?
We found that if there is an inheritance relationship between seeds and the length is consistent, the position importance of the same position on different seeds is consistent.
Suppose there are seeds $A$ and $B$. If seed $B$ is mutated from seed $A$, then there is an inheritance relationship between seeds $A$ and $B$.
Note that inheritance relationships are transitive.
Suppose the seed $A$ is mutated to get $B$, and the seed $B$ is mutated to get $C$. Then, there is also an inheritance relationship between $A$ and $C$.
We discuss why such seeds have the same position importance distribution in two cases.

\textbf{The case of two seeds.}
If there are seeds $A$ and $B$, the paths of $A$ and $B$ are inconsistent. The lengths of seeds $A$ and $B$ are the same.
Assuming that $A$ can mutate the position $i$ to get $B$, then $B$ can also mutate the position $i$ to get A.
Moreover, the CMPs flipped during the two conversions of $A \rightarrow B$ and $B \rightarrow A$ are the same.
Therefore, we believe that "the contribution of the position $i$ to CMP flipping in $A$" and "the contribution of the position $i$ to CMP flipping in $B$" is consistent.

\textbf{The case of multiple seeds.}
If $A$ mutates position $i$ to get $B$, $B$ mutates position $j$ to get $C$. The lengths of the seeds $A$, $B$, and $C$ are the same.
If we ignore the intermediate node $B$ and integrate two mutations, it becomes: $A$ mutates positions $i,j$ at the same time, and $C$ can be found. In the same way, $C$ can also find $A$ by mutating positions $i, j$ at the same time.
Moreover, the CMPs flipped during the two conversions of $A \rightarrow C$ and $C \rightarrow A$ are the same.
Therefore, we believe that "the contribution of position $i,j$ to CMP flipping in $A$" and "the contribution of position $i,j$ to CMP flipping in $C$" are consistent.

Therefore, if the seeds are inherited and have the same length, they share the same position importance distribution.
With this feature, we propose the family system.
More specifically, we group seeds with inheritance relationships and the same length into a family.
All seeds within each family share the same position importance distribution.
Therefore, we can combine all mutations of all seeds in the family to generate a shared position importance distribution.
Formally, assume that family $F$ contains M seeds, that is, $F = \{S_{1}, \ldots, S_{M}\}$. All seeds in this family have length $N$, and each seed $S_{i}$ has its own mutation set $M_{i}$.
Therefore, we merge the mutation sets $M_{all} = \{M_{i} | i \in [1,M]\}$ of all seeds, and generate a shared position importance distribution $D = \{\beta_{i} | i \in [1,N]\}$.
Among them, the position importance $\beta_{i}$ of the jth position $p_{j}$ can be calculated as:
\begin{equation} \label{equ:share}
\beta_{j} = \sum_{r \in M_{all}} V_{r,p_{i}}
\end{equation}
Among them, $V_{r,p_{i}}$ represents the Shapley Value of $p_{i}$ in mutation $r$.
In this way, even if some seeds are only mutated dozens of times, we can still calculate the position importance of each position for it.


\section{Shapley-based Boosting}
\zhu{New section: Title: 3. Shapley-based Boosting; This includes the insights and family construction}

\subsection{Family Construct}

The key of building a family is that the mutation does not change the length of original seeds. However, many fuzzers mutate seeds via changing the length of seeds, such as inserting positions and deleting positions. To enrich family members, \tool{} will withdraw all mutators that change length when new code are discovered.
If the result can still find the same new edges after withdrawing those mutators, \tool{} will retain the result to a family based on inheritance relationship and seed length.
if we select a seed from family $N$ and generate an 
For example, as shown in Figure~\ref{fig:family_update}, we select a seed from family $N$ and mutate it. 
If an input $i_1$ discovers new edges, \tool{} will withdraw all mutators that change length, which generates another input $i_2$. If $i_2$ can still find the same new edges that $i_1$ finds, \tool{} retains $i_2$ to the family $N$.
Otherwise, $i_1$ will form a new family $N+1$ if mutation of $i_1$ can further discover new edges.
As a result, \tool{} has a reasonable number of families and family members. 

\begin{figure}[t!]
\includegraphics[width=\linewidth]{images/upate.png}
\caption{The update of family and family members.}
\label{fig:family_update}
\end{figure}



\subsection{Mutation}\zkp{change the section name}
The Shapley Value analysis process is embedded in fuzzing. After a period of fuzzing, we obtained the position importance of some positions. Then, we can focus on mutating positions with higher position importance.
However, when can position importance be used to guide the direction of fuzzing?
To solve this problem, we divide fuzzing into two modes: Shapley analysis mode and Shapley-guided mutation mode.
Suppose we mutate a seed $S$.

In the Shapley analysis mode, we randomly select positions for mutation like the AFL strategy, and use the Shapley Value to analyze the contribution of each position during the mutation process, and finally get the position importance of each position.

In Shapley-guided mutation mode, we construct a set of positions whose position importance is greater than 0, representing the positions on the seed that contribute to CMP flipping. Then, we randomly select positions from among them for mutation.
If the position importance of a position is higher, it means it is more important. Then we should allocate more mutators to mutate the position and its surrounding positions.
Formally, in a mutation $M$ of the seed $S$, assuming that the position $p_{j}$ whose position importance is $\beta_{j}$ is to be mutated, then the number of mutators $Num $ allocated can be calculated as:

\begin{equation}
Num = 
\begin{cases}
\frac{5}{1+e^{\beta_{j}}} - 2.5& \beta_{j} > 0\\
0& \beta_{j} \leq 0
\end{cases}
\end{equation}
Since the scope of different mutators is different, if the position importance of a position is greater, the probability of its surrounding positions being mutated is also greater.

Further, Shapley analysis mode tends to mutate all positions to optimize position importance distribution of a seed, while B tends to use the existing position importance to guide the fuzzing direction.
We need to balance the two modes.
To switch mutation modes, \tool{} uses a simple yet effective indicator calculated as:

\begin{equation} \label{equ:cost}
c = \frac{N_{exec}}{N_{new\_paths}},
\end{equation}
where $N_{exec}$ is the number of executions, and $N_{new\_paths}$ is the number of new paths found in those executions. 


The result $c$ is the cost to discover one new path. Lower cost $c$ indicates higher efficiency of a mutation mode.
Both Shapley analysis mode and Shapley-guided mutation mode have their own costs $c$. When deciding the mode to perform, \tool{} compares the costs of the two modes, and selects the mode with lower cost.



% \subsection{Insight}
% So, why do we repeatedly mutate the positions that contribute to CMP flipping?
% Two of the reasons for this problem are the direct and indirect coupling of path constraints.
% The \textit{direct coupling} means that the flipping of a path constraint has to consider the results of other path constraints in the same execution path. Therefore, repeated mutation of certain positions can explore all the directly coupled constraints.
% On the other hand, different program logic may process the same format of inputs, indicating that different constraints could be related to the same positions of different inputs (\textit{indirect coupling}).
% Therefore, the mutation of the same positions across different seeds can discover new code along different paths.


% \begin{sloppypar}
% We exemplify the two reasons by a real-world program \texttt{readelf} in this section.
% The program \texttt{readelf} processes files with ELF format and shows the information of ELF. An ELF file is mainly composed of a series of sections whose information is recorded and managed by the section headers. 
% As shown in Figure~\ref{example_readelf}, \texttt{readelf} processes ELF files via a sequence of tasks. For example, to process objects, \texttt{readelf} will execute the sequence of functions \texttt{process\_relocs()}, \texttt{process\_version\_sections()}, and \texttt{process\_section\_contents()}.
% \end{sloppypar}

% % \begin{figure*}[t!]
% % \centering
% % \includegraphics[width=0.85\linewidth]{images/motivation.pdf}
% % \caption{The reason for the results of SHAP analysis.}
% % \label{example_readelf}
% % \end{figure*}


% \textit{Direct Coupling.} The direct coupling indicates the direct influence among different path constraints along the same execution path. In Figure~\ref{example_readelf}, the path constraint in line 5 is defined by the function \texttt{process\_section\_contents()}, whose boolean output is determined by the constraints of lines 16, 17 and 18. That is, the constraint in line 5 is determined by three other constraints. To make the condition in line 5 \textit{true} (\ie the value of \texttt{res} in line 19 is \textit{false}), an input needs to satisfy 1) condition in line 16 is \textit{false}, and 2) one of the conditions in lines 17 and 18 is \textit{true}. This requires a fuzzer to fuzz the constraints of lines 16, 17 and 18 simultaneously. 
% Therefore, the repeated mutation of positions related to a single constraint can help fuzz code lines that are guarded by complex path constraints (\ie deep code).


% \textit{Indirect Coupling.} The indirect coupling indicates that two path constraints process the same input format. For example, in Figure~\ref{example_readelf}, both the constraints of lines 10 and 23 check the value of \texttt{sh\_type}, which represents the types of sections. 
% Therefore, if a seed $S_1$ has inferred the related positions of \texttt{sh\_type} to resolve the constraint in line 10, a fuzzer can mutate those positions in another seed $S_2$ that intends to resolve the constraint in line 23. As long as the meaning of those positions remains the same between seeds $S_1$ and $S_2$, the fuzzer can quickly explore the \texttt{case}s in function \texttt{process\_version\_sections()}. 
% Therefore, to boost the efficiency of fuzzing, a fuzzer can repeatedly mutate positions that have discovered new coverage across different execution paths.

% \subsection{Explainability Analysis}
% The relationship between position and edge discovery is complex, including direct correlation and indirect correlation.
% Most existing methods only solve the direct correlation, such as GREYONE, Angora, etc.
% The indirect correlation is complicated because it is affected by the CFG graph. Only some simple cases can be solved at present.
% For example, Matryoshka aims to solve the problem of nested conditions.
% However, nested conditions are only one case that is indirectly related.
% Indirect correlations also include more complex situations.
% Therefore, we approach this problem from the perspective of statistical analysis.
% We regard the fuzzing process as a black box model, the input is mutated positions, and the output is the number of new edges discovered. In other words, we look for the relationship between position and edge discovery from a higher dimension.

% To quantify the contribution of each position to edge discovery on a seed, we used AFL++ to run fuzzing experiments with a set of diversified seed inputs. 
% Specifically, we continuously mutate each initial seed for 24 hours.
% Note that only the initial seed is mutated in this process, and the new seeds generated by it are not mutated. During the mutation process, if mutation of some byte positions discovers new code, we iterate all the combinations of those mutated bytes, and record the new edges discovered by each combination. For example, suppose a mutation finds new edges, and its mutated positions are \{1,3,4\}. 
% We need to collect additionally how many new edges each subset \{1\}/\{3\}/\{4\}/\{1,3\}/\{1,4\}/\{3,4\} can discover. Then we calculate the contribution of each position based on Equation~\ref{equ:shapely}. 
% Finally, we accumulate all contributions of a position across all mutations.
% The result of our analysis is the contribution of each byte position to code discovery.

% We conduct experiments on 18 programs, including \textit{nm}, \textit{readelf}, \textit{size}, \textit{objdump}, \textit{tiff2bw}, \textit{tiffsplit} and so on.
% There are also 9 types of program input, including \textit{elf}, \textit{tiff}, \textit{pdf}, \textit{text}, \textit{mp4}, \textit{flv}, \textit{wav}, \textit{jpg} and \textit{mp3}.
% % We repeated the experiment three times to avoid the influence of randomness.
% We draw a scatter diagram to describe how many new edges are contributed by the top X\% positions of the shapey value.
% The result is shown in the Figure~\ref{shap_scatter}.
% A point in the figure indicates that under a program and a seed, the top X\% positions of the shapey value can contribute Y\% of the new edges.
% We found that under some programs, 1\% of bytes can contribute more than 80\% of new edges.
% Therefore, we can draw a conclusion: The discovery of code largely depends on a small portion of byte positions.


% \begin{figure}[t!]
% \centering
% \includegraphics[width=\linewidth]{images/shap_scatter.png}
% \caption{Top X\% positions of the shapey value VS Percentage of contributing new edges.}
% \label{shap_scatter}
% \end{figure}

==> obsolete/technique-3.2.tex <==
\section{Design of \tool} \label{sec:design}
\zhu{TODO: describe this section; }

\zhu{TODO: a figure to show the formulation of byte mutation, cooperative game}


\subsection{Cooperative Game Among Bytes} \label{subsec:cg_all}
As mentioned, bytes in a seed are collaboratively mutated to discover new edges. Therefore, we formulate the process of byte mutation as a cooperative game and use Shapley value to quantify the contribution of each byte. We first formulate the mutation of one seed and then extend it to multiple seeds based on the characteristics of mutation. 
% To increase the efficiency of fuzzing, we further simplify the calculation of Shapley value for fuzzing.


% and then simplify the calculation of Shapley value to increase the efficiency of fuzzing. Based on the characteristics of mutation, we extend the formulation from one seed to multiple seeds. 




\subsubsection{Shapley Value} \label{subsec:shapval}

The Shapley Value is a solution used in Cooperative Game Theory that fairly distributes gains among several players working in a coalition. 
A cooperative game is one that $N$ players form coalitions and obtain gains by a characteristic function.
Shapley Value can be used to quantify the contribution of each player in a game.
% Following Lloyd S. Shapley~\cite{Shapley},
In the Cooperative Game Theory,
the Shapley Value $\phi_{j}$ of the player $x_{j}$ to the coalition can be calculated as~\cite{Shapley}:
\begin{equation} \label{equ:shapely}
    \phi_{j}(X)=\sum_{P \subseteq X \backslash \{x_{j}\}} \frac{|P| !(N-|P|-1) !}{N !}(\mathcal{F}(P \cup \{x_{j}\})-\mathcal{F}(P)),
\end{equation}
where there are $N$ players in the game, and a coalition $P$ is formed by $m (m \leq N)$ players.
$X$ is the set of all players and $X \backslash \{x_{j}\}$ is all possible coalitions of players excluding the player $x_{j}$. $|P|$ is the number of players in the set $P$.
$\mathcal{F}(\ast)$ is a characteristic function that describes the gain $R$ that the coalition of players can obtain, \ie $R = \mathcal{F}(P)$.
$\mathcal{F}(P \cup \{x_{j}\})-\mathcal{F}(P)$ is the marginal contribution of the player $x_{j}$ on the coalition $P$, which describes the effect on the gain of including the player $x_{j}$. In other words, the Shapley value $\phi_{j}$ is a weighted average of $x_{j}$'s marginal contributions across all possible player coalitions. 
In other words, the Shapley value reflects the importance of the player $x_j$ in the game.


Coverage-guided fuzzing usually has some initial seeds, and mutation of them may generate new seeds.
If an input that is generated by mutating a seed discovers new edges comparing to the overall discovered coverage, the input is retained as a new seed. For the following fuzzing trials, the new seed will be selected and mutated to generate new inputs. 
This process of generating new inputs and testing them can be regarded the process of Shapley analysis, \ie \textit{trying possible combinations of bytes}.
Yet, the problem is how to gather the trails in fuzzing so that these trails belong to the same cooperative game. 


% \zhu{remove this?}
% The Equation~(\ref{equ:shapely}) only calculates the Shapley value of the player $x_j$ in a single sample. In some scenarios, such as machine learning, different samples will be utilized to calculate Shapley values for the same player. To measure the importance of a player when multiple samples exist, studies accumulate the Shapley values of the player on all samples~\cite{SV1,SV2,SV3}. Specifically, assuming that $Y$ is the set containing all samples, the importance of the player $x_j$ is calculated as:
% \begin{equation} \label{equ:featureImportance}
%     \eta_{j}=\sum_{y \in Y}\phi_{y,j}
% \end{equation}


% Formulation of Byte Mutation
\subsubsection{Cooperative Game in One Seed} \label{subsec:cg_oneseed}
For a seed, the \textbf{cooperative game} is the schedule of bytes on the seed, including the selection of some certain bytes and the mutation of the selected bytes. This game finds a total of $n$ edges and the Shapley value is utilized to analyze the contribution of each byte pertaining to the discovery of those $n$ edges. Thus, a \textbf{player} in the game is a byte in the seed $S_0$, and the \textbf{coalition} is that some certain bytes are mutated together. Since coverage-guided fuzzing aims to discover new code, we define the \textbf{gain} as the number of \textit{self-new edges} discovered by an input $i$ generated by mutating the seed $S_0$. 
To ensure that the gain is consistent during fuzzing, the \textit{self-new edges} are defined as the new edges when comparing the edges discovered by the input $i$ and the initial seed $S_0$. From the perspective of program logic, \textit{a byte related to more path constraints will have larger contribution to the code discovery}. Thus, the use of self-new edges can provide more information about the relations between input bytes and path constraints.
For most fuzzers, such as AFL-based fuzzers~\cite{aflchurn, Zhu2020CSI}, new edges are obtained by comparing to the overall coverage. However, this kind of new edges is ``stateful'' because the order of mutation can influence the result. As a result, depending on the time of mutation, the gain of the same mutation may be different. Therefore, we use self-new edges to avoid the variation of gain. Finally, the \textbf{characteristic function} $\mathcal{F}(*)$ is the mapping between the collaborative mutation and the number of self-new edges.
With the formulation of byte mutation, we can use Equation~(\ref{equ:shapely}) to calculate the Shapley value for each byte. Since the Shapley value reflects the importance of a byte pertaining to code discovery, we can improve the efficiency of fuzzing by \textit{assigning more energy to the bytes with higher Shapley values}.


\subsubsection{Cooperative Game Across Seeds} \label{subsec:cg_multiseed}
Multiple seeds are possible to be treated as one seed from the perspective of Shapley analysis.
Although Section~\ref{subsec:cg_oneseed} formulate byte mutation based on one seed $S_0$, the process of calculating Shapley values will generate new seeds. 
% If a cooperative mutation in $S_0$ discovers new edges comparing to the overall discovered coverage, the generated input by this mutation is retained as a new seed $S_1$. 
If the mutation does not change the length of the original seed $S_0$, the new seed $S_1$ is actually one of the combinations in the cooperative game of seed $S_0$. If the length is changed, the relative positions of bytes are changed, as well as the number of players in the cooperative game. Therefore, without changing length, any mutation of seed $S_1$ still belongs to the cooperative game of seed $S_0$. For example, if seed $S_0$ is mutated byte $i$ to get seed $S_1$, and $S_1$ is mutated byte $j$ to get seed $S_2$. The lengths of the seeds $S_0$, $S_1$, and $S_2$ are the same.
Then, the seed $S_2$ can be obtained by mutating bytes $i,j$ in seed $S_0$.
% Therefore, if multiple seeds are generated from the same original seed and they have the same length, such seeds participate in the same cooperative game.
Therefore, the seeds, which are retained from the same original seed and do not change the length, are part of the combinations for the original seed.
We group such seeds (\eg seeds $S_0$, $S_1$ and $S_2$) into a \textit{family} so that seeds in the same family participate in the same cooperative game. 
To conclude, seeds in a family 1) inherit from the same original seed, 2) obtain the player subset $P$ in Equation~(\ref{equ:shapely}) by comparing to the original seed, and 3) have the same length.


The family can release the overhead of Shapley analysis because it gathers different seeds into the same cooperative game.
During fuzzing, all seeds will be selected and mutated. If we treat byte mutation in every seed as an individual cooperative game, it will have too much overhead.
In Section~\ref{subsec:cg_multiseed}, we conclude that seeds in the same family belong to the same cooperative game. Therefore, we gather the seeds belonging to the same family together, and mutations of all seeds in the family are used to calculate the Shapley values for the first seed in the family. 
The Shapley values for bytes of the first seed are shared with all other seeds in the same family.



\subsection{Shapley-based Boosting}



Since a byte include both position (the order in an input) and value, we transform Equation~(\ref{equ:shapely}) into \zhu{ML form}.


% From the perspective of Cooperative Game Theory, we understand the mutation process for a seed as a learning process to analyze the relationships between positions and code discovery.
% The mutation process includes several mutations, and each mutation mainly has the following three steps: select mutated positions, generate the mutation input, and put it into the target program for execution.
% Discovering all new edges in the target program essentially requires constantly flipping the CMPs in the program.
% The flipping of CMPs has two cases: If we flip those CMPs with unexplored branches, we can directly discover new edges. Flipping those CMPs where all branches have been explored may also trigger other program logic to discover new edges deep in the program.
% Thus, we believe that a position's efficiency is determined by its contributions to CMP flipping.
% Since a mutation may mutate multiple positions simultaneously, the CMP flipping is the result of the coalition of positions.
% Naturally, we can use Shapley Value to measure the contribution of each position in a mutation.

% The mutation process for a seed involves several mutations to the seed.
% Since Shapley Value analyzes an observation, we regard a mutation as an observation.
% To apply Shapley Value to analyze each mutation, we need to redefine the concepts required by Shapley Value in fuzzing.

% \subsubsection{Conceptual mapping between fuzzing and cooperative game}
% In the mutation process for a seed $S$, assume there is a mutation $M$ and the mutation position sequence $M_{pos} = \{p_{1}, \ldots, p_{n}\}$.
% In a mutation, we generate a mutated input for the seed $S$ based on the mutated position sequence, and put the mutated input into the target program to execute to get the feedback result.
% We treat a mutation on seed $S$ as \textbf{a game}.
% More specifically, we treat a position on the seed $S$ as a \textbf{player}, and the mutated position sequence $M_{pos}$ as a \textbf{coalition}.
% Our goal is to establish the mapping relationship between position and CMP flipping, that is, to analyze which positions on the seed $S$ can flip CMPs.
% The most intuitive idea is to define \textbf{gain} as whether the path exercised by the mutated input has changed relative to the seed $S$. If it changes, it means that mutated positions contribute to CMP flipping. Otherwise, it does not.

% But for a CMP, it is enough for us to extract only one combination of positions that can flip it on the seed $S$.
% Repeated extraction will only cause functional redundancy. That is, multiple extracted positions are related to the same CMP.
% Therefore, we finally define \textbf{gain} as: the number of new edges found by the mutated input relative to the seed $S$, that is, the number of \textbf{self-new edges}. Note that the \textbf{self-new edges} of the seed $S$ refer to the new edges discovered relative to the seed $S$ and its generated mutated inputs.
% Finally, we define the \textbf{characteristic function} $\mathcal{F}(*)$ as:
% Given a seed $S$ and target program $P$, the mapping between mutated position sequence and the number of self-new edges.


\subsection{Simplification of Shapley Calculation}\label{subsec:simp_shap}
\zhu{TODO: remove}
In Section~\ref{subsec:cg_all}, we formulate the byte mutation as a cooperative game and use Equation~(\ref{equ:shapely}) to quantify the importance of each byte. However, it is not practical for fuzzing to test all possible combinations (all possible inputs) for all seeds.
To improve the efficiency of fuzzing, we simplify the calculation of Shapley value by 1) gathering all mutations in the same family into the same cooperative game, 2) ignoring the generated inputs that do not discover self-new edges, and 3) reducing the combinations of bytes when self-new edges are discovered.


During fuzzing, all seeds will be selected and mutated. If we treat byte mutation in every seed as an individual cooperative game, it will have too much overhead.
In Section~\ref{subsec:cg_multiseed}, we conclude that seeds in the same family belong to the same cooperative game. Therefore, we gather the seeds belonging to the same family together, and mutations of all seeds in the family are used to calculate the Shapley values for the first seed in the family. 
The Shapley values for bytes of the first seed are shared with all other seeds in the same family.
% As a result, each cooperative game will obtain more combinations to calculate Shapley values, approximating to a more accurate result.


% As for the reduction of combinations, we achieve it based on the binary result of examining a path constraint, \ie an input either examines the \textit{then}-branch or the \textit{else}-branch of a path constraint.
% When self-new edges are discovered, the mutations may be performed directly on the original seed or on other seeds in the family. 




% \zhu{move to the next section?}
% During fuzzing, all seeds will be selected and mutated. If we treat byte mutation in every seed as an individual cooperative game, it will have too much overhead.
% In Section~\ref{subsec:cg_multiseed}, we conclude that seeds in the same family belong to the same cooperative game. Therefore, we gather the seeds belonging to the same family together, and mutations of all seeds in the family are used to calculate the Shapley values for the first seed in the family. As a result, each cooperative game will obtain more combinations to calculate Shapley values, approximating to a more accurate result.

Basically, we update Shapley values for bytes only when the mutation of a seed discovers self-new edges.
If a mutation does not discover self-new edges, then $\mathcal{F}(\ast) = 0$. In this case, we do not need to update the Shapley values. 
% As for the second solution of simplification, based on Equation~(\ref{equ:shapely}), if $\mathcal{F}(\ast) = 0$, we do not need to calculate the corresponding term in Shapley value. Therefore, if a generated input does not discover self-new edges ($\mathcal{F}(\ast) = 0$), we ignore its calculation for Shapley value. 
This will significantly reduce the overhead of calculating Shapley value since most mutations cannot discover self-new edges.


As for the reduction of combinations, we achieve it based on the binary result of testing a program, \ie an input either examines the \textit{then}-branch or the \textit{else}-branch of a path constraint. 




Based on this program logic, we simplify the calculation of Shapley value by reducing the players (bytes) in the cooperative game.
% Based on this property, we simplify the calculation of Shapley value in both a single seed and seeds in the same family. 
For a single seed, if a cooperative mutation discovers self-new edges, we remove the redundant bytes that do not influence the result of self-new edges. If fuzzing mutates bytes $M_{b} = \{b_1, b_2, ..., b_n\}$ to discover self-new edges, for a redundant byte $b_i$, $\mathcal{F}(M_b\backslash \{b_i\}) = \mathcal{F}(M_{b})$. This immediately derives that the related item in the Shapley value is zero. Therefore, we do not need to calculate the Shapley value for the redundant bytes. If $N_b$ is the set of bytes after removing mutations of all redundant bytes in $M_b$, exclusion of any byte $b_j$ in $N_b$ will not discover self-new edges, \ie $\mathcal{F}(N_b\backslash \{b_j\}) = 0$. According to Equation~(\ref{equ:shapely}), all bytes in the set $N_b$ have the same Shapley value  pertaining to the set $N_b$. Therefore, when self-new edges are discovered during fuzzing, we only need to calculate Shapley value for one byte in the set $N_b$.


To reduce players of a seed in a family, the  
% As for a family, we simplify the calculation of Shapley value by reducing the players (bytes) 

the cooperative game is played based on the original seed in the family (more details in Section~\ref{subsec:cg_multiseed}).
Consider the situation that seed $S_0$ is the original one, seed $S_1$ is obtained by mutating bytes $M_{0}$ in $S_0$, and seed $S_2$ is retained by mutating bytes $M_{1}$ in $S_1$. 


\zhu{A more complex situation is the inherit of seeds.}





% Most coverage-guided fuzzing has some initial seeds, and mutation of them may generate new seeds.
% If an input that is generated by mutating $S_0$ discovers new edges comparing to the overall discovered coverage, the input is retained as a new seed $S_1$. For the following fuzzing trials, the seed $S_1$ will be selected and mutated to generate new inputs. 
% This process of generating new inputs and testing them is actually the process of Shapley analysis. 





\zhu{TODO: describe fuzzing process (mutation on new seeds); simplify Shapley based on this process; no new edges==> no need to calculate Shapley; new edges: all mutations of seeds in the same family are the possible combinations.}


Suppose in a mutation of seed $S$, mutation position sequence $M_{pos} = \{p_{1}, \ldots, p_{n}\}$. There are a total of $N$ mutated positions. Based on the Equation~\ref{equ:shapely} of Shapley Value, the contribution $\phi_{j}$ of position $p_{j}$ to CMP flipping can be calculated as:
\begin{equation} \label{equ:shapelyFuzzing}
    \phi_{j}=\sum_{T \subseteq M_{pos} \backslash \{p_{j}\}} \frac{|T| !(N-|T|-1) !}{N !}(\mathcal{F}(T \cup \{p_{j}\})-\mathcal{F}(T))
\end{equation}

The contribution of position $p_{j}$ in the mutation $M$ is the weighted average of the marginal contribution of the position $p_{j}$ in all possible subsets of the mutation position sequence $M_{pos}$, which brings a time complexity of $2^{N}$.
If we quantify the contribution of each position to CMP flipping during the fuzzing process, the throughput will be severely reduced, which will affect the efficiency of fuzzing.
Therefore, we need to use program features to simplify the calculation Equation~\ref{equ:shapelyFuzzing}.

First of all, we found that there are often some redundant mutated positions in a mutation. Mutation of redundant positions does not affect the discovery of self-new edges.
Formally, given the mutation position sequence $M_{pos} = \{p_{1}, \ldots, p_{n}\}$. If position $p_{j}$ satisfies the formula ~\ref{equ:redundant}, it means that the mutation of position $p_{j}$ is redundant.
\begin{equation} \label{equ:redundant}
    \mathcal{F}(M_{pos}) = \mathcal{F}(M_{pos} \backslash \{p_{j}\})
\end{equation}
Therefore, the effect of $M_{pos} \backslash \{p_{j}\}$ is the same as $M_{pos}$.
Then, we can replace $M_{pos}$ with $M_{pos} \backslash \{p_{j}\}$ so that the number of positions we need to analyze is reduced.

Secondly, the flipping of CMPs in the program often depends on the simultaneous mutation of multiple positions, that is, the 0-N case.
Suppose a CMP flip depends on the simultaneous mutation of all positions in $M_{pos} = \{p_{1}, \ldots, p_{n}\}$. Therefore, any subset of $M_{pos}$ cannot flip this CMP, that is:
\begin{equation} \label{equ:necessary}
    \mathcal{F}(m) = 0, m \subset M_{pos}
\end{equation}

In this case, the Equation~\ref{equ:shapelyFuzzing} can be simplified to:
\begin{equation} \label{equ:shapelyFuzzing01}
    \phi_{j}= \frac{|M_{pos}| !(N-|M_{pos}|-1) !}{N !}(\mathcal{F}(M_{pos}))
\end{equation}
So, $\phi_{j}$ is no longer related to $j$.
Suppose we can determine that each position in a mutation is necessary. In that case, we can directly use the formula ~\ref{equ:shapelyFuzzing01} to calculate the Shapley Value of each position, so that we no longer need to analyze the execution of the $M_{pos}$ subset.

Based on the above two characteristics, we propose our simplified Shapley Value calculation algorithm. The specific process is shown in the algorithm~\ref{alg:shapley}.

\begin{algorithm}[h]
\footnotesize
\caption{Algorithm of Simplified Shapley Value Calculation}\label{alg:shapley}
\KwIn{
    A mutation $M$,the mutated position sequence $M_{pos} = \{p_{1}, \ldots, p_{n}\}$ and a function $\mathcal{F}(*)$ mapping between mutated position sequence and self-new edges.
    
}

$SV[n] = {0}$\; 
$totalEdges = \mathcal{F}(M_{pos})$\;
$flag = 1$\;
\For{$pos \in M_{pos}$}{
    \If{$\mathcal{F}(M_{pos} \backslash \{pos\}) == totalEdges$}{
        $M_{pos}.delete(pos)$\;
    }
    \lElseIf{$\mathcal{F}(M_{pos} \backslash \{pos\}) \neq 0$}{
        $flag = 0$
    }
}
\eIf{$flag$}{
    $averageSV = simplifiedShapleyAnalysis(M_{pos}, \mathcal{F})$\;
    \For{$i \in n$}{
        $SV[i] = averageSV$\;
    }
}
{
    \For{$i \in n$}{
        $SV[i] = shapleyAnalysis(M_{pos}, \mathcal{F})$\;
    }
}
\end{algorithm}

Based on the algorithm ~\ref{alg:shapley}, we can quantify the contribution of each position to CMP flipping in each mutation, that is, the Shapley Value.
First, given the mutated position sequence $M_{pos}$, we initialize the Shapley Value of each position in $M_{pos}$, and record the number of self-new edges $totalEdges$ found by $M_{pos}$ (lines 1-2).
Second, we cancel the mutation of each position one by one, and remove redundant positions to reduce the number of positions required for analysis (lines 4-6).
Third, we analyze whether the mutation conforms to the 0-N case.
Specifically, we analyze whether the discovery of self-new edges depends on the simultaneous mutation of all remaining positions. If other values other than 0 and $totalEdges$ are found when canceling the mutation of each position, it means that the 0-N case is not met (line 7).
Finally, in the 0-N case, we consider all remaining positions to contribute equally to the self-new edges. Therefore, we directly use Equation~\ref{equ:shapelyFuzzing01} to calculate the Shapley Value of each position without analyzing the results of each subset (lines 8-11).
If it does not meet the 0-1 situation, we will continue to use the formula ~\ref{equ:shapelyFuzzing} for detailed analysis (lines 12-14).

\subsubsection{Position Importance}
Since the mutation process for a seed includes several mutations, we can accumulate the Shapley Value of a position on all mutations to obtain position importance. Position importance is used to quantify the importance of a position on the seed in CMP flipping.
Formally, assume that during the mutation process on the seed $S$, $R$ is the set of mutations for which self-new edges are found. The position importance $\beta_{j}$ of position $p_{i}$ can be calculated as:
\begin{equation} \label{equ:totalContribution}
\beta_{j} = \sum_{r \in R} SV_{r,p_{i}}
\end{equation}
Among them, $SV_{r,p_{i}}$ represents the Shapley Value of $p_{i}$ in the mutation $r$.


% % \section{family system}
% \subsection{Cooperative Game Across Seeds}
% % \zhu{Title: 2.4 cooperative game across seeds}

% However, according to the formula~\ref{equ:totalContribution}, the calculation of position importance relies on a single seed having enough mutations.
% However, the energy distribution of seeds during fuzzing is inconsistent.
% Some seeds can only be mutated dozens of times, which cannot accurately calculate the position importance of each position on the seed.
% Suppose we can gather those seeds with the same position importance distribution into a family. In that case, these seeds can share the calculation process of position importance, that is, put the mutations of these seeds together to generate a shared position importance distribution.
% The same position importance distribution means that the same position on different seeds has the same position importance.
% Specifically, assuming that seeds $A$ and $B$ have the same position importance distribution, the mutation sets of seeds $A$ and $B$ are $M_{A}$ and $M_{B}$, respectively.
% Therefore, we can combine $M_{A}$ and $M_{B}$ to get a shared mutation set $M_{A, B}$.
% Finally, based on Equation~\ref{equ:totalContribution}, we can use $M_{A, B}$ to generate the shared position importance distribution of seeds $A$ and $B$.

% % \subsection{Why does the Family System matters}
% So, how to gather those seeds with the same position importance distribution into a family?
% We found that if there is an inheritance relationship between seeds and the length is consistent, the position importance of the same position on different seeds is consistent.
% Suppose there are seeds $A$ and $B$. If seed $B$ is mutated from seed $A$, then there is an inheritance relationship between seeds $A$ and $B$.
% Note that inheritance relationships are transitive.
% Suppose the seed $A$ is mutated to get $B$, and the seed $B$ is mutated to get $C$. Then, there is also an inheritance relationship between $A$ and $C$.
% We discuss why such seeds have the same position importance distribution in two cases.

% \textbf{The case of two seeds.}
% If there are seeds $A$ and $B$, the paths of $A$ and $B$ are inconsistent. The lengths of seeds $A$ and $B$ are the same.
% Assuming that $A$ can mutate the position $i$ to get $B$, then $B$ can also mutate the position $i$ to get A.
% Moreover, the CMPs flipped during the two conversions of $A \rightarrow B$ and $B \rightarrow A$ are the same.
% Therefore, we believe that "the contribution of the position $i$ to CMP flipping in $A$" and "the contribution of the position $i$ to CMP flipping in $B$" is consistent.

% \textbf{The case of multiple seeds.}
% If $A$ mutates position $i$ to get $B$, $B$ mutates position $j$ to get $C$. The lengths of the seeds $A$, $B$, and $C$ are the same.
% If we ignore the intermediate node $B$ and integrate two mutations, it becomes: $A$ mutates positions $i,j$ at the same time, and $C$ can be found. In the same way, $C$ can also find $A$ by mutating positions $i, j$ at the same time.
% Moreover, the CMPs flipped during the two conversions of $A \rightarrow C$ and $C \rightarrow A$ are the same.
% Therefore, we believe that "the contribution of position $i,j$ to CMP flipping in $A$" and "the contribution of position $i,j$ to CMP flipping in $C$" are consistent.


\subsection{Approximation of Shapley Calculation}
\zhu{Although we simplify the calculation of Shapley value, the result is still an approximation to the entire Shapley analysis. Therefore, the obtained Shapley values during fuzzing can only reflect the partial contributions of bytes. Future mutations may increase or decrease the Shapley value of a byte. Therefore, we use CMAB to balance the trade-off between using approximate Shapley values and trying more possible combinations?.}


\zhu{Shapley is a posterior solution; how to predict based on it? ;use CMAB to approximating?}

\section{Shapley-based Boosting}
\zhu{TODO: CMAB for shapley-based mutation and havoc mutation}

\subsection{Family Construct}
Therefore, if the seeds are inherited and have the same length, they share the same position importance distribution.
With this feature, we propose the family system.
More specifically, we group seeds with inheritance relationships and the same length into a family.
All seeds within each family share the same position importance distribution.
Therefore, we can combine all mutations of all seeds in the family to generate a shared position importance distribution.
Formally, assume that family $F$ contains M seeds, that is, $F = \{S_{1}, \ldots, S_{M}\}$. All seeds in this family have length $N$, and each seed $S_{i}$ has its own mutation set $M_{i}$.
Therefore, we merge the mutation sets $M_{all} = \{M_{i} | i \in [1,M]\}$ of all seeds, and generate a shared position importance distribution $D = \{\beta_{i} | i \in [1,N]\}$.
Among them, the position importance $\beta_{i}$ of the jth position $p_{j}$ can be calculated as:
\begin{equation} \label{equ:share}
\beta_{j} = \sum_{r \in M_{all}} V_{r,p_{i}}
\end{equation}
Among them, $V_{r,p_{i}}$ represents the Shapley Value of $p_{i}$ in mutation $r$.
In this way, even if some seeds are only mutated dozens of times, we can still calculate the position importance of each position for it.


The key of building a family is that the mutation does not change the length of original seeds. However, many fuzzers mutate seeds via changing the length of seeds, such as inserting positions and deleting positions. To enrich family members, \tool{} will withdraw all mutators that change length when new code are discovered.
If the result can still find the same new edges after withdrawing those mutators, \tool{} will retain the result to a family based on inheritance relationship and seed length.
if we select a seed from family $N$ and generate an 
For example, as shown in Figure~\ref{fig:family_update}, we select a seed from family $N$ and mutate it. 
If an input $i_1$ discovers new edges, \tool{} will withdraw all mutators that change length, which generates another input $i_2$. If $i_2$ can still find the same new edges that $i_1$ finds, \tool{} retains $i_2$ to the family $N$.
Otherwise, $i_1$ will form a new family $N+1$ if mutation of $i_1$ can further discover new edges.
As a result, \tool{} has a reasonable number of families and family members. 

\begin{figure}[t!]
\includegraphics[width=\linewidth]{images/upate.png}
\caption{The update of family and family members.}
\label{fig:family_update}
\end{figure}



\subsection{Mutation}\zkp{change the section name}
The Shapley Value analysis process is embedded in fuzzing. After a period of fuzzing, we obtained the position importance of some positions. Then, we can focus on mutating positions with higher position importance.
However, when can position importance be used to guide the direction of fuzzing?
To solve this problem, we divide fuzzing into two modes: Shapley analysis mode and Shapley-guided mutation mode.
Suppose we mutate a seed $S$.

In the Shapley analysis mode, we randomly select positions for mutation like the AFL strategy, and use the Shapley Value to analyze the contribution of each position during the mutation process, and finally get the position importance of each position.

In Shapley-guided mutation mode, we construct a set of positions whose position importance is greater than 0, representing the positions on the seed that contribute to CMP flipping. Then, we randomly select positions from among them for mutation.
If the position importance of a position is higher, it means it is more important. Then we should allocate more mutators to mutate the position and its surrounding positions.
Formally, in a mutation $M$ of the seed $S$, assuming that the position $p_{j}$ whose position importance is $\beta_{j}$ is to be mutated, then the number of mutators $Num $ allocated can be calculated as:

\begin{equation}
Num = 
\begin{cases}
\frac{5}{1+e^{\beta_{j}}} - 2.5& \beta_{j} > 0\\
0& \beta_{j} \leq 0
\end{cases}
\end{equation}
Since the scope of different mutators is different, if the position importance of a position is greater, the probability of its surrounding positions being mutated is also greater.

Further, Shapley analysis mode tends to mutate all positions to optimize position importance distribution of a seed, while B tends to use the existing position importance to guide the fuzzing direction.
We need to balance the two modes.
To switch mutation modes, \tool{} uses a simple yet effective indicator calculated as:

\begin{equation} \label{equ:cost}
c = \frac{N_{exec}}{N_{new\_paths}},
\end{equation}
where $N_{exec}$ is the number of executions, and $N_{new\_paths}$ is the number of new paths found in those executions. 


The result $c$ is the cost to discover one new path. Lower cost $c$ indicates higher efficiency of a mutation mode.
Both Shapley analysis mode and Shapley-guided mutation mode have their own costs $c$. When deciding the mode to perform, \tool{} compares the costs of the two modes, and selects the mode with lower cost.






==> obsolete/technique-3.3.tex <==
\section{Design of \tool} \label{sec:design}
\zhu{TODO: describe this section; }




\subsection{Shapley Analysis Among Bytes} \label{subsec:cg_all}

As mentioned, bytes in a seed are collaboratively mutated to discover new edges. Therefore, we formulate the process of byte mutation as a cooperative game and use Shapley value to quantify the contribution of each byte. We first formulate the mutation of one seed and then extend it to multiple seeds based on the characteristics of mutation. 


\zhu{TODO: a figure to show the formulation of byte mutation, and family}



\subsubsection{Shapley Value} \label{subsec:shapval}

The Shapley Value is a solution used in Cooperative Game Theory that fairly distributes gains among several players working in a coalition. 
A cooperative game is one that $N$ players form coalitions and obtain gains by a characteristic function.
Shapley Value can be used to quantify the contribution of each player in a game.
% Following Lloyd S. Shapley~\cite{Shapley},
In the Cooperative Game Theory,
the Shapley Value $\phi_{j}$ of the player $x_{j}$ to the coalition can be calculated as~\cite{Shapley}:
\begin{equation} \label{equ:shapely}
    \phi_{j}=\sum_{G \subseteq X \backslash \{x_{j}\}} \frac{|G| !(N-|G|-1) !}{N !}(\mathcal{F}(G \cup \{x_{j}\})-\mathcal{F}(G)),
\end{equation}
where there are $N$ players in the game, and a coalition $G$ is formed by $m (m \leq N)$ players.
$X$ is the set of all players and $X \backslash \{x_{j}\}$ is all possible coalitions of players excluding the player $x_{j}$. $|G|$ is the number of players in the set $G$.
$\mathcal{F}(\ast)$ is a characteristic function that describes the gain $R$ that the coalition of players can obtain, \ie $R = \mathcal{F}(G)$.
$\mathcal{F}(G \cup \{x_{j}\})-\mathcal{F}(G)$ is the marginal contribution of the player $x_{j}$ on the coalition $G$, which describes the effect on the gain of including the player $x_{j}$. In other words, the Shapley value $\phi_{j}$ is a weighted average of $x_{j}$'s marginal contributions across all possible player coalitions. 
In other words, the Shapley value reflects the importance of the player $x_j$ in the game.


Coverage-guided fuzzing usually has some initial seeds, and mutation of them may generate new seeds.
If an input that is generated by mutating a seed discovers new edges comparing to the overall discovered coverage, the input is retained as a new seed. For the following fuzzing trials, the new seed will be selected and mutated to generate new inputs. 
This process of generating new inputs and testing them can be regarded the process of Shapley analysis, \ie \textit{trying possible combinations of bytes}.
Yet, the problem is how to gather the trails in fuzzing so that these trails belong to the same Shapley analysis. 


% \zhu{remove this?}
% The Equation~(\ref{equ:shapely}) only calculates the Shapley value of the player $x_j$ in a single sample. In some scenarios, such as machine learning, different samples will be utilized to calculate Shapley values for the same player. To measure the importance of a player when multiple samples exist, studies accumulate the Shapley values of the player on all samples~\cite{SV1,SV2,SV3}. Specifically, assuming that $Y$ is the set containing all samples, the importance of the player $x_j$ is calculated as:
% \begin{equation} \label{equ:featureImportance}
%     \eta_{j}=\sum_{y \in Y}\phi_{y,j}
% \end{equation}


% Formulation of Byte Mutation
\subsubsection{Shapley Analysis in One Seed} \label{subsec:cg_oneseed}

For a seed, the \textbf{cooperative game} is the schedule of bytes on the seed, including the selection of some certain bytes and the mutation of the selected bytes. This game finds a total of $n$ edges and the Shapley value is utilized to analyze the contribution of each byte pertaining to the discovery of those $n$ edges. Thus, a \textbf{player} in the game is a byte in the seed $S_0$, and the \textbf{coalition} is that some certain bytes are mutated together. Since coverage-guided fuzzing aims to discover new code, we define the \textbf{gain} as the number of \textit{self-new edges} discovered by an input $i$ generated by mutating the seed $S_0$. 
To ensure that the gain is consistent during fuzzing, the \textit{self-new edges} are defined as the new edges when comparing the edges discovered by the input $i$ and the initial seed $S_0$. From the perspective of program logic, \textit{a byte related to more path constraints will have larger contribution to the code discovery}. Thus, the use of self-new edges can provide more information about the relations between input bytes and path constraints.
For most fuzzers, such as AFL-based fuzzers~\cite{aflchurn, Zhu2020CSI}, new edges are obtained by comparing to the overall coverage. However, this kind of new edges is ``stateful'' because the order of mutation can influence the result. As a result, depending on the time of mutation, the gain of the same mutation may be different. Therefore, we use self-new edges to avoid the variation of gain. Finally, the \textbf{characteristic function} $\mathcal{F}(*)$ is the mapping between the collaborative mutation and the number of self-new edges.
With the formulation of byte mutation, we can use Equation~(\ref{equ:shapely}) to calculate the Shapley value for each byte. Since the Shapley value reflects the importance of a byte pertaining to code discovery, we can improve the efficiency of fuzzing by \textit{assigning more energy to the bytes with higher Shapley values}.


\subsubsection{Shapley Analysis Across Seeds} \label{subsec:cg_multiseed}
Multiple seeds are possible to be treated as one seed from the perspective of Shapley analysis.
Although Section~\ref{subsec:cg_oneseed} formulate byte mutation based on one seed $S_0$, the process of calculating Shapley values will generate new seeds. 
% If a cooperative mutation in $S_0$ discovers new edges comparing to the overall discovered coverage, the generated input by this mutation is retained as a new seed $S_1$. 
If the mutation does not change the length of the original seed $S_0$, the new seed $S_1$ is actually one of the combinations in the Shapley analysis of seed $S_0$. If the length is changed, the relative positions of bytes are changed, as well as the number of players in the Shapley analysis. Therefore, without changing length, any mutation of seed $S_1$ still belongs to the Shapley analysis of seed $S_0$. For example, if seed $S_0$ is mutated byte $i$ to get seed $S_1$, and $S_1$ is mutated byte $j$ to get seed $S_2$. The lengths of the seeds $S_0$, $S_1$, and $S_2$ are the same.
Then, the seed $S_2$ can be obtained by mutating bytes $i,j$ in seed $S_0$.
% Therefore, if multiple seeds are generated from the same original seed and they have the same length, such seeds participate in the same cooperative game.
Therefore, the seeds, which are retained from the same original seed and do not change the length, are part of the combinations for the original seed.
We group such seeds (\eg seeds $S_0$, $S_1$ and $S_2$) into a \textit{family} so that seeds in the same family participate in the same cooperative game. 
To conclude, seeds in a family 1) inherit from the same original seed, 2) obtain the subset of players in Equation~(\ref{equ:shapely}) by comparing to the original seed, and 3) have the same length.


The family can release the overhead of Shapley analysis because it gathers different seeds into the same Shapley analysis.
During fuzzing, all seeds will be selected and mutated. If we treat byte mutation in every seed as an individual Shapley analysis, it will have too much overhead.
In Section~\ref{subsec:cg_multiseed}, we conclude that seeds in the same family belong to the same cooperative game. Therefore, we gather the seeds belonging to the same family together, and mutations of all seeds in the family are used to calculate the Shapley values for the first seed in the family. 
The Shapley values for bytes of the first seed are shared with all other seeds in the same family.


\subsection{Shapley Value Update}
In this section, we transform the calculation of Shapley value into a form that can be updated during fuzzing. We then reduce the overhead of calculating Shapley values based on properties of fuzzing. 
% As a result, the Shapley values can be utilized to guide byte mutation in fuzzing.



\subsubsection{Transformation of Shapley Value} \label{subsec:trans_shap}
Since a byte include both position (the order in an input) and value, all possible combinations of byte mutation include combinations of byte positions coupled with combinations of byte values.
In Equation~(\ref{equ:shapely}), when the subset $G$ of bytes is selected, the byte positions are fixed but the byte values have different combinations. Therefore, the gain of the subset $G$ comes from all the combinations of byte values. In fuzzing, a combination of byte values is an input generated by mutating the bytes of subset $G$. Therefore, the gain of subset $G$ is obtained by accumulating gains of all inputs belonging to $G$. Then, we have
\begin{equation} \label{equ:sum_value}
    \mathcal{F}(V) = \sum_{v\in V} \mathcal{F}(\{v\}),
\end{equation}
where $V$ is the set of all possible combinations of byte values in $G$, $v$ (an input) is a combination belonging to $V$, and $\{v\}$ is a set that only have one element $v$. 
With equations~(\ref{equ:shapely}) and (\ref{equ:sum_value}), let $k(G)=\frac{|G| !(N-|G|-1) !}{N !}$ and $P$ be the positions selected in $G$, then we have
\begin{equation} \label{equ:shapely_sum}
\begin{split}
\phi_{j} & = \sum_{G \subseteq X \backslash \{x_{j}\}} k(G) \bigl( \mathcal{F}(G \cup \{x_{j}\})-\mathcal{F}(G) \bigr) \\
         & = \sum_{P \subseteq X \backslash \{x_{j}\}} k(P) \Bigl( \sum_{v\in V} \mathcal{F}(\{v\}\cup\{x_j\}) - \sum_{v\in V} \mathcal{F}(\{v\}) \Bigr) \\
         & = \sum_{P \subseteq X \backslash \{x_{j}\}} k(P) \biggl( \sum_{v\in V} \Bigl( \mathcal{F}(\{v\}\cup\{x_j\}) - \mathcal{F}(\{v\}) \Bigr) \biggr) ,\\
         % & = \sum_{G \subseteq X \backslash \{x_{j}\}} \biggl( \sum_{v\in V} k(P)\Bigl( \mathcal{F}(\{v\}\cup\{x_j\}) - \mathcal{F}(\{v\}) \Bigr) \biggr) \\
         & = \sum_{P \subseteq X \backslash \{x_{j}\}} \sum_{v\in V} k(P)\Bigl( \mathcal{F}(\{v\}\cup\{x_j\}) - \mathcal{F}(\{v\}) \Bigr) \\
         & = \sum_{P \subseteq X \backslash \{x_{j}\}} \sum_{v\in V} \varphi_{j,v}
\end{split}
\end{equation}
where 
\begin{equation}\label{equ:shap_eta}
    \varphi_{j,v} = k(P)\Bigl( \mathcal{F}(\{v\}\cup\{x_j\}) - \mathcal{F}(\{v\}) \Bigr)
\end{equation}


Equation~(\ref{equ:shapely_sum}) indicates that the Shapley value of the byte $x_j$ can be accumulated by analyzing individual inputs. Specifically, each time an input $v$ discovers self-new edges, we can use $\varphi_{j,v}$ to calculate the local contribution of byte $x_j$ based on the input. Then, when more inputs are generated, we accumulate their $\varphi$ to update the Shapley value of byte $x_j$. 
Therefore, we can use Shapley value to guide fuzzing without changing the most fuzzing logic described in Section~\ref{subsec:shapval}. 
Notably, the contribution of a byte $x_j$ has the same meaning to the contribution of its position $j$ because positions are fixed when bytes have been selected.


\subsubsection{Shapley Update During Fuzzing}
As mentioned in Section~\ref{subsec:cg_multiseed}, Shapley values are calculated for the original seed in a family, which can significantly improve the efficiency of fuzzing. To further improve the efficiency of fuzzing, we update Shapley values by 1) ignoring the generated inputs that do not discover self-new edges, and 2) reducing the combinations of bytes when self-new edges are discovered.
If a mutation does not discover self-new edges, then $\mathcal{F}(\ast) = 0$. Therefore, the Shapley value remains the same and we do not need to update it.
If a cooperative mutation discovers self-new edges, we remove the redundant bytes that do not influence the result of self-new edges. If fuzzing mutates bytes $M_{b} = \{b_1, b_2, ..., b_n\}$ to discover self-new edges, for a redundant byte $b_i$, we get $\mathcal{F}(M_b\backslash \{b_i\}) = \mathcal{F}(M_{b})$. This immediately derives that the value of the related $\varphi$ is zero. Therefore, we do not need to update Shapley values for redundant bytes.
For the necessary bytes that influence the result of self-new edges, denoted as $N_b$, exclusion of any byte $b_j$ in $N_b$ will not discover self-new edges, \ie $\mathcal{F}(N_b\backslash \{b_j\}) = 0$. 
% This lies in the fact that an input either examines the \textit{then}-branch or the \textit{else}-branch of a path constraint. 
Therefore, all necessary bytes in this mutation have the same value of $\varphi$, indicating that we can only calculate $\varphi$ for one necessary byte to update Shapley values for all necessary bytes. 
In fuzzing, when self-new edges are discovered, we recover mutations of bytes to check whether those bytes are redundant.
If the recovery of the mutation of a byte does not change the result of self-new edges, the byte is a redundant byte.


\subsubsection{Family Update}
The family for seeds can reduce the overhead of calculating Shapley values because Shapley values for one seed can be shared with multiple seeds.  
The key of building a family is that the mutation does not change the length of original seeds. Yet, some mutators, such as \textit{deletion of bytes}, in fuzzing will change the length of seeds. 
To enrich family members, \tool{} will withdraw all mutators that change length when new code are discovered.
If the result can still find the same new edges after withdrawing those mutators, \tool{} will retain the result of withdrawing to the family.
For example, as shown in Figure~\ref{fig:family_update}, we select a seed from family $N$ and mutate it. 
If an input $i_1$ discovers new edges, \tool{} will withdraw all mutators that change length, which generates another input $i_2$. If $i_2$ can still find the same new edges that $i_1$ finds, \tool{} retains $i_2$ as a new seed and adds it to the family $N$.
Otherwise, $i_1$ will form a new family $N+1$ if mutation of $i_1$ can further discover new edges.
As a result, \tool{} has a reasonable number of families and family members.


\begin{figure}[t!]
\includegraphics[width=\linewidth]{images/upate.png}
\caption{\zhu{remove?} The update of family and family members.}
\label{fig:family_update}
\end{figure}


% % $\mathcal{F}(\ast) = 0$
% % From the perspective of Cooperative Game Theory, we understand the mutation process for a seed as a learning process to analyze the relationships between positions and code discovery.
% % The mutation process includes several mutations, and each mutation mainly has the following three steps: select mutated positions, generate the mutation input, and put it into the target program for execution.
% % Discovering all new edges in the target program essentially requires constantly flipping the CMPs in the program.
% % The flipping of CMPs has two cases: If we flip those CMPs with unexplored branches, we can directly discover new edges. Flipping those CMPs where all branches have been explored may also trigger other program logic to discover new edges deep in the program.
% % Thus, we believe that a position's efficiency is determined by its contributions to CMP flipping.
% % Since a mutation may mutate multiple positions simultaneously, the CMP flipping is the result of the coalition of positions.
% % Naturally, we can use Shapley Value to measure the contribution of each position in a mutation.

% % The mutation process for a seed involves several mutations to the seed.
% % Since Shapley Value analyzes an observation, we regard a mutation as an observation.
% % To apply Shapley Value to analyze each mutation, we need to redefine the concepts required by Shapley Value in fuzzing.

% % \subsubsection{Conceptual mapping between fuzzing and cooperative game}
% % In the mutation process for a seed $S$, assume there is a mutation $M$ and the mutation position sequence $M_{pos} = \{p_{1}, \ldots, p_{n}\}$.
% % In a mutation, we generate a mutated input for the seed $S$ based on the mutated position sequence, and put the mutated input into the target program to execute to get the feedback result.
% % We treat a mutation on seed $S$ as \textbf{a game}.
% % More specifically, we treat a position on the seed $S$ as a \textbf{player}, and the mutated position sequence $M_{pos}$ as a \textbf{coalition}.
% % Our goal is to establish the mapping relationship between position and CMP flipping, that is, to analyze which positions on the seed $S$ can flip CMPs.
% % The most intuitive idea is to define \textbf{gain} as whether the path exercised by the mutated input has changed relative to the seed $S$. If it changes, it means that mutated positions contribute to CMP flipping. Otherwise, it does not.

% % But for a CMP, it is enough for us to extract only one combination of positions that can flip it on the seed $S$.
% % Repeated extraction will only cause functional redundancy. That is, multiple extracted positions are related to the same CMP.
% % Therefore, we finally define \textbf{gain} as: the number of new edges found by the mutated input relative to the seed $S$, that is, the number of \textbf{self-new edges}. Note that the \textbf{self-new edges} of the seed $S$ refer to the new edges discovered relative to the seed $S$ and its generated mutated inputs.
% % Finally, we define the \textbf{characteristic function} $\mathcal{F}(*)$ as:
% % Given a seed $S$ and target program $P$, the mapping between mutated position sequence and the number of self-new edges.


% \subsection{Simplification of Shapley Calculation}\label{subsec:simp_shap}
% \zhu{TODO: remove}
% In Section~\ref{subsec:cg_all}, we formulate the byte mutation as a cooperative game and use Equation~(\ref{equ:shapely}) to quantify the importance of each byte. However, it is not practical for fuzzing to test all possible combinations (all possible inputs) for all seeds.
% To improve the efficiency of fuzzing, we simplify the calculation of Shapley value by 1) gathering all mutations in the same family into the same cooperative game, 2) ignoring the generated inputs that do not discover self-new edges, and 3) reducing the combinations of bytes when self-new edges are discovered.


% During fuzzing, all seeds will be selected and mutated. If we treat byte mutation in every seed as an individual cooperative game, it will have too much overhead.
% In Section~\ref{subsec:cg_multiseed}, we conclude that seeds in the same family belong to the same cooperative game. Therefore, we gather the seeds belonging to the same family together, and mutations of all seeds in the family are used to calculate the Shapley values for the first seed in the family. 
% The Shapley values for bytes of the first seed are shared with all other seeds in the same family.
% % As a result, each cooperative game will obtain more combinations to calculate Shapley values, approximating to a more accurate result.


% % As for the reduction of combinations, we achieve it based on the binary result of examining a path constraint, \ie an input either examines the \textit{then}-branch or the \textit{else}-branch of a path constraint.
% % When self-new edges are discovered, the mutations may be performed directly on the original seed or on other seeds in the family. 




% % \zhu{move to the next section?}
% % During fuzzing, all seeds will be selected and mutated. If we treat byte mutation in every seed as an individual cooperative game, it will have too much overhead.
% % In Section~\ref{subsec:cg_multiseed}, we conclude that seeds in the same family belong to the same cooperative game. Therefore, we gather the seeds belonging to the same family together, and mutations of all seeds in the family are used to calculate the Shapley values for the first seed in the family. As a result, each cooperative game will obtain more combinations to calculate Shapley values, approximating to a more accurate result.

% Basically, we update Shapley values for bytes only when the mutation of a seed discovers self-new edges.
% If a mutation does not discover self-new edges, then $\mathcal{F}(\ast) = 0$. In this case, we do not need to update the Shapley values. 
% % As for the second solution of simplification, based on Equation~(\ref{equ:shapely}), if $\mathcal{F}(\ast) = 0$, we do not need to calculate the corresponding term in Shapley value. Therefore, if a generated input does not discover self-new edges ($\mathcal{F}(\ast) = 0$), we ignore its calculation for Shapley value. 
% This will significantly reduce the overhead of calculating Shapley value since most mutations cannot discover self-new edges.


% As for the reduction of combinations, we achieve it based on the binary result of testing a program, \ie an input either examines the \textit{then}-branch or the \textit{else}-branch of a path constraint. 




% Based on this program logic, we simplify the calculation of Shapley value by reducing the players (bytes) in the cooperative game.
% % Based on this property, we simplify the calculation of Shapley value in both a single seed and seeds in the same family. 
% For a single seed, if a cooperative mutation discovers self-new edges, we remove the redundant bytes that do not influence the result of self-new edges. If fuzzing mutates bytes $M_{b} = \{b_1, b_2, ..., b_n\}$ to discover self-new edges, for a redundant byte $b_i$, $\mathcal{F}(M_b\backslash \{b_i\}) = \mathcal{F}(M_{b})$. This immediately derives that the related item in the Shapley value is zero. Therefore, we do not need to calculate the Shapley value for the redundant bytes. If $N_b$ is the set of bytes after removing mutations of all redundant bytes in $M_b$, exclusion of any byte $b_j$ in $N_b$ will not discover self-new edges, \ie $\mathcal{F}(N_b\backslash \{b_j\}) = 0$. According to Equation~(\ref{equ:shapely}), all bytes in the set $N_b$ have the same Shapley value  pertaining to the set $N_b$. Therefore, when self-new edges are discovered during fuzzing, we only need to calculate Shapley value for one byte in the set $N_b$.


% To reduce players of a seed in a family, the  
% % As for a family, we simplify the calculation of Shapley value by reducing the players (bytes) 

% the cooperative game is played based on the original seed in the family (more details in Section~\ref{subsec:cg_multiseed}).
% Consider the situation that seed $S_0$ is the original one, seed $S_1$ is obtained by mutating bytes $M_{0}$ in $S_0$, and seed $S_2$ is retained by mutating bytes $M_{1}$ in $S_1$. 


% \zhu{A more complex situation is the inherit of seeds.}





% % Most coverage-guided fuzzing has some initial seeds, and mutation of them may generate new seeds.
% % If an input that is generated by mutating $S_0$ discovers new edges comparing to the overall discovered coverage, the input is retained as a new seed $S_1$. For the following fuzzing trials, the seed $S_1$ will be selected and mutated to generate new inputs. 
% % This process of generating new inputs and testing them is actually the process of Shapley analysis. 





% \zhu{TODO: describe fuzzing process (mutation on new seeds); simplify Shapley based on this process; no new edges==> no need to calculate Shapley; new edges: all mutations of seeds in the same family are the possible combinations.}


% Suppose in a mutation of seed $S$, mutation position sequence $M_{pos} = \{p_{1}, \ldots, p_{n}\}$. There are a total of $N$ mutated positions. Based on the Equation~\ref{equ:shapely} of Shapley Value, the contribution $\phi_{j}$ of position $p_{j}$ to CMP flipping can be calculated as:
% \begin{equation} \label{equ:shapelyFuzzing}
%     \phi_{j}=\sum_{T \subseteq M_{pos} \backslash \{p_{j}\}} \frac{|T| !(N-|T|-1) !}{N !}(\mathcal{F}(T \cup \{p_{j}\})-\mathcal{F}(T))
% \end{equation}

% The contribution of position $p_{j}$ in the mutation $M$ is the weighted average of the marginal contribution of the position $p_{j}$ in all possible subsets of the mutation position sequence $M_{pos}$, which brings a time complexity of $2^{N}$.
% If we quantify the contribution of each position to CMP flipping during the fuzzing process, the throughput will be severely reduced, which will affect the efficiency of fuzzing.
% Therefore, we need to use program features to simplify the calculation Equation~\ref{equ:shapelyFuzzing}.

% First of all, we found that there are often some redundant mutated positions in a mutation. Mutation of redundant positions does not affect the discovery of self-new edges.
% Formally, given the mutation position sequence $M_{pos} = \{p_{1}, \ldots, p_{n}\}$. If position $p_{j}$ satisfies the formula ~\ref{equ:redundant}, it means that the mutation of position $p_{j}$ is redundant.
% \begin{equation} \label{equ:redundant}
%     \mathcal{F}(M_{pos}) = \mathcal{F}(M_{pos} \backslash \{p_{j}\})
% \end{equation}
% Therefore, the effect of $M_{pos} \backslash \{p_{j}\}$ is the same as $M_{pos}$.
% Then, we can replace $M_{pos}$ with $M_{pos} \backslash \{p_{j}\}$ so that the number of positions we need to analyze is reduced.

% Secondly, the flipping of CMPs in the program often depends on the simultaneous mutation of multiple positions, that is, the 0-N case.
% Suppose a CMP flip depends on the simultaneous mutation of all positions in $M_{pos} = \{p_{1}, \ldots, p_{n}\}$. Therefore, any subset of $M_{pos}$ cannot flip this CMP, that is:
% \begin{equation} \label{equ:necessary}
%     \mathcal{F}(m) = 0, m \subset M_{pos}
% \end{equation}

% In this case, the Equation~\ref{equ:shapelyFuzzing} can be simplified to:
% \begin{equation} \label{equ:shapelyFuzzing01}
%     \phi_{j}= \frac{|M_{pos}| !(N-|M_{pos}|-1) !}{N !}(\mathcal{F}(M_{pos}))
% \end{equation}
% So, $\phi_{j}$ is no longer related to $j$.
% Suppose we can determine that each position in a mutation is necessary. In that case, we can directly use the formula ~\ref{equ:shapelyFuzzing01} to calculate the Shapley Value of each position, so that we no longer need to analyze the execution of the $M_{pos}$ subset.


% \subsubsection{Position Importance}
% Since the mutation process for a seed includes several mutations, we can accumulate the Shapley Value of a position on all mutations to obtain position importance. Position importance is used to quantify the importance of a position on the seed in CMP flipping.
% Formally, assume that during the mutation process on the seed $S$, $R$ is the set of mutations for which self-new edges are found. The position importance $\beta_{j}$ of position $p_{i}$ can be calculated as:
% \begin{equation} \label{equ:totalContribution}
% \beta_{j} = \sum_{r \in R} SV_{r,p_{i}}
% \end{equation}
% Among them, $SV_{r,p_{i}}$ represents the Shapley Value of $p_{i}$ in the mutation $r$.


% % \section{family system}
% \subsection{Cooperative Game Across Seeds}
% % \zhu{Title: 2.4 cooperative game across seeds}

% However, according to the formula~\ref{equ:totalContribution}, the calculation of position importance relies on a single seed having enough mutations.
% However, the energy distribution of seeds during fuzzing is inconsistent.
% Some seeds can only be mutated dozens of times, which cannot accurately calculate the position importance of each position on the seed.
% Suppose we can gather those seeds with the same position importance distribution into a family. In that case, these seeds can share the calculation process of position importance, that is, put the mutations of these seeds together to generate a shared position importance distribution.
% The same position importance distribution means that the same position on different seeds has the same position importance.
% Specifically, assuming that seeds $A$ and $B$ have the same position importance distribution, the mutation sets of seeds $A$ and $B$ are $M_{A}$ and $M_{B}$, respectively.
% Therefore, we can combine $M_{A}$ and $M_{B}$ to get a shared mutation set $M_{A, B}$.
% Finally, based on Equation~\ref{equ:totalContribution}, we can use $M_{A, B}$ to generate the shared position importance distribution of seeds $A$ and $B$.

% % \subsection{Why does the Family System matters}
% So, how to gather those seeds with the same position importance distribution into a family?
% We found that if there is an inheritance relationship between seeds and the length is consistent, the position importance of the same position on different seeds is consistent.
% Suppose there are seeds $A$ and $B$. If seed $B$ is mutated from seed $A$, then there is an inheritance relationship between seeds $A$ and $B$.
% Note that inheritance relationships are transitive.
% Suppose the seed $A$ is mutated to get $B$, and the seed $B$ is mutated to get $C$. Then, there is also an inheritance relationship between $A$ and $C$.
% We discuss why such seeds have the same position importance distribution in two cases.

% \textbf{The case of two seeds.}
% If there are seeds $A$ and $B$, the paths of $A$ and $B$ are inconsistent. The lengths of seeds $A$ and $B$ are the same.
% Assuming that $A$ can mutate the position $i$ to get $B$, then $B$ can also mutate the position $i$ to get A.
% Moreover, the CMPs flipped during the two conversions of $A \rightarrow B$ and $B \rightarrow A$ are the same.
% Therefore, we believe that "the contribution of the position $i$ to CMP flipping in $A$" and "the contribution of the position $i$ to CMP flipping in $B$" is consistent.

% \textbf{The case of multiple seeds.}
% If $A$ mutates position $i$ to get $B$, $B$ mutates position $j$ to get $C$. The lengths of the seeds $A$, $B$, and $C$ are the same.
% If we ignore the intermediate node $B$ and integrate two mutations, it becomes: $A$ mutates positions $i,j$ at the same time, and $C$ can be found. In the same way, $C$ can also find $A$ by mutating positions $i, j$ at the same time.
% Moreover, the CMPs flipped during the two conversions of $A \rightarrow C$ and $C \rightarrow A$ are the same.
% Therefore, we believe that "the contribution of position $i,j$ to CMP flipping in $A$" and "the contribution of position $i,j$ to CMP flipping in $C$" are consistent.


% \subsection{Approximation of Shapley Calculation}
% \zhu{Although we simplify the calculation of Shapley value, the result is still an approximation to the entire Shapley analysis. Therefore, the obtained Shapley values during fuzzing can only reflect the partial contributions of bytes. Future mutations may increase or decrease the Shapley value of a byte. Therefore, we use CMAB to balance the trade-off between using approximate Shapley values and trying more possible combinations?.}


% \zhu{Shapley is a posterior solution; how to predict based on it? ;use CMAB to approximating?}

% \section{Shapley-based Boosting}
% \zhu{TODO: CMAB for shapley-based mutation and havoc mutation}

% \subsection{Family Construct}
% Therefore, if the seeds are inherited and have the same length, they share the same position importance distribution.
% With this feature, we propose the family system.
% More specifically, we group seeds with inheritance relationships and the same length into a family.
% All seeds within each family share the same position importance distribution.
% Therefore, we can combine all mutations of all seeds in the family to generate a shared position importance distribution.
% Formally, assume that family $F$ contains M seeds, that is, $F = \{S_{1}, \ldots, S_{M}\}$. All seeds in this family have length $N$, and each seed $S_{i}$ has its own mutation set $M_{i}$.
% Therefore, we merge the mutation sets $M_{all} = \{M_{i} | i \in [1,M]\}$ of all seeds, and generate a shared position importance distribution $D = \{\beta_{i} | i \in [1,N]\}$.
% Among them, the position importance $\beta_{i}$ of the jth position $p_{j}$ can be calculated as:
% \begin{equation} \label{equ:share}
% \beta_{j} = \sum_{r \in M_{all}} V_{r,p_{i}}
% \end{equation}
% Among them, $V_{r,p_{i}}$ represents the Shapley Value of $p_{i}$ in mutation $r$.
% In this way, even if some seeds are only mutated dozens of times, we can still calculate the position importance of each position for it.


% The key of building a family is that the mutation does not change the length of original seeds. However, many fuzzers mutate seeds via changing the length of seeds, such as inserting positions and deleting positions. To enrich family members, \tool{} will withdraw all mutators that change length when new code are discovered.
% If the result can still find the same new edges after withdrawing those mutators, \tool{} will retain the result to a family based on inheritance relationship and seed length.
% % if we select a seed from family $N$ and generate an 
% For example, as shown in Figure~\ref{fig:family_update}, we select a seed from family $N$ and mutate it. 
% If an input $i_1$ discovers new edges, \tool{} will withdraw all mutators that change length, which generates another input $i_2$. If $i_2$ can still find the same new edges that $i_1$ finds, \tool{} retains $i_2$ to the family $N$.
% Otherwise, $i_1$ will form a new family $N+1$ if mutation of $i_1$ can further discover new edges.
% As a result, \tool{} has a reasonable number of families and family members. 



% \subsection{Mutation}\zkp{change the section name}
% The Shapley Value analysis process is embedded in fuzzing. After a period of fuzzing, we obtained the position importance of some positions. Then, we can focus on mutating positions with higher position importance.
% However, when can position importance be used to guide the direction of fuzzing?
% To solve this problem, we divide fuzzing into two modes: Shapley analysis mode and Shapley-guided mutation mode.
% Suppose we mutate a seed $S$.

% In the Shapley analysis mode, we randomly select positions for mutation like the AFL strategy, and use the Shapley Value to analyze the contribution of each position during the mutation process, and finally get the position importance of each position.

% In Shapley-guided mutation mode, we construct a set of positions whose position importance is greater than 0, representing the positions on the seed that contribute to CMP flipping. Then, we randomly select positions from among them for mutation.
% If the position importance of a position is higher, it means it is more important. Then we should allocate more mutators to mutate the position and its surrounding positions.
% Formally, in a mutation $M$ of the seed $S$, assuming that the position $p_{j}$ whose position importance is $\beta_{j}$ is to be mutated, then the number of mutators $Num $ allocated can be calculated as:

% \begin{equation}
% Num = 
% \begin{cases}
% \frac{5}{1+e^{\beta_{j}}} - 2.5& \beta_{j} > 0\\
% 0& \beta_{j} \leq 0
% \end{cases}
% \end{equation}
% Since the scope of different mutators is different, if the position importance of a position is greater, the probability of its surrounding positions being mutated is also greater.

% Further, Shapley analysis mode tends to mutate all positions to optimize position importance distribution of a seed, while B tends to use the existing position importance to guide the fuzzing direction.
% We need to balance the two modes.
% To switch mutation modes, \tool{} uses a simple yet effective indicator calculated as:

% \begin{equation} \label{equ:cost}
% c = \frac{N_{exec}}{N_{new\_paths}},
% \end{equation}
% where $N_{exec}$ is the number of executions, and $N_{new\_paths}$ is the number of new paths found in those executions. 


% The result $c$ is the cost to discover one new path. Lower cost $c$ indicates higher efficiency of a mutation mode.
% Both Shapley analysis mode and Shapley-guided mutation mode have their own costs $c$. When deciding the mode to perform, \tool{} compares the costs of the two modes, and selects the mode with lower cost.


% \subsection{CMAB-Guided Mutation}
% \zhu{TODO: 1. explore more samples to update Shapley value; 2. assign more energy to bytes with higher Shapley values; 3. CMAB: contextual multi-armed bandit}

% (We maintain a shared pool in each family to record the position importance obtained by each position on all seeds in the family.)

% We know from motivation that a small number of positions contribute most of the new edges, and repeated mutations of positions can still discover new edges.
% Intuitively, we can select the position for each seed from the shared pool to mutate according to the position importance. The greater the position importance, the greater the probability of mutation.
% In this way, we are able to discover more new edges.

% However, we will encounter two problems in this process:
% 1) Question 1: position importance is knowledge obtained from historical data. It can only give a coarse-grained mutation direction, and we still need to adjust the weight of each position on different seeds in real-time.
% 2) Question 2: The position importance distribution of seed is continuously optimized during the fuzzing process, which relies on a large amount of mutation data. Therefore, we should allocate enough energy to all positions on the seed to be able to generate accurate position importance distribution.

% To solve these two problems, we propose CMAB-Guided Mutation.
% CMAB-Guided Mutation contains two modes: exploration mode and exploitation mode.

% \textbf{Exploitation Mode.}
% In the exploitation mode, we tend to select positions with larger position importance from the shared pool, and adjust the mutation probability of the positions in real-time according to the feedback.
% The easiest way is to model the problem of selecting positions as a multi-armed bandit (MAB) problem.
% Then, it is natural to regard an arm as a position in the shared pool and regard the reward as the number of new edges found.
% Then, due to the different paths of the seeds, the probability of finding new edges on different seeds at the same position is different.
% That is to say, on different seeds, the relationship between the same position and reward is different.
% Therefore, when we select a position from the shared pool, we also need to consider the path where the seed exercises.
% Therefore, we should model the problem of selecting positions as a contextual multi-armed bandit (CMAB) problem.
% Here, the user refers to the seed, and context refers to the path the seed exercises.
% LinUCB is a widely used lightweight algorithm in CMAB, which is suitable for use in the fuzzing process.
% LinUCB can recommend the arm that is more likely to get the highest reward for the user based on the user's context.
% Finally, given a seed and its context, we use LinUCB to score each position in the shared pool.
% To use the context to guide the position selection of the seed, each arm needs to maintain a dataset, which is used to record the context of the users who have selected the arm and the rewards obtained.

% Formally, given a seed $s$, its path is $x_{s}$. For position $p$ in the shared pool, its score in seed $s$ is calculated based on LinUCB\cite{linucb}:
% \begin{equation} \label{equ:Fitness_calculation}
% Score(s,p) = x_{s}^{T}(D_{p}^{T}D_{p} + I_{k})^{-1} D_{p}^{T} R_{p} + \alpha \sqrt{x_{s}^{T} (D_{p}^{T}D_{p} + I_{d})^{-1} x_{s}} + \phi_{p},
% \end{equation}
% where $(D_{p}, R_{p})$ is the dataset maintained by position $p$, where $D_{p}$ is a set of all context of seeds that position $p$ has encountered and $R_{p}$ is a set of corresponding rewards.
% $I_{k}$ is a k-dimensional identity matrix, and $k$ is the dimension of the feature vector.
% $\phi_{p}$ is the position importance of position $p$.

% After calculating the scores of all positions on the seed $s$,
% Finally, we generate a position selection possibility based on the scores of all positions on the seed $s$.
% Given a seed $s$, the probability $Poss_{s,p}$ of position p being selected is calculated as:
% \begin{equation} \label{equ:Fitness_calculation}
% Poss_{s,p} = \frac{Score(s,p)}{\sum_{h \in H} Score(s,h)}
% \end{equation}
% where $H$ is the set of all positions in the shared pool.

% \textbf{Exploration Mode.}
% In exploration mode, we assign the same mutation probability to all positions, so that we can get a more accurate position importance distribution (solve problem 2).

% Finally, during the fuzzing process, the two modes are constantly switched based on their respective efficiency. More specifically, we use a simple yet effective indicator calculated as:
% \begin{equation} \label{equ:cost}
% c = \frac{N_{exec}}{N_{new\_paths}},
% \end{equation}
% where $N_{exec}$ is the number of executions, and $N_{new\_paths}$ is the number of new paths found in those executions. 

% The result $c$ is the cost to discover one new path. Lower cost $c$ indicates higher efficiency of a mutation mode.
% Both exploration mode and exploitation mode have their own costs $c$. When deciding the mode to perform, \tool{} compares the costs of the two modes, and selects the mode with lower cost.


\subsection{Mutation with Contextual Multi-armed Bandit}
As mentioned in Section~\ref{subsec:trans_shap}, the importance of a byte is the same to the importance of its position for seeds. 
% Thus, in the following, we mostly use \textit{position importance} to represent the contribution of a byte, \ie its Shapley value.
Thus, in the following, we interchangeably use the terms of \textit{position importance}, \textit{byte importance}, and Shapley value.
The insight from Section~\ref{sec:motivation} indicates that more energy can be assigned to bytes with higher position importance. However, since the Shapley value is calculated based on part of all possible inputs during fuzzing, it cannot guarantee that the bytes with high Shapley values can always maintain high.
Besides, seeds share the position importance with the original seed in the same family.   
Although a position may have a high Shapley value, the difficulty of solving path constraints varies in different execution paths.
Intuitively, when mutation of some bytes cannot discover new code, we do not want to waste more energy on those bytes.
Therefore, we need to balance the trade-off between 1) guiding fuzzing based on Shapley values and 2) updating Shapley values for all bytes. 


To optimize the position selection so that fuzzing maximizes code discovery, \tool{} models the problem of selecting positions as a Contextual Multi-armed Bandit (CMAB) problem. Based on the experience of playing arms, CMAB tries to maximize the rewards of playing multi-armed bandits, taking into account the personality of a player (\ie the context). The trade-off in CMAB is between 1) focusing on the arms with higher historical performance and 2) updating rewards for all arms. This exactly fits into our problem of selecting byte positions.


Based on CMAB, \tool{} builds a probability distribution for selecting positions, and it prefers the positions that are more likely to discover new code. To build the probability distribution, CMAB first calculate scores to each position. Given a seed $s$, the feature vector $f_{s}$ extracted from the corresponding execution path (\ie the context), and a position $p$, the score of the position is calculated as:
\begin{equation} \label{equ:score_cal}
Score(s,p) = E[r_{s,p}|f_{s}] + 0.5 U_{s,p},
\end{equation}
where $E[r_{s,p}|f_{s}]$ is the expected reward and $U_{s,p}$ is the upper confidence bound. \zhu{$r_{s,p}$?}


% For Equation~(\ref{equ:score_cal}), the more a position is selected, the smaller its $U_{s,p}$ is.





\zhu{TODO}
% \zhu{TODO: \begin{itemize}
%     % \item As mentioned in Section~\ref{subsec:trans_shap}, the importance of a byte is the same to the importance of its position for seeds. In the following, ... 
%     % \item The information of position importance is shared by seeds in the same family.
%     % \item Seeds in the same family share the importance (Shapley value) of positions.
%     \item (However, due to the different paths of the seeds, the difficulty of finding new edges on different seeds at the same position is different.) Although a position may have high a Shapley value, the difficulty of solving path constraints varies in different seeds. When mutation of some bytes cannot discover new code, we do not want to waste more energy on those bytes. ==> need adjustment; need context of seeds
%     % \item The insight from Section~\ref{sec:motivation} is that more energy can be assigned to positions with higher Shapley values. (However, we cannot guarantee that positions with higher Shapley values can always discover more new code.) However, since the Shapley value is calculated based on part of all possible inputs, it cannot guarantee that the bytes with high Shapley values can always maintain high. 
%     % Therefore, we need to balance the trade-off between guiding fuzzing based on Shapley values and updating Shapley values for all bytes. 
% \end{itemize}}
% \zhu{TODO: 1. explore more samples to update Shapley value; 2. assign more energy to bytes with higher Shapley values; 3. CMAB: contextual multi-armed bandit}


% The position importance of each position recorded in the shared pool is knowledge obtained from historical data.
% It can only give a coarse-grained mutation direction.
% However, due to the different paths of the seeds, the difficulty of finding new edges on different seeds at the same position is different.
% Therefore, we still need to adjust the weight of each position on different seeds in real time according to the feedback.
% At the same time, the position importance distribution in the shared pool is continuously optimized during the fuzzing process, which relies on a large amount of mutation data. Therefore, we should assign enough energy to all positions for mutation to generate accurate position importance distribution.
% To optimize the position selection so that they can maximize code discovery, \tool{} models the problem of selecting positions as a contextual multi-armed bandit (CMAB) problem. Based on the experience of playing some arms, the CMAB tries to maximize the rewards of playing multi-armed bandits, taking into account the personality of a player (\ie the context).
% % The CMAB problem is the trade-off between playing more arms and focusing on some specific arms, \ie the problem of \textit{exploration vs. exploitation}.
% The CMAB problem is the trade-off between selecting arm with the best historical performance and selecting arm with fewer mutations.
% Meanwhile, the maximization of the reward reflects the search of the most contributing byte positions.
% Each byte position in a shared pool is an arm, and the seed that selects positions is the player. 
% The context for the CMAB problem is the execution path that the current seed exercises. 
% Therefore, the CMAB for byte mutation is to balance between exploring more positions and exploiting the best positions. 
% Based on CMAB, \tool{} builds a probability distribution for selecting positions, and it prefers the positions that are more likely to discover new code.

To introduce context into position selection, we need to build a relationship between context and reward, which relies on the history data. Thus, each arm needs to maintain a dataset $(\mathcal{D}, \mathcal{R})$, where $\mathcal{D}$ is a set of all history feature vectors and $\mathcal{R}$ is a set of corresponding rewards.
To achieve balance between exploitation and exploration, the scores calculated by \tool{} includes the expected reward and the upper confidence bound.

\textit{Expected Reward.} To avoid affecting throughput, we assume a linear relationship between the reward and the feature vector to save computational time. 
Given a seed $s$, the feature vector $f_{s}$ extracted from the corresponding execution path (\ie the context), and a position $p$ recorded in a shared pool, the expected reward $E[r_{s,p}|f_{s}]$ can be calculated by:

\begin{equation} \label{equ:E_calculation}
E[r_{s,p}|f_{s}] = f_{s}^{T}\hat{\theta} + \phi_{p}, %A_{p}^{-1}b_{p}
\end{equation}
where $\hat{\theta}$ is the best coefficient vector. 
Applying ridge regression to the dataset $(\mathcal{D}, \mathcal{R})$,
$\hat{\theta}$ can be estimated by:
\begin{equation} 
\hat{\theta} = (D_{p}^{T}D_{p} + I_{k})^{-1} D_{p}^{T} R_{p},
\end{equation}
where $(D_{p}, R_{p})$ is the dataset maintained by position $p$, $I_{k}$ is a k-dimensional identity matrix, and $k$ is the dimension of the feature vector.

\textit{Upper Confidence Bound.}
The second part of a score is the upper confidence bound $U_{s,p}$, which is calculated based on~\cite{walsh2009exploring}:
\begin{equation} \label{equ:U_calculation}
U_{s,p} = \sqrt{f_{s}^{T} (D_{p}^{T}D_{p} + I_{d})^{-1} f_{s}}
\end{equation}

Then, the score of each position $Score(s,p)$ is defined as:
\begin{equation} \label{equ:Fitness_calculation}
Score(s,p) = E[r_{s,p}|f_{s}] + \alpha U_{s,p},
\end{equation}
where $\alpha$ is a hyper-parameter for users to set and $\phi_{p}$ is the position importance of position $p$.
Based on our experience, we set $\alpha = 0.5$ in our experiments.
For Equation~(\ref{equ:Fitness_calculation}), the more a position is selected, the smaller its $U_{s,p}$ is. Therefore, \tool{} achieves the trade-off between exploration and exploitation.
Note that, as soon as the position importance in the shared pool is updated, we empty the dataset maintained on each arm and re-collect the data.


\subsection{Overall Algorithm}
\zhu{TODO: change the algorithm}
Based on the above two characteristics, we propose our simplified Shapley Value calculation algorithm. The specific process is shown in the algorithm~\ref{alg:shapley}.

\begin{algorithm}[h]
\footnotesize
\caption{Algorithm of Shapley-guided Fuzzing}\label{alg:shapley}
\KwIn{
    A mutation $M$,the mutated position sequence $M_{pos} = \{p_{1}, \ldots, p_{n}\}$ and a function $\mathcal{F}(*)$ mapping between mutated position sequence and self-new edges.
    
}

$SV[n] = {0}$\; 
$totalEdges = \mathcal{F}(M_{pos})$\;
$flag = 1$\;
\For{$pos \in M_{pos}$}{
    \If{$\mathcal{F}(M_{pos} \backslash \{pos\}) == totalEdges$}{
        $M_{pos}.delete(pos)$\;
    }
    \lElseIf{$\mathcal{F}(M_{pos} \backslash \{pos\}) \neq 0$}{
        $flag = 0$
    }
}
\eIf{$flag$}{
    $averageSV = simplifiedShapleyAnalysis(M_{pos}, \mathcal{F})$\;
    \For{$i \in n$}{
        $SV[i] = averageSV$\;
    }
}
{
    \For{$i \in n$}{
        $SV[i] = shapleyAnalysis(M_{pos}, \mathcal{F})$\;
    }
}
\end{algorithm}


Based on the algorithm ~\ref{alg:shapley}, we can quantify the contribution of each position to CMP flipping in each mutation, that is, the Shapley Value.
First, given the mutated position sequence $M_{pos}$, we initialize the Shapley Value of each position in $M_{pos}$, and record the number of self-new edges $totalEdges$ found by $M_{pos}$ (lines 1-2).
Second, we cancel the mutation of each position one by one, and remove redundant positions to reduce the number of positions required for analysis (lines 4-6).
Third, we analyze whether the mutation conforms to the 0-N case.
Specifically, we analyze whether the discovery of self-new edges depends on the simultaneous mutation of all remaining positions. If other values other than 0 and $totalEdges$ are found when canceling the mutation of each position, it means that the 0-N case is not met (line 7).
Finally, in the 0-N case, we consider all remaining positions to contribute equally to the self-new edges. Therefore, we directly use Equation~\ref{equ:shapelyFuzzing01} to calculate the Shapley Value of each position without analyzing the results of each subset (lines 8-11).
If it does not meet the 0-1 situation, we will continue to use the formula ~\ref{equ:shapelyFuzzing} for detailed analysis (lines 12-14).



\subsection{Threats to Validity}
\zhu{TODO}

Our \tool{} is proposed based on the results of SHAP analysis, which is an empirical method. Thus, we were concerned about the generality of our claims due to the small number of samples. 
However, we analyzed the root causes of the SHAP results to support our claims.  
These root causes, direct and indirect coupling of path constraints, are general observations of the nature of programs and independent from our empirical study.
Even if our claim does not include all programs, we believe it satisfies the majority of modern programs.


The second concern comes from the internal threat to validity, which is our solution to optimize byte selection. 
Our solution is based on two assumptions. The first is that there are valuable positions for us to optimize. The second is that our family system can capture the structural information of target programs. 
For the first assumption, we use the random mutation mode to obtain valuable positions.
However, random mutations can only increase the number of valuable positions up to a limit.
To solve this problem, we can use existing solutions that find constraint-related byte positions, such as GreyOne~\cite{greyone}, Angora~\cite{angora} and Driller~\cite{driller}. These solutions are efficient in finding positions related to a single path constraint, which is exactly what we want.
For the second assumption, it is mainly used to share valuable positions among different seeds. This requires that valuable positions in different seeds are still related to path constraints.
However, the family system can only roughly satisfy this requirement. 
One solution to solve this is to analyze programs case by case. That is, we capture the structural information based on syntax analysis tools or even manually determine the constraint-related positions in different seeds.
Yet, we believe such a solution limits the scalability of fuzzing, \ie it is only effective in specific programs.
Although the family system cannot accurately capture structural information, CMAB refines the selection of valuable positions, which is scalable to fuzz programs.


==> obsolete/technique-3.4.tex <==
\section{Design of \tool} \label{sec:design}
% \zhu{TODO: describe the figure \ref{Framework} of framework; }

Our \tool{} focuses on the byte mutation and seeks out important byte positions.
We understand the byte mutation across multiple seeds as a process of Shapley analysis and use Shapley value to quantify the contribution of each byte.
Figure~\ref{Framework} shows the framework of our \tool{}, which uses Shapley values of bytes to boost fuzzing efficiency.
We treat the schedule of bytes on the seed as the cooperative game and calculate the Shapley value for each byte.
To release the overhead of Shapley analysis, we deduce that the seeds, which are retained from the same original seed and do not change the length, belong to the same cooperative game and share the same Shapley values for bytes.
Thus, we group such seeds into a family to calculate the shared Shapley values in the family.


% Motivated by Section~\ref{sec:motivation}, assigning more energy to the bytes with higher Shapley values can discover more new edges. 
Fuzzing efficiency can be improved by assigning more energy to the bytes with higher Shapley values. 
However, we need to mutate all bytes and generate all possible inputs to get an accurate Shapley Value during fuzzing.
To achieve the trade-off between focusing on bytes with higher Shapley values and updating Shapley values for all bytes, \tool{} uses CMAB to build a probability distribution for optimizing this trade-off.


\subsection{Shapley Analysis Among Bytes} \label{subsec:cg_all}

As mentioned, bytes in a seed are collaboratively mutated to discover new edges. Therefore, we formulate the process of byte mutation as a cooperative game and use Shapley value to quantify the contribution of each byte. We first formulate the mutation of one seed and then extend it to multiple seeds based on the characteristics of mutation. 


% \zhu{TODO: a figure to show the formulation of byte mutation, and family}



\subsubsection{Shapley Value} \label{subsec:shapval}

The Shapley Value is a solution used in Cooperative Game Theory that fairly distributes gains among several players working in a coalition. 
A cooperative game is one that $N$ players form coalitions and obtain gains by a characteristic function.
Shapley Value can be used to quantify the contribution of each player in a game.
% Following Lloyd S. Shapley~\cite{Shapley},
In the Cooperative Game Theory,
the Shapley Value $\phi_{j}$ of the player $x_{j}$ to the coalition can be calculated as~\cite{Shapley}:
\begin{equation} \label{equ:shapely}
    \phi_{j}=\sum_{G \subseteq X \backslash \{x_{j}\}} \frac{|G| !(N-|G|-1) !}{N !}(\mathcal{F}(G \cup \{x_{j}\})-\mathcal{F}(G)),
\end{equation}
where there are $N$ players in the game, and a coalition $G$ is formed by $m (m \leq N)$ players.
$X$ is the set of all players and $X \backslash \{x_{j}\}$ is all possible coalitions of players excluding the player $x_{j}$. $|G|$ is the number of players in the set $G$.
$\mathcal{F}(\ast)$ is a characteristic function that describes the gain $R$ that the coalition of players can obtain, \ie $R = \mathcal{F}(G)$.
$\mathcal{F}(G \cup \{x_{j}\})-\mathcal{F}(G)$ is the marginal contribution of the player $x_{j}$ on the coalition $G$, which describes the effect on the gain of including the player $x_{j}$. In other words, the Shapley value $\phi_{j}$ is a weighted average of $x_{j}$'s marginal contributions across all possible player coalitions. 
In other words, the Shapley value reflects the importance of the player $x_j$ in the game.


Coverage-guided fuzzing usually has some initial seeds, and mutation of them may generate new seeds.
If an input that is generated by mutating a seed discovers new edges comparing to the overall discovered coverage, the input is retained as a new seed. For the following fuzzing trials, the new seed will be selected and mutated to generate new inputs. 
This process of generating new inputs and testing them can be regarded the process of Shapley analysis, \ie \textit{trying possible combinations of bytes}.
Yet, the problem is how to gather the trails in fuzzing so that these trails belong to the same Shapley analysis. 


% \zhu{remove this?}
% The Equation~(\ref{equ:shapely}) only calculates the Shapley value of the player $x_j$ in a single sample. In some scenarios, such as machine learning, different samples will be utilized to calculate Shapley values for the same player. To measure the importance of a player when multiple samples exist, studies accumulate the Shapley values of the player on all samples~\cite{SV1,SV2,SV3}. Specifically, assuming that $Y$ is the set containing all samples, the importance of the player $x_j$ is calculated as:
% \begin{equation} \label{equ:featureImportance}
%     \eta_{j}=\sum_{y \in Y}\phi_{y,j}
% \end{equation}



\begin{figure*}[t!]
\includegraphics[width=\linewidth]{images/framework.png}
\caption{The Framework of \tool{}. Based on the SHAP analysis, \tool{} organizes seeds via the family system. To maximize the code discovery, CMAB is utilized to optimize Shapley-guided byte mutation.
}
\label{Framework}
\end{figure*}


% Formulation of Byte Mutation
\subsubsection{Shapley Analysis in One Seed} \label{subsec:cg_oneseed}

For a seed, the \textbf{cooperative game} is the schedule of bytes on the seed, including the selection of some certain bytes and the mutation of the selected bytes. This game finds a total of $n$ edges and the Shapley value is utilized to analyze the contribution of each byte pertaining to the discovery of those $n$ edges. Thus, a \textbf{player} in the game is a byte in the seed $S_0$, and the \textbf{coalition} is that some certain bytes are mutated together. Since coverage-guided fuzzing aims to discover new code, we define the \textbf{gain} as the number of \textit{self-new edges} discovered by an input $i$ generated by mutating the seed $S_0$. 
To ensure that the gain is consistent during fuzzing, the \textit{self-new edges} are defined as the new edges when comparing the edges discovered by the input $i$ and the initial seed $S_0$. From the perspective of program logic, \textit{a byte related to more path constraints will have larger contribution to the code discovery}. Thus, the use of self-new edges can provide more information about the relations between input bytes and path constraints.
For most fuzzers, such as AFL-based fuzzers~\cite{aflchurn, Zhu2020CSI}, new edges are obtained by comparing to the overall coverage. However, this kind of new edges is ``stateful'' because the order of mutation can influence the result. As a result, depending on the time of mutation, the gain of the same mutation may be different. Therefore, we use self-new edges to avoid the variation of gain. Finally, the \textbf{characteristic function} $\mathcal{F}(*)$ is the mapping between the collaborative mutation and the number of self-new edges.
With the formulation of byte mutation, we can use Equation~(\ref{equ:shapely}) to calculate the Shapley value for each byte. Since the Shapley value reflects the importance of a byte pertaining to code discovery, we can improve the efficiency of fuzzing by \textit{assigning more energy to the bytes with higher Shapley values}.


\subsubsection{Shapley Analysis Across Seeds} \label{subsec:cg_multiseed}
Multiple seeds are possible to be treated as one seed from the perspective of Shapley analysis.
Although Section~\ref{subsec:cg_oneseed} formulate byte mutation based on one seed $S_0$, the process of calculating Shapley values will generate new seeds. 
% If a cooperative mutation in $S_0$ discovers new edges comparing to the overall discovered coverage, the generated input by this mutation is retained as a new seed $S_1$. 
If the mutation does not change the length of the original seed $S_0$, the new seed $S_1$ is actually one of the combinations in the Shapley analysis of seed $S_0$. If the length is changed, the relative positions of bytes are changed, as well as the number of players in the Shapley analysis. Therefore, without changing length, any mutation of seed $S_1$ still belongs to the Shapley analysis of seed $S_0$. For example, if seed $S_0$ is mutated byte $i$ to get seed $S_1$, and $S_1$ is mutated byte $j$ to get seed $S_2$. The lengths of the seeds $S_0$, $S_1$, and $S_2$ are the same.
Then, the seed $S_2$ can be obtained by mutating bytes $i,j$ in seed $S_0$.
% Therefore, if multiple seeds are generated from the same original seed and they have the same length, such seeds participate in the same cooperative game.
Therefore, the seeds, which are retained from the same original seed and do not change the length, are part of the combinations for the original seed.
We group such seeds (\eg seeds $S_0$, $S_1$ and $S_2$) into a \textit{family} so that seeds in the same family participate in the same cooperative game. 
To conclude, seeds in a family 1) inherit from the same original seed, 2) obtain the subset of players in Equation~(\ref{equ:shapely}) by comparing to the original seed, and 3) have the same length.


The family can release the overhead of Shapley analysis because it gathers different seeds into the same Shapley analysis.
During fuzzing, all seeds will be selected and mutated. If we treat byte mutation in every seed as an individual Shapley analysis, it will have too much overhead.
In Section~\ref{subsec:cg_multiseed}, we conclude that seeds in the same family belong to the same cooperative game. Therefore, we gather the seeds belonging to the same family together, and mutations of all seeds in the family are used to calculate the Shapley values for the first seed in the family. 
The Shapley values for bytes of the first seed are shared with all other seeds in the same family.


\subsection{Shapley Value Update}
In this section, we transform the calculation of Shapley value into a form that can be updated during fuzzing. We then reduce the overhead of calculating Shapley values based on properties of fuzzing. 
% As a result, the Shapley values can be utilized to guide byte mutation in fuzzing.



\subsubsection{Transformation of Shapley Value} \label{subsec:trans_shap}
Since a byte include both position (the order in an input) and value, all possible combinations of byte mutation include combinations of byte positions coupled with combinations of byte values.
In Equation~(\ref{equ:shapely}), when the subset $G$ of bytes is selected, the byte positions are fixed but the byte values have different combinations. Therefore, the gain of the subset $G$ comes from all the combinations of byte values. In fuzzing, a combination of byte values is an input generated by mutating the selected positions of $G$. Moreover, the gain of subset $G$ is obtained by accumulating gains of all inputs belonging to $G$. Then, we have
\begin{equation} \label{equ:sum_value}
    \mathcal{F}(V) = \sum_{v\in V} \mathcal{F}(\{v\}),
\end{equation}
where $V$ is the set of all possible combinations of byte values in $G$, $v$ (an input) is a combination belonging to $V$, and $\{v\}$ is a set that only have one element $v$. 
With equations~(\ref{equ:shapely}) and (\ref{equ:sum_value}), let $k(G)=\frac{|G| !(N-|G|-1) !}{N !}$ and $P$ be the positions selected in $G$, then we have
\begin{equation} \label{equ:shapely_sum}
\begin{split}
\phi_{j} & = \sum_{G \subseteq X \backslash \{x_{j}\}} k(G) \bigl( \mathcal{F}(G \cup \{x_{j}\})-\mathcal{F}(G) \bigr) \\
         & = \sum_{P \subseteq X \backslash \{x_{j}\}} k(P) \Bigl( \sum_{v\in V} \mathcal{F}(\{v\}\cup\{x_j\}) - \sum_{v\in V} \mathcal{F}(\{v\}) \Bigr) \\
         & = \sum_{P \subseteq X \backslash \{x_{j}\}} k(P) \biggl( \sum_{v\in V} \Bigl( \mathcal{F}(\{v\}\cup\{x_j\}) - \mathcal{F}(\{v\}) \Bigr) \biggr) ,\\
         % & = \sum_{G \subseteq X \backslash \{x_{j}\}} \biggl( \sum_{v\in V} k(P)\Bigl( \mathcal{F}(\{v\}\cup\{x_j\}) - \mathcal{F}(\{v\}) \Bigr) \biggr) \\
         & = \sum_{P \subseteq X \backslash \{x_{j}\}} \sum_{v\in V} k(P)\Bigl( \mathcal{F}(\{v\}\cup\{x_j\}) - \mathcal{F}(\{v\}) \Bigr) \\
         & = \sum_{P \subseteq X \backslash \{x_{j}\}} \sum_{v\in V} \varphi_{j,v}
\end{split}
\end{equation}
where 
\begin{equation}\label{equ:shap_eta}
    \varphi_{j,v} = k(P)\Bigl( \mathcal{F}(\{v\}\cup\{x_j\}) - \mathcal{F}(\{v\}) \Bigr)
\end{equation}


Equation~(\ref{equ:shapely_sum}) indicates that the Shapley value of the byte $x_j$ can be accumulated by analyzing individual inputs. Specifically, each time an input $v$ discovers self-new edges, we can use $\varphi_{j,v}$ to calculate the local contribution of byte $x_j$ based on the input. Then, when more inputs are generated, we accumulate their $\varphi$ to update the Shapley value of byte $x_j$. 
Therefore, we can use Shapley value to guide fuzzing without changing the most fuzzing logic described in Section~\ref{subsec:shapval}. 
Notably, the contribution of a byte $x_j$ has the same meaning to the contribution of its position $j$ because positions are fixed when bytes have been selected.


\subsubsection{Shapley Update During Fuzzing}
As mentioned in Section~\ref{subsec:cg_multiseed}, Shapley values are calculated for the original seed in a family, which can significantly improve the efficiency of fuzzing. To further improve the efficiency of fuzzing, we update Shapley values by 1) ignoring the generated inputs that do not discover self-new edges, and 2) reducing the combinations of bytes when self-new edges are discovered.
If a mutation does not discover self-new edges, then $\mathcal{F}(\ast) = 0$. Therefore, the Shapley value remains the same and we do not need to update it.
If a cooperative mutation discovers self-new edges, we remove the redundant bytes that do not influence the result of self-new edges. If fuzzing mutates bytes $M_{b} = \{b_1, b_2, ..., b_n\}$ to discover self-new edges, for a redundant byte $b_i$, we get $\mathcal{F}(M_b\backslash \{b_i\}) = \mathcal{F}(M_{b})$. This immediately derives that the value of the related $\varphi$ is zero. Therefore, we do not need to update Shapley values for redundant bytes.
For the necessary bytes that influence the result of self-new edges, denoted as $N_b$, exclusion of any byte $b_j$ in $N_b$ will not discover self-new edges, \ie $\mathcal{F}(N_b\backslash \{b_j\}) = 0$. 
% This lies in the fact that an input either examines the \textit{then}-branch or the \textit{else}-branch of a path constraint. 
Therefore, all necessary bytes in this mutation have the same value of $\varphi$, indicating that we can only calculate $\varphi$ for one necessary byte to update Shapley values for all necessary bytes. 
In fuzzing, when self-new edges are discovered, we recover mutations of bytes to check whether those bytes are redundant.
If the recovery of the mutation of a byte does not change the result of self-new edges, the byte is a redundant byte.


\subsubsection{Family Update}
The family for seeds can reduce the overhead of calculating Shapley values because Shapley values for one seed can be shared with multiple seeds.  
The key of building a family is that the mutation does not change the length of original seeds. Yet, some mutators, such as \textit{deletion of bytes}, in fuzzing will change the length of seeds. 
To enrich family members, \tool{} will withdraw all mutators that change length when new code are discovered.
If the result can still find the same new edges after withdrawing those mutators, \tool{} will retain the result of withdrawing to the family.
For example, as shown in Figure~\ref{fig:family_update}, we select a seed from family $N$ and mutate it. 
If an input $i_1$ discovers new edges, \tool{} will withdraw all mutators that change length, which generates another input $i_2$. If $i_2$ can still find the same new edges that $i_1$ finds, \tool{} retains $i_2$ as a new seed and adds it to the family $N$.
Otherwise, $i_1$ will form a new family $N+1$ if mutation of $i_1$ can further discover new edges.
As a result, \tool{} has a reasonable number of families and family members.


\begin{figure}[t!]
\includegraphics[width=\linewidth]{images/upate.png}
\caption{The update of family and family members.}
\label{fig:family_update}
\end{figure}



% with Contextual Multi-armed Bandit
\subsection{Shapley-guided Mutation}
\label{subsec:mutate}
% As mentioned in Section~\ref{subsec:trans_shap}, the importance of a byte is the same to the importance of its position for seeds. 
% % Thus, in the following, we mostly use \textit{position importance} to represent the contribution of a byte, \ie its Shapley value.
% Thus, in the following, we interchangeably use the terms of \textit{position importance}, \textit{byte importance}, and Shapley value.
The insight from Section~\ref{sec:motivation} indicates that more energy can be assigned to bytes with higher Shapley values. However, since the Shapley value is calculated based on part of all possible inputs during fuzzing, it cannot guarantee that the bytes with high Shapley values can always maintain high.
Besides, seeds share the byte importance with the original seed in the same family.   
Although a byte may have a high Shapley value, the difficulty of solving path constraints varies in different execution paths.
When some bytes are frequently selected but with no new edges discovered, we do not want to waste more energy on those bytes.
Therefore, while considering the frequency of executed paths, we need to balance the trade-off between 1) focusing on bytes with high Shapley values and 2) updating Shapley values for all bytes. 


To maximize code discovery, \tool{} uses Contextual Multi-armed Bandit (CMAB)~\cite{CMAB, linucb} to achieve the trade-off in using Shapley values.
% models the problem of using Shapley values as a Contextual Multi-armed Bandit (CMAB) problem. 
Based on the experience of playing arms, CMAB tries to maximize the rewards of playing multi-armed bandits, taking into account the personality of a player (\ie the context). The trade-off in CMAB is between 1) focusing on the arms with higher historical performance and 2) updating rewards for all arms. This exactly fits into our problem of selecting bytes based on Shapley values.


With Shapley values, \tool{} uses CMAB to build a probability distribution for selecting bytes.
% , and it prefers the positions that are more likely to discover new code. 
To build the probability distribution, CMAB calculates scores for each byte. The higher scores are assigned with higher probabilities. Given a seed $s$, the feature vector $f_{s}$ extracted from the corresponding execution path (\ie the context), and a byte $p$, the score of the byte is calculated as:
\begin{equation} \label{equ:score_cal}
Score(s,p) = E[\phi_{p}|f_{s}] + 0.5 U_{s,p},
\end{equation}
where $E[\phi_{p}|f_{s}]$ is the expected reward, $U_{s,p}$ is the upper confidence bound, and $\phi_{p}$ is the Shapley value of byte $p$. As mentioned, the same $\phi_p$ in different execution paths has different influence on discovering new code. Therefore, we use $f_s$ to represent the context of $\phi_{p}$, and $f_s$ is extracted based on its seed.
% \zhu{briefly explain how to get $f_s$, and what's the duty of it}
% \zkp{
% First, we find ten center seeds in the seed queue whose paths are as far as possible from each other.
% Then, for a seed $s$, we compute the cosine similarity between the path exercised by that seed and the paths exercised by ten center seeds to obtain a fixed dimensional vector $f_s$.
% }
% \zhu{todo: \textit{The key in our model is that each time the Shapley value of any byte is updated, we reset the dataset for all bytes and re-collect data}. As a result, the probability distribution of CMAB model is reset and rebuilt based on sole Shapley values. In other words, Shapley values dominate the distribution at the beginning. When Shapley values are not updated, the distribution will gradually be dominated by $E[\phi_{p}|f_{s}]$ and $U_{s,p}$. Therefore, our model achieves the trade-off in using Shapley values as aforementioned.}

To calculate $E[\phi_{p}|f_{s}]$ and $U_{s,p}$, byte $p$ needs to maintain a tuple $(D_{p}, R_{p})$, where $D_p$ is a matrix about all history feature vectors and $R_p$ is a vector about Shapley values. 
To update the tuple $(D_{p}, R_{p})$:
\begin{equation}
\begin{split}
    D_p & = D_p + f_sf^T_s \\
    R_p & = R_p + \phi_p f_s
\end{split}
\end{equation}


\textit{Expected Reward.} In our model, the expected reward can be calculated by:
\begin{equation} \label{equ:E_calculation}
E[\phi_{p}|f_{s}] = f_{s}^{T}\hat{\theta},
\end{equation}
where $\hat{\theta}$ is the best coefficient vector, and it can be estimated by applying ridge regression to the tuple $(D_{p}, R_{p})$:
\begin{equation} 
\hat{\theta} = (D_{p}^{T}D_{p} + I_{k})^{-1} D_{p}^{T} R_{p},
\end{equation}
where $I_{k}$ is a k-dimensional identity matrix, and $k$ is the dimension of the feature vector $f_s$.
% To fuzz more on low-frequent paths~\cite{aflfast}, $f_{s}^{T}\hat{\theta}$ reflects how frequently execution paths are exercised. \zhu{briefly explain how to get $f_s$.}
% Therefore, the expected reward considers both position importance and the frequency of exercising execution paths.


\textit{Upper Confidence Bound.}
The second part of the score is the upper confidence bound $U_{s,p}$, which can be calculated by~\cite{walsh2009exploring}:
\begin{equation} \label{equ:U_calculation}
U_{s,p} = \sqrt{f_{s}^{T} (D_{p}^{T}D_{p} + I_{d})^{-1} f_{s}}
\end{equation}
The more a byte is selected, the smaller its $U_{s,p}$ is. Thus, the $U_{s,p}$ intends to assign more energy to the bytes that have been less frequently selected, \ie the bytes with low Shapley values.
When bytes with high Shapley values are selected frequently, their scores will be decreased, as well the selection probability.
As a result, the score calculated by Equation~(\ref{equ:score_cal}) achieves the trade-off for Shapley-guided fuzzing.
% Note that, as soon as the position importance is updated, we empty the dataset maintained on each position and re-collect the data.


% \textit{Dataset Update.}
% To update the score of each position, we update data for the dataset $(D_p, R_p)$ after a mutation of a seed $s$.
% Since fuzzing has a high chance to mutate multiple positions simultaneously, the reward in $R_p$ is not for a single position but for multiple positions. Therefore, \tool{} assigns the average reward to each selected position. Given a position $p$, the reward $r_{s, p}$ in $R_p$ is calculated as:
% \begin{equation} \label{equ:Reward}
% r_{s, p} = \frac{sign()}{n}  \times \frac{1}{\omega} + \phi_p,
% \end{equation}
% \zhu{move $\phi_p$ here.}
% where $sign()$ is 1 when a mutation of bytes differs execution path from the seed $s$'s or otherwise 0, $n$ is the number of mutated positions in this mutation, and $\omega$ is the frequency of the path exercised by the mutated input. The frequency is calculated as $\omega = \frac{N_{path}}{N_{total}}$, where $N_{path}$ is the number of times the path has been exercised and $N_{total}$ is the total number of executions during fuzzing.
% Finally, the tuple $(f_{s}, r_{s,p})$ of position $p$ is added into the dataset $(D_p, R_p)$.


\subsection{Overall Algorithm}
\zhu{TODO: change the algorithm or remove?}
% Based on the above two characteristics, we propose our simplified Shapley Value calculation algorithm. The specific process is shown in the algorithm~\ref{alg:shapley}.

% \begin{algorithm}[h]
% \footnotesize
% \caption{Algorithm of Shapley-guided Fuzzing}\label{alg:shapley}
% \KwIn{
%     A mutation $M$,the mutated position sequence $M_{pos} = \{p_{1}, \ldots, p_{n}\}$ and a function $\mathcal{F}(*)$ mapping between mutated position sequence and self-new edges.
    
% }

% $SV[n] = {0}$\; 
% $totalEdges = \mathcal{F}(M_{pos})$\;
% $flag = 1$\;
% \For{$pos \in M_{pos}$}{
%     \If{$\mathcal{F}(M_{pos} \backslash \{pos\}) == totalEdges$}{
%         $M_{pos}.delete(pos)$\;
%     }
%     \lElseIf{$\mathcal{F}(M_{pos} \backslash \{pos\}) \neq 0$}{
%         $flag = 0$
%     }
% }
% \eIf{$flag$}{
%     $averageSV = simplifiedShapleyAnalysis(M_{pos}, \mathcal{F})$\;
%     \For{$i \in n$}{
%         $SV[i] = averageSV$\;
%     }
% }
% {
%     \For{$i \in n$}{
%         $SV[i] = shapleyAnalysis(M_{pos}, \mathcal{F})$\;
%     }
% }
% \end{algorithm}


% Based on the algorithm ~\ref{alg:shapley}, we can quantify the contribution of each position to CMP flipping in each mutation, that is, the Shapley Value.
% First, given the mutated position sequence $M_{pos}$, we initialize the Shapley Value of each position in $M_{pos}$, and record the number of self-new edges $totalEdges$ found by $M_{pos}$ (lines 1-2).
% Second, we cancel the mutation of each position one by one, and remove redundant positions to reduce the number of positions required for analysis (lines 4-6).
% Third, we analyze whether the mutation conforms to the 0-N case.
% Specifically, we analyze whether the discovery of self-new edges depends on the simultaneous mutation of all remaining positions. If other values other than 0 and $totalEdges$ are found when canceling the mutation of each position, it means that the 0-N case is not met (line 7).
% Finally, in the 0-N case, we consider all remaining positions to contribute equally to the self-new edges. Therefore, we directly use Equation~\ref{equ:shapelyFuzzing01} to calculate the Shapley Value of each position without analyzing the results of each subset (lines 8-11).
% If it does not meet the 0-1 situation, we will continue to use the formula ~\ref{equ:shapelyFuzzing} for detailed analysis (lines 12-14).



\subsection{Threats to Validity}

\tool{} models the process of byte mutation as a cooperative game and uses Shapley analysis to quantify the contribution of each byte.
Assume that self-new edges are found in a mutation, and the number of its mutated positions is $N$.
To calculate the Shapley value, we need to analyze the number of self-new edges found in $2^{N}$ subsets of mutated positions.
To reduce the overhead, \tool{} uses two special cases to simplify the process of Shapley analysis.
Firstly, if there are redundant bytes that do not influence the result of the self-new edge, we remove these bytes to reduce $N$.
Secondly, if the mutated bytes are necessary for the discovery of self-new edges, these bytes have the same Shapley value.
However, if these two conditions are not met and $N$ is large, some overhead will be introduced.
In the future, we can use some lightweight and improved algorithms of Shapley value to alleviate this problem.


Moreover, \tool{} builds a family system to alleviate the overhead brought by Shapley analysis. Within a family, all seeds in the same family share the same Shapley values for bytes.
However, when maintaining a family, we ignore mutated inputs that change length.
This is because the use of mutators that change seed length may disorders byte positions in seeds, and we cannot achieve position mapping between seeds.
We can study mathematical theory for the Shapley analysis of changeable length in the future.
In the existing version, if a new seed is generated by changing length, we use this seed to create a new family to alleviate this problem.




% Our \tool{} is proposed based on the results of Shapley experiments in Section~\ref{sec:motivation}, which is an empirical study. Thus, we are concerned about the generality of our claims. 
% However, we analyze the root causes of the Shapley results to support our claims.  
% These root causes are general observations of the nature of programs and independent from our empirical study.
% Even if our claim does not include all programs, we believe it satisfies the majority of modern programs.
% \zhu{TODO} 
% The second concern comes from the internal threat to validity, which is our solution to optimize byte mutation. 
% % Our solution formulate byte mutation for seeds in a family but not for all seeds. Therefore, the performance may not be the best outside a family. To 
% There is a conflict to use Shapley values to guide fuzzing. 
% On the one hand, Shapley values calculated during fuzzing is incomplete because the calculation does not use all possible inputs. The problem of incomplete Shapley values is that they cannot accurately reflect the importance of a byte. On the other hand, if the calculation is complete, all possible inputs have been generated. No more inputs can be generated to discover new code. 
% Fortunately, the root causes for Shapley results in Section~\ref{sec:motivation} allow the use of incomplete Shapley values. Even for positions that temporarily have high Shapley values, they still have the chance to be related to multiple (unseen) path constraints. Therefore, the incomplete Shapley values can still be utilized to guide fuzzing. Besides, we use CMAB to mitigate the problem of incomplete Shapley values. Our experiments in Section~\ref{sec:eval} also support that byte mutation guided by incomplete Shapley values is effective.

% Our solution is based on two assumptions. The first is that there are valuable positions for us to optimize. The second is that our family system can capture the structural information of target programs. 
% For the first assumption, we use the random mutation mode to obtain valuable positions.
% However, random mutations can only increase the number of valuable positions up to a limit.
% To solve this problem, we can use existing solutions that find constraint-related byte positions, such as GreyOne~\cite{greyone}, Angora~\cite{angora} and Driller~\cite{driller}. These solutions are efficient in finding positions related to a single path constraint, which is exactly what we want.
% For the second assumption, it is mainly used to share valuable positions among different seeds. This requires that valuable positions in different seeds are still related to path constraints.
% However, the family system can only roughly satisfy this requirement. 
% One solution to solve this is to analyze programs case by case. That is, we capture the structural information based on syntax analysis tools or even manually determine the constraint-related positions in different seeds.
% Yet, we believe such a solution limits the scalability of fuzzing, \ie it is only effective in specific programs.
% Although the family system cannot accurately capture structural information, CMAB refines the selection of valuable positions, which is scalable to fuzz programs.


==> sections/discussion.tex <==
\zkp{
\section{DISCUSSION AND LIMITATION}
While our approach has shown promising performance and effectiveness, there are still certain potential factors that could constrain the practical application of \tool{}.

\subsection{The Impact of Self-New Edges}
As new edge discovery becomes progressively more difficult over time, \tool{} utilizes self-new edges as a metric to measure gains and identify bytes that may impact multiple branches. Nevertheless, in some cases, bytes that contribute to the self-new edge may not necessarily lead to the discovery of extra new edges.
First, We consider "self-new edges" as intermediate waypoints between the "current seed" and "extra new edges". If we discover more self-new edges, it implies that our exploration of seed mutations has reached a broader code space, thus increasing the probability of finding extra new edges in the future. Then, we decrease the influence of it by using CMAB. Based on the idea of intermediate waypoints, if the bytes with high Shapley values can discover more self-new edges, the discovered more self-new edges might contain new edges. If they cannot (no self-new edges means no new edges), CMAB will decrease the scores of those bytes, which decreases the influence of ineffective self-new edges.

\subsection{Semantics Consistency in Families}
To reduce the overhead of calculating Shapley values, the seeds in a family share the same Shapley values. However, despite implementing a strict family construction method (seeds with genetic relationships and same lengths), there may still be cases where the semantics between seeds are inconsistent.
We use CMAB in Shapley-guided byte selection to identify inefficient bytes, which can mitigate this problem.
In Equation~\ref{equ:score_cal}, $E[\phi_{p}|f_{s}]$ represents the Shapley Value that byte $p$ may potentially acquire in the future and favors the selection of high Shapley value bytes. $U_{s,p}$ represents the upper confidence bound, which decreases as a byte is selected more frequently. If we choose to mutate byte $p$ and its Shapley value does not increase during this process, the score calculated will gradually decrease.

}


